OneAdapt: Fast Configuration Adaptation for Video Analytics Applications via Backpropagation

Deep learning inference on streaming media data, such as object detection in video or LiDAR feeds and text extraction from audio waves, is now ubiquitous. To achieve high inference accuracy, these applications typically require significant network bandwidth to gather high-fidelity data and extensive GPU resources to run deep neural networks (DNNs). While the high demand for network bandwidth and GPU resources could be substantially reduced by optimally adapting the configuration knobs, such as video resolution and frame rate, current adaptation techniques fail to meet three requirements simultaneously: adapt configurations (i) with minimum extra GPU or bandwidth overhead; (ii) to reach near-optimal decisions based on how the data affects the final DNN's accuracy, and (iii) do so for a range of configuration knobs. This paper presents OneAdapt, which meets these requirements by leveraging a gradient-ascent strategy to adapt configuration knobs. The key idea is to embrace DNNs' differentiability to quickly estimate the accuracy's gradient to each configuration knob, called AccGrad. Specifically, OneAdapt estimates AccGrad by multiplying two gradients: InputGrad (i.e. how each configuration knob affects the input to the DNN) and DNNGrad (i.e. how the DNN input affects the DNN inference output). We evaluate OneAdapt across five types of configurations, four analytic tasks, and five types of input data. Compared to state-of-the-art adaptation schemes, OneAdapt cuts bandwidth usage and GPU usage by 15-59% while maintaining comparable accuracy or improves accuracy by 1-5% while using equal or fewer resources.

==> control.tex <==
%!TEX root = main.tex
%!TEX spellcheck = en_US 


\tightsection{\name protocol design}


% This section formally describes \name's core streaming control algorithm (\S\ref{subsec:formalizing},\ref{subsec:feedback}), how \name adapts its bitrate to handle bandwidth fluctuation (\S\ref{subsec:adaptation}).
% , and
% several \name refinements that lead to significant improvement in practice (\S\ref{subsec:optimization}).




\vspace{0.4cm}

\tightsubsection{General workflow of \name}

\name first chop video stream to {\em chunks} (as in \cite{awstream,dash}). For each chunk, the camera first encodes it at low quality level and sends the resulting video to the server through stream A. Then, the  server-side DNN will run inference on that video chunk. After that, \name extrapolates the \ambiguous regions and send those regions back with the inference results. Upon arrival, the camera re-encodes those \ambiguous regions with high quality and send them back to the server through stream B. The server then perform for a second iteration inference and update the inference results to the camera.


% \tightsubsection{Formalizing \name control logic}
% \label{subsec:formalizing}


% % \mypara{Terminology}
% %\mypara{Frames and regions}
% We start with a general framework of \name's control logic. 
% A video stream is chopped to {\em segments}\footnote{The concept of segments is equivalent to video chunks used in the DASH protocols~\cite{dash} and AWStream~\cite{awstream}.} (each contains a set of $n$ consecutive frames), and \name operates on a segment-by-segment basis. 
% %Each segment contains a set of $n$ consecutive video frames;
% %\eg if the video is 30fps and $n=30$, each segment represent one-second worth of video\footnote{The concept of segments is equivalent to video chunks used in the DASH protocols~\cite{dash} and AWStream~\cite{awstream}.}.
% In each frame, one can ``spatially sample'' one or more regions (a region is a bounding box) and together they form a {\em region set}.
% %can be spatially sampled with one or more regions, and these regions sampled forms a {\em region set}. 
% We use $\Seg$ to denote a segment, $\Regions$ a region set, and $\Video_{\Seg,\Regions,\Level}$ the video generated from a region set $\Regions$ of segment $\Seg$ encoded in quality level $\Level$, which specifies the resolution and qp (quantization parameters).
% Two special types of regions are particularly useful. 
% First, a region covering the full frame can form a region set, labeled $\Regions_{\Full}$, so $\Video_{\Seg,\Regions_{\Full},\Level}$ denotes the entire segment encoded in quality level $\Level$ (\ie without any spatial sampling).
% Second, a frame can have an empty region set which effectively means it is skipped.

% %
% %There are two special types of region sets: 
% %(1) When each region covers the full area of a frame, the region set is referred by $\Regions_{\Full}$, and $\Video_{\Seg,\Regions_{\Full},\Level}$ denotes the entire segment encoded in quality level $\Level$ without any spatial sampling.
% %(2) These regions may not be aligned across frames, so one can also skip a frame by assigning an empty region in the frame. 



% %
% %\SetKwFunction{KwFn}{Fn}
% %\SetArgSty{textrm}
% %\begin{algorithm}[t!]
% %{\small
% %\DontPrintSemicolon
% %\KwIn{Segment $\Seg$, and the DNN-generated region proposal $\Regions_{\Srv}$ and detection results $\Detections_{\Srv}$ (only detections with confidence score over $\alpha$) on the low-quality video of $\Seg$.
% %DNN confidence score threshold $\alpha$, maximum IoU $\beta$ between a proposed region and a detected bounding box, maximum area of a feedback region $\gamma$.}
% %\KwOut{Feedback region set $\Regions_{\Feedback}$ (which the camera then send again in higher quality level $\Level_{\High}$)% and first-iteration detection results $\Detections_{\First}$
% %}
% %%\tcc{\footnotesize Get DNN's region proposal and detection results}
% %%$\Regions_{\Srv}, \Detections_{\Srv}\leftarrow DNN(\Video_{\Seg,\Regions_{\Full}, \Level_{\Low}})$\\
% %\SetKwFunction{FFeedback}{create\_feedback}
% %\SetKwProg{Fn}{Function}{:}{}
% %\Fn{\FFeedback{$\Seg,\Regions_{\Srv},\Detections_{\Srv}$}}{
% %\tcc{\footnotesize Initialize feedback region set}
% %$\Regions_{\Feedback}\leftarrow\emptyset$\\%,\Detections_{\First}\leftarrow\emptyset$\\
% %\For{$\textrm{frame $\Frame$ in }\Seg$}{
% %	\For{$\textrm{region }r\in \Regions_{\Srv}\cap\Frame$}{
% %		$keep\leftarrow True$\\
% %		\For{$\textrm{box }b\in \Detections_{\Srv}\cap\Frame$}{
% %			\If{$IoU(r,b)>\beta$ or $r_{confidence}>\alpha$}{
% %				\tcc{\footnotesize Skip if it overlaps with an already detected object}
% %				$keep\leftarrow False$; \textrm{break}
% %			}
% %		}
% %		\If{$r.\textrm{area} > \gamma$}{
% %			$keep\leftarrow False$\tcc{\footnotesize Skip large regions}
% %		}
% %		\If{\textrm{keep}}{
% %			$\Regions_{\Feedback}\leftarrow\Regions_{\Feedback}\cup\{r\}$
% %		}
% %	}
% %}
% %\Return{$\Regions_{\Feedback}$}
% %}
% %% $(n,0,\dots,0)\rightarrow$\\
% %% \tcc{Find the best decisions and QoE under}    
% %\tightcaption{\name logic to choose feedback regions.}
% %\label{alg:feedback}
% %}
% %\vspace{0.5cm}
% %\end{algorithm}







% %\mypara{Iterative process}
% \name's iterative protocol (\S\ref{sec:overview}) can now be formalized as follows. 
% For each segment $\Seg$, the camera first encodes it at low quality level $\Level_{\Low}$ and sends the resulting video $\Video_{\Seg,\Regions_{\Full}, \Level_{\Low}}$ to the server (Stream A). 
% Then, the server-side DNN runs inference on the video and returns the {\em high-confidence inference output} $\Detections_{\Srv}$ (the part of DNN output that already has high confidence with low-quality video), as well as the {\em proposed region set} $\Regions_{\Srv}$ (regions deemed as likely to contain inference).
% The high-confidence inference output and the set of proposed regions are then combined to generate the feedback region set, denoted by $\Regions_{\Feedback}$.
% %but without sufficient confidence to get full results yet (we will explain how to do it next). 
% The feedback region set will then be sent back as feedback to the camera, which then encodes these regions at higher quality level $\Level_{\High}$ and sends the resulting video $\Video_{\Seg,\Regions_{\Feedback}, \Level_{\High}}$ to the server for a second iteration inference (Stream B).

% %Next, we explain how the proposed region set $\Regions_{\Srv}$ and high-confidence inference output $\Detections_{\Srv}$ are extracted from DNN output and how they generate feedback region set $\Regions_{\Feedback}$.

% % \hh{Do we need to mention anything about why we stop at two rounds?  If we think confidence is key, we could either keep going until we have high confidence in everything or we cannot get higher quality video.  Should we say something like, "while it might be possible to keep iterating beyond two round of inference we found no practical benefit to this approach"?}




\tightsubsection{\cameranew{General logic on extracting \ambiguous regions}}
\label{subsec:feedback}



%\mypara{Proposed region set and high-confidence inference output}
\cameraold{We first introduce how the proposed region set $\Regions_{\Srv}$ and high-confidence inference output $\Detections_{\Srv}$ are extracted from DNN output for various vision tasks (\eg object detection, face recognition, and semantic segmentation).
It is important that their definitions are agnostic to the exact vision tasks and the DNNs.
This means the generation of feedback regions is independent to the particular vision task and DNN.
}

\cameranew{
We first introduce the input and output of our \ambiguous region extraction algorithm. It is important that their definitions are agnostic to the exact vision tasks and the DNNs.
This means the generation of our \ambiguous regions is independent to the particular vision task and DNN.
}



\cameraold{
\myparashort{High-confidence inference output  $\Detections_{\Srv}$,} in object detection (face recognition or semantic segmentation), is a list of DNN-returned elements (labeled bounding boxes in object detection, faces in face recognition, or pixels in semantic segmentation), each associated with its coordinates and confidence score.
We use the elements that have confidence score over a threshold, which suggests they are ready to be reported.

%can be the subset of DNN-returned labeled bounding boxes (faces or pixels), each associated with its coordinates and confidence score.
%The elements (boxes, faces, or pixels) are those whose classification confidence score is over a threshold, which suggests they are ready to be reported.



%\myparashort{Proposed region set $\Regions_{\Srv}$} includes the regions (typically boxes\ktedit{, which can be efficiently encoded by current codec}) that have high {\em objectness} scores---likelihood to be part of object of {\em any} class of interest. \ktedit{For high, we mean that the object score is greater then a threshold $\theta$ (0.5 by default).}

\myparashort{\cameraold{Proposed region set} \cameranew{High objectness score results} $\Regions_{\Srv}$} includes the regions (we use rectangle-shape boxes for encoding efficiency) that have high {\em objectness} scores---likelihood to be part of object of {\em any} class of interest. 
%\ktedit{For high, we mean that the object score is greater then a threshold $\theta$ (0.5 by default).}
The objectness scores of proposed regions can be obtained in two ways. 
First, they can be directly obtained from the RPN results, if the inference pipeline is based on RPN (\eg FastRCNN, FasterRCNN, MTCNN, or MaskRCNN~\cite{maskrcnn}) which explicitly proposes regions and evaluates their objectness scores.
Second, they can be obtained from the DNN's inference output.
For instance, Yolo~\cite{yolo} assigns each potential region a list of per-class confidence scores, and the scores of various classes can be summed up to get the objectness score per region\footnote{We acknowledge that the sum of confidence scores across all classes does not directly translate to the likelihood of a region being in any of the classes. That said, we have empirically found it a good indicator of objectness.}.
Another example is that pixel-level inference output can be similarly used to derive objectness scores of regions. 
In semantic segmentation output, each pixel will be assigned with a per-class confidence score. For each region (\name uses 64x64 blocks), we can calculate its objectness score by summing up the confidence scores across all pixels and all classes.
}




\cameranew{
\mypara{Input} The input is two sets: high-confidence results $\Detections_{\Srv}$ and high-objectness-score results $\Regions_{\Srv}$. 
Both of them are a list of elements extracted from DNN, each associated with its coordinates and score.
An element can be a labeled bounding box in bounding-box-based application (like object detection and face recognition), or a pixel in pixel-based application (like semantic segmentation). The high-confidence results are those inference results that have confidence score over a threshold. We will talk about the specific technique to generate high-objectness-score results $\Regions_{\Srv}$ later.

\mypara{Output}
The output is \ambiguous regions. It contains several rectangle-shaped bounding boxes (we will illustrate the rationale later). 
Fig. ~\ref{fig:input-output} shows the input and the output of our \ambiguous region extraction algorithm.
}



% \ktedit{The regions and their corresponding scores can either be directly obtained by RPN (\eg FastRCNN, FasterRCNN, MTCNN), or by exploring the raw output from server-side neural network. Take Yolo (a face recognition network) as an example. Yolo assign each potential region a list of per-class confidence scores. We then sum up through this list and obtain the objectness score. Another example are semantic segmentation networks. These networks will assign each pixel a background probability and several per-class probabilities. Thus, by clamping these probabilities, we obtain the object score (and also the background score) for this pixel. To leverage the codec, we group these pixels to 64x64 blocks. }

% The objectness score per region can be directly obtained if the inference pipeline is based on RPN (\eg FastRCNN, FasterRCNN, MTCNN) which explicitly proposes regions and evaluate their objectness scores. \ktedit{\name accept those regions with confidence scores larger than a threshold $\theta$ (0.5, by default).} 
% For instance, Yolo \ktedit{(a face recognition network)} assigns each potential region \ktedit{remove this? (hundreds of them in total)} a list of per-class confidence scores and we then calculate the objectness score per region by adding up the confidence scores of all classes (\ie the likelihood of the region containing any object of interest) and propose the regions whose objectness scores exceed a threshold.
% Finally, for pixel-level inference (\eg semantic segmentation), each pixel will have a confidence score, and \name enumerates all 64x64 blocks (squares can be encoded efficiently by standard codecs) and in each region and calculates the objectness scores by summing up all per-pixel confidence scores.




\cameraold{

\SetKwFunction{KwFn}{Fn}
\SetArgSty{textrm}
\begin{algorithm}[t!]
{\small
\DontPrintSemicolon
\KwIn{The DNN-generated \cameraold{region proposal} \cameranew{high-objectness-score set} $\Regions_{\Srv}$ and detection results $\Detections_{\Srv}$ on the low-quality video.
%DNN confidence score threshold $\alpha$, maximum IoU $\beta$ between a proposed region and a detected bounding box, maximum area of a feedback region $\gamma$.
}
\KwOut{\cameranew{\Ambiguous element set} $\Regions_{\Feedback}$ \cameraold{(which the camera then sends again in higher quality level $\Level_{\High}$)}% and first-iteration detection results $\Detections_{\First}$
}
%\tcc{\footnotesize Get DNN's region proposal and detection results}
%$\Regions_{\Srv}, \Detections_{\Srv}\leftarrow DNN(\Video_{\Seg,\Regions_{\Full}, \Level_{\Low}})$\\
\SetKwFunction{FFeedback}{create\_feedback\_per\_frame}
\SetKwProg{Fn}{Function}{:}{}
\Fn{\FFeedback{$\Regions_{\Srv},\Detections_{\Srv}$}}{
\tcc{\scriptsize Initialize \cameraold{feedback region} \cameranew{\ambiguous element}  set}
$\Regions_{\Feedback}\leftarrow\emptyset$\\%,\Detections_{\First}\leftarrow\emptyset$\\
\For{$\textrm{region }r\in \Regions_{\Srv}$}{
	$keep\leftarrow True$\\
	\tcc{\scriptsize Skip large regions}
	\If{$r.\textrm{area} > \gamma$}{
		$keep\leftarrow False$
	}
	\tcc{\scriptsize Skip if it overlaps with high-confidence inference result}
	\For{$b\in \Detections_{\Srv}$}{
		\If{$r$ and $b$ overlap}{
			$keep\leftarrow False$; \textrm{break}
		}
	}
	\tcc{\scriptsize Skip low objectness sore regions}
	\If{$r.\textrm{objectness} < \theta$} {
	    $keep \leftarrow False$
	}
	\If{$keep$}{
		$\Regions_{\Feedback}\leftarrow\Regions_{\Feedback}\cup\{r\}$
	}
}

\Return{$\Regions_{\Feedback}$}
}
% $(n,0,\dots,0)\rightarrow$\\
% \tcc{Find the best decisions and QoE under}    
\tightcaption{\name logic to select \cameraold{feedback regions}\cameranew{\ambiguous elements}}
\label{alg:feedback}
}
\vspace{0.5cm}
\end{algorithm}
}





\cameraold{\mypara{Selecting feedback regions}}
\cameranew{\mypara{General logic}}
%how to generate feedback region set $\Regions_{\Feedback}$. %is generated by combining $\Regions_{\Srv}$ and  $\Detections_{\Srv}$.
% At a high level, \name selects the regions proposed by the DNN for which the DNN does not confidently detect any object. 
% Specifically, g
%Given the low quality video stream $\Video_{\Seg,\Regions_{\Full}, \Level_{\Low}}$, DNN will return two results:
%{\em DNN region proposal}, $\Regions_{\Srv}$, which is a region set over segment $\Seg$, and
%{\em DNN inference results}, $\Detections_{\Srv}$ (\eg in object detection, $\Detections_{\Srv}$ is a set of labeled bounding boxes).
% They are combined with the following logic to produce the feedback region set $\Regions_{\Feedback}$.
\cameranew{
First, \name generates \ambiguous {\bf elements} from high-objectness-score results $\Regions_{\Srv}$ that meets three criteria:}
\cameraold{
As described in Algorithm~\ref{alg:feedback}, \name picks from $\Regions_{\Srv}$ the feedback regions that meet two criteria:}
%and add it to the feedback region set $\Regions_{\Feedback}$, if it meets two criteria: 
%whose confidence score is over $\alpha$ and 
%the IoU (intersection-over-union) between the region and the bounding box is over $\beta$, and
(a) each feedback region (in terms of the fraction of the whole frame) is less than a threshold $\gamma$ (by default, 4\%\footnote{Although 4\% of the whole frame size looks low, it actual is quite high (roughly the size of a truck in a distance of 70ft from the camera).});
(b) each feedback region does not overlap significantly with any high-confident inference output $\Detections_{\Srv}$,\footnote{In object detection, a proposed region does not overlap with a detected region if their IoU (intersection-over-union) is below a predetermined threshold (0.3, by default).
In semantic segmentation, two elements overlaps only when they are the same pixel.}; and
(c) the objectness score of a region is over a threshold $\theta$; 
%Intuitively, these criteria are designed to filter out types of DNN-proposed regions. 
%First, either very unlikely to contain real objects or contain object but are already detected in the low-quality video segment.
The rationale behind them is as follow.
\cameraold{
(a) filters out the regions that the DNN is already confident based on the low-quality video.
(b) filters out large proposed regions, because if it does contain an object, it should have been detected by the DNN with high confidence already.
Finally, (c) uses a threshold of objectness score (by default 0.5) as a control knob to adjust the bandwidth demand of the second round (Stream B).
}
\cameranew{(a) filters out large regions, because if it does contain an object, it should have been detected by the DNN already \footnote{\cameranew{Large objects are usually much easier for the model to detect than small objects. This is because large objects are at higher resolution (thus revealing more details), and occupy more pixels (thus activating more neurons). So if large objects cannot be correctly detected, the streaming quality is too low to provide reasonable feedback.
}.}.
(b) filters out the regions that the DNN is already confident based on the low-quality video.
Finally, (c) uses a threshold of objectness score (by default 0.5) as a control knob to adjust the bandwidth demand of the second round (Stream B).

After generating \ambiguous elements, \name then use application-specific algorithm to group \ambiguous {\bf elements} to \ambiguous {\bf regions}.
}

\begin{figure}[t!]
    \centering
    \subfloat[Bounding-box-based application (Object detection)]
    {
        \includegraphics[width=0.49\columnwidth]{figs/bbox-app.pdf}
        \label{fig:bbox-app}
    }
    \subfloat[Pixel-based application (Semantic segmentation)]
    {
        \includegraphics[width=0.49\columnwidth]{figs/pixel-app.pdf}
        \label{fig:pixel-app}
    }
    
    \tightcaption{Illustration on the input and the output of the \ambiguous region extraction algorithm of \name on two types of applications.}
    \label{fig:input-output}
\end{figure}

% \begin{figure}
% \centering
% \includegraphics[width=0.99\columnwidth]{figs/ambiguity-illustrated.pdf}
% \tightcaption{Ambiguous elements lies in the gap between high-confidence results and high-objectness-score results.}
% \label{fig:ambiguity-illustrated}
% \end{figure}



% \begin{figure}
% \centering
%\includegraphics[width=0.85\columnwidth]{figs/example-feedback.pdf}
% \hspace*{-1cm}
% \includegraphics[width=1.1\columnwidth]{figs/example-feedback-new.pdf}
% \tightcaption{
% \cameraold{Illustrative example of \name's logic to choose feedback region set (Algorithm~\ref{alg:feedback}) from region proposal and detected result returned by the server-side DNN} 
% \cameranew{Illustration of our general logic on ambiguous elements generation from high-objectness-score results and high-confidence results. Need to update this figure for consistant naming.}   \vspace{-0.2cm}
% %\jc{replace it with a real example}
% }
% \label{fig:demonstrate-algorithm}
% \end{figure}

% \mypara{Illustrative example}


\cameraold{
Figure~\ref{fig:example-feedback} shows an example of Algorithm~\ref{alg:feedback} in action (on a single frame). 
The region proposal $\Regions_{\Srv}$ and inference result $\Detections_{\Srv}$ are produced by running FasterRCNN-ResNet101, a typical object detection model, on one frame from one of the traffic video; we get $\Regions_{\Srv}$ the FasterRCNN output (after the built-in non-maximum suppression removes duplicated bounding boxes).
The example shows that, among the nine DNN-proposed regions, one is too large and four overlap substantially with detected bounding boxes, so the feedback region set contains four regions. 
}

%\jc{Kuntai: list all parameters used by object dtection and segmentation DDS, their definitions and whether they were used}
%\kt{Should we add a table that illustrates: 1. the symbol of each hyper-parameters 2. the default value of them 3. whether they appears in sensitivity test?}




\cameranew{

\tightsubsection{Applying the logic in various vision tasks}
\label{subsec:apps}

In the general logic, there are two critical parts that are application specific. One is how to generate high-objectness-score results, the other is why and how we group \ambiguous elements to \ambiguous regions. We will answer them below.

\mypara{Generate high-objectness-score results}
We exploit the rich intermediate output produced from DNNs of various applications to generate high-objectness-score results.
\begin{packeditemize}
\item{\bf Bounding-box-based inference:}
For bounding-box-based inference (\eg object detection, face recognition), our observation is that: most of the DNNs explicitly propose regions to anchor the objects and evaluate their objectness scores \footnote{As for the network that assign the classification score of multi-classes for each region (like YoLo), we instead use the sum of all non-background scores. We acknowledge that the sum of confidence scores does not directly translate to the likelihood of a region being in any of the classes. That said, we have empirically found it a good indicator of objectness.\label{fn:objectness}}). Thus, we could generate the high-objectness-score results $\Regions_{\Srv}$ naturally.


\item{\bf Pixel-based inference:}
For pixel-based inference (\eg semantic segmentation), the high-objectness-score results are a collection of pixels with corresponding objectness score. We can obtain the objectness score for each pixel in the same way we extract objectness scores in YoLo. 

\end{packeditemize}

\mypara{Group \ambiguous elements to \ambiguous regions}
To save bandwidth, it is inevitable to leverage modern video codec (there might be even 8x penalty in bandwidth if not as shown in Fig. \ref{fig:eval-contrib-codec})).

However, in bounding-box-based applications, the \ambiguous elements may significantly overlap, resulting in irregular boundary; in pixel-based applications, the \ambiguous elements mainly lie in the both small objects and the boundary of large objects, resulting in irregular shape.
Both of them are not friendly to modern video codec.
Consequently, we want to {\bf group} \ambiguous {\bf elements} to rectangle-shaped \ambiguous {\bf regions} to make our content {\bf codec-friendly}. 
The specific techniques are:
\begin{packeditemize}
\item{\bf Bounding-box-based inference:}
The \ambiguous elements here are a set of bounding boxes with corresponding objectness score.
We eliminate duplicated bounding boxes (i.e. bounding boxes that overlaps significantly with each other) inside \ambiguous elements through replacing them by the minimum rectangle that covers them to obtain final \ambiguous regions.
Figure~\ref{fig:bbox-app} demonstrates the final input and the output of \ambiguous region extraction on object detection.

\item{\bf Pixel-based inference:}
The \ambiguous elements in pixel-based application are a set of pixels with corresponding objectness score. 
We select several $k\times k$ (by default, $k=64$) rectangle-shaped bounding boxes by repeatedly choosing the rectangle with maximum objectness scores (the objectness score of a rectangle is the sum of the objectness score of all pixels inside), and zero out the objectness score of pixels inside. 
We repeat this process until the average objectness score of current region is too small, or until all the proposed regions contains $4\%$ pixels of the whole frame. 
These rectangles will be the final \ambiguous regions.
Figure \ref{fig:pixel-app} demonstrates the final input and the output of \ambiguous region extraction on segmentation.
\end{packeditemize}

\cameranew{
\mypara{Encode \ambiguous regions efficiently} To encode \ambiguous regions yields from various applications, at stream B, we will first send the \ambiguous regions from the server to the camera. For each frame that are mentioned in the \ambiguous regions, the camera then {\bf black out} all the pixels that does not belongs to \ambiguous regions. After that, the camera encode those frames to a mp4 video through the video codec and send them back to the server.

\mypara{Why it is efficient} Compared to directly encoding \ambiguous regions as separate images, our approach efficiently leverages two core algorithms in modern video codec: motion estimation and entropy encoding. As \ambiguous regions will contain some similar objects, the motion estimation algorithm could effectively detect and leverage this similarity to save bandwidth. Moreover, as the regions that we blacked out shares the same RGB value (0,0,0), they will be transformed to a similar binary string. The entropy encoder will discover this and pick a very short string to represent all of them. Thus, the black regions will only consume little bandwidth. We will demonstrate experimental results on this in Fig. \ref{fig:eval-contrib-codec}.
}

}





\tightsubsection{Handling bandwidth variation}
\label{subsec:adaptation}





% \name faces an additional challenge: because its control logic is content-dependent, even if the available bandwidth is fixed \name might need to adapt to ensure bandwidth limits are respected as content requires more regions to be sent back to the server.  

%At a high level, \name can dynamically increase/reduce its bandwidth demand within the aforementioned control logic framework, by varying its parameters (knobs).

Like other video streaming protocols, \name must adapt its bandwidth usage to handle bandwidth fluctuation. 
There are three control knobs: the low quality level and the high quality level, and the region proposal objectness threshold $\theta$.
We empirically find that these knobs affect the bandwidth/accuracy tradeoff in a similar way (\ie on the same Pareto boundary; \S\ref{subsec:sensitivity}), so \name only tunes low quality level and high quality level, while fixing the objectness threshold at 0.5.

%Other parameters, such as DNN confidence threshold $\alpha$, \ktedit{region proposal confidence threshold $\theta$}, IoU threshold $\beta$, and maximum proposed region area $\gamma$ will affect how many regions are requested in the second iteration, but we found changing these parameters has only minor effect, in part because the total areas of objects are often relatively small.
% The last three parameters control how many regions in $\Regions_{\Srv}$ should be kept in $\Regions_{\Feedback}$.
% Rather than alter the number of regions sent back (which would prevent detections in regions that were not sent) we choose to dynamically tune the low and high quality parameters.  This choice means that all objects are---in principle---detectable regardless of available bandwidth, although the probability of detection will decrease with decreasing quality.



To tune the low and high quality regions we implement a feedback control system, illustrated in Figure~\ref{fig:feedback-control}.  We base this controller on prior work that proposes a virtual, adaptive control system that can be customized for specific deployments \cite{CALOREE,FAST}. Instantiating the controller requires specifying three things: a bandwidth constraint to be met, feedback for monitoring bandwidth usage, and the tunable parameters that affect the bandwidth.  For \name, the bandwidth constraint is the estimated bandwidth for the next segment (labelled (1) in the figure), the feedback is the total bandwidth (for both low and high quality) from the last segment (2), and the tunable parameters are the resolution and quantization parameters of both the low and high quality (3).
% The controller consists of the content estimator, controller, and optimizer which are automatically customized when we specify the above three inputs (goal, feedback, and parameters).  
The controller continually estimates the \emph{base} behavior---in this case, the last segment's bandwidth if the default parameter settings had been used.  The controller then takes this base behavior as well as the difference between the desired bandwidth for the next segment and the achieved bandwidth for the previous segment and computes a scaling factor for the base bandwidth.  This scaling factor is passed to an optimizer which finds the low and high quality settings that deliver the scaled bandwidth while maximizing F1 score.  


\begin{figure}
\centering
\includegraphics[width=1.0\columnwidth]{figs/DDSControl.pdf}
\tightcaption{\name's adaptive feedback control system dynamically tunes the low and high quality configurations based on the difference between the estimated available bandwidth for the next segment and that used for the previous segment.}
\label{fig:feedback-control}
\end{figure}


%Figure~\ref{??} illustrates the feedback-based control loop to adapt to bandwidth variation.
%\jc{Hank/Ahsan, could you write a paragraph about the control loop}


%We would like to highlight that this controller works under a critical assumptions: the areas of the feedback regions are relatively stable, which makes the bandwidth demand of the same knob setting predictable. 
%Our evaluation result in \S\ref{subsec:eval-adaptation} empirically shows this assumption is reasonable. 
%It is important that this does not mean the feedback regions are predictable; rather, the feedback regions can vary significantly over a short period of time (which is also why \name can compress video more efficiently than prior work that must compress whole frames).
%The above assumption only requires their total areas to be relatively stable. 
%For instance, in a highway video (\eg Figure~\ref{fig:example-feedback}), the exact locations of the vehicles may change, but the total area of the feedback regions around the vehicles can be relatively stable as long as the number of cars in the video does not change significantly. 


%Moreover, if the assumption holds, the controller enjoys provides several useful formal properties. \
Our dynamic adaptation has several useful formal properties based on its use of feedback control.
% First, the content estimator handles non-linearities in the relationship between the parameters and bandwidth.  Intuitively, we can think of the parameter-bandwidth relationship as a curve and the content estimator as drawing a tangent to that curve.
% The controller then uses that tangent as a linear approximation to the true behavior \cite{ICSE2014}. 
\cameranew{First, the content estimator handles dynamic changes in operating conditions which change the relationship between the parameters and bandwidth. The adaptation mechanism uses a Kalman Filter to continually estimate the \emph{base} bandwidth. Hence, when the video content changes, the control model is updated in the following iteration, allowing \name to capture unmodeled non-linearities in the relationship between quality settings and bandwidth. Intuitively, we can think of the relationship between bandwidth and quality parameters as a curve and the base bandwidth (estimated by the Kalman filter) as a tangent to that curve. When adjusting the quality parameters, the \name controller uses this tangent as a linear approximation to the true behavior. This adjustment technique provides robustness in the face of shifts and variations in the system including when there does not exist a single model that captures all dynamics of the system \cite{ICSE2014}.}
The achieved bandwidth, then, will converge to the desired bandwidth in time proportional to the logarithm of the error in this estimation \cite{CALOREE}.    
Second, the optimizer finds the highest quality given the bandwidth specified by the controller.  This optimality is achieved by scheduling configurations over multiple segments.  As the system has a small, constant number of constraints (simply respecting the bandwidth requirement), an optimal solution can be found in constant time. \cite{Kim2015}. 



\tightsection{Implementation}
\label{sec:impl}

% Here, we describe the changes needed to deploy \name over a video client and DNN server.
We implement \name with about 2K lines of code, mostly in Python and the code is available and will be updated in~\cite{dds-code-repo}.

\tightsubsection{\name Interface}
\label{subsec:interface}


\name sits between the low-level functions (video codec and DNN inference) and the high-level applications (\eg object query or face recognition).
% As illustrated in Figure~\ref{fig:apis}, 
It provides ``south-bound'' APIs and ``north-bound'' APIs, both making minimum assumptions about the exact implementation of the low-level and high-level functions.

South-bound APIs interact with the video codec and DNN. 
Our implementation only uses the APIs already exposed by the x264 MPEG video, such as \texttt{x264\_encoder\_encode}\cite{x264}. 
From DNN, \name implements two functions: 
(1) region proposals ($\Regions_{\Srv}$), each with a specified location; and 
(2) detection results ($\Detections_{\Srv}$) including the detected objects/identities each with a specified location and a detection confidence score.

North-bound APIs implement the same analyst-facing (north-bound) APIs as the DNNs (\name can simply forward any function call to DNNs), so the high-level applications (\eg~\cite{optasia,deeplens-sanjay}) do not need to change and \name can be deployed transparently to analysts.
The only assumption is that, because \name runs the DNN twice on the same video segment, the two DNN detection results must be merged into a single detection result; we did this in a similar way as how DNNs internally to merge redundant results (\eg~\cite{tu2012fuzzy}).

% \begin{figure}
% \centering
% \includegraphics[width=1.0\columnwidth]{figs/apis.pdf}
% \tightcaption{\name sits between applications and DNN/video codec, and exposes north-bound and south-bound APIs.}
% \label{fig:apis}
% \end{figure}



% \tightsubsection{Interfaces}
% \label{subsec:interfaces}

% \cameranew{
% \mypara{Camera requirements of \name}
% Our camera-side requirements are:
% \begin{packeditemize}
%     \item Buffer several images after sent.
%     \item Put rectangle-shaped image on a black background.
%     \item Encode with parameter given from \name.
%     \item Stream the video to the server.
%     \item Concatenate analytic results.
% \end{packeditemize}
% The first two requirements are introduced to re-encode \ambiguous regions in high quality. The third and forth requirements are the normal camera requirements.
% We require the camera to concatenate analytic results in order to reduce the response delay of \name. We will introduce corresponding technique below.
% }

\tightsubsection{Performance optimization}
\label{subsec:optimization}


\cameraold{\mypara{Saving bandwidth by leveraging codec}
% \tightsubsection{Reducing bandwidth needs by video codec}
% \label{subsec:reduce-bw}
A naive implementation of Stream B would encode each region as separate images where the requested regions have high quality and the rest of the frames have low quality. %\ap{I replaced resolution with quality to (1) keep the terminology consistent (2) incorporate same resolution but lower qp cases as well}
But the total size of these images would be much greater than the original video segment in even the higher quality level without cropping the regions!
%\ap{not clear what "similar quality" is, we talk about two different qualities in the previous sentence. Also, I think maybe we can change the structure of this paragraph a little?}
The reason is that video codecs (\eg H.264/H.265), after decades of optimization, are very effective in exploiting spatial redundancy and temporal redundancy between video frames to reduce the encoded video size.
So instead, we leverage this encoding effectiveness.
In each frame, we set the pixels outside of the requested regions in the high quality image to black, \ie RGB=(0,0,0), and encode these images into a video file (mp4).%\ap{the reader won't know what background and foreground pixels are in this case}
% This refinement will be evaluated in Figure~\ref{fig:eval-refinements}(b).
}

\mypara{Reducing \cameranew{average} delay via early reporting}
\begin{figure}
\centering
\includegraphics[width=1\columnwidth]{figs/early-report.pdf}
\tightcaption{Illustration on how \name reduces response delay through early reporting on semantic segmentation. The error is calculated based on the inference result of a ultra-high quality video that we used to derive ground truth. Over 90\% of the results are early reported in stream A.}
\label{fig:early-report}
\end{figure}
% \label{subsec:reduce-delay}
The cost that \name pays to get better performance is the worst-case response delay; the result of Stream B will wait for two ``round trips'' before it can be returned to the analysts.
\cameranew{However, chances are that we could reduce the average delay per object.}
We leverage the observation that a substantial fraction of the DNN output from the low-quality video (Stream A) already has high confidence and thus can be returned without waiting for Stream B. 
While this optimization does not change the bandwidth consumption or worst-case response delay, it substantially reduces the delay of many inference results. 
In object detection, we empirically found that over $90\%$ of all final detected objects could have been detected in Stream A. 
These objects can be returned much faster than any prior approach, because Stream A uses a quality level much lower than what other work (\eg~\cite{awstream,nn-meets-pn,adascale}) would need to achieve the same accuracy. 
Similarly, in semantic segmentation, we found that the label of over $93\%$ of all pixels could been reported through stream A. Fig. ~\ref{fig:early-report} demonstrates how \name reduce response delay through early reporting.
% This refinement will be evaluated in Figure~\ref{fig:eval-refinements}(b).




% \tightsubsection{Leveraging camera-side heuristics}
% \label{subsec:integration}

\mypara{Leveraging camera-side heuristics}
%\hh{This part (and the corresponding part in the evaluation is interesting, but I don't find it crucial to the larger point.  A candidate to cut for space.  We could even cut here and then include a subset of the results just to argue that it is strictly better.}
\cameranew{When the connection to the server is poor, \name will alternatively attempt to leverage camera-side compute.}
\cameraold{
The key advantage of doing so is not only incorporating more computing power, but to leverage that the cameras have access to the raw (full resolution) video.
Here, we use tracking as a camera-side heuristics that can be incorporated in \name. 
}
%In particular, the framework introduced in \S\ref{subsec:formalizing} is amenable to two types of camera-side heuristics, which have been used in prior work.
%\mypara{Camera-side tracking}
\cameraold{
Tracking is usually less compute-intensive than tasks such as object detection, so some prior work has proposed having the camera track objects (\eg using \cite{kcf}) detected by the server-side logic (\eg~\cite{glimpse}).
\name can benefit from a similar idea by requesting fewer frames in the feedback regions and performing camera-side tracking between the requested frames.
For instance, given a 30-frame segment, the server will decide regions in each of the 15 frames, but instead of requesting all of them from the camera, it only requests the regions in the first frame and sends back the final results of the first frame to the camera which then tracks them using local tracking logic.
}
\cameranew{
\name will use a similar technique as Glimpse~\cite{glimpse}, which uses camera-side tracking to generate inference results on new frames based on the results on previous frames, to handle server disconnection.
}
% As we will see in Figure~\ref{fig:eval-client-integration}(a), being able to track objects by the camera allows \name to request significantly fewer frames without hurting accuracy too much.

%\mypara{Camera-side region proposal}
%There are cheaper yet less accurate region proposal techniques (\eg~\cite{mobilenetv2}) that could detect regions of interest, and some prior work has proposed to use such heuristics to identify frames with more objects and send only these frames (\eg~\cite{vigil}).
%Although completely relying on camera-side region proposal logic can lead to false positives (\ie proposed regions without real object) and false negatives (\ie missing a region with real object), \name can benefit from it by combining these regions with \name's DNN-generated region proposal. 
%In particular, when the camera receives the feedback region set from the server, it can send, not only these requested regions, but the regions proposed by local heuristics as well. 
%This can sometimes reduce \name's false negatives, since the camera can see the raw video, so it may find regions of extremely small objects, which the server-side DNN might have missed by analyzing the low-quality video.
%As we will see in Figure~\ref{fig:eval-client-integration}(b), being able to run region proposal locally by the camera allows \name to sometimes improve accuracy (by sending regions that the server misses) without paying much cost of bandwidth.
%\hh{I feel like this needs one more sentence about how even if the camera-side makes region proposals, the scheme still benefits from server-side proposals.}




%Although relying only on these results will cause lots of false negatives too, this allows \name to return these results in Stream A without waiting for Stream B, so majority of the results (\eg detected objects) can have an extremely low response delay.














==> design-new.tex <==
%!TEX root = main.tex
%!TEX spellcheck = en_US 


\tightsection{DNN-Driven Video Streaming}
\label{sec:overview}

In this section, we present the design of \name and discuss its design rationale and performance tradeoffs. % with the framework introduced in \S\ref{subsec:cost-accuracy-delay}.


\tightsubsection{Overall workflow}
We explore an alternative approach, called {\em DNN-driven streaming} (\name). 
In \name, the compression and streaming behaviors are driven by the feedback judiciously generated by the server-side DNN, rather than the low-complexity local heuristics on the camera side, in order to capture what the analytics engine needs from the real-time video content.
% \mypara{Iterative streaming}
Figure~\ref{fig:contrast-dds} contrasts the workflow of \name with that of the traditional source-driven approach: source-driven streaming is ``single-shot'' (\ie camera using simple heuristics to determine how the video should be streamed out), but \name is {\em iterative} and logically contains two streams:
\begin{packeditemize}
	\item {\bf Stream A (passive, low quality):} The camera continuously sends the video in low quality to the server.
	\item {\bf Stream B (feedback-driven):} The server frequently (\eg every handful of frames) extracts the {\em \ambiguous regions} from the DNN outputs on the Stream A video and sends them back to the camera as feedback. 
	Upon receiving the feedback from the server, the camera then re-encodes the recent history video accordingly and sends it to the server for a second-round inference on these ``zoomed-in'' images. 
\end{packeditemize}
The key to \name's success is the design of the \ambiguous regions, which we discuss next.

\begin{figure}
\centering
\includegraphics[width=0.75\columnwidth]{figs/contrast-dds.pdf}
\tightcaption{Contrasting the new real-time DNN-driven streaming (iterative) with traditional video streaming in video analytics.}
\label{fig:contrast-dds}
\vspace{-0.2cm}
\end{figure}


\tightsubsection{Feedback regions}
\label{subsec:feedback}

\cameranew{
\mypara{High-level framework}
\name extracts the \ambiguous regions by utilizing the information naturally returned/generated by the server-side DNN, rather than a wholesale change on the  DNN architecture. 
To deal with a variety of DNNs with different outputs, \name uses a custom logic to extract \ambiguous regions from each DNN. 
But these logics share the same framework (explained next) and are integrated with DNNs using a similar interface (explained in \S\ref{subsec:interface}).
For convenience, we use the term ``elements'' to denote the unit of a vision task---a bounding box (in object detection and face recognition) and a pixel (in semantic segmentation).
At a high level, given the DNN output on the low-quality video, we first identify the elements that are likely to be in the DNN output on the high-quality video but not in the DNN output on the low-quality video, and we then pick a small number of rectangles (for encoding efficiency) as the \ambiguous regions to cover these elements.
% ``\objectness'' scores in each frame and then filter out those regions that are already confidently detected. After that, we pick those rectangles that has high \objectness scores.
% We refer to the result of this process as the {\em \ambiguous regions} and send them back the the camera as the feedback.
Next, we present how this high-level logic is used in two classes of vision tasks.






\mypara{Object detection (based on bounding boxes)}
% Generate high-\objectness-score results.
Most bounding-box-based DNNs are anchor-based (though some are anchor-free \cite{carion2020end}). 
This means that a DNN will first identify regions that might contain objects and then examine each region. 
Each proposed region is associated with an objectness score that indicates how likely an object is in the region.
For DNNs (\eg FasterRCNN-ResNet101~\cite{DBLP:journals/pami/RenHG017}) that use region proposal networks (RPNs), each proposed region is directly associated with an objectness score. 
However, not all object-detection DNNs use RPNs. 
For instance, Yolo~\cite{yolo} does not and instead, it assigns a score for each class in each region in the final output. 
In this case, we sum up the scores of non-background classes as the objectness score, which indicates how likely a region includes a non-background object.
% \footnote{Most of the DNNs propose regions through region proposal network. We then extract the regions and corresponding scores of the output of that. In some DNNs like YoLo\cite{yolo}, the proposed regions are assigned with scores for each class. In this case, we sum up the scores of non-background classes as the \objectness score. These regions are typically generated from different shape from input and need to be normalized by their shape.}. 
We keep regions with objectness score over a threshold (\eg 0.5 for FasterRCNN-ResNet101, and Figure~\ref{fig:eval-sensitivity-bw} will show \name's performance under different objectness thresholds).
From these high-objectness regions, we apply two filters to remove those that are already in the DNN output on the low-quality video (Stream A).
First, we filter out those regions that have over 30\% IoU (intersection-over-union) overlap with the labeled bounding boxes returned by DNN on the low-quality video. 
We empirically pick 30\% because it works well on all the videos in our dataset.
Second, we remove regions that are over 4\% of the frame size (roughly 20\% of each dimension), because we empirically find that if an object is large, the DNN should have successfully detected it. 
The remaining region proposals (bounding boxes) are used as \ambiguous regions. 

Figure \ref{subfig:bbox} shows an example: there are nine bounding boxes in high-objectness-score results, three of which overlap with inference results in Stream A and one of which is too large. 
The remaining five regions are the \ambiguous regions.
% \footnote{We empirically pick 0.3 mean the intersection over union is larger than 0.3} with successfully-detected objects.
% We also empirically eliminate those regions that occupies 4\% or more of the whole frames. Those regions are typically so large that they may cover multiple objects, which are already covered by other regions.

% high-\objectness-score elements from the intermediate results generated whilst performing inference. For those DNNs that explicitly leverage region proposal network (like in Faster-rcnn-resnet101\cite{model-zoo}) to delineate potential regions that contains objects, we could directly use the output of that. If not, the DNN will also implicitly propose regions with per-class scores. We could assign \objectness scores to these regions through summing up the scores of non-background classes and obtain regions with \objectness scores. 

% perform filtering
% After that, we filter out those regions that significantly overlap\footnote{By significant, we mean the intersection over union is larger than 0.3} with successfully-detected objects.

% We then picks those rectangles with \objectness score higher than a \objectness score threshold\footnote{We empirically set this threshold to 0.5 and will vary it in Figure \ref{fig:sensitivity-parameters}}. Among these rectangles, we further merge those rectangles that mutually overlaps\footnote{We merge the rectangles by replacing them with the minimum rectangles that covers all of them}. These rectangles will be our \ambiguous regions.


\begin{figure}[t]
\centering
    \subfloat[Bounding-box-based tasks]
    {
        \includegraphics[width=0.43\columnwidth]{figs/bbox-app.pdf}
        \label{subfig:bbox}
    }
    \subfloat[Pixel-based tasks]
    {   
        \includegraphics[width=0.43\columnwidth]{figs/pixel-app.pdf}
        \label{subfig:pixel}
    }
\tightcaption{Illustration on how \name generates \ambiguous regions on two types of applications.
}
\vspace{-0.2cm}
\label{fig:demonstrate-app}
\end{figure}

\mypara{Semantic segmentation (based on pixels)}
Semantic segmentation DNNs assign each pixel a class label (see Figure~\ref{fig:vision-tasks}), and in addition, they also give a score of each class for each pixel (the class with the highest score is the class label).
% the inference results are pixels assigned with multi-class classification scores.
% For those neural networks that do not output probability directly, we then apply a softmax function among classes to map those scores to probabilities.
We first assign a score of $1+max'-max$ to each pixel, 
% For each pixel, we ta $1+max'-max$ as the \objectness score, 
where $max$ is the largest score among classes of interest and $max'$ is the second largest. 
Intuitively, the higher the score is, the more ``indecisive'' the DNN is about which class a pixel belongs to.
% After that, we filter out those elements that are confidently detected, i.e., with large $max-max'$, by replacing their \objectness score with 0.
We then pick the \ambiguous regions by creating $k$ rectangles that cover as many high-score pixels as possible. 
We repeatedly pick the $n\times n$ rectangle in which the pixels have maximum average score and zero out the scores of corresponding pixels until we found $k$ rectangles. 
The values of $n$ and $k$ control the total number of pixels in the \ambiguous regions ($k\cdot n^2$). 
We use $n=32$ and $k=16$, though we do not claim them to be optimal values. (Figure~\ref{fig:sensitivity-parameters} shows the performance under different $k$ values.)
Figure~\ref{subfig:pixel} shows an example and the selection of one \ambiguous region.
We can see that the high-score pixels typically lie at the boundaries of objects. 
% , and we pick the regions (we only show one in the example) with high scores.
%this shape should be above $8\times8$ and below $200\times 200$. 
% When this shape grows larger, the $k$ should be smaller correspondingly. 
% The $k$ here serves the same function as \objectness score threshold in bounding-box-based vision tasks. The larger the $k$ is, the lower the average \objectness score will be inside those selected rectangles. We use the resulting rectangles as our \ambiguous regions.
 


}

We notice three properties of the above logic. 
\begin{packeditemize}
\item First, the \ambiguous regions are likely in the DNN output but not yet in DNN's output on low-quality video. 
This provides useful clue about where video quality should be increased in Stream B.
\item Second, to save bandwidth of Stream B, the \ambiguous regions are created with shapes that can be efficiently encoded. 
Thus, they are different from any direct (intermediate/final) output of DNNs (\eg region proposals).
\item Third, the algorithms to extract \ambiguous regions only assume the format of the DNN output, rather than particular DNN architectures or parameters. 
\end{packeditemize}

% We  only relies on the output of semantic segmentation algorithm. This property makes our method generalizable to all existing semantic segmentation methods.

% \jc{discuss the pros and cons of the above logics}
% An important design question then is {\em what should be the ideal feedback?} We believe it should meet three criteria.
% First, it should entail sufficient information to inform follow-up actions in the second iteration to achieve high accuracy (\ie sufficient). 
% Second, it should avoid wasting bandwidth on those objects that are already detected under the first iterations (\ie bandwidth-efficient).
% Third, it should apply to a wide range of DNN-based vision tasks (\ie generalizable).

% For each pixel, we found that the {\em range} of its scores is a good indicator of its \objectness\footnote{In segmentation, classifying the pixel as background is also important, thus we treat background as a special kind of object}. The higher this range is, the more 
% confident that it belongs to a certain type of object.



\tightsubsection{Handling bandwidth variation}
Like other video streaming protocols, \name must adapt its bandwidth usage to handle fluctuations in available bandwidth.
There are several effective control knobs that affect the bandwidth usage of \name. However, we empirically find that these knobs affect the bandwidth-accuracy tradeoff in a similar way (\ie on the same Pareto boundary; \S\ref{subsec:sensitivity}), so \name only tunes low quality level and high quality level.

%Other parameters, such as DNN confidence threshold $\alpha$, \ktedit{region proposal confidence threshold $\theta$}, IoU threshold $\beta$, and maximum proposed region area $\gamma$ will affect how many regions are requested in the second iteration, but we found changing these parameters has only minor effect, in part because the total areas of objects are often relatively small.
% The last three parameters control how many regions in $\Regions_{\Srv}$ should be kept in $\Regions_{\Feedback}$.
% Rather than alter the number of regions sent back (which would prevent detections in regions that were not sent) we choose to dynamically tune the low and high quality parameters.  This choice means that all objects are---in principle---detectable regardless of available bandwidth, although the probability of detection will decrease with decreasing quality.



To tune the low and high quality levels, we implement a feedback control system (illustrated in Figure~\ref{fig:feedback-control}). Our controller is based on prior work that proposes a virtual, adaptive control system that can be customized for specific deployments \cite{CALOREE,FAST}. 
To instantiate this controller, \name needs to specify three things:
%Instantiating the controller requires specifying three things: 
a bandwidth constraint to be met, feedback for monitoring bandwidth usage, and the tunable parameters that affect bandwidth usage. For \name, the bandwidth constraint is the estimated available bandwidth for the next segment (labelled (1) in the figure), the feedback is the total bandwidth usage (for both low and high quality) from the last segment (2), and the tunable parameters are the resolution and quantization parameters (\ie the QP in Figure \ref{fig:feedback-control}) of both the low and high quality (3).
% The controller consists of the content estimator, controller, and optimizer which are automatically customized when we specify the above three inputs (goal, feedback, and parameters).  
The controller continually estimates the \emph{base} bandwidth usage; \ie the last segment's bandwidth usage if the {\em default} parameter settings had been used.  The controller then takes this base behavior as well as the difference between the desired bandwidth constraint for the next segment and the achieved bandwidth usage for the previous segment and computes a scaling factor for the base bandwidth.  This scaling factor is passed to an optimizer which finds the low and high quality settings that deliver the scaled bandwidth usage while maximizing F1 score.  


\begin{figure}
\centering
\includegraphics[width=0.9\columnwidth]{figs/DDSControl.pdf}
\tightcaption{\name's adaptive feedback control system dynamically tunes the low and high quality configurations based on the difference between the estimated available bandwidth for the next segment and that used for the previous segment.}
\label{fig:feedback-control}
\vspace{-0.2cm}
\end{figure}


%Figure~\ref{??} illustrates the feedback-based control loop to adapt to bandwidth variation.
%\jc{Hank/Ahsan, could you write a paragraph about the control loop}


%We would like to highlight that this controller works under a critical assumptions: the areas of the feedback regions are relatively stable, which makes the bandwidth demand of the same knob setting predictable. 
%Our evaluation result in \S\ref{subsec:eval-adaptation} empirically shows this assumption is reasonable. 
%It is important that this does not mean the feedback regions are predictable; rather, the feedback regions can vary significantly over a short period of time (which is also why \name can compress video more efficiently than prior work that must compress whole frames).
%The above assumption only requires their total areas to be relatively stable. 
%For instance, in a highway video (\eg Figure~\ref{fig:example-feedback}), the exact locations of the vehicles may change, but the total area of the feedback regions around the vehicles can be relatively stable as long as the number of cars in the video does not change significantly. 


%Moreover, if the assumption holds, the controller enjoys provides several useful formal properties. \
\name's dynamic bandwidth adaptation has several useful formal properties based on its use of feedback control.

% First, the content estimator handles non-linearities in the relationship between the parameters and bandwidth.  Intuitively, we can think of the parameter-bandwidth relationship as a curve and the content estimator as drawing a tangent to that curve.
% The controller then uses that tangent as a linear approximation to the true behavior \cite{ICSE2014}. 
\cameranew{First, the content estimator can handle {\em dynamic} video content which changes the relationship between the parameters and bandwidth usage. The adaptation mechanism uses a Kalman Filter to continually estimate the \emph{base} bandwidth usage. Hence, when the video content changes, the control model---that captures the relationship between the parameters and bandwidth usage---will update itself, allowing \name to capture unmodeled non-linearities in the relationship between quality settings and bandwidth use. Intuitively, we can think of the relationship between bandwidth usage and quality parameters as a curve and the base bandwidth (estimated by the Kalman filter) as a tangent to that curve. When adjusting the quality parameters, the \name controller uses this tangent as a linear approximation to the true behavior. Using this formulation, the bandwidth usage converges to the bandwidth constraint in time proportional to the logarithm of the error in this estimation \cite{CALOREE}. This adjustment technique provides robustness in the face of shifts and variations in the system including when there does not exist a single control model that captures all system dynamics \cite{ICSE2014}. }

\cameranew{Second, the optimizer finds the highest quality given the bandwidth usage specified by the controller.  This optimality is achieved by scheduling configurations over multiple segments.  As the system has a small, constant number of constraints (simply respecting the bandwidth requirement), an optimal solution can be found in constant time~\cite{Kim2015}. }     


\tightsubsection{Design rationale and performance analysis}
\label{subsec:design-rationale-performance-analysis}

\myparaq{Why driven by server}
At first glance, the idea of server-driven region extraction seems similar to Vigil~\cite{vigil} and EAAR~\cite{eaar}, which also identifie and send only regions likely with objects to the server. 
But we argue that the region extraction methods of Vigil and EAAR spend extra bandwidth on objects that can be detected at low quality, and they do not generalize to applications like semantic segmentation.
Moreover, both of them do not leverage modern video codec to save bandwidth.
Furthermore, Vigil's camera-side local model uses simpler feature extractor than the server-side DNN, and thus might miss objects when analyzing challenging video content (as illustrated in Figure~\ref{fig:contrast-model}).
%Thus, both Vigil and Glimpse will have sub-optimal performance. 
As we will show in \S\ref{subsec:eval-overall}, even if Vigil uses a model (MobileNet-SSD) that runs only 3$\times$ faster than the server-side DNN~\cite{model-zoo}, it still misses about 40\% more objects of interest than \name and sends over 30\% more data; EAAR consumes 4$\times$ bandwidth and still less accurate than \name. 
\S\ref{subsec:eval-overall} will give more analysis.



\cameranew{
\mypara{Analysis of \name's network usage} 
% When compared with a baseline that sends the whole video at the quality level of Stream B, 
The bandwidth usage of \name is governed by two factors: (1) the quality levels of Stream A and Stream B, and (2) the areas of the \ambiguous regions of Stream B.
If Stream A uses a high quality level, the bandwidth usage will be dominated by Stream A and the \ambiguous regions selected in Stream B will be less relevant. 
But if Stream A uses a very low quality level, \name cannot extract meaningful \ambiguous regions from the DNN output on the low-quality video. 
(\S\ref{subsec:eval-method} gives the detail configurations of Stream A and B.)
The areas of \ambiguous regions have a complex relationship with the video content. 
Intuitively, \ambiguous regions will be smaller when less objects/pixels are associated with small objects or hard-to-classify boundaries. 
When \ambiguous regions are so large that Stream B is almost the same size of the original video, then \name will not save much bandwidth. 

% First, if the total area of objects (as a fraction of the frame size) is smaller, Stream B will tend to use less bandwidth.
% The second iteration would consume even more bandwidth than directly sending out the whole high quality video if this property is not guaranteed. 
% Second, the bandwidth usage Stream A is determined by its quality level, so Stream A's quality level should be much lower than Stream B.

% \kt{(res, qp) = (0.8,36) for Stream A and (0.8, 26) for Stream B in object detection, (res, qp) = (1.0, 36) for Stream A and (1.0, 26) for Stream B in semantic segmentation\footnote{\cameranew{We use the full resolution in semantic segmentation to provide analytic results to every pixels.
% }} and (res, qp)=(0.7, 38) for Stream A and (res, qp)=(0.8, 26) for Stream B in face recognition\footnote{\cameranew{We use a lower low quality than object detection since face recognition is easier in terms of object types and object numbers in a frame.}}, where res here means how much we scale the width and the hight of the video, and qp means the quantization parameter of the encoder.}
% Though \name reduces the network cost, it needs to run inference twice on each frame sent in Stream B, so it needs twice the number of GPU cycles. 

To use the analysis in \S\ref{subsec:limitations}, when the total cost of a video analytics system is dominated by the network cost (Setting 1), \name will reach better cost-accuracy tradeoffs than the baselines, although it will do poorly when the cost is dominated by the server cost (Setting 2).

% Second, the quality of the first iteration should not be too low. Otherwise, the \ambiguous regions extracted from \name will be too inaccurate to be useful. 
% Third, the quality gap between Stream A and Stream B should be large. This is because a higher configuration in the second iteration could help \name recover more objects in stream B.


% If \name could provide a sizable gain on bandwidth, it is perfectly applicable on those network-cost-dominant scenarios. On server-side-cost-dominant scenarios, however, \name might be sub-optimal since \name requires extra DNN inference in order to save bandwidth.

\mypara{Delay analysis of \name}
One concern of \name is the extra delay in Stream B. 
% Thus, the worst-time delay of \name will be longer than the baselines. 
% This makes \name suboptimal in those applications like augmented reality. 
We introduce an optimization in \S\ref{subsec:optimization} to reduce the average response delay by reporting the objects/pixels that are already detected in Stream A. 
This allows \name to achieve a lower average response delay than the baselines at similar accuracy (see Figure~\ref{fig:delay-acc}), since Stream A has a low response delay and many objects/pixels will not need Stream B.
}
% applicable in those applications average delay.
% where $t_{stream}^A$ is the streaming delay in stream A, $\%streamB$ are the fraction of objects that are detected after stream B, $[\%streamB>0]$ is the truth value of proposition $\%streamB>0$, $t_{enc}$ is the time for the camera to perform re-encoding, $t_{stream}^B$ is the streaming delay in stream B and $t_{serv}$ is the server processing time. Typically, $\%streamB<10\%$. Hence, the effect that \name could reduce $t_{stream}^A$ by saving bandwidth is usually more significant then the extra average delay brought by stream B.



%\kt{where should we put the things about worst delay?}

% \mypara{In what setting will \name work}
% Here, we talk about in which scenarios will \name works, and in which scenarios will \name likely be sub-optimal. First, if the application values the worst-time response delay, \name might not be applicable due to one extra iteration. Second, if the overall cost is dominant by server-side cost, \name might also be undesirable due to the extra computation in the second iteration. However, \name is perfectly applicable when the overall cost is dominant by the streaming cost, since \name is able to effectively save the bandwidth.







\tightsection{Implementation}
\label{sec:impl}

% Here, we describe the changes needed to deploy \name over a video client and DNN server.
We implement \name mostly in Python and the code is available and will be regularly updated in~\cite{dds-code-repo}.

\tightsubsection{\name Interface}
\label{subsec:interface}


\name sits between the low-level functions (video codec and DNN inference) and the high-level applications (\eg object-detection queries).
% As illustrated in Figure~\ref{fig:apis}, 
It provides ``south-bound'' APIs and ``north-bound'' APIs, both making minimum assumptions about the exact implementation of the low-level and high-level functions.

The south-bound APIs interact with the video codec and DNN. 
Our implementation uses the APIs already exposed by the x264 MPEG video, such as \texttt{x264\_encoder\_encode}~\cite{x264}. 
From DNN, \name implements two functions: 
(1) \ambiguous regions, each with a specified location; and 
(2) detection results including the detected pixels/bounding boxes each with a specified location and a detection confidence score.

The north-bound APIs implement the same analyst-facing (north-bound) APIs as the DNNs (\name can simply forward any function call to DNNs), so the high-level applications (\eg~\cite{optasia,deeplens-sanjay}) do not need to change and \name can be deployed transparently from the analysts' perspective.
The only difference is that \name runs the DNN twice on the same video segment, so the two DNN inference results must be merged into a single result, which is logically similar to how DNNs internally merge redundant results (\eg~\cite{tu2012fuzzy}).

% \begin{figure}
% \centering
% \includegraphics[width=1.0\columnwidth]{figs/apis.pdf}
% \tightcaption{\name sits between applications and DNN/video codec, and exposes north-bound and south-bound APIs.}
% \label{fig:apis}
% \end{figure}



% \tightsubsection{Interfaces}
% \label{subsec:interfaces}

% \cameranew{
% \mypara{Camera requirements of \name}
% Our camera-side requirements are:
% \begin{packeditemize}
%     \item Buffer several images after sent.
%     \item Put rectangle-shaped image on a black background.
%     \item Encode with parameter given from \name.
%     \item Stream the video to the server.
%     \item Concatenate analytic results.
% \end{packeditemize}
% The first two requirements are introduced to re-encode \ambiguous regions in high quality. The third and forth requirements are the normal camera requirements.
% We require the camera to concatenate analytic results in order to reduce the response delay of \name. We will introduce corresponding technique below.
% }

\tightsubsection{Optimization}
\label{subsec:optimization}


\mypara{Saving bandwidth by leveraging codec}
% \tightsubsection{Reducing bandwidth needs by video codec}
% \label{subsec:reduce-bw}
A naive implementation of Stream B would encode each \ambiguous region as a separate high-quality image. %where the \ambiguous regions have high quality and the rest of the frames have low quality. %\ap{I replaced resolution with quality to (1) keep the terminology consistent (2) incorporate same resolution but lower qp cases as well}
But we found that the total size of these images would be much greater than the original video without cropping out the regions!
%\ap{not clear what "similar quality" is, we talk about two different qualities in the previous sentence. Also, I think maybe we can change the structure of this paragraph a little?}
The reason is that the video codecs (\eg H.264/H.265), after decades of optimization, are very effective in exploiting the spatial redundancies within a frame and the temporal redundancies between frames to reduce the encoded video size.
\name leverages such encoding effectiveness.
It sets the pixels outside of the \ambiguous regions in the high quality image to black (to remove spatial redundancies), and encodes these images into a video file (to remove temporal redundancies).%\ap{the reader won't know what background and foreground pixels are in this case}
% This refinement will be evaluated in Figure~\ref{fig:eval-refinements}(b).

\mypara{Reducing \cameranew{average} delay via early reporting}
% \begin{figure}
% \centering
% \includegraphics[width=1\columnwidth]{figs/early-report.pdf}
% \tightcaption{Illustration on how \name reduces response delay through early reporting on semantic segmentation. The error is calculated based on the inference result of a ultra-high quality video that we used to derive ground truth. Over 90\% of the results are early reported in Stream A.}
% \label{fig:early-report}
% \end{figure}
% \label{subsec:reduce-delay}
The cost that \name pays to get better performance is the worst-case response delay: the result of Stream B will wait for two rounds of inference before it can be returned.
% However, chances are that we could reduce the average delay per object.
We leverage the observation that a substantial fraction of the DNN output from the low-quality video (Stream A) already has high confidence and thus can be returned without waiting for Stream B. 
While this optimization does not change the bandwidth consumption or worst-case response delay, it substantially reduces the delay of many inference results. 
In object detection, we empirically found that over $90\%$ of all final detected objects could have been detected in Stream A. 
These objects can be returned much faster than any prior approach, because Stream A uses a quality level much lower than what other work (\eg~\cite{awstream,nn-meets-pn,adascale}) would need to achieve the same accuracy. 
Similarly, in semantic segmentation, we found that the label of over $93\%$ of all pixels can be returned by Stream A, without the need of Stream B.
%Figure~\ref{fig:early-report} demonstrates how \name reduce average response delay through early reporting.
% This refinement will be evaluated in Figure~\ref{fig:eval-refinements}(b).




% \tightsubsection{Leveraging camera-side heuristics}
% \label{subsec:integration}

\mypara{Camera-side heuristics for fault tolerance}
%\hh{This part (and the corresponding part in the evaluation is interesting, but I don't find it crucial to the larger point.  A candidate to cut for space.  We could even cut here and then include a subset of the results just to argue that it is strictly better.}
\cameranew{When the connection to the server is poor or the server is disconnected, \name will leverage camera-side compute (if available).
Like Glimpse~\cite{glimpse}, \name can use a camera-side tracking logic to generate inference results on new frames based on the results of the previous frames. 
% , to handle server disconnection.
}
\cameraold{The key advantage of doing so is not only incorporating more computing power, but to leverage that the cameras have access to the raw (full resolution) video.
Here, we use tracking as a camera-side heuristics that can be incorporated in \name.}
%In particular, the framework introduced in \S\ref{subsec:formalizing} is amenable to two types of camera-side heuristics, which have been used in prior work.
%\mypara{Camera-side tracking}
\cameraold{Tracking is usually less compute-intensive than tasks such as object detection, so some prior work has proposed having the camera track objects (\eg using \cite{kcf}) detected by the server-side logic (\eg~\cite{glimpse}).
\name can benefit from a similar idea by requesting fewer frames in the feedback regions and performing camera-side tracking between the requested frames.
For instance, given a 30-frame segment, the server will decide regions in each of the 15 frames, but instead of requesting all of them from the camera, it only requests the regions in the first frame and sends back the final results of the first frame to the camera which then tracks them using local tracking logic.}


==> discuss.tex <==
%!TEX root = main.tex
%!TEX spellcheck = en_US 

\tightsection{Limitations and discussion}

\mypara{Strict server-side resource budget}
In some sense, \name reduces bandwidth usage at the expense of relying on server-side DNN to run inference more than once per frame.
Similar tradeoffs can be found in AWStream, which triggers costly reprofiling periodically, and CloudSeg, which enforces an upfront super-resolution model customization process.
All these techniques may not be directly applicable where server resources have strict budgets or GPU cost is proportional to its usage (\eg cloud instances).

% \jc{limitations include what DNN we can handle, not applicable where server resource have strict budget (nor does awstream), and else?}
%While the design so far is functionally sufficient, it can suffer from performance issues if implemented as is.
%Here we highlight two optimizations that we found effective in our implementation. 
%As we will see in \S\ref{??}, these two techniques each contributed significantly to the performance of \name. 

% \hh{Maybe kill this whole section?  The first part is redundant with earlier text.  The second part says that we can't use confidence of detection as feedback, but it is part of the feedback.   There is a subtlety that confidence doesn't work, but confidence plus regions does and that is not coming across here.}


% A naive implementation of Stream B would encode each request feedback region as separate images where the requested regions have high resolution and the rest of the frames have low resolution.
% But the total size of these images would be much greater than the original video segment in the same quality level without cropping the regions!
% The reason is that video codec (\eg H.264/H.265), after decades of optimization, is very effective in exploiting spatial redundancy between pixels and temporal redundancy between video frames to reduce the encoded video size.
% Thus, we decided to leverage its encoding effectiveness.
% In each frame, instead of encoding high-quality requested regions over low-quality background, we set the background pixels to black, \ie RGB=(0,0,0), and encode these images into a video file (mp4).


%\mypara{Lessons learned} 
%Although DNN-driven streaming sounds intuitive, the development of \name was surprisingly challenging. Some lessons we learned were.
%\begin{packeditemize}
%\item {\em Feedback is the key differentiator.} 
%Despite rich output by ML algorithms, finding the right feedback signals is crucial.
%One could (1) use low confidence as an indicator that a region should be requested in higher quality (\eg~\cite{simpleproto}) or (2) directly request all proposed regions. 
%However, we found that lower confidence score may not always indicate a region has no object and sending all regions requires too much bandwidth. 
%Instead, when they are combined (\ie using proposed regions with low confidence), \name showed significant performance gains and robustness.
%\item {\em Not every optimization saves bandwidth.}
%Due to some unintuitive characteristics of modern video codecs, optimization that sounds useful sometime does not save much bandwidth; \eg reducing frame rate by 50\% will sometimes only save 10-20\% of bandwidth because the key frame is much larger than other frames and is rarely dropped. 
%\end{packeditemize}



% An early design of \name (described in~\cite{simpleproto}) used confidence score of each detected objects to indicate if the results from the low-quality video should be returned or requested in higher quality in the second round. 
% This looks like a reasonable design at first, but after countless experiments, we found the confidence values have at best a fairly weak correlation with whether a detected object is correct, and thus deriving feedback from confidence values did not yield desirable results.
% In contrast, once we switched to region proposal as the basis of feedback signal, it took us a much shorter time to get much better results. 


\myparashort{Implication to privacy:}
Privacy is an emerging concern in video analytics~\cite{wangpublishing}. 
While \name does not explicitly preserve privacy, it is amenable to privacy-preserving techniques. 
Since \name does not send out full resolution video, it could be repurposed to denature videos before sending only a part of the video to the server.
% We leave these ideas to future work.


\myparashort{Edge AI accelerators:}
Though \name makes minimal assumption on camera's local computation capacity, it benefits from the trend of more accelerators being added on edge devices, by using camera-side heuristics as described in \S\ref{subsec:optimization}. 
We also envision \name running alongside the camera local analytics to share the workload and provide higher inference accuracy with minimal bandwidth overheads.





% \section{Discussion}
% \begin{itemize}
% 	\item Implication to privacy: \name doesn't directly address privacy though it is amenable to privacy-preserving techniques, like denaturing etc
% 	\item What about DNN pipelines models?
% 	\item What about other vision tasks? 
% 	\item What about server-to-server? still useful. decoding and inference can be parallelized.
% 	\item Discuss edge AI accelerators
% \end{itemize}








==> eval-new.tex <==
%!TEX root = main.tex
%!TEX spellcheck = en_US 

% \jc{
% \begin{itemize}
% \item need to make the accuracy gap higher! 
% \begin{itemize}
% \item remove the idealistic assumption of awstream so that it may choose suboptimal configs for a good half of time. 
% \item try more specialized server-side model.
% \item adapt dds's 1st-round config to content.
% \item (backup: need justification of why the accuracy improvement of 5\% is important.)
% \end{itemize}
% \item add cloudseg in fig 11 and 12
% \item look into how bandwidth adaptation can be improved.
% \item add sensitivity analysis. accuracy/bw tradeoffs under different dds params (1st-iteration config, region proposal threshold)
% \item add segmentation like fig 11
% \end{itemize}
% }

% \subsection{Methodology}
% \begin{itemize}
% \item Setup
% \item Datasets
% \item Baselines
% \end{itemize}


% \subsection{End-to-end performance}

% \begin{itemize}
% \item Bandwidth vs. errors: 
% \begin{itemize}
% \item A table to compare DDS, AWStream, CloudSeg, Glimpse. 
% \item Figure~\ref{fig:eval-overall} comparing only DDS, AWStream, cloudseg with various parameters for three applications
% \end{itemize}
% \item Performance under various queries: DDS vs. AWStream under ``all object query'', ``vehicle only'', ``bus only'', ``truck only'', etc
% \item Response delay vs. error: Figure~\ref{fig:eval-realtime} with multiple DDS vs. response delay with various chunk size
% \end{itemize}


% \subsection{Sensitivity analysis}
% \begin{itemize}
% \item Sensitivity to server-side DNN: current figure 14
% \item Sensitivity to parameter settings: new graph from Kuntai
% \item Sensitivity to available bandwidth: 
% \item Sensitivity to bandwidth prediction error:
% \end{itemize}

\begin{figure*}[t!]
    \centering
    \hspace{-0.2cm}
    \subfloat[Object detection (Traffic)]
    {
        \includegraphics[width=0.22\textwidth]{figs/det_res_traffic.pdf}
        \label{subfig:1}
    }
    \hspace{-0.2cm}
    \subfloat[Object detection (Dashcam)]
    {
        \includegraphics[width=0.22\textwidth]{figs/det_res_dash.pdf}
        \label{subfig:2}
    }
    \hspace{-0.2cm}
    \subfloat[Object detection (Drone)]
    {
        \includegraphics[width=0.22\textwidth]{figs/det_res_drone.pdf}
        \label{subfig:2}
    }
    \hspace{-0.2cm}
    \subfloat[Face recognition (Friends)]
    {
        \includegraphics[width=0.22\textwidth]{figs/det_res_friend.pdf}
        \label{subfig:1}
    }
    
    \hspace{-0.2cm}
    \subfloat[Semantic segmentation (Traffic)]
    {
        \includegraphics[width=0.22\textwidth]{figs/seg_res_traffic.pdf}
        \label{fig:detection-traffic}
    }
    \hspace{-0.2cm}
    \subfloat[Sem. segmentation (Dashcam)]
    {
        \includegraphics[width=0.22\textwidth]{figs/seg_res_dash.pdf}
        \label{subfig:2}
    }
    \hspace{-0.2cm}
    \subfloat[Semantic segmentation (Drone)]
    {
        \includegraphics[width=0.22\textwidth]{figs/seg_res_drone.pdf}
        \label{subfig:2}
    }
    \hspace{-0.2cm}
    \subfloat[Face recognition (TBBT)]
    {
        \includegraphics[width=0.22\textwidth]{figs/det_res_tbbt.pdf}
        \label{subfig:1}
    }
    \tightcaption{The normalized bandwidth consumption v.s. inference accuracy of \name and several baselines on various video genres and applications. \name achieves high accuracy with 55\% bandwidth savings on object detection and 42\% on semantic segmentation, and 36\% on face recognition. %Color encoding indicates different solutions: \name (red), AWStream (blue), CloudSeg (green), Glimpse (yellow) and Vigil (Purple).
    Ellipses show the 1-$\sigma$ range of results.}
    \label{fig:eval-overall}
\end{figure*}


\tightsection{Evaluation}
\label{sec:eval}


The key takeaways of our evaluation are:
\begin{packeditemize}
\item On three vision tasks, \name achieves same or higher accuracy than the baselines while using 18-58\% less bandwidth (Figure~\ref{fig:eval-overall}) and 25-65\% lower average response delay (Figure~\ref{fig:freshness}). 
\item \name sees even more improvements on certain video genres where objects are small (Figure~\ref{fig:by-dataset}) and on applications where the specific target objects appear rarely (Figure~\ref{fig:motor}).
\item \name's gains remain substantial under various 
% across various video genres (Figure~\ref{fig:by-dataset}), 
bandwidth budgets (Figure~\ref{fig:bw-budget}) and bandwidth fluctuation (Figure~\ref{fig:eval-bw-variance}).
% , and as a result, the average response delay of \name is up to 30\% lower than that of the state-of-the-art.
% \item \name adapts to bandwidth fluctuation while maintaining high accuracy and low response delay.
\item \name poses limited additional compute overhead on both the camera and the server (Figure~\ref{fig:eval-overhead}).
% \item \name benefits substantially from careful implementation (Figure~\ref{fig:eval-refinements}) and opportunistically leveraging camera local heuristics (Figure~\ref{fig:eval-client-integration}).
\end{packeditemize}


\begin{table}[]
 \footnotesize
\begin{tabular}{rccccc}
\hline
    {\em Name}                     &  {\em Vision tasks} & {\em Total length} & {\em \# videos}  & {\em \# objs/IDs} \\ \hline \hline
Traffic       & obj detect / segment            & 2331s     & 7              & 24789           \\ \hline
Drone        & obj detect / segment             & 163s & 13        & 41678           \\ \hline
Dashcam  & obj detect / segment               & 5361s    & 9      & 24691          \\ \hline
Friends  & face recog      & 6000s      & 10        & 15022             \\ \hline
TBBT & face recog & 6000s & 10 & 12109\\
\hline
\end{tabular}
\vspace{0.4cm}
\tightcaption{Summary of our datasets.} %\kt{Write Friends instead of Sitcom (Friends), or else the table will overlap with the text on the right}}
\vspace{-0.6cm}
\label{tab:datasets}
\end{table}




%\begin{table*}[]
%\footnotesize
%\begin{tabular}{|c|c||c|c|c|c|>{\centering\arraybackslash}m{0.88cm}||c|c|c|c|>{\centering\arraybackslash}m{0.88cm}|}
%\hline
%\multicolumn{2}{|c||}{\multirow{2}{*}{}}                                                    & \multicolumn{5}{c||}{{\bf Bandwidth usage (mbps)}}         & \multicolumn{5}{c|}{{\bf Accuracy}}           \\ \hhline{~|~|-|-|-|-|-|-|-|-|-|-|} %\cline{3-12} 
%\multicolumn{2}{|c||}{}                                                                                 & \cellcolor[HTML]{9AFF99}DDS (ours)  & AWStream & CloudSeg & Glimpse & Vigil & \cellcolor[HTML]{9AFF99}DDS (ours) & AWStream & CloudSeg & Glimpse & Vigil \\ \hline
%\multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}{\bf Object}\\{\bf detection}\end{tabular}}      & Traffic &\cellcolor[HTML]{9AFF99}{\bf3.1}$\pm$0.4&7.0$\pm$1.0&5.0$\pm$0.5&0.9$\pm$0.2&5.7$\pm$0.3&\cellcolor[HTML]{9AFF99}{\bf.861}$\pm$.022&.857$\pm$.023&.665$\pm$.049&.267$\pm$.048&.506$\pm$.042\\ \hhline{~|-|-|-|-|-|-|-|-|-|-|-|} %\cline{2-12} 
%                                                                                            & Dashcam &\cellcolor[HTML]{9AFF99}{\bf3.3}$\pm$0.4&5.2$\pm$0.6&3.9$\pm$0.4&1.4$\pm$0.2&3.7$\pm$0.5&\cellcolor[HTML]{9AFF99}{\bf.843}$\pm$.018&.840$\pm$.017&.675$\pm$.065&.289$\pm$.018&.451$\pm$.024    \\ \hhline{~|-|-|-|-|-|-|-|-|-|-|-|} %\cline{2-12} 
%                                                                                            & Drone  &\cellcolor[HTML]{9AFF99}{\bf6.8}$\pm$0.8&15.4$\pm$1.2&9.1$\pm$0.9&2.2$\pm$0.2&17.8$\pm$1.7&\cellcolor[HTML]{9AFF99}{\bf.811}$\pm$.023&.794$\pm$.023&.681$\pm$.057&.265$\pm$.048&.732$\pm$.024    \\ \hline
%\multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}{\bf Semantic}\\{\bf segmentation}\end{tabular}} & Traffic &\cellcolor[HTML]{9AFF99}{\bf4.5}$\pm$0.6&6.4$\pm$0.9&5.0$\pm$0.5&\cellcolor[gray]{0.8}~&\cellcolor[gray]{0.8}~&\cellcolor[HTML]{9AFF99}{\bf.753}$\pm$.034&.751$\pm$.035&.272$\pm$.045&\cellcolor[gray]{0.8}~&\cellcolor[gray]{0.8}~    \\ \hhline{~|-|-|-|-|-|-|-|-|-|-|-|} %\cline{2-12} 
%                                                                                            & Dashcam &\cellcolor[HTML]{9AFF99}{\bf4.4}$\pm$0.5&6.6$\pm$0.9&5.4$\pm$0.6&\cellcolor[gray]{0.8}~&\cellcolor[gray]{0.8}~&\cellcolor[HTML]{9AFF99}{\bf.601}$\pm$.061&.581$\pm$.052&.216$\pm$.038&\cellcolor[gray]{0.8}~&\cellcolor[gray]{0.8}~   \\  \hhline{~|-|-|-|-|-|-|-|-|-|-|-|} %\cline{2-12} 
%                                                                                            & Drone  &\cellcolor[HTML]{9AFF99}{\bf6.8}$\pm$0.5&10.8$\pm$1.1&8.9$\pm$1.0&\cellcolor[gray]{0.8}~&\cellcolor[gray]{0.8}~&\cellcolor[HTML]{9AFF99}{\bf.842}$\pm$.014&.841$\pm$.016&.488$\pm$.053&\cellcolor[gray]{0.8}~&\cellcolor[gray]{0.8}~     \\ \hline
%{\bf Face recog.}                                                                           & Sitcom  &   \cellcolor[HTML]{9AFF99}          &          &          &         &       &    \cellcolor[HTML]{9AFF99}        &          &          &         &       \\ \hline
%\end{tabular}
%\vspace{0.2cm}
%\tightcaption{\jc{change this back to graphs}}
%\label{tab:perf-summary}
%\end{table*}




\tightsubsection{Methodology}
\label{subsec:eval-method}


\mypara{Experiment setup}
We build an emulator of video streaming that can measure the exact analytics accuracy and bandwidth usage.
\cameranew{Although existing video analytics platforms might support \name, we implement and test \name and all baselines in our emulator for a fair comparison.}
It consists of a client (camera) that encodes/decodes locally stored videos and a fully functional server that runs any given DNN and a separate video encoder/decoder. 
\cameranew{We run DNN inference on RTX 2080 super and all other computations on Intel Xeon Silver 4100.
}
Unless stated otherwise, we use FasterRCNN-ResNet101~\cite{DBLP:journals/pami/RenHG017} as the server-side DNN for object detection, InsightFace~\cite{Insightface,deng2018arcface} for face recognition and FCN-ResNet101~\cite{long2015fully} \cameranew{for semantic segmentation}. 
% \kt{Do we still need the sentence below?}
% \name extracts region proposals feedback regions of the object detection pipeline using FasterRCNN\cite{DBLP:journals/pami/RenHG017}, those of the face recognition pipeline using MTCNN\cite{DBLP:journals/corr/ZhangZL016}, and those of semantic segmentation using the method described in
% \S\ref{subsec:feedback}.
As we will see in \S\ref{subsec:eval-application}, different choices of DNNs will not qualitatively change the takeaways.
When needed, we vary video quality along the quantization parameter (from \{26,28,30,32,34,36,38,40\}, we call it QP for short) and the resolution (from scale factors of \{0.8,0.7,0.5\}), and \name uses 36 (QP) as low quality and 26 (QP) as high quality, with resolution scale set to 0.8 in object detection and 1.0 in semantic segmentation\footnote{We use full resolution in semantic segmentation to keep the same number of labeled pixels as in the ground truth which assigns each pixel a class label.}. 
\cameranew{
We do not consider the network cost of AWStream to profile the accuracy-bandwidth relationships under different QP-resolution combinations. This makes the AWStream bandwidth usage is strictly less than its actual one.}
% For \name, we uses the configuration stated in \S\ref{subsec:design-rationale-performance-analysis}.
% The accuracy is measured by F1 score (see \S\ref{subsec:dva} for details).
% The bandwidth demand is measured by \fillme.
% In addition, the emulator also implements some camera-side heuristics needed by the baselines (see the baseline description) and \name extension (\S\ref{subsec:integration}).
In most graphs, we assume a stable network connection, but in \S\ref{subsec:sensitivity}, we will 
\cameranew{test \name under different network bandwidth and latency and a few real network traces.}

\mypara{Datasets}
To evaluate \name over various video genres, we compile five video datasets  
% (in total, 49 videos, 29 for object detection and 20 for face recognition, summarized in Table~\ref{tab:datasets} and their links can be found in~\cite{DDSrepo}) 
each representing a real-world scenario (summarized in Table~\ref{tab:datasets} and their links can be found in~\cite{dds-data-repo}).
These videos are obtained from two public sources.
First, we get videos from {\em aiskyeye}~\cite{aiskyeye}, a computer-vision benchmark designed to test DNN accuracies on drone videos.
Nonetheless, \name and the baselines can be affected by factors such as fraction of frames with objects of interest or size of the regions with objects.
Therefore, we try to cover a range of values along these factors (including objects of various sizes and frames with various number of objects) by adding YouTube videos as follows.
We search keywords (\eg ``highway traffic video HD'') in private browsing mode (to avoid personalization biases); among the top results, we manually remove the videos that are irrelevant (\eg news report that mentions traffic), and we download the remaining videos in their entirety or the first 10-minutes (if they exceed 10 minutes).
The vision tasks are (1) to detect (or segment) vehicles in traffic and dashcam videos, (2) to detect humans in drone videos, and (3) to recognize identities in sitcom videos. 
Because many of these videos do not have human-annotated ground truth, for fairness, we use the DNN output on the full-size original video as the reference result to calculate accuracy.
% ground truth as the DNN results when the video is in its original quality. 
For instance, in object detection, the accuracy is defined by the F1 score with respect to the server-side DNN output in highest resolution (original) with over 30\% confidence score.
% , and this ground truth will be used to calculate the accuracy of \name and all baselines. \hh{I don't like calling this ground truth, since we know we don't have it.  We do clearly define what we mean.  I would prefer to change this to something like: "We define accuracy in terms of the DNN results when the video is in its full, original quality."  That might be too disruptive if we use the term "ground truth" throughout.  If it is not to disruptive, I would greatly prefer avoiding the term ground truth when the true value cannot be obtained.}



\mypara{Baselines}
We use five baselines to represent two state-of-the-art techniques (see \S\ref{subsec:machine-centric}): 
camera-side heuristics (Glimpse ~\cite{glimpse}, Vigil~\cite{vigil}, EAAR ~\cite{eaar}) and adaptive streaming (AWStream~\cite{awstream}, CloudSeg~\cite{cloudseg}). 
% , AdaScale~\cite{adascale})
We made a few minor modifications to ensure the comparison is fair. % or even favorable to the baselines.
First, all baselines and \name use the same server-side DNN.
Second, although \name needs no more camera-side compute power than encoding, camera-side heuristics baselines are given sufficient compute resource to 
% all require camera-side computing capacity to run inference/heuristics. 
% In particular, we assume the camera can 
run more advanced tracking~\cite{kcf} and object detection algorithm~\cite{mobilenetv2} than what Glimpse and Vigil\footnote{\cameranew{Our implementation of Vigil does not include the optimization of setting the background pixels in same RGB color, but in a separate experiment, we find that on the object detection videos (Table~\ref{tab:datasets}), this optimization only reduces Vigil's bandwidth usage by 10-20\% and leads to similarly low accuracy.}} originally used, so these baselines' performance is strictly better than their original designs. 
Third, all DNNs used in baselines and \name are pre-trained (\ie not transfer-learned with samples from the test dataset); In particular, our implementation of CloudSeg uses the pre-trained super-resolution model~\cite{ahn2018fast} from the website~\cite{carn-pytorch}.
This ensures the gains are due to the video streaming algorithm, not due to DNN fine-tuning, and it also helps reproducibility.
% Third, we assume AWStream directly selects the quality level just below the bandwidth target (without needing to probe the bandwidth).
% Notice that AdaScale's resolution selection logic was not designed to fit on a cheap camera. 
% For fairness, in our implementation of AdaScale, we train a classification model that runs roughly at the same speed at other camera-side heuristics. 
% We also use a slightly cheaper model (\fillme) than in AdaScale to predict the best resolution, but this model is already more expensive than other camera-side logic, so its real performance will be strictly worse. \hh{Something in the previous sentence reads funny as it sounds like we made AdaScale worse.  I think that "real"  performance means the published result (that uses the more expensive model?) but it is not clear why using a more expensive model would make the result worse.  Bottom line: I just didn't follow that part of the argument.}
%and \name can access a profile of accuracy vs. bandwidth consumption of each mpeg setting (resolution and QP) and the profile is updated periodically (by default, every 10 seconds). 
%This assumption again favors AWStream than \name, since \name uses less bandwidth than AWStream (\ie \name has more spare bandwidth to send high-quality frames to the server), so \name can update this profile at least as often as AWStream. \hh{If necessary, we could relax this assumption greatly.  The controller will be robust to errors in the profile that AWStream won't be able to tolerate.}
% Two additional notes on baselines: 
% First, the original AdaScale design only considers images. To make it work with video streaming, we use it to predict the best resolution on the first frame of each segment, which will be used to encode the entire segment.
Finally, although \name could lower the frame rate, to ensure that the accuracies are always calculated on the same set of images, we do not sample frames and only vary the resolution and QP in \name. %, which are also the most effective knobs~\cite{awstream}. 
% \hh{This does sort of contradict earlier claims about how we could temporally sample the video.  I know we still could do it---so it is not actually a contratdiction---but it is interesting that doing so is destructive for both humans and machines.}

\mypara{Performance metrics}
We use the definition of accuracy and average response delay from \S\ref{subsec:dva}.
To avoid impact of video content on bandwidth usage, we report bandwidth usages of \name and the baselines after normalizing them against the bandwidth usage of each original video. 



%\begin{figure}
%\centering
%\includegraphics[width=0.8\columnwidth]{figs/eval-per-dataset.pdf}
%\tightcaption{Distributions of improvement (bandwidth savings) by dataset.}
%\label{fig:eval-per-datasets}
%\end{figure}



%\begin{figure*}[t!]
%    \centering
%    \subfloat[Performance per dataset]
%    {
%        \includegraphics[width=0.3\textwidth]{figs/eval-per-dataset-2.pdf}
%        \label{subfig:1}
%    }
%    \subfloat[Impact of area per object]
%    {
%        \includegraphics[width=0.235\textwidth]{figs/figures_dds_0910/figure10/mean_area_bw.pdf}
%        \label{subfig:2}
%    }
%    \subfloat[Impact of total area of objects]
%    {
%        \includegraphics[width=0.235\textwidth]{figs/figures_dds_0910/figure10/total_area_bw.pdf}
%        \label{subfig:3}
%    }
%    \subfloat[Impact of \% of frame with objects]
%    {
%        \includegraphics[width=0.235\textwidth]{figs/figures_dds_0910/figure10/num_ratio_bw.pdf}
%        \label{subfig:4}
%    }
%    \tightcaption{Dissecting \name improvements along four dimensions. }
%    \label{fig:eval-sensitivity-object}
%\end{figure*}


\tightsubsection{End-to-end improvements}
\label{subsec:eval-overall}

 
% in terms of three important metrics: accuracy, bandwidth savings, and response delay. 


%\begin{table}[]
%\footnotesize
%\begin{tabular}{|c||c|c|c|c||c|c|c|c|}
%\hline
%\multirow{2}{*}{} & \multicolumn{4}{c||}{\textbf{Bandwidth usage (kbps)}} & \multicolumn{4}{c|}{\textbf{Accuracy (F1)}}  \\ \cline{2-9} 
% & DDS & AWS & ClSg & Glmps & DDS & AWS & ClSg & Glmps \\ \hline
%\begin{tabular}[c]{@{}c@{}}Traffic \\ (obj detect)\end{tabular} &  &  &  &  &  &  &  &   \\ \hline
%\begin{tabular}[c]{@{}c@{}}Dashcam \\ (obj detect)\end{tabular} &  &  &  &  &  &  &  &  \\ \hline
%\begin{tabular}[c]{@{}c@{}}Drone \\ (obj detect)\end{tabular} &  &  &  &  &  &  &  &  \\ \hline
%\begin{tabular}[c]{@{}c@{}}Traffic \\ (segmentation)\end{tabular} &  &  &  &  &  &  &  &   \\ \hline
%\begin{tabular}[c]{@{}c@{}}Dashcam \\ (segmentation)\end{tabular} &  &  &  &  &  &  &  &  \\ \hline
%\begin{tabular}[c]{@{}c@{}}Drone \\ (segmentation)\end{tabular} &  &  &  &  &  &  &  &  \\ \hline
%\begin{tabular}[c]{@{}c@{}}Sitcom \\ (face recog)\end{tabular} &  &  &  &  &  &  &  &  \\ \hline
%\end{tabular}
%\vspace{0.2cm}
%\tightcaption{}
%\end{table}



%\begin{table}[]
%\small
%\begin{tabular}{|c||c|c|c|c||c|c|c|c|}
%\hline
%\multirow{2}{*}{} & \multicolumn{4}{c||}{\textbf{Bandwidth usage (kbps)}} & \multicolumn{4}{c|}{\textbf{Accuracy (F1)}}  \\ \cline{2-9} 
% & DDS & AWS & ClSg & Glmp & DDS & AWS & ClSg & Glmp \\ \hline
%Traffic (obj) &  &  &  &  &  &  &  &   \\ \hline
%Drone (obj) &  &  &  &  &  &  &  &  \\ \hline
%Dashcam (obj) &  &  &  &  &  &  &  &  \\ \hline
%Traffic (seg) &  &  &  &  &  &  &  &   \\ \hline
%Drone (seg) &  &  &  &  &  &  &  &  \\ \hline
%Dashcam (seg) &  &  &  &  &  &  &  &  \\ \hline
%Sitcom (face) &  &  &  &  &  &  &  &   \\ \hline
%\end{tabular}
%\vspace{0.2cm}
%\tightcaption{}
%\end{table}

%\begin{table*}[]
%\small
%\begin{tabular}{|c||c|c|c|c||c|c|c|c|}
%\hline
%\multirow{2}{*}{} & \multicolumn{4}{c|}{\textbf{Bandwidth usage (kbps)}} & \multicolumn{4}{c|}{\textbf{Accuracy (F1)}}  \\ \cline{2-9} 
% & DDS & AWStream & CloudSeg & Glimpse & DDS & AWS & CloudSeg & Glimpse \\ \hline
%Traffic (object detection) &  &  &  &  &  &  &  &   \\ \hline
%Drone (object detection) &  &  &  &  &  &  &  &  \\ \hline
%Dashcam (object detection) &  &  &  &  &  &  &  &  \\ \hline
%Traffic (segmentation) &  &  &  &  &  &  &  &   \\ \hline
%Drone (segmentation) &  &  &  &  &  &  &  &  \\ \hline
%Dashcam (segmentation) &  &  &  &  &  &  &  &  \\ \hline
%Sitcom (face recognition) &  &  &  &  &  &  &  &   \\ \hline
%\end{tabular}
%\vspace{0.2cm}
%\tightcaption{}
%\end{table*}



%
%
%\begin{figure}[t!]
%    \centering
%    \hspace{-0.3cm}
%    \subfloat[Object detection]
%    {
%        \includegraphics[width=0.235\textwidth]{figs/det_res_delay.pdf}
%        \label{subfig:1}
%    }
%    \hspace{-0.1cm}
%    \subfloat[Face recognition]
%    {
%        \includegraphics[width=0.235\textwidth]{figs/face_res_delay.pdf}
%        \label{subfig:2}
%    }
%    \tightcaption{\name strikes better balance between accuracy and real-timeness than prior work.}
%    \label{fig:eval-realtime}
%\end{figure}


We start with \name's overall performance gains over the baselines along bandwidth savings, accuracy, and average response delay.

\mypara{Bandwidth saving} 
\cameraold{Figure~\ref{fig:eval-overall} compares the bandwidth-accuracy tradeoffs of \name with those of the baselines, when the total available bandwidth is set to match the size of the original video (we will vary the available bandwidth in \S\ref{subsec:sensitivity}). 
Across three vision tasks, \name achieves higher or comparable accuracy than AWStream and CloudSeg but uses 55\% less bandwidth in object detection and 42\% in semantic segmentation.
Glimpse and Vigil do sometime use less bandwidth but they have much lower accuracy.
Overall, even if \name is less accurate or uses more bandwidth, it always has an overwhelming gain on the other metric.}\cameranew{Figure~\ref{fig:eval-overall} compares the bandwidth-accuracy tradeoffs of \name with those of the baselines. 
In each application, we use a fixed \name configuration and normalize the bandwidth usage against the size of the highest-quality videos (which we use to derive the ground truth). 
We also lower the frame rate to 1~FPS to speed up the experiments and confirm on a randomly sampled set of videos that the 1~FPS optimization has minimal impact on \name's relative bandwidth savings and accuracy gains.
% (the accuracy difference is smaller than 1.5\% before and after sampling)
% (the bandwidth before sampling is about $15.5\pm 1.0\times$ larger than after sampling for those configurations used in Figure \ref{fig:eval-overall})
} Across three vision tasks, \name achieves higher or comparable accuracy than AWStream but uses 55\% less bandwidth in object detection and 42\% in semantic segmentation.
Glimpse sometimes uses less bandwidth but has much lower accuracy. 
Vigil, Glimpse, CloudSeg and EAAR consumes more bandwidth than \name with lower accuracy. Overall, even if \name is less accurate or uses more bandwidth, it always has an overwhelming gain on the other metric. 
% \name also outperforms the baselines of Glimpse and Vigil on accuracy by \fillme-\fillme\% without using more bandwidth. 


% Figure~\ref{fig:eval-overall} shows the bandwidth-accuracy tradeoff of \name and other baselines in two different applications. 
% We set available bandwidth to match the size of the original video.
% Figure~\ref{fig:eval-overall}(a) shows that, among the 29 videos of object detection (first three rows of Table~\ref{tab:datasets}), \name saves bandwidth by 40-60\% compared to AWStream, while achieving comparable accuracy.
% \name also outperforms the baselines of Glimpse and Vigil on accuracy by 30-70\% without using more bandwidth. 
% Similarly, Figure~\ref{fig:eval-overall}(b) also shows that, in face recognition (last row of Table~\ref{tab:datasets}), \name saves 30-55\% bandwidth compared to AWStream (with at least the same accuracy) and improves accuracy by 35-50\% over Glimpse and Vigil. 





%because \name reduces the bandwidth demand and despite needing a second iteration, most objects can be reported with high confidence in the first iteration (\S\ref{subsec:reduce-delay}). 
%These findings corroborate the need to reduce bandwidth demand and also show the benefit of reporting high-confidence results right after the first iteration . 
%Glimpse and Vigil (not shown) sometimes have shorter processing delay because most of their frames will be processed locally by a camera-side tracker, but their accuracy is much lower than \name and other baselines.



\begin{figure}[t]
\centering
    \subfloat[Precision on traffic video]
    {
        \includegraphics[width=0.46\columnwidth]{figs/det_res_traffic_pr.pdf}
        \label{fig:precision}
    }
    \subfloat[Recall on traffic video]
    {   
        \includegraphics[width=0.46\columnwidth]{figs/det_res_traffic_re.pdf}
        \label{fig:recall}
    }
\tightcaption{The normalized bandwidth consumption v.s. precision and recall of DDS and several baselines on traffic camera.}
\label{fig:precision-recall}
\end{figure}    

\begin{figure}[t]
\centering
    \subfloat[Object detection]
    {
        \includegraphics[height=0.23\columnwidth]{figs/det_res_delay.pdf}
        \label{subfig:1}
    }
    \subfloat[Semantic segmentation]
    {   
        \includegraphics[height=0.23\columnwidth]{figs/seg_res_delay.pdf}
        \label{subfig:2}
    }
\tightcaption{Response delay of \name is consistently lower than AWStream under various lengths of video segment. }
\label{fig:freshness}
\vspace{-0.2cm}
\end{figure}






% Figure~\ref{fig:eval-realtime} shows the tradeoffs between response delay and accuracy. 
% In both applications, we see that despite being an iterative protocol, \name still reduces the response delay by 15-30\% compared to AWStream which run server-side DNN processing on all frames. 
% These findings corroborate the need to reduce bandwidth demand and also show the benefit of reporting high-confidence results right after the first iteration (\S\ref{subsec:reduce-delay}). 
% Glimpse and Vigil sometimes have shorter processing delay because most of their frames will be processed locally by a camera-side tracker, but their accuracy is much lower than \name and other baselines.
% \jc{change to the new figure}



% \mypara{Distribution of improvements}
% Figure~\ref{fig:eval-per-datasets} partitions the improvement of \name by datasets. 
% In each dataset, we show the distribution of \name's bandwidth savings (in time windows of one minute) and the distribution of AWStream's bandwidth savings when it achieves same or higher accuracy.
% \jc{some takeaways}





% \mypara{Why \name outperforms in bandwidth-accuracy trade-off}
We explain this result from two  perspectives.

% \kt{I edited the part below}
\begin{packeditemize}

\cameranew{
\item {\em Precision and recall:} 
Figure~\ref{fig:precision-recall} corroborates our intuition (\S\ref{subsec:sources-of-limitations}) that the camera-side heuristics, used by Vigil, Glimpse and EAAR to select frames/regions, are limited by camera-side compute power and thus tend to either miss objects (as illustrated in Figure~\ref{fig:contrast-model}) and produce spurious objects (\eg Vigial and Glimpse), or use too much bandwidth to achieve decent accuracy (\eg EAAR).
We notice that CloudSeg has a lower recall than AWStream (whereas the original paper shows otherwise on a different dataset). 
We speculate that this is because we use a pre-trained super-resolution model (in consistent with the implementation of other baselines), whereas the original paper fine-tunes the super-resolution model to the dataset. 
% Figure~\ref{fig:precision-recall} corroborates with this intuition---Vigil and Glimpse 
% , we see that these heuristics either trust too much on camera-side results and leads to false positives and low precision (like Vigil and Glimpse), or is not effective enough to save sufficient bandwidth (like EAAR).
% \item {\em Recall:}
% Overall, Figure \ref{fig:recall} shows that the accuracy is mainly bounded by those objects that are difficult to detect in low quality.
% The low recall of Vigil and Glimpse demonstrates that the camera-side heuristics tend to miss those objects that even the server struggles to detect (this is also illustrated in Figure \ref{fig:contrast-model}).
\name has a higher precision because it uses the output of the server-side DNN model; it achieves high recall because it re-examines the uncertain regions from the low-quality video.
}
\item {\em Encoding:} 
Glimpse, Vigil, and EAAR all send individual frames separately, whereas  \name uses a video codec to leverage the temporal similarities across frames. Moreover, AWStream and CloudSeg do use video codec, but they do not leverage the non-uniform quality distribution, and \name (Stream B) 
only encodes the difficult-to-detect regions/pixels at a higher quality.
% with only small regions encoded in high resolution to improve accuracy as \name.
% s that these methods do not leverage modern video codec. Hence, these methods have to use extra bits for those inter-frame information.
\end{packeditemize}


\mypara{Response delay}
Figure~\ref{fig:freshness} shows the response delay of \name and AWStream (the baseline whose accuracy is the closest to \name) with the same length of a segment (number of consecutive frames encoded as a segment before sent to the server). 
In this experiment, we use a fixed bandwidth at the bitrate of the highest-quality video, which we use to derive the ground truth. 
Note that we exclude the buffering delay for the camera to accumulate the frames in each segment (which is the same between AWStream and \name) as well as the delay for \name to concatenate the pixel matrices in Stream A and Stream B (which can be sped up by standard libraries, such as openCL). 
% \jc{Kuntai, please give an example}
% The segment length limits the lower bound of the delay and 
For the same segment length, we see that \name reduces the average response delay by about 5-25\% compared with AWStream, despite that \name needs two iterations per frame. 
This is because \name detects most of the objects in Stream A whereas AWStream sends a single video stream and spends more time to transmit that stream through the network.
To put it into perspective, popular video sites use 4-second to 8-second segments~\cite{zhang2017modeling} (\ie over 120 frames per segment), a range in which \name's gains are considerable.
% \cameranew{
% % \item {\em Why \name reduces delay:}
% The to early reporting (illustrated in Figure \ref{fig:early-report}), the response delay of \name is much lower than AWStream because it detects most of the objects and sends most of the pixels in the first, low quality iteration. AWStream sends a single video stream and spends more time to encode that stream with quality.
% }









\cameraold{
\mypara{Intuition} 
\name achieves significant bandwidth savings compared to AWStream because \name is driven by DNN-generated feedback on the real-time video content while AWStream is content agnostic. Thus, \name aggressively compresses video by cropping out only \cameraold{regions of interest}\cameranew{ambiguous regions} in the Stream B. 
The bandwidth savings compared to Glimpse or Vigil result from the fact that camera-side heuristics lack crucial server-side information required to select the important frames \cameranew{and crop those regions that could really improve the inference results (i.e. ambiguous regions)}.
For fairness, we do not customize the super-resolution model to the specific video content; as a result, the super-resoluted frames actually leads to lower accuracy from the server DNN.
\name's response delay is much lower than AWStream because it detects most of the objects and sends most of the pixels in the first, low quality iteration. AWStream sends a single video stream and spends more time to encode that stream with quality.
% \jc{need to explain why cloudseg sucks so badly}
}

%\begin{figure}[t!]
%    \centering
%    \subfloat[By dataset]
%    {
%        \includegraphics[width=0.18\textwidth]{figs/box-datasets.pdf}
%        \label{subfig:1}
%    }
%    \subfloat[Per-object area]
%    {
%        \includegraphics[width=0.15\textwidth]{figs/box_mean_area_bw.pdf}
%        \label{subfig:2}
%    }
%    \subfloat[Total object area]
%    {
%        \includegraphics[width=0.15\textwidth]{figs/box_total_area_bw.pdf}
%        \label{subfig:3}
%    }
%    \tightcaption{Dissecting \name improvements along three dimensions. 
%    The candlesticks show maximum, median and minimum, and the boxes show 95\% confidence range.}
%    \label{fig:eval-sensitivity-object}
%\end{figure}





\tightsubsection{Sensitivity to application settings}
\label{subsec:eval-application}


\mypara{Impact of video genres}
Next, Figure~\ref{fig:by-dataset} shows the distribution of per-video bandwidth savings with respect to AWStream (dividing AWStream's bandwidth usage by \name's when \name's accuracy is at least as high as AWStream) in three datasets. 
There is substantial performance variability, even among the videos of the same type.
This is because \name's gains depend on the size of objects missed by the low-quality encoding, which varies with videos (\S\ref{subsec:design-rationale-performance-analysis}).

That said, the impact of content on performance gains can be task-dependent.
For instance, in object detection, the dashcam videos show less improvement than the other two datasets, but in semantic segmentation, the dashcam videos show the most improvement!
This contrast highlights the difference between the two tasks.
In object detection, when an object is not confidently classified, \name will send an entire bounding box to the server. 
However, semantic segmentation typically sends the pixels at the boundary of objects, whose size is less affected by the size of objects.
Since the dashcam videos have more large objects, they show more gains from \name when the task is semantic segmentation.
% contrast will appear only in dashcam videos.

%For each video, the bandwidth saving is measured by dividing AWStream's bandwidth usage that achieves highest yet lower-than-\name accuracy by \name's bandwidth usage. 


% \mypara{Impact of video genres}
% % \mypara{Impact of content characteristics}
% We have seen \name's overall improvements across all videos in our datasets.
% Figure~\ref{fig:eval-sensitivity-object} dissects \name's improvements along three dimensions
% % For clarity, we compare \name's bandwidth savings with AWStream, which achieves comparable accuracy to \name. 
% The bandwidth of \name is normalized by the bandwidth demand of AWStream when it achieves an accuracy that is closest to yet lower than \name's. The values on y-axis are less than 1 showing that the savings of \name with respect to AWStream are typically higher when they achieve the same accuracy.

% \begin{packeditemize}
% \item Figure~\ref{fig:eval-sensitivity-object}(a) shows that \name's gains are consistent between datasets; with the sitcom (face recognition) and traffic cameras exhibiting a slightly greater performance variance.
% \item Figure~\ref{fig:eval-sensitivity-object}(b) groups videos by the {\em average sizes of objects in each video}. 
% We can see that \name has more gains (especially the higher end) when objects on average are smaller. 
% \item Figure~\ref{fig:eval-sensitivity-object}(c) groups videos by the {\em total area with objects per frame}. We see that \name's gains are more obvious when total object areas are smaller, which corroborates our intuition that \name sends less data on non-object areas.
% \end{packeditemize}

\begin{figure}[t!]
    \centering
    \hspace{-0.3cm}
    \subfloat[Object detection]
    {
        \includegraphics[width=0.205\textwidth]{figs/det_cdf.pdf}
        \label{subfig:1}
    }
    \subfloat[Semantic segmentation]
    {
        \includegraphics[width=0.2\textwidth]{figs/seg_cdf.pdf}
        \label{subfig:2}
    }
    \tightcaption{Distributions of per-video bandwidth savings in two datasets.
    The gains of \name are video dependent.
    \vspace{-0.2cm}}
    \label{fig:by-dataset}
\end{figure}
% \begin{figure}[t!]
% %    \centering
%     \subfloat[Traffic videos]
%     {
%         \includegraphics[width=0.17\textwidth]{figs/placeholder-per-dataset.pdf}
%         \label{subfig:1}
%     }
%     \subfloat[Dashcam videos]
%     {
%         \includegraphics[width=0.17\textwidth]{figs/placeholder-per-dataset.pdf}
%         \label{subfig:2}
%     }
%     \subfloat[Drone videos]
%     {
%         \includegraphics[width=0.17\textwidth]{figs/placeholder-per-dataset.pdf}
%         \label{subfig:3}
%     }
%     \tightcaption{\jc{TODO}}
%     \label{}
% \end{figure}


\mypara{Impact of the targeted objects}
So far we have evaluated \name when the target object classes appear frequently in video, but an advantage of \name is that it saves more bandwidth when the server-side DNN only detects particular objects and these objects appear less frequently.
To show it, we change the segmentation task from detecting all objects to detecting only motorcyles. 
Figure~\ref{fig:motor} shows the \name's bandwidth savings (when achieving same or higher accuracy than AWStream) on three traffic videos in which motorcyles do appear but only in a small fraction of frames, and compare the bandwidth savings with those when the task is over all classes. 
\name's gains are more significant when only motorcyles are the target objects, and the gains are higher when the motorcyles take a smaller fraction of pixels and frames (\eg Video 2).


\begin{figure}[t!]
    \centering
    % \vspace{-0.3cm}
    \includegraphics[width=0.5\columnwidth]{figs/motor.pdf}
    \tightcaption{Segmentation on only motorcycles achieves 2-4$\times$ more bandwidth savings than segmentation on all classes. 
    \vspace{-0.2cm}}
    \label{fig:motor}
\end{figure}

\mypara{Impact of DNN architecture}
Last but not least, we test different DNN architectures on a randomly-selected traffic video (5-minute long). We find that \name achieves substantial bandwidth savings under different server-side DNN models: FasterRCNN-ResNet101 (44\%) and FasterRCNN-ResNet50~\cite{model-zoo} (54\%) has the same architecture but different feature extractors, while Yolo~\cite{yolo} (51\%) uses a different architecture and feature extractor (\S\ref{subsec:feedback}).
This implies that the benefit of \name is agnostic to the server-side DNN architecture. 
We leave a full examination of different DNN architectures (\eg MaskRCNN~\cite{maskrcnn}) to future work.

% \begin{figure}
% \centering
% \includegraphics[width=0.65\columnwidth]{figs/eval-sensitivity-dnn.pdf}
% \tightcaption{After changing the server-side DNN, \name still achieves 40+\% bandwidth savings (compared to AWStream when it achieves the closest yet lower accuracy to \name).}
% \label{fig:eval-sensitivity-dnn}
% \end{figure}




\subsection{Sensitivity to network settings}
\label{subsec:sensitivity}

\mypara{Accuracy vs. available bandwidth}
We then vary the available bandwidth and compare \name with AWStream, which is performance-wise the closest baseline. 
\cameranew{Figure~\ref{fig:bw-budget} shows that given different available bandwidth, \name can adapt its configurations to cope with them while achieving higher accuracy}.
We notice that the accuracy of semantic segmentation is lower than that of object detection (\ie the segmentation model is more sensitive to quality degradation). 
We speculate that this is because the segmentation accuracy is highly sensitive to the pixels around the object edges, which tend to be modified with slight quality degradation (this effect seems more pronounced when small objects are close to each other).
% \footnote{\cameranew{
% Our hypothesis on the low accuracy of semantic segmentation is that: the encoder saves bandwidth at a cost of blurring the boundaries of object in the video. 
% As a result, a large portion of pixels that lies between the objects are wrongfully classified as objects. This will significantly lower the accuracy since a lot of objects are pretty close in our dataset.}
% }.



\begin{figure}[t!]
    \centering
    \subfloat[Object detection]
    {
        \includegraphics[width=0.2\textwidth]{figs/det_res_vs.jpg}
        \label{subfig:1}
    }
    \subfloat[Semantic segmentation]
    {
        \includegraphics[width=0.1955\textwidth]{figs/seg_res_vs.jpg}
        \label{subfig:bw-budget-segmentation}
    }
    \tightcaption{
    % \name achieves high accuracy with 2$\times$ bandwidth savings on two different applications. Ellipses show 1-$\sigma$ range of results. To test AWStream under different network conditions, we run it with three target bandwidth $\{100,80,60\}\%\times$ bandwidth demands of the original videos.  
    \name outperforms AWStream (the closest baseline) in accuracy under various bandwidth consumption budgets.}
    \label{fig:bw-budget}
\end{figure}



\cameranew{
\begin{figure}[t]
\centering
    \subfloat[Bandwidth vs. streaming delay]
    {
        \includegraphics[width=0.215\textwidth]{figs/bandwidth-delay.pdf}
        \label{fig:bandwidth-delay}
    }
    \subfloat[Latency vs. streaming delay]
    {   
        \includegraphics[width=0.215\textwidth]{figs/latency-delay.pdf}
        \label{fig:latency-delay}
    }
\tightcaption{The response delay of AWStream, camera-only approach and \name with respect to different network bandwidth and network latency. \name is more sensitive to network latency.
}
\label{fig:vary-network-bandwidth-delay}
\end{figure}}


\cameranew{
\mypara{Impact of network bandwidth and latency} 
Figure~\ref{fig:bandwidth-delay} shows the impact of varying network bandwidth (while keeping the network latency at 10ms) on the streaming delay of \name and AWStream. 
We ensure that the accuracy of \name is always higher than the accuracy of AWStream.
We use Linux netem to vary the network bandwidth and latency.
% For this experiment we compare the impact of bandwidth alone, keeping network latency constant at 10ms. 
We see that DDS has lower streaming delay (\ie less time is spent on the network) than AWStream. 
This is because \name sends less data over the network than AWStream and many objects/pixels need only one iteration to be detected and classified.
% This is because \name is able to finalize majority of the results during the low quality iteration which requires a significantly smaller amount of data to be transferred than as compared to AWStream. While \name does incur additional delay due to the second iteration, the black-background optimization in \name's second iteration is able to reduce the impact of the second iteration on the overall delay. The bandwidth utilization from both phases is less than the bandwidth utilization of AWStream, which has to wait for the results to be received in a bulk. 
% The pure camera approach is not sensitive to the network setting and thus has no streaming delay.
Similarly, Figure~\ref{fig:latency-delay} shows the impact of network latency (while keeping the bandwidth at 500kbps) on the streaming delay of \name and AWStream. 
% For this experiment we keep a constant maximum bandwidth of 500kbps while modifying network latency. 
We see that when latency is over a threshold ($\sim$90ms in this experiment), \name has higher streaming delay than AWStream. 
This is because for those objects detected in Stream B, they experience two iterations, which makes the streaming delay of \name more sensitive to long network latency than AWStream. 
% Additionally, \name must also wait for the results to arrive from the server after the first iteration so that it may prepare the high quality iteration accordingly. 
% Hence, in settings where the network latency is high the latency cost can start to dominate bandwidth savings provided by \name.
}




\mypara{Impact of bandwidth variance}
Figure~\ref{fig:eval-bw-variance} compares \name with AWStream under an increasing bandwidth variance. 
We use synthetic network bandwidth traces to \cameranew{evaluate the impact of bandwidth variance in a controlled manner}. The available bandwidth of this trace is drawn from a normal distribution of $900\cdot N(1,\sigma^2)$Kbps while we increase $\sigma$ from \cameranew{0.1 to 0.9.}
We observe that \name maintains a higher accuracy than AWStream. 
Although \name and AWStream use the same bandwidth estimator (average of the last two segments), \name uses the available bandwidth more efficiently because \name's feedback control system continually adapts the model configuration parameters to bandwidth. 
Thus, \name adaptively selects the best possible configuration parameters at each time instant. 
% Further, the available configuration parameters for low and high quality video enable a wider range of possible adaptations and thus \name tunes its behavior at a finer granularity compared with AWStream. 
Even when the variance in available bandwidth is high ($\sigma>0.7$), \name maintains a relatively low response delay while AWStream's delay increases.


\begin{figure}[t!]
    \centering
    \subfloat[Accuracy]
    {
        \includegraphics[width=0.20\textwidth]{figs/variance_f1.jpg}
        \label{subfig:1}
    }
    % \hspace{-.9cm}
    \subfloat[Network delay]
    {
        \includegraphics[width=0.20 \textwidth]{figs/variance_delay.jpg}
        \label{subfig:2}
    }
    \tightcaption{\name can handle bandwidth variance and maintain a sizeable gain over the baseline of AWStream even under substantial bandwidth fluctuation. }
\vspace{-0.2cm}
\label{fig:eval-bw-variance}
\end{figure}

\begin{figure}[t!]
    \centering
    \subfloat[Network trace 1]
    {
        \includegraphics[width=0.235\textwidth]{figs/available_bw_trace_1.jpg}
        \label{subfig:1}
    }
    \subfloat[Network trace 2]
    {
        \includegraphics[width=0.235\textwidth]{figs/available_bw_trace_2.jpg}
        \label{subfig:2}
    }
    \tightcaption{Impact of available bandwidth on performance under re-scaled real network trace.
    % \jc{need to change vary the scaling factor, maybe run it on two different traces?}.
    }
\vspace{-0.2cm}
\label{fig:eval-sensitivity-bw}
\end{figure}

\cameranew{
\mypara{Under real network traces}
Next, Figure~\ref{fig:eval-sensitivity-bw} evaluates \name against AWStream on two real network traces~\cite{networktrace}.
Since the available bandwidth in the traces on average exceeds the bandwidth needed to stream the original video, we stress-test \name by scaling the available bandwidth by a constant factor to mimic settings where multiple cameras share the bottleneck bandwidth (TCP-induced variances are ignored).
In particular, we scale the average bandwidth of trace to 1,100kbps and 600kbps, while retaining the relative bandwidth variance in the trace. %\hh{We should say what the factor is.}
We can see \name consistently achieves higher accuracy under different mean available bandwidth.
}

\mypara{Impact of parameter settings} 
Figure~\ref{fig:sensitivity-parameters} shows the impact of key parameters of \name on its accuracy/bandwidth tradeoffs: 
the QP in Stream A (``low QP''), the QP in Stream B (``high QP''), the objectness threshold, and the number of feedback regions (\ie the $k$ introduced in \S\ref{subsec:feedback}).
We vary one parameter at a time and test them on the same set of traffic videos. 
The figures show that by varying these parameters, we can flexibly trade accuracy for bandwidth usage. 
% \footnote{\kt{The Pareto boundary of \name in this figure is different from Figure \ref{fig:bw-budget} since we use different sets of parameters in these two Figures.}}.
Overall, their effect roughly falls on the same Pareto boundary, so there may not be significant difference between the choices of parameters to vary when coping with bandwidth fluctuation.


\begin{figure}[t!]
    \centering
    \subfloat[Object detection]
    {
        \includegraphics[height=0.23\columnwidth]{figs/det_res_sensitivity.pdf}
        \label{subfig:1}
    }
    \subfloat[Semantic segmentation]
    {
        \includegraphics[height=0.23\columnwidth]{figs/seg_res_sensitivity.pdf}
        \label{subfig:2}
    }
    \tightcaption{Sensitivity analysis of \name's parameters. By varying these parameters, \name can flexibly adapt itself to reach desirable accuracy for a given bandwidth constraint.}
\label{fig:sensitivity-parameters}
\vspace{-0.2cm}
\end{figure}

%\tightsubsection{Handling bandwidth fluctuation}
%\label{subsec:eval-adaptation}





%\mypara{Under real network traces}
%Next, Figure~\ref{fig:eval-sensitivity-bw} evaluates \name against AWStream on two real network traces captured from cellular network carriers~\cite{networktrace}.
%On average, the available bandwidth in the traces usually exceeds the bandwidth needed to stream the original video, we stress test \name by scaling the available bandwidth down by a constant factor to simulate different mean available bandwidth, 1,100kbps (dark shade) and 600kbps (light shade), while retaining the real bandwidth variance in the trace. %\hh{We should say what the factor is.}
%We can see \name consistently achieves higher accuracy {\em and} lower response delay under different mean available bandwidth.
%
%
%\begin{figure}[t!]
%    \centering
%    \subfloat[Network trace 1]
%    {
%        \includegraphics[width=0.235\textwidth]{figs/available_bw_trace_1.pdf}
%        \label{subfig:1}
%    }
%    \subfloat[Network trace 2]
%    {
%        \includegraphics[width=0.235\textwidth]{figs/available_bw_trace_2.pdf}
%        \label{subfig:2}
%    }
%    \tightcaption{Impact of available bandwidth on performance. 
%    % \jc{need to change vary the scaling factor, maybe run it on two different traces?}.
%    }
%\label{fig:eval-sensitivity-bw}
%\end{figure}



\tightsubsection{System microbenchmarks}


\begin{figure}[t!]
    \centering
    \subfloat[Server GPU]
    {
        \includegraphics[height=0.103\textwidth]{figs/server_gpu.pdf}
        \label{subfig:3}
    }
    \subfloat[Server CPU]
    {
        \includegraphics[height=0.103\textwidth]{figs/server_cpu.pdf}
        \label{subfig:server-cpu}
    }
    \subfloat[Client CPU]
    {
        \includegraphics[height=0.104\textwidth]{figs/client_cpu.pdf}
        \label{subfig:1}
    }
    \tightcaption{Compared to prior solutions, \name has low additional systems overhead on both client and server.}
\label{fig:eval-overhead}
\vspace{-0.2cm}
\end{figure}



\mypara{Camera-side and server-side overheads}
% \cameranew{
% \name and the baselines all trade camera-side and server-side resources for a better streaming quality in one way or another. 
% From this perspective, we should also learn about the extra server-side and camera-side overhead that these design choices bring, rather than merely evaluate their performance.
% }
Figure~\ref{fig:eval-overhead} compares the systems overheads of \name with the baselines. 
We benchmark their performance on our server, with one RTX 2080 Super and one 16-core Intel Xeon Silver 4100. 
We scale the CPU and GPU usage by normalizing their runtime (\eg 2x runtime on the same number of fully used CPUs will be translated to 2x more CPU usage).
% We further rescale the average CPU and GPU usage for all the approaches according to their running time to make sure the comparison is fair. 
Figure~\ref{fig:eval-overhead} shows that compared to AWStream (when the profiling cost is excluded), \name has 2x more overheads at both client-side CPU (the CPU usage may exceed 100\% since it may leverage more than one CPU cores), server-side CPU and server-side GPU.
This is because \name invokes extra encoding, decoding and inference costs in Stream B. 
However, the profiling cost of AWStream is a substantial server-side CPU and GPU costs. 
We estimate it by profiling 30 configurations (compared to 216 claimed in \cite{awstream}) over a 10-second video every 4 minutes (which is much less often than profiling a 30-second video every 2 minutes as used in~\cite{awstream}), the server-side CPU and GPU costs of AWStream have already become higher than \name.
That said, we acknowledge that if AWStream updates the profile less frequently (\eg every tens of minutes), its GPU usage could be lower than \name, but that might cause its profile to be out of date and less accurate.
\cameraold{On the camera side, Vigil is able to find more objects and thus deploys more trackers than Glimpse correspondingly. 
Hence, the client-side CPU overhead of Vigil is significantly higher than Glimpse. }
\cameranew{On the server side, both Vigil and Glimpse incur minimal CPU overheads (since they do not need to decode the video) and much less GPU overheads than \name and AWStream (since their camera-side logics reduce the need for server-side inference). }
% Thus, we did not plot the server-side CPU usage of Vigil and Glimpse in \ref{subfig:server-cpu}.

\cameraold{
On the server side, Vigil and Glimpse use much less GPU and CPU cycles than \name and AWStream, because they run inference only on a small fraction of frames (which in part leads to lower accuracy). 
% \name has a higher GPU utilization than AWStream due to the two iterations of inference. 
%However, we expect that this gap can be narrowed if the second iteration, which inherently has less data to process can be processed with a faster DNN that can handle smaller input sizes~\cite{google-tradeoff-benchmark}.
The reason \name has lower GPU usage than AWStream, despite running inference twice per frame, is that AWStream profiles a list of configurations (\eg pairs of QP and resolution) (total 216 configuration in \cite{awstream}) and that cost is non-trivial. 
In our implementation, we evaluate only 24 configurations on 15 frames in each 300-frames video, and the average GPU usage of AWStream is already higher than \name. 
That said, we acknowledge that if AWStream updates the profile less frequently (\eg every few minutes), its GPU usage could be lower than \name, but that might cause its profile to be out of date.}

%and each frame now need to be evaluated 2.15 times on average. So \name actually use less GPU resources.
%
%\ktedit{One may think that \name has higher GPU cost than AWStream since \name need to evaluate each frame twice but AWStream only evaluate each frame once. We argue that AWStream requires {\em expensive profiling} in order to explore the best possible configuration. In our implementation, We only evaluate 24 configurations (compared to 216 configs in \cite{awstream}) on 15 frames per 300 frames and each frame now need to be evaluated 2.15 times on average. So \name actually use less GPU resources.}
%\jc{explain the gpu cost of awstream. specific setting}
%
%\jc{put the numbers in the context of the extra cost of two-pass cost}

%\begin{table}[t]
%\small
%\begin{tabular}{ccccc}
%\hline
%                & \begin{tabular}[c]{@{}c@{}}Camera\\ encoding\end{tabular} & \begin{tabular}[c]{@{}c@{}}Network\\ comm.\end{tabular} & \begin{tabular}[c]{@{}c@{}}Server\\ decoding\end{tabular} & \begin{tabular}[c]{@{}c@{}}Server\\ inference\end{tabular} \\ \hline\hline
%Stream A (??\%) & ??                                                        & ??                                                      & ??                                                        & ??                                                         \\ \hline
%Stream B (??\%) & ??                                                        & ??                                                      & ??                                                        & ??                                                         \\ \hline
%\end{tabular}
%\tightcaption{Breakdown of \name response delay}
%\label{tab:breakdown}
%\end{table}
%
%
%\mypara{Breakdown of response delays}
%Assuming the above setup, the \name response delay consists of two iterations with Stream A contributing \fillme\% and Stream B \fillme\%.
%As shown in Table~\ref{tab:breakdown}, each iteration can be further broken down to the contributions of four steps: 
%camera-side encoding, network communication, server-side decoding, and server-side GPU processing.
%The most important takeaway from 
%It is also important to notice that many detected objects/faces with be returned directly by Stream A (without the delay of Stream B).

%\begin{figure}
%\centering
%\includegraphics[width=0.7\columnwidth]{figs/eval-overhead.pdf}
%\tightcaption{Compared to prior solutions, \name has minimal systems overhead on both client and server}
%\label{fig:eval-overhead}
%\end{figure}


\begin{figure}[t]
\centering
\includegraphics[width=0.53\columnwidth]{figs/fault-tolerance.jpg}
\tightcaption{\name can handle server disconnection (or server failure) gracefully by falling back to client-side logic}
\label{fig:eval-resilience}
\vspace{-0.1cm}
\end{figure}

% \hh{I didn't get anything out of the following section of results on fault tolerance.  It looks to me like if the server goes down the accuracy is terrible and basically useless, which I would expect.  Consider cutting this for space.}
\mypara{Fault tolerance}
We stress test \name with temporary server-side disconnection. 
By default, the camera runs \name protocol, and it also has a local object tracking algorithm as a backup. 
Figure~\ref{fig:eval-resilience} shows the time-series of response delay and accuracy.
First, \name maintains a desirable accuracy, but at $t=5$ second, the server is disconnected.
We see that \name waits for a short time (until server times out at $t=5.5$) and falls back to tracking the last detection results from the server DNN.
This allows for a graceful degradation in accuracy, rather than crashing or delaying the inference indefinitely. 
Between the server disconnection and the timeout, the segments will be placed in a queue, and when the local inference begins, the queue will be gradually cleaned up.
When the server is back online (at $t=13$), the camera will be notified with at most a segment-worth of delay (0.5 second), and begin to use the regular \name protocol to resume video analytics. Meanwhile the camera will continue to send a liveness probe every video  segment.


%\tightsubsection{System refinements}
%\label{subsec:eval-indepth}

\begin{figure}[t!]
    \centering
    \hspace{-0.3cm}
    \subfloat[Reducing bandwidth usage by smarter encoding]
    {
        \includegraphics[width=0.22\textwidth]{figs/eval-contrib-codec.pdf}
        \label{fig:eval-contrib-codec}
    }
    \hspace{0.2cm}
    \subfloat[Reducing response delay by early reporting ]
    {
        \includegraphics[width=0.22\textwidth]{figs/eval-contrib-early.pdf}
        \label{fig:eval-contrib-early}
    }
    \tightcaption{System refinements to (a) reduce Stream B bandwidth and (b) reduce response delay (both of them are introduced in \S\ref{subsec:optimization}).}
    \label{fig:eval-refinements}
\vspace{-0.1cm}
\end{figure}

\mypara{Performance optimization}
Figure~\ref{fig:eval-refinements} examines two performance refinements.
First, figure~\ref{fig:eval-refinements}(a) shows that (1) putting the proposed regions on a black background frame yields about 2$\times$ bandwidth savings over encoding each region separately; and (2) compressing these frames in an mp4-format leads to another 10$\times$ bandwidth savings.
Second, figure~\ref{fig:eval-refinements}(b) shows that returning the first-iteration output (\ie the high-confidence results in Stream A before Stream B starts), we reduce the average response delay by about $\sim40\%$. 

% \hh{Consider cutting the heuristics for space.  Although is we want to compromise, we could cut the high-level description in section 4 and keep this.}
%\mypara{Camera heuristics integration} \kt{The performance of corresponding Fig. is not impressive, do we still need this part?}
%Figure~\ref{fig:eval-client-integration} shows the additional performance improvements of \name by integrating a camera-side tracking algorithm, similar to the client of Glimpse~\cite{glimpse}.
%Instead of processing all frames by \name, we evenly sample one frame every 15 frames and track the objects detected on the sampled frames over time until the next sampled frame (more details in \S\ref{subsec:integration}).
%The experiments are based on one traffic video and one dashcam video, on which the original \name performs poorly.
%We can see that by incorporating camera-side tracking, \name uses a much lower bandwidth with only a minor drop in accuracy.

% Second, we consider a camera-side object detection logic, similar to the client of Vigil~\cite{vigil}, to propose regions of interest per frame. 
% We use the output bounding boxes of mobilenet-ssd. 
% By combining these camera-proposed regions with the region proposals of \name (in Stream B), we can achieve higher accuracy, because the camera object detection runs on the raw images, so it can sometimes detect very tiny objects. 
% Although \name's bandwidth demands increase, it is still much lower than that of the baseline of AWStream which achieves similar accuracy. 

%\begin{figure}[t!]
%    \centering
%    \includegraphics[width=0.5\columnwidth]{figs/det_res_tracking.pdf}
%    % \hspace{-0.3cm}
%    
%    % \subfloat{Comparison between \name with w/(o) camera-side tracking logic} 
%    % {
%    %     \includegraphics[width=0.235\textwidth]{figs/figures_dds_0910/figure12/det_res_tracking.pdf}
%    % }
%    
%    % % Kuntai: we put two graphs together
%    % \iffalse
%    % \subfloat[\name with camera-side tracking logic]
%    % {
%    %     \includegraphics[width=0.235\textwidth]{figs/figures_dds_0910/figure12/det_res_tracking.pdf}
%    %     \label{subfig:1}
%    % }
%    % \hspace{-0.1cm}
%    % \subfloat[\name with camera-side region proposal]
%    % {
%    %     \includegraphics[width=0.235\textwidth]{figs/figures_dds_0910/figure12/det_res_ssd.pdf}
%    %     \label{subfig:2}
%    % }
%    % \fi
%    \tightcaption{\name achieves better performance when integrated with a camera-side tracking logic. \kt{Do we still need this graph? The performance is not that good since camera-side heuristics hurts the accuracy of region proposal and inference accuracy.}}
%    %\jc{Kuntai, please start the y-axis from 0, and shouldn't x-axis be bandwidth?}
%    \label{fig:eval-client-integration}
%\end{figure}











==> gradient.tex <==

\section{\accgrad}

\kt{How to calculate \outputgrad}
\kt{Give empirical evidence}
\kt{Derive optimal configuration}

In this section, we introduce the definition of \outputgrad and how to calculate it in detail.



\subsection{Calculating \outputgrad}


\mypara{Notations}
Assume the system contains $n$ knobs: $k_1, \cdots, k_n$ and the current values of them are $v_1,\cdots, v_n$.
Thus, the current configuration of the system is $(v_1,\cdots,v_n)$.
We will focus on discussing how to calculate the \outputgrad for the $i^{th}$ knob.
So we denote the configuration of the system as $(\cdots v_i \cdots)$ to focus on the value of $i^{th}$ knob $v_i$.
Let the input processing function be $I$, which maps the configuration $(\cdots v_i \cdots)$ to the input of the DNN $I(\cdots v_i \cdots)$.
The DNN $D$ then forward the input $I(\cdots v_i \cdots)$ and get the corresponding output $D(I(\cdots v_i \cdots))$ as the inference results.

\mypara{Strawman way of measuring \outputgrad}
\outputgrad aims capture how much a small change in the current value of each knob \textit{flips} the DNN-returned confidence scores from below (or above) than the confidence threshold $\theta$ to above (or below) the confidence threshold $\theta$. 
We provide a strawman way of measuring \outputgrad by measuring the number of flips via measuring the change of number of the confidence scores above the threshold, where we count the number of the confidence scores above the threshold using the following function:
\begin{equation}
\footnotesize
    N(res) = \sum_{score\in res.scores} step(score - \theta),
\end{equation}
where $res$ is the inference results, $res.scores$ refer to the confidence scores inside the inference results and ideally $step(x)=1$ for $x>0$ and $step(x)=0$ for $x\leq 0$.
As a result, we define \outputgrad as
\begin{equation}
\footnotesize
    \frac{\Delta N}{\Delta v_i} = \frac{ |N(D(I(\cdots v_i + \delta \cdots) -  N(D(I(\cdots v_i \cdots)|}{\delta},
\end{equation}
where $\delta$ is a small change on the $i^{th}$ knob, and $|\cdot|$ refers to the absolute value function.


This strawman has one counter-example: if a confidence score changes from less than $\theta$ to greater than $\theta$, and another confidence score changes in the opposite direction, there should be two flips in total.
But as changing from less than $\theta$ to greater than $\theta$ increases $N$ and changing in another way decreases $N$, these two changes cancel each other and thus the value of $N$ actually does not change.


\mypara{Leveraging DNN differentiability}
As shown in \S\ref{subsec:differnetiability}, calculating \outputgrad (\ie $\frac{\Delta N}{\Delta v_i}$) trivially results in extra DNN inference.
To reduce such extra inference, we leverage the differentiability of the DNN.
Intuitively, in order to calculate how DNN output changes with respect to the knob change (\ie \outputgrad), we can calculate how DNN output changes with respect to the DNN input change, and then study how DNN input changes with respect to the knob change.
% how changing system knobs alters the DNN input, and then calculate how changing the DNN input alters the DNN output.
Formally, we can approximate\footnote{It is an approximation since chain rule only strictly holds when the change of the knob value $\delta$ is sufficiently small. However, in practice the knobs can only be chosen from a given set of values, thus $\delta$ cannot be arbitrarily small.} $\frac{\Delta N}{\Delta v_i}$ by the following chain rule:
\begin{equation}
    \frac{\Delta N}{\Delta v_i} \approx \frac{\partial N}{\partial I} \cdot \frac{\Delta I}{\Delta v_i},
\end{equation}
where $I$ is the input to the DNN. The first term $\frac{\partial N}{\partial I}$ is the partial derivative of $N$ with respect to $I$, which can be calculated analytically by performing backpropagation on the function $N(D(I))$\footnote{As the $step$ function in $N$ is not differentiable, \name instead use $sigmoid(k\cdot x)$ to approximate the function $step(x)$, where $sigmoid$ is the sigmoid function $\frac{1}{1+\exp(-x)}$. These two functions are almost identical when $k$ is large. In \name we take $k=20$.}, and the second term can be calculated by simply calculating the change of the DNN input, \ie $\frac{I(\cdots v_i+\delta \cdots)-I(\cdots v_i \cdots )}{\delta}$.



Recall the counter-example of the strawman way of calculating \outputgrad: the change made to the number of confidence scores above the confidence threshold might cancel each other.
To resolve this issue, we let any change on the DNN input (\ie $I(\cdots v_i+\delta \cdots)-I(\cdots v_i \cdots )$) always result in the change of the number of confidence scores above.
Mathematically we define \outputgrad as:
\begin{equation}
    \frac{\partial N}{\partial v_i} = \left| \frac{\partial N}{\partial I} \right| \cdot \left|\frac{\Delta I}{\Delta v_i}\right|,
\end{equation}
where $|A|$ here means taking the absolute value of every elements inside $A$.








% \mypara{Limitation of \outputgrad}
% Cannot optimize for hidden objects.





% Then, \accgrad of the $i^{th}$ knob $k_i$ is defined as:
% \begin{equation}
%     \frac{\partial Acc}{\partial v_i} = \frac{Acc(D(In_t(\cdots v_i \cdots)) - Acc(D(In_t(\cdots v_i+\delta  \cdots))}{\delta},
% \end{equation}
% where $v_i$ and $v_i+\delta$ is two consecutive values of knob $k_i$.


% With this gradient. \name can quickly adapt to optimal by re-allocating the resource from low \accgrad knobs to knobs with high \accgrad.

\subsection{Rationales of \accgrad}


We compare \accgrad to two main lines of work: profiling-based approach and DNN-driven approach, and illustrate the rationales of why \accgrad is better.



\mypara{Comparing to profiling-based approach}
\accgrad can be generated without extra inference (we will illustrate how to calculate \accgrad without extra inference in \S\ref{??}), while profiling-based approach needs to perform multiple extra inferences to obtain the profile.
To put this cost into context, take AWStream~\cite{awstream}, a profiling-based system analytics as an example.
In AWStream, fully profiling just \textit{one-second} video on three video encoding knobs already takes \textit{52} seconds of inference\footnote{We define one second of inference as inference on a 30FPS video}.

As a result, when the server-side compute is limited, the profiling-based approach either need to profile only a constrained subset of configurations (\eg downsample the configuration space by 50x), resulting in selecting sub-optimal configurations (and thus sub-optimal resource-accuracy trade-off), or need to profile much less frequently (\eg only profile 1/50 worth of data), making these systems unable to update the outdated profile, thus achieving sub-optimal resource-accuracy trade-off.


\mypara{Comparing to DNN-driven approach}

\kt{main argument, TBD}





% To obtain the knob-accuracy impact in real-time, we present \name. We first show that knob-accuracy impact is a better feedback for the underlying system, and discuss the APIs and mechanisms of obtaining accuracy gradient.

% % \subsection{Accuracy gradient as a better predictor}
% \kt{Introduce API}

% To better predict the accuracy, the key is to know the impact of knobs on accuracy in real-time.

% Obtaining knob-accuracy impact enables us to do two things.
% First, it can cheaply identify whether the current configuration is locally optimal or not.
% This is because checking the local optimality is essentially go through each knob and compare between the accuracy gain of changing the knob and the extra delay caused by the knob.
% In other word, we can check the local optimality by directly comparing between the knob-accuracy impact and extra delay.
% Second, it can better estimate the accuracy change of an unknown configuration under the same video content.


% One may worry that knob-accuracy impact will let the system stuck in the local optimal.
% We argue that for one single knob, when it goes from the cheapest value to the most expensive value, the accuracy gain will become smaller but the streaming delay will still grow in a steady pace. 
% As a result, the overall accuracy - delay objective is in general \textit{concave} and have no local optimal.


% \subsection{Key idea: accuracy-knob gradient}


% \begin{itemize}
%     \item 
%     \accres suggests that the change of accuracy with respect to knob value change can reflect the ability of trading resource for accuracy for each individual knob. 
    
%     \item In order to measure this change, we propose a new metric: \accgrad, defined as the difference of accuracy, divided by the difference of two consecutive values of one knob.
%     \item With \accgrad, \name can quickly adapt to optimal by allocate more resources to those knobs with high \accgrad to improve accuracy, and cut the resource usage of those knobs with low \accgrad to save resource.
%     \item Compared to frequent profiling: avoid extra inference.
%     \item Compared to server-side DNN output: use DNN parameters as a reliable performance estimator.
%     \item Show an example like AccMPEG.
%     % \item Present accuracy gradient as the solution and define accuracy gradient as the diff of accuracy divided by the diff of two consecutive parameter values.
%     % % \item With accuracy gradient, we can prune out those configurations that yeild similar accuracy without extra inference.
%     % % \jc{Gradient -> which parameters does not improve accuracy; which parameters does improve accuracy}
%     % \item First, accuracy gradient can be calculated without extra inference. We will further discuss this in \S\ref{subsec:decoupling}.
%     % \item Second, accuracy gradient can help \name to quickly approach to optimal. With accuracy gradient, \name can identify which parameters have huge impact on accuracy and improve accuracy by adapting these parameters. On the other hand, accuracy gradient also allows \name to identify which parameters have little impact on accuracy and save resource usage from these parameters.
% \end{itemize}

\subsection{Calculating \accgrad}
\label{subsec:calculate-accgrad}


However, calculating \accgrad directly incurs high overhead.
This is because calculating \accgrad requires calculating the accuracy change.
However, calculating accuracy change requires two kinds of extra inference:
\begin{packeditemize}
    \item Calculating the accuracy change for one designate knob (\ie calculate the accuracy before and after changing this knob by a small amount $\delta$, and calculate the difference of these two accuracy values) requires calculating the accuracy metric first, which requires the inference results under \textit{the most resource-demanding configuration} as the ``ground truth'', resulting in high GPU compute overhead.
    To put this overhead into context, in Chameleon~\cite{chameleon}, about $\sim$50\% of the overall GPU compute is used to calculate such ground truth.
    As a result, by removing this overhead, \name can already achieves 2x compute cost reduction compared to Chameleon.
    
    \item Calculating the accuracy change for multiple knobs requires \name to evaluate the accuracy change on every knob and thus requires extra inference when changing every knob.
    Further, the number of extra inference \textit{scales} with the number of total knobs.
    This makes it much difficult for the underlying system to handle more knobs.
\end{packeditemize}


To reduce the above two overhead, we first consider reducing the first overhead: how to avoid calculating the ``ground truth'' when calculating the accuracy change for one knob.
As \accres indicates:
\begin{itemize}
    \item \textit{Statistically}, the \textit{sign} of accuracy change is statistically determined by the resource usage before and after changing the knob: the accuracy statistically goes higher if the resource usage is higher after changing, and vise versa.
    \item \textit{Statistically}, the \textit{magnitude} of accuracy change is positively correlated to the \textit{change} of inference results. If the inference results barely change, the accuracy also barely changes, and vice versa.
\end{itemize}

The resource usage before and after changing one designated knob is easy to obtain. 
Take video quantization parameter (which is widely applied in video analytic systems~\cite{dds,awstream,eaar,chameleon,videostorm,vstore}) as an example.
If the value of this parameter goes higher, the video is encoded in lower quality and thus the resource usage decreases.
However, the challenge is to measure the \textit{change} of inference results as inference results might be of different format (\eg a sequence of text in speech translation, several human keypoints in human keypoint detection, etc).


To handle this challenge, we leverage the following two observations:
\begin{packeditemize}
    \item 
    In DNN-based analytic applications (like autonomous driving and video classification), only those \textit{confident} inference results (\ie the inference results that are of confidence scores higher than a threshold $\theta$) will be counted as true detection results and participant in accuracy calculation.
    \item 
    As previous work observes~\cite{dds}, those inference results that are almost detected but not (\ie the confidence scores are slightly below $\theta$) are likely to change the inference results.
\end{packeditemize}

To capture these two insights, our proxy to the accuracy change is:
\begin{align}
    & |Acc(D(In_t(\cdots v_i \cdots)) - Acc(D(In_t(\cdots v_i+\delta  \cdots))| \\
    \propto  & |f(D(In_t(\cdots v_i \cdots)) - f(D(In_t(\cdots v_i+\delta  \cdots))|,
\end{align}
where $f(x) = \sum_{s\in x.scores} sigmoid(k\cdot (s - \theta))$,  $x.scores$ is the confidence scores of each inference result of $x$, $sigmoid$ is the sigmoid function $sigmoid(x) = 1 / (1 + e^{-x})$, $k$ is a scaling parameter\footnote{In our experiment, we pick $k=20$ as it makes the sigmoid value close to 0.9 when the confidence score is just 0.1 larger than the confidence threshold} and $\theta$ is the confidence threshold.
This function captures the two above observations. First, this function ``counts'' the number of objects that are above the confidence threshold since the $sigmoid(k\cdot (s - \theta))$ is close to $1$ when the confidence score $s$ is higher than $\theta$ and is close to $0$ when the confidence score is slightly lower than $\theta$.\
Second, those inference results that are almost detected but not can significantly change the sigmoid value even if their confidence scores is just changed by a little.
For example, by fixing $k=20$ (which is the default choice of $k$ in \name), the corresponding sigmoid value already changes $0.1$ even when the confidence score just slightly changes from $\theta - 0.01$ to $\theta + 0.01$.




To reduce the second overhead, we leverage the chain rule of gradient, which says:
\begin{equation}
    \frac{\partial Acc}{\partial v_i} = \frac{\partial Acc}{\partial In_t}\cdot \frac{\partial In_t}{\partial v_i}
\end{equation}
The first term can be calculated without extra inference, and the second term is not related to DNN inference.














% \begin{comment}
% Calculating the knob-accuracy impact in real-time can consumes a lot of resource.
% For example, a naive way to calculate knob-accuracy impact is to enumerate every knob, change that knob a bit and observe the change of accuracy.
% However, this requires running the end-to-end system $O(n)$ times, where $n$ is the number of knobs. 
% \kt{Write a running example here}


% To overcome this difficulty, our approach is to obtain knob-accuracy impact by get the gradient of knobs with respect to accuracy (we call this gradient \textit{knob-accuracy gradient}).
% Obtaining knob-accuracy gradient requires us to 
% To answer this, we use chain rule to decouple the gradient into two parts:
% $$
% \frac{\partial Acc}{\partial k_i} = \frac{\partial Acc}{\partial I}\cdot \frac{\partial I}{\partial k_i},
% $$
% where $Acc$ means the accuracy function, $k_i$ means the $i^{th}$ knob, $I$ means the input of the DNN\footnote{As both of the two gradient is of matrix format, the $\cdot$ should be the inner product. We use $\cdot$ for simplicity.}.
% It makes use of two key properties of AI pipelines to drastically reduce the cost of calculating this gradient:
% \begin{packeditemize}
%     \item The analytic DNN is analytically differentiable.
%     \item For a large subset of knobs, obtaining the numerical gradient of the input to DNN with respect to knobs can be done locally on the camera and thus does not require sensor-server communication.
% \end{packeditemize}
% \end{comment}



% \subsection{Calculating accuracy change}

% \begin{itemize}
%     \item Previous work use most expensive configuration as the ground truth. Works well for evaluation purpose, but calculating this metric at runtime is too expensive.
%     \item To give context, \kt{raise some examples}
%     \item We instead propose a cheap run-time approximation of accuracy: accuracy \textit{proxy}. 
%     \item The key idea is to estimate the sign and estimate the magnitude.
%     \item Show the math formula.
% \end{itemize}

% \begin{itemize}
%     \item Trivially calcualte the gradient of accuracy proxy requires extra inference.
%     \item We make several assumptions to remove the extra cost.
% \end{itemize}



\subsection{Deriving optimal configuration}

By exposing \accgrad, \name allows the user to derive the optimal configuration.

\mypara{Objective function} 
The objective function of \name is $$Obj(c) = Acc(D(In_t(c))) - \lambda Delay(c),$$ where $c$ is the configuration, $Acc, D, In_t$ is the accuracy function, the DNN, the DNN input correspondingly, $Delay$ is the delay function and $\lambda$ trades between accuracy and end-to-end delay: higher $\lambda$ results in lower end-to-end delay but also lowers the accuracy.

By optimizing the objective function above, the configuration $c$ that \name gets will be optimal (if $c$ lies on a sub-optimal tradeoff, it means that there is another configuration $c'$ that has higher accuracy and/or lower delay. This makes $Obj(c') > Obj(c)$, which contradicts with the fact that $c$ optimizes the objective function.)




\mypara{Obtaining \delaygrad}

\mypara{Obtaining optimal configuration} To illustrate how \name optimizes the objective function $Obj(c)$ above using \accgrad, we use an simple example, where the configuration of the system $c$ is made up of two knobs $c=(v_1, v_2)$, where $v_1\in \{0,1,2\}$ and $v_2\in \{1,2,3\}$ are two knobs of the underlying system.
\name first creates two variables\footnote{The reason of creating these two variables is enable the use of widely-used gradient-based optimizers as these optimizers typically assumes the variable to be continuous.} $0 \leq v_1' \leq 2$ and $1\leq v_2' \leq 3$.
When running the analytic system, \name obtain the value $v_1, v_2$ of the knobs of the underlying system by a mapping function $map$.
This mapping function $map$ maps, say $v_1'$, back to $v_1$ by choosing the value from the knob values of $v_1$ (\ie $\{1,2,3\}$) such that is closest to $v_1'$.
Assume currently $v_1' = 0.3$, $v_2' = 2.7$.
As a result, we have $v_1 = map(v_1'; \{0,1,2\}) = map(0.3; \{1,2,3\}) = 1$, and $v_2 = map(v_2'; \{1,2,3\}) = map(2.7; \{1,2,3\}) = 3.$
After running the analytic system, \name obtains \accgrad and \delaygrad for $v_1, v_2$.
\name then assign the gradient of $v_1, v_2$ to $v_1'$, $v_2'$, optimizes $v_1', v_2'$  through Adam optimizer (a widely-used optimizer~\cite{??,??}) and truncates $v_1', v_2'$ so that they satisfy $0 \leq v_1' \leq 2$ and $1\leq v_2' \leq 3$.

% \name allows each knob to take any value between the smallest knob value to the largest knob value.
% When inference, \name will then pick the closest value inside all knob values that the underlying system accepts as the chosen knob value.
% For example, say for the knob $k_1$, the underlying system accepts $k_1=1,2,3$. Then \name allows $k_1$ to be any value inside the interval $[1,3]$.
% But 
% \name maximizes the objective function above through Adam optimizer~\cite{adam}, a commonly used optimizer for non-convex optimization~\cite{??}.



==> gradient_v2.tex <==

\tightsection{\outputgrad}


In this section, we introduce the way \name calculates \outputgrad and show the correlation between \outputgrad and the accuracy change.



\tightsubsection{Calculating \outputgrad}

\mypara{Notations}
Assume the system contains $n$ knobs: $k_1, \cdots, k_n$ and the current values of them are $v_1,\cdots, v_n$.
The current configuration of the system is $(v_1,\cdots,v_n)$.
We will focus on how to calculate the \outputgrad for the $i^{th}$ knob, whose current value is $v_i$.
% So we denote the configuration of the system as $(\cdots v_i \cdots)$ to focus on the value of $i^{th}$ knob $v_i$.
Let the input processing function be $I$, which maps the configuration $(\cdots v_i \cdots)$ to the input of the DNN $I(\cdots v_i \cdots)$ (with other knobs set at their current values).
We then feed the input $I(\cdots v_i \cdots)$ through the DNN $D$ to get the corresponding output $D(I(\cdots v_i \cdots))$ as the inference results.

\outputgrad aims to capture how much a small change $\Delta v_i$ on the current value of $v_i$ \textit{flips} the DNN-returned confidence scores from below (or above) the confidence threshold $\theta$ to above (or below) the confidence threshold $\theta$. 
Thus \outputgrad can be expressed as
\begin{equation}
\footnotesize
    \frac{\Delta N}{\Delta v_i} = \frac{ |N(D(I(\cdots v_i + \delta \cdots) -  N(D(I(\cdots v_i \cdots)|}{\Delta v_i},
\end{equation}
where
\begin{equation}
\footnotesize
    N(res) = \sum_{score\in res.scores} step(score - \theta).
\end{equation}
Here, $res$ is the inference results, $res.scores$ refer to the confidence scores inside the inference results and $step$ is a function defined as $step(x)=1$ for $x>0$ and $step(x)=0$ for $x\leq 0$.



\mypara{Leveraging DNN differentiability}
As shown in \S\ref{subsec:differnetiability}, calculating \outputgrad (\ie $\frac{\Delta N}{\Delta v_i}$) naively would require two separate inference on the same data input with two different configurations. 
To save the extra inference, \name instead harnesses the differentiability of the DNN.
Intuitively, \outputgrad (how DNN output changes with respect to the knob change) can be decoupled into two parts: (1) how DNN output changes with respect to the DNN input change, and (2) how DNN input changes with respect to the knob change.
% how changing system knobs alters the DNN input, and then calculate how changing the DNN input alters the DNN output.
Formally, we can approximate $\frac{\Delta N}{\Delta v_i}$ by following the chain rule:
\begin{equation}
    \frac{\Delta N}{\Delta v_i} \approx \frac{\partial N}{\partial I} \cdot \frac{\Delta I}{\Delta v_i},
\end{equation}
where $I$ is the input to the DNN. 

The first term $\frac{\partial N}{\partial I}$ is the partial derivative of $N$ with respect to $I$, which can be calculated analytically by performing backpropagation on the function $N(D(I))$.
To make the $step$ function (which we use to define function $N$) differentiable, \name uses $sigmoid(k\cdot x)$ to approximate the function $step(x)$, where $sigmoid$ is the sigmoid function $\frac{1}{1+\exp(-x)}$. These two functions are almost identical when $k$ is large. In \name we take $k=20$. 
The second term can be calculated by simply calculating the change of the DNN input, \ie $\frac{I(\cdots v_i+\Delta v_i \cdots)-I(\cdots v_i \cdots )}{\Delta v_i}$.


Mathematically, this approximation is correct, but it may not work in practice, since the ``chain rule'' only holds when the change of the knob value $\delta$ is infinitesimally small. Unfortunately, in practice, the knobs can only be chosen from a given set of values, so $\Delta v_i$ cannot be arbitrarily small (\eg since frame rate must be integers, the smallest change on frame rate must be at least one).

\name uses a pragmatic approach to address this problem. 
The intuition is that each knob must have a ``direction'' along which any change should only increase or keep the accuracy. 
This is because these knobs trade resource usage for accuracy, so when changing the knob value incurs higher resource usage, it tends to improve accuracy as well.
For instance, increasing the frame rate should rarely lower accuracy. 
Based on the intuition, we redefine \outputgrad as 
\begin{equation}
    \frac{\partial N}{\partial v_i} = \left| \frac{\partial N}{\partial I} \right| \cdot \left|\frac{\Delta I}{\Delta v_i}\right|,
\end{equation}
\kt{Talk about why this equation resolves the limitation}
where $|A|$ here means taking the absolute value of every element inside $A$.
This way, as long as $\Delta v_i$ changes in the direction of improving accuracy, this definition at least guarantees that $N$ always increases in the right direction.

\begin{comment}


\subsection{Calculating \outputgrad}


\mypara{Notations}
Assume the system contains $n$ knobs: $k_1, \cdots, k_n$ and the current values of them are $v_1,\cdots, v_n$.
The current configuration of the system is $(v_1,\cdots,v_n)$.
We will focus on how to calculate the \outputgrad for the $i^{th}$ knob, whose current value is $v_i$.
% So we denote the configuration of the system as $(\cdots v_i \cdots)$ to focus on the value of $i^{th}$ knob $v_i$.
Let the input processing function be $I$, which maps the configuration $(\cdots v_i \cdots)$ to the input of the DNN $I(\cdots v_i \cdots)$ (with other knobs set at their current values).
The DNN $D$ then feeds the input $I(\cdots v_i \cdots)$ and get the corresponding output $D(I(\cdots v_i \cdots))$ as the inference results.

\mypara{Naive way of measuring \outputgrad}
\outputgrad aims to capture how much a small change in the current value of each knob \textit{flips} the DNN-returned confidence scores from below (or above) the confidence threshold $\theta$ to above (or below) the confidence threshold $\theta$. 
A naive way to measure \outputgrad is by counting the number of flips via measuring the change of number of the confidence scores above the threshold, where we count the number of the confidence scores above the threshold using the following function:
\begin{equation}
\footnotesize
    N(res) = \sum_{score\in res.scores} step(score - \theta),
\end{equation}
where $res$ is the inference results, $res.scores$ refer to the confidence scores inside the inference results and $step$ is a function defined as $step(x)=1$ for $x>0$ and $step(x)=0$ for $x\leq 0$.
As a result, the naive definition of \outputgrad is
\begin{equation}
\footnotesize
    \frac{\Delta N}{\Delta v_i} = \frac{ |N(D(I(\cdots v_i + \delta \cdots) -  N(D(I(\cdots v_i \cdots)|}{\delta},
\end{equation}
where $\delta$ is a small change on the $i^{th}$ knob, and $|\cdot|$ refers to the absolute value function.


Other than running inference twice, this naive definition has another problem: if a confidence score changes from less than $\theta$ to greater than $\theta$, and another confidence score changes in the opposite direction, there should be two flips in total.
But as changing from less than $\theta$ to greater than $\theta$ increases $N$ and changing in another way decreases $N$, these two changes cancel each other out, and the value of $N$ actually does not change.


\mypara{Leveraging DNN differentiability}
As shown in \S\ref{subsec:differnetiability}, calculating \outputgrad (\ie $\frac{\Delta N}{\Delta v_i}$) in the naive way results in extra DNN inference.
To reduce such extra inference, \name instead leverages the differentiability of the DNN to calculate \outputgrad.
Intuitively, in order to calculate how DNN output changes with respect to the knob change (\ie \outputgrad), we can calculate how DNN output changes with respect to the DNN input change, and then study how DNN input changes with respect to the knob change.
% how changing system knobs alters the DNN input, and then calculate how changing the DNN input alters the DNN output.
Formally, we can approximate\footnote{It is an approximation since the ``chain rule'' only holds when the change of the knob value $\delta$ is sufficiently small. However, in practice the knobs can only be chosen from a given set of values, thus $\delta$ cannot be arbitrarily small.} $\frac{\Delta N}{\Delta v_i}$ by following the chain rule:
\begin{equation}
    \frac{\Delta N}{\Delta v_i} \approx \frac{\partial N}{\partial I} \cdot \frac{\Delta I}{\Delta v_i},
\end{equation}
where $I$ is the input to the DNN. The first term $\frac{\partial N}{\partial I}$ is the partial derivative of $N$ with respect to $I$, which can be calculated analytically by performing backpropagation on the function $N(D(I))$\footnote{As the $step$ function in $N$ is not differentiable, \name instead uses $sigmoid(k\cdot x)$ to approximate the function $step(x)$, where $sigmoid$ is the sigmoid function $\frac{1}{1+\exp(-x)}$. These two functions are almost identical when $k$ is large. In \name we take $k=20$.}, and the second term can be calculated by simply calculating the change of the DNN input, \ie $\frac{I(\cdots v_i+\delta \cdots)-I(\cdots v_i \cdots )}{\delta}$.



Recall the counter-example of the strawman way of calculating \outputgrad: the change made to the number of confidence scores above the confidence threshold might cancel each other.
To resolve this issue, we let any change on the DNN input (\ie $I(\cdots v_i+\delta \cdots)-I(\cdots v_i \cdots )$) always result in the change of the number of confidence scores above.
Mathematically, we achieve this goal by defining \outputgrad as:
\begin{equation}
    \frac{\partial N}{\partial v_i} = \left| \frac{\partial N}{\partial I} \right| \cdot \left|\frac{\Delta I}{\Delta v_i}\right|,
\end{equation}
where $|A|$ here means taking the absolute value of every elements inside $A$.



\end{comment}




% \mypara{Limitation of \outputgrad}
% Cannot optimize for hidden objects.





% Then, \accgrad of the $i^{th}$ knob $k_i$ is defined as:
% \begin{equation}
%     \frac{\partial Acc}{\partial v_i} = \frac{Acc(D(In_t(\cdots v_i \cdots)) - Acc(D(In_t(\cdots v_i+\delta  \cdots))}{\delta},
% \end{equation}
% where $v_i$ and $v_i+\delta$ is two consecutive values of knob $k_i$.


% With this gradient. \name can quickly adapt to optimal by re-allocating the resource from low \accgrad knobs to knobs with high \accgrad.

\subsection{\outputgrad correlates with accuracy change}
\label{subsec:correlation}

\outputgrad, multiplied by the change of the knobs, has a practical implication that it nicely correlates with how the absolute value of the accuracy changes with knobs.
Intuitively, the confidence threshold of a detection or classification result determines whether this detection or classification result is accepted (and thus participating in the accuracy calculation) or rejected (and thus having no effect on the accuracy).

We can formalize this intuition as follows. We multiply \outputgrad by the change of the $i^{th}$ knob:
\begin{equation}
    \frac{\partial N}{\partial v_i} \cdot |\Delta v_i| = \left| \frac{\partial N}{\partial I} \right| \cdot \left|\frac{\Delta I}{\Delta v_i}\right| \cdot |\Delta v_i| = \left| \frac{\partial N}{\partial I} \right|  \cdot |\Delta I|.
\end{equation}
Note that $\Delta v_i$ is a scalar value.
We find that the metric $Proxy = \left| \frac{\partial N}{\partial I} \right|  \cdot |\Delta I|$ nicely correlates with the absolute change of accuracy $|\Delta Acc|$.
As shown in Figure~\ref{fig:proxy}, we show that $Proxy$ (X-axis) correlates with the absolute value of accuracy change (Y-axis) on a three-second video chunk.
The reason we pick three-second video chunk is to show that the correlation between \outputgrad and the accuracy is already significant within just a short video chunk.

\begin{figure}[t]
    \centering
    % \includegraphics[width=0.5\columnwidth]{figs/placeholder-eval-overall-1.pdf}
    % \subfloat[][\centering{Object detection\\~~~~(Dashcam)}]
    % {
    %     \includegraphics[width=0.24\textwidth]{figs/detection_dashcam_FPN.pdf}
    %     \label{subfig:1}
    % }
        \includegraphics[width=0.45\columnwidth]{figs/proxy_encode.pdf} 

    %  \subfloat[][6 knobs]
    % {
    %     \includegraphics[width=0.32\columnwidth]{figs/rgb_video_e2e_8x8.pdf} 
    %     \label{subfig:1}
    % }
    
    
    \tightcaption{$Proxy$ (X-axis) nicely correlates with the absolute value of accuracy change $\Delta Acc$ (Y-axis).}
    \label{fig:proxy}
\end{figure}








% We compare \accgrad to two main lines of work: profiling-based approach and DNN-driven approach, and illustrate the rationales of why \accgrad is better.



% \mypara{Comparing to profiling-based approach}
% \accgrad can be generated without extra inference (we will illustrate how to calculate \accgrad without extra inference in \S\ref{??}), while profiling-based approach needs to perform multiple extra inferences to obtain the profile.
% To put this cost into context, take AWStream~\cite{awstream}, a profiling-based system analytics as an example.
% In AWStream, fully profiling just \textit{one-second} video on three video encoding knobs already takes \textit{52} seconds of inference\footnote{We define one second of inference as inference on a 30FPS video}.

% As a result, when the server-side compute is limited, the profiling-based approach either need to profile only a constrained subset of configurations (\eg downsample the configuration space by 50x), resulting in selecting sub-optimal configurations (and thus sub-optimal resource-accuracy trade-off), or need to profile much less frequently (\eg only profile 1/50 worth of data), making these systems unable to update the outdated profile, thus achieving sub-optimal resource-accuracy trade-off.


% \mypara{Comparing to DNN-driven approach}

% \kt{main argument, TBD}





% To obtain the knob-accuracy impact in real-time, we present \name. We first show that knob-accuracy impact is a better feedback for the underlying system, and discuss the APIs and mechanisms of obtaining accuracy gradient.

% % \subsection{Accuracy gradient as a better predictor}
% \kt{Introduce API}

% To better predict the accuracy, the key is to know the impact of knobs on accuracy in real-time.

% Obtaining knob-accuracy impact enables us to do two things.
% First, it can cheaply identify whether the current configuration is locally optimal or not.
% This is because checking the local optimality is essentially go through each knob and compare between the accuracy gain of changing the knob and the extra delay caused by the knob.
% In other word, we can check the local optimality by directly comparing between the knob-accuracy impact and extra delay.
% Second, it can better estimate the accuracy change of an unknown configuration under the same video content.


% One may worry that knob-accuracy impact will let the system stuck in the local optimal.
% We argue that for one single knob, when it goes from the cheapest value to the most expensive value, the accuracy gain will become smaller but the streaming delay will still grow in a steady pace. 
% As a result, the overall accuracy - delay objective is in general \textit{concave} and have no local optimal.


% \subsection{Key idea: accuracy-knob gradient}


% \begin{itemize}
%     \item 
%     \accres suggests that the change of accuracy with respect to knob value change can reflect the ability of trading resource for accuracy for each individual knob. 
    
%     \item In order to measure this change, we propose a new metric: \accgrad, defined as the difference of accuracy, divided by the difference of two consecutive values of one knob.
%     \item With \accgrad, \name can quickly adapt to optimal by allocate more resources to those knobs with high \accgrad to improve accuracy, and cut the resource usage of those knobs with low \accgrad to save resource.
%     \item Compared to frequent profiling: avoid extra inference.
%     \item Compared to server-side DNN output: use DNN parameters as a reliable performance estimator.
%     \item Show an example like AccMPEG.
%     % \item Present accuracy gradient as the solution and define accuracy gradient as the diff of accuracy divided by the diff of two consecutive parameter values.
%     % % \item With accuracy gradient, we can prune out those configurations that yeild similar accuracy without extra inference.
%     % % \jc{Gradient -> which parameters does not improve accuracy; which parameters does improve accuracy}
%     % \item First, accuracy gradient can be calculated without extra inference. We will further discuss this in \S\ref{subsec:decoupling}.
%     % \item Second, accuracy gradient can help \name to quickly approach to optimal. With accuracy gradient, \name can identify which parameters have huge impact on accuracy and improve accuracy by adapting these parameters. On the other hand, accuracy gradient also allows \name to identify which parameters have little impact on accuracy and save resource usage from these parameters.
% \end{itemize}

% \subsection{Calculating \accgrad}
% \label{subsec:calculate-accgrad}


% However, calculating \accgrad directly incurs high overhead.
% This is because calculating \accgrad requires calculating the accuracy change.
% However, calculating accuracy change requires two kinds of extra inference:
% \begin{packeditemize}
%     \item Calculating the accuracy change for one designate knob (\ie calculate the accuracy before and after changing this knob by a small amount $\delta$, and calculate the difference of these two accuracy values) requires calculating the accuracy metric first, which requires the inference results under \textit{the most resource-demanding configuration} as the ``ground truth'', resulting in high GPU compute overhead.
%     To put this overhead into context, in Chameleon~\cite{chameleon}, about $\sim$50\% of the overall GPU compute is used to calculate such ground truth.
%     As a result, by removing this overhead, \name can already achieves 2x compute cost reduction compared to Chameleon.
    
%     \item Calculating the accuracy change for multiple knobs requires \name to evaluate the accuracy change on every knob and thus requires extra inference when changing every knob.
%     Further, the number of extra inference \textit{scales} with the number of total knobs.
%     This makes it much difficult for the underlying system to handle more knobs.
% \end{packeditemize}


% To reduce the above two overhead, we first consider reducing the first overhead: how to avoid calculating the ``ground truth'' when calculating the accuracy change for one knob.
% As \accres indicates:
% \begin{itemize}
%     \item \textit{Statistically}, the \textit{sign} of accuracy change is statistically determined by the resource usage before and after changing the knob: the accuracy statistically goes higher if the resource usage is higher after changing, and vise versa.
%     \item \textit{Statistically}, the \textit{magnitude} of accuracy change is positively correlated to the \textit{change} of inference results. If the inference results barely change, the accuracy also barely changes, and vice versa.
% \end{itemize}

% The resource usage before and after changing one designated knob is easy to obtain. 
% Take video quantization parameter (which is widely applied in video analytic systems~\cite{dds,awstream,eaar,chameleon,videostorm,vstore}) as an example.
% If the value of this parameter goes higher, the video is encoded in lower quality and thus the resource usage decreases.
% However, the challenge is to measure the \textit{change} of inference results as inference results might be of different format (\eg a sequence of text in speech translation, several human keypoints in human keypoint detection, etc).


% To handle this challenge, we leverage the following two observations:
% \begin{packeditemize}
%     \item 
%     In DNN-based analytic applications (like autonomous driving and video classification), only those \textit{confident} inference results (\ie the inference results that are of confidence scores higher than a threshold $\theta$) will be counted as true detection results and participant in accuracy calculation.
%     \item 
%     As previous work observes~\cite{dds}, those inference results that are almost detected but not (\ie the confidence scores are slightly below $\theta$) are likely to change the inference results.
% \end{packeditemize}

% To capture these two insights, our proxy to the accuracy change is:
% \begin{align}
%     & |Acc(D(In_t(\cdots v_i \cdots)) - Acc(D(In_t(\cdots v_i+\delta  \cdots))| \\
%     \propto  & |f(D(In_t(\cdots v_i \cdots)) - f(D(In_t(\cdots v_i+\delta  \cdots))|,
% \end{align}
% where $f(x) = \sum_{s\in x.scores} sigmoid(k\cdot (s - \theta))$,  $x.scores$ is the confidence scores of each inference result of $x$, $sigmoid$ is the sigmoid function $sigmoid(x) = 1 / (1 + e^{-x})$, $k$ is a scaling parameter\footnote{In our experiment, we pick $k=20$ as it makes the sigmoid value close to 0.9 when the confidence score is just 0.1 larger than the confidence threshold} and $\theta$ is the confidence threshold.
% This function captures the two above observations. First, this function ``counts'' the number of objects that are above the confidence threshold since the $sigmoid(k\cdot (s - \theta))$ is close to $1$ when the confidence score $s$ is higher than $\theta$ and is close to $0$ when the confidence score is slightly lower than $\theta$.\
% Second, those inference results that are almost detected but not can significantly change the sigmoid value even if their confidence scores is just changed by a little.
% For example, by fixing $k=20$ (which is the default choice of $k$ in \name), the corresponding sigmoid value already changes $0.1$ even when the confidence score just slightly changes from $\theta - 0.01$ to $\theta + 0.01$.




% To reduce the second overhead, we leverage the chain rule of gradient, which says:
% \begin{equation}
%     \frac{\partial Acc}{\partial v_i} = \frac{\partial Acc}{\partial In_t}\cdot \frac{\partial In_t}{\partial v_i}
% \end{equation}
% The first term can be calculated without extra inference, and the second term is not related to DNN inference.














% % \begin{comment}
% % Calculating the knob-accuracy impact in real-time can consumes a lot of resource.
% % For example, a naive way to calculate knob-accuracy impact is to enumerate every knob, change that knob a bit and observe the change of accuracy.
% % However, this requires running the end-to-end system $O(n)$ times, where $n$ is the number of knobs. 
% % \kt{Write a running example here}


% % To overcome this difficulty, our approach is to obtain knob-accuracy impact by get the gradient of knobs with respect to accuracy (we call this gradient \textit{knob-accuracy gradient}).
% % Obtaining knob-accuracy gradient requires us to 
% % To answer this, we use chain rule to decouple the gradient into two parts:
% % $$
% % \frac{\partial Acc}{\partial k_i} = \frac{\partial Acc}{\partial I}\cdot \frac{\partial I}{\partial k_i},
% % $$
% % where $Acc$ means the accuracy function, $k_i$ means the $i^{th}$ knob, $I$ means the input of the DNN\footnote{As both of the two gradient is of matrix format, the $\cdot$ should be the inner product. We use $\cdot$ for simplicity.}.
% % It makes use of two key properties of AI pipelines to drastically reduce the cost of calculating this gradient:
% % \begin{packeditemize}
% %     \item The analytic DNN is analytically differentiable.
% %     \item For a large subset of knobs, obtaining the numerical gradient of the input to DNN with respect to knobs can be done locally on the camera and thus does not require sensor-server communication.
% % \end{packeditemize}
% % \end{comment}



% % \subsection{Calculating accuracy change}

% % \begin{itemize}
% %     \item Previous work use most expensive configuration as the ground truth. Works well for evaluation purpose, but calculating this metric at runtime is too expensive.
% %     \item To give context, \kt{raise some examples}
% %     \item We instead propose a cheap run-time approximation of accuracy: accuracy \textit{proxy}. 
% %     \item The key idea is to estimate the sign and estimate the magnitude.
% %     \item Show the math formula.
% % \end{itemize}

% % \begin{itemize}
% %     \item Trivially calcualte the gradient of accuracy proxy requires extra inference.
% %     \item We make several assumptions to remove the extra cost.
% % \end{itemize}



% \subsection{Deriving optimal configuration}

% By exposing \accgrad, \name allows the user to derive the optimal configuration.

% \mypara{Objective function} 
% The objective function of \name is $$Obj(c) = Acc(D(In_t(c))) - \lambda Delay(c),$$ where $c$ is the configuration, $Acc, D, In_t$ is the accuracy function, the DNN, the DNN input correspondingly, $Delay$ is the delay function and $\lambda$ trades between accuracy and end-to-end delay: higher $\lambda$ results in lower end-to-end delay but also lowers the accuracy.

% By optimizing the objective function above, the configuration $c$ that \name gets will be optimal (if $c$ lies on a sub-optimal tradeoff, it means that there is another configuration $c'$ that has higher accuracy and/or lower delay. This makes $Obj(c') > Obj(c)$, which contradicts with the fact that $c$ optimizes the objective function.)




% \mypara{Obtaining \delaygrad}

% \mypara{Obtaining optimal configuration} To illustrate how \name optimizes the objective function $Obj(c)$ above using \accgrad, we use an simple example, where the configuration of the system $c$ is made up of two knobs $c=(v_1, v_2)$, where $v_1\in \{0,1,2\}$ and $v_2\in \{1,2,3\}$ are two knobs of the underlying system.
% \name first creates two variables\footnote{The reason of creating these two variables is enable the use of widely-used gradient-based optimizers as these optimizers typically assumes the variable to be continuous.} $0 \leq v_1' \leq 2$ and $1\leq v_2' \leq 3$.
% When running the analytic system, \name obtain the value $v_1, v_2$ of the knobs of the underlying system by a mapping function $map$.
% This mapping function $map$ maps, say $v_1'$, back to $v_1$ by choosing the value from the knob values of $v_1$ (\ie $\{1,2,3\}$) such that is closest to $v_1'$.
% Assume currently $v_1' = 0.3$, $v_2' = 2.7$.
% As a result, we have $v_1 = map(v_1'; \{0,1,2\}) = map(0.3; \{1,2,3\}) = 1$, and $v_2 = map(v_2'; \{1,2,3\}) = map(2.7; \{1,2,3\}) = 3.$
% After running the analytic system, \name obtains \accgrad and \delaygrad for $v_1, v_2$.
% \name then assign the gradient of $v_1, v_2$ to $v_1'$, $v_2'$, optimizes $v_1', v_2'$  through Adam optimizer (a widely-used optimizer~\cite{??,??}) and truncates $v_1', v_2'$ so that they satisfy $0 \leq v_1' \leq 2$ and $1\leq v_2' \leq 3$.

% \name allows each knob to take any value between the smallest knob value to the largest knob value.
% When inference, \name will then pick the closest value inside all knob values that the underlying system accepts as the chosen knob value.
% For example, say for the knob $k_1$, the underlying system accepts $k_1=1,2,3$. Then \name allows $k_1$ to be any value inside the interval $[1,3]$.
% But 
% \name maximizes the objective function above through Adam optimizer~\cite{adam}, a commonly used optimizer for non-convex optimization~\cite{??}.



==> gradient_v3.tex <==

% \tightsection{\outputgrad}


% \subsection{Estimate accuracy change via DNN differentiability}

% \begin{itemize}
%     \item The key question of quickly adapting to the optimal configuration with no extra inference is: for arbitrary configuration change $\Delta c$, if the configuration changes from $c$ to $c+\Delta c$, how to know the accuracy improvement $Acc(c+\Delta c) - Acc(c)$ without extra DNN inference?
%     % how to estimate the accuracy improvement if the configuration changes. In other word, how to estimate  from current configuration $c$ to another configuration $c+\Delta c$. In other word, how to estimate $Acc(c+\Delta c) - Acc(c)$ without evaluating $Acc(c+\Delta c)$?
    
%     \kt{Write the expensive configuration here}
%     \item An ideal way of answering this question is to harness DNN differentiability and calculate \accgrad $\frac{\partial Acc}{\partial c}$. With this gradient, we can estimate the accuracy change by
%     $$Acc(c+\Delta c) - Acc(c) = \frac{\partial Acc}{\partial c} \cdot \Delta c.$$
    
%     \item However, calculating such \accgrad requires the access of ``ground-truth'', which introduces non-trivial overhead.
    
%     \item We demonstrate that \accgrad is equivalent to \outputgrad with some assumptions (\S\ref{??}).
%     We empirically evaluate these assumptions and find these assumptions hold statistically.
%     Further, we demonstrate that accuracy change estimated by \outputgrad linearly correlates with the real accuracy change (\S\ref{??}).
    

% \end{itemize}

% \subsection{\accgrad is equivalent to \outputgrad}

% In this section, we focus the discussion on object detection with a simple accuracy function (counting the number of correctly-detected objects).
% The discussion process is similar in other applications.


% Mathematically, we use $Acc(res(c), res_{hq}),$ to represent the accuracy function, where $res(c)$ is the inference results generated by configuration $c$, and $res_{hq}$ is the inference result under the most resource-consuming configuration. As our accuracy function is counting the number of correctly-detected objects, we write:
% \begin{align*}
% Acc(res(c), res_{hq})=\sum_{ele(c)\in res(c)} step(ele(e).conf-\theta)\cdot correct(ele, res_{hq}),
% \end{align*}
% where $ele$ is one element assigned with a confidence score (\eg an object in object detection, a pixel in semantic segmentation) inside the inference result $res$ and $correct$ is used to decide whether $ele$ counts as an detected element in $res_{hq}$.
% We assume that the elements above the confidence threshold $\theta$ are correctly detected (we will verify this assumption in the next section).
% In other word, $correct(ele(c), res_{hq})$ always equals to 1.
% % , which is defined as follow in object detection application:
% % \begin{align*}
% % correct(ele(c), res_{hq})=[\max_{ele_{hq}\in res_{hq}, ele_{hq}.conf > \theta}{ IoU(ele(c), ele_{hq})}>0.5]
% % \end{align*}

% As a result, the accuracy function is equals to counting the number of objects (we denote this number as $N$) detected in the inference result $res(c)$. In other word,
% \begin{align*}
%     Acc(res(c), res_{hq}) = N(res(c)) = \sum_{ele(c)\in res(c)} step(ele(e).conf-\theta).
% \end{align*}

% % We assume that for those e

% % As the function above is a piece-wise constant function, the gradient of it with respect to $c$ is $0$. In other word, we write:
% % \begin{align*}
% %     \frac{\partial correct}{\partial c}=0.
% % \end{align*}

% % As a result, we write
% % \begin{align*}
% % &|\partial Acc(res,res_{hq})| \\
% % &= |\partial (\sum_{i=1}^N step(obj_i(v).conf-\theta) \cdot correct(obj_i(v),res_{hq}))| \\
% % &=|\sum_{i=1}^N \partial (step(obj_i(v).conf-\theta) \cdot correct(obj_i(v),res_{hq}))|\\
% % &=|\sum_{i=1}^N \partial step(obj_i(v).conf-\theta) \cdot correct(obj_i(v),res_{hq})|\\
% % &\leq |\sum_{i=1}^N \partial step(obj_i(v).conf-\theta) \cdot 1|\\
% % &=|\partial N(res)|
% % \end{align*}



% % Here $N(res)=\sum_{i=1}^Nstep(obj_i(v).conf-\theta)$ is the number of confidence scores above the threshold. This metric does not rely on the ground truth anymore.

% % Assumption: $|\partial Acc|=|\partial N|$, which means that there is no false positive in the inference results.

% As a result, we have
% \begin{align*}
%     \frac{\partial Acc(res(c);res_{hq})}{\partial c}=\frac{\partial N(res(c))}{\partial c},
% \end{align*}
% which implies that \accgrad is equals to \outputgrad.

% \subsection{Calculating \outputgrad}

% % Thus, we calculate

% % $$
% % |\partial Acc(D(I(v)),D(I(v_{hq})))|= |\partial N(D(I(v)))|=|\frac{\partial N\circ D}{\partial I}\cdot \frac{\partial I}{\partial v_1} | = |\frac{\partial N\circ D}{\partial I}\cdot \frac{\partial I}{\partial v_1} |
% % =|Outputgrad_{v_1}|
% % $$

% % where we define $Outputgrad_{v_1}= \frac{\partial N\circ D}{\partial I}\cdot \frac{\partial I}{\partial v_1}\bigg|_{v=(0,0)}$

% % We assume that $\partial Acc>0.$ so we have

% % $$
% % \frac{\partial Acc(D(I(v)),D(I(v_{hq})))}{\partial v_1}=Outputgrad_{v_1}
% % $$







% \subsection{Empirical verifications of the assumptions}


% Statistically verify these assumptions.


% %  is to estimate how the accuracy $Acc$ changes when the configuration $c$ change from $c$ to $c+\Delta c$ via $\frac{\partial Acc}{\partial c}\cdot \Delta c.$
% % We first show that, with some assumptions, $\frac{\partial Acc}{\partial c} = \frac{\partial O}{\partial c}$. 
% % We then show that these assumptions, though not strictly holds, are still maintaining highly authentic whem 

% % is to calculate the gradient of accuracy $Acc$ with respect to the knob values $v$ (\ie 


% % In this section, we introduce the way \name calculates \outputgrad and show the correlation between \outputgrad and the accuracy change.



% % \jc{Talk about the property of \outputgrad}





% \tightsubsection{Calculating \outputgrad}

% \mypara{Notations}
% Assume the system contains $n$ knobs: $k_1, \cdots, k_n$ and the current values of them are $v_1,\cdots, v_n$.
% The current configuration of the system is $(v_1,\cdots,v_n)$.
% We will focus on how to calculate the \outputgrad for the $i^{th}$ knob, whose current value is $v_i$.
% % So we denote the configuration of the system as $(\cdots v_i \cdots)$ to focus on the value of $i^{th}$ knob $v_i$.
% Let the input processing function be $I$, which maps the configuration $(\cdots v_i \cdots)$ to the input of the DNN $I(\cdots v_i \cdots)$ (with other knobs set at their current values).
% We then feed the input $I(\cdots v_i \cdots)$ through the DNN $D$ to get the corresponding output $D(I(\cdots v_i \cdots))$ as the inference results.

% \mypara{A strawmen definition}
% \outputgrad aims to capture how much a small change $\Delta v_i$ on the current value of $v_i$ \textit{flips} the DNN-returned confidence scores from below (or above) the confidence threshold $\theta$ to above (or below) the confidence threshold $\theta$. 
% Thus, a strawmen definition of \outputgrad would be counting the change of the amount of above-threshold confidence scores:
% \begin{equation}
% \footnotesize
%     \bigg|\frac{\Delta N}{\Delta v_i}\bigg| = \bigg|\frac{ N(D(I(\cdots v_i + \delta \cdots) -  N(D(I(\cdots v_i \cdots)}{\Delta v_i}\bigg|,
% \end{equation}
% where
% \begin{equation}
% \footnotesize
%     N(res) = \sum_{score\in res.scores} step(score - \theta).
% \end{equation}
% Here, $res$ is the inference results, $res.scores$ refer to the confidence scores inside the inference results and $step$ is a function defined as $step(x)=1$ for $x>0$ and $step(x)=0$ for $x\leq 0$.
% We take the abosolute value on both side as the number of flips are always positive.

% \mypara{Improve the strawmen definition}
% However, the strawmen definition above has one limitation: as $N$ only captures the number of above-threshold confidence scores, if two of the confidence scores change from below/above the threshold to above/below the threshold, the change of $N$ will be zero, but the change of the DNN inference results is non-zero.

% To study the cause of limitation above,  we rewrite the definition of $\Delta N$ using the fundamental theorem of calculus:
% \begin{equation}
%     \Delta N = \int_{v_i}^{v_i+\delta} \frac{\partial N}{\partial v_i}\mathbf{d} v_i.
% \end{equation}
% When the change of the knob value $v_i$ alters the confidence score from below/above the threshold to above/below the threshold, the gradient $\frac{\partial N}{\partial v_i}$ will be positive/negative. 
% % However, when the confidence score changes from above-threshold to below-threshold, the gradient $\frac{\partial N}{\partial v}$ will be negative.
% As a result, when we integrate over the gradient term $\frac{\partial N}{\partial v_i}$, the positive part of the gradient and the negative part of the gradient cancel each other. This triggers the limitation mentioned above.

% To address this limitation, we only need to make the gradient term always non-negative. In other word, we define $\Delta N$ as:
% \begin{equation}
%     \Delta N = \int_{v_i}^{v_i+\delta} \left|\frac{\partial N}{\partial v_i}\right|\mathbf{d} v_i.
%     \label{eq:accgrad-definition}
% \end{equation}
% % However, the gradient term $\frac{\partial N(res)}{\partial I}$ can be either positive (when the number of above-threshold confidence scores inside the inference results $res$ increases) or negative (when the number decreases).
% % As a result, when we integrate over the gradient term $\frac{\partial N(res)}{\partial I}$, the positive effect and negative effect will cancel each other, resulting in no change


% % To handle this challenge, the key is to make sure that the change of $N$, no matter decreasing or increasing, will always be counted positively as a change. To do so, we put on an absolute value on the change of N.
% % \begin{equation}
% % \footnotesize
% %     \frac{\Delta N}{\Delta v_i} = \int_{v_i}^{v_i+\delta} \bigg|\frac{\partial N(D(I(\cdots u_i \cdots)))}{\partial u_i}\bigg| \mathbf{d} u_i
% %     % \frac{ |N(D(I(\cdots v_i + \delta \cdots) -  N(D(I(\cdots v_i \cdots)|}{\Delta v_i},
% % \end{equation}



% \mypara{Leveraging DNN differentiability}
% However, calculating output-knob
% As shown in \S\ref{subsec:differnetiability}, calculating \outputgrad (\ie $\frac{\Delta N}{\Delta v_i}$) naively would require two separate inference on the same data input with two different configurations. 
% To save the extra inference, \name instead harnesses the differentiability of the DNN.
% Intuitively, \outputgrad (how DNN output changes with respect to the knob change) can be decoupled into two parts: (1) how DNN output changes with respect to the DNN input change, and (2) how DNN input changes with respect to the knob change.
% % how changing system knobs alters the DNN input, and then calculate how changing the DNN input alters the DNN output.
% Formally, we can approximate $\frac{\Delta N}{\Delta v_i}$ by following the chain rule:
% \begin{equation}
%     \frac{\Delta N}{\Delta v_i} \approx \frac{\partial N}{\partial I} \cdot \frac{\Delta I}{\Delta v_i},
% \end{equation}
% where $I$ is the input to the DNN. 

% The first term $\frac{\partial N}{\partial I}$ is the partial derivative of $N$ with respect to $I$, which can be calculated analytically by performing backpropagation on the function $N(D(I))$.
% To make the $step$ function (which we use to define function $N$) differentiable, \name uses $sigmoid(k\cdot x)$ to approximate the function $step(x)$, where $sigmoid$ is the sigmoid function $\frac{1}{1+\exp(-x)}$. These two functions are almost identical when $k$ is large. In \name we take $k=20$. 
% The second term can be calculated by simply calculating the change of the DNN input, \ie $\frac{I(\cdots v_i+\Delta v_i \cdots)-I(\cdots v_i \cdots )}{\Delta v_i}$.


% Mathematically, this approximation is correct, but it may not work in practice, since the ``chain rule'' only holds when the change of the knob value $\delta$ is infinitesimally small. Unfortunately, in practice, the knobs can only be chosen from a given set of values, so $\Delta v_i$ cannot be arbitrarily small (\eg since frame rate must be integers, the smallest change on frame rate must be at least one).

% \name uses a pragmatic approach to address this problem. 
% The intuition is that each knob must have a ``direction'' along which any change should only increase or keep the accuracy. 
% This is because these knobs trade resource usage for accuracy, so when changing the knob value incurs higher resource usage, it tends to improve accuracy as well.
% For instance, increasing the frame rate should rarely lower accuracy. 
% Based on the intuition, we redefine \outputgrad as 
% \begin{equation}
%     \frac{\partial N}{\partial v_i} = \left| \frac{\partial N}{\partial I} \right| \cdot \left|\frac{\Delta I}{\Delta v_i}\right|,
% \end{equation}
% \kt{Talk about why this equation resolves the limitation}
% where $|A|$ here means taking the absolute value of every element inside $A$.
% This way, as long as $\Delta v_i$ changes in the direction of improving accuracy, this definition at least guarantees that $N$ always increases in the right direction.

% \begin{comment}


% \subsection{Calculating \outputgrad}


% \mypara{Notations}
% Assume the system contains $n$ knobs: $k_1, \cdots, k_n$ and the current values of them are $v_1,\cdots, v_n$.
% The current configuration of the system is $(v_1,\cdots,v_n)$.
% We will focus on how to calculate the \outputgrad for the $i^{th}$ knob, whose current value is $v_i$.
% % So we denote the configuration of the system as $(\cdots v_i \cdots)$ to focus on the value of $i^{th}$ knob $v_i$.
% Let the input processing function be $I$, which maps the configuration $(\cdots v_i \cdots)$ to the input of the DNN $I(\cdots v_i \cdots)$ (with other knobs set at their current values).
% The DNN $D$ then feeds the input $I(\cdots v_i \cdots)$ and get the corresponding output $D(I(\cdots v_i \cdots))$ as the inference results.

% \mypara{Naive way of measuring \outputgrad}
% \outputgrad aims to capture how much a small change in the current value of each knob \textit{flips} the DNN-returned confidence scores from below (or above) the confidence threshold $\theta$ to above (or below) the confidence threshold $\theta$. 
% A naive way to measure \outputgrad is by counting the number of flips via measuring the change of number of the confidence scores above the threshold, where we count the number of the confidence scores above the threshold using the following function:
% \begin{equation}
% \footnotesize
%     N(res) = \sum_{score\in res.scores} step(score - \theta),
% \end{equation}
% where $res$ is the inference results, $res.scores$ refer to the confidence scores inside the inference results and $step$ is a function defined as $step(x)=1$ for $x>0$ and $step(x)=0$ for $x\leq 0$.
% As a result, the naive definition of \outputgrad is
% \begin{equation}
% \footnotesize
%     \frac{\Delta N}{\Delta v_i} = \frac{ |N(D(I(\cdots v_i + \delta \cdots) -  N(D(I(\cdots v_i \cdots)|}{\delta},
% \end{equation}
% where $\delta$ is a small change on the $i^{th}$ knob, and $|\cdot|$ refers to the absolute value function.


% Other than running inference twice, this naive definition has another problem: if a confidence score changes from less than $\theta$ to greater than $\theta$, and another confidence score changes in the opposite direction, there should be two flips in total.
% But as changing from less than $\theta$ to greater than $\theta$ increases $N$ and changing in another way decreases $N$, these two changes cancel each other out, and the value of $N$ actually does not change.


% \mypara{Leveraging DNN differentiability}
% As shown in \S\ref{subsec:differnetiability}, calculating \outputgrad (\ie $\frac{\Delta N}{\Delta v_i}$) in the naive way results in extra DNN inference.
% To reduce such extra inference, \name instead leverages the differentiability of the DNN to calculate \outputgrad.
% Intuitively, in order to calculate how DNN output changes with respect to the knob change (\ie \outputgrad), we can calculate how DNN output changes with respect to the DNN input change, and then study how DNN input changes with respect to the knob change.
% % how changing system knobs alters the DNN input, and then calculate how changing the DNN input alters the DNN output.
% Formally, we can approximate\footnote{It is an approximation since the ``chain rule'' only holds when the change of the knob value $\delta$ is sufficiently small. However, in practice the knobs can only be chosen from a given set of values, thus $\delta$ cannot be arbitrarily small.} $\frac{\Delta N}{\Delta v_i}$ by following the chain rule:
% \begin{equation}
%     \frac{\Delta N}{\Delta v_i} \approx \frac{\partial N}{\partial I} \cdot \frac{\Delta I}{\Delta v_i},
% \end{equation}
% where $I$ is the input to the DNN. The first term $\frac{\partial N}{\partial I}$ is the partial derivative of $N$ with respect to $I$, which can be calculated analytically by performing backpropagation on the function $N(D(I))$\footnote{As the $step$ function in $N$ is not differentiable, \name instead uses $sigmoid(k\cdot x)$ to approximate the function $step(x)$, where $sigmoid$ is the sigmoid function $\frac{1}{1+\exp(-x)}$. These two functions are almost identical when $k$ is large. In \name we take $k=20$.}, and the second term can be calculated by simply calculating the change of the DNN input, \ie $\frac{I(\cdots v_i+\delta \cdots)-I(\cdots v_i \cdots )}{\delta}$.



% Recall the counter-example of the strawman way of calculating \outputgrad: the change made to the number of confidence scores above the confidence threshold might cancel each other.
% To resolve this issue, we let any change on the DNN input (\ie $I(\cdots v_i+\delta \cdots)-I(\cdots v_i \cdots )$) always result in the change of the number of confidence scores above.
% Mathematically, we achieve this goal by defining \outputgrad as:
% \begin{equation}
%     \frac{\partial N}{\partial v_i} = \left| \frac{\partial N}{\partial I} \right| \cdot \left|\frac{\Delta I}{\Delta v_i}\right|,
% \end{equation}
% where $|A|$ here means taking the absolute value of every elements inside $A$.



% \end{comment}




% % \mypara{Limitation of \outputgrad}
% % Cannot optimize for hidden objects.





% % Then, \accgrad of the $i^{th}$ knob $k_i$ is defined as:
% % \begin{equation}
% %     \frac{\partial Acc}{\partial v_i} = \frac{Acc(D(In_t(\cdots v_i \cdots)) - Acc(D(In_t(\cdots v_i+\delta  \cdots))}{\delta},
% % \end{equation}
% % where $v_i$ and $v_i+\delta$ is two consecutive values of knob $k_i$.


% % With this gradient. \name can quickly adapt to optimal by re-allocating the resource from low \accgrad knobs to knobs with high \accgrad.

% \subsection{\outputgrad correlates with accuracy change}
% \label{subsec:correlation}

% \outputgrad, multiplied by the change of the knobs, has a practical implication that it nicely correlates with how the absolute value of the accuracy changes with knobs.
% Intuitively, the confidence threshold of a detection or classification result determines whether this detection or classification result is accepted (and thus participating in the accuracy calculation) or rejected (and thus having no effect on the accuracy).

% We can formalize this intuition as follows. We multiply \outputgrad by the change of the $i^{th}$ knob:
% \begin{equation}
%     \frac{\partial N}{\partial v_i} \cdot |\Delta v_i| = \left| \frac{\partial N}{\partial I} \right| \cdot \left|\frac{\Delta I}{\Delta v_i}\right| \cdot |\Delta v_i| = \left| \frac{\partial N}{\partial I} \right|  \cdot |\Delta I|.
% \end{equation}
% Note that $\Delta v_i$ is a scalar value.
% We find that the metric $Proxy = \left| \frac{\partial N}{\partial I} \right|  \cdot |\Delta I|$ nicely correlates with the absolute change of accuracy $|\Delta Acc|$.
% As shown in Figure~\ref{fig:proxy}, we show that $Proxy$ (X-axis) correlates with the absolute value of accuracy change (Y-axis) on a three-second video chunk.
% The reason we pick three-second video chunk is to show that the correlation between \outputgrad and the accuracy is already significant within just a short video chunk.

% \begin{figure}[t]
%     \centering
%     % \includegraphics[width=0.5\columnwidth]{figs/placeholder-eval-overall-1.pdf}
%     % \subfloat[][\centering{Object detection\\~~~~(Dashcam)}]
%     % {
%     %     \includegraphics[width=0.24\textwidth]{figs/detection_dashcam_FPN.pdf}
%     %     \label{subfig:1}
%     % }
%         \includegraphics[width=0.45\columnwidth]{figs/proxy_encode.pdf} 

%     %  \subfloat[][6 knobs]
%     % {
%     %     \includegraphics[width=0.32\columnwidth]{figs/rgb_video_e2e_8x8.pdf} 
%     %     \label{subfig:1}
%     % }
    
    
%     \tightcaption{$Proxy$ (X-axis) nicely correlates with the absolute value of accuracy change $\Delta Acc$ (Y-axis).}
%     \label{fig:proxy}
% \end{figure}








% % We compare \accgrad to two main lines of work: profiling-based approach and DNN-driven approach, and illustrate the rationales of why \accgrad is better.



% % \mypara{Comparing to profiling-based approach}
% % \accgrad can be generated without extra inference (we will illustrate how to calculate \accgrad without extra inference in \S\ref{??}), while profiling-based approach needs to perform multiple extra inferences to obtain the profile.
% % To put this cost into context, take AWStream~\cite{awstream}, a profiling-based system analytics as an example.
% % In AWStream, fully profiling just \textit{one-second} video on three video encoding knobs already takes \textit{52} seconds of inference\footnote{We define one second of inference as inference on a 30FPS video}.

% % As a result, when the server-side compute is limited, the profiling-based approach either need to profile only a constrained subset of configurations (\eg downsample the configuration space by 50x), resulting in selecting sub-optimal configurations (and thus sub-optimal resource-accuracy trade-off), or need to profile much less frequently (\eg only profile 1/50 worth of data), making these systems unable to update the outdated profile, thus achieving sub-optimal resource-accuracy trade-off.


% % \mypara{Comparing to DNN-driven approach}

% % \kt{main argument, TBD}





% % To obtain the knob-accuracy impact in real-time, we present \name. We first show that knob-accuracy impact is a better feedback for the underlying system, and discuss the APIs and mechanisms of obtaining accuracy gradient.

% % % \subsection{Accuracy gradient as a better predictor}
% % \kt{Introduce API}

% % To better predict the accuracy, the key is to know the impact of knobs on accuracy in real-time.

% % Obtaining knob-accuracy impact enables us to do two things.
% % First, it can cheaply identify whether the current configuration is locally optimal or not.
% % This is because checking the local optimality is essentially go through each knob and compare between the accuracy gain of changing the knob and the extra delay caused by the knob.
% % In other word, we can check the local optimality by directly comparing between the knob-accuracy impact and extra delay.
% % Second, it can better estimate the accuracy change of an unknown configuration under the same video content.


% % One may worry that knob-accuracy impact will let the system stuck in the local optimal.
% % We argue that for one single knob, when it goes from the cheapest value to the most expensive value, the accuracy gain will become smaller but the streaming delay will still grow in a steady pace. 
% % As a result, the overall accuracy - delay objective is in general \textit{concave} and have no local optimal.


% % \subsection{Key idea: accuracy-knob gradient}


% % \begin{itemize}
% %     \item 
% %     \accres suggests that the change of accuracy with respect to knob value change can reflect the ability of trading resource for accuracy for each individual knob. 
    
% %     \item In order to measure this change, we propose a new metric: \accgrad, defined as the difference of accuracy, divided by the difference of two consecutive values of one knob.
% %     \item With \accgrad, \name can quickly adapt to optimal by allocate more resources to those knobs with high \accgrad to improve accuracy, and cut the resource usage of those knobs with low \accgrad to save resource.
% %     \item Compared to frequent profiling: avoid extra inference.
% %     \item Compared to server-side DNN output: use DNN parameters as a reliable performance estimator.
% %     \item Show an example like AccMPEG.
% %     % \item Present accuracy gradient as the solution and define accuracy gradient as the diff of accuracy divided by the diff of two consecutive parameter values.
% %     % % \item With accuracy gradient, we can prune out those configurations that yeild similar accuracy without extra inference.
% %     % % \jc{Gradient -> which parameters does not improve accuracy; which parameters does improve accuracy}
% %     % \item First, accuracy gradient can be calculated without extra inference. We will further discuss this in \S\ref{subsec:decoupling}.
% %     % \item Second, accuracy gradient can help \name to quickly approach to optimal. With accuracy gradient, \name can identify which parameters have huge impact on accuracy and improve accuracy by adapting these parameters. On the other hand, accuracy gradient also allows \name to identify which parameters have little impact on accuracy and save resource usage from these parameters.
% % \end{itemize}

% % \subsection{Calculating \accgrad}
% % \label{subsec:calculate-accgrad}


% % However, calculating \accgrad directly incurs high overhead.
% % This is because calculating \accgrad requires calculating the accuracy change.
% % However, calculating accuracy change requires two kinds of extra inference:
% % \begin{packeditemize}
% %     \item Calculating the accuracy change for one designate knob (\ie calculate the accuracy before and after changing this knob by a small amount $\delta$, and calculate the difference of these two accuracy values) requires calculating the accuracy metric first, which requires the inference results under \textit{the most resource-demanding configuration} as the ``ground truth'', resulting in high GPU compute overhead.
% %     To put this overhead into context, in Chameleon~\cite{chameleon}, about $\sim$50\% of the overall GPU compute is used to calculate such ground truth.
% %     As a result, by removing this overhead, \name can already achieves 2x compute cost reduction compared to Chameleon.
    
% %     \item Calculating the accuracy change for multiple knobs requires \name to evaluate the accuracy change on every knob and thus requires extra inference when changing every knob.
% %     Further, the number of extra inference \textit{scales} with the number of total knobs.
% %     This makes it much difficult for the underlying system to handle more knobs.
% % \end{packeditemize}


% % To reduce the above two overhead, we first consider reducing the first overhead: how to avoid calculating the ``ground truth'' when calculating the accuracy change for one knob.
% % As \accres indicates:
% % \begin{itemize}
% %     \item \textit{Statistically}, the \textit{sign} of accuracy change is statistically determined by the resource usage before and after changing the knob: the accuracy statistically goes higher if the resource usage is higher after changing, and vise versa.
% %     \item \textit{Statistically}, the \textit{magnitude} of accuracy change is positively correlated to the \textit{change} of inference results. If the inference results barely change, the accuracy also barely changes, and vice versa.
% % \end{itemize}

% % The resource usage before and after changing one designated knob is easy to obtain. 
% % Take video quantization parameter (which is widely applied in video analytic systems~\cite{dds,awstream,eaar,chameleon,videostorm,vstore}) as an example.
% % If the value of this parameter goes higher, the video is encoded in lower quality and thus the resource usage decreases.
% % However, the challenge is to measure the \textit{change} of inference results as inference results might be of different format (\eg a sequence of text in speech translation, several human keypoints in human keypoint detection, etc).


% % To handle this challenge, we leverage the following two observations:
% % \begin{packeditemize}
% %     \item 
% %     In DNN-based analytic applications (like autonomous driving and video classification), only those \textit{confident} inference results (\ie the inference results that are of confidence scores higher than a threshold $\theta$) will be counted as true detection results and participant in accuracy calculation.
% %     \item 
% %     As previous work observes~\cite{dds}, those inference results that are almost detected but not (\ie the confidence scores are slightly below $\theta$) are likely to change the inference results.
% % \end{packeditemize}

% % To capture these two insights, our proxy to the accuracy change is:
% % \begin{align}
% %     & |Acc(D(In_t(\cdots v_i \cdots)) - Acc(D(In_t(\cdots v_i+\delta  \cdots))| \\
% %     \propto  & |f(D(In_t(\cdots v_i \cdots)) - f(D(In_t(\cdots v_i+\delta  \cdots))|,
% % \end{align}
% % where $f(x) = \sum_{s\in x.scores} sigmoid(k\cdot (s - \theta))$,  $x.scores$ is the confidence scores of each inference result of $x$, $sigmoid$ is the sigmoid function $sigmoid(x) = 1 / (1 + e^{-x})$, $k$ is a scaling parameter\footnote{In our experiment, we pick $k=20$ as it makes the sigmoid value close to 0.9 when the confidence score is just 0.1 larger than the confidence threshold} and $\theta$ is the confidence threshold.
% % This function captures the two above observations. First, this function ``counts'' the number of objects that are above the confidence threshold since the $sigmoid(k\cdot (s - \theta))$ is close to $1$ when the confidence score $s$ is higher than $\theta$ and is close to $0$ when the confidence score is slightly lower than $\theta$.\
% % Second, those inference results that are almost detected but not can significantly change the sigmoid value even if their confidence scores is just changed by a little.
% % For example, by fixing $k=20$ (which is the default choice of $k$ in \name), the corresponding sigmoid value already changes $0.1$ even when the confidence score just slightly changes from $\theta - 0.01$ to $\theta + 0.01$.




% % To reduce the second overhead, we leverage the chain rule of gradient, which says:
% % \begin{equation}
% %     \frac{\partial Acc}{\partial v_i} = \frac{\partial Acc}{\partial In_t}\cdot \frac{\partial In_t}{\partial v_i}
% % \end{equation}
% % The first term can be calculated without extra inference, and the second term is not related to DNN inference.














% % % \begin{comment}
% % % Calculating the knob-accuracy impact in real-time can consumes a lot of resource.
% % % For example, a naive way to calculate knob-accuracy impact is to enumerate every knob, change that knob a bit and observe the change of accuracy.
% % % However, this requires running the end-to-end system $O(n)$ times, where $n$ is the number of knobs. 
% % % \kt{Write a running example here}


% % % To overcome this difficulty, our approach is to obtain knob-accuracy impact by get the gradient of knobs with respect to accuracy (we call this gradient \textit{knob-accuracy gradient}).
% % % Obtaining knob-accuracy gradient requires us to 
% % % To answer this, we use chain rule to decouple the gradient into two parts:
% % % $$
% % % \frac{\partial Acc}{\partial k_i} = \frac{\partial Acc}{\partial I}\cdot \frac{\partial I}{\partial k_i},
% % % $$
% % % where $Acc$ means the accuracy function, $k_i$ means the $i^{th}$ knob, $I$ means the input of the DNN\footnote{As both of the two gradient is of matrix format, the $\cdot$ should be the inner product. We use $\cdot$ for simplicity.}.
% % % It makes use of two key properties of AI pipelines to drastically reduce the cost of calculating this gradient:
% % % \begin{packeditemize}
% % %     \item The analytic DNN is analytically differentiable.
% % %     \item For a large subset of knobs, obtaining the numerical gradient of the input to DNN with respect to knobs can be done locally on the camera and thus does not require sensor-server communication.
% % % \end{packeditemize}
% % % \end{comment}



% % % \subsection{Calculating accuracy change}

% % % \begin{itemize}
% % %     \item Previous work use most expensive configuration as the ground truth. Works well for evaluation purpose, but calculating this metric at runtime is too expensive.
% % %     \item To give context, \kt{raise some examples}
% % %     \item We instead propose a cheap run-time approximation of accuracy: accuracy \textit{proxy}. 
% % %     \item The key idea is to estimate the sign and estimate the magnitude.
% % %     \item Show the math formula.
% % % \end{itemize}

% % % \begin{itemize}
% % %     \item Trivially calcualte the gradient of accuracy proxy requires extra inference.
% % %     \item We make several assumptions to remove the extra cost.
% % % \end{itemize}



% % \subsection{Deriving optimal configuration}

% % By exposing \accgrad, \name allows the user to derive the optimal configuration.

% % \mypara{Objective function} 
% % The objective function of \name is $$Obj(c) = Acc(D(In_t(c))) - \lambda Delay(c),$$ where $c$ is the configuration, $Acc, D, In_t$ is the accuracy function, the DNN, the DNN input correspondingly, $Delay$ is the delay function and $\lambda$ trades between accuracy and end-to-end delay: higher $\lambda$ results in lower end-to-end delay but also lowers the accuracy.

% % By optimizing the objective function above, the configuration $c$ that \name gets will be optimal (if $c$ lies on a sub-optimal tradeoff, it means that there is another configuration $c'$ that has higher accuracy and/or lower delay. This makes $Obj(c') > Obj(c)$, which contradicts with the fact that $c$ optimizes the objective function.)




% % \mypara{Obtaining \delaygrad}

% % \mypara{Obtaining optimal configuration} To illustrate how \name optimizes the objective function $Obj(c)$ above using \accgrad, we use an simple example, where the configuration of the system $c$ is made up of two knobs $c=(v_1, v_2)$, where $v_1\in \{0,1,2\}$ and $v_2\in \{1,2,3\}$ are two knobs of the underlying system.
% % \name first creates two variables\footnote{The reason of creating these two variables is enable the use of widely-used gradient-based optimizers as these optimizers typically assumes the variable to be continuous.} $0 \leq v_1' \leq 2$ and $1\leq v_2' \leq 3$.
% % When running the analytic system, \name obtain the value $v_1, v_2$ of the knobs of the underlying system by a mapping function $map$.
% % This mapping function $map$ maps, say $v_1'$, back to $v_1$ by choosing the value from the knob values of $v_1$ (\ie $\{1,2,3\}$) such that is closest to $v_1'$.
% % Assume currently $v_1' = 0.3$, $v_2' = 2.7$.
% % As a result, we have $v_1 = map(v_1'; \{0,1,2\}) = map(0.3; \{1,2,3\}) = 1$, and $v_2 = map(v_2'; \{1,2,3\}) = map(2.7; \{1,2,3\}) = 3.$
% % After running the analytic system, \name obtains \accgrad and \delaygrad for $v_1, v_2$.
% % \name then assign the gradient of $v_1, v_2$ to $v_1'$, $v_2'$, optimizes $v_1', v_2'$  through Adam optimizer (a widely-used optimizer~\cite{??,??}) and truncates $v_1', v_2'$ so that they satisfy $0 \leq v_1' \leq 2$ and $1\leq v_2' \leq 3$.

% % \name allows each knob to take any value between the smallest knob value to the largest knob value.
% % When inference, \name will then pick the closest value inside all knob values that the underlying system accepts as the chosen knob value.
% % For example, say for the knob $k_1$, the underlying system accepts $k_1=1,2,3$. Then \name allows $k_1$ to be any value inside the interval $[1,3]$.
% % But 
% % \name maximizes the objective function above through Adam optimizer~\cite{adam}, a commonly used optimizer for non-convex optimization~\cite{??}.



==> intro_v2.tex <==
\section{Introduction}
Deep-neural-network-based (DNN-based) analytics on data streams (\eg video
streams or LiDAR feeds) are everywhere. This inspires system research for
these applications.
\jc{can we cite some dnn-based analytics systems use cases, where the input distribution varies over time, in terms of frequency of object occurrences, shape/size, etc? be as concrete as possible please}

We observe that these systems expose an \textit{increasing} number of internal knobs.
The underlying trend that drives this increase is two-fold (further discussion in \S\ref{subsec:numer_of_knobs}). First, these systems need to develop new knobs to not only provide accurate analytic results under all kinds of resource availability due to heterogeneous deployment settings, but to also handle new emerging applications (\eg LiDAR-based object detection for autonomous driving and infrared-based human detection for night-time security monitoring).
Second, as the need of DNN-based analytics quickly grow, these systems need to partition existing knobs to a more fine-grained version to support more concurrent DNN-based analytic jobs.

% % redirected enumerate to packedenumerate for reformater in macro.tex. DON'T
% % CHANGE!
% \begin{enumerate}
%   \item 
% As DNN-based analytics are deployed on heterogeneous deployment settings that have different types of resource budgets, this requires the corresponding systems to propose new knobs in order to fit into
% different resource budgets. Take video analytics as an example. If the
% user analyzes the video feeds locally by a compute-constrained mobile
% phone, the main focus for the systems is to fit into the compute budget
% of the phone (\eg by skipping those frames that are highly similar to
% their previous frames~\cite{reducto,glimpse}). However, if the user
% instead streams the video feeds to a GPU-equipped server through a
% bandwidth-limited LTE network, the main focus is instead fitting into
% the limited LTE bandwidth (\eg by performing video
% compression~\cite{accmpeg,vigil,glimpse,reducto}).

%   \item As DNN-based analytics quickly expand, the corresponding systems need to
%         partition existing knobs into more fine-grained version to capture more
%         resource-saving opportunities. Take video-based vehicle detection as an
%         example. Chameleon~\cite{chameleon} and AWStream~\cite{awstream}
%         identify that the system only need to encode the video in a high
%         encoding quality when the vehicle appears. To further explore the
%         potential of varying video encoding quality, the following
%         work~\cite{dds,eaar,accmpeg} finds that a lot of areas in the video do
%         not need to be encoded in high quality (\eg the areas that contain
%         non-vehicle-related backgrounds like trees and buildings) and proposes
%         fine-grained spatial encoding quality to capture this opportunity.
%   \item Since new applications quickly emerge (\eg LiDAR-based object detection,
%         Infrared-based human detection \kt{a bunch of citations here}), this requires the deep learning systems
%         to develop new knobs (or even developing new system components) to fit
%         into the need of different applications. For example, in order to handle
%         LiDAR data, people are proposing new encoding standard and new
%         knobs~\cite{MPEG-point} to efficiently encode and process LiDAR data.
%         \roy{I understand you are trying to distinguish old types of application
%         and new ones, but I still feel the first and third items are kind of
%         repetitive? Both items are trying to say there is the need for new
%         knobs, right? Maybe merge them into one?}
% \end{enumerate}

Not only the number of knobs are huge, these knobs also need to be timely adapted~\cite{awstream,chameleon,dds,eaar,elf} due to input data change or resource budget change in order to achieve high inference accuracy.
Thus, the research question is: how to navigate the large configuration space (\ie all possible choices of knob values) and and pick the optimal configuration that generates accurate inference results under the current resource budget?

The first way to address this problem is to \textit{frequently profile} the
system with different configurations to obtain their resource usage and
inference accuracy, and then pick the configuration that meets the resource
budget and generates the most accurate inference results~\cite{chameleon,awstream,vstore,videostorm}. However, this approach
needs to analyze extra configurations to obtain the profile, thus incurring \textit{extra} inference.


The other approach performs no extra inference and instead, derive the
configuration from recent DNN outputs (including intermediate outputs) through cheap heuristics~\cite{dds,eaar,elf} or through DNN-based configuration generator~\cite{accmpeg,casva}). 
However, there can be many configurations that meet the resource budget. 
Without profiling most of them, it is difficult to separate the configurations that yield similar DNN output from those that yield more accurate DNN output by merely looking at recent DNN outputs.
As a result, this approach waste resource on those configurations that yield similar DNN output and thus cannot quickly adapt to the optimal configuration.


In addition, the previous work in this approach designs hand-crafted heuristics catered only for individual applications or configurations. 
Take video object detection as an example. 
DDS~\cite{dds} analyzes the video and then resend those part of the video that may contain objects in higher fidelity.
As the resending part of the video is generated by leveraging the output of a specific DNN component (region proposal) that aims to facilitate object detection, this heuristics cannot be reused for tasks like video classification.
Moreover, this heuristics cannot be reused to for the knobs in frame discarding techniques (\ie discarding those frames that produces similar inference results compared to previous frames~\cite{vigil,glimpse,reducto}), since its adaptation logic (\ie resending part of the video that may contain objects) happens \textit{after} DNN inference while frame filtering need to be performed \textit{before} DNN inference to save GPU compute cost.


An ideal configuration adaptation systems should meet these two
requirements: 1. quickly adapt to optimal configuration in a large configuration
space without extra inference 2. minimum assumption to the underlying system

\jc{i guess the rest of the intro haven't been updated since last wednesday. just to recap, here's the flow:
\begin{packeditemize}
    \item start with a new abstraction, \accgrad, to more efficiently adapt configurations than prior schemes, especially in a large configuration space, and why?
    we present \name, the first efficient implementation of \accgrad
    we should clarify that prior work could expose this abstraction as well, but they suffer high overhead (why?). 
    \item \name approximates \accgrad based on two observations: 
    (1) the values of each configuration can be ordered in a way that \fillme, and
    (2) the more changes of confidence scores around the threshold, the more accuracy will change.
    \item based on the two observations, \name does \fillme
    \item operators can use \name to tune a range of configurations that influences dnn input. this class of config covers many existing systems. but notably, this doesn't cover \fillme (may point to a synergy with recent online learning papers like ekya --- in some sense, they also handle input drift, but they choose to retrain the model, and our approach is more lightweight.)
\end{packeditemize}}

We present our system: \name, which meets these two requirements. 
To quickly adapt to optimal configuration, \name calculates the \textit{gradient} of accuracy with respect to each knob (hereinafter \accgrad, defined as the accuracy change if changing one knob valued by a little).
% leverages a property of DNN-based analytic system knobs: for most of the knobs, if changing the value of one knob results in spending more (or less) resource, the corresponding inference result would statistically become more (or less) accurate.
% This property suggests that each knob is able to \textit{trade resource for accuracy}.
% To quantitatively measure this ability, \name calculates the \textit{gradient} of accuracy with respect to each knob (hereinafter \accgrad, defined as how changing each individual knob by a little alters the accuracy).
With \accgrad, \name can quickly adapt to the optimal configuration in a
large configuration space by allocating more resources to those knobs with
high \accgrad to improve accuracy and cutting the resource usage of knobs with
\accgrad to save resource without hurting accuracy.





% insight that motivates \name is two properties we observe in deep learning
% system knobs. The first property is: for most of the knobs, if changing the
% value of one knob results in spending more (or less) resource, the corresponding
% inference result would statistically become more (or less) accurate. This
% property suggests that the change of accuracy with respect to knob value change
% can reflect the ability of trading resource for accuracy for each individual
% knob. With \accchange, \name can quickly adapt to the optimal configuration in a
% large configuration space: \name can allocate more resources to those knobs with
% high \accchange to improve accuracy and cut the resource usage of knobs with
% \accchange to save resource without hurting accuracy.



% There is one more challenge to calculate \accgrad.


The first challenge of calculating \accgrad is: how to calculate the accuracy change when changing a knob value by a little?
Directly calculating this accuracy change requires the underlying system to obtain the ground truth first (previous work define the ground truth as the inference results generated under the most expensive configuration to avoid the need for human annotation~\cite{dds,awstream,chameleon,vstore,videostorm,ekya,focus}).
This imposes non-trivial overhead due to extra inference on the most expensive configuration (\eg in Chameleon~\cite{chameleon}, calculating the ground truth\footnote{Chameleon is actually calculating multiple
resource-consuming configurations as the ``ground truth'', but the overhead is
still due to calculating ground truth.} consumes $\sim$50\% of the overall GPU
compute). 
To resolve this issue, we develop a proxy for accuracy difference (we call this proxy \accproxy). 
% The main idea is to reuse the existing inference results and measure the accuracy change if the same input
% data \textit{were} processed by a new configuration. 
Concretely, \accproxy estimates the sign and the magnitude of accuracy change by the following rule:
\begin{packeditemize}
\item 
The \textit{sign} of accuracy change is determined by which input (between the two DNN input generated before and after changing one knob value) is of \textit{less distortion} compared to the DNN input generated under most expensive configuration.
\item 
We estimate the \textit{magnitude} of accuracy change through checking the \textit{dissimilarity} between the two inference results generated before and after the knob value change.
The intuition behind this estimation is that: if the inference results generated before and after the knob change are highly similar, the inference accuracy of these two inference results should also be highly similar.
\end{packeditemize}
By using this proxy, calculating accuracy difference no longer relies on the generation of ground truth, and 


However, even with the optimization above, trivially calculating \accgrad in a knob-by-knob manner (\ie
calculate the accuracy change by alternating the value of one knob value
while the value of other knobs value remaining unchanged, and repeat this process
for all knobs) still requires extra inference to get the inference results after each knob value change. 
To avoid such extra inference, \name leverages the following two properties:
\begin{packeditemize}
    \item
    On the knobs side, most of the knobs treat DNN as a \textit{black box} and affect DNN inference results solely by changing the DNN input.
    As a result, calculating how changing each individual knob alters DNN input requires no extra inference.
    \item 
    On the DNN side, the DNN itself is differentiable to its input (via backpropagation algorithm).
    Thus, calculating how changing the DNN input alters the accuracy requires no extra inference.
\end{packeditemize}
These two properties suggest that to calculate how changing the system knobs alters the accuracy (\ie~\accgrad), we can first calculate how changing system knobs alters the DNN input, and then study how changing the DNN input alters the accuracy. 
The former can be calculated in a knob-by-knob manner without the participant of the DNN (thus avoid extra DNN inference) and the latter only requires one backpropagation (thus incurring no extra inference).

% compared to the ground truth DNN input, and estimate the magnitude of accuracy
% change by comparing the difference of inference results between the old and the
% new configuration. 
% We find that the \textit{gradient} of this accuracy metric can be calculated \textit{without} extra inference.

To conclude, the contribution of this paper is two-fold:
\begin{packeditemize}
    \item A general adaptation framework for DNN-based analytic systems that quickly adapt to
optimal configuration through \accgrad.
    \item Two techniques to calculate \accgrad without extra inference.

\end{packeditemize}

\begin{comment}

  Deep learning applications on streaming data (\eg video streams or LiDAR
  feeds) are everywhere. For example, in autonomous driving, people use video
  cameras and LiDAR sensors and leverage object detection deep neural networks
  (DNNs) to sense the surrounding environment and avoid potential collisions. In
  augmented reality, people use video cameras and LiDAR sensors to localize the
  remote objects and render the virtual objects on top of real objects. This
  trend inspires system research for these applications, like live
  analytics~\cite{??}, retrospective analytics~\cite{??}, database for analytic
  purpose~\cite{vstore,noscope}, etc.

  We identify two important characteristics of these systems. First, they
  contain large configuration spaces (\eg in AWStream~\cite{awstream}, there are
  216 different configurations inside its configuration space). Second, these
  configurations need to be \textit{timely} adapted according to their input
  (\eg we may want to use higher video resolution when a small car enters the
  video frame in order to detect this small car) and the current resource budget
  so that they can generate the inference results as accurate as possible.

  As a result, the key challenge for these systems is: how to navigate the large
  configuration space and pick the optimal configuration that generates the most
  accurate inference results under the current resource budget.

  The first way to address this problem is to \textit{frequently profile} the
  system with different configurations to obtain their resource usage and
  inference accuracy, and then pick the configuration that meets the resource
  budget and generates the most accurate inference
  results~\cite{awstream,chameleon,vstore}. However, in order to profile, this
  approach has to perform \textit{extra} inference on the GPU, resulting in high
  GPU cost.

  The other approach performs no extra inference and instead, picks the
  configuration based on the recent configuration and its corresponding DNN
  output. However, there can be many configurations that meet the resource
  budget. Without profiling most of them, it is difficult to separate the
  configurations that yield similar DNN output from those that yield more
  accurate DNN output. In addition, the previous work in this approach designs
  hand-craft heuristics catered for different applications.

  Thus, the requirements of an ideal configuration adaptation system are
  three-fold:
  \begin{enumerate}
    \item No extra DNN inference
    \item Pruning out the configurations with similar accuracy
    \item Agnostic to the underlying applications
  \end{enumerate}

  We present our system: \name that meets these three requirements. The idea is
  to calculate the \textit{gradient} of inference accuracy with respect to the
  configurations to \textit{predict} which of them improve inference accuracy
  and which do not. The key insight that enables us to calculate this gradient
  is by decoupling this gradient into two terms. The first term is the gradient
  of inference accuracy with respect to the DNN input, which can be calculated
  by backpropagation without performing extra inference on any other
  configuration. The second term is the gradient of the DNN input with respect
  to the configurations, which does not require DNN inference.

  To make our system practical, we also identify another source of overhead
  introduced by calculating inference accuracy. In order to calculate inference
  accuracy, previous work needs to refer to the configuration with \textit{the
  most} resource usage and use the corresponding inference results as the
  ``ground truth'' to evaluate the accuracy of inference results generated from
  other configurations. Calculating the ``ground truth'' uses much higher
  resource usage (including the streaming cost of streaming the data and the GPU
  cost to generate inference results) than the current optimal configuration. To
  reduce this cost, we introduce a \textit{proxy} of accuracy that
  \textit{indirectly optimizes} accuracy by using the DNN input (instead of the
  DNN output), thus requiring no DNN inference.

  To conclude, the contributions of this paper are:
  \begin{enumerate}
    \item A way to calculate gradient with no extra inference
    \item An accuracy proxy that indirectly optimizes the accuracy without
          running extra inference.
  \end{enumerate}
  We quantitatively evaluate these two contributions, we perform experiments on
  XXX datasets, XXX applications and XXX

\end{comment}


==> intro_v3.tex <==
\tightsection{Introduction}
% Deep-neural-network-based (DNN-based) analytics on data streams (\eg video
% streams or LiDAR feeds) are everywhere.
% For example, people leverage DNNs to analyze traffic video feeds for traffic monitorings~\cite{trafficvision, traffictechnologytoday, goodvision,intuvisiontech, vision-zero, msr}, analyze the information from multiple types of sensors (including camera, LiDAR and Radar sensors) to enable long-range vehicle and pedestrian detection for autonomous driving~\cite{tusimple,waymo,motional}.
% The input data stream varies a lot over time.
% For example, in autonomous driving, the number and the moving speed of vehicles and pedestrians varies a lot over time (\eg the number of vehicles and humans will be much higher when driving in daytime), areas (\eg the vehicle movement speed is much higher when driving in the highway), current location (\eg the number of pedestrains will be much higher at the crossroad), traffic condition (\eg the number of vehicles significantly increases in traffic congestion).
% \jc{highlight the need for tuning configuration knobs when you bring up "data stream varies over time"}
% This trend inspires system research for these applications~\cite{vigil,glimpse,mcdnn,videostorm,noscope,neurosurgeon,awstream,chameleon,focus,adascale,filterforward,vstore,cracking,dds,reducto,blazeit,yoda,vcm,elf,ekya}.
% % \jc{can we cite some dnn-based analytics systems use cases, where the input distribution varies over time, in terms of frequency of object occurrences, shape/size, etc? be as concrete as possible please} \kt{done}

% Deep-neural-network-based (DNN-based) analytics on data streams (\eg video
% streams or LiDAR feeds) are everywhere.
\kt{Slightly change the logic here. Now I pitch the temporal variabilities as an opportunity to save resources.}
Many applications rely on DNNs to perform accurate inference on various data streams (\eg video streams or LiDAR feeds).
For example, DNNs are used to analyze traffic videos to monitor vehicle speed and spot traffic jams~\cite{trafficvision, traffictechnologytoday, goodvision,intuvisiontech, vision-zero, msr} , and analyze data streams from infrared cameras, LiDAR sensors, and radar sensors to detect vehicles and pedestrians for autonomous driving~\cite{tusimple,waymo-blog,motional}.
% \jc{kuntai, the logic here is quite muddy.. it's unclear why content varying over time is interesting/important. 
% maybe try a different flow: as these DNN-based applications require high accuracy, they use a great amount of compute and network resource. 
% Many prior efforts have leveraged a common feature of these data streams: their content varies greatly over time. 
% For example...
% To leverage these opportunities, recent work exposes...
% }
As these DNN-based applications require high accuracy, they use a great amount of GPU compute and network resources. 
To mitigate this issue, many prior efforts try to leverage a common characteristic of these data streams---their contents vary greatly over time---to reduce the resource usage of these DNN-based applications.
% The content of these data streams vary greatly over time.
% For example, in autonomous driving, the number and the moving speed of vehicles are constantly changing over time (\eg the number of vehicles will be much higher compared to driving in night time), location (\eg cars move faster on the highway) and traffic condition (\eg the number of vehicles significantly increases in traffic congestion).
% For example, in dashcam video streams, the number and the moving speed of vehicles are constantly changing over time (\eg the number of vehicles will be much larger during daytime than during night), location (\eg cars move faster on the highway) and traffic conditions (\eg the number of vehicles significantly increases in traffic congestion).
% For example, in one traffic video stream that aims to localize vehicles on a traffic lane,
For example, in a traffic video stream, the moving speed of vehicles can be much lower during red traffic light compared to green traffic light, so one can analyze less frames during red traffic light (and thus save GPU compute resource) and still accurately capture the motion of the vehicles.
% \jc{highlight the need for tuning configuration knobs when you bring up "data stream varies over time"}
% Facing this trend, the system research community develop \textit{adaptation-required knobs} to \textit{enable} saving resources when the data can be safely analyzed by using less resource without hurting accuracy and timely \textit{adapt} these knobs to save resource when such data appears. ~\cite{vigil,glimpse,mcdnn,videostorm,noscope,neurosurgeon,awstream,chameleon,focus,adascale,filterforward,vstore,cracking,dds,reducto,blazeit,yoda,vcm,elf,ekya}.
% To save resources through such temporal variability in the data streams,
Technically, to capture such resource-saving opportunity introduced by the temporal variability in the data streams,
recent proposals~\cite{vigil,glimpse,mcdnn,videostorm,noscope,neurosurgeon,awstream,chameleon,focus,adascale,filterforward,vstore,cracking,dds,reducto,blazeit,yoda,vcm,elf,ekya} expose internal tunable parameters (referred to as \textit{knobs}) and \textit{timely configure} these knobs (we denote the knobs together with their configured values as a \textit{configuration}) according to the data streams to save resources (in GPU compute and network) while maintaining high inference accuracy.
% \jc{can we cite some dnn-based analytics systems use cases, where the input distribution varies over time, in terms of frequency of object occurrences, shape/size, etc? be as concrete as possible please} \kt{done}



% \jc{how about we pitch them as two parallel trends: (1) temporal variation of input, and (2) an increasingly number of knobs, $\rightarrow$ the challenge of timely adaptation in a large configuration space.}

% We observe that these systems expose an \textit{increasing} number of internal knobs.
% The underlying trend that drives this increase is two-fold (further discussion in \S\ref{subsec:numer_of_knobs}). 
% % First, these systems need to develop new knobs to not only provide accurate analytic results under all kinds of resource budget due to heterogeneous deployment settings, but to also handle new emerging applications (\eg LiDAR-based object detection for autonomous driving and infrared-based human detection for night-time security monitoring).
% First, these systems need to develop new knobs to not only trade-off between the accuracy and different kind of resources in order to handle all kinds of resource budget due to heterogeneous deployment settings, but to also handle new emerging applications (\eg LiDAR-based object detection for autonomous driving and infrared-based human detection for night-time security monitoring).
% \ga{It'll be helpful to make it explicit that knobs also regulate the resource demand and hence can be used to handle heterogeneous resource budget.}
% \kt{fixed}
% % These knobs trade-off between accuracy and different kinds of resource in order to
% Second, as the need of DNN-based analytics quickly grow, these systems need to tune existing type of knobs at a finer granularity to support more concurrent DNN-based analytic jobs. \ga{The need to partition isn't clear. Why were the knobs joined in the first place, before partitioning?} \kt{fixed}

We observe that there is already a broad set of knobs\footnote{Previous work proposes at least 16 knobs includes 6 video encoding knobs~\cite{vstore, chameleon, dds, videostorm, awstream}, 9 frame filtering knobs~\cite{reducto, vigil, glimpse}, and the knobs that differentiate spatial video quality knob~\cite{dds,accmpeg,eaar}, which can be partitioned into thousands of knobs if tuned in fine granularity~\cite{accmpeg}.}\cite{vstore,chameleon,dds,videostorm,awstream,reducto,vigil,glimpse,dds,accmpeg}, 
and the set is still growing, thanks to two trends.
% We observe that the number of such configuration knobs is already huge (\eg more than 16 different knobs\footnote{These 16 knobs includes 6 video encoding knobs~\cite{vstore,chameleon,dds,videostorm,awstream}, 9 frame filtering knobs~\cite{reducto,vigil,glimpse}, and the knobs that differentiate spatial video quality knob~\cite{dds,accmpeg}, which can be partitioned to thousands of knobs if tuned in a fine granularity.} are introduced in video analytic systems~\cite{vstore,chameleon,dds,videostorm,awstream,reducto,vigil,glimpse,accmpeg}) and is still expanding.
% We observe that these systems expose an expanding set of configuration knobs that leverages temporal variabilities in the data stream to save resource without hurting the accuracy.
% % be adapted to the temporal variations of the input data stream to save resource.
% There are two reasons behind this trend. 
% First, these systems need to develop new knobs to not only provide accurate analytic results under all kinds of resource budget due to heterogeneous deployment settings, but to also handle new emerging applications (\eg LiDAR-based object detection for autonomous driving and infrared-based human detection for night-time security monitoring).
First, when people deploy DNN-based analytic systems into practice, they found that these systems need more knobs to explore new resource-saving opportunities introduced by new types of data streams (\eg LiDAR feeds), new applications (\eg video captioning) and new deployment settings (\eg multi-camera video analytics~\cite{chameleon, vigil}, multi-server video analytics~\cite{elf}).
% First, these systems need more knobs to not only trade between different type of resources to fit into more deployment settings (\eg the user may stream the data out from cheap camera through expensive LTE network for analytics. In this case, it is more ideal for the system to trade server-side compute for bandwidth~\cite{dds,eaar} instead of trade camera-side compute for bandwidth~\cite{vigil,glimpse,accmpeg} to simultaneously reduce the bandwidth usage without  the camera-side compute usage), but to also 
% \ga{It'll be helpful to make it explicit that knobs also regulate the resource demand and hence can be used to handle heterogeneous resource budget.}
% \kt{fixed}
% These knobs trade-off between accuracy and different kinds of resource in order to
Second, as these systems need to run more analytic jobs than before,
% these systems need to support more concurrent analytic jobs under the same resource budget, which requires them to 
they need to tune existing knobs at a finer granularity (by partitioning existing knobs into \textit{multiple} fine-grained knobs) to further reduce the resource usage of each analytic job.
% further reduce the resource demand for running one analytic job without hurting the accuracy.
For example, in a dashcam video stream, when the input video contains \textit{only one} small object, one may need to encode \textit{the whole video} in high fidelity in order to make this object detected, resulting in high bandwidth usage~\cite{chameleon,awstream}.
% when the input video contains one small object, one may need to encode and stream the whole video into high resolution to detect such object, resulting in high bandwidth usage~\cite{chameleon,awstream}.
However, prior effort~\cite{dds,eaar,accmpeg} shows that the areas that are not related to the object can be encoded in low fidelity to save bandwidth and realizes this potential by \textit{partitioning} the video into different areas and assigning different areas with different fidelities.
% , by assigning different areas with different resolutions\footnote{In fact, prior work assigns different areas with different quantization parameters, a parameter that controls the fidelity of the encoded video without changing the resolution. We use resolution in the text for understandability consideration.}, it only needs to encode the area that contains the object into high resolution and other areas can be safely encoded in low resolution. This significantly reduces the bandwidth usage.

% % redirected enumerate to packedenumerate for reformater in macro.tex. DON'T
% % CHANGE!
% \begin{enumerate}
%   \item 
% As DNN-based analytics are deployed on heterogeneous deployment settings that have different types of resource budgets, this requires the corresponding systems to propose new knobs in order to fit into
% different resource budgets. Take video analytics as an example. If the
% user analyzes the video feeds locally by a compute-constrained mobile
% phone, the main focus for the systems is to fit into the compute budget
% of the phone (\eg by skipping those frames that are highly similar to
% their previous frames~\cite{reducto,glimpse}). However, if the user
% instead streams the video feeds to a GPU-equipped server through a
% bandwidth-limited LTE network, the main focus is instead fitting into
% the limited LTE bandwidth (\eg by performing video
% compression~\cite{accmpeg,vigil,glimpse,reducto}).

%   \item As DNN-based analytics quickly expand, the corresponding systems need to
%         partition existing knobs into more fine-grained version to capture more
%         resource-saving opportunities. Take video-based vehicle detection as an
%         example. Chameleon~\cite{chameleon} and AWStream~\cite{awstream}
%         identify that the system only need to encode the video in a high
%         encoding quality when the vehicle appears. To further explore the
%         potential of varying video encoding quality, the following
%         work~\cite{dds,eaar,accmpeg} finds that a lot of areas in the video do
%         not need to be encoded in high quality (\eg the areas that contain
%         non-vehicle-related backgrounds like trees and buildings) and proposes
%         fine-grained spatial encoding quality to capture this opportunity.
%   \item Since new applications quickly emerge (\eg LiDAR-based object detection,
%         Infrared-based human detection \kt{a bunch of citations here}), this requires the deep learning systems
%         to develop new knobs (or even developing new system components) to fit
%         into the need of different applications. For example, in order to handle
%         LiDAR data, people are proposing new encoding standard and new
%         knobs~\cite{MPEG-point} to efficiently encode and process LiDAR data.
%         \roy{I understand you are trying to distinguish old types of application
%         and new ones, but I still feel the first and third items are kind of
%         repetitive? Both items are trying to say there is the need for new
%         knobs, right? Maybe merge them into one?}
% \end{enumerate}

% Not only the number of knobs are already huge (\eg in video analytics, previous work introduces 6 video codec encoding knobs~\cite{vstore,chameleon,dds,videostorm,awstream}, 9 frame filtering knobs~\cite{reducto,vigil,glimpse} and even thousands of knobs for fine-grained video encoding quality assignment~\cite{accmpeg}) and still expanding
% % \ga{Quantify.}
% , these knobs also need to be timely adapted~\cite{awstream,chameleon,dds,eaar,elf} due to input data change or resource budget change in order to achieve high inference accuracy.
% Thus, the research question is: how to navigate the large configuration space (\ie all possible choices of knob values) and and pick the optimal configuration that generates accurate inference results under the current resource budget?


% As the number of knobs are already huge (\eg more than 16 different knobs\footnote{These 16 knobs includes 6 video encoding knobs~\cite{vstore,chameleon,dds,videostorm,awstream}, 9 frame filtering knobs~\cite{reducto,vigil,glimpse}, and the knobs that differentiate spatial video quality knob~\cite{dds,accmpeg}, which may include thousands of knobs if tuned in a fine granularity.} are introduced in video analytic systems~\cite{vstore,chameleon,dds,videostorm,awstream,reducto,vigil,glimpse,accmpeg}) and is still expanding,
% \ga{Quantify.}
% , these knobs also need to be timely adapted~\cite{awstream,chameleon,dds,eaar,elf} due to input data change or resource budget change in order to achieve high inference accuracy.
Given the \textit{large yet expanding} set of knobs, the research question of this paper is:
\textit{among a large number of configurations, how to quickly and optimally configure each knob to achieve high accuracy with a given resource budget?}

The first way to address this problem is to \textit{frequently profile}
different configurations to obtain their resource usage and
inference accuracy, and then pick the configuration that yields high inference accuracy without exceeding a given resource budget~\cite{chameleon,awstream,vstore,videostorm}.
% meets the resource
% budget and generates the most accurate inference results
However, each profiling
needs to run \textit{extra} inference to analyze multiple configurations (some are expensive in terms of resource usage). %before obtaining the profile.
% As a result, when the optimal configuration changes, this approach need to perform the extra inference to obtain the new optimal configuration, thus incurring high delay when the GPU resource is limited.
Thus, when the GPU compute is limited, this approach needs to either profile less frequently, resulting in using outdated configurations when the optimal configuration has drifted away, or significantly prune the search space (which may contain only suboptimal configurations). %profile fewer configurations, which may miss the optimal configuration. 
% Both of them lead to a sub-optimal trade-off between the accuracy and the resource usage.
% \ga{Call out the downsides of extra inference.} \kt{fixed}

The second approach is to train a cheap model (\eg neural network) to predict the optimal configuration and then leverage this model to adapt the configuration.
However, as the compute of such model is limited due to \fillme, the model may no longer being able to predict the optimal configuration when the input content changes.
For example, \fillme.





% \kt{This para needs a rewrite}
% The other approach performs no extra inference and instead, computes the
% configuration based on recent DNN outputs (including intermediate outputs) through cheap heuristics~\cite{dds,eaar,elf} or through DNN-based configuration generator~\cite{accmpeg,casva}). 
% \ga{What does ``derives the configuration'' mean?} \kt{fixed}
% % However, there can be many configurations that meet the resource budget. \ga{There has been no mention of budget so far.}
% % Without profiling most of them, it is difficult to separate the configurations that yield similar DNN output from those that yield more accurate DNN output by merely looking at recent DNN outputs.
% % As a result, this approach waste resource on those configurations that yield similar DNN output and thus cannot quickly adapt to the optimal configuration. 
% \ga{I don't fully follow this paragraph and it needs more explanation. That said, can I view the techniques in this paragraph as a pruning mechanism to identify the promising configurations?}
% \kt{This para needs a rewrite}
The second approach performs no extra inference and adapts the
configuration based on recent DNN outputs (including intermediate outputs)~\cite{dds,eaar,elf,accmpeg,casva}.
% \jc{i still dont quite get why we use dds here. isn't some bandit/RL-based solution a better fit?}
% For instance, DDS~\cite{dds} tunes encoding quality by first encoding all pixels at a low quality and streaming them to the server-side DNN, whose output (region proposal) is then used to tune the quality at different regions.
Though no extra inference is run, this approach tends to adapt {\em slowly}, as each DNN output reveals limited information regarding the \textit{highly complex} relationship between the configurations and DNN inference output/accuracy, due to the complexity of the DNN itself and the preprocessing modules before the DNN (\eg video codecs).
We take EAAR~\cite{eaar}, a system for video object detection, as an example.
EAAR adjusts the video encoding quality by collecting the regions from the DNN that may contain objects of interest and encoding these regions in higher encoding quality on future video frames.
% After that, it encodes these regions in high quality on the next video frame.
Thus, the objects inside these regions are much more likely to be detected.
% This approach then lets the sensor encode all these regions in high encoding quality on the next video frame so that the objects inside these regions can be accurately detected.
However, as the regions generated by the DNN may not include all the regions that contain the objects, the object detection DNN may miss some objects and thus EAAR needs to further adjust the regions corresponding to these missing objects.
% For instance, the impact of configuration on DNN accuracy is affected by two complex blackboxes: DNN itself as well as the video codecs.
% However, the \textit{adaptation speed} (\ie the time it takes to obtain the optimal configuration) of this approach can be slow.
% For example, DDS~\cite{dds} tunes the encoding quality of different areas of the video in the following steps.
% First, DDS let the camera encode the whole video into low quality and stream it to the server.
% The server then analyzes the video to obtain the areas that may contain objects and let the camera resend those areas in high encoding quality for an extra round of inference.
% % through cheap heuristics~\cite{dds,eaar,elf} or through DNN-based configuration generator~\cite{accmpeg,casva}).
% However, the \textit{adaptation speed} (\ie the time it takes to obtain the optimal configuration) of this approach can be slow.
% % explore many configurations to accumulate enough DNN outputs before converging to the optimal one.
% % need to accumulate enough DNN outputs in order to obtain the optimal configuration.
% % This is because this approach only examine one configuration at a time.
% This is because they only get one DNN output at a time.
% As the relationship between the configuration to the inference accuracy is highly complex (due to complexity inside the underlying system (\eg video codec) and the DNN itself), this approach needs to spend time accumulating enough DNN outputs before obtaining the optimal configuration, resulting in slow adaptation speed.
% Thus, it is difficult to identify whether a new configuration improves accuracy or not based on the current DNN output.
% the performance of other configurations.
% the DNN ouput on just one configuration is not enough for this approach to immediately obtain the optimal configuration thus
% As a result, 
% this approach needs to accumulate enough DNN outputs to reach the optimal configuration. 
% The optimal configuration may have already changed (due to the change of input content or resource budget) before this approach reaching it.
% The optimal configuration may have already changed.

% However, there can be many configurations that meet the resource budget.
% Without profiling most of them, it is difficult to separate the configurations that yield similar DNN output from those that yield more accurate DNN output by merely looking at recent DNN outputs.
% As a result, this approach waste resource on those configurations that yield similar DNN output and thus cannot quickly adapt to the optimal configuration. 


\kt{rewrote this para.}
Moreover, the heuristics used in the second approach are designed for specific types of knobs and are not directly applicable to other knobs (though these heuristics \textit{could} be augmented and used to adapt other knobs).
% even if they can be purposely built to efficiently support some knobs. 
% are hand-crafted for individual applications or configurations and thus not generalizable to other configurations and applications.
We take EAAR~\cite{eaar}, a system that serves object detection, as an example.
EAAR assigns the regions that may contain objects based on the current frame and encodes these regions with higher encoding quality to in the future frames to make more objects detected.
In a higher level, EAAR applies the decision generated from the current frame to the future frames.
However, this may not be a suitable way to adapt the knobs that, for example, decide which video frames can bypass the DNN inference.
This is because the optimal decision may vary a lot between the current frame and the future frames: if the current frame needs to be forwarded through the DNN, it is more likely that the next frame should bypass the DNN inference.
As a result, EAAR may not directly apply to the DNN-bypassing knobs.
% However, EAAR may be sub-optimal if applied to the knobs that decide which video frames can bypass the DNN inference without hurting the inference accuracy.
% This is because EAAR make an assumption that do not fit this set of knobs.
% Concretely, the current design of EAAR generates the configuration on one frame and apply it to the future frames, which assumes that the optimal knobs on one frame generalizes to the future frames.
% However, this assumption may not be true in the scenario of bypassing DNN inference: if one frame needs to be forwarded through the DNN, it is more likely that the next frame should bypass the DNN inference, and vise versa.
% The violation of this assumption results in the sub-optimal adaptation behavior of EAAR: EAAR may continuously performing inference on a few frames and then continuously bypassing the DNN inference on the next few frames, while the optimal way is to perform inference intermittently.
% This 
% This is because making such decision requires the adaptation algorithm to analyze these frames without performing DNN inference on these frames, while the current design of EAAR lets the DNN ingest this frame first and then analyze this frame leverage the intermediate analytical results on this frame for further use.
% performing DNN inference on this frame and then harnessing the intermediate outputs generated by the DNN inferences. 
% As a result, EAAR either obtains no extra information on one frame besides the pixel values of this frame (thus cannot make accurate decision on whether letting this frame bypassing DNN inference or not), or analyzes this frame at the cost of performing DNN inference (thus this frame cannot bypass the DNN inference).
% does not extract any information of one frame  while the current design of EAAR always inference on the current frame and are agnostic to the future frames.
% making such a decision requires estimating the similarity of the inference results, between those discarded frames and reserved frames, while EAAR focusing on extracting the regions that may contain objects, where only a small subset of them will appear in the final inference results.
% Take DDS~\cite{dds} as an example, which analyzes the video and then resends some areas of the video that may contain objects of higher fidelity.
% As the recent areas are derived from the output of a specific DNN component (region proposal) that aims to facilitate object detection, this heuristic is not directly applicable to tasks like video classification.
% Moreover, this heuristic does not apply to tune frame-discarding knobs~\cite{vigil,glimpse,reducto} that discard similar frames to save GPU compute, because the way DDS obtains the output to tune the knobs incur more GPU compute in the first place. 
% the knobs in frame discarding techniques 
% (\ie discarding the frames that produce similar inference results compared to previous frames~\cite{vigil,glimpse,reducto}) without further adjustments, since its adaptation logic (\ie resending some areas of the video that may contain objects) happens \textit{after} DNN inference while frame filtering needs to be performed \textit{before} DNN inference to save GPU compute cost. 
% As a result, DDS does not directly generalize to other 
% \ga{How is this paragraph on DDS pertaining to profiling and avoiding extra inference? The relationship isn't clear.} \kt{fixed}
% \jc{not sure ganesh's comment was addressed. i think the confusion is whether you are criticizing dds's logic being inefficient or not generalizable. if it's the latter, just say it explicitly.}


% An ideal configuration adaptation system should meet these two
% requirements: 1. quickly adapt to optimal configuration in a large configuration
% space without extra inference 2. minimum assumption to the underlying system.

An ideal configuration adaptation system, therefore, needs to \textit{serve a wide range of knobs and applications and quickly adapt to the optimal configuration among a large amount of configurations with no extra inference}.

% \kt{Pitch the cause of the previous work limitation as they only using DNN outputs -- which can change a lot between different configuration and video content -- to predict the performance on unknown configuration and unknown content.
% Our approach combines the DNN parameters -- which does not change between different configuration and video content -- to better generalize the prediction of the performance on unknown configuration and unknown content.
% }

% \jc{i guess the rest of the intro hasn't been updated since last wednesday. just to recap, here's the flow:
% \begin{packeditemize}
%     \item start with a new abstraction, \accgrad, to more efficiently adapt configurations than prior schemes, especially in a large configuration space, and why?
%     we present \name, the first efficient implementation of \accgrad
%     we should clarify that prior work could expose this abstraction as well, but they suffer high overhead (why?). 
%     \item \name approximates \accgrad based on two observations: 
%     (1) the values of each configuration can be ordered in a way that \fillme, and
%     (2) the more changes of confidence scores around the threshold, the more accuracy will change.
%     \item based on the two observations, \name does \fillme
%     \item operators can use \name to tune a range of configurations that influences dnn input. this class of config covers many existing systems. but notably, this doesn't cover \fillme (may point to a synergy with recent online learning papers like ekya --- in some sense, they also handle input drift, but they choose to retrain the model, and our approach is more lightweight.)
% \end{packeditemize}}

% \kt{Stress that knob is trading res usage for acc}
% \kt{Adaptation goal: expose an abstraction: monitoring both }

% \kt{
% Expose 1 abstraction:
% resource-knob gradient
% DNN output (We use the change of confidence values around the threshold, see \S\ref{??} for further detail) gradient
% % confidence change gradient
% Say it correlates with accuracy?
% With this gradient, we can 1). efficiently optimize knobs

% Previous work, if repurposed, incurs extra inference.

% Advantage: can be calculated without extra inference
% }


% To realize these two objectives, we expose a new abstraction: , which means the performance change divided by knobs change when changing the knobs by a little.
% Concretely, performance gradient includes resource usage gradient, and DNN output gradient (we measure the DNN output change by measuring the absolute change of confidence scores around the confidence threshold. See \S\ref{??} for further details).


We advocate that the adaptation system for DNN-based analytics should expose a new abstraction: \textit{\outputgrad}, which estimates \textit{the gradient of DNN output with respect to each knob}.
We present \name, a system that implements \outputgrad and uses it to adapt configurations with constant GPU overhead and no extra inference.
% Based on \outputgrad, we present \name, a configuration adaptation system that implements \outputgrad with constant GPU overhead and with no extra inference.
Specifically, \name measures \outputgrad by how much a small change in the current value of each knob \textit{flips} the DNN-returned confidence scores from below (or above) the confidence threshold to above (or below). 
% We measure \outputgrad by how much a small change in the current value of each knob affects the DNN-returned confidence scores near (both below and above) the given confidence threshold.
Note that this measurement does not impose an extra burden on the application side since most of the applications already expose confidence scores to indicate the uncertainty of DNN outputs and use confidence thresholds to filter out DNN outputs with low confidence. %those uncertain results returned from the DNN.
Statistically, more changes in the ``near-confidence-threshold'' DNN outputs will likely cause more changes in the inference accuracy (as will be elaborated in \S\ref{subsec:correlation})\footnote{This correlation does \textit{not} assume that a confidence score always directly indicates the accuracy of its corresponding detection/classification results.}.
% \outputgrad correlates with how much the accuracy \textit{changes} with knobs 
Intuitively, this is because the confidence threshold determines whether a detection or classification result is accepted (as part of the accuracy calculation) or rejected (thus having no effect on the accuracy).
% When the knob change only alters the DNN output by a little, the corresponding accuracy change also tends to be minor.
% Thus, more change on the ``near-threshold'' DNN outputs, more changes on the inference accuracy.




% how much the DNN output changes when varying each individual knob by a little (we measure the DNN output change by measuring the change of those confidence scores around the confidence threshold, see \S\ref{??} for the mathematical formulation and the intuition behind).
% We call this metric \outputgrad for short.
% when slightly changing the knob  (we call it \outputgrad for short).
% We will cover the detail


% \kt{Should we allocate a paragraph to talk about the overhead of calculating ground truth here?}
% We acknowledge that using DNN output change cannot obtain the exact number of the accuracy change.
% However, we still think that this is a valuable choice, as
% directly calculating this accuracy change requires the underlying system to obtain the ground truth first (previous work define the ground truth as the inference results generated under the most expensive configuration to avoid the need for human annotation~\cite{dds,awstream,chameleon,vstore,videostorm,ekya,focus}).
% This imposes non-trivial overhead due to extra inference on the most expensive configuration (\eg in Chameleon~\cite{chameleon}, calculating the ground truth\footnote{Chameleon is actually calculating multiple
% resource-consuming configurations as the ``ground truth'', but the overhead is
% still due to calculating ground truth.} consumes $\sim$50\% of the overall GPU
% compute). 



With the \outputgrad, the adaptation system can quickly adapt to the optimal configuration by assigning more resources to the knobs with high \outputgrad to improve the accuracy, or cut the resource usage of the knobs with low \outputgrad without hurting the accuracy.


However, it can be expensive to calculate \outputgrad over a space of many knobs. %may incur high amount of extra inference.
% This is because previous work needs to calculate \outputgrad in a knob-by-knob manner (\ie inference on the DNN and calculate the DNN output change by alternating the value of one knob while fixing other knobs, and repeat this process for all knobs). 
Previous work~\cite{chameleon,vstore,videostorm,awstream} would have had to calculate \outputgrad in a knob-by-knob manner (\ie inference on the DNN and calculate the DNN output change by alternating the value of one knob while fixing other knobs, and repeat this process for all knobs). 
% Thus, one more knob, one more extra inference.
% Thus, more knobs will lead to more inference.


To avoid such extra inference, \name leverages the \textit{differentiability} of the DNN to implement \outputgrad with constant GPU overhead and with no extra inference.
% We show that \outputgrad, the first system that implements can be calculated without any extra inference and with constant GPU overhead.
% We develop \name, a configuration adaptation system that optimizes the configuration based on \outputgrad.
% The insight of \name is to leverage the \textit{differentiability} of DNN to reduce the cost of calculating \outputgrad.
We {\em decouple} the calculation of \outputgrad (\ie how changing the knobs alters the DNN output) to how changing system knobs alters the DNN input and how changing the DNN input alters the DNN output.
% Concretely, in order to calculate how changing the knobs alters the DNN output (\ie \outputgrad), we can calculate how changing system knobs alters the DNN input, and then calculate how changing the DNN input alters the DNN output.
% \kt{Should we add a math formula of chain rule here? Like output/knob = output/input * input/knob?}
The former can be calculated in a knob-by-knob manner without DNN inference (\ie no GPU compute), and the latter can be obtained via {\em backpropagation} (which is a constant GPU overhead without extra inference as it can reuse the existing computation graph of DNN inference).

% We show that \outputgrad can be calculated with constant GPU overhead and without any extra inference, regardless of the number of the knobs, and develop \name, a configuration adaptation system, that optimizes the knobs based on \outputgrad.
% \name reduces the cost of extra inference by treating \outputgrad as an actual gradient and leveraging the following two properties to decouple this gradient through the chain rule.
% % \kt{I feel like this is the place to introduce the separation of the knob side v.s. the DNN side, as this separation is used (and only used) to reduce the cost of calculating the gradient}
% \begin{packeditemize}
%     \item 
%     On the DNN side, the DNN output is differentiable to its input (via backpropagation algorithm).
%     Thus, calculating how changing the DNN input alters the DNN output requires no extra inference.
%     \item
%     On the knob side, a wide range, \textit{not all}, of the knobs treat DNN as a \textit{black box} and affect DNN inference results solely by changing the DNN input.
%     As a result, calculating how changing each individual knob alters DNN input requires no extra inference.
% \end{packeditemize}
% These two properties suggest that to calculate how changing the knobs alters the DNN output (\ie \outputgrad), we can first calculate how changing system knobs alters the DNN input, and then study how changing the DNN input alters the DNN output. 
% \kt{Should we add a math formula of chain rule here? Like output/knob = output/input * input/knob?}
% The former can be calculated in a knob-by-knob manner without the participant of the DNN (thus avoid extra DNN inference), and obtaining the latter only requires one backpropagation (this creates a constant GPU overhead, but it is reusing the computation graph created by existing DNN inference, thus incurring no extra inference).


Operators can use \name to tune a wide range of knobs that influences DNN input (as shown in Table~\ref{tab:rich-set-of-knobs}).
That said, \name does {\em not} apply to knobs that alter the DNN itself, 
such as retraining the DNN weights~\cite{ekya,noscope,mcdnn}.
Similar to \name, they also adapt to changes in input distribution, they involve substantial computation and thus tend to happen at a coarser timescale than the knobs considered in \name. 
% such as customizing the DNN according to the current content of the input~\cite{ekya,noscope,mcdnn}.
% In some sense, both the DNN customization approach and \name are adapting to the varying content in the input data stream.
% However, in order to maintain high accuracy, DNN customization approach needs to retrain the DNN when the input content varies, and thus incurs high GPU overhead, while \name adapts the knobs inside the underlying system that serves the DNN, which is much more lightweight.


In short, the contributions of this paper are two-fold:
\begin{packeditemize}
    \item A new abstraction, \outputgrad, that enables quick adaptation of configurations for DNN-based analytics.
    % \item A new abstraction, \outputgrad, that enables the configuration adaptation framework for DNN-based analytic systems to quickly adapt to optimal configuration through \accgrad.
    \item A configuration adaptation system, \name, that implements \outputgrad with constant GPU overhead and without extra inference.
    % \item An implementation, \name, that implements \outputgrad with constant GPU overhead and with no extra inference.

\end{packeditemize}

We evaluate \name across 7 different DNN-based analytic pipelines and across 54 videos. \name achieves similar accuracy with 10-43\% end-to-end delay reduction, or achieves 1-10\% higher accuracy with similar end-to-end delay compared to the baselines on 8 different applications.
Also, we show that the performance gain of \name compared to the baselines becomes larger when there are more knobs or the knobs become more fine-grained.

\textbf{This work does not raise any ethical issues.}







% Expose abstraction:
% confidence change gradient with respect to resource


% Confidence scores -> a generalizable format
% Confidence thresholds -> a widely adopted component in the accuracy of applications in real world.

% % The key to achieve this goal is to calculate how much each knob changes the confidence scores that are close to the confidence thresholds 

% To quickly adapt to optimal configuration without extra inference, the intuition of \name is to allocate more resource to the knobs that maximally change the confidence scores inside the inference results that are around  with confidence scores \textit{around} the confidence thresholds.
% to maximally change \textit{which} inference results participants the accuracy
% Concretely, \name calculates 


% Why this works: two assumptions on the knobs 1. more resource, higher accuracy and 2. if the confidence scores around the confidence thresholds doesn't change, the accuracy barely change.

% We present \name that efficiently calculates such metric on each knob.
% The key for \name to success is to leverage the differentiability of DNN to \textit{predict} the performance of a run-time system.

% our approach is to: grant more resources to the knobs can maximally change the part of the inference results that the confidence scores are around the confidence thresholds, and cut the resource usage of those knobs that barely change 


% To quickly calculate this metric, we leverage the differentiability of the DNN to quickly obtain how DNN input affects the confidence scores around the confidence thresholds.



% We present our system: \name, which meets these two requirements. 
% To quickly adapt to optimal configuration, \name calculates the \textit{gradient} of accuracy with respect to each knob (hereinafter \accgrad, defined as the accuracy change if changing one knob valued by a little).
% % leverages a property of DNN-based analytic system knobs: for most of the knobs, if changing the value of one knob results in spending more (or less) resource, the corresponding inference result would statistically become more (or less) accurate.
% % This property suggests that each knob is able to \textit{trade resource for accuracy}.
% % To quantitatively measure this ability, \name calculates the \textit{gradient} of accuracy with respect to each knob (hereinafter \accgrad, defined as how changing each individual knob by a little alters the accuracy).
% With \accgrad, \name can quickly adapt to the optimal configuration in a
% large configuration space by allocating more resources to those knobs with
% high \accgrad to improve accuracy and cutting the resource usage of knobs with
% \accgrad to save resource without hurting accuracy.





% % insight that motivates \name is two properties we observe in deep learning
% % system knobs. The first property is: for most of the knobs, if changing the
% % value of one knob results in spending more (or less) resource, the corresponding
% % inference result would statistically become more (or less) accurate. This
% % property suggests that the change of accuracy with respect to knob value change
% % can reflect the ability of trading resource for accuracy for each individual
% % knob. With \accchange, \name can quickly adapt to the optimal configuration in a
% % large configuration space: \name can allocate more resources to those knobs with
% % high \accchange to improve accuracy and cut the resource usage of knobs with
% % \accchange to save resource without hurting accuracy.



% % There is one more challenge to calculate \accgrad.


% The first challenge of calculating \accgrad is: how to calculate the accuracy change when changing a knob value by a little?
% Directly calculating this accuracy change requires the underlying system to obtain the ground truth first (previous work define the ground truth as the inference results generated under the most expensive configuration to avoid the need for human annotation~\cite{dds,awstream,chameleon,vstore,videostorm,ekya,focus}).
% This imposes non-trivial overhead due to extra inference on the most expensive configuration (\eg in Chameleon~\cite{chameleon}, calculating the ground truth\footnote{Chameleon is actually calculating multiple
% resource-consuming configurations as the ``ground truth'', but the overhead is
% still due to calculating ground truth.} consumes $\sim$50\% of the overall GPU
% compute). 
% To resolve this issue, we develop a proxy for accuracy difference (we call this proxy \accproxy). 
% % The main idea is to reuse the existing inference results and measure the accuracy change if the same input
% % data \textit{were} processed by a new configuration. 
% Concretely, \accproxy estimates the sign and the magnitude of accuracy change by the following rule:
% \begin{packeditemize}
% \item 
% The \textit{sign} of accuracy change is determined by which input (between the two DNN input generated before and after changing one knob value) is of \textit{less distortion} compared to the DNN input generated under most expensive configuration.
% \item 
% We estimate the \textit{magnitude} of accuracy change through checking the \textit{dissimilarity} between the two inference results generated before and after the knob value change.
% The intuition behind this estimation is that: if the inference results generated before and after the knob change are highly similar, the inference accuracy of these two inference results should also be highly similar.
% \end{packeditemize}
% By using this proxy, calculating accuracy difference no longer relies on the generation of ground truth, and 


% However, even with the optimization above, trivially calculating \accgrad in a knob-by-knob manner (\ie
% calculate the accuracy change by alternating the value of one knob value
% while the value of other knobs value remaining unchanged, and repeat this process
% for all knobs) still requires extra inference to get the inference results after each knob value change. 
% To avoid such extra inference, \name leverages the following two properties:
% \begin{packeditemize}
%     \item
%     On the knobs side, most of the knobs treat DNN as a \textit{black box} and affect DNN inference results solely by changing the DNN input.
%     As a result, calculating how changing each individual knob alters DNN input requires no extra inference.
%     \item 
%     On the DNN side, the DNN itself is differentiable to its input (via backpropagation algorithm).
%     Thus, calculating how changing the DNN input alters the accuracy requires no extra inference.
% \end{packeditemize}
% These two properties suggest that to calculate how changing the system knobs alters the accuracy (\ie~\accgrad), we can first calculate how changing system knobs alters the DNN input, and then study how changing the DNN input alters the accuracy. 
% The former can be calculated in a knob-by-knob manner without the participant of the DNN (thus avoid extra DNN inference) and the latter only requires one backpropagation (thus incurring no extra inference).

% compared to the ground truth DNN input, and estimate the magnitude of accuracy
% change by comparing the difference of inference results between the old and the
% new configuration. 
% We find that the \textit{gradient} of this accuracy metric can be calculated \textit{without} extra inference.

% \begin{comment}

%   Deep learning applications on streaming data (\eg video streams or LiDAR
%   feeds) are everywhere. For example, in autonomous driving, people use video
%   cameras and LiDAR sensors and leverage object detection deep neural networks
%   (DNNs) to sense the surrounding environment and avoid potential collisions. In
%   augmented reality, people use video cameras and LiDAR sensors to localize the
%   remote objects and render the virtual objects on top of real objects. This
%   trend inspires system research for these applications, like live
%   analytics~\cite{??}, retrospective analytics~\cite{??}, database for analytic
%   purpose~\cite{vstore,noscope}, etc.

%   We identify two important characteristics of these systems. First, they
%   contain large configuration spaces (\eg in AWStream~\cite{awstream}, there are
%   216 different configurations inside its configuration space). Second, these
%   configurations need to be \textit{timely} adapted according to their input
%   (\eg we may want to use higher video resolution when a small car enters the
%   video frame in order to detect this small car) and the current resource budget
%   so that they can generate the inference results as accurate as possible.

%   As a result, the key challenge for these systems is: how to navigate the large
%   configuration space and pick the optimal configuration that generates the most
%   accurate inference results under the current resource budget.

%   The first way to address this problem is to \textit{frequently profile} the
%   system with different configurations to obtain their resource usage and
%   inference accuracy, and then pick the configuration that meets the resource
%   budget and generates the most accurate inference
%   results~\cite{awstream,chameleon,vstore}. However, in order to profile, this
%   approach has to perform \textit{extra} inference on the GPU, resulting in high
%   GPU cost.

%   The other approach performs no extra inference and instead, picks the
%   configuration based on the recent configuration and its corresponding DNN
%   output. However, there can be many configurations that meet the resource
%   budget. Without profiling most of them, it is difficult to separate the
%   configurations that yield similar DNN output from those that yield more
%   accurate DNN output. In addition, the previous work in this approach designs
%   hand-craft heuristics catered for different applications.

%   Thus, the requirements of an ideal configuration adaptation system are
%   three-fold:
%   \begin{enumerate}
%     \item No extra DNN inference
%     \item Pruning out the configurations with similar accuracy
%     \item Agnostic to the underlying applications
%   \end{enumerate}

%   We present our system: \name that meets these three requirements. The idea is
%   to calculate the \textit{gradient} of inference accuracy with respect to the
%   configurations to \textit{predict} which of them improve inference accuracy
%   and which do not. The key insight that enables us to calculate this gradient
%   is by decoupling this gradient into two terms. The first term is the gradient
%   of inference accuracy with respect to the DNN input, which can be calculated
%   by backpropagation without performing extra inference on any other
%   configuration. The second term is the gradient of the DNN input with respect
%   to the configurations, which does not require DNN inference.

%   To make our system practical, we also identify another source of overhead
%   introduced by calculating inference accuracy. In order to calculate inference
%   accuracy, previous work needs to refer to the configuration with \textit{the
%   most} resource usage and use the corresponding inference results as the
%   ``ground truth'' to evaluate the accuracy of inference results generated from
%   other configurations. Calculating the ``ground truth'' uses much higher
%   resource usage (including the streaming cost of streaming the data and the GPU
%   cost to generate inference results) than the current optimal configuration. To
%   reduce this cost, we introduce a \textit{proxy} of accuracy that
%   \textit{indirectly optimizes} accuracy by using the DNN input (instead of the
%   DNN output), thus requiring no DNN inference.

%   To conclude, the contributions of this paper are:
%   \begin{enumerate}
%     \item A way to calculate gradient with no extra inference
%     \item An accuracy proxy that indirectly optimizes the accuracy without
%           running extra inference.
%   \end{enumerate}
%   We quantitatively evaluate these two contributions, we perform experiments on
%   XXX datasets, XXX applications and XXX

% \end{comment}


==> intro_v4.tex <==
\tightsection{Introduction}
% Deep-neural-network-based (DNN-based) analytics on data streams (\eg video
% streams or LiDAR feeds) are everywhere.
% For example, people leverage DNNs to analyze traffic video feeds for traffic monitorings~\cite{trafficvision, traffictechnologytoday, goodvision,intuvisiontech, vision-zero, msr}, analyze the information from multiple types of sensors (including camera, LiDAR and Radar sensors) to enable long-range vehicle and pedestrian detection for autonomous driving~\cite{tusimple,waymo,motional}.
% The input data stream varies a lot over time.
% For example, in autonomous driving, the number and the moving speed of vehicles and pedestrians varies a lot over time (\eg the number of vehicles and humans will be much higher when driving in daytime), areas (\eg the vehicle movement speed is much higher when driving in the highway), current location (\eg the number of pedestrains will be much higher at the crossroad), traffic condition (\eg the number of vehicles significantly increases in traffic congestion).
% \jc{highlight the need for tuning configuration knobs when you bring up "data stream varies over time"}
% This trend inspires system research for these applications~\cite{vigil,glimpse,mcdnn,videostorm,noscope,neurosurgeon,awstream,chameleon,focus,adascale,filterforward,vstore,cracking,dds,reducto,blazeit,yoda,vcm,elf,ekya}.
% % \jc{can we cite some dnn-based analytics systems use cases, where the input distribution varies over time, in terms of frequency of object occurrences, shape/size, etc? be as concrete as possible please} \kt{done}

% Deep-neural-network-based (DNN-based) analytics on data streams (\eg video
% streams or LiDAR feeds) are everywhere.

\kt{Rewrote this para.}
Many applications send data streams to DNNs for analytical purposes.
% Many applications rely on DNNs to perform accurate inference on various data streams (\eg video streams or LiDAR feeds).
For example, DNNs are used to analyze traffic video feeds to monitor vehicle speed and spot traffic jams~\cite{trafficvision, traffictechnologytoday, goodvision,intuvisiontech, vision-zero, msr} , and analyze data streams from infrared cameras, LiDAR sensors, and radar sensors to detect vehicles and pedestrians for autonomous driving~\cite{tusimple,waymo-blog,motional}.
% \jc{kuntai, the logic here is quite muddy.. it's unclear why content varying over time is interesting/important. 
% maybe try a different flow: as these DNN-based applications require high accuracy, they use a great amount of compute and network resource. 
% Many prior efforts have leveraged a common feature of these data streams: their content varies greatly over time. 
% For example...
% To leverage these opportunities, recent work exposes...
% }
As these DNN-based applications require high accuracy, they use a great amount of GPU compute and/or network resources, which makes DNN-based applications too expensive for people to afford\kt{citation here}.
Fortunately, many prior efforts identify a resource-saving opportunity: the content of the data stream varies a lot over time and some of the content allows these applications to generate accurate analytic results with \textit{much less} resource usage.
% (\ie the amount of resource required to provide accurate analytic results) varies alongside with the content of the data stream, and reduce the resource usage by using less resource when resource demand is low.
% To reduce the resource usage, many prior efforts identifies the variability of the content of the data stream.
% a common characteristic of these data streams---their contents vary greatly over time---to reduce the resource usage of these DNN-based applications.
% The content of these data streams vary greatly over time.
% For example, in autonomous driving, the number and the moving speed of vehicles are constantly changing over time (\eg the number of vehicles will be much higher compared to driving in night time), location (\eg cars move faster on the highway) and traffic condition (\eg the number of vehicles significantly increases in traffic congestion).
% For example, in dashcam video streams, the number and the moving speed of vehicles are constantly changing over time (\eg the number of vehicles will be much larger during daytime than during night), location (\eg cars move faster on the highway) and traffic conditions (\eg the number of vehicles significantly increases in traffic congestion).
% For example, in one traffic video stream that aims to localize vehicles on a traffic lane,
For example, in a traffic video stream, the moving speed of vehicles can be much lower during red traffic light compared to green traffic light, so one can analyze less frames during red traffic light (and thus save GPU compute resource) and still accurately capture the motion of the vehicles.
% \jc{highlight the need for tuning configuration knobs when you bring up "data stream varies over time"}
% Facing this trend, the system research community develop \textit{adaptation-required knobs} to \textit{enable} saving resources when the data can be safely analyzed by using less resource without hurting accuracy and timely \textit{adapt} these knobs to save resource when such data appears. ~\cite{vigil,glimpse,mcdnn,videostorm,noscope,neurosurgeon,awstream,chameleon,focus,adascale,filterforward,vstore,cracking,dds,reducto,blazeit,yoda,vcm,elf,ekya}.
% To save resources through such temporal variability in the data streams,
Technically, to capture such resource-saving opportunity,
recent proposals~\cite{vigil,glimpse,mcdnn,videostorm,noscope,neurosurgeon,awstream,chameleon,focus,adascale,filterforward,vstore,cracking,dds,reducto,blazeit,yoda,vcm,elf,ekya} expose internal tunable parameters (referred to as \textit{knobs}) and \textit{timely configure} these knobs (we denote the knobs together with their configured values as a \textit{configuration}) according to the content of the data streams to save resources (\eg GPU compute and network) while maintaining high inference accuracy.
% \jc{can we cite some dnn-based analytics systems use cases, where the input distribution varies over time, in terms of frequency of object occurrences, shape/size, etc? be as concrete as possible please} \kt{done}



% \jc{how about we pitch them as two parallel trends: (1) temporal variation of input, and (2) an increasingly number of knobs, $\rightarrow$ the challenge of timely adaptation in a large configuration space.}

% We observe that these systems expose an \textit{increasing} number of internal knobs.
% The underlying trend that drives this increase is two-fold (further discussion in \S\ref{subsec:numer_of_knobs}). 
% % First, these systems need to develop new knobs to not only provide accurate analytic results under all kinds of resource budget due to heterogeneous deployment settings, but to also handle new emerging applications (\eg LiDAR-based object detection for autonomous driving and infrared-based human detection for night-time security monitoring).
% First, these systems need to develop new knobs to not only trade-off between the accuracy and different kind of resources in order to handle all kinds of resource budget due to heterogeneous deployment settings, but to also handle new emerging applications (\eg LiDAR-based object detection for autonomous driving and infrared-based human detection for night-time security monitoring).
% \ga{It'll be helpful to make it explicit that knobs also regulate the resource demand and hence can be used to handle heterogeneous resource budget.}
% \kt{fixed}
% % These knobs trade-off between accuracy and different kinds of resource in order to
% Second, as the need of DNN-based analytics quickly grow, these systems need to tune existing type of knobs at a finer granularity to support more concurrent DNN-based analytic jobs. \ga{The need to partition isn't clear. Why were the knobs joined in the first place, before partitioning?} \kt{fixed}

We observe that there is already a broad set of knobs\footnote{Previous work proposes at least 16 knobs includes 6 video encoding knobs~\cite{vstore, chameleon, dds, videostorm, awstream}, 9 frame filtering knobs~\cite{reducto, vigil, glimpse}, and the knobs that differentiate spatial video quality knob~\cite{dds,accmpeg,eaar}, which can be partitioned into thousands of knobs if tuned in fine granularity~\cite{accmpeg}.}\cite{vstore,chameleon,dds,videostorm,awstream,reducto,vigil,glimpse,dds,accmpeg}, 
and the set is still growing, thanks to two trends.
% We observe that the number of such configuration knobs is already huge (\eg more than 16 different knobs\footnote{These 16 knobs includes 6 video encoding knobs~\cite{vstore,chameleon,dds,videostorm,awstream}, 9 frame filtering knobs~\cite{reducto,vigil,glimpse}, and the knobs that differentiate spatial video quality knob~\cite{dds,accmpeg}, which can be partitioned to thousands of knobs if tuned in a fine granularity.} are introduced in video analytic systems~\cite{vstore,chameleon,dds,videostorm,awstream,reducto,vigil,glimpse,accmpeg}) and is still expanding.
% We observe that these systems expose an expanding set of configuration knobs that leverages temporal variabilities in the data stream to save resource without hurting the accuracy.
% % be adapted to the temporal variations of the input data stream to save resource.
% There are two reasons behind this trend. 
% First, these systems need to develop new knobs to not only provide accurate analytic results under all kinds of resource budget due to heterogeneous deployment settings, but to also handle new emerging applications (\eg LiDAR-based object detection for autonomous driving and infrared-based human detection for night-time security monitoring).
First, when people deploy DNN-based analytic systems into practice, they found that these systems need more knobs to explore new resource-saving opportunities introduced by new types of data streams (\eg LiDAR feeds), new applications (\eg video captioning) and new deployment settings (\eg multi-camera video analytics~\cite{chameleon, vigil}, multi-server video analytics~\cite{elf}).
% First, these systems need more knobs to not only trade between different type of resources to fit into more deployment settings (\eg the user may stream the data out from cheap camera through expensive LTE network for analytics. In this case, it is more ideal for the system to trade server-side compute for bandwidth~\cite{dds,eaar} instead of trade camera-side compute for bandwidth~\cite{vigil,glimpse,accmpeg} to simultaneously reduce the bandwidth usage without  the camera-side compute usage), but to also 
% \ga{It'll be helpful to make it explicit that knobs also regulate the resource demand and hence can be used to handle heterogeneous resource budget.}
% \kt{fixed}
% These knobs trade-off between accuracy and different kinds of resource in order to
Second, as these systems need to run more analytic jobs than before,
% these systems need to support more concurrent analytic jobs under the same resource budget, which requires them to 
they need to tune existing knobs at a finer granularity (by partitioning existing knobs into \textit{multiple} fine-grained knobs) to further reduce the resource usage of each analytic job.
% further reduce the resource demand for running one analytic job without hurting the accuracy.
For example, in a dashcam video stream, when the input video contains \textit{only one} small object, one may need to encode \textit{the whole video} in high fidelity in order to make this object detected, resulting in high bandwidth usage~\cite{chameleon,awstream}.
% when the input video contains one small object, one may need to encode and stream the whole video into high resolution to detect such object, resulting in high bandwidth usage~\cite{chameleon,awstream}.
However, prior effort~\cite{dds,eaar,accmpeg} shows that the areas that are not related to the object can be encoded in low fidelity to save bandwidth and realizes this potential by \textit{partitioning} the video into different areas and assigning different areas with different fidelities.
% , by assigning different areas with different resolutions\footnote{In fact, prior work assigns different areas with different quantization parameters, a parameter that controls the fidelity of the encoded video without changing the resolution. We use resolution in the text for understandability consideration.}, it only needs to encode the area that contains the object into high resolution and other areas can be safely encoded in low resolution. This significantly reduces the bandwidth usage.

% % redirected enumerate to packedenumerate for reformater in macro.tex. DON'T
% % CHANGE!
% \begin{enumerate}
%   \item 
% As DNN-based analytics are deployed on heterogeneous deployment settings that have different types of resource budgets, this requires the corresponding systems to propose new knobs in order to fit into
% different resource budgets. Take video analytics as an example. If the
% user analyzes the video feeds locally by a compute-constrained mobile
% phone, the main focus for the systems is to fit into the compute budget
% of the phone (\eg by skipping those frames that are highly similar to
% their previous frames~\cite{reducto,glimpse}). However, if the user
% instead streams the video feeds to a GPU-equipped server through a
% bandwidth-limited LTE network, the main focus is instead fitting into
% the limited LTE bandwidth (\eg by performing video
% compression~\cite{accmpeg,vigil,glimpse,reducto}).

%   \item As DNN-based analytics quickly expand, the corresponding systems need to
%         partition existing knobs into more fine-grained version to capture more
%         resource-saving opportunities. Take video-based vehicle detection as an
%         example. Chameleon~\cite{chameleon} and AWStream~\cite{awstream}
%         identify that the system only need to encode the video in a high
%         encoding quality when the vehicle appears. To further explore the
%         potential of varying video encoding quality, the following
%         work~\cite{dds,eaar,accmpeg} finds that a lot of areas in the video do
%         not need to be encoded in high quality (\eg the areas that contain
%         non-vehicle-related backgrounds like trees and buildings) and proposes
%         fine-grained spatial encoding quality to capture this opportunity.
%   \item Since new applications quickly emerge (\eg LiDAR-based object detection,
%         Infrared-based human detection \kt{a bunch of citations here}), this requires the deep learning systems
%         to develop new knobs (or even developing new system components) to fit
%         into the need of different applications. For example, in order to handle
%         LiDAR data, people are proposing new encoding standard and new
%         knobs~\cite{MPEG-point} to efficiently encode and process LiDAR data.
%         \roy{I understand you are trying to distinguish old types of application
%         and new ones, but I still feel the first and third items are kind of
%         repetitive? Both items are trying to say there is the need for new
%         knobs, right? Maybe merge them into one?}
% \end{enumerate}

% Not only the number of knobs are already huge (\eg in video analytics, previous work introduces 6 video codec encoding knobs~\cite{vstore,chameleon,dds,videostorm,awstream}, 9 frame filtering knobs~\cite{reducto,vigil,glimpse} and even thousands of knobs for fine-grained video encoding quality assignment~\cite{accmpeg}) and still expanding
% % \ga{Quantify.}
% , these knobs also need to be timely adapted~\cite{awstream,chameleon,dds,eaar,elf} due to input data change or resource budget change in order to achieve high inference accuracy.
% Thus, the research question is: how to navigate the large configuration space (\ie all possible choices of knob values) and and pick the optimal configuration that generates accurate inference results under the current resource budget?


% As the number of knobs are already huge (\eg more than 16 different knobs\footnote{These 16 knobs includes 6 video encoding knobs~\cite{vstore,chameleon,dds,videostorm,awstream}, 9 frame filtering knobs~\cite{reducto,vigil,glimpse}, and the knobs that differentiate spatial video quality knob~\cite{dds,accmpeg}, which may include thousands of knobs if tuned in a fine granularity.} are introduced in video analytic systems~\cite{vstore,chameleon,dds,videostorm,awstream,reducto,vigil,glimpse,accmpeg}) and is still expanding,
% \ga{Quantify.}
% , these knobs also need to be timely adapted~\cite{awstream,chameleon,dds,eaar,elf} due to input data change or resource budget change in order to achieve high inference accuracy.
Given the \textit{large yet expanding} set of knobs, the research question of this paper is:
\textit{among a large number of configurations, how to quickly adapt to optimal configuration that achieves high accuracy under a given resource budget?}


The first way to address this problem is to frequently profile different configurations to obtain their resource usage and accuracy, and then pick the configuration that yeilds high inference accuracy without exceeding the resource budgets\cite{chameleon,awstream,vstore,videostorm}.
% meets the resource
% budget and generates the most accurate inference results
However, each profiling
needs to run \textit{extra} inference to analyze multiple configurations (some are expensive in terms of resource usage). %before obtaining the profile.
% As a result, when the optimal configuration changes, this approach need to perform the extra inference to obtain the new optimal configuration, thus incurring high delay when the GPU resource is limited.
Thus, when the GPU compute is limited, this approach needs to either profile less frequently, resulting in using outdated configurations when the optimal configuration has drifted away, or significantly prune the search space (which may contain only suboptimal configurations). %profile fewer configurations, which may miss the optimal configuration. 
% Both of them lead to a sub-optimal trade-off between the accuracy and the resource usage.
% \ga{Call out the downsides of extra inference.} \kt{fixed}









% \kt{This para needs a rewrite}
% The other approach performs no extra inference and instead, computes the
% configuration based on recent DNN outputs (including intermediate outputs) through cheap heuristics~\cite{dds,eaar,elf} or through DNN-based configuration generator~\cite{accmpeg,casva}). 
% \ga{What does ``derives the configuration'' mean?} \kt{fixed}
% % However, there can be many configurations that meet the resource budget. \ga{There has been no mention of budget so far.}
% % Without profiling most of them, it is difficult to separate the configurations that yield similar DNN output from those that yield more accurate DNN output by merely looking at recent DNN outputs.
% % As a result, this approach waste resource on those configurations that yield similar DNN output and thus cannot quickly adapt to the optimal configuration. 
% \ga{I don't fully follow this paragraph and it needs more explanation. That said, can I view the techniques in this paragraph as a pruning mechanism to identify the promising configurations?}
% \kt{This para needs a rewrite}
\kt{rewrote the next 3 paras}
The second approach~\cite{dds,eaar,elf} performs no extra inference and instead generate new configuration by leveraging region proposal (DNN-generated bounding boxes that may contain objects inside).
For example, based on the region proposal of the current frame, EAAR~\cite{eaar} encodes the bounding boxes inside the region proposal of the current video frame  in higher encoding quality on future frames so that the objects inside the region proposals are more likely to be detected.
However, this approach may generate sub-optimal configuration, as this approach assigns the \textit{same} configuration (\eg encoding quality~\cite{dds,eaar}) for all the pixels inside each bounding box (unless multiple regions overlap) while an optimal configuration may assign \textit{different} configuration for different pixels inside a bounding box.
For example, \kt{plot a figure here.}
% This is sub-optimal as some pixels inside the bounding box can be in lower encoding quality (\eg those pixels that are outside the object but inside the region) and some pixels outside the bounding boxes may require higher encoding quality.
% However, instead of comparing between different configurations, this approach generates new configuration by postprocessing region proposals.
% As a result, it can only explore those configurations that are generatable from the heuristics, which may miss the optimal configuration that may not be generatable from the heuristics.
% For example, EAAR~\cite{eaar} encodes the regions inside the region proposals with higher encoding quality so that the objects inside the region proposals are more likely to be detected.
% However, as shown by AccMPEG\cite{accmpeg}, not all pixels inside the region proposal need to be in higher quality, and some pixels outside the region proposal needs to be in higher quality.





% based on recent DNN outputs (including intermediate outputs)~\cite{dds,eaar,elf,accmpeg,casva}.
% % \jc{i still dont quite get why we use dds here. isn't some bandit/RL-based solution a better fit?}
% % For instance, DDS~\cite{dds} tunes encoding quality by first encoding all pixels at a low quality and streaming them to the server-side DNN, whose output (region proposal) is then used to tune the quality at different regions.
% Though no extra inference is run, this approach tends to adapt {\em slowly}, as each DNN output reveals limited information regarding the \textit{highly complex} relationship between the configurations and DNN inference output/accuracy, due to the complexity of the DNN itself and the preprocessing modules before the DNN (\eg video codecs).
% We take EAAR~\cite{eaar}, a system for video object detection, as an example.
% EAAR adjusts the video encoding quality by collecting the regions from the DNN that may contain objects of interest and encoding these regions in higher encoding quality on future video frames.
% % After that, it encodes these regions in high quality on the next video frame.
% Thus, the objects inside these regions are much more likely to be detected.
% % This approach then lets the sensor encode all these regions in high encoding quality on the next video frame so that the objects inside these regions can be accurately detected.
% However, as the regions generated by the DNN may not include all the regions that contain the objects, the object detection DNN may miss some objects and thus EAAR needs to further adjust the regions corresponding to these missing objects.
% For instance, the impact of configuration on DNN accuracy is affected by two complex blackboxes: DNN itself as well as the video codecs.
% However, the \textit{adaptation speed} (\ie the time it takes to obtain the optimal configuration) of this approach can be slow.
% For example, DDS~\cite{dds} tunes the encoding quality of different areas of the video in the following steps.
% First, DDS let the camera encode the whole video into low quality and stream it to the server.
% The server then analyzes the video to obtain the areas that may contain objects and let the camera resend those areas in high encoding quality for an extra round of inference.
% % through cheap heuristics~\cite{dds,eaar,elf} or through DNN-based configuration generator~\cite{accmpeg,casva}).
% However, the \textit{adaptation speed} (\ie the time it takes to obtain the optimal configuration) of this approach can be slow.
% % explore many configurations to accumulate enough DNN outputs before converging to the optimal one.
% % need to accumulate enough DNN outputs in order to obtain the optimal configuration.
% % This is because this approach only examine one configuration at a time.
% This is because they only get one DNN output at a time.
% As the relationship between the configuration to the inference accuracy is highly complex (due to complexity inside the underlying system (\eg video codec) and the DNN itself), this approach needs to spend time accumulating enough DNN outputs before obtaining the optimal configuration, resulting in slow adaptation speed.
% Thus, it is difficult to identify whether a new configuration improves accuracy or not based on the current DNN output.
% the performance of other configurations.
% the DNN ouput on just one configuration is not enough for this approach to immediately obtain the optimal configuration thus
% As a result, 
% this approach needs to accumulate enough DNN outputs to reach the optimal configuration. 
% The optimal configuration may have already changed (due to the change of input content or resource budget) before this approach reaching it.
% The optimal configuration may have already changed.

% However, there can be many configurations that meet the resource budget.
% Without profiling most of them, it is difficult to separate the configurations that yield similar DNN output from those that yield more accurate DNN output by merely looking at recent DNN outputs.
% As a result, this approach waste resource on those configurations that yield similar DNN output and thus cannot quickly adapt to the optimal configuration. 


Moreover, the heuristics used in the second approach are designed for specific types of knobs and are not directly applicable to other knobs (though these heuristics \textit{could} be augmented and used to adapt other knobs).
% even if they can be purposely built to efficiently support some knobs. 
% are hand-crafted for individual applications or configurations and thus not generalizable to other configurations and applications.
For example, EAAR~\cite{eaar} generates new configuration of future frames based on region proposal of the current frame.
As a result, EAAR may not be ideal for tuning, for example, determining whether to analyze this frame or not.
This is because the optimal configuration of this frame may vary a lot compared to next frame.
% This is because  as these knobs require the system to analyze the temporal characteristics of these frame, which are not analyzed by EAAR.
% We take EAAR~\cite{eaar}, a system that serves object detection, as an example.
% EAAR assigns the regions that may contain objects based on the current frame and encodes these regions with higher encoding quality to in the future frames to make more objects detected.
% In a higher level, EAAR applies the decision generated from the current frame to the future frames.
% However, this may not be a suitable way to adapt the knobs that, for example, decide which video frames can bypass the DNN inference.
% This is because the optimal decision may vary a lot between the current frame and the future frames: if the current frame needs to be forwarded through the DNN, it is more likely that the next frame should bypass the DNN inference.
% As a result, EAAR may not directly apply to the DNN-bypassing knobs.



The third approach trains models (\eg saliency generator~\cite{accmpeg,??} or configuration generator~\cite{casva}) and leverages these models to generate new configuration.
However, the accuracy of these models degrade over time and are not accurate enough to generate optimal configuration when the characteristics of the input data changes (\eg when a remote small object appears in the video). 
% unless these models are as complex as the DNN and the.
This is because the mapping between the input and its corresponding optimal configuration is highly complex due to the complexity of the DNN itself and the preprocessing modules before the DNN (\eg video codecs~\cite{h265,h264}).
\kt{an example figure to support this point.}
As a result, these models is not able to accurately learn this mapping (unless these models are as complex as the DNN and the preprocessing modules) and may produce sub-optimal configurations when the content of the input data shifts (\eg when a drone quickly flies away the ground), unless these models are frequently retrained, which requires extra inference to label the optimal configuration before retraining starts.
% and then leverage this model to adapt the configuration.
% However, as the compute of such model is limited due to \fillme, the model may no longer being able to predict the optimal configuration when the input content changes.
% For example, \fillme.





% Moreover, the heuristics used in the second approach are designed for specific types of knobs and are not directly applicable to other knobs (though these heuristics \textit{could} be augmented and used to adapt other knobs).
% % even if they can be purposely built to efficiently support some knobs. 
% % are hand-crafted for individual applications or configurations and thus not generalizable to other configurations and applications.
% We take EAAR~\cite{eaar}, a system that serves object detection, as an example.
% EAAR assigns the regions that may contain objects based on the current frame and encodes these regions with higher encoding quality to in the future frames to make more objects detected.
% In a higher level, EAAR applies the decision generated from the current frame to the future frames.
% However, this may not be a suitable way to adapt the knobs that, for example, decide which video frames can bypass the DNN inference.
% This is because the optimal decision may vary a lot between the current frame and the future frames: if the current frame needs to be forwarded through the DNN, it is more likely that the next frame should bypass the DNN inference.
% As a result, EAAR may not directly apply to the DNN-bypassing knobs.
% However, EAAR may be sub-optimal if applied to the knobs that decide which video frames can bypass the DNN inference without hurting the inference accuracy.
% This is because EAAR make an assumption that do not fit this set of knobs.
% Concretely, the current design of EAAR generates the configuration on one frame and apply it to the future frames, which assumes that the optimal knobs on one frame generalizes to the future frames.
% However, this assumption may not be true in the scenario of bypassing DNN inference: if one frame needs to be forwarded through the DNN, it is more likely that the next frame should bypass the DNN inference, and vise versa.
% The violation of this assumption results in the sub-optimal adaptation behavior of EAAR: EAAR may continuously performing inference on a few frames and then continuously bypassing the DNN inference on the next few frames, while the optimal way is to perform inference intermittently.
% This 
% This is because making such decision requires the adaptation algorithm to analyze these frames without performing DNN inference on these frames, while the current design of EAAR lets the DNN ingest this frame first and then analyze this frame leverage the intermediate analytical results on this frame for further use.
% performing DNN inference on this frame and then harnessing the intermediate outputs generated by the DNN inferences. 
% As a result, EAAR either obtains no extra information on one frame besides the pixel values of this frame (thus cannot make accurate decision on whether letting this frame bypassing DNN inference or not), or analyzes this frame at the cost of performing DNN inference (thus this frame cannot bypass the DNN inference).
% does not extract any information of one frame  while the current design of EAAR always inference on the current frame and are agnostic to the future frames.
% making such a decision requires estimating the similarity of the inference results, between those discarded frames and reserved frames, while EAAR focusing on extracting the regions that may contain objects, where only a small subset of them will appear in the final inference results.
% Take DDS~\cite{dds} as an example, which analyzes the video and then resends some areas of the video that may contain objects of higher fidelity.
% As the recent areas are derived from the output of a specific DNN component (region proposal) that aims to facilitate object detection, this heuristic is not directly applicable to tasks like video classification.
% Moreover, this heuristic does not apply to tune frame-discarding knobs~\cite{vigil,glimpse,reducto} that discard similar frames to save GPU compute, because the way DDS obtains the output to tune the knobs incur more GPU compute in the first place. 
% the knobs in frame discarding techniques 
% (\ie discarding the frames that produce similar inference results compared to previous frames~\cite{vigil,glimpse,reducto}) without further adjustments, since its adaptation logic (\ie resending some areas of the video that may contain objects) happens \textit{after} DNN inference while frame filtering needs to be performed \textit{before} DNN inference to save GPU compute cost. 
% As a result, DDS does not directly generalize to other 
% \ga{How is this paragraph on DDS pertaining to profiling and avoiding extra inference? The relationship isn't clear.} \kt{fixed}
% \jc{not sure ganesh's comment was addressed. i think the confusion is whether you are criticizing dds's logic being inefficient or not generalizable. if it's the latter, just say it explicitly.}


% An ideal configuration adaptation system should meet these two
% requirements: 1. quickly adapt to optimal configuration in a large configuration
% space without extra inference 2. minimum assumption to the underlying system.

Therefore, an ideal configuration adaptation system needs to serve \textit{a wide range of knobs}, and compare between different configurations formed by these knobs  \textit{without extra inference}.

% \kt{Pitch the cause of the previous work limitation as they only using DNN outputs -- which can change a lot between different configuration and video content -- to predict the performance on unknown configuration and unknown content.
% Our approach combines the DNN parameters -- which does not change between different configuration and video content -- to better generalize the prediction of the performance on unknown configuration and unknown content.
% }

% \jc{i guess the rest of the intro hasn't been updated since last wednesday. just to recap, here's the flow:
% \begin{packeditemize}
%     \item start with a new abstraction, \accgrad, to more efficiently adapt configurations than prior schemes, especially in a large configuration space, and why?
%     we present \name, the first efficient implementation of \accgrad
%     we should clarify that prior work could expose this abstraction as well, but they suffer high overhead (why?). 
%     \item \name approximates \accgrad based on two observations: 
%     (1) the values of each configuration can be ordered in a way that \fillme, and
%     (2) the more changes of confidence scores around the threshold, the more accuracy will change.
%     \item based on the two observations, \name does \fillme
%     \item operators can use \name to tune a range of configurations that influences dnn input. this class of config covers many existing systems. but notably, this doesn't cover \fillme (may point to a synergy with recent online learning papers like ekya --- in some sense, they also handle input drift, but they choose to retrain the model, and our approach is more lightweight.)
% \end{packeditemize}}

% \kt{Stress that knob is trading res usage for acc}
% \kt{Adaptation goal: expose an abstraction: monitoring both }

% \kt{
% Expose 1 abstraction:
% resource-knob gradient
% DNN output (We use the change of confidence values around the threshold, see \S\ref{??} for further detail) gradient
% % confidence change gradient
% Say it correlates with accuracy?
% With this gradient, we can 1). efficiently optimize knobs

% Previous work, if repurposed, incurs extra inference.

% Advantage: can be calculated without extra inference
% }


% To realize these two objectives, we expose a new abstraction: , which means the performance change divided by knobs change when changing the knobs by a little.
% Concretely, performance gradient includes resource usage gradient, and DNN output gradient (we measure the DNN output change by measuring the absolute change of confidence scores around the confidence threshold. See \S\ref{??} for further details).


\kt{rewrote this part}
We advocate that the adaptation system for DNN-based analytics should expose a new abstraction: \textit{\outputgrad}, which estimates \textit{the gradient of DNN output with respect to each knob}.
We present \name, a system that implements \outputgrad and uses it to adapt configurations with constant GPU overhead and no extra inference.
% Based on \outputgrad, we present \name, a configuration adaptation system that implements \outputgrad with constant GPU overhead and with no extra inference.
% Specifically, \name measures \outputgrad by how much a small change in the current value of each knob \textit{flips} the DNN-returned confidence scores from below (or above) the confidence threshold to above (or below). 
Specifically, \name measures \outputgrad by how much a small change in the current value of each knob changes the output\footnote{We measure the change of output by summing up all values inside the output and measuring the change of the sum}.
% We measure \outputgrad by how much a small change in the current value of each knob affects the DNN-returned confidence scores near (both below and above) the given confidence threshold.
% Note that this measurement does not impose an extra burden on the application side since most of the applications already expose confidence scores to indicate the uncertainty of DNN outputs and use confidence thresholds to filter out DNN outputs with low confidence. %those uncertain results returned from the DNN.
One may question that why \name studies the output of the DNN instead of the accuracy of the application.
To answer this question, \name makes an assumption: when we \textit{only} change the value of \textit{one single knob} in a way that makes the system consume more resource, \textit{statistically} the accuracy will be improved. Moreover, more change on the output, more accuracy improvement.
We empirically validate that this assumption over a wide range of knobs and applications (see \S\ref{??} for details).
% We will talk about the applicability and the 
% Moreover, more change in the output, more improvement on accuracy (see \S\ref{??} for more rationales).
% We 
%those uncertain results returned from the DNN.
% Statistically, more changes in the ``near-confidence-threshold'' DNN outputs will likely cause more changes in the inference accuracy (as will be elaborated in \S\ref{subsec:correlation})\footnote{This correlation does \textit{not} assume that a confidence score always directly indicates the accuracy of its corresponding detection/classification results.}.
% % \outputgrad correlates with how much the accuracy \textit{changes} with knobs 
% Intuitively, this is because the confidence threshold determines whether a detection or classification result is accepted (as part of the accuracy calculation) or rejected (thus having no effect on the accuracy).
% When the knob change only alters the DNN output by a little, the corresponding accuracy change also tends to be minor.
% Thus, more change on the ``near-threshold'' DNN outputs, more changes on the inference accuracy.




% how much the DNN output changes when varying each individual knob by a little (we measure the DNN output change by measuring the change of those confidence scores around the confidence threshold, see \S\ref{??} for the mathematical formulation and the intuition behind).
% We call this metric \outputgrad for short.
% when slightly changing the knob  (we call it \outputgrad for short).
% We will cover the detail


% \kt{Should we allocate a paragraph to talk about the overhead of calculating ground truth here?}
% We acknowledge that using DNN output change cannot obtain the exact number of the accuracy change.
% However, we still think that this is a valuable choice, as
% directly calculating this accuracy change requires the underlying system to obtain the ground truth first (previous work define the ground truth as the inference results generated under the most expensive configuration to avoid the need for human annotation~\cite{dds,awstream,chameleon,vstore,videostorm,ekya,focus}).
% This imposes non-trivial overhead due to extra inference on the most expensive configuration (\eg in Chameleon~\cite{chameleon}, calculating the ground truth\footnote{Chameleon is actually calculating multiple
% resource-consuming configurations as the ``ground truth'', but the overhead is
% still due to calculating ground truth.} consumes $\sim$50\% of the overall GPU
% compute). 



With the \outputgrad, the adaptation system can quickly adapt to the optimal configuration by assigning more resources to the knobs with high \outputgrad to improve the accuracy, or cut the resource usage of the knobs with low \outputgrad without hurting the accuracy.


However, it can be expensive to calculate \outputgrad over a space of many knobs. %may incur high amount of extra inference.
% This is because previous work needs to calculate \outputgrad in a knob-by-knob manner (\ie inference on the DNN and calculate the DNN output change by alternating the value of one knob while fixing other knobs, and repeat this process for all knobs). 
Previous work~\cite{chameleon,vstore,videostorm,awstream} would have had to calculate \outputgrad in a knob-by-knob manner (\ie inference on the DNN and calculate the DNN output change by alternating the value of one knob while fixing other knobs, and repeat this process for all knobs). 
% Thus, one more knob, one more extra inference.
% Thus, more knobs will lead to more inference.


To avoid such extra inference, \name leverages the \textit{differentiability} of the DNN to implement \outputgrad with constant GPU overhead and with no extra inference.
% We show that \outputgrad, the first system that implements can be calculated without any extra inference and with constant GPU overhead.
% We develop \name, a configuration adaptation system that optimizes the configuration based on \outputgrad.
% The insight of \name is to leverage the \textit{differentiability} of DNN to reduce the cost of calculating \outputgrad.
We {\em decouple} the calculation of \outputgrad (\ie how changing the knobs alters the DNN output) to how changing system knobs alters the DNN input and how changing the DNN input alters the DNN output.
% Concretely, in order to calculate how changing the knobs alters the DNN output (\ie \outputgrad), we can calculate how changing system knobs alters the DNN input, and then calculate how changing the DNN input alters the DNN output.
% \kt{Should we add a math formula of chain rule here? Like output/knob = output/input * input/knob?}
The former can be calculated in a knob-by-knob manner without DNN inference (\ie no GPU compute), and the latter can be obtained via {\em backpropagation} (which is a constant GPU overhead without extra inference as it can reuse the existing computation graph of DNN inference).

% We show that \outputgrad can be calculated with constant GPU overhead and without any extra inference, regardless of the number of the knobs, and develop \name, a configuration adaptation system, that optimizes the knobs based on \outputgrad.
% \name reduces the cost of extra inference by treating \outputgrad as an actual gradient and leveraging the following two properties to decouple this gradient through the chain rule.
% % \kt{I feel like this is the place to introduce the separation of the knob side v.s. the DNN side, as this separation is used (and only used) to reduce the cost of calculating the gradient}
% \begin{packeditemize}
%     \item 
%     On the DNN side, the DNN output is differentiable to its input (via backpropagation algorithm).
%     Thus, calculating how changing the DNN input alters the DNN output requires no extra inference.
%     \item
%     On the knob side, a wide range, \textit{not all}, of the knobs treat DNN as a \textit{black box} and affect DNN inference results solely by changing the DNN input.
%     As a result, calculating how changing each individual knob alters DNN input requires no extra inference.
% \end{packeditemize}
% These two properties suggest that to calculate how changing the knobs alters the DNN output (\ie \outputgrad), we can first calculate how changing system knobs alters the DNN input, and then study how changing the DNN input alters the DNN output. 
% \kt{Should we add a math formula of chain rule here? Like output/knob = output/input * input/knob?}
% The former can be calculated in a knob-by-knob manner without the participant of the DNN (thus avoid extra DNN inference), and obtaining the latter only requires one backpropagation (this creates a constant GPU overhead, but it is reusing the computation graph created by existing DNN inference, thus incurring no extra inference).


Operators can use \name to tune a wide range of applications and knobs that influences DNN input (as shown in Table~\ref{tab:rich-set-of-knobs}).
That said, \name does {\em not} apply to all knobs and applications.
In terms of knobs, \name does {\em not} apply to knobs that alter the DNN itself, 
such as retraining the DNN weights~\cite{ekya,noscope,mcdnn}.
Similar to \name, they also adapt to changes in input distribution, they involve substantial computation and thus tend to happen at a coarser timescale than the knobs considered in \name. 
In terms of applications, \name does {\em not} apply to those applications that \fillme.
% such as customizing the DNN according to the current content of the input~\cite{ekya,noscope,mcdnn}.
% In some sense, both the DNN customization approach and \name are adapting to the varying content in the input data stream.
% However, in order to maintain high accuracy, DNN customization approach needs to retrain the DNN when the input content varies, and thus incurs high GPU overhead, while \name adapts the knobs inside the underlying system that serves the DNN, which is much more lightweight.


In short, the contributions of this paper are two-fold:
\begin{packeditemize}
    \item A new abstraction, \outputgrad, that enables quick adaptation of configurations for DNN-based analytics.
    % \item A new abstraction, \outputgrad, that enables the configuration adaptation framework for DNN-based analytic systems to quickly adapt to optimal configuration through \accgrad.
    \item A configuration adaptation system, \name, that implements \outputgrad with constant GPU overhead and without extra inference.
    % \item An implementation, \name, that implements \outputgrad with constant GPU overhead and with no extra inference.

\end{packeditemize}

We evaluate \name across 7 different DNN-based analytic pipelines and across 54 videos. \name achieves similar accuracy with 10-43\% end-to-end delay reduction, or achieves 1-10\% higher accuracy with similar end-to-end delay compared to the baselines on 8 different applications.
Also, we show that the performance gain of \name compared to the baselines becomes larger when there are more knobs or the knobs become more fine-grained.

\textbf{This work does not raise any ethical issues.}







% Expose abstraction:
% confidence change gradient with respect to resource


% Confidence scores -> a generalizable format
% Confidence thresholds -> a widely adopted component in the accuracy of applications in real world.

% % The key to achieve this goal is to calculate how much each knob changes the confidence scores that are close to the confidence thresholds 

% To quickly adapt to optimal configuration without extra inference, the intuition of \name is to allocate more resource to the knobs that maximally change the confidence scores inside the inference results that are around  with confidence scores \textit{around} the confidence thresholds.
% to maximally change \textit{which} inference results participants the accuracy
% Concretely, \name calculates 


% Why this works: two assumptions on the knobs 1. more resource, higher accuracy and 2. if the confidence scores around the confidence thresholds doesn't change, the accuracy barely change.

% We present \name that efficiently calculates such metric on each knob.
% The key for \name to success is to leverage the differentiability of DNN to \textit{predict} the performance of a run-time system.

% our approach is to: grant more resources to the knobs can maximally change the part of the inference results that the confidence scores are around the confidence thresholds, and cut the resource usage of those knobs that barely change 


% To quickly calculate this metric, we leverage the differentiability of the DNN to quickly obtain how DNN input affects the confidence scores around the confidence thresholds.



% We present our system: \name, which meets these two requirements. 
% To quickly adapt to optimal configuration, \name calculates the \textit{gradient} of accuracy with respect to each knob (hereinafter \accgrad, defined as the accuracy change if changing one knob valued by a little).
% % leverages a property of DNN-based analytic system knobs: for most of the knobs, if changing the value of one knob results in spending more (or less) resource, the corresponding inference result would statistically become more (or less) accurate.
% % This property suggests that each knob is able to \textit{trade resource for accuracy}.
% % To quantitatively measure this ability, \name calculates the \textit{gradient} of accuracy with respect to each knob (hereinafter \accgrad, defined as how changing each individual knob by a little alters the accuracy).
% With \accgrad, \name can quickly adapt to the optimal configuration in a
% large configuration space by allocating more resources to those knobs with
% high \accgrad to improve accuracy and cutting the resource usage of knobs with
% \accgrad to save resource without hurting accuracy.





% % insight that motivates \name is two properties we observe in deep learning
% % system knobs. The first property is: for most of the knobs, if changing the
% % value of one knob results in spending more (or less) resource, the corresponding
% % inference result would statistically become more (or less) accurate. This
% % property suggests that the change of accuracy with respect to knob value change
% % can reflect the ability of trading resource for accuracy for each individual
% % knob. With \accchange, \name can quickly adapt to the optimal configuration in a
% % large configuration space: \name can allocate more resources to those knobs with
% % high \accchange to improve accuracy and cut the resource usage of knobs with
% % \accchange to save resource without hurting accuracy.



% % There is one more challenge to calculate \accgrad.


% The first challenge of calculating \accgrad is: how to calculate the accuracy change when changing a knob value by a little?
% Directly calculating this accuracy change requires the underlying system to obtain the ground truth first (previous work define the ground truth as the inference results generated under the most expensive configuration to avoid the need for human annotation~\cite{dds,awstream,chameleon,vstore,videostorm,ekya,focus}).
% This imposes non-trivial overhead due to extra inference on the most expensive configuration (\eg in Chameleon~\cite{chameleon}, calculating the ground truth\footnote{Chameleon is actually calculating multiple
% resource-consuming configurations as the ``ground truth'', but the overhead is
% still due to calculating ground truth.} consumes $\sim$50\% of the overall GPU
% compute). 
% To resolve this issue, we develop a proxy for accuracy difference (we call this proxy \accproxy). 
% % The main idea is to reuse the existing inference results and measure the accuracy change if the same input
% % data \textit{were} processed by a new configuration. 
% Concretely, \accproxy estimates the sign and the magnitude of accuracy change by the following rule:
% \begin{packeditemize}
% \item 
% The \textit{sign} of accuracy change is determined by which input (between the two DNN input generated before and after changing one knob value) is of \textit{less distortion} compared to the DNN input generated under most expensive configuration.
% \item 
% We estimate the \textit{magnitude} of accuracy change through checking the \textit{dissimilarity} between the two inference results generated before and after the knob value change.
% The intuition behind this estimation is that: if the inference results generated before and after the knob change are highly similar, the inference accuracy of these two inference results should also be highly similar.
% \end{packeditemize}
% By using this proxy, calculating accuracy difference no longer relies on the generation of ground truth, and 


% However, even with the optimization above, trivially calculating \accgrad in a knob-by-knob manner (\ie
% calculate the accuracy change by alternating the value of one knob value
% while the value of other knobs value remaining unchanged, and repeat this process
% for all knobs) still requires extra inference to get the inference results after each knob value change. 
% To avoid such extra inference, \name leverages the following two properties:
% \begin{packeditemize}
%     \item
%     On the knobs side, most of the knobs treat DNN as a \textit{black box} and affect DNN inference results solely by changing the DNN input.
%     As a result, calculating how changing each individual knob alters DNN input requires no extra inference.
%     \item 
%     On the DNN side, the DNN itself is differentiable to its input (via backpropagation algorithm).
%     Thus, calculating how changing the DNN input alters the accuracy requires no extra inference.
% \end{packeditemize}
% These two properties suggest that to calculate how changing the system knobs alters the accuracy (\ie~\accgrad), we can first calculate how changing system knobs alters the DNN input, and then study how changing the DNN input alters the accuracy. 
% The former can be calculated in a knob-by-knob manner without the participant of the DNN (thus avoid extra DNN inference) and the latter only requires one backpropagation (thus incurring no extra inference).

% compared to the ground truth DNN input, and estimate the magnitude of accuracy
% change by comparing the difference of inference results between the old and the
% new configuration. 
% We find that the \textit{gradient} of this accuracy metric can be calculated \textit{without} extra inference.

% \begin{comment}

%   Deep learning applications on streaming data (\eg video streams or LiDAR
%   feeds) are everywhere. For example, in autonomous driving, people use video
%   cameras and LiDAR sensors and leverage object detection deep neural networks
%   (DNNs) to sense the surrounding environment and avoid potential collisions. In
%   augmented reality, people use video cameras and LiDAR sensors to localize the
%   remote objects and render the virtual objects on top of real objects. This
%   trend inspires system research for these applications, like live
%   analytics~\cite{??}, retrospective analytics~\cite{??}, database for analytic
%   purpose~\cite{vstore,noscope}, etc.

%   We identify two important characteristics of these systems. First, they
%   contain large configuration spaces (\eg in AWStream~\cite{awstream}, there are
%   216 different configurations inside its configuration space). Second, these
%   configurations need to be \textit{timely} adapted according to their input
%   (\eg we may want to use higher video resolution when a small car enters the
%   video frame in order to detect this small car) and the current resource budget
%   so that they can generate the inference results as accurate as possible.

%   As a result, the key challenge for these systems is: how to navigate the large
%   configuration space and pick the optimal configuration that generates the most
%   accurate inference results under the current resource budget.

%   The first way to address this problem is to \textit{frequently profile} the
%   system with different configurations to obtain their resource usage and
%   inference accuracy, and then pick the configuration that meets the resource
%   budget and generates the most accurate inference
%   results~\cite{awstream,chameleon,vstore}. However, in order to profile, this
%   approach has to perform \textit{extra} inference on the GPU, resulting in high
%   GPU cost.

%   The other approach performs no extra inference and instead, picks the
%   configuration based on the recent configuration and its corresponding DNN
%   output. However, there can be many configurations that meet the resource
%   budget. Without profiling most of them, it is difficult to separate the
%   configurations that yield similar DNN output from those that yield more
%   accurate DNN output. In addition, the previous work in this approach designs
%   hand-craft heuristics catered for different applications.

%   Thus, the requirements of an ideal configuration adaptation system are
%   three-fold:
%   \begin{enumerate}
%     \item No extra DNN inference
%     \item Pruning out the configurations with similar accuracy
%     \item Agnostic to the underlying applications
%   \end{enumerate}

%   We present our system: \name that meets these three requirements. The idea is
%   to calculate the \textit{gradient} of inference accuracy with respect to the
%   configurations to \textit{predict} which of them improve inference accuracy
%   and which do not. The key insight that enables us to calculate this gradient
%   is by decoupling this gradient into two terms. The first term is the gradient
%   of inference accuracy with respect to the DNN input, which can be calculated
%   by backpropagation without performing extra inference on any other
%   configuration. The second term is the gradient of the DNN input with respect
%   to the configurations, which does not require DNN inference.

%   To make our system practical, we also identify another source of overhead
%   introduced by calculating inference accuracy. In order to calculate inference
%   accuracy, previous work needs to refer to the configuration with \textit{the
%   most} resource usage and use the corresponding inference results as the
%   ``ground truth'' to evaluate the accuracy of inference results generated from
%   other configurations. Calculating the ``ground truth'' uses much higher
%   resource usage (including the streaming cost of streaming the data and the GPU
%   cost to generate inference results) than the current optimal configuration. To
%   reduce this cost, we introduce a \textit{proxy} of accuracy that
%   \textit{indirectly optimizes} accuracy by using the DNN input (instead of the
%   DNN output), thus requiring no DNN inference.

%   To conclude, the contributions of this paper are:
%   \begin{enumerate}
%     \item A way to calculate gradient with no extra inference
%     \item An accuracy proxy that indirectly optimizes the accuracy without
%           running extra inference.
%   \end{enumerate}
%   We quantitatively evaluate these two contributions, we perform experiments on
%   XXX datasets, XXX applications and XXX

% \end{comment}


==> intro_v5.tex <==

\tightsection{Introduction}
\label{sec:intro}

% \kt{Claim we generalize to other data sources}

% \kt{How timely identify a differentc onfiguration is better}

% % \kt{align the example here with the example that optimal config frequently changes}
% % \kt{add streaming aspect}
% Many applications rely on DNNs to perform accurate inference on various data streams (\eg video streams, audio streams and LiDAR feeds).
% For example, people collect data streams from various sensors (\eg infrared cameras, LiDAR sensors, and radar sensors)  and analyze them through DNNs to detect vehicles and pedestrains\cite{trafficvision, traffictechnologytoday, goodvision,intuvisiontech, vision-zero, msr,tusimple,waymo-blog,motional}.
% % people use DNNs to analyze traffic videos to monitor vehicle speed and spot traffic jams~ and to analyze data streams from other sensors (\eg infrared cameras, LiDAR sensors, and radar sensors) to detect vehicles and pedestrians for autonomous driving~.\jc{the text until here can be a bit tightened}
% % As the computation power on these sensors are restricted, they need to stream their data through networks to remote server for DNN-baesd inference~\cite{?,?}.
% % \kt{mention that data needs to be streamed to the server.}
% As these DNN-based applications require high accuracy, they use a great amount of bandwidth and/or GPU computation resources.
% % \jc{too vague. spill out GPU cycles and bandwidth.}
% Thus, practical systems for these applications may not have enough bandwidth to stream all uncompressed data from the sensor to the DNN (if the streaming is needed for analytics), and/or enough GPU compute resource to run DNN inference on all input data (\eg all frames of a video stream).
% % As a result, many prior efforts leverage the content of the input data to save resources without hurting the accuracy.
% As a result, many prior efforts save resources by identifying the content of the input data that can be analyzed with fewer resources without hurting accuracy.
% For instance, consider vehicle detection in a traffic monitoring video stream.
% When the red light appears, the speed of vehicles is slow, allowing the analytic system to reduce the frame sampling rate (thus minimizes the number of frames being analyzed) and still accurately determining the position and the movement of the vehicles.
% % \jc{too vague. why content can be leveraged to save resource? should be quite intuitive, so just a couple of short examples are enough. no need for long examples. }
% % For example, in dashcam video streams, the number and the moving speed of vehicles are constantly changing over 
% % time (\eg the number of vehicles will be much larger during daytime than during night), 
% % location (\eg cars move faster on the highway) and traffic conditions (\eg the number of vehicles significantly increases in traffic congestion).
% Technically, recent proposals~\cite{vigil,glimpse,mcdnn,videostorm,noscope,neurosurgeon,awstream,chameleon,focus,adascale,filterforward,vstore,cracking,dds,reducto,blazeit,yoda,vcm,elf,ekya} expose internal tunable parameters (referred to as \textit{configuration knobs}, see Table \ref{tab:rich-set-of-knobs} for a full list of configuration knobs) and timely \textit{configure} these knobs (we denote the knobs together with their configured values as a \textit{configuration}) according to the content of the input data, in a way that saves resources (in GPU compute and network) while maintaining high inference accuracy.
% \jc{not clear how and why knobs help leverage content to tune knobs.}
% \kt{I emphasized that prior work leverages the content of the input data to save resource, and gave an example. Hope that this is clearer}


% \kt{add configuration}

Many applications rely on deep neural nets (DNNs) for accurate inference on various types of input data\jc{this term was "data stream" but later you also used "data source". "input data" sounds more reasonable to me, but regardless, please do a pass to make this term consistent}~\cite{trafficvision, traffictechnologytoday, goodvision,intuvisiontech, vision-zero, msr,tusimple,waymo-blog,motional}.
%(\eg video, audio, and LiDAR feed)
For example, a DNN can analyze video frames to 
% people analyze data streams from various sensors (\eg infrared cameras, LiDAR sensors, and radar sensors) using DNNs to 
detect vehicles and pedestrians, or analyze an audio stream to extract text. 
These applications often run DNN inference on cloud/edge servers, causing resource contention in both {\bf network bandwidth} to stream high-fidelity data (\eg high-quality video) from distributed sensors to the analytics servers and in {\bf GPU compute cycles} to run expensive DNN inference on many data points (\eg each video frame).

\begin{comment}
As these DNN-based applications require high accuracy, they use a great amount of bandwidth and/or GPU computation resources.
Thus, practical systems for these applications may not have enough bandwidth to stream all uncompressed data from the sensor to the DNN (if the streaming is needed for analytics), and/or enough GPU compute resources to run DNN inference on all input data (\eg all frames of a video stream).
\end{comment}

% why setting knobs is key
Many previous efforts have shown that {\em optimally tuning a range of knobs} (\eg video frame rate and resolution) can greatly save resource usage and achieve high accuracy.
Table~\ref{tab:rich-set-of-knobs} shows a list of example knobs.
We use a {\em configuration} to refer to a particular setting of the knobs used by an application (\eg a particular frame rate and resolution).
% To mitigate resource contention, many prior efforts expose internal tunable parameters (hereinafter \textit{knobs}) and timely configure these knobs (we denote the knobs together with their configured values as a \textit{configuration}).
% have proposed to tune various knobs of these DNN-based analytics systems. 
% expose internal tunable parameters (referred to as knobs) and
% timely configure these knobs (we denote the knobs together
% with their configured values as a configuration)
% (\S\ref{sec:related}).
% ~\cite{vigil,glimpse,mcdnn,videostorm,noscope,neurosurgeon,awstream,chameleon,focus,adascale,filterforward,vstore,cracking,dds,reducto,blazeit,yoda,vcm,elf,ekya}.
% They show that an optimal configuration of these knobs can significantly reduce resource usage in both network bandwidth and GPU 
% % {\em if} one always sets these knobs {\em optimally}, resource usage in both network bandwidth and GPU compute can be significantly reduced 
% without affecting inference accuracy.
% Multiple knobs are often tuned together to save more resources (see Table~\ref{tab:rich-set-of-knobs} for a list of knobs considered).
% uses the {\em optimal setting} of these knobs, 
% high inference accuracy could be obtained while significantly reducing resource usage in both network bandwidth and GPU compute.
The challenge is that the optimal configuration {\em varies} over time with the input data, so it must be {\em adapted timely}. 
For instance, when the vehicles stop at the red light or move slowly, feeding the traffic video feed at a low frame rate to a DNN can still accurately detect vehicles,
% at only one frame per second (fps) in a traffic video, 
but when the light turns green, the DNN must analyze frames much more frequently (\eg 30fps) to detect fast-moving vehicles. 
In this case, the configuration of frame rate
% of feeding data to the DNN---
must be dynamically adapted depending on the video content.

% Multiple knobs are often tuned together to save more resources (see Table~\ref{tab:rich-set-of-knobs} for a list of knobs considered), 
% % With more knobs to tune (see Table~\ref{tab:rich-set-of-knobs} for a list of knobs considered), more resources {\em could} be saved 
% but it is more challenging to adapt in
% % It becomes more challenging to tune more knobs (see Table~\ref{tab:rich-set-of-knobs} for a list of knobs considered) at the same time, which leads to 
% a multi-dimensional space of {\em configurations} (each being a combination of knobs).

% The {\em optimal settings} of these configuration knobs should achieve the highest inference accuracy but use bandwidth and GPU resources within a given budget. 


% \kt{I slightly changed the logic here. The goal is to implicitly explain that the adaptation frequency can be larger than the rate of optimal configuration changes}
% However, the optimal setting of these configuration knobs varies with changes in the input data stream, and thus must be adapted frequently to avoid sticking to an outdated configuration (this aligns with the observation of prior work). 
% In the vehicle-detection example, when the red light appears, the vehicles move slowly and the DNNs can accurately detect vehicles using 1fps.
% However, under green light, the vehicles move much faster and the video needs to be analyzed much more frequently (\eg 30fps) to accurately detect fast-moving vehicles.



% Technically, recent proposals~\cite{vigil,glimpse,mcdnn,videostorm,noscope,neurosurgeon,awstream,chameleon,focus,adascale,filterforward,vstore,cracking,dds,reducto,blazeit,yoda,vcm,elf,ekya} expose internal tunable parameters (referred to as \textit{configuration knobs}, see Table \ref{tab:rich-set-of-knobs} for a full list of configuration knobs) and timely \textit{configure} these knobs (we denote the knobs together with their configured values as a \textit{configuration}) to the \textit{optimal configuration} (\ie a configuration that achieves highest accuracy under the bandwidth and GPU computation budget).
% \kt{I changed `` the content of input data'' to `` the input data''.}
% \jc{not clear how and why knobs help leverage content to tune knobs.}
% \kt{I emphasized that prior work leverages the content of the input data to save resource, and gave an example. Hope that this is clearer}




% % DNN-based analytics are popular. 
% % The data needs to be streamed from the sensor to the server.
% % DNN-based analytics are resource-demanding (in terms of bandwidth and/or GPU compute). Goal: reduce resource usage while achieving high accuracy.
% % Many prior works in this space achieve this goal by exposing internal tunable parameters (we refer to as \textit{knobs}) and frequently adapting their configurations to achieve high accuracy within the resource budget (give an example configs and a forward pointer to the full list).  
% % Facing this trend, people develop adaptive analytic systems to handle various kind of videos and maximally reduce the resource usage while maintaining high accuracy.
% % \item However, these adaptive systems may sometimes use high amount of resource but still yield low analytic accuracy when the video content is challenging.

% % Prior work observes that the optimal config (the config with the highest accuracy under the budget) frequently changes. \\
% % Example: no object of interest --> low frame rate is 100\% accurate. A new object comes into the video --> low frame rate may only achieve an accuracy of 50\% as it cannot capture the movement of the object. 
% \kt{Do we need to bring up the point where the optimal configuration may not change when the input data does not vary? I feel like this point is a noise but people may question this.}
% Prior work~\cite{awstream,chameleon,dds,eaar}) observes that the optimal configuration frequently varies as the input data constantly changes over time.
% % As the optimal configuration depends on the content of the input data (the configuration with the highest accuracy under a certain resource budget), prior work observes that the optimal configuration  can change frequently~\cite{??}.
% \jc{this claim again comes out of the blue. again, it would have been more natural to first connect the setting of knobs with content, and then say because the content changes over time, the best knob settings must change too} 
% \kt{Done.}
% For example, when there are no objects of interest in a video, analyzing the video with a low frame rate is 100\% accurate. However, when a new object enters the video, a low frame rate may only achieve an accuracy of 50\% as it cannot capture the movement of the object.
% As a result, a frequent adaptation of the configuration (ideally once per \fillme seconds) is necessary to minimize the amount of time spent using an outdated configuration.
% \jc{the term "frequently" is a bit vague. can we give some concrete numbers how "frequently" configs should be adapted? also give a forward pointer 2.2 that has some empirical measurements?}


% \item
% As a result, the research question is: how to quickly adapt to the optimal config (given that optimal config frequently changes)? 
% \jc{this sentence is not wrong but misses the key point. the point is not "how to adapt", but what information you need to adapt. in this sense, the key is ability to estimate which configuration has the highest accuracy given some resource constraint? 
% you can later say to answer this question, you don't need to know the accuracy of all configs; instead, we only need the gradient}


% \kt{Define how people do it today.}
The key question, therefore, is as input data evolves over time, 
{\em how to quickly check if the current configuration should be changed.} In other words, whether a different configuration can yield much higher accuracy or lower resource usage without hurting accuracy. 

% better adapt configurations of DNN analytics systems is 
% As a result, the key research question of these configuration adaptation systems
% % \jc{let's call them "configuration adaptation systems"? anyway, we should stick to the same term whenever we refer to such systems}
% is: 
% \textit{how to timely identify if a different configuration is better---higher accuracy under a given resource budget, or much less resource usage while maintaining similar accuracy or both---than the current configuration.}
% identify the \textit{optimal} configuration?
% (the configuration with the highest accuracy under the resource budget)\jc{optimal config should've been defined much earlier, not here} 
% and quickly adapt to the optimal configuration\jc{once the optimal config is identified, isn't "quickly adapting to it" trivial? either drop it or rephrase}?


% \item Such event is runtime-specific.
% To recover from the accuracy drop after such sudden change, one need to quickly adapt to the optimal.
% We observe that the change of optimal configuration (\ie the configuration that generates highest accuracy within resource budget) can change abruptly and unpredictably.
% \kt{A concrete example here.}
%     For example, when there is no object of interest in the video, one can encode the video using low frame rate to save resource.
%     However, when a moving object appears in the video, the video needs to be encoded using high frame rate in order to accurately capture the motion of this object.
%     And when this moving object leaves, there is no object of interest in the video and the video can again be encoded using a low frame rate.
    % In order to capture the frequent change of optimal config, one needs to adapt the configuration with a frequency faster than once every 3 seconds (a measurement to support this point: 20\% accuracy gain if adapting once every 3 seconds compared to adapting once every 15 seconds).
    % \jc{this is weak. it only says once every 3 seconds is better than once every 15. maybe you should ALSO say once every 3 seconds is almost the same as once every second?}
    % The design question is: how to frequently and optimally adapt the configuration to achieve high accuracy with a given resource budget?


    % Is there exist another config, that has much higher accuracy than the current config and still within resource budget?


    % \kt{Goal: check  if there is a config with higher accuracy under the resource budget and adapt to it}
    % \begin{packeditemize}

    \mypara{Prior approaches}
    To answer this question, two general approaches exist, but they fall short for different reasons (\S\ref{subsec:configuration-adaptation}).
    First, {\em profiling-based} methods periodically run {\em extra} DNN inferences to profile the accuracy of alternative configurations and then use these profiles to identify the optimal configuration~\cite{awstream,chameleon,videostorm,vstore}. 
    % runs inference with many configurations to {\em profile} which configuration has the highest accuracy with minimum resource usage~\cite{awstream,chameleon,videostorm,vstore}. 
    However, the extra DNN inferences incur significant GPU overhead.
    % to run significantly more extra DNN inference on the same input data. 
    % Moreover, it often uses extra bandwidth to stream input data at a much higher quality to test their inference accuracy.
    For example, AWStream~\cite{awstream}'s profiling step test 
    % runs DNN inferences with 
    different combinations of resolutions, frame rates, and quantization parameters, which causes up-to 17$\times$ more GPU cycles than normal inference.
    % , causing 17$\times$ extra GPU overhead. % than regular DNN inference.
    With limited compute resource, the profiling overhead will slow down configuration adaptation and cause the configuration to be outdated when input data changes over time. 
    % they are unable to profile configurations frequently,
    % % Thus, it is difficult to profile configurations frequently, 
    % leading to the use of outdated configurations when the optimal configuration changes.
    % knobs (resolution, frame rate, and quantization parameter) on a \textit{10-second} video consumes the same amount of GPU computation as analyzing more than an \textit{8-minute} video.
    
    % The first~\cite{awstream,chameleon,videostorm,vstore} periodically performs extra DNN inference to profile the accuracy and resource usage of all configurations and picks the configuration that has the highest accuracy within the resource budget.
    % However, each profiling needs to perform multiple extra DNN inferences, resulting in high GPU computation overhead.
    % For example, in AWStream~\cite{awstream}, running full profiling on just 3 knobs (resolution, frame rate, and quantization parameter) on a \textit{10-second} video consumes the same amount of GPU computation as analyzing more than an \textit{8-minute} video.
    % As a result, when the GPU compute and/or the network bandwidth is restricted, this approach needs to either profile less frequently, leading to the use of outdated configurations when the optimal configuration changes, or significantly prune the search space (which may contain only suboptimal configurations).
    % --> need extra streaming and inference --> when the bandwidth and/or GPU resource is limited, either identify the optimal config slowly or downsample the config space and may miss the optimal config

    % \kt{ask Ganesh why we should add this work}
    % The second approach performs no extra inference and adapts the configuration based on recent DNN outputs (including intermediate DNN outputs). 
    % Though no extra inference is run, this approach also tends to adapt slowly, as each DNN output reveals limited information regarding the highly complex relationship between the configurations and DNN inference output/accuracy, due to the complexity of the DNN itself and the preprocessing modules before the DNN (e.g., video codecs). We take EAAR, a system for video object detection, as an example. 
    % EAAR adjusts the video encoding quality by collecting the regions from the DNN that may contain objects of interest and encoding these regions in higher encoding quality on future video frames. Thus, the objects inside these regions are much more likely to be detected.
    % However, as the regions generated by the DNN may not be exactly aligned with the region that actually contains the objects, the object detection DNN may fail to detect some objects and thus EAAR needs to further adjust the corresponding regions.

    % \kt{also mention the other line of work that adapts based on DNN output}
    % To improve the adaptation speed, 
    % \kt{I prefer n those works that adapt based on DNN output as the rationale below also applies to them.}

    Second, {\em heuristic-based} methods avoid extra inference and pick the configuration using {\em cheap} heuristics~\cite{dds,reducto,vigil,glimpse,eaar,accmpeg,casva,elf}.
    % by running simple heuristics on data streams 
    % analyzing the data streams through cheap heuristics 
    % \eg calculating frame differences~\cite{reducto} or region-of-interest proposed by DNNs on recent input~\cite{dds}.
    % (\eg calculating frame differences~\cite{glimpse,reducto} or region-of-interest proposed by DNNs~\cite{dds,eaar,elf} on recent input).
    % ) or using past DNN inference results (\eg region-of-interest proposed by DNNs~\cite{dds,eaar,elf} on recent input).
    % from DNN intermediate results~\cite{dds,eaar,elf}).
    Though they may adapt faster
    % (\eg once every second) 
    than profiling-based methods, but the cheap heuristics may sometimes pick suboptimal configurations that have low accuracy.
    % pick the configuration with accuracy much lower than the optimal one (see \S\fillme for more rationales).
    For instance, a typical heuristic selects a new frame to feed to DNN
    % calculates frame difference
    % \footnote{Reducto calculates frame differences based on various frame feature extractors in computer vision literature.} 
    % and sent out 
    % a video frame to the server for DNN analysis 
    when its pixels differ significantly from the last analyzed frame (\eg~\cite{reducto}).
    % the frame significantly differs from the last analyzed frame.
    % to determine whether the current video frame needs to be sent out to the server for analytics.
    % If the frame difference between the current frame and the previously-sent frame is larger than a threshold, Reducto will send out the current frame.
    However, a high pixel-level difference may fail to indicate frames with new objects of interest, when the video background moves quickly (\eg dashcam video from a moving vehicle) which causes great pixel changes.
    % , frame difference is caused mostly by background pixels and thus becomes a poor indicator for the arrival or movement of objects of interest.
    As a result, it might run the DNN on too many frames while the objects of interest remain the same.
    % , which uses more network bandwidth and GPU cycles than necessary, or analyze too few frames and miss real objects of interest.
    % \jc{kuntai, check if this is correct}
    % of whether there is an object of interest or not.
    % large regardless of whether there is an object of interest or not.
    % As a result, Reducto may send out frames when no object of interest appears, thus having insufficient resources to frequently send out frames when the object of interest appears, resulting in low accuracy.
    % \item To improve the adaptation speed, the other line of work performs no extra DNN inference and instead pick the config through cheap heuristics.
    % These heuristics can adapt quickly\jc{"adapt quickly" sounds vague. do you mean adapt config every frame or second?}. 
    % \kt{guess  the accuracy}

    % \jc{Is DDS a good example of knob-specific design as well?}
    % \kt{yes it is, my plan is to focus on Reducto in intro and introduce server-driven works in motivation section.}
    Moreover, many existing techniques are designed only for {\em specific} data types or configuration knobs.
    % , and it is unclear how effective they will be on other types of data (\eg LiDAR point cloud, depth map, or audio waves).
    % Even in video analytics, the proposed heuristics often work well only for {\em specific knobs}.
    % and do not generalize to other types of knobs.
    For example, Reducto~\cite{reducto} selects which frames to run DNN inference based on inter-frame difference, but the inter-frame difference is ill-suited to tuning the encoding quality parameters of a video frame, which depends on the content {\em within} a frame, rather than how it differs from other frames. 
    % See \S\ref{subsec:configuration-adaptation} for more examples.
    Likewise, DDS~\cite{dds} tunes the region-of-interest quality parameter within each frame, but its logic may not naturally extend to tuning  knobs of non-video input data, such as LiDAR point cloud, depth map, or audio waves.
    % each fine-grained spatial block to improve inference accuracy on each frame, 
    % but it is not aware whether the current frame is redundant given past inference results.
    

    % \jc{mostly in video. generalize to other data types}
    % \jc{kuntai, check if this is correct}
    
    
    % is not effective when tuning the resolution of each video frame.
    % This is because whether the current frame should be encoded in high resolution or not depends on the current frame itself (\eg the current frame should be encoded in high resolution when there are multiple small objects) rather than the frame difference between the current frame and previously-sent frame.


    % Moreover, these works tailor for specific types of knobs and do not generalize to other type of knobs.
    % \jc{Is DDS a good example of knob-specific design as well?}
    % \kt{yes it is, my plan is to focus on Reducto in intro and introduce server-driven works in motivation section.}
    % % For example, Reducto filters the video frames on the camera to save server-side GPU compute cost without hurting the accuracy.
    % % Concretely, Reducto measures the similarity between the current frame and the previously-sent frame using metrics in computer vision literature and discards the current frame if it is highly similar to the previously-sent frame.
    % For example, Reducto may not be useful in terms of tuning the resolution of each video frame.
    % This is because whether the current frame should be encoded in high resolution or not depends on the current frame itself (\eg the current frame should be encoded in high resolution when there are multiple small objects inside) and does not depend on the frame difference between the current frame and previously-sent frame.
    % \kt{read classic papers, daily read intro}
    % \kt{Para1: tell people why DNN can calculate ''how much changing a bit knob can affect accuracy'', because we can split the change to}    
    % \kt{2 high-level key ideas, give it a try}
    % \kt{Para2: why having this is better than previous work}
    

    % We propose an alternative approach to handle uncertain QoE degradation.
    % Goal: let people know why we are better.


    % 造潜艇：
    % 方法1：我能造一个小型的核反应堆，
    % connect from what's new to why you are better
    % new: gradient decoupling + gradient descent.
    In short, prior work falls short on at least one of the three fronts: 
    (1) frequent adaptation, (2) choice of near-optimal configuration, and (3) not tied to specific configuration knobs.
    % (1) adapt frequently, (2) reach a near-optimal configuration, and (3) apply to a range of configuration knobs.

    % \jc{
    % \begin{itemize}
    %     \item we focus on \outputgrad. 
    %     \item we can compute \outputgrad efficiently
    %     \item based on \outputgrad ==> gradient ascent
    %     \item why it's better than profiling (faster) and heuristics (dnn output -> accuracy)
    %     \item caveats of gradient ascent
    % \end{itemize}}

\jc{we should be introducing our system here. i tried an alternative flow in intro\_v6.tex that introduces the high-level idea first, and then how to estimate \outputgrad efficiently.}


\myparashort{\name: Fast adaptation based on \outputgrad}
This paper presents \name, a new approach to configuration adaptation that improves on all three fronts.
The key step of \name is to quickly estimate the {\em gradient of the inference results with respect to each configuration knob} (explained shortly), which we refer to as {\bf \outputgrad}.
\outputgrad shows how a small change in the configuration of each knob can change the inference accuracy.
Intuitively, once the estimate of \outputgrad can be frequently updated, \name can use a {\em gradient-ascent} strategy to adapt the configuration in a
the way that increases accuracy without using more resources.

\myparashort{Cheap estimation of \outputgrad}
Our key idea is that \outputgrad can be calculated by leveraging DNN's {\em differentiability}, with no extra DNN inference.
Differentiability is an inherent property of almost all DNNs~\cite{paszke2017automatic} but has so far been only used in DNN training. 
Our insight is that most knobs only transform the raw input data to DNN's input (\eg frame filtering, image downscaling, etc), so the \outputgrad of a knob can be decoupled into:
\begin{packedenumerate}
\item {\em \dnngrad:} How the DNN's output changes with respect to the DNN's input.
\item {\em \inputgrad:} How the DNN's input changes with respect to the knob's configuration.
\end{packedenumerate}
Both can be computed efficiently: 
computing \dnngrad can be done with a single backpropagation operation on the DNN, and 
computing \inputgrad does not need GPU.
Moreover, if the system has multiple configuration knobs, \dnngrad can be calculated once and re-used to derive the \outputgrad of different knobs.  
Intuitively, \dnngrad describes DNN's sensitivity to a change in DNN's input, which is agnostic to {\em which} knob causes the change in DNN's input.
For instance, the \dnngrad of an object-detection DNN will be high for pixels associated with key visual features of an object.
To further reduce the compute and memory overhead of DNN backpropagation, \name also includes several optimizations detailed in \S\ref{sec:cost}.

    \myparashort{\outputgrad: How DNN inference changes with configuration.}
    To improve on three fronts, we take a different approach by focusing on the {\em gradient} of the inference results with respect to each configuration knob---how much the inference results would change if a small change was added to each configuration knob of the current configuration. We refer to it as {\em \outputgrad}.
    % This gradient, which we refer to as {\em \accgrad}, captures how much DNN's output would change if a small change was added to the current configuration.

    

    % The insight to focus on \outputgrad is two-fold:
    % \begin{packeditemize}
    % % \item \accgrad allows us to calculate the change in accuracy, which is easier to calculate than the exact accuracy number. 
    % % This is because the change in accuracy is triggered by the change in inference results and thus correlates with the change in inference results (we will show empirical evidence in \S\ref{??}), but calculating the accuracy requires one to annotate the input data by using human annotation or by referring to the inference results with respect to the most expensive configuration.
    % % Differentiability is a key property of DNNs that differentiates DNNs and other traditional applications.
    % % However, as far as we know, previous work only uses this property as a way to train DNNs.
    % % We are the first one that expands the use case of the differentiability of DNN to scenarios outside DNN training.
    % % \kt{Maybe phrase this sentence more carefully?}
    % \item 
    %     \jc{let's drop this here. it doesn't seem really necessary to spill it out here. Instead, put it in the para starting with "by performing gradient ascent ...." as a reason why maximizing output change also maximizes accuracy. }
    %     \kt{I'm not sure about this, can we discuss? For me, outputgrad comes out of blue and we need a para to say that it correlates with accuracy.}
    % Second, a large change in inference results could statistically indicate a large change in inference accuracy.
    % Thus, \outputgrad could indicate how configuration should be changed to improve accuracy (see \S\ref{??} for empirical evidence).
    % \kt{Explain the difference between DNN output and inference accuracy, then say why statistically they aligns}
    
    % \end{packeditemize}
    % As far as we know, we are the first one that uses differentiability of DNNs in non-training environment.

    
    % Second, we embrace that DNNs are naturally {\em differentiable}. 
    % Differentiability is a common property of all DNNs but is rarely utilized by prior work to adapt configurations of DNN-based applications.
    % As elaborated shortly, differentiability makes it possible to cheaply estimate \accgrad (with minimum GPU compute overhead).
    % \end{packeditemize}

    % The insight to focus on \accgrad is two-fold.
    % First, we embrace that DNNs are naturally {\em differentiable}. 
    % Differentiability is a common property of all DNNs but is rarely utilized by prior work to adapt configurations of DNN-based applications.
    % As elaborated shortly, differentiability makes it possible to cheaply estimate \accgrad (with minimum GPU compute overhead).
    % Second, a large change in DNN output could statistically indicate a large change in inference accuracy.
    % Thus, \accgrad could indicate how configuration should be changed to improve accuracy.


    

    

    % \jc{please tighten this para. too much info before getting back to your smart cost-saving idea}
    % Inspired by these two insights, we propose \name, a configuration adaptation system that frequently calculates \outputgrad and runs a {\em gradient-ascent} strategy
    % % \footnote{Note that we can adapt even faster by using more sophisticated optimization techniques\cite{??}, but we choose not to use those techniques to demonstrate the quick adaptation speed provided by our \outputgrad only.}
    % to gradually search for the optimal configuration. 
    % First, we partition the input data stream (\eg video frames) into {\em adaptation intervals}, each of \fillme seconds.
    % % (hereinafter \textit{adaptation intervals}) 
    % % and perform adaptation in an interval-by-interval manner. \kt{Let me reconfirm the time window in my eval code}.
    % In each adaptation interval, we estimate \outputgrad and decide the configuration for the next adaptation interval by choosing to increase, decrease or keep the value of each knob so that the accuracy is maximized without exceeding the resource budget.
    % In each adaptation interval, we first estimate \outputgrad of DNN inference output
    % ---how DNN output would change with a small change on each knob value. 
    % (We will explain how to do it with minimum overhead next.)
    % Then we use this information to decide for each configuration knob whether to keep its current value, increase or decrease it by a small amount, providing that the new configuration will not exceed the resource budget. 
    % identify a new configuration that maximally improves accuracy without exceeding the resource budget.
    % We use this new configuration for the next adaptation interval and repeat the same adaptation steps on the next adaptation interval.
    % As the content of the input data is continuous, the new configuration is likely to generate more accurate inference results compared to the original configuration.
    % Note that 
    % As a result, the inference results of the new configuration are likely to be more accurate than the current configuratio

    % \jc{move this to after the gradient decoupling discussion}
    % For example, \kt{an example here, follows the fps \& resolution example.}


    % However, this gradient-ascent-based approach has its caveats.

    
    
    
    
    % \kt{explain why it is OK to reuse}
    
    % \jc{1. estimate gradient => reuse gradient to pick config in next step => use the new config in the next step => go back}
    
    % while these heuristics can have much lower accuracy than the optimal configuration.

    

    % \jc{
    % \begin{packeditemize}
    %     \item Compare between backprop and saliency
    %     \item caveats of gradient descent:
    %     \begin{packeditemize}
    %         \item each step must be small => we estimate \accgrad extremely fast, so can adapt very frequently
    %         \item how to deal with local optimum => ??
    %     \end{packeditemize}
        
    % \end{packeditemize}
    % }

    % An ideal configuration adaptation system, therefore, needs to serve a wide range of knobs and applications, and quickly identify the optimal configuration with no extra inference.

    % We take an alternative approach. Unlike previous work that only obtains the accuracy from the current configuration, we further obtain the \textit{gradient} of the accuracy with respect to the current configuration (hereinafter \accgrad, we will define it later).
    % This \accgrad can be \textit{cheaply} computed \textit{without running DNN inference} by leveraging the differentiability of the DNNs.
    % Using this \textit{cheap} \accgrad, we can then \textit{frequently} run \textit{gradient ascent} to quickly adapt to a near-optimal config (empirically within 2 seconds).
    % As a result, we can adapt to a near-optimal config within 2 seconds.
    
    % based on the accuracy of the current configuration, we can further derive the gradient of accuracy with respect to the current configuration by leveraging the fact that DNNs are differentiable, 
    % based on the accuracy of the current configuration, we can further by leveraging the fact that DNNs are differentiable, we can calculate the gradient of accuracy with respect to the current configuration  \textit{without extra DNN inference} and use this gradient to identify a configuration that can significantly improve accuracy.
    % As a result, we can frequently pick the configuration that can significantly improve accuracy, allowing us to adapt to a near-optimal optimal configuration within 2-3 seconds.
    % If we can find a direction that maximally improves accuracy, we can reach the optimal within 3-4 steps.
    % We take an alternative approach that adapts the configuration gradually, which allows us to adapt quickly (by stepping towards a new config right after identifying a config that may improve the accuracy under the resource budget) and adapt to a near-optimal config (by constantly finding a config that may improve the accuracy under the resource budget).
    % The key to this approach is to decide which config should be picked in the next step.
    % We leverage the \textit{gradient} of accuracy to determine this config based on two reasons:
    % \begin{packeditemize}
    % \item mathematically the gradient of accuracy points to the config that improves accuracy the most
    % \item the cost of calculating the gradient of accuracy (in terms of network and GPU compute) can be significantly reduced by leveraging the fact that DNNs are differentiable.
    % \end{packeditemize}

    % We can update right after obtaining the gradient (instead of obtaining
    
    % The limitation of prior works comes from the fact that they abstract the DNN (together with the underlying system components, like video codecs) as a black box.
    % As a result, they either need to run this black box multiple times to accurately identify the optimal configuration (resulting in slow adaptation speed), or need to build cheap proxies to estimate the performance of this black box (resulting in selecting configurations with much lower accuracy than the optimal configuration).
    
    % However, different from adapting the configuration of traditional applications (like job scheduling), DNNs have a unique property that makes them much more amenable to configuration adaptation.
    % \kt{this sentence is a bit out-of-the-blue, need a way to fix it.}
    % Concretely, DNNs are designed to be \textit{differentiable}, granting them the ability to \textit{adapt} DNN parameters to fit different input content (\eg different images in the training set) through the DNN training process. 
    % On a high level, the goal of configuration adaptation is also adapting its parameters (\ie knobs) to fit different input content. 
    % This inspires us to leverage the differentiability of DNN for configuration adaptation.

    % The spirit of this algorithm is akin to \textit{gradient ascent}. One may wonder that 
    % \jc{to make this gradient-ascent search practical, the key technical challenge is how to {\em quickly and accurately estimate \accgrad for multiple configuration knobs with minimum extra GPU computation.}
    %     \begin{packeditemize}
    %         \item use differentiability to decouple
    %         \item faster backdrop (yitian)
    %     \end{packeditemize}}
        
    % \kt{Not sure where should I put this.}
    % The key in our approach is to calculate \accgrad (defined as the change of inference accuracy if each knob of the current configuration was changed by a small amount).
    % \accgrad can directly suggest which knobs to change so that inference accuracy will likely increase by the largest amount in the coming second, without using more network and GPU compute resources than the budget. 
    % Concretely, we give more resources to the knobs with high Output-Knob Gradient to improve the accuracy by the largest amount and cut the resource usage of those knobs with low Output-Knob Gradient to save resources with minimum degradation in accuracy. 


    
    % \kt{Though how to use the gradient is crucial, understanding this sentence requires a lot of extra knowledge (like config knob value bounds to resource, more resource -> higher accuracy). Not sure how to fix this for now.}
    
    % Although doing so may not immediately adapt to the optimal configuration, this \accgrad-based adaptation can adapt to a near-optimal configuration within a handful of steps (empirically, we can adapt to a near-optimal config within 2-3 seconds).

    
    % if we know the gradient of accuracy with respect to the current configuration (\ie how much does increasing the value of each knob change the accuracy, hereinafter \accgrad), we can accurately estimate the accuracy of a large subset of configs (see \S\fillme for further detail) and adapt to a near-optimal config within 2 seconds by assigning more resource to those knobs with a high gradient of accuracy, or cut the resource usage of those knobs with a low gradient of accuracy without hurting the inference accuracy (see \S\fillme for further detail).
    % \kt{it is definitely better if we can illustrate the rationale of why gradient converges so fast. I do not have a good argument yet and I will keep on trying.}.


    % \kt{If you can get gradient, 1. quick adapt 2. near-optimal config in 2/3 steps}
    % However, generally these heuristics sacrifices the ability of picking the optimal configuration at once. generally more difficult for these approach to pick the optimal configuration at once.
    % \kt{generaly sacrifices the optimality}
    % \kt{mention that this approach adapts faster}
    % However, as the optimal configuration is jointly determined by the current video input and the DNN itself, how DNN processes the current video is highly complex (due to the complexity of the DNN) the relationship between the current video input to the corresponding optimal configuration heavily depends on how DNN processes the current video
     % .
     % As a result, these heuristics will have low accuracy.
    %  However, in order to accurately identify the optimal configuration, one needs to check whether a different config in the resource budget can generate more accurate inference results or not, requiring extra DNN inference on this config.
    % As these heuristics does not perform extra inference, they may fail to accurately identify the optimal config and end up using a sub-optimal config, resulting in low accuracy
    
    
    % extra DNN inference without DNN inference, cheap heuristics may fail to identify such configuration-changing event in the video and thus cannot fix such accuracy drop.
    % \kt{DDS falls into this category}
    % \item Difference: other configs is no longer visible.
    % \item No extra inference and generate new config with heuristics.
    % \item Adapt without extra DNN inference (using heuristics)
    % These heuristics may generate a suboptimal config upon change.
    % Without comparing to other configs, we cannot tell whether the current config is optimal or not --> will use sub-optimal configuration when the heuristics --> low accuracy
    % \kt{Should we take server-driven approach into account here?}

    % mappin between config and accuracy is highly complex --> DNN output / video input only reveals limited information regarding this highly-complex space --> need to accumulate enough information to achieve optimal.

    % \kt{What is gradient}
    % \kt{how to use this gradient}
    % \kt{Empirically we can adapt to optimal within 3-4 steps}

    % \kt{Ideally, first we want to reduce the cost of extra inference on other configs, and then reduce the cost on golden config.}
    % \jc{
    % to make this gradient-ascent search practical, the key technical challenge is how to {\em quickly and accurately estimate \accgrad for multiple configuration knobs with minimum extra GPU computation.}
    %     \begin{packeditemize}
    %         \item use differentiability to decouple
    %         \item faster backdrop (yitian)
    %     \end{packeditemize}}
    
    
    % Remove this paragraph as it makes the reader impatient.
    % To make \name practical, the key technical challenge is how to cheaply and accurately estimate \outputgrad with minimum extra GPU computation.
    % Remember that \outputgrad is how much the inference output would change if a small change was made to each knob of the current configuration.
    % A naive way to compute \outputgrad on each configuration knob will require running two DNN inferences, one without change to the knob value and one with a small change to its value, and comparing their difference. 
    % With each configuration knob requiring one extra DNN inference on GPU, the overhead to obtain \outputgrad on one configuration grows with more configuration knobs, and this overhead must be added to each adaptation interval.
    % To put this overhead into context, one may need to tune 3 knobs~\cite{awstream,casva} in order to maximally reduce the bandwidth usage while maintaining high inference accuracy.
    % As a result, one needs to perform 3 times extra DNN inference to obtain \outputgrad for each adaptation interval, costing 4x more GPU resource usage compared to using existing techniques~\cite{casva}.
    
    
    
    % \kt{Done. Change to one insight \& merge with gradient decoupling}
    Our insight is that by leveraging the {\em differentiability} of the DNNs, \outputgrad can be calculated with no extra DNN inference.
    Differentiability is a common property of almost all DNNs~\cite{paszke2017automatic} but has so far been only used in DNN training. 
    We demonstrate that DNN differentiability can be used to  quickly and optimally adapt configurations of DNN analytics systems.
    % -based inference applications.
    % Note that calculating \outputgrad through its definition (how much the inference results would change if a small change was added to the current configuration) causes substantial GPU compute overhead, as it requires one to change the configuration knobs \textit{one-by-one} in order to obtain the change in accuracy and thus the extra DNN inference required by \outputgrad is \textit{proportional} to the number of knobs.
    % To put this overhead into context, one may need to tune more than 3000 knobs in order to tune the encoding quality of different spatial regions in the video~\cite{eaar,accmpeg}.
    % To calculate the \accgrad in real-time, one needs to perform >3000 extra DNN inference, costing >3000x GPU resource compared to using existing techniques~\cite{eaar,accmpeg}.
    % \kt{We need a figure for this decoupling.}
    % \kt{Remind people of differentiability}
    % The idea here is that \outputgrad (\ie how configuration changes the DNN output) equals to the multiplication of two terms:
    % \kt{The original text: The idea here is that \outputgrad (\ie how configuration changes the DNN output) equals to the multiplication of two terms:}
    % \kt{I prefer to not use multiplication as it gives people the wrong impression that we are just multiplying two numbers.}
    Specifically, we decouple the calculation of \outputgrad of each knob (gradient of the inference results with respect to the knob) into two components:
    % we leverage the differentiability of DNNs by decoupling \outputgrad (\ie how much the inference output would change if a small change was made to each knob of the current configuration) to two terms:
    % \kt{For me, the key is to address Ganesh's concern may be to write these two terms in a way that they feel like a matrix.}
    \begin{packedenumerate}
        % \item {\em DNN output's gradient w.r.t DNN input:} how the inference output changes with the DNN input.
        \item {\em \dnngrad:} How DNN's output changes with a small change in different parts of the DNN input.
        % DNN output's\footnote{\jc{need a short footnote to explain what the DNN output mean or should capture. maybe put some old text "thresholding, etc" here. this can also be merged with the "saliency" footnote}} gradient with respect to a small change in different parts of DNN input.
    %     \footnote{\dnngrad is similar to the notion of DNN's ``saliency'' in computer vision.\jc{kuntai, please rethink this point} 
    % \hl{However, existing saliency estimators put objects in high saliency, while \dnngrad puts pixels that may change the inference results in high saliency, making \dnngrad outperforms existing saliency estimators. See XXX for more rationales.} \kt{Address one expert reviewers' novelty concern.}}
        % DNN input. how much DNN output changes regarding a small change of different parts of DNN input. We call this term \dnngrad for short.
        % \jc{Should we call this term ``saliency''? I feel like calling it saliency gives people a better understanding of what this term is, and implicitly explains why this term can be shared across knobs, but we then need to defend this is a new saliency.}
        % \item {\em DNN input's gradient w.r.t configuration:} how the DNN input changes with the configuration, and
        \item {\em \inputgrad:} How different parts of the DNN input change with a small change in the knob value.
        % DNN input's gradient with respect to a small change in the current value of each configuration knob.
        % regarding configuration how much different parts of DNN input changes regarding the change of the current configuration.
    \end{packedenumerate}
    % f(2,2), (1,0), (0,1)
    % f(3)-f(2)/1 == f(1) - f(2)/ -1
    % f(2+x,2)-f(2,2) = f(2,2) + f'(2,2) * (x, 0) + O((x,0)^2)    
    % Intuitively, the first term captures the importance of different parts of DNN input, 
    % The key is our first insight is that a DNN's output is differentiable with respect to the DNN input. 
    It is important to notice that due to DNN differentiability, \dnngrad can be efficiently calculated by DNN's backpropagation operation, and computing \inputgrad does not need GPUs.
    More importantly, if the system has multiple configuration knobs, \dnngrad can be calculated once and re-used to derive the \outputgrad of different knobs.  
    % without extra DNN inference on GPU.
    This is because \dnngrad describes DNN's sensitivity to each part of the DNN input, and it remains largely the same if the change in DNN input is not dramatic.
    For instance, the \dnngrad of an object-detection DNN will be high for pixels associated with key visual features of an object.
    % and remains largely the same when a small change is applied to different knobs.
    % \ga{DNN grad same -> Input change small ->  output change small -> } \kt{this is a important question but difficult to answer. I'll prioritize other part and then circle back to this later.}
    % Thus, if the system has multiple configuration knobs, \dnngrad will be calculated only once and re-used to derive \outputgrad of different knobs without extra DNN inference on GPU.
    % the first term can be calculated via one backpropagation and then shared across multiple knobs \jc{Should we defend this share?}.
    % This is a constant GPU-time operation without extra inference because it reuses the layer-wise features generated alongside DNN inference.
    % Additionally, the second term is operating between DNN inputs and thus not involving any DNN inference.
    % Therefore, computing \outputgrad for multiple configuration knobs only requires a one-time backpropagation on GPU and no extra DNN inference.
    % calculated in a knob-by-knob manner without DNN inference (\ie no GPU compute)
    \name also includes optimizations to further reduce the GPU and memory overhead of DNN backpropagation (see more details in \S\ref{sec:cost}).

    % \jc{edit ends here}
    % \jc{Junchen can you read here and see if it works for you?}
    % Further, given that backpropagation poses high GPU computation and memory overhead (even greater than DNN inference~\cite{?,?}), we present a set of techniques to further reduce the GPU computation and memory overhead of backpropagation by computing the saliency at a coarser granularity (see \S\ref{??} for details).

    % Configuration change (0,1)
    % (Grad, I(2,3) - I(2,2)) = D(I(3,2)) - D(I(2,2))
    % Configuration change (1,0)
    % (Grad, I(3,2) - I(2,2)) = D(I(2,3)) - D(I(2,2))
    % Ganesh: why D(I(3,2)) != D(I(2,3)) but exist such a grad?
    % The first term can be reused 
    
    % To avoid such extra DNN inference, OneAdapt leverages the differentiability of the DNN to implement \outputgrad. 
    % Concretely, we \textit{decouple} \outputgrad (\ie (how much the inference results would change if a small change was added to the current configuration) to 
    % \begin{packeditemize}
    %     \item {\em Configuration to DNN input:} how does the DNN input change with the configuration, and
    %     \item {\em DNN input to output :} how does the inference results change with the DNN input.
    % \end{packeditemize}
    % The former can be calculated in a knob-by-knob manner without DNN inference (\ie no GPU compute), and the latter can be obtained via {\em backpropagation} (which is a constant GPU overhead without extra inference as it can reuse the existing computation graph of DNN inference).
    
    
    % Calculating the former term does not require DNN inference.
    % The latter term corresponds to the gradient of inference results with respect to the DNN input of the current configuration\footnote{Note that it can be mathematically proved that the latter term corresponds to the gradient of inference results with respect to the DNN input of the current configuration (under the assumption that changing configuration only creates a small change to DNN input). We also show more empirical evidence in \S\fillme.} and can be calculated using backpropagation, which requires extra GPU computation and GPU memory but does not require extra DNN inference as it can reuse the existing computation graph of DNN inference.
    
    % This is a metric that only depends on the current configuration, and thus can be calculated once using backpropagation algorithm and then shared across .
    % As a result, calculating \outputgrad requires one backpropagation (constant GPU overhead) and no extra DNN inference.

    % \kt{Will expand this paragraph after finalize Yitian's backpropagation cost reduction technique}
    % While the calculation of \outputgrad no longer requires extra DNN inference,  In \S\fillme, we present a set of techniques aimed at reducing the GPU overhead and other types of overhead (such as bandwidth overhead and camera-side overhead) associated with the computation of \outputgrad. 
    % These techniques allow us to calculate \outputgrad with minimum overhead \kt{quantify this. Will do it after Yitian's experiment.}
    % \kt{A sentence that highlights the low overhead of \outputgrad. Will add it after Yitian finishes her experiments.}

    % Based on \outputgrad, 
    \myparashort{\name: Using \outputgrad to adapt configuration.}
    We present \name, a new configuration adaptation system, which frequently estimates \outputgrad (every second) and uses the up-to-date \outputgrad to perform {\em gradient ascent} to adapt the configuration in a way that increases accuracy without using more resources (\S\ref{sec:design}).
    We empirically observe that \name's gradient ascent converges to a near-optimal configuration within a few iterations.
\name's fast convergence can be attributed to the configuration-accuracy relationship being mostly {\em concave}---as the configuration uses more (compute/network) resources, the change in the input to the DNN becomes more marginal, and so does the DNN output.
For example, as a video analytic system increases the video encoding resolution, the pixel change becomes more marginal (mostly on ``high-frequency'' details), causing the DNN output to stabilize (objects' confidence scores will change more slowly and less frequently cross the confidence threshold, leading to fewer newly detected objects).
Due to this concavity, gradient ascent can eventually converge to a global optimal configuration. 


One may worry that calculating \outputgrad once every second may result in a high end-to-end delay (the delay of obtaining the DNN inference results), as calculating \outputgrad requires running backpropagation, which is even more expensive than DNN inference as it may require both extra GPU compute and extra GPU memory.  
We point out that as \name runs its adaptation logic \textit{after} generating inference results, the extra GPU compute and memory overhead does not affect the end-to-end delay unless there is not enough resource for \name to run its adaptation in real-time.
We also present a suite of techniques in \S\ref{???} to further reduce the GPU overhead (and other types of overheads) of \name.


\kt{Need to add more text to address: (1). the assumptions of OneAdapt (2). the scope where OneAdapt generalizes. (3). Why it is OK to have the overhead of backpropagation}

% It splits the input data stream into {\em adaptation intervals} (\eg every second), and at a high level, in each adaptation interval, we obtain DNN output using the current configuration, calculate \outputgrad, and uses the \outputgrad to adjust the configuration knob values using a gradient-ascent algorithm to increase accuracy in the next adaptation interval while adhering to the resource budget (see \S\ref{??} for details).
    
    
    % strategy to gradually search for the optimal configuration. 
    % decide the configuration for the next adaptation interval by adjusting the configuration knobs of the current configuration, either increasing,  decreasing, or retaining them,  to maximize accuracy 
    % \kt{Should we explain why \outputgrad correlates with accuracy here?}
    


    % \name outperforms previous work on all three fronts (\ie adapt frequently, converge to a near-optimal configuration, and generalize to different types of knobs and analytic tasks).
    % \kt{Done. Put the rationale of \outputgrad correlates with accuracy here.}
    % \begin{packeditemize}
    % \item
    
\begin{figure}
    \centering
    \includegraphics[width=0.7\columnwidth]{figs/contrast_different_approach.jpg}
    \tightcaption{
    Contrasting our approach with prior work. Our approach quickly adapts to a near-optimal configuration after the change of input content, while profiling-based methods adapt slowly and heuristics adapt to a configuration with much lower accuracy than the optimal one.
    }
    \label{fig:adaptation-behavior}
\end{figure}

    % \jc{move figure 2 in intro?} \kt{done}
    % \hl{
    Figure~\ref{fig:adaptation-behavior} compares \name with previous approaches.
    % }
    Unlike profiling-based methods, \name uses much less compute to calculate \outputgrad than profiling, so it can adapt configuration much more frequently  and react more timely to the change of source data.
    % \name could adapt right at the following second after the input content changes), 
    % because it takes much less compute and network resources than profiling.
    % the profiling-based baseline adapts slowly (once every minute~\cite{awstream}) may wait for at most a minute to react 
    % \item
    % Compared to heuristics that run no extra DNN inference,
    Unlike simple heuristics, \name can adapt more optimally because \outputgrad captures how configuration affects the actual DNN output. The more DNN output changes, the more inference accuracy changes (\S\ref{subsec:limitation}). 
    % \name can adapt to a near-optimal configuration where the works that perform no extra DNN inference may pick configuration with much lower accuracy.
    % This is because \outputgrad can indicate the accuracy of different configurations.
    % Intuitively, when a knob is of large \outputgrad, changing it can significantly impact the inference results.
    % Thus, by allocating more resources to this knob (\eg by increasing its value), the improvement in inference accuracy is also likely to be substantial.
    % \S\ref{??} shows more details on how we indicate the accuracy of other configurations and the correlation between our indicated accuracy and actual inference accuracy.
    % As a result, if we assign this knob more resources (\eg by increasing its value),  the accuracy improvement also tends to be significant.
    % Second, a large change in inference results could statistically indicate a large change in inference accuracy.
    % Thus, \outputgrad could indicate how configuration should be changed to improve accuracy (see \S\ref{??} for empirical evidence)., where the accuracy of these works can be much lower than the optimal configuration.
    % \item
    Moreover, since DNNs are differentiable, \name could generalize a wide range of DNN-based analytic tasks (Table \ref{tab:pipeline} for a list of pipelines that \name can optimize).
    That said, 
    % The second limitation is that, though \name can be used to tune a wide range of configuration knobs, it 
    \name as-is does not apply to those knobs that alter the DNN itself, such as retraining the DNN weights~\cite{ekya,mcdnn,noscope} (see \S\ref{subsec:limitation}). 
    Also, \name does not generalize to generative tasks like text generation and image generation.
    % Similar to \name, they also adapt to changes in input distribution. 
    % However, DNN retraining involves substantial computation and thus tends to adapt at a coarser timescale, while the knobs considered in \name require frequent adaptation.

    
    % (as \name only assumes the DNNs to be differentiable, which holds for almost all DNNs~\cite{?,?}) and a wide range of knobs (as \name poses minimum assumptions to the configuration knobs, see 
    % % \S\fillme for a full list of assumptions).
    % Table \ref{tab:rich-set-of-knobs} for a list of knobs that \name can optimize.
    % \end{packeditemize}


    
    % \kt{need a rewrite}
    % One may find the similarity between estimating the region-of-interest in the input video and calculating how DNN input affects inference results.
    % However, compared to existing region-of-interest 
    % \begin{packeditemize}
    %     \item Region-proposal-based: a region that is far away from any of the bounding boxes can affect the inference results a lot
    %     \item Camera-side cheap DNN: due to camera-side compute limit, a cheap DNN either misses regions that change inference results or wrongfully perceive those regions that have minor impact on the inference results as impactful. \kt{need to discuss AccMPEG in related work.}
    %     \item Saliency-based approach: pose high camera-side overhead. May highlight the objects that the final DNN does not detect.
    % \end{packeditemize}


    % \kt{No part of the paper should be like a math paper.}
    % \kt{Junchen can you check this paragraph?}
    % \jc{
    % rewrite this. i like what you said last night about why the whole config-accuracy plane is concave (i.e., only one global optimum)}
    % \kt{done}

We evaluate \name across 9 different DNN-based analytic pipelines, with 5 types of data, 4 analytic tasks, 6 configuration knobs, 59 videos, and 200 audios.
\name achieves similar accuracy with 15-59\% resource usage reduction, or achieves 15\% higher accuracy with similar resource usage compared to the baselines on 9 different applications.
We also show that the performance gain of \name over the baselines increases with more knobs or the finer-grained knobs. % become more fine-grained.
    


\begin{comment}
    

That said, \name's gradient-ascent strategy
    % has two main limitations. 
    % First, \name adapts configurations based on gradient ascent, which has its own caveats, such as the possibility that the search 
is not guaranteed to converge quickly to the optimal configuration.
    % the converged configuration is sub-optimal.
    % However, we empirically show that \name can reach a near-optimal configuration within \fillme seconds (\S\ref{??}).
    Intuitively, this can be understood that gradient-ascent can always converge to optimal if configuration-accuracy relationship is {\em concave}---as the configuration uses more (compute/network) resources, the change in the input to the DNN becomes more marginal, and so does the DNN output.
    In practice, such concavity does hold in most cases.
    % because the configuration-accuracy relationship is mostly \textit{concave}. % due to the following observation:
    % As the configuration uses more (compute/network) resources, the change in the input to the DNN becomes more marginal, and so does the DNN output.
    % are given to the analytic system (\eg by increasing the value of one configuration knob), 
    % the accuracy of DNN inference results improves slower and slower as the .
    For example, as a video analytic system increases the video encoding resolution, the pixel change becomes more marginal (mostly on ``high-frequency'' details), causing the DNN output to stabilize (objects' confidence scores will change more slowly and less frequently cross the confidence threshold, leading to fewer newly detected objects).
    % when we assign the system more and more resource by increasing the resolution, initially every pixel value change significantly.
    % Thus, the DNN inference results also tend to change significantly, making the accuracy significantly improved. 
    % At a higher resolution, however, most of the pixels no longer change except for those pixels that are related to the fine details (\eg the boundary of an object) when we further increase the resolution.
    % As a result, the inference results only changes a little, resulting in marginal accuracy improvement.
    % We also empirically confirm that the configuration--accuracy space is concave in \S\fillme.
    % By leveraging the concavity of the configuration--accuracy space, our gradient-ascent-based approach can quickly converge~\cite{?,?} and can converge to the global optimal (as there is no local optimal in the configuration--accuracy space under the resource budget).

\end{comment}

    % \jc{merged the "no dnn knob" para to two paras earlier}
    % The second limitation is that, though \name can be used to tune a wide range of configuration knobs, it does not apply to those knobs that alter the DNN itself, such as retraining the DNN weights~\cite{??}. 
    % Similar to \name, they also adapt to changes in input distribution. 
    % However, DNN retraining involves substantial computation and thus tends to adapt at a coarser timescale, while the knobs considered in \name require frequent adaptation.
    
    % \kt{Talk about the cases, where the accuracy improvement may not become more and more marginal.}
    % \kt{Other potential concerns: (1) why treat discrete configs as almost continuous variables, (2) why the better configuration at this second will likely lead to better result at the next second, (3) what if the content is noisy and makes the gradient noisy}
    


    
    % The intuition behind the fast convergence is that as long as the \outputgrad with respect to one configuration knob is non-zero, tuning that knob will likely improve accuracy.
    % % Further, as the input data is constantly changing over time, it is less likely for a local optimal to persist.
    % Thus, \name is unlikely to be stuck in a local optimum, which corroborates our empirical observation of \name.
    % (See \S\ref{??} for more details.)
    
    
    % Despite the low cost of \outputgrad estimation, the configuration adaptation based on gradient ascent in \name has its own caveats, including the inability to guarantee a quick convergence or the optimality of the converged configuration. 
    % However, our experiments demonstrate that \name can attain a much better configuration within \fillme seconds. 
    % It can be intuitively understood that if the \accgrad with respect to a particular configuration knob is non-zero, adjusting that knob will likely lead to improved accuracy. Additionally, since the input data is continuously changing over time, it is less likely for a local optimum to persist. As a result, \name is unlikely to become stuck in a local optimum, which is supported by our empirical findings on \name. (Further details can be found in Section \ref{??}.)
    
    % At a high level, \name uses a greedy gradient-ascent search to tune configurations and gradually improve accuracy under the resource constraint, but given the complex relationship between accuracy and configuration, 



  
    % \kt{Multiple times per second sounds weird. But one time per second sounds like we are adapting slowly, especially given that we need multiple steps to converge} 
    % than profiling-based work (\eg once every 15 seconds \kt{back this number up in footnote}), and can thus adapt to a new near-optimal within \fillme seconds after the optimal config changes.
    
    % \kt{needs to work on this rationale as we are not directly optimizing accuracy...}
    % We are more likely to find a near-optimal config compared to heuristics-based approaches as we adapt configurations based on the change of inference results, which correlates to accuracy (though we may not adapt right to the optimal configuration).
    % \kt{Across different tasks, different knobs}
    % Moreover, our approach can generalize to a wide range of knobs as we perform the adaptation based on the inference results.
    % That said, our approach cannot handle all knobs and we will illustrate those knobs that we cannot handle soon.
    
    
    
    

    
    % To reduce such GPU compute overhead, we calculate \outputgrad by splitting it into two terms:
    % \begin{packeditemize}
    %     \item calculating the change of DNN input when changing each knob by a little, which requires no extra GPU compute, and 
    %     \item calculating how much the change of current DNN input affects the inference results.
    % \end{packeditemize}
    % Note that The latter term can be measured by calculating the \textit{gradient} of the inference results with respect to the current DNN input through backpropagation algorithm.

    
    % We find that the first term does not require GPU and the latter term can be \textit{reused} across different knobs.
    % Our rationale is that, if changing a region of the current DNN input affects the accuracy a lot, it means that the DNN is uncertain about the inference results corresponding to this region. 
    % As we are changing each knob by a little amount when calculating \accgrad, the corresponding DNN input is still highly similar to the current DNN input, and the DNN is still likely to be uncertain about the inference results corresponding to this region.
    % As a result, this region will still have a significant impact on accuracy.
    
    % Further, the latter term corresponds to the \textit{gradient} of accuracy with respect to the DNN input, which can be directly calculated by the backpropagation algorithm (see \S\ref{??} for more illustrative examples and rationales).
    % As a result, by reusing the latter term across multiple knobs, calculating \accgrad only requires running backpropagation and no longer requires extra DNN inference (as backpropagation reuses the computation graph generated by existing DNN inference).

    
    

    
    % Our rationale is that: the ability of accuracy change
    % Ganesh: different DNN output, why single gradient?
    % Initial counterpoint: for a linear function, no matter how your DNN input changes, the output is still stable.
    % \kt{Here is just a placeholder argument. Will improve it later.}
    % This is because the granularity of existing knobs does not require an accurate pixel-by-pixel gradient.
    

    % As backpropagation can be even more expensive than DNN inference as it may require both extra GPU compute and extra GPU memory.  We will present a suite of techniques to further reduce this cost in \S\ref{???}.

    % \kt{Resource-constrained gradient ascent}
    % By obtaining \accgrad cheaply, we can then run gradient ascent to quickly adapt to a near-optimal configuration. 
    % Empirically, we find that we can adapt to a near-optimal configuration within 2 seconds.
    % Note that we can adapt even more faster by using more sophisticated optimization techniques\cite{??}, but we choose not to use those techniques to demonstrate the quick adaptation speed provided by our \accgrad only.

    % \kt{gradient ascent caveats}
    % \kt{Why local optimal OK, solution is greedy, 1. if the solution is far away why can you get there, 2. why you won't stick into local optimal}
    
    % \kt{Here is a placeholder para. Need to rewrite every sentence.}
    % At a high level, \name uses a greedy gradient-ascent search to tune configurations to gradually improve accuracy (constrained by resource usage), but given the complex relationship between accuracy and configuration, it cannot guarantee that (i) the search will quickly converge in a few steps, or (ii) the converged configuration is optimal.
    % Fortunately, our experiment shows that \name can converge at a much better configuration within 2-4 (??) seconds. 
    % Intuitively, as long as the \accgrad with respect to one configuration knob is non-zero, tuning that knob will likely improve accuracy.
    % Thus, with multiple configuration knobs, \name is unlikely to be stuck in a local optimum, which corroborates our empirical observation of \name when tuning more than three configuration knobs together.
    % (See \S\ref{??} for more details.)
    
    % First, prior work has shown that it suffices to tune each configuration knob with no more than six values (\eg \fillme uses \fillme levels of resolutions), so it does not take too long to 
    % Since \accgrad allows \name to tune all configuration knobs together, 
    
    % Gradient ascent does not guarantee that we can quickly adapt to a near-optimal config based on two reasons.
    % One, if the optimal config is \textit{far away} from the current config, it may take a long time to adapt to a near-optimal config.
    % In our case, the optimal config is not far from the current config, because each knob typically has less than 6 values.
    % As a result, the distance between the optimal config and the current config on each knob is less than 6.
    % As \accgrad allows us to change all knobs simultaneously, it means that we can achieve a near-optimal config within 6 steps.
    % We also empirically show that we can hit the optimal config within 6 steps.

    
    % we can change all the knobs simultaneously.
    % As each knob typically contains less than 10 values, even if we only change each knob by the smallest amount, we can hit the optimal config within \fillme steps.
    
    % \kt{Not sure if we need to bring up the point that increasing the knob always increases the accuracy.}
    % Second, one may worry that our solution may get stuck into a local optimal config.
    % However, as a local optimal config means that the accuracy of it cannot be improved by changing \textit{any} knob, the number of local optimal config will be smaller when there are multiple knobs.
    % Moreover, it is less likely for a local optimal to persist as the input video content is constantly changing.
    
    % less likely to happen when there are multiple knobs, as 
    % It is less likely to happen when there are multiple knobs as a local
    
    


    % We present \name, a configuration adaptation system that adapt the configuration by running \accgrad-based gradient ascent.
    % \name can quickly adapts to near-optimal config without extra DNN inference.

    
    
    % Note that we will introduce more techniques to further reduce the overhead (in terms of both network and GPU compute)  of obtaining \accgrad in \S\fillme.


    % We will 

    

    


    

    



    % \kt{a para here for gradient ascent and its caveats}



    
    % GPU compute overhead (we will further reduce GPU compute overhead and network overhead in \S\fillme).
    % \kt{propose gradient decoupling here without referring to }
    % One may think of calculating \accgrad in a knob-by-knob manner.
    % Concretely, to calculate this gradient for each knob, we need to calculate the accuracy between two configs (the current config, and the current config with the value of this knob increased) and then calculate the change of accuracy, divided by the change of knob value.
    % Previous work calculates the accuracy of a config by comparing inference results of that config with the inference results of the most resource-demanding config\kt{footnote chameleon here}, resulting in extra streaming and DNN inference overhead.
    % This overhead can be substantial \kt{quantify it}.
    % To reduce this overhead, our observation is: the change of accuracy between two configs is proportional to the corresponding change of inference results\kt{a pointer to how to measure the change of accuracy}.
    % \kt{It does not sounds like something that can reduce the cost of inference}
    % Intuitively, if the inference results of two configs are the same, their corresponding accuracy are also the same.
    % If the inference results changes significantly, the accuracy also tends to change significantly.
    % \kt{a pointer to empirical evidence}.

    % \item We take an alternative approach: we leverage\jc{"leverage" sounds like gradient is known but not used before and you just leverage it..} the \textit{gradient} of accuracy with respect to the current configuration (\accgrad for short) to adapt the config.
    % \jc{the next sentence is important, and needs some work}
    % This gradient enables us to quickly adapt to the optimal config, as gradient\jc{do you mean \accgrad?} points out the direction\jc{direction is a new term. avoid it} that increases accuracy\jc{accuracy on the current frame, current second, next second, or something else?} the most and those configs that are not on the gradient direction\jc{what do you mean by a config being on the gradient direction?!} increase accuracy slower\jc{what do you mean "increasing accuracy slower"?!} (compared to those configs that are on the gradient direction) and can be filtered out (unless the configurations are far away\jc{what do you mean "far away"?} from the current configuration, or the configs that align\jc{again, what does "aligning with gradient direction" mean?!} with gradient direction are out of resource budget\jc{this term is used without explanation}, we will further illustrate the details in \S\fillme). \jc{ok, I take it back. this sentence doesn't need some work; it needs a lot of work :) }



    % \item To illustrate why using gradient enables us to quickly adapt to the optimal, we start by describing the \textit{concavity} between the configurations and their corresponding accuracy. \\
    % We observe that, as the video analytic system consumes more and more resource (by changing the configuration), the accuracy improvement  becomes more and more marginal.
    % In other word, the gradient of accuracy diminishes when the config consumes more and more resource.
    % Mathematically, we formulate this observation by assuming the mapping between the configuration and the accuracy is concave.
    % \kt{Put a figure here and to illustrate why the observation transforms to concavity.}
    % We empirically measure this concavity in \S\fillme.


    % \item By introducing \accgrad, we can leverage the concavity of the mapping between configuration and accuracy to quickly converge to the optimal config.

    % \jc{the flow is broken here. the next para seems to assume that people are already convinced that having so-called "gradient" is highly useful. this is never established.}



    
% \kt{make a point after mentioning the cost reduction problem: the knobs are related to DNN input}
%     However, calculating \accgrad for each knob individually incurs high overhead, as it requires extra DNN inference (to obtain the inference results of a config besides the current config) on every knob.
%     As a result, the amount of extra DNN inference is proportional to the number of knobs.
%     This overhead can be substantial.
%     For example, one may need to tune more than 3000 knobs in order to tune the encoding quality of different spatial regions in the video~\cite{eaar,accmpeg}.
%     To calculate the \accgrad in real-time, one needs to perform >3000 extra DNN inference, costing >3000x GPU resource compared to using existing techniques~\cite{eaar,accmpeg}.

%     \kt{This point need to be mentioned much earlier}
%     To reduce this overhead, we calculate \accgrad for all knobs jointly by splitting the change of DNN output into two parts:
%     \begin{packeditemize}
%         \item calculating the DNN input change (No need for GPU), and 
%         \item calculating how the DNN input change affects inference results (note that this term corresponds to the \textit{gradient} of the inference results wrt DNN input and can be calculated using one single backpropagation).
%     \end{packeditemize}
%     As a result, calculating \accgrad only requires one backpropagation (which does not incur extra DNN inference, as backpropagation reuses the computation graph generated by existing DNN inference).
%     \kt{needs more explanation: change the input, why we can reuse the same backprop gradient}
%     \kt{If the inference results actually changes, why we can reuse the gradient}


    % \kt{Introduce gradient descent.}

    % \kt{Why using gradient descent}


    
    
    
    % We present a suite of techniques to further reduce the cost of camera-side compute, network bandwidth and GPU compute.


% Operators can use \name to tune a wide range of knobs that influences DNN input (as shown in Table~\ref{tab:rich-set-of-knobs}).
% That said, \name does {\em not} apply to knobs that alter the DNN itself, 
% such as retraining the DNN weights~\cite{ekya,noscope,mcdnn}.
% Similar to \name, they also adapt to changes in input distribution, they involve substantial computation and thus tend to happen at a coarser timescale than the knobs considered in \name. 




In short, the contributions of this paper are two-fold:
\begin{packeditemize}
    \item Design of \name, a new configuration-adaptation system that runs gradient ascent based on fast computation of \outputgrad.
    % \name's gradient-ascent-based search.
    \item Implemented a prototype of \name and integrated it with a benchmark of 9 DNN applications (which cover 5 data types, 4 analytic tasks, and 5 configuration knobs). \name achieves similar accuracy while reducing resource usage by 15-59\% or improves accuracy by 1-5\%  with the same or less resource usage when compared to state-of-the-art adaptation heuristics. 
\end{packeditemize}




\textbf{This work does not raise any ethical issues.}
    
    

    % \kt{2. Given 2 DNN output to estimate accuracy change (talk about golden config)}
    % \kt{quantify the overhead of not using saliency (maybe say multiple macroblocks)} \kt{Explain the difference between OneAdapt and prior work, especially compares with AccMPEG, compare saliency}
    % \kt{How to predict the second DNN output based on the first DNN output}
    
    % \item However, previous work would have had to calculate the gradient of accuracy in the following two steps:
    % \begin{packeditemize}
    %     \item First, obtain the inference results of a golden configuration as a reference point to calculate accuracy.
    %     \item Second, calculate the gradient of accuracy with respect to each knob (\ie temporarily increase the value of one knob, run DNN inference to get the inference results of changed config, calculate the change of accuracy divided by the change of knob value, and repeat this process for other knobs),\jc{i don't get this sentence at all. and this seems secondary to me}
    % \end{packeditemize}
    % where both steps requires extra DNN inference.
    % % \begin{packeditemize}
    % % \item calculating the change of accuracy by alternating the value of one knob in the current configuration while keeping the values of other knobs fixed,
    % % \item dividing the change of accuracy by the change of the knob value,
    % % \item repeating this process for all knobs,
    % % \end{packeditemize} resulting in extra DNN inference on both the golden config (in order to obtain a reference inference results to calculate the accuracy) and the configs nearby the current config.

    % \item To reduce the overhead of the first step (obtain the inference results of a golden configuration as a reference point), we leverage the inference results of the current configuration as a reference point to \textit{estimate} the accuracy of other configurations.
    % Concretely, the accuracy change of other configurations compared to the current configuration is proportional to the corresponding inference results change: if there is no inference results change, there is no accuracy change; if there is a large inference results change, the accuracy change also tend to be large.
    % \kt{Empirical numbers to back it up}

    % \item To reduce the overhead of the second step (running DNN inference to calculate the change of inference results), we can split the change of inference results into two parts. Specifically, we can calculate the inference results change by
    % \begin{packeditemize}
    %     \item calculating the DNN input change (No need for GPU), and 
    %     \item calculating how the DNN input change affects inference results (note that this term corresponds to the \textit{gradient} of the inference results wrt DNN input and can be calculated using one single backpropagation)
    % \end{packeditemize}
    % \kt{Empirical numbers to back this up.}

    % \item 
    % By integrating these two techniques together, one can estimate \accgrad without extra DNN inference and with constant GPU overhead (caused by backpropagation).
    % We present \name, a configuration adaptation system that adapts the configuration by \accgrad.

    % \item Compare \name against region-proposal-based approach and saliency-based approach.

    % \item Experiment result highlight.
    

    
    
    % Our insight comes from an empirical observation: 
    % Mathematically, this insight can be restated as: the mapping between the configuration and its corresponding accuracy is \textit{concave}.
    % By using gradient, we can leverage this concavity to quickly converge to the configuration with highest accuracy under the resource budget.
    
    
    % This is because gradient leverage an important structure in the configuration to efficiently skip those configurations that generate low accuracy.

    % \item 

    % % 1. better config --> locally better config
    % % 2. one knob --> 
    % % 3. multi-knob --> 
    % \item To calculate the gradient of accuracy with respect to each individual knobs, we state an observation. If we increase the value of just one knob:
    % \begin{packeditemize}
    % \item The resource consumption will increase (or decrease)
    % \item The corresponding inference results will become more (or less accurate)
    % \item more change in the inference results, more accuracy improvement (or degradation)
    % \end{packeditemize}
    % % This assumption allows us to quickly check if a different config (that differs from the current config on only one knob) has much higher accuracy: we only need to check if the config consumes more resource and if the inference results are highly different.
    % This assumption allows us to estimate the \textit{gradient} of accuracy wrt each knob.
    % Concretely, we estimate the gradient of accuracy wrt each knob by temporarily increasing that knob a little and checking the inference results difference and resource usage.
    


    % \item 
    % Based on this assumption, we propose a basic version of our proposal: BaseAdapt.
    % Every 1/3 seconds \kt{need to defend 1/3 second}, BaseAdapt will calculate the \accgrad of nearby configs by performing the following steps for each knob:
    % \begin{packeditemize}
    %     \item 
    %     Temporarily increase and decrease the value of the designated knob, obtain their inference results on this 1/3-second video and estimate the accuracy.
    %     Temporarily increase the value of the designated knob in the current config by 1 and obtain the inference results on the 1/3-second video
    %     \item Calculate the change of inference results (before and after increasing the knob value) and estimate the change of accuracy based on the change of inference results,
    % \end{packeditemize}
    % estimate the accuracy change of nearby configs based on the accuracy change of increasing each knobs (a forward pointer here) and then select the config in nearby configs that yield high accuracy within the resource budget.

    % \item 
    % This algorithm can frequently adapt by probing only a small subset of configurations (instead of profiling the whole config space like in profiling-based approach).
    % One may worry that BaseAdapt may converge slowly (as BaseAdapt may stuck in a local optimal, and the optimal config may not be in nearby configs).
    % That said, empirically we find that our solution can still quickly converge to the optimal config. 
    % This is because the locally optimal config only appears occasionally and does not persist, so it is less likely to stuck in a locally optimal config for a long time.
    % Also, it typically takes only 3 - 4 steps to go from the current config to adapt to the optimal config.
    % Empirical evidence here to support these points.
    % Advantage: Avoid the extra overhead caused by evaluating golden config and adaptation is much more frequent (once every 1/3 second) \\
    % Disadvantage:  a lot of extra DNN inference.


    % \item Solve the first issue. Insight: gradient

    % \item Solve the second issue. Insight: gradient decoupling.

    % \kt{propose gradient as a way to reduce the camera-side overhead.}
    
    % Changing the value of one single knob will result in consuming more (or less) resources the inference results would statistically become more (or less) accurate. The accuracy improvement (degradation) is proportional to how much the inference results changed.
    

    % \item
    % We assume that: if a config differs with the current config on \textit{just one knob}, 
    % \begin{packeditemize}
    % \item whether this config has higher accuracy or not depends on whether it has higher resource usage or not.
    % \item the absolute accuracy difference compared to the current config is small when the inference results of this config is small, and vise versa.
    % \end{packeditemize}
    % We empirically evaluate this assumption across a wide range of knobs. 

    % \item
    % The technique above allows us to make 
    

    

    % \item Our insight is that: if there is a config with higher accuracy under the budget
    % there is a config with higher accuracy nearby and we can find this config by merely checking its output.

    
    


    % \kt{Observation: check output to tell accuracy change}
    % \kt{Why better than profiling: 1. frequent 2. 3-4 steps to optimal 3. local optimal is not an issue}
    % \kt{Why better than heuristics: when there exist a config that has higher ACC under the budget, our approach can quickly converge to that config.}
    % However, heuristics do not leverage DNN input.  bounded by their compute, may not be able to find this optimal config
    % while there are cases where heuristics cannot identify such change and may still leverage a suboptimal config
    % config with lower accuracy due the compute limit of their heuristics (a pointer to illustrate why these work generate poor config)}

    
%     \item  Profiling-based.
%         Profiling-based approach leverages the inference results of golden configuration (the most resource-consuming configuration\footnote{Chameleon\cite{chameleon} uses multiple configurations as the reference point to estimate accuracy}) to estimate the accuracy of different configurations.
%         However, \textit{before} calculating the accuracy of different configs, this approach needs to spend extra bandwidth and compute to stream video to the server and run extra DNN inference.
% %         \begin{packeditemize}
% %         \item stream  video to the server
% %         \item spend extra inference to analyze golden configuration 
% %         % \jc{these two points are not separate. just say they use golden config but it takes more bandwidth and compute}
% %         \end{packeditemize}
%         Thus, when the resource (in terms of banwidth and/or GPU compute) is limited, this approach needs to profile less frequently, resulting in using outdated configurations when the optimal configuration has drifted away
%         % , or  significantly prune the search space (which may contain only suboptimal configurations).
%         % estimate the accuracy of a configuration by running {\em extra inference with much more expensive} configurations and comparing their inference results. 
%         % the difference with the inference results of the most expensive configuration 
%         % need extra inference to handle multiple knobs.
%         \kt{here we need to talk general solutions in this space}
%         \kt{The alternative should be something that use few configs}
%         \item 
%         Server-side configuration selection.
%         Existing design selects which regions need to be encoded in high quality based on bounding boxes (region proposals or detections) generated by the DNN to identify which regions need to be encoded in higher quality --> may miss regions critical to improving inference results but far from {\em any} bounding box --> selecting suoptimal regions
        
%         \item 
%         Sensor-side configuration selection.
%         Sensor-side has limited compute power --> relatively simple logic --> selecting suboptimal configuration
%         \kt{People may think of model cascading}
        % : the camera-side heuristics is inaccurate due to the compute limit of camera.
        % : the server-side region proposal is inaccurate since it use bounding box as the unit to assign resource.
    % \end{packeditemize}
    
    % \kt{bring cost considerations in the limitaion instead of saying "frequent"}
    % \kt{Get a sense of how other configurations is working --> condition change we cannot calcu}
    % \item 
    % The research question of this paper is: how to compare the current config with other configurations without extra inference?
    % \item 
    % These three lines of work share one common limitation: they cannot frequently and precisely estimate the accuracy of  different configurations.\\
    % Profiling-based approach --> need to stream uncompressed video and evaluate golden config --> accuracy estimation not frequent enough.\\
    % Configuration selection --> accuracy estimation not precise enough --> wrongfully estimate the accuracy of a different configuration and thus choose suboptimal configuration
    
    
    
    % \item 
    % We takes an alternative approach: instead of estimating the accuracy of \textit{all} configurations, we estimate the accuracy of a \textit{subset} of configurations that are close\kt{need to define what is ``close''.} to current configuration (we call this subset of configurations \textit{nearby configurations}).
    
    % Our insight is that we can rely on the current configuration (instead of the golden configuration) to anchor the accuracy of these nearby configs.
    % Concretely, if the inference results change \textit{for a certain amount}\kt{a pointer here that points to how to calculate this amount} from the current config to a nearby config, the absolute change of accuracy tends to also be proportional to this amount. We then identify whether the accuracy improves or drops by whether the nearby config consumes more resource or not.
    % A measurement to support this point: the linear correlation coefficient between accuracy and inference results change is greater than 0.7 in nearby configs
    
    
    
    % \item 
    % This insight inspires a basic version of our proposal: BaseAdapt.
    % Every 1/3 seconds \kt{need to defend 1/3 second}, BaseAdapt will estimate the accuracy of nearby configs by performing the following steps for each knob:
    % \begin{packeditemize}
    %     \item Temporarily increase the value of the designated knob in the current config and obtain the inference results on the 1/3-second video
    %     \item Calculate the change of inference results (before and after increasing the knob value) and estimate the change of accuracy based on the change of inference results,
    % \end{packeditemize}
    % estimate the accuracy change of nearby configs based on the accuracy change of increasing each knobs (a forward pointer here) and then select the config in nearby configs that yield high accuracy within the resource budget.
    % Advantage: the adaptation is frequent (once every 1/3 second) \\
    % Disadvantage: the profiling overhead is significant: the profiling overhead already consumes more than 50\% of the resource when adapting just one single knob. Moreover, this overhead is proportional to the \# of knobs, making this solution impractical.
    
    % \item 
    % To reduce the overhead, we optimize the most resource-demanding operation in BaseAdapt: calculate the change of inference results.
    % Our insight is that we can split the change of inference results to two parts. Specifically, we can calculating the inference results change by
    % \begin{packeditemize}
    %     \item calculating the DNN input change (No need for GPU), and 
    %     \item calculating how the DNN input change affects inference results (note that this term corresponds to the \textit{gradient} of the inference results wrt DNN input and can be calculated using one single backpropagation)
    % \end{packeditemize}
    % Calculating the change of inference results in this way reduces the overhead of BaseAdapt by more than 100x as it no longer requires extra DNN inference and only requires one single backpropagation.
    % Based on this optimization, we propose \name.
    
    % \item We propose a suite of techniques to further reduce the overhead of \name.
    
    % \item Claim that \name does not work for DNN knobs. 
    
    % \begin{packeditemize}
    %     \item We may stuck into a local optimal
    %     \kt{Yes, but not frequently, rationale: local optimal won't persist}
    %     \item The adaptation speed of our approach may be slow: it may take several steps to approach to the optimal.
    % \end{packeditemize}
    % \kt{empirically, current config -> optimal only takes 3-4 steps}
    % \kt{say that the overhead of BaseAdapt is significant (compared to normal inference/profiling-based approach)}
    
    % \item
    % How to calculate this difference with low overhead?
    % Our insight is that 
    
    % The issue of just knowing such information is that one may stuck into a configuration that has highest accuracy among nearby configurations.
    
    % This information is enough for an adaptation system to approach the optimal, as there is no stable local optimal in the configuration space within a given resource budget.
    % For those configurations that does not hit the resource budget, we ca
    
    
    % Profiling-based approach estimate accuracy with extra streaming and inference overhead, 
    % Configuration search can generate optimal configuration at the cost of streaming uncompressed video and , while configuration generation may constantly generate suboptimal configuration.
    % generating new configuration  new configuration may generate suboptimal configuration, 
    
    % --- extra inference is too expensive, simple heuristics not accurate enough, server-side feedback too coarse-grained.
    % estimating the accuracy by obtaining the inference results of the most expensive configuration as the ``ground-truth''.
    % 2. handling multiple knobs by either running extra inference or relying on inaccurate heuristics
    % \item To handle the first limitation, our insight is that: estimating the effect of changing the config on inference accuracy can be estimated without running expensive extra inference. 
    % specifically, the change of inference accuracy can be measured by the change of inference results.
    % If there is no change in inference results, the inference accuracy also does not change.
    % If the inference results change significantly, the accuracy change also tends to be significant.
    % We then infer whether the accuracy improves or not by whether the new config consumes more resource or not.
    % \kt{A jump here.}
    % Essentially, we can quickly calculate the {\em gradient between the change of a SINGLE config knob and  change of the DNN inference accuracy} by changing that knob and running one extra inference.
    % \kt{How does that help in terms of getting the accuracy w/ extra inference}
    % \kt{1. Why is nearby OK (local optimal) 2. not referring to the golden configuration (what enables us to quickly calculate the gradient)}
    % \kt{Golden configuration?? Nearby?? Gradient??}
    % \kt{??How to move to the optimal configuration as fast as possible?}
    % (some statistical evidence!)
    % while estimating the absolute number of accuracy requires the ``ground truth'', estimating the accuracy change when changing the current configuration to another configuration does not, as we can estimate the magnitude of accuracy by looking at the change of the output, and estimate the sign of accuracy change by whether the configuration consumes more resource or not.
    % \item This way of estimating the accuracy change via output change is not generally accurate. 
    % For example, there may be one configuration that the output changes a lot compared to the current configuration, but the accuracy of these two configurations are the same.
    % However, we find that this approach is statistically accurate when we only consider those configurations that only alters one knob compared to the current configuration.
    % \item 
    % \kt{Why does it work? Monotonicity}
    % this insight inspires a basic version of our proposal: BaseAdapt.
    % % We propose a solution BaseAdapt based on this insight. Once 
    % every $k$ frames, BaseAdapt will change each config knob by a small amount, estimate its change on inference accuracy, and change the config knobs in the direction that maximizes the inference accuracy within a resource budget. 
    % \item 
    % \kt{Why baseadapt is inefficient}
    % BaseAdapt frequently adapts the configs (every $k$ frames) --> it reacts to sudden changes in the input earlier and converges to a close-to-optimal config faster than existing solutions. 
    % BUT BaseAdapt does NOT handle more config knobs efficiently. 
    % \item our full solution OneAdapt can quickly calculate the {\em gradient between the change of a MULTIPLE config knob and  change of the DNN inference output.}
    % Specifically, we SPLIT this gradient to two parts: 
    % (1) calculating the output change by first calculating the DNN input change (No need for GPU), and 
    % (2) calculating how the DNN input change affects DNN output (one single backpropagation regardless of the \# of knobs).
    % both inference on the current configuration $c$ and all configurations that are close to $c$ (\ie the configurations that differs with $c$ on only one knob with the difference value smaller than a threshold), and then move to the closest configuration.
    % \item We find that this solution is better than the baseline when there is only one knob. However, the performance of this solution is suboptimal when there are multiple knobs, as calculating the change of output with respect to every knob requires extra inference to handle multiple knobs simultaneously (the second limitation).
    % To reduce the overhead caused by extra inference, we calculate the change of output by leveraging the differentiability of the DNN.
    % Specifically, we can calculate the output change by first calculating the DNN input change, and then calculating how the DNN input change affects DNN output.
    % The former can be calculated without accessing the DNN (thus requires no extra inference), and the latter can be calculated using backpropagation
    % \item With this insight, we present OneAdapt, a solution based on BaseAdapt that calculates the output change by leveraging the differentiability of the DNN.
    
    % Evaluation: across 4 types of data sources and 3 applications, \name achieves \fillme\% more throughput without hurting accuracy, or increases accuracy by \fillme\% with similar throughput.



% \tightsection{Introduction}
% % Deep-neural-network-based (DNN-based) analytics on data streams (\eg video
% % streams or LiDAR feeds) are everywhere.
% % For example, people leverage DNNs to analyze traffic video feeds for traffic monitorings~\cite{trafficvision, traffictechnologytoday, goodvision,intuvisiontech, vision-zero, msr}, analyze the information from multiple types of sensors (including camera, LiDAR and Radar sensors) to enable long-range vehicle and pedestrian detection for autonomous driving~\cite{tusimple,waymo,motional}.
% % The input data stream varies a lot over time.
% % For example, in autonomous driving, the number and the moving speed of vehicles and pedestrians varies a lot over time (\eg the number of vehicles and humans will be much higher when driving in daytime), areas (\eg the vehicle movement speed is much higher when driving in the highway), current location (\eg the number of pedestrains will be much higher at the crossroad), traffic condition (\eg the number of vehicles significantly increases in traffic congestion).
% % \jc{highlight the need for tuning configuration knobs when you bring up "data stream varies over time"}
% % This trend inspires system research for these applications~\cite{vigil,glimpse,mcdnn,videostorm,noscope,neurosurgeon,awstream,chameleon,focus,adascale,filterforward,vstore,cracking,dds,reducto,blazeit,yoda,vcm,elf,ekya}.
% % % \jc{can we cite some dnn-based analytics systems use cases, where the input distribution varies over time, in terms of frequency of object occurrences, shape/size, etc? be as concrete as possible please} \kt{done}

% % Deep-neural-network-based (DNN-based) analytics on data streams (\eg video
% % streams or LiDAR feeds) are everywhere.

% \kt{Rewrote this para.}
% Many applications send data streams to DNNs for analytical purposes.
% % Many applications rely on DNNs to perform accurate inference on various data streams (\eg video streams or LiDAR feeds).
% For example, DNNs are used to analyze traffic video feeds to monitor vehicle speed and spot traffic jams~\cite{trafficvision, traffictechnologytoday, goodvision,intuvisiontech, vision-zero, msr} , and analyze data streams from infrared cameras, LiDAR sensors, and radar sensors to detect vehicles and pedestrians for autonomous driving~\cite{tusimple,waymo-blog,motional}.
% % \jc{kuntai, the logic here is quite muddy.. it's unclear why content varying over time is interesting/important. 
% % maybe try a different flow: as these DNN-based applications require high accuracy, they use a great amount of compute and network resource. 
% % Many prior efforts have leveraged a common feature of these data streams: their content varies greatly over time. 
% % For example...
% % To leverage these opportunities, recent work exposes...
% % }
% As these DNN-based applications require high accuracy, they use a great amount of GPU compute and/or network resources, which makes DNN-based applications too expensive for people to afford\kt{citation here}.
% Fortunately, many prior efforts identify a resource-saving opportunity: the content of the data stream varies a lot over time and some of the content allows these applications to generate accurate analytic results with \textit{much less} resource usage.
% % (\ie the amount of resource required to provide accurate analytic results) varies alongside with the content of the data stream, and reduce the resource usage by using less resource when resource demand is low.
% % To reduce the resource usage, many prior efforts identifies the variability of the content of the data stream.
% % a common characteristic of these data streams---their contents vary greatly over time---to reduce the resource usage of these DNN-based applications.
% % The content of these data streams vary greatly over time.
% % For example, in autonomous driving, the number and the moving speed of vehicles are constantly changing over time (\eg the number of vehicles will be much higher compared to driving in night time), location (\eg cars move faster on the highway) and traffic condition (\eg the number of vehicles significantly increases in traffic congestion).
% % For example, in dashcam video streams, the number and the moving speed of vehicles are constantly changing over time (\eg the number of vehicles will be much larger during daytime than during night), location (\eg cars move faster on the highway) and traffic conditions (\eg the number of vehicles significantly increases in traffic congestion).
% % For example, in one traffic video stream that aims to localize vehicles on a traffic lane,
% For example, in a traffic video stream, the moving speed of vehicles can be much lower during red traffic light compared to green traffic light, so one can analyze less frames during red traffic light (and thus save GPU compute resource) and still accurately capture the motion of the vehicles.
% % \jc{highlight the need for tuning configuration knobs when you bring up "data stream varies over time"}
% % Facing this trend, the system research community develop \textit{adaptation-required knobs} to \textit{enable} saving resources when the data can be safely analyzed by using less resource without hurting accuracy and timely \textit{adapt} these knobs to save resource when such data appears. ~\cite{vigil,glimpse,mcdnn,videostorm,noscope,neurosurgeon,awstream,chameleon,focus,adascale,filterforward,vstore,cracking,dds,reducto,blazeit,yoda,vcm,elf,ekya}.
% % To save resources through such temporal variability in the data streams,
% Technically, to capture such resource-saving opportunity,
% recent proposals~\cite{vigil,glimpse,mcdnn,videostorm,noscope,neurosurgeon,awstream,chameleon,focus,adascale,filterforward,vstore,cracking,dds,reducto,blazeit,yoda,vcm,elf,ekya} expose internal tunable parameters (referred to as \textit{knobs}) and \textit{timely configure} these knobs (we denote the knobs together with their configured values as a \textit{configuration}) according to the content of the data streams to save resources (\eg GPU compute and network) while maintaining high inference accuracy.
% % \jc{can we cite some dnn-based analytics systems use cases, where the input distribution varies over time, in terms of frequency of object occurrences, shape/size, etc? be as concrete as possible please} \kt{done}



% % \jc{how about we pitch them as two parallel trends: (1) temporal variation of input, and (2) an increasingly number of knobs, $\rightarrow$ the challenge of timely adaptation in a large configuration space.}

% % We observe that these systems expose an \textit{increasing} number of internal knobs.
% % The underlying trend that drives this increase is two-fold (further discussion in \S\ref{subsec:numer_of_knobs}). 
% % % First, these systems need to develop new knobs to not only provide accurate analytic results under all kinds of resource budget due to heterogeneous deployment settings, but to also handle new emerging applications (\eg LiDAR-based object detection for autonomous driving and infrared-based human detection for night-time security monitoring).
% % First, these systems need to develop new knobs to not only trade-off between the accuracy and different kind of resources in order to handle all kinds of resource budget due to heterogeneous deployment settings, but to also handle new emerging applications (\eg LiDAR-based object detection for autonomous driving and infrared-based human detection for night-time security monitoring).
% % \ga{It'll be helpful to make it explicit that knobs also regulate the resource demand and hence can be used to handle heterogeneous resource budget.}
% % \kt{fixed}
% % % These knobs trade-off between accuracy and different kinds of resource in order to
% % Second, as the need of DNN-based analytics quickly grow, these systems need to tune existing type of knobs at a finer granularity to support more concurrent DNN-based analytic jobs. \ga{The need to partition isn't clear. Why were the knobs joined in the first place, before partitioning?} \kt{fixed}

% We observe that there is already a broad set of knobs\footnote{Previous work proposes at least 16 knobs includes 6 video encoding knobs~\cite{vstore, chameleon, dds, videostorm, awstream}, 9 frame filtering knobs~\cite{reducto, vigil, glimpse}, and the knobs that differentiate spatial video quality knob~\cite{dds,accmpeg,eaar}, which can be partitioned into thousands of knobs if tuned in fine granularity~\cite{accmpeg}.}\cite{vstore,chameleon,dds,videostorm,awstream,reducto,vigil,glimpse,dds,accmpeg}, 
% and the set is still growing, thanks to two trends.
% % We observe that the number of such configuration knobs is already huge (\eg more than 16 different knobs\footnote{These 16 knobs includes 6 video encoding knobs~\cite{vstore,chameleon,dds,videostorm,awstream}, 9 frame filtering knobs~\cite{reducto,vigil,glimpse}, and the knobs that differentiate spatial video quality knob~\cite{dds,accmpeg}, which can be partitioned to thousands of knobs if tuned in a fine granularity.} are introduced in video analytic systems~\cite{vstore,chameleon,dds,videostorm,awstream,reducto,vigil,glimpse,accmpeg}) and is still expanding.
% % We observe that these systems expose an expanding set of configuration knobs that leverages temporal variabilities in the data stream to save resource without hurting the accuracy.
% % % be adapted to the temporal variations of the input data stream to save resource.
% % There are two reasons behind this trend. 
% % First, these systems need to develop new knobs to not only provide accurate analytic results under all kinds of resource budget due to heterogeneous deployment settings, but to also handle new emerging applications (\eg LiDAR-based object detection for autonomous driving and infrared-based human detection for night-time security monitoring).
% First, when people deploy DNN-based analytic systems into practice, they found that these systems need more knobs to explore new resource-saving opportunities introduced by new types of data streams (\eg LiDAR feeds), new applications (\eg video captioning) and new deployment settings (\eg multi-camera video analytics~\cite{chameleon, vigil}, multi-server video analytics~\cite{elf}).
% % First, these systems need more knobs to not only trade between different type of resources to fit into more deployment settings (\eg the user may stream the data out from cheap camera through expensive LTE network for analytics. In this case, it is more ideal for the system to trade server-side compute for bandwidth~\cite{dds,eaar} instead of trade camera-side compute for bandwidth~\cite{vigil,glimpse,accmpeg} to simultaneously reduce the bandwidth usage without  the camera-side compute usage), but to also 
% % \ga{It'll be helpful to make it explicit that knobs also regulate the resource demand and hence can be used to handle heterogeneous resource budget.}
% % \kt{fixed}
% % These knobs trade-off between accuracy and different kinds of resource in order to
% Second, as these systems need to run more analytic jobs than before,
% % these systems need to support more concurrent analytic jobs under the same resource budget, which requires them to 
% they need to tune existing knobs at a finer granularity (by partitioning existing knobs into \textit{multiple} fine-grained knobs) to further reduce the resource usage of each analytic job.
% % further reduce the resource demand for running one analytic job without hurting the accuracy.
% For example, in a dashcam video stream, when the input video contains \textit{only one} small object, one may need to encode \textit{the whole video} in high fidelity in order to make this object detected, resulting in high bandwidth usage~\cite{chameleon,awstream}.
% % when the input video contains one small object, one may need to encode and stream the whole video into high resolution to detect such object, resulting in high bandwidth usage~\cite{chameleon,awstream}.
% However, prior effort~\cite{dds,eaar,accmpeg} shows that the areas that are not related to the object can be encoded in low fidelity to save bandwidth and realizes this potential by \textit{partitioning} the video into different areas and assigning different areas with different fidelities.
% % , by assigning different areas with different resolutions\footnote{In fact, prior work assigns different areas with different quantization parameters, a parameter that controls the fidelity of the encoded video without changing the resolution. We use resolution in the text for understandability consideration.}, it only needs to encode the area that contains the object into high resolution and other areas can be safely encoded in low resolution. This significantly reduces the bandwidth usage.

% % % redirected enumerate to packedenumerate for reformater in macro.tex. DON'T
% % % CHANGE!
% % \begin{enumerate}
% %   \item 
% % As DNN-based analytics are deployed on heterogeneous deployment settings that have different types of resource budgets, this requires the corresponding systems to propose new knobs in order to fit into
% % different resource budgets. Take video analytics as an example. If the
% % user analyzes the video feeds locally by a compute-constrained mobile
% % phone, the main focus for the systems is to fit into the compute budget
% % of the phone (\eg by skipping those frames that are highly similar to
% % their previous frames~\cite{reducto,glimpse}). However, if the user
% % instead streams the video feeds to a GPU-equipped server through a
% % bandwidth-limited LTE network, the main focus is instead fitting into
% % the limited LTE bandwidth (\eg by performing video
% % compression~\cite{accmpeg,vigil,glimpse,reducto}).

% %   \item As DNN-based analytics quickly expand, the corresponding systems need to
% %         partition existing knobs into more fine-grained version to capture more
% %         resource-saving opportunities. Take video-based vehicle detection as an
% %         example. Chameleon~\cite{chameleon} and AWStream~\cite{awstream}
% %         identify that the system only need to encode the video in a high
% %         encoding quality when the vehicle appears. To further explore the
% %         potential of varying video encoding quality, the following
% %         work~\cite{dds,eaar,accmpeg} finds that a lot of areas in the video do
% %         not need to be encoded in high quality (\eg the areas that contain
% %         non-vehicle-related backgrounds like trees and buildings) and proposes
% %         fine-grained spatial encoding quality to capture this opportunity.
% %   \item Since new applications quickly emerge (\eg LiDAR-based object detection,
% %         Infrared-based human detection \kt{a bunch of citations here}), this requires the deep learning systems
% %         to develop new knobs (or even developing new system components) to fit
% %         into the need of different applications. For example, in order to handle
% %         LiDAR data, people are proposing new encoding standard and new
% %         knobs~\cite{MPEG-point} to efficiently encode and process LiDAR data.
% %         \roy{I understand you are trying to distinguish old types of application
% %         and new ones, but I still feel the first and third items are kind of
% %         repetitive? Both items are trying to say there is the need for new
% %         knobs, right? Maybe merge them into one?}
% % \end{enumerate}

% % Not only the number of knobs are already huge (\eg in video analytics, previous work introduces 6 video codec encoding knobs~\cite{vstore,chameleon,dds,videostorm,awstream}, 9 frame filtering knobs~\cite{reducto,vigil,glimpse} and even thousands of knobs for fine-grained video encoding quality assignment~\cite{accmpeg}) and still expanding
% % % \ga{Quantify.}
% % , these knobs also need to be timely adapted~\cite{awstream,chameleon,dds,eaar,elf} due to input data change or resource budget change in order to achieve high inference accuracy.
% % Thus, the research question is: how to navigate the large configuration space (\ie all possible choices of knob values) and and pick the optimal configuration that generates accurate inference results under the current resource budget?


% % As the number of knobs are already huge (\eg more than 16 different knobs\footnote{These 16 knobs includes 6 video encoding knobs~\cite{vstore,chameleon,dds,videostorm,awstream}, 9 frame filtering knobs~\cite{reducto,vigil,glimpse}, and the knobs that differentiate spatial video quality knob~\cite{dds,accmpeg}, which may include thousands of knobs if tuned in a fine granularity.} are introduced in video analytic systems~\cite{vstore,chameleon,dds,videostorm,awstream,reducto,vigil,glimpse,accmpeg}) and is still expanding,
% % \ga{Quantify.}
% % , these knobs also need to be timely adapted~\cite{awstream,chameleon,dds,eaar,elf} due to input data change or resource budget change in order to achieve high inference accuracy.
% Given the \textit{large yet expanding} set of knobs, the research question of this paper is:
% \textit{among a large number of configurations, how to quickly adapt to optimal configuration that achieves high accuracy under a given resource budget?}


% The first way to address this problem is to frequently profile different configurations to obtain their resource usage and accuracy, and then pick the configuration that yeilds high inference accuracy without exceeding the resource budgets\cite{chameleon,awstream,vstore,videostorm}.
% % meets the resource
% % budget and generates the most accurate inference results
% However, each profiling
% needs to run \textit{extra} inference to analyze multiple configurations (some are expensive in terms of resource usage). %before obtaining the profile.
% % As a result, when the optimal configuration changes, this approach need to perform the extra inference to obtain the new optimal configuration, thus incurring high delay when the GPU resource is limited.
% Thus, when the GPU compute is limited, this approach needs to either profile less frequently, resulting in using outdated configurations when the optimal configuration has drifted away, or significantly prune the search space (which may contain only suboptimal configurations). %profile fewer configurations, which may miss the optimal configuration. 
% % Both of them lead to a sub-optimal trade-off between the accuracy and the resource usage.
% % \ga{Call out the downsides of extra inference.} \kt{fixed}









% % \kt{This para needs a rewrite}
% % The other approach performs no extra inference and instead, computes the
% % configuration based on recent DNN outputs (including intermediate outputs) through cheap heuristics~\cite{dds,eaar,elf} or through DNN-based configuration generator~\cite{accmpeg,casva}). 
% % \ga{What does ``derives the configuration'' mean?} \kt{fixed}
% % % However, there can be many configurations that meet the resource budget. \ga{There has been no mention of budget so far.}
% % % Without profiling most of them, it is difficult to separate the configurations that yield similar DNN output from those that yield more accurate DNN output by merely looking at recent DNN outputs.
% % % As a result, this approach waste resource on those configurations that yield similar DNN output and thus cannot quickly adapt to the optimal configuration. 
% % \ga{I don't fully follow this paragraph and it needs more explanation. That said, can I view the techniques in this paragraph as a pruning mechanism to identify the promising configurations?}
% % \kt{This para needs a rewrite}
% \kt{rewrote the next 3 paras}
% The second approach~\cite{dds,eaar,elf} performs no extra inference and instead generate new configuration by leveraging region proposal (DNN-generated bounding boxes that may contain objects inside).
% For example, based on the region proposal of the current frame, EAAR~\cite{eaar} encodes the bounding boxes inside the region proposal of the current video frame  in higher encoding quality on future frames so that the objects inside the region proposals are more likely to be detected.
% However, this approach may generate sub-optimal configuration, as this approach assigns the \textit{same} configuration (\eg encoding quality~\cite{dds,eaar}) for all the pixels inside each bounding box (unless multiple regions overlap) while an optimal configuration may assign \textit{different} configuration for different pixels inside a bounding box.
% For example, \kt{plot a figure here.}
% % This is sub-optimal as some pixels inside the bounding box can be in lower encoding quality (\eg those pixels that are outside the object but inside the region) and some pixels outside the bounding boxes may require higher encoding quality.
% % However, instead of comparing between different configurations, this approach generates new configuration by postprocessing region proposals.
% % As a result, it can only explore those configurations that are generatable from the heuristics, which may miss the optimal configuration that may not be generatable from the heuristics.
% % For example, EAAR~\cite{eaar} encodes the regions inside the region proposals with higher encoding quality so that the objects inside the region proposals are more likely to be detected.
% % However, as shown by AccMPEG\cite{accmpeg}, not all pixels inside the region proposal need to be in higher quality, and some pixels outside the region proposal needs to be in higher quality.





% % based on recent DNN outputs (including intermediate outputs)~\cite{dds,eaar,elf,accmpeg,casva}.
% % % \jc{i still dont quite get why we use dds here. isn't some bandit/RL-based solution a better fit?}
% % % For instance, DDS~\cite{dds} tunes encoding quality by first encoding all pixels at a low quality and streaming them to the server-side DNN, whose output (region proposal) is then used to tune the quality at different regions.
% % Though no extra inference is run, this approach tends to adapt {\em slowly}, as each DNN output reveals limited information regarding the \textit{highly complex} relationship between the configurations and DNN inference output/accuracy, due to the complexity of the DNN itself and the preprocessing modules before the DNN (\eg video codecs).
% % We take EAAR~\cite{eaar}, a system for video object detection, as an example.
% % EAAR adjusts the video encoding quality by collecting the regions from the DNN that may contain objects of interest and encoding these regions in higher encoding quality on future video frames.
% % % After that, it encodes these regions in high quality on the next video frame.
% % Thus, the objects inside these regions are much more likely to be detected.
% % % This approach then lets the sensor encode all these regions in high encoding quality on the next video frame so that the objects inside these regions can be accurately detected.
% % However, as the regions generated by the DNN may not include all the regions that contain the objects, the object detection DNN may miss some objects and thus EAAR needs to further adjust the regions corresponding to these missing objects.
% % For instance, the impact of configuration on DNN accuracy is affected by two complex blackboxes: DNN itself as well as the video codecs.
% % However, the \textit{adaptation speed} (\ie the time it takes to obtain the optimal configuration) of this approach can be slow.
% % For example, DDS~\cite{dds} tunes the encoding quality of different areas of the video in the following steps.
% % First, DDS let the camera encode the whole video into low quality and stream it to the server.
% % The server then analyzes the video to obtain the areas that may contain objects and let the camera resend those areas in high encoding quality for an extra round of inference.
% % % through cheap heuristics~\cite{dds,eaar,elf} or through DNN-based configuration generator~\cite{accmpeg,casva}).
% % However, the \textit{adaptation speed} (\ie the time it takes to obtain the optimal configuration) of this approach can be slow.
% % % explore many configurations to accumulate enough DNN outputs before converging to the optimal one.
% % % need to accumulate enough DNN outputs in order to obtain the optimal configuration.
% % % This is because this approach only examine one configuration at a time.
% % This is because they only get one DNN output at a time.
% % As the relationship between the configuration to the inference accuracy is highly complex (due to complexity inside the underlying system (\eg video codec) and the DNN itself), this approach needs to spend time accumulating enough DNN outputs before obtaining the optimal configuration, resulting in slow adaptation speed.
% % Thus, it is difficult to identify whether a new configuration improves accuracy or not based on the current DNN output.
% % the performance of other configurations.
% % the DNN ouput on just one configuration is not enough for this approach to immediately obtain the optimal configuration thus
% % As a result, 
% % this approach needs to accumulate enough DNN outputs to reach the optimal configuration. 
% % The optimal configuration may have already changed (due to the change of input content or resource budget) before this approach reaching it.
% % The optimal configuration may have already changed.

% % However, there can be many configurations that meet the resource budget.
% % Without profiling most of them, it is difficult to separate the configurations that yield similar DNN output from those that yield more accurate DNN output by merely looking at recent DNN outputs.
% % As a result, this approach waste resource on those configurations that yield similar DNN output and thus cannot quickly adapt to the optimal configuration. 


% Moreover, the heuristics used in the second approach are designed for specific types of knobs and are not directly applicable to other knobs (though these heuristics \textit{could} be augmented and used to adapt other knobs).
% % even if they can be purposely built to efficiently support some knobs. 
% % are hand-crafted for individual applications or configurations and thus not generalizable to other configurations and applications.
% For example, EAAR~\cite{eaar} generates new configuration of future frames based on region proposal of the current frame.
% As a result, EAAR may not be ideal for tuning, for example, determining whether to analyze this frame or not.
% This is because the optimal configuration of this frame may vary a lot compared to next frame.
% % This is because  as these knobs require the system to analyze the temporal characteristics of these frame, which are not analyzed by EAAR.
% % We take EAAR~\cite{eaar}, a system that serves object detection, as an example.
% % EAAR assigns the regions that may contain objects based on the current frame and encodes these regions with higher encoding quality to in the future frames to make more objects detected.
% % In a higher level, EAAR applies the decision generated from the current frame to the future frames.
% % However, this may not be a suitable way to adapt the knobs that, for example, decide which video frames can bypass the DNN inference.
% % This is because the optimal decision may vary a lot between the current frame and the future frames: if the current frame needs to be forwarded through the DNN, it is more likely that the next frame should bypass the DNN inference.
% % As a result, EAAR may not directly apply to the DNN-bypassing knobs.



% The third approach trains models (\eg saliency generator~\cite{accmpeg,??} or configuration generator~\cite{casva}) and leverages these models to generate new configuration.
% However, the accuracy of these models degrade over time and are not accurate enough to generate optimal configuration when the characteristics of the input data changes (\eg when a remote small object appears in the video). 
% % unless these models are as complex as the DNN and the.
% This is because the mapping between the input and its corresponding optimal configuration is highly complex due to the complexity of the DNN itself and the preprocessing modules before the DNN (\eg video codecs~\cite{h265,h264}).
% \kt{an example figure to support this point.}
% As a result, these models is not able to accurately learn this mapping (unless these models are as complex as the DNN and the preprocessing modules) and may produce sub-optimal configurations when the content of the input data shifts (\eg when a drone quickly flies away the ground), unless these models are frequently retrained, which requires extra inference to label the optimal configuration before retraining starts.
% % and then leverage this model to adapt the configuration.
% % However, as the compute of such model is limited due to \fillme, the model may no longer being able to predict the optimal configuration when the input content changes.
% % For example, \fillme.





% % Moreover, the heuristics used in the second approach are designed for specific types of knobs and are not directly applicable to other knobs (though these heuristics \textit{could} be augmented and used to adapt other knobs).
% % % even if they can be purposely built to efficiently support some knobs. 
% % % are hand-crafted for individual applications or configurations and thus not generalizable to other configurations and applications.
% % We take EAAR~\cite{eaar}, a system that serves object detection, as an example.
% % EAAR assigns the regions that may contain objects based on the current frame and encodes these regions with higher encoding quality to in the future frames to make more objects detected.
% % In a higher level, EAAR applies the decision generated from the current frame to the future frames.
% % However, this may not be a suitable way to adapt the knobs that, for example, decide which video frames can bypass the DNN inference.
% % This is because the optimal decision may vary a lot between the current frame and the future frames: if the current frame needs to be forwarded through the DNN, it is more likely that the next frame should bypass the DNN inference.
% % As a result, EAAR may not directly apply to the DNN-bypassing knobs.
% % However, EAAR may be sub-optimal if applied to the knobs that decide which video frames can bypass the DNN inference without hurting the inference accuracy.
% % This is because EAAR make an assumption that do not fit this set of knobs.
% % Concretely, the current design of EAAR generates the configuration on one frame and apply it to the future frames, which assumes that the optimal knobs on one frame generalizes to the future frames.
% % However, this assumption may not be true in the scenario of bypassing DNN inference: if one frame needs to be forwarded through the DNN, it is more likely that the next frame should bypass the DNN inference, and vise versa.
% % The violation of this assumption results in the sub-optimal adaptation behavior of EAAR: EAAR may continuously performing inference on a few frames and then continuously bypassing the DNN inference on the next few frames, while the optimal way is to perform inference intermittently.
% % This 
% % This is because making such decision requires the adaptation algorithm to analyze these frames without performing DNN inference on these frames, while the current design of EAAR lets the DNN ingest this frame first and then analyze this frame leverage the intermediate analytical results on this frame for further use.
% % performing DNN inference on this frame and then harnessing the intermediate outputs generated by the DNN inferences. 
% % As a result, EAAR either obtains no extra information on one frame besides the pixel values of this frame (thus cannot make accurate decision on whether letting this frame bypassing DNN inference or not), or analyzes this frame at the cost of performing DNN inference (thus this frame cannot bypass the DNN inference).
% % does not extract any information of one frame  while the current design of EAAR always inference on the current frame and are agnostic to the future frames.
% % making such a decision requires estimating the similarity of the inference results, between those discarded frames and reserved frames, while EAAR focusing on extracting the regions that may contain objects, where only a small subset of them will appear in the final inference results.
% % Take DDS~\cite{dds} as an example, which analyzes the video and then resends some areas of the video that may contain objects of higher fidelity.
% % As the recent areas are derived from the output of a specific DNN component (region proposal) that aims to facilitate object detection, this heuristic is not directly applicable to tasks like video classification.
% % Moreover, this heuristic does not apply to tune frame-discarding knobs~\cite{vigil,glimpse,reducto} that discard similar frames to save GPU compute, because the way DDS obtains the output to tune the knobs incur more GPU compute in the first place. 
% % the knobs in frame discarding techniques 
% % (\ie discarding the frames that produce similar inference results compared to previous frames~\cite{vigil,glimpse,reducto}) without further adjustments, since its adaptation logic (\ie resending some areas of the video that may contain objects) happens \textit{after} DNN inference while frame filtering needs to be performed \textit{before} DNN inference to save GPU compute cost. 
% % As a result, DDS does not directly generalize to other 
% % \ga{How is this paragraph on DDS pertaining to profiling and avoiding extra inference? The relationship isn't clear.} \kt{fixed}
% % \jc{not sure ganesh's comment was addressed. i think the confusion is whether you are criticizing dds's logic being inefficient or not generalizable. if it's the latter, just say it explicitly.}


% % An ideal configuration adaptation system should meet these two
% % requirements: 1. quickly adapt to optimal configuration in a large configuration
% % space without extra inference 2. minimum assumption to the underlying system.

% Therefore, an ideal configuration adaptation system needs to serve \textit{a wide range of knobs}, and compare between different configurations formed by these knobs  \textit{without extra inference}.

% % \kt{Pitch the cause of the previous work limitation as they only using DNN outputs -- which can change a lot between different configuration and video content -- to predict the performance on unknown configuration and unknown content.
% % Our approach combines the DNN parameters -- which does not change between different configuration and video content -- to better generalize the prediction of the performance on unknown configuration and unknown content.
% % }

% % \jc{i guess the rest of the intro hasn't been updated since last wednesday. just to recap, here's the flow:
% % \begin{packeditemize}
% %     \item start with a new abstraction, \accgrad, to more efficiently adapt configurations than prior schemes, especially in a large configuration space, and why?
% %     we present \name, the first efficient implementation of \accgrad
% %     we should clarify that prior work could expose this abstraction as well, but they suffer high overhead (why?). 
% %     \item \name approximates \accgrad based on two observations: 
% %     (1) the values of each configuration can be ordered in a way that \fillme, and
% %     (2) the more changes of confidence scores around the threshold, the more accuracy will change.
% %     \item based on the two observations, \name does \fillme
% %     \item operators can use \name to tune a range of configurations that influences dnn input. this class of config covers many existing systems. but notably, this doesn't cover \fillme (may point to a synergy with recent online learning papers like ekya --- in some sense, they also handle input drift, but they choose to retrain the model, and our approach is more lightweight.)
% % \end{packeditemize}}

% % \kt{Stress that knob is trading res usage for acc}
% % \kt{Adaptation goal: expose an abstraction: monitoring both }

% % \kt{
% % Expose 1 abstraction:
% % resource-knob gradient
% % DNN output (We use the change of confidence values around the threshold, see \S\ref{??} for further detail) gradient
% % % confidence change gradient
% % Say it correlates with accuracy?
% % With this gradient, we can 1). efficiently optimize knobs

% % Previous work, if repurposed, incurs extra inference.

% % Advantage: can be calculated without extra inference
% % }


% % To realize these two objectives, we expose a new abstraction: , which means the performance change divided by knobs change when changing the knobs by a little.
% % Concretely, performance gradient includes resource usage gradient, and DNN output gradient (we measure the DNN output change by measuring the absolute change of confidence scores around the confidence threshold. See \S\ref{??} for further details).


% \kt{rewrote this part}
% We advocate that the adaptation system for DNN-based analytics should expose a new abstraction: \textit{\outputgrad}, which estimates \textit{the gradient of DNN output with respect to each knob}.
% We present \name, a system that implements \outputgrad and uses it to adapt configurations with constant GPU overhead and no extra inference.
% % Based on \outputgrad, we present \name, a configuration adaptation system that implements \outputgrad with constant GPU overhead and with no extra inference.
% % Specifically, \name measures \outputgrad by how much a small change in the current value of each knob \textit{flips} the DNN-returned confidence scores from below (or above) the confidence threshold to above (or below). 
% Specifically, \name measures \outputgrad by how much a small change in the current value of each knob changes the output\footnote{We measure the change of output by summing up all values inside the output and measuring the change of the sum}.
% % We measure \outputgrad by how much a small change in the current value of each knob affects the DNN-returned confidence scores near (both below and above) the given confidence threshold.
% % Note that this measurement does not impose an extra burden on the application side since most of the applications already expose confidence scores to indicate the uncertainty of DNN outputs and use confidence thresholds to filter out DNN outputs with low confidence. %those uncertain results returned from the DNN.
% One may question that why \name studies the output of the DNN instead of the accuracy of the application.
% To answer this question, \name makes an assumption: when we \textit{only} change the value of \textit{one single knob} in a way that makes the system consume more resource, \textit{statistically} the accuracy will be improved. Moreover, more change on the output, more accuracy improvement.
% We empirically validate that this assumption over a wide range of knobs and applications (see \S\ref{??} for details).
% % We will talk about the applicability and the 
% % Moreover, more change in the output, more improvement on accuracy (see \S\ref{??} for more rationales).
% % We 
% %those uncertain results returned from the DNN.
% % Statistically, more changes in the ``near-confidence-threshold'' DNN outputs will likely cause more changes in the inference accuracy (as will be elaborated in \S\ref{subsec:correlation})\footnote{This correlation does \textit{not} assume that a confidence score always directly indicates the accuracy of its corresponding detection/classification results.}.
% % % \outputgrad correlates with how much the accuracy \textit{changes} with knobs 
% % Intuitively, this is because the confidence threshold determines whether a detection or classification result is accepted (as part of the accuracy calculation) or rejected (thus having no effect on the accuracy).
% % When the knob change only alters the DNN output by a little, the corresponding accuracy change also tends to be minor.
% % Thus, more change on the ``near-threshold'' DNN outputs, more changes on the inference accuracy.




% % how much the DNN output changes when varying each individual knob by a little (we measure the DNN output change by measuring the change of those confidence scores around the confidence threshold, see \S\ref{??} for the mathematical formulation and the intuition behind).
% % We call this metric \outputgrad for short.
% % when slightly changing the knob  (we call it \outputgrad for short).
% % We will cover the detail


% % \kt{Should we allocate a paragraph to talk about the overhead of calculating ground truth here?}
% % We acknowledge that using DNN output change cannot obtain the exact number of the accuracy change.
% % However, we still think that this is a valuable choice, as
% % directly calculating this accuracy change requires the underlying system to obtain the ground truth first (previous work define the ground truth as the inference results generated under the most expensive configuration to avoid the need for human annotation~\cite{dds,awstream,chameleon,vstore,videostorm,ekya,focus}).
% % This imposes non-trivial overhead due to extra inference on the most expensive configuration (\eg in Chameleon~\cite{chameleon}, calculating the ground truth\footnote{Chameleon is actually calculating multiple
% % resource-consuming configurations as the ``ground truth'', but the overhead is
% % still due to calculating ground truth.} consumes $\sim$50\% of the overall GPU
% % compute). 



% With the \outputgrad, the adaptation system can quickly adapt to the optimal configuration by assigning more resources to the knobs with high \outputgrad to improve the accuracy, or cut the resource usage of the knobs with low \outputgrad without hurting the accuracy.


% However, it can be expensive to calculate \outputgrad over a space of many knobs. %may incur high amount of extra inference.
% % This is because previous work needs to calculate \outputgrad in a knob-by-knob manner (\ie inference on the DNN and calculate the DNN output change by alternating the value of one knob while fixing other knobs, and repeat this process for all knobs). 
% Previous work~\cite{chameleon,vstore,videostorm,awstream} would have had to calculate \outputgrad in a knob-by-knob manner (\ie inference on the DNN and calculate the DNN output change by alternating the value of one knob while fixing other knobs, and repeat this process for all knobs). 
% % Thus, one more knob, one more extra inference.
% % Thus, more knobs will lead to more inference.


% To avoid such extra inference, \name leverages the \textit{differentiability} of the DNN to implement \outputgrad with constant GPU overhead and with no extra inference.
% % We show that \outputgrad, the first system that implements can be calculated without any extra inference and with constant GPU overhead.
% % We develop \name, a configuration adaptation system that optimizes the configuration based on \outputgrad.
% % The insight of \name is to leverage the \textit{differentiability} of DNN to reduce the cost of calculating \outputgrad.
% We {\em decouple} the calculation of \outputgrad (\ie how changing the knobs alters the DNN output) to how changing system knobs alters the DNN input and how changing the DNN input alters the DNN output.
% % Concretely, in order to calculate how changing the knobs alters the DNN output (\ie \outputgrad), we can calculate how changing system knobs alters the DNN input, and then calculate how changing the DNN input alters the DNN output.
% % \kt{Should we add a math formula of chain rule here? Like output/knob = output/input * input/knob?}
% The former can be calculated in a knob-by-knob manner without DNN inference (\ie no GPU compute), and the latter can be obtained via {\em backpropagation} (which is a constant GPU overhead without extra inference as it can reuse the existing computation graph of DNN inference).

% % We show that \outputgrad can be calculated with constant GPU overhead and without any extra inference, regardless of the number of the knobs, and develop \name, a configuration adaptation system, that optimizes the knobs based on \outputgrad.
% % \name reduces the cost of extra inference by treating \outputgrad as an actual gradient and leveraging the following two properties to decouple this gradient through the chain rule.
% % % \kt{I feel like this is the place to introduce the separation of the knob side v.s. the DNN side, as this separation is used (and only used) to reduce the cost of calculating the gradient}
% % \begin{packeditemize}
% %     \item 
% %     On the DNN side, the DNN output is differentiable to its input (via backpropagation algorithm).
% %     Thus, calculating how changing the DNN input alters the DNN output requires no extra inference.
% %     \item
% %     On the knob side, a wide range, \textit{not all}, of the knobs treat DNN as a \textit{black box} and affect DNN inference results solely by changing the DNN input.
% %     As a result, calculating how changing each individual knob alters DNN input requires no extra inference.
% % \end{packeditemize}
% % These two properties suggest that to calculate how changing the knobs alters the DNN output (\ie \outputgrad), we can first calculate how changing system knobs alters the DNN input, and then study how changing the DNN input alters the DNN output. 
% % \kt{Should we add a math formula of chain rule here? Like output/knob = output/input * input/knob?}
% % The former can be calculated in a knob-by-knob manner without the participant of the DNN (thus avoid extra DNN inference), and obtaining the latter only requires one backpropagation (this creates a constant GPU overhead, but it is reusing the computation graph created by existing DNN inference, thus incurring no extra inference).


% Operators can use \name to tune a wide range of applications and knobs that influences DNN input (as shown in Table~\ref{tab:rich-set-of-knobs}).
% That said, \name does {\em not} apply to all knobs and applications.
% In terms of knobs, \name does {\em not} apply to knobs that alter the DNN itself, 
% such as retraining the DNN weights~\cite{ekya,noscope,mcdnn}.
% Similar to \name, they also adapt to changes in input distribution, they involve substantial computation and thus tend to happen at a coarser timescale than the knobs considered in \name. 
% In terms of applications, \name does {\em not} apply to those applications that \fillme.
% % such as customizing the DNN according to the current content of the input~\cite{ekya,noscope,mcdnn}.
% % In some sense, both the DNN customization approach and \name are adapting to the varying content in the input data stream.
% % However, in order to maintain high accuracy, DNN customization approach needs to retrain the DNN when the input content varies, and thus incurs high GPU overhead, while \name adapts the knobs inside the underlying system that serves the DNN, which is much more lightweight.


% In short, the contributions of this paper are two-fold:
% \begin{packeditemize}
%     \item A new abstraction, \outputgrad, that enables quick adaptation of configurations for DNN-based analytics.
%     % \item A new abstraction, \outputgrad, that enables the configuration adaptation framework for DNN-based analytic systems to quickly adapt to optimal configuration through \accgrad.
%     \item A configuration adaptation system, \name, that implements \outputgrad with constant GPU overhead and without extra inference.
%     % \item An implementation, \name, that implements \outputgrad with constant GPU overhead and with no extra inference.

% \end{packeditemize}

% We evaluate \name across 7 different DNN-based analytic pipelines and across 54 videos. \name achieves similar accuracy with 10-43\% end-to-end delay reduction, or achieves 1-10\% higher accuracy with similar end-to-end delay compared to the baselines on 8 different applications.
% Also, we show that the performance gain of \name compared to the baselines becomes larger when there are more knobs or the knobs become more fine-grained.

% \textbf{This work does not raise any ethical issues.}







% % Expose abstraction:
% % confidence change gradient with respect to resource


% % Confidence scores -> a generalizable format
% % Confidence thresholds -> a widely adopted component in the accuracy of applications in real world.

% % % The key to achieve this goal is to calculate how much each knob changes the confidence scores that are close to the confidence thresholds 

% % To quickly adapt to optimal configuration without extra inference, the intuition of \name is to allocate more resource to the knobs that maximally change the confidence scores inside the inference results that are around  with confidence scores \textit{around} the confidence thresholds.
% % to maximally change \textit{which} inference results participants the accuracy
% % Concretely, \name calculates 


% % Why this works: two assumptions on the knobs 1. more resource, higher accuracy and 2. if the confidence scores around the confidence thresholds doesn't change, the accuracy barely change.

% % We present \name that efficiently calculates such metric on each knob.
% % The key for \name to success is to leverage the differentiability of DNN to \textit{predict} the performance of a run-time system.

% % our approach is to: grant more resources to the knobs can maximally change the part of the inference results that the confidence scores are around the confidence thresholds, and cut the resource usage of those knobs that barely change 


% % To quickly calculate this metric, we leverage the differentiability of the DNN to quickly obtain how DNN input affects the confidence scores around the confidence thresholds.



% % We present our system: \name, which meets these two requirements. 
% % To quickly adapt to optimal configuration, \name calculates the \textit{gradient} of accuracy with respect to each knob (hereinafter \accgrad, defined as the accuracy change if changing one knob valued by a little).
% % % leverages a property of DNN-based analytic system knobs: for most of the knobs, if changing the value of one knob results in spending more (or less) resource, the corresponding inference result would statistically become more (or less) accurate.
% % % This property suggests that each knob is able to \textit{trade resource for accuracy}.
% % % To quantitatively measure this ability, \name calculates the \textit{gradient} of accuracy with respect to each knob (hereinafter \accgrad, defined as how changing each individual knob by a little alters the accuracy).
% % With \accgrad, \name can quickly adapt to the optimal configuration in a
% % large configuration space by allocating more resources to those knobs with
% % high \accgrad to improve accuracy and cutting the resource usage of knobs with
% % \accgrad to save resource without hurting accuracy.





% % % insight that motivates \name is two properties we observe in deep learning
% % % system knobs. The first property is: for most of the knobs, if changing the
% % % value of one knob results in spending more (or less) resource, the corresponding
% % % inference result would statistically become more (or less) accurate. This
% % % property suggests that the change of accuracy with respect to knob value change
% % % % can reflect the ability of trading resource for accuracy for each individual
% % % knob. With \accchange, \name can quickly adapt to the optimal configuration in a
% % % large configuration space: \name can allocate more resources to those knobs with
% % % high \accchange to improve accuracy and cut the resource usage of knobs with
% % % \accchange to save resource without hurting accuracy.



% % % There is one more challenge to calculate \accgrad.


% % The first challenge of calculating \accgrad is: how to calculate the accuracy change when changing a knob value by a little?
% % Directly calculating this accuracy change requires the underlying system to obtain the ground truth first (previous work define the ground truth as the inference results generated under the most expensive configuration to avoid the need for human annotation~\cite{dds,awstream,chameleon,vstore,videostorm,ekya,focus}).
% % This imposes non-trivial overhead due to extra inference on the most expensive configuration (\eg in Chameleon~\cite{chameleon}, calculating the ground truth\footnote{Chameleon is actually calculating multiple
% % resource-consuming configurations as the ``ground truth'', but the overhead is
% % still due to calculating ground truth.} consumes $\sim$50\% of the overall GPU
% % compute). 
% % To resolve this issue, we develop a proxy for accuracy difference (we call this proxy \accproxy). 
% % % The main idea is to reuse the existing inference results and measure the accuracy change if the same input
% % % data \textit{were} processed by a new configuration. 
% % Concretely, \accproxy estimates the sign and the magnitude of accuracy change by the following rule:
% % \begin{packeditemize}
% % \item 
% % The \textit{sign} of accuracy change is determined by which input (between the two DNN input generated before and after changing one knob value) is of \textit{less distortion} compared to the DNN input generated under most expensive configuration.
% % \item 
% % We estimate the \textit{magnitude} of accuracy change through checking the \textit{dissimilarity} between the two inference results generated before and after the knob value change.
% % The intuition behind this estimation is that: if the inference results generated before and after the knob change are highly similar, the inference accuracy of these two inference results should also be highly similar.
% % \end{packeditemize}
% % By using this proxy, calculating accuracy difference no longer relies on the generation of ground truth, and 


% % However, even with the optimization above, trivially calculating \accgrad in a knob-by-knob manner (\ie
% % calculate the accuracy change by alternating the value of one knob value
% % while the value of other knobs value remaining unchanged, and repeat this process
% % for all knobs) still requires extra inference to get the inference results after each knob value change. 
% % To avoid such extra inference, \name leverages the following two properties:
% % \begin{packeditemize}
% %     \item
% %     On the knobs side, most of the knobs treat DNN as a \textit{black box} and affect DNN inference results solely by changing the DNN input.
% %     As a result, calculating how changing each individual knob alters DNN input requires no extra inference.
% %     \item 
% %     On the DNN side, the DNN itself is differentiable to its input (via backpropagation algorithm).
% %     Thus, calculating how changing the DNN input alters the accuracy requires no extra inference.
% % \end{packeditemize}
% % These two properties suggest that to calculate how changing the system knobs alters the accuracy (\ie~\accgrad), we can first calculate how changing system knobs alters the DNN input, and then study how changing the DNN input alters the accuracy. 
% % The former can be calculated in a knob-by-knob manner without the participant of the DNN (thus avoid extra DNN inference) and the latter only requires one backpropagation (thus incurring no extra inference).

% % compared to the ground truth DNN input, and estimate the magnitude of accuracy
% % change by comparing the difference of inference results between the old and the
% % new configuration. 
% % We find that the \textit{gradient} of this accuracy metric can be calculated \textit{without} extra inference.

% % \begin{comment}

% %   Deep learning applications on streaming data (\eg video streams or LiDAR
% %   feeds) are everywhere. For example, in autonomous driving, people use video
% %   cameras and LiDAR sensors and leverage object detection deep neural networks
% %   (DNNs) to sense the surrounding environment and avoid potential collisions. In
% %   augmented reality, people use video cameras and LiDAR sensors to localize the
% %   remote objects and render the virtual objects on top of real objects. This
% %   trend inspires system research for these applications, like live
% %   analytics~\cite{??}, retrospective analytics~\cite{??}, database for analytic
% %   purpose~\cite{vstore,noscope}, etc.

% %   We identify two important characteristics of these systems. First, they
% %   contain large configuration spaces (\eg in AWStream~\cite{awstream}, there are
% %   216 different configurations inside its configuration space). Second, these
% %   configurations need to be \textit{timely} adapted according to their input
% %   (\eg we may want to use higher video resolution when a small car enters the
% %   video frame in order to detect this small car) and the current resource budget
% %   so that they can generate the inference results as accurate as possible.

% %   As a result, the key challenge for these systems is: how to navigate the large
% %   configuration space and pick the optimal configuration that generates the most
% %   accurate inference results under the current resource budget.

% %   The first way to address this problem is to \textit{frequently profile} the
% %   system with different configurations to obtain their resource usage and
% %   inference accuracy, and then pick the configuration that meets the resource
% %   budget and generates the most accurate inference
% %   results~\cite{awstream,chameleon,vstore}. However, in order to profile, this
% %   approach has to perform \textit{extra} inference on the GPU, resulting in high
% %   GPU cost.

% %   The other approach performs no extra inference and instead, picks the
% %   configuration based on the recent configuration and its corresponding DNN
% %   output. However, there can be many configurations that meet the resource
% %   budget. Without profiling most of them, it is difficult to separate the
% %   configurations that yield similar DNN output from those that yield more
% %   accurate DNN output. In addition, the previous work in this approach designs
% %   hand-craft heuristics catered for different applications.

% %   Thus, the requirements of an ideal configuration adaptation system are
% %   three-fold:
% %   \begin{enumerate}
% %     \item No extra DNN inference
% %     \item Pruning out the configurations with similar accuracy
% %     \item Agnostic to the underlying applications
% %   \end{enumerate}

% %   We present our system: \name that meets these three requirements. The idea is
% %   to calculate the \textit{gradient} of inference accuracy with respect to the
% %   configurations to \textit{predict} which of them improve inference accuracy
% %   and which do not. The key insight that enables us to calculate this gradient
% %   is by decoupling this gradient into two terms. The first term is the gradient
% %   of inference accuracy with respect to the DNN input, which can be calculated
% %   by backpropagation without performing extra inference on any other
% %   configuration. The second term is the gradient of the DNN input with respect
% %   to the configurations, which does not require DNN inference.

% %   To make our system practical, we also identify another source of overhead
% %   introduced by calculating inference accuracy. In order to calculate inference
% %   accuracy, previous work needs to refer to the configuration with \textit{the
% %   most} resource usage and use the corresponding inference results as the
% %   ``ground truth'' to evaluate the accuracy of inference results generated from
% %   other configurations. Calculating the ``ground truth'' uses much higher
% %   resource usage (including the streaming cost of streaming the data and the GPU
% %   cost to generate inference results) than the current optimal configuration. To
% %   reduce this cost, we introduce a \textit{proxy} of accuracy that
% %   \textit{indirectly optimizes} accuracy by using the DNN input (instead of the
% %   DNN output), thus requiring no DNN inference.

% %   To conclude, the contributions of this paper are:
% %   \begin{enumerate}
% %     \item A way to calculate gradient with no extra inference
% %     \item An accuracy proxy that indirectly optimizes the accuracy without
% %           running extra inference.
% %   \end{enumerate}
% %   We quantitatively evaluate these two contributions, we perform experiments on
% %   XXX datasets, XXX applications and XXX

% % \end{comment}
% % 

==> intro_v6.tex <==

\tightsection{Introduction}
\label{sec:intro}

% \kt{Claim we generalize to other data sources}

% \kt{How timely identify a differentc onfiguration is better}

% % \kt{align the example here with the example that optimal config frequently changes}
% % \kt{add streaming aspect}
% Many applications rely on DNNs to perform accurate inference on various data streams (\eg video streams, audio streams and LiDAR feeds).
% For example, people collect data streams from various sensors (\eg infrared cameras, LiDAR sensors, and radar sensors)  and analyze them through DNNs to detect vehicles and pedestrains\cite{trafficvision, traffictechnologytoday, goodvision,intuvisiontech, vision-zero, msr,tusimple,waymo-blog,motional}.
% % people use DNNs to analyze traffic videos to monitor vehicle speed and spot traffic jams~ and to analyze data streams from other sensors (\eg infrared cameras, LiDAR sensors, and radar sensors) to detect vehicles and pedestrians for autonomous driving~.\jc{the text until here can be a bit tightened}
% % As the computation power on these sensors are restricted, they need to stream their data through networks to remote server for DNN-baesd inference~\cite{?,?}.
% % \kt{mention that data needs to be streamed to the server.}
% As these DNN-based applications require high accuracy, they use a great amount of bandwidth and/or GPU computation resources.
% % \jc{too vague. spill out GPU cycles and bandwidth.}
% Thus, practical systems for these applications may not have enough bandwidth to stream all uncompressed data from the sensor to the DNN (if the streaming is needed for analytics), and/or enough GPU compute resource to run DNN inference on all input data (\eg all frames of a video stream).
% % As a result, many prior efforts leverage the content of the input data to save resources without hurting the accuracy.
% As a result, many prior efforts save resources by identifying the content of the input data that can be analyzed with fewer resources without hurting accuracy.
% For instance, consider vehicle detection in a traffic monitoring video stream.
% When the red light appears, the speed of vehicles is slow, allowing the analytic system to reduce the frame sampling rate (thus minimizes the number of frames being analyzed) and still accurately determining the position and the movement of the vehicles.
% % \jc{too vague. why content can be leveraged to save resource? should be quite intuitive, so just a couple of short examples are enough. no need for long examples. }
% % For example, in dashcam video streams, the number and the moving speed of vehicles are constantly changing over 
% % time (\eg the number of vehicles will be much larger during daytime than during night), 
% % location (\eg cars move faster on the highway) and traffic conditions (\eg the number of vehicles significantly increases in traffic congestion).
% Technically, recent proposals~\cite{vigil,glimpse,mcdnn,videostorm,noscope,neurosurgeon,awstream,chameleon,focus,adascale,filterforward,vstore,cracking,dds,reducto,blazeit,yoda,vcm,elf,ekya} expose internal tunable parameters (referred to as \textit{configuration knobs}, see Table \ref{tab:rich-set-of-knobs} for a full list of configuration knobs) and timely \textit{configure} these knobs (we denote the knobs together with their configured values as a \textit{configuration}) according to the content of the input data, in a way that saves resources (in GPU compute and network) while maintaining high inference accuracy.
% \jc{not clear how and why knobs help leverage content to tune knobs.}
% \kt{I emphasized that prior work leverages the content of the input data to save resource, and gave an example. Hope that this is clearer}


% \kt{add configuration}

Many applications rely on deep neural nets (DNNs) for accurate inference on various types of input data~\cite{trafficvision, traffictechnologytoday, goodvision,intuvisiontech, vision-zero, msr,tusimple,waymo-blog,motional}.
For example, a DNN can analyze video frames to
detect vehicles and pedestrians, or analyze an audio stream to extract text. 
These applications often run DNN inference on cloud/edge servers, causing resource contention in both {\bf network bandwidth} to stream high-fidelity data (\eg high-quality video) from distributed sensors to the analytics servers and in {\bf GPU compute cycles} to run expensive DNN inference on many data points (\eg each video frame).


% why setting knobs is key
% To mitigate resource contention, many prior efforts expose internal tunable parameters (hereinafter \textit{knobs}) and timely configure these knobs (we denote the knobs together with their configured values as a \textit{configuration}).
% They show that an optimal configuration of these knobs can significantly reduce resource usage in both network bandwidth and GPU without affecting inference accuracy.
% Multiple knobs are often tuned together to save more resources (see Table~\ref{tab:rich-set-of-knobs} for a list of knobs considered).
% % uses the {\em optimal setting} of these knobs, 
% % high inference accuracy could be obtained while significantly reducing resource usage in both network bandwidth and GPU compute.
% The challenge, however, is that the optimal setting of these knobs {\em varies} with temporal changes in the source data and thus must be adapted timely. 
% For instance, a DNN can accurately detect vehicles at only one frame per second (fps) in a traffic video, if the vehicles stop at the red light or move slowly, but when the light turns green, the DNN must analyze frames much more frequently (\eg 30fps) to detect fast-moving vehicles. 
% In this case, the knob---frame rate of feeding data to the DNN---must adapt dynamically depending on the changes in the video content.


% why setting knobs is key
% Many prior efforts expose internal tunable parameters (hereinafter \textit{knobs}) and timely configure these knobs (we denote the knobs together with their configured values as a \textit{configuration}).
Many previous efforts have shown that {\em optimally tuning a range of knobs} (\eg video frame rate and resolution) can greatly save resource usage and achieve high accuracy.
Table~\ref{tab:rich-set-of-knobs} shows a list of example knobs.
We use a {\em configuration} to refer to a particular setting of the knobs used by an application (\eg a particular frame rate and resolution).
% To mitigate resource contention, many prior efforts expose internal tunable parameters (hereinafter \textit{knobs}) and timely configure these knobs (we denote the knobs together with their configured values as a \textit{configuration}).
% have proposed to tune various knobs of these DNN-based analytics systems. 
% expose internal tunable parameters (referred to as knobs) and
% timely configure these knobs (we denote the knobs together
% with their configured values as a configuration)
% (\S\ref{sec:related}).
% ~\cite{vigil,glimpse,mcdnn,videostorm,noscope,neurosurgeon,awstream,chameleon,focus,adascale,filterforward,vstore,cracking,dds,reducto,blazeit,yoda,vcm,elf,ekya}.
% They show that an optimal configuration of these knobs can significantly reduce resource usage in both network bandwidth and GPU 
% % {\em if} one always sets these knobs {\em optimally}, resource usage in both network bandwidth and GPU compute can be significantly reduced 
% without affecting inference accuracy.
% Multiple knobs are often tuned together to save more resources (see Table~\ref{tab:rich-set-of-knobs} for a list of knobs considered).
% uses the {\em optimal setting} of these knobs, 
% high inference accuracy could be obtained while significantly reducing resource usage in both network bandwidth and GPU compute.
The challenge is that the optimal configuration {\em varies} over time with the input data, so it must be {\em adapted timely}. 
For instance, when the vehicles stop at the red light or move slowly, feeding the traffic video feed at a low frame rate to a DNN can still accurately detect vehicles,
% at only one frame per second (fps) in a traffic video, 
but when the light turns green, the DNN must analyze frames much more frequently (\eg 30fps) to detect fast-moving vehicles. 
In this case, the configuration of frame rate
% of feeding data to the DNN---
must be dynamically adapted depending on the video content.

% Multiple knobs are often tuned together to save more resources (see Table~\ref{tab:rich-set-of-knobs} for a list of knobs considered), 
% % With more knobs to tune (see Table~\ref{tab:rich-set-of-knobs} for a list of knobs considered), more resources {\em could} be saved 
% but it is more challenging to adapt in
% % It becomes more challenging to tune more knobs (see Table~\ref{tab:rich-set-of-knobs} for a list of knobs considered) at the same time, which leads to 
% a multi-dimensional space of {\em configurations} (each being a combination of knobs).

% The {\em optimal settings} of these configuration knobs should achieve the highest inference accuracy but use bandwidth and GPU resources within a given budget. 


% \kt{I slightly changed the logic here. The goal is to implicitly explain that the adaptation frequency can be larger than the rate of optimal configuration changes}
% However, the optimal setting of these configuration knobs varies with changes in the input data stream, and thus must be adapted frequently to avoid sticking to an outdated configuration (this aligns with the observation of prior work). 
% In the vehicle-detection example, when the red light appears, the vehicles move slowly and the DNNs can accurately detect vehicles using 1fps.
% However, under green light, the vehicles move much faster and the video needs to be analyzed much more frequently (\eg 30fps) to accurately detect fast-moving vehicles.



% Technically, recent proposals~\cite{vigil,glimpse,mcdnn,videostorm,noscope,neurosurgeon,awstream,chameleon,focus,adascale,filterforward,vstore,cracking,dds,reducto,blazeit,yoda,vcm,elf,ekya} expose internal tunable parameters (referred to as \textit{configuration knobs}, see Table \ref{tab:rich-set-of-knobs} for a full list of configuration knobs) and timely \textit{configure} these knobs (we denote the knobs together with their configured values as a \textit{configuration}) to the \textit{optimal configuration} (\ie a configuration that achieves highest accuracy under the bandwidth and GPU computation budget).
% \kt{I changed `` the content of input data'' to `` the input data''.}
% \jc{not clear how and why knobs help leverage content to tune knobs.}
% \kt{I emphasized that prior work leverages the content of the input data to save resource, and gave an example. Hope that this is clearer}




% % DNN-based analytics are popular. 
% % The data needs to be streamed from the sensor to the server.
% % DNN-based analytics are resource-demanding (in terms of bandwidth and/or GPU compute). Goal: reduce resource usage while achieving high accuracy.
% % Many prior works in this space achieve this goal by exposing internal tunable parameters (we refer to as \textit{knobs}) and frequently adapting their configurations to achieve high accuracy within the resource budget (give an example configs and a forward pointer to the full list).  
% % Facing this trend, people develop adaptive analytic systems to handle various kind of videos and maximally reduce the resource usage while maintaining high accuracy.
% % \item However, these adaptive systems may sometimes use high amount of resource but still yield low analytic accuracy when the video content is challenging.

% % Prior work observes that the optimal config (the config with the highest accuracy under the budget) frequently changes. \\
% % Example: no object of interest --> low frame rate is 100\% accurate. A new object comes into the video --> low frame rate may only achieve an accuracy of 50\% as it cannot capture the movement of the object. 
% \kt{Do we need to bring up the point where the optimal configuration may not change when the input data does not vary? I feel like this point is a noise but people may question this.}
% Prior work~\cite{awstream,chameleon,dds,eaar}) observes that the optimal configuration frequently varies as the input data constantly changes over time.
% % As the optimal configuration depends on the content of the input data (the configuration with the highest accuracy under a certain resource budget), prior work observes that the optimal configuration  can change frequently~\cite{??}.
% \jc{this claim again comes out of the blue. again, it would have been more natural to first connect the setting of knobs with content, and then say because the content changes over time, the best knob settings must change too} 
% \kt{Done.}
% For example, when there are no objects of interest in a video, analyzing the video with a low frame rate is 100\% accurate. However, when a new object enters the video, a low frame rate may only achieve an accuracy of 50\% as it cannot capture the movement of the object.
% As a result, a frequent adaptation of the configuration (ideally once per \fillme seconds) is necessary to minimize the amount of time spent using an outdated configuration.
% \jc{the term "frequently" is a bit vague. can we give some concrete numbers how "frequently" configs should be adapted? also give a forward pointer 2.2 that has some empirical measurements?}


% \item
% As a result, the research question is: how to quickly adapt to the optimal config (given that optimal config frequently changes)? 
% \jc{this sentence is not wrong but misses the key point. the point is not "how to adapt", but what information you need to adapt. in this sense, the key is ability to estimate which configuration has the highest accuracy given some resource constraint? 
% you can later say to answer this question, you don't need to know the accuracy of all configs; instead, we only need the gradient}


% \kt{Define how people do it today.}
The key question, therefore, is as input data evolves over time, 
{\em how to quickly check if the current configuration should be changed.} In other words, whether a different configuration can yield much higher accuracy or lower resource usage without hurting accuracy. 

% better adapt configurations of DNN analytics systems is 
% As a result, the key research question of these configuration adaptation systems
% % \jc{let's call them "configuration adaptation systems"? anyway, we should stick to the same term whenever we refer to such systems}
% is: 
% \textit{how to timely identify if a different configuration is better---higher accuracy under a given resource budget, or much less resource usage while maintaining similar accuracy or both---than the current configuration.}
% identify the \textit{optimal} configuration?
% (the configuration with the highest accuracy under the resource budget)\jc{optimal config should've been defined much earlier, not here} 
% and quickly adapt to the optimal configuration\jc{once the optimal config is identified, isn't "quickly adapting to it" trivial? either drop it or rephrase}?


% \item Such event is runtime-specific.
% To recover from the accuracy drop after such sudden change, one need to quickly adapt to the optimal.
% We observe that the change of optimal configuration (\ie the configuration that generates highest accuracy within resource budget) can change abruptly and unpredictably.
% \kt{A concrete example here.}
%     For example, when there is no object of interest in the video, one can encode the video using low frame rate to save resource.
%     However, when a moving object appears in the video, the video needs to be encoded using high frame rate in order to accurately capture the motion of this object.
%     And when this moving object leaves, there is no object of interest in the video and the video can again be encoded using a low frame rate.
    % In order to capture the frequent change of optimal config, one needs to adapt the configuration with a frequency faster than once every 3 seconds (a measurement to support this point: 20\% accuracy gain if adapting once every 3 seconds compared to adapting once every 15 seconds).
    % \jc{this is weak. it only says once every 3 seconds is better than once every 15. maybe you should ALSO say once every 3 seconds is almost the same as once every second?}
    % The design question is: how to frequently and optimally adapt the configuration to achieve high accuracy with a given resource budget?


    % Is there exist another config, that has much higher accuracy than the current config and still within resource budget?


    % \kt{Goal: check  if there is a config with higher accuracy under the resource budget and adapt to it}
    % \begin{packeditemize}

    \mypara{Prior approaches}
    To answer this question, two general approaches exist, but they fall short for different reasons (\S\ref{subsec:configuration-adaptation}).
    
    First, {\em profiling-based} methods (\eg~\cite{awstream,chameleon,videostorm,vstore}) periodically run {\em extra} DNN inferences to profile the accuracy of alternative configurations and then use these profiles to identify the optimal configuration. 
    % runs inference with many configurations to {\em profile} which configuration has the highest accuracy with minimum resource usage~\cite{awstream,chameleon,videostorm,vstore}. 
    However, the extra DNN inferences incur significant GPU overhead.
    % to run significantly more extra DNN inference on the same input data. 
    % Moreover, it often uses extra bandwidth to stream input data at a much higher quality to test their inference accuracy.
    For example, AWStream~\cite{awstream}'s profiling step test 
    % runs DNN inferences with 
    different combinations of resolutions, frame rates, and quantization parameters, which causes up-to 17$\times$ more GPU cycles than normal inference.
    % , causing 17$\times$ extra GPU overhead. % than regular DNN inference.
    With limited compute resource, the profiling overhead will slow down configuration adaptation and cause the configuration to be outdated when input data changes over time. 
    % they are unable to profile configurations frequently,
    % % Thus, it is difficult to profile configurations frequently, 
    % leading to the use of outdated configurations when the optimal configuration changes.
    % knobs (resolution, frame rate, and quantization parameter) on a \textit{10-second} video consumes the same amount of GPU computation as analyzing more than an \textit{8-minute} video.
    
    % The first~\cite{awstream,chameleon,videostorm,vstore} periodically performs extra DNN inference to profile the accuracy and resource usage of all configurations and picks the configuration that has the highest accuracy within the resource budget.
    % However, each profiling needs to perform multiple extra DNN inferences, resulting in high GPU computation overhead.
    % For example, in AWStream~\cite{awstream}, running full profiling on just 3 knobs (resolution, frame rate, and quantization parameter) on a \textit{10-second} video consumes the same amount of GPU computation as analyzing more than an \textit{8-minute} video.
    % As a result, when the GPU compute and/or the network bandwidth is restricted, this approach needs to either profile less frequently, leading to the use of outdated configurations when the optimal configuration changes, or significantly prune the search space (which may contain only suboptimal configurations).
    % --> need extra streaming and inference --> when the bandwidth and/or GPU resource is limited, either identify the optimal config slowly or downsample the config space and may miss the optimal config

    % \kt{ask Ganesh why we should add this work}
    % The second approach performs no extra inference and adapts the configuration based on recent DNN outputs (including intermediate DNN outputs). 
    % Though no extra inference is run, this approach also tends to adapt slowly, as each DNN output reveals limited information regarding the highly complex relationship between the configurations and DNN inference output/accuracy, due to the complexity of the DNN itself and the preprocessing modules before the DNN (e.g., video codecs). We take EAAR, a system for video object detection, as an example. 
    % EAAR adjusts the video encoding quality by collecting the regions from the DNN that may contain objects of interest and encoding these regions in higher encoding quality on future video frames. Thus, the objects inside these regions are much more likely to be detected.
    % However, as the regions generated by the DNN may not be exactly aligned with the region that actually contains the objects, the object detection DNN may fail to detect some objects and thus EAAR needs to further adjust the corresponding regions.

    % \kt{also mention the other line of work that adapts based on DNN output}
    % To improve the adaptation speed, 
    % \kt{I prefer n those works that adapt based on DNN output as the rationale below also applies to them.}

    Second, {\em heuristic-based} methods~\cite{dds,reducto,vigil,glimpse,eaar,accmpeg,casva,elf} avoid extra inference and pick the configuration using {\em cheap} heuristics.
    % by running simple heuristics on data streams 
    % analyzing the data streams through cheap heuristics 
    % \eg calculating frame differences~\cite{reducto} or region-of-interest proposed by DNNs on recent input~\cite{dds}.
    % (\eg calculating frame differences~\cite{glimpse,reducto} or region-of-interest proposed by DNNs~\cite{dds,eaar,elf} on recent input).
    % ) or using past DNN inference results (\eg region-of-interest proposed by DNNs~\cite{dds,eaar,elf} on recent input).
    % from DNN intermediate results~\cite{dds,eaar,elf}).
    Though they may adapt faster
    % (\eg once every second) 
    than profiling-based methods, but the cheap heuristics may sometimes pick suboptimal configurations that have low accuracy.
    % pick the configuration with accuracy much lower than the optimal one (see \S\fillme for more rationales).
    For instance, a typical heuristic selects a new frame to feed to DNN
    % calculates frame difference
    % \footnote{Reducto calculates frame differences based on various frame feature extractors in computer vision literature.} 
    % and sent out 
    % a video frame to the server for DNN analysis 
    when its pixels differ significantly from the last analyzed frame (\eg~\cite{reducto}).
    % the frame significantly differs from the last analyzed frame.
    % to determine whether the current video frame needs to be sent out to the server for analytics.
    % If the frame difference between the current frame and the previously-sent frame is larger than a threshold, Reducto will send out the current frame.
    However, a high pixel-level difference may fail to indicate frames with new objects of interest, when the video background moves quickly (\eg dashcam video from a moving vehicle) which causes great pixel changes.
    % , frame difference is caused mostly by background pixels and thus becomes a poor indicator for the arrival or movement of objects of interest.
    As a result, it might run the DNN on too many frames while the objects of interest remain the same.
    % , which uses more network bandwidth and GPU cycles than necessary, or analyze too few frames and miss real objects of interest.
    % \jc{kuntai, check if this is correct}
    % of whether there is an object of interest or not.
    % large regardless of whether there is an object of interest or not.
    % As a result, Reducto may send out frames when no object of interest appears, thus having insufficient resources to frequently send out frames when the object of interest appears, resulting in low accuracy.
    % \item To improve the adaptation speed, the other line of work performs no extra DNN inference and instead pick the config through cheap heuristics.
    % These heuristics can adapt quickly\jc{"adapt quickly" sounds vague. do you mean adapt config every frame or second?}. 
    % \kt{guess  the accuracy}

    % \jc{Is DDS a good example of knob-specific design as well?}
    % \kt{yes it is, my plan is to focus on Reducto in intro and introduce server-driven works in motivation section.}
    Moreover, many existing techniques are designed only for {\em specific} data types or knobs.
    % , and it is unclear how effective they will be on other types of data (\eg LiDAR point cloud, depth map, or audio waves).
    % Even in video analytics, the proposed heuristics often work well only for {\em specific knobs}.
    % and do not generalize to other types of knobs.
    For example, Reducto~\cite{reducto} selects which frames to run DNN inference based on inter-frame difference, but the inter-frame difference is ill-suited to tuning the encoding quality parameters of a video frame, which depends on the content {\em within} a frame, rather than how it differs from other frames. 
    % See \S\ref{subsec:configuration-adaptation} for more examples.
    Likewise, DDS~\cite{dds} tunes the region-of-interest quality parameter within each frame, but its logic may not naturally extend to tuning  knobs of non-video input data, such as LiDAR point cloud, depth map, or audio waves.
    % each fine-grained spatial block to improve inference accuracy on each frame, 
    % but it is not aware whether the current frame is redundant given past inference results.
    

    % \jc{mostly in video. generalize to other data types}
    % \jc{kuntai, check if this is correct}
    
    
    % is not effective when tuning the resolution of each video frame.
    % This is because whether the current frame should be encoded in high resolution or not depends on the current frame itself (\eg the current frame should be encoded in high resolution when there are multiple small objects) rather than the frame difference between the current frame and previously-sent frame.


    % Moreover, these works tailor for specific types of knobs and do not generalize to other type of knobs.
    % \jc{Is DDS a good example of knob-specific design as well?}
    % \kt{yes it is, my plan is to focus on Reducto in intro and introduce server-driven works in motivation section.}
    % % For example, Reducto filters the video frames on the camera to save server-side GPU compute cost without hurting the accuracy.
    % % Concretely, Reducto measures the similarity between the current frame and the previously-sent frame using metrics in computer vision literature and discards the current frame if it is highly similar to the previously-sent frame.
    % For example, Reducto may not be useful in terms of tuning the resolution of each video frame.
    % This is because whether the current frame should be encoded in high resolution or not depends on the current frame itself (\eg the current frame should be encoded in high resolution when there are multiple small objects inside) and does not depend on the frame difference between the current frame and previously-sent frame.
    % \kt{read classic papers, daily read intro}
    % \kt{Para1: tell people why DNN can calculate ''how much changing a bit knob can affect accuracy'', because we can split the change to}    
    % \kt{2 high-level key ideas, give it a try}
    % \kt{Para2: why having this is better than previous work}
    

    % We propose an alternative approach to handle uncertain QoE degradation.
    % Goal: let people know why we are better.


    % 造潜艇：
    % 方法1：我能造一个小型的核反应堆，
    % connect from what's new to why you are better
    % new: gradient decoupling + gradient descent.
    In short, prior work falls short on at least one of the three fronts: 
    (1) frequent adaptation, (2) choice of near-optimal configuration, and (3) not tied to specific configuration knobs.
    % (1) adapt frequently, (2) reach a near-optimal configuration, and (3) apply to a range of configuration knobs.

    % \jc{
    % \begin{itemize}
    %     \item we focus on \outputgrad. 
    %     \item we can compute \outputgrad efficiently
    %     \item based on \outputgrad ==> gradient ascent
    %     \item why it's better than profiling (faster) and heuristics (dnn output -> accuracy)
    %     \item caveats of gradient ascent
    % \end{itemize}}

% \jc{we should be introducing our system here. i tried an alternative flow in intro\_v6.tex that introduces the high-level idea first, and then how to estimate \outputgrad efficiently.}

% \jc{here's an alternative draft for the following paragraphs}

\myparashort{\name: Fast adaptation based on \outputgrad.}
This paper presents \name, a new approach to configuration adaptation that improves on all three fronts.
The key of \name is a new method to quickly estimate {\em gradient of the DNN inference accuracy with respect to each knob at current configuration}.
We refer to this gradient as the \outputgrad of each knob.
\outputgrad effectively shows how much can a small change in the configuration of each knob change DNN accuracy.
{\em If} \outputgrad can be estimated frequently, say every second, \name can adopt a {\em gradient ascent} strategy that uses the up-to-date \outputgrad to change the configuration of each knob in a way that maximally increases accuracy or reduces resource usage without hurting accuracy.
Our gradient-ascent strategy outperforms previous work for the following reasons:

\begin{packeditemize}
\item Compared to profiling-based methods, \name can update the \outputgrad's estimate and use it to adapt {\em more frequently} than waiting until the slow profiling finishes (\eg every minute~\cite{awstream}). 
% \name updates the \outputgrad's estimates every second, and so it does with the configuration.
More importantly, \outputgrad indicates that given the input data content, which knob's configuration should be changed to maximally increase accuracy or reduce resource usage without affecting accuracy. 
% This allows \name to adapt to changes in input data earlier than profiling-based methods which must wait until the next profiling (\eg every minute~\cite{awstream}). 

\item Compared to heuristics-based methods, \name's gradient-ascent can converge to a {\em closer-to-optimal} configuration.
Most heuristics used in prior work adapt configuration by analyzing only the input data, rather than how the data might affect the final DNN's output.
By contrast, we formally prove that under reasonable assumptions, 
% \outputgrad statistically indicates how the accuracy of the final DNN changes with each knob and 
\name's gradient-ascent strategy almost always converges (\S\ref{subsec:limitation}). 
We have also validated these properties in a wide range of empirical evaluations (\S\ref{sec:eval}).

\end{packeditemize}

\begin{figure}
    \centering
    \includegraphics[width=0.6\columnwidth]{figs/contrast_different_approach.jpg}
    \tightcaption{
    Contrasting our approach with prior work. Our approach quickly adapts to a near-optimal configuration after the change of input content, while profiling-based methods adapt slowly and heuristics adapt to a configuration with much lower accuracy than the optimal one.
    }
    \label{fig:adaptation-behavior}
\end{figure}


\myparashort{Cheap estimation of \outputgrad}
The key technical nugget of \name is how to quickly estimate \outputgrad for all knobs. 
Our insight is that this can be achieved by leveraging DNN's {\em differentiability}, with no extra DNN inference.
Differentiability is an inherent property of almost all DNNs~\cite{paszke2017automatic} but has so far been only used in DNN training. 
If a knob only transforms the raw input data to DNN's input (\eg frame filtering, image downscaling, etc), then the \outputgrad of a knob can be decoupled into:
\begin{packedenumerate}
\item {\em \dnngrad:} How the DNN's output changes with respect to the DNN's input.
\item {\em \inputgrad:} How the DNN's input changes with respect to the knob's configuration.
\end{packedenumerate}
Both can be computed efficiently: 
\dnngrad can be efficiently computed by a single backpropagation operation on the DNN, and 
computing \inputgrad does not need GPU.
Moreover, if the system has multiple knobs, \dnngrad can be calculated once and re-used to derive the \outputgrad of different knobs.  
Intuitively, this is because \dnngrad describes DNN's sensitivity to a change in the DNN's input, which is agnostic to {\em which} knob causes the change in DNN's input.
% For instance, the \dnngrad of an object-detection DNN will be high for pixels associated with key visual features of an object.

We also formally prove that the multiplication of \dnngrad and \inputgrad is correlated with the true gradient of inference accuracy with respect to each knob (\S\ref{sec:proof}). 
This is intuitively true because a significant change in the inference results (\ie large \outputgrad) is often accompanied by a substantial change in accuracy. 



% \myparashort{\name: Fast adaptation based on \outputgrad}
% This paper presents \name, a configuration adaptation system that improves on all three fronts.
% The key of \name is to quickly estimate 
% {\em gradient of the inference results with respect to each knob}, which we refer to as \outputgrad.
% \outputgrad represents how a small change in the configuration of a knob can change the inference accuracy.
% We will explain how to quickly (\eg within a second) estimate \outputgrad shortly.
% With \outputgrad's estimate being frequently updated, \name then uses a {\em gradient ascent} strategy driven by \outputgrad to adapt configuration in a way that maximally increases accuracy or reduces resource usage without hurting accuracy.

% % The \outputgrad-based gradient ascent strategy allows \name to outperform prior works on these three fronts.
% % Compared to profiling-based work, 



% % Intuitively, once the estimate of \outputgrad can be frequently updated, \name can use a {\em gradient-ascent} strategy to adapt the configuration in the way that increases accuracy without using more resources.





% % \myparashort{\name: Fast adaptation based on \outputgrad}
% % This paper presents \name, a new approach configuration adaptation that improves on all three fronts.
% % The key step of \name is to calculate the {\em gradient of the inference results with respect to each configuration knob} (which we refer to as {\bf \outputgrad}) once every second.
% % \outputgrad shows how a small change in the configuration of each knob can change the inference accuracy.
% % Intuitively, once the estimate of \outputgrad can be frequently updated, \name can use a {\em gradient-ascent} strategy to adapt the configuration in the way that increases accuracy without using more resources.

% The \outputgrad-based gradient ascent allows \name to outperform previous work on all three requirements.


%    % % \jc{move figure 2 in intro?} \kt{done}
%    %  % \hl{
%    %  Figure~\ref{fig:adaptation-behavior} compares \name with previous approaches.
%    %  % }
%    %  Unlike profiling-based methods, \name uses much less compute to calculate \outputgrad than profiling, so it can adapt configuration much more frequently  and react more timely to the change of source data.
%    %  % \name could adapt right at the following second after the input content changes), 
%    %  % because it takes much less compute and network resources than profiling.
%    %  % the profiling-based baseline adapts slowly (once every minute~\cite{awstream}) may wait for at most a minute to react 
%    %  % \item
%    %  % Compared to heuristics that run no extra DNN inference,
%    %  Unlike simple heuristics, \name can adapt more optimally because \outputgrad captures how configuration affects the actual DNN output. The more DNN output changes, the more inference accuracy changes (\S\ref{subsec:limitation}). 
%    %  % \name can adapt to a near-optimal configuration where the works that perform no extra DNN inference may pick configuration with much lower accuracy.
%    %  % This is because \outputgrad can indicate the accuracy of different configurations.
%    %  % Intuitively, when a knob is of large \outputgrad, changing it can significantly impact the inference results.
%    %  % Thus, by allocating more resources to this knob (\eg by increasing its value), the improvement in inference accuracy is also likely to be substantial.
%    %  % \S\ref{??} shows more details on how we indicate the accuracy of other configurations and the correlation between our indicated accuracy and actual inference accuracy.
%    %  % As a result, if we assign this knob more resources (\eg by increasing its value),  the accuracy improvement also tends to be significant.
%    %  % Second, a large change in inference results could statistically indicate a large change in inference accuracy.
%    %  % Thus, \outputgrad could indicate how configuration should be changed to improve accuracy (see \S\ref{??} for empirical evidence)., where the accuracy of these works can be much lower than the optimal configuration.
%    %  % \item
%    %  Moreover, since DNNs are differentiable, \name could generalize a wide range of DNN-based analytic tasks (Table \ref{tab:pipeline} for a list of pipelines that \name can optimize).
%    %  That said, 
%    %  % The second limitation is that, though \name can be used to tune a wide range of configuration knobs, it 
%    %  \name as-is does not apply to those knobs that alter the DNN itself, such as retraining the DNN weights~\cite{ekya,mcdnn,noscope} (see \S\ref{subsec:limitation}). 
%    %  % Also, \name does not generalize to generative tasks like text generation and image generation.
%    %  % Similar to \name, they also adapt to changes in input distribution. 
%    %  % However, DNN retraining involves substantial computation and thus tends to adapt at a coarser timescale, while the knobs considered in \name require frequent adaptation.
    
% \mypara{Adapt frequently} Compared to profiling-based work, \name adapts much more frequently (as \name updates its configuration at \textit{every second} but profiling-based work updates its configuration once every minute~\cite{awstream}).
% Moreover, \name reacts to the change of the input content much earlier (as \name adapts to the change of input content right at that second but the profiling-based work needs to wait till the next profiling).
% We demonstrate the adaptation behavior of \name and profiling-based work in Figure~\ref{fig:adaptation-behavior}.

%  \mypara{Converge to a near-optimal configuration}
% Compared to the heuristics-based approaches that may have much lower accuracy than the optimal configuration, \name can adapt to a near-optimal configuration (as shown in Figure~\ref{fig:adaptation-behavior}) based on two main reasons (please refer to \S\ref{??} for the detailed version .

% First, the adaptation of \name improves accuracy as \outputgrad correlates with the gradient of accuracy.
% This is because a significant change in the inference results (\ie large \outputgrad) is often accompanied
% by a substantial change in accuracy. 
% To further demonstrate the correlation between \outputgrad and the gradient of accuracy, we prove that \outputgrad is the same as the gradient accuracy under a simplified accuracy function and some assumptions (see \S\ref{??}) for further detail).


% Second, \name can quickly converge to a near-optimal configuration as the configuration-accuracy relationship being mostly {\em concave}---as the configuration uses more (compute/network) resources, the change in the input to the DNN becomes more marginal, and so does the DNN output.
% For example, as a video analytic system increases the video encoding resolution, the pixel change becomes more marginal (mostly on ``high-frequency'' details, like object boundaries), causing the DNN output to stabilize (objects' confidence scores will change more slowly and less frequently cross the confidence threshold, leading to fewer newly detected objects).
% Due to this concavity, gradient ascent can eventually converge to a global optimal configuration. 

% \kt{A third reason: if config A is better than config B on this second, it is likely that config A is better than config B on the next second. I feel like this point is a bit of a noise, should we include it?}



% \mypara{Generalize to different knobs and applications}
% Compared to prior works that focus on RGB-video-based video analytic tasks, we show that \name can be applied to various types of analytic tasks (\eg object detection, segmentation, audio-to-text), input data (\eg LiDAR videos, depth videos, audio waves) and most of existing knobs (see Table~\ref{tab:rich-set-of-knobs} for the list of knobs that \name can handle) in our evaluation (\S\ref{sec:eval}).
% % Third, \name can generalize to different applications and DNNs (as \name only assumes the DNNs to be differentiable, which holds for almost all DNNs) and a wide range of knobs .
% However, we want to clarify that \name as-is \textbf{does not generalize} to knobs that alter the final DNN itself (\eg DNN selection).
% Also, \name may not generalize to generative tasks (\eg text generation, image generation).

% \mypara{Cheap calculation of \outputgrad}
% As \name frequently calculates \outputgrad, the challenge of \name is how to calculate \outputgrad with minimum resource overhead.
% Our key idea is that \outputgrad can be calculated \textbf{with no extra DNN inference by leveraging DNN's  differentiability}.
% Differentiability is an inherent property of almost all DNNs~\cite{paszke2017automatic} but has so far been mostly used in DNN training. 
% Our insight is that most knobs only transform the raw input data to DNN's input (\eg frame filtering, image downscaling, etc), so the \outputgrad of a knob can be decoupled into:
% \begin{packedenumerate}
% \item {\em \dnngrad:} How the DNN's output changes with respect to the DNN's input.
% \item {\em \inputgrad:} How the DNN's input changes with respect to the knob's configuration.
% \end{packedenumerate}
% Both can be computed efficiently: 
% computing \dnngrad can be done with a single backpropagation operation on the DNN, and 
% computing \inputgrad does not need GPU.
% Moreover, if the system has multiple configuration knobs, \dnngrad can be calculated once and re-used to derive the \outputgrad of different knobs.  
% Intuitively, \dnngrad describes DNN's sensitivity to a change in DNN's input, which is agnostic to {\em which} knob causes the change in DNN's input.
% For instance, the \dnngrad of an object-detection DNN will be high for pixels associated with key visual features of an object.



As \name introduces the extra overhead of DNN backpropagation, 
% As the overhead of backpropagation is substantial (about 2x extra GPU memory usage and 1x extra GPU computation), 
\name provides a suite of techniques that reduce this GPU compute and memory overhead 
% (together with other types of overheads) 
in \S\ref{sec:cost}, including reusing the backpropagation results between different frames (which reduces the backpropagation overhead by 10$\times$), and removing unneeded computation in backpropagation.
We want to clarify that as long as there are sufficient resources for \name to run in real-time, the extra overhead of \name does \textit{not} increase the end-to-end delay (the delay of obtaining the inference results), as the adaptation logic of \name runs after generating the inference results.




    % \myparashort{\outputgrad: How DNN inference changes with configuration.}
    % To improve on three fronts, we take a different approach by focusing on the {\em gradient} of the inference results with respect to each configuration knob---how much the inference results would change if a small change was added to each configuration knob of the current configuration. We refer to it as {\em \outputgrad}.
    % This gradient, which we refer to as {\em \accgrad}, captures how much DNN's output would change if a small change was added to the current configuration.

    

    % The insight to focus on \outputgrad is two-fold:
    % \begin{packeditemize}
    % % \item \accgrad allows us to calculate the change in accuracy, which is easier to calculate than the exact accuracy number. 
    % % This is because the change in accuracy is triggered by the change in inference results and thus correlates with the change in inference results (we will show empirical evidence in \S\ref{??}), but calculating the accuracy requires one to annotate the input data by using human annotation or by referring to the inference results with respect to the most expensive configuration.
    % % Differentiability is a key property of DNNs that differentiates DNNs and other traditional applications.
    % % However, as far as we know, previous work only uses this property as a way to train DNNs.
    % % We are the first one that expands the use case of the differentiability of DNN to scenarios outside DNN training.
    % % \kt{Maybe phrase this sentence more carefully?}
    % \item 
    %     \jc{let's drop this here. it doesn't seem really necessary to spill it out here. Instead, put it in the para starting with "by performing gradient ascent ...." as a reason why maximizing output change also maximizes accuracy. }
    %     \kt{I'm not sure about this, can we discuss? For me, outputgrad comes out of blue and we need a para to say that it correlates with accuracy.}
    % Second, a large change in inference results could statistically indicate a large change in inference accuracy.
    % Thus, \outputgrad could indicate how configuration should be changed to improve accuracy (see \S\ref{??} for empirical evidence).
    % \kt{Explain the difference between DNN output and inference accuracy, then say why statistically they aligns}
    
    % \end{packeditemize}
    % As far as we know, we are the first one that uses differentiability of DNNs in non-training environment.

    
    % Second, we embrace that DNNs are naturally {\em differentiable}. 
    % Differentiability is a common property of all DNNs but is rarely utilized by prior work to adapt configurations of DNN-based applications.
    % As elaborated shortly, differentiability makes it possible to cheaply estimate \accgrad (with minimum GPU compute overhead).
    % \end{packeditemize}

    % The insight to focus on \accgrad is two-fold.
    % First, we embrace that DNNs are naturally {\em differentiable}. 
    % Differentiability is a common property of all DNNs but is rarely utilized by prior work to adapt configurations of DNN-based applications.
    % As elaborated shortly, differentiability makes it possible to cheaply estimate \accgrad (with minimum GPU compute overhead).
    % Second, a large change in DNN output could statistically indicate a large change in inference accuracy.
    % Thus, \accgrad could indicate how configuration should be changed to improve accuracy.


    

    

    % \jc{please tighten this para. too much info before getting back to your smart cost-saving idea}
    % Inspired by these two insights, we propose \name, a configuration adaptation system that frequently calculates \outputgrad and runs a {\em gradient-ascent} strategy
    % % \footnote{Note that we can adapt even faster by using more sophisticated optimization techniques\cite{??}, but we choose not to use those techniques to demonstrate the quick adaptation speed provided by our \outputgrad only.}
    % to gradually search for the optimal configuration. 
    % First, we partition the input data stream (\eg video frames) into {\em adaptation intervals}, each of \fillme seconds.
    % % (hereinafter \textit{adaptation intervals}) 
    % % and perform adaptation in an interval-by-interval manner. \kt{Let me reconfirm the time window in my eval code}.
    % In each adaptation interval, we estimate \outputgrad and decide the configuration for the next adaptation interval by choosing to increase, decrease or keep the value of each knob so that the accuracy is maximized without exceeding the resource budget.
    % In each adaptation interval, we first estimate \outputgrad of DNN inference output
    % ---how DNN output would change with a small change on each knob value. 
    % (We will explain how to do it with minimum overhead next.)
    % Then we use this information to decide for each configuration knob whether to keep its current value, increase or decrease it by a small amount, providing that the new configuration will not exceed the resource budget. 
    % identify a new configuration that maximally improves accuracy without exceeding the resource budget.
    % We use this new configuration for the next adaptation interval and repeat the same adaptation steps on the next adaptation interval.
    % As the content of the input data is continuous, the new configuration is likely to generate more accurate inference results compared to the original configuration.
    % Note that 
    % As a result, the inference results of the new configuration are likely to be more accurate than the current configuratio

    % \jc{move this to after the gradient decoupling discussion}
    % For example, \kt{an example here, follows the fps \& resolution example.}


    % However, this gradient-ascent-based approach has its caveats.

    
    
    
    
    % \kt{explain why it is OK to reuse}
    
    % \jc{1. estimate gradient => reuse gradient to pick config in next step => use the new config in the next step => go back}
    
    % while these heuristics can have much lower accuracy than the optimal configuration.

    

    % \jc{
    % \begin{packeditemize}
    %     \item Compare between backprop and saliency
    %     \item caveats of gradient descent:
    %     \begin{packeditemize}
    %         \item each step must be small => we estimate \accgrad extremely fast, so can adapt very frequently
    %         \item how to deal with local optimum => ??
    %     \end{packeditemize}
        
    % \end{packeditemize}
    % }

    % An ideal configuration adaptation system, therefore, needs to serve a wide range of knobs and applications, and quickly identify the optimal configuration with no extra inference.

    % We take an alternative approach. Unlike previous work that only obtains the accuracy from the current configuration, we further obtain the \textit{gradient} of the accuracy with respect to the current configuration (hereinafter \accgrad, we will define it later).
    % This \accgrad can be \textit{cheaply} computed \textit{without running DNN inference} by leveraging the differentiability of the DNNs.
    % Using this \textit{cheap} \accgrad, we can then \textit{frequently} run \textit{gradient ascent} to quickly adapt to a near-optimal config (empirically within 2 seconds).
    % As a result, we can adapt to a near-optimal config within 2 seconds.
    
    % based on the accuracy of the current configuration, we can further derive the gradient of accuracy with respect to the current configuration by leveraging the fact that DNNs are differentiable, 
    % based on the accuracy of the current configuration, we can further by leveraging the fact that DNNs are differentiable, we can calculate the gradient of accuracy with respect to the current configuration  \textit{without extra DNN inference} and use this gradient to identify a configuration that can significantly improve accuracy.
    % As a result, we can frequently pick the configuration that can significantly improve accuracy, allowing us to adapt to a near-optimal optimal configuration within 2-3 seconds.
    % If we can find a direction that maximally improves accuracy, we can reach the optimal within 3-4 steps.
    % We take an alternative approach that adapts the configuration gradually, which allows us to adapt quickly (by stepping towards a new config right after identifying a config that may improve the accuracy under the resource budget) and adapt to a near-optimal config (by constantly finding a config that may improve the accuracy under the resource budget).
    % The key to this approach is to decide which config should be picked in the next step.
    % We leverage the \textit{gradient} of accuracy to determine this config based on two reasons:
    % \begin{packeditemize}
    % \item mathematically the gradient of accuracy points to the config that improves accuracy the most
    % \item the cost of calculating the gradient of accuracy (in terms of network and GPU compute) can be significantly reduced by leveraging the fact that DNNs are differentiable.
    % \end{packeditemize}

    % We can update right after obtaining the gradient (instead of obtaining
    
    % The limitation of prior works comes from the fact that they abstract the DNN (together with the underlying system components, like video codecs) as a black box.
    % As a result, they either need to run this black box multiple times to accurately identify the optimal configuration (resulting in slow adaptation speed), or need to build cheap proxies to estimate the performance of this black box (resulting in selecting configurations with much lower accuracy than the optimal configuration).
    
    % However, different from adapting the configuration of traditional applications (like job scheduling), DNNs have a unique property that makes them much more amenable to configuration adaptation.
    % \kt{this sentence is a bit out-of-the-blue, need a way to fix it.}
    % Concretely, DNNs are designed to be \textit{differentiable}, granting them the ability to \textit{adapt} DNN parameters to fit different input content (\eg different images in the training set) through the DNN training process. 
    % On a high level, the goal of configuration adaptation is also adapting its parameters (\ie knobs) to fit different input content. 
    % This inspires us to leverage the differentiability of DNN for configuration adaptation.

    % The spirit of this algorithm is akin to \textit{gradient ascent}. One may wonder that 
    % \jc{to make this gradient-ascent search practical, the key technical challenge is how to {\em quickly and accurately estimate \accgrad for multiple configuration knobs with minimum extra GPU computation.}
    %     \begin{packeditemize}
    %         \item use differentiability to decouple
    %         \item faster backdrop (yitian)
    %     \end{packeditemize}}
        
    % \kt{Not sure where should I put this.}
    % The key in our approach is to calculate \accgrad (defined as the change of inference accuracy if each knob of the current configuration was changed by a small amount).
    % \accgrad can directly suggest which knobs to change so that inference accuracy will likely increase by the largest amount in the coming second, without using more network and GPU compute resources than the budget. 
    % Concretely, we give more resources to the knobs with high Output-Knob Gradient to improve the accuracy by the largest amount and cut the resource usage of those knobs with low Output-Knob Gradient to save resources with minimum degradation in accuracy. 


    
    % \kt{Though how to use the gradient is crucial, understanding this sentence requires a lot of extra knowledge (like config knob value bounds to resource, more resource -> higher accuracy). Not sure how to fix this for now.}
    
    % Although doing so may not immediately adapt to the optimal configuration, this \accgrad-based adaptation can adapt to a near-optimal configuration within a handful of steps (empirically, we can adapt to a near-optimal config within 2-3 seconds).

    
    % if we know the gradient of accuracy with respect to the current configuration (\ie how much does increasing the value of each knob change the accuracy, hereinafter \accgrad), we can accurately estimate the accuracy of a large subset of configs (see \S\fillme for further detail) and adapt to a near-optimal config within 2 seconds by assigning more resource to those knobs with a high gradient of accuracy, or cut the resource usage of those knobs with a low gradient of accuracy without hurting the inference accuracy (see \S\fillme for further detail).
    % \kt{it is definitely better if we can illustrate the rationale of why gradient converges so fast. I do not have a good argument yet and I will keep on trying.}.


    % \kt{If you can get gradient, 1. quick adapt 2. near-optimal config in 2/3 steps}
    % However, generally these heuristics sacrifices the ability of picking the optimal configuration at once. generally more difficult for these approach to pick the optimal configuration at once.
    % \kt{generaly sacrifices the optimality}
    % \kt{mention that this approach adapts faster}
    % However, as the optimal configuration is jointly determined by the current video input and the DNN itself, how DNN processes the current video is highly complex (due to the complexity of the DNN) the relationship between the current video input to the corresponding optimal configuration heavily depends on how DNN processes the current video
     % .
     % As a result, these heuristics will have low accuracy.
    %  However, in order to accurately identify the optimal configuration, one needs to check whether a different config in the resource budget can generate more accurate inference results or not, requiring extra DNN inference on this config.
    % As these heuristics does not perform extra inference, they may fail to accurately identify the optimal config and end up using a sub-optimal config, resulting in low accuracy
    
    
    % extra DNN inference without DNN inference, cheap heuristics may fail to identify such configuration-changing event in the video and thus cannot fix such accuracy drop.
    % \kt{DDS falls into this category}
    % \item Difference: other configs is no longer visible.
    % \item No extra inference and generate new config with heuristics.
    % \item Adapt without extra DNN inference (using heuristics)
    % These heuristics may generate a suboptimal config upon change.
    % Without comparing to other configs, we cannot tell whether the current config is optimal or not --> will use sub-optimal configuration when the heuristics --> low accuracy
    % \kt{Should we take server-driven approach into account here?}

    % mappin between config and accuracy is highly complex --> DNN output / video input only reveals limited information regarding this highly-complex space --> need to accumulate enough information to achieve optimal.

    % \kt{What is gradient}
    % \kt{how to use this gradient}
    % \kt{Empirically we can adapt to optimal within 3-4 steps}

    % \kt{Ideally, first we want to reduce the cost of extra inference on other configs, and then reduce the cost on golden config.}
    % \jc{
    % to make this gradient-ascent search practical, the key technical challenge is how to {\em quickly and accurately estimate \accgrad for multiple configuration knobs with minimum extra GPU computation.}
    %     \begin{packeditemize}
    %         \item use differentiability to decouple
    %         \item faster backdrop (yitian)
    %     \end{packeditemize}}
    
    
    % Remove this paragraph as it makes the reader impatient.
    % To make \name practical, the key technical challenge is how to cheaply and accurately estimate \outputgrad with minimum extra GPU computation.
    % Remember that \outputgrad is how much the inference output would change if a small change was made to each knob of the current configuration.
    % A naive way to compute \outputgrad on each configuration knob will require running two DNN inferences, one without change to the knob value and one with a small change to its value, and comparing their difference. 
    % With each configuration knob requiring one extra DNN inference on GPU, the overhead to obtain \outputgrad on one configuration grows with more configuration knobs, and this overhead must be added to each adaptation interval.
    % To put this overhead into context, one may need to tune 3 knobs~\cite{awstream,casva} in order to maximally reduce the bandwidth usage while maintaining high inference accuracy.
    % As a result, one needs to perform 3 times extra DNN inference to obtain \outputgrad for each adaptation interval, costing 4x more GPU resource usage compared to using existing techniques~\cite{casva}.
    
    
    
    % % \kt{Done. Change to one insight \& merge with gradient decoupling}
    % Our insight is that by leveraging the {\em differentiability} of the DNNs, \outputgrad can be calculated with no extra DNN inference.
    % Differentiability is a common property of almost all DNNs~\cite{paszke2017automatic} but has so far been only used in DNN training. 
    % We demonstrate that DNN differentiability can be used to  quickly and optimally adapt configurations of DNN analytics systems.
    % -based inference applications.
    % Note that calculating \outputgrad through its definition (how much the inference results would change if a small change was added to the current configuration) causes substantial GPU compute overhead, as it requires one to change the configuration knobs \textit{one-by-one} in order to obtain the change in accuracy and thus the extra DNN inference required by \outputgrad is \textit{proportional} to the number of knobs.
    % To put this overhead into context, one may need to tune more than 3000 knobs in order to tune the encoding quality of different spatial regions in the video~\cite{eaar,accmpeg}.
    % To calculate the \accgrad in real-time, one needs to perform >3000 extra DNN inference, costing >3000x GPU resource compared to using existing techniques~\cite{eaar,accmpeg}.
    % \kt{We need a figure for this decoupling.}
    % \kt{Remind people of differentiability}
    % The idea here is that \outputgrad (\ie how configuration changes the DNN output) equals to the multiplication of two terms:
    % \kt{The original text: The idea here is that \outputgrad (\ie how configuration changes the DNN output) equals to the multiplication of two terms:}
    % \kt{I prefer to not use multiplication as it gives people the wrong impression that we are just multiplying two numbers.}
    % Specifically, we decouple the calculation of \outputgrad of each knob (gradient of the inference results with respect to the knob) into two components:
    % we leverage the differentiability of DNNs by decoupling \outputgrad (\ie how much the inference output would change if a small change was made to each knob of the current configuration) to two terms:
    % \kt{For me, the key is to address Ganesh's concern may be to write these two terms in a way that they feel like a matrix.}
    % \begin{packedenumerate}
    %     % \item {\em DNN output's gradient w.r.t DNN input:} how the inference output changes with the DNN input.
    %     \item {\em \dnngrad:} How DNN's output changes with a small change in different parts of the DNN input.
    %     % DNN output's\footnote{\jc{need a short footnote to explain what the DNN output mean or should capture. maybe put some old text "thresholding, etc" here. this can also be merged with the "saliency" footnote}} gradient with respect to a small change in different parts of DNN input.
    % %     \footnote{\dnngrad is similar to the notion of DNN's ``saliency'' in computer vision.\jc{kuntai, please rethink this point} 
    % % \hl{However, existing saliency estimators put objects in high saliency, while \dnngrad puts pixels that may change the inference results in high saliency, making \dnngrad outperforms existing saliency estimators. See XXX for more rationales.} \kt{Address one expert reviewers' novelty concern.}}
    %     % DNN input. how much DNN output changes regarding a small change of different parts of DNN input. We call this term \dnngrad for short.
    %     % \jc{Should we call this term ``saliency''? I feel like calling it saliency gives people a better understanding of what this term is, and implicitly explains why this term can be shared across knobs, but we then need to defend this is a new saliency.}
    %     % \item {\em DNN input's gradient w.r.t configuration:} how the DNN input changes with the configuration, and
    %     \item {\em \inputgrad:} How different parts of the DNN input change with a small change in the knob value.
    %     % DNN input's gradient with respect to a small change in the current value of each configuration knob.
    %     % regarding configuration how much different parts of DNN input changes regarding the change of the current configuration.
    % \end{packedenumerate}
    % % f(2,2), (1,0), (0,1)
    % % f(3)-f(2)/1 == f(1) - f(2)/ -1
    % % f(2+x,2)-f(2,2) = f(2,2) + f'(2,2) * (x, 0) + O((x,0)^2)    
    % % Intuitively, the first term captures the importance of different parts of DNN input, 
    % % The key is our first insight is that a DNN's output is differentiable with respect to the DNN input. 
    % It is important to notice that due to DNN differentiability, \dnngrad can be efficiently calculated by DNN's backpropagation operation, and computing \inputgrad does not need GPUs.
    % More importantly, if the system has multiple configuration knobs, \dnngrad can be calculated once and re-used to derive the \outputgrad of different knobs.  
    % % without extra DNN inference on GPU.
    % This is because \dnngrad describes DNN's sensitivity to each part of the DNN input, and it remains largely the same if the change in DNN input is not dramatic.
    % For instance, the \dnngrad of an object-detection DNN will be high for pixels associated with key visual features of an object.
    % % and remains largely the same when a small change is applied to different knobs.
    % % \ga{DNN grad same -> Input change small ->  output change small -> } \kt{this is a important question but difficult to answer. I'll prioritize other part and then circle back to this later.}
    % % Thus, if the system has multiple configuration knobs, \dnngrad will be calculated only once and re-used to derive \outputgrad of different knobs without extra DNN inference on GPU.
    % % the first term can be calculated via one backpropagation and then shared across multiple knobs \jc{Should we defend this share?}.
    % % This is a constant GPU-time operation without extra inference because it reuses the layer-wise features generated alongside DNN inference.
    % % Additionally, the second term is operating between DNN inputs and thus not involving any DNN inference.
    % % Therefore, computing \outputgrad for multiple configuration knobs only requires a one-time backpropagation on GPU and no extra DNN inference.
    % % calculated in a knob-by-knob manner without DNN inference (\ie no GPU compute)
    % \name also includes optimizations to further reduce the GPU and memory overhead of DNN backpropagation (see more details in \S\ref{sec:cost}).

    % \jc{edit ends here}
    % \jc{Junchen can you read here and see if it works for you?}
    % Further, given that backpropagation poses high GPU computation and memory overhead (even greater than DNN inference~\cite{?,?}), we present a set of techniques to further reduce the GPU computation and memory overhead of backpropagation by computing the saliency at a coarser granularity (see \S\ref{??} for details).

    % Configuration change (0,1)
    % (Grad, I(2,3) - I(2,2)) = D(I(3,2)) - D(I(2,2))
    % Configuration change (1,0)
    % (Grad, I(3,2) - I(2,2)) = D(I(2,3)) - D(I(2,2))
    % Ganesh: why D(I(3,2)) != D(I(2,3)) but exist such a grad?
    % The first term can be reused 
    
    % To avoid such extra DNN inference, OneAdapt leverages the differentiability of the DNN to implement \outputgrad. 
    % Concretely, we \textit{decouple} \outputgrad (\ie (how much the inference results would change if a small change was added to the current configuration) to 
    % \begin{packeditemize}
    %     \item {\em Configuration to DNN input:} how does the DNN input change with the configuration, and
    %     \item {\em DNN input to output :} how does the inference results change with the DNN input.
    % \end{packeditemize}
    % The former can be calculated in a knob-by-knob manner without DNN inference (\ie no GPU compute), and the latter can be obtained via {\em backpropagation} (which is a constant GPU overhead without extra inference as it can reuse the existing computation graph of DNN inference).
    
    
    % Calculating the former term does not require DNN inference.
    % The latter term corresponds to the gradient of inference results with respect to the DNN input of the current configuration\footnote{Note that it can be mathematically proved that the latter term corresponds to the gradient of inference results with respect to the DNN input of the current configuration (under the assumption that changing configuration only creates a small change to DNN input). We also show more empirical evidence in \S\fillme.} and can be calculated using backpropagation, which requires extra GPU computation and GPU memory but does not require extra DNN inference as it can reuse the existing computation graph of DNN inference.
    
    % This is a metric that only depends on the current configuration, and thus can be calculated once using backpropagation algorithm and then shared across .
    % As a result, calculating \outputgrad requires one backpropagation (constant GPU overhead) and no extra DNN inference.

    % \kt{Will expand this paragraph after finalize Yitian's backpropagation cost reduction technique}
    % While the calculation of \outputgrad no longer requires extra DNN inference,  In \S\fillme, we present a set of techniques aimed at reducing the GPU overhead and other types of overhead (such as bandwidth overhead and camera-side overhead) associated with the computation of \outputgrad. 
    % These techniques allow us to calculate \outputgrad with minimum overhead \kt{quantify this. Will do it after Yitian's experiment.}
    % \kt{A sentence that highlights the low overhead of \outputgrad. Will add it after Yitian finishes her experiments.}

    % Based on \outputgrad, 
    
%     \myparashort{\name: Using \outputgrad to adapt configuration.}
%     We present \name, a new configuration adaptation system, which frequently estimates \outputgrad (every second) and uses the up-to-date \outputgrad to perform {\em gradient ascent} to adapt the configuration in a way that increases accuracy without using more resources (\S\ref{sec:design}).
%     We empirically observe that \name's gradient ascent converges to a near-optimal configuration within a few iterations.
% \name's fast convergence can be attributed to the configuration-accuracy relationship being mostly {\em concave}---as the configuration uses more (compute/network) resources, the change in the input to the DNN becomes more marginal, and so does the DNN output.
% For example, as a video analytic system increases the video encoding resolution, the pixel change becomes more marginal (mostly on ``high-frequency'' details), causing the DNN output to stabilize (objects' confidence scores will change more slowly and less frequently cross the confidence threshold, leading to fewer newly detected objects).
% Due to this concavity, gradient ascent can eventually converge to a global optimal configuration. 


% One may worry that calculating \outputgrad once every second may result in a high end-to-end delay (the delay of obtaining the DNN inference results), as calculating \outputgrad requires running backpropagation, which is even more expensive than DNN inference as it may require both extra GPU compute and extra GPU memory.  
% We point out that as \name runs its adaptation logic \textit{after} generating inference results, the extra GPU compute and memory overhead does not affect the end-to-end delay unless there is not enough resource for \name to run its adaptation in real-time.
% We also present a suite of techniques in \S\ref{???} to further reduce the GPU overhead (and other types of overheads) of \name.


% \kt{Need to add more text to address: (1). the assumptions of OneAdapt (2). the scope where OneAdapt generalizes. (3). Why it is OK to have the overhead of backpropagation}

% It splits the input data stream into {\em adaptation intervals} (\eg every second), and at a high level, in each adaptation interval, we obtain DNN output using the current configuration, calculate \outputgrad, and uses the \outputgrad to adjust the configuration knob values using a gradient-ascent algorithm to increase accuracy in the next adaptation interval while adhering to the resource budget (see \S\ref{??} for details).
    
    
    % strategy to gradually search for the optimal configuration. 
    % decide the configuration for the next adaptation interval by adjusting the configuration knobs of the current configuration, either increasing,  decreasing, or retaining them,  to maximize accuracy 
    % \kt{Should we explain why \outputgrad correlates with accuracy here?}
    


    % \name outperforms previous work on all three fronts (\ie adapt frequently, converge to a near-optimal configuration, and generalize to different types of knobs and analytic tasks).
    % \kt{Done. Put the rationale of \outputgrad correlates with accuracy here.}
    % \begin{packeditemize}
    % \item
    


    % % \jc{move figure 2 in intro?} \kt{done}
    % % \hl{
    % Figure~\ref{fig:adaptation-behavior} compares \name with previous approaches.
    % % }
    % Unlike profiling-based methods, \name uses much less compute to calculate \outputgrad than profiling, so it can adapt configuration much more frequently  and react more timely to the change of source data.
    % % \name could adapt right at the following second after the input content changes), 
    % % because it takes much less compute and network resources than profiling.
    % % the profiling-based baseline adapts slowly (once every minute~\cite{awstream}) may wait for at most a minute to react 
    % % \item
    % % Compared to heuristics that run no extra DNN inference,
    % Unlike simple heuristics, \name can adapt more optimally because \outputgrad captures how configuration affects the actual DNN output. The more DNN output changes, the more inference accuracy changes (\S\ref{subsec:limitation}). 
    % % \name can adapt to a near-optimal configuration where the works that perform no extra DNN inference may pick configuration with much lower accuracy.
    % % This is because \outputgrad can indicate the accuracy of different configurations.
    % % Intuitively, when a knob is of large \outputgrad, changing it can significantly impact the inference results.
    % % Thus, by allocating more resources to this knob (\eg by increasing its value), the improvement in inference accuracy is also likely to be substantial.
    % % \S\ref{??} shows more details on how we indicate the accuracy of other configurations and the correlation between our indicated accuracy and actual inference accuracy.
    % % As a result, if we assign this knob more resources (\eg by increasing its value),  the accuracy improvement also tends to be significant.
    % % Second, a large change in inference results could statistically indicate a large change in inference accuracy.
    % % Thus, \outputgrad could indicate how configuration should be changed to improve accuracy (see \S\ref{??} for empirical evidence)., where the accuracy of these works can be much lower than the optimal configuration.
    % % \item
    % Moreover, since DNNs are differentiable, \name could generalize a wide range of DNN-based analytic tasks (Table \ref{tab:pipeline} for a list of pipelines that \name can optimize).
    % That said, 
    % % The second limitation is that, though \name can be used to tune a wide range of configuration knobs, it 
    % \name as-is does not apply to those knobs that alter the DNN itself, such as retraining the DNN weights~\cite{ekya,mcdnn,noscope} (see \S\ref{subsec:limitation}). 
    % % Also, \name does not generalize to generative tasks like text generation and image generation.
    % % Similar to \name, they also adapt to changes in input distribution. 
    % % However, DNN retraining involves substantial computation and thus tends to adapt at a coarser timescale, while the knobs considered in \name require frequent adaptation.

    
    % (as \name only assumes the DNNs to be differentiable, which holds for almost all DNNs~\cite{?,?}) and a wide range of knobs (as \name poses minimum assumptions to the configuration knobs, see 
    % % \S\fillme for a full list of assumptions).
    % Table \ref{tab:rich-set-of-knobs} for a list of knobs that \name can optimize.
    % \end{packeditemize}


    
    % \kt{need a rewrite}
    % One may find the similarity between estimating the region-of-interest in the input video and calculating how DNN input affects inference results.
    % However, compared to existing region-of-interest 
    % \begin{packeditemize}
    %     \item Region-proposal-based: a region that is far away from any of the bounding boxes can affect the inference results a lot
    %     \item Camera-side cheap DNN: due to camera-side compute limit, a cheap DNN either misses regions that change inference results or wrongfully perceive those regions that have minor impact on the inference results as impactful. \kt{need to discuss AccMPEG in related work.}
    %     \item Saliency-based approach: pose high camera-side overhead. May highlight the objects that the final DNN does not detect.
    % \end{packeditemize}


    % \kt{No part of the paper should be like a math paper.}
    % \kt{Junchen can you check this paragraph?}
    % \jc{
    % rewrite this. i like what you said last night about why the whole config-accuracy plane is concave (i.e., only one global optimum)}
    % \kt{done}

We evaluate \name across 9 analytic pipelines (see Table~\ref{tab:pipeline} for the detail of these pipelines), which cover 4 analytic tasks (vehicle detection, human detection segmentation, audio-to-text), 5 types of input data (\eg LiDAR videos, audio waves), and 5 types of knobs (\eg video codec knobs, frame filtering thresholds).
% Our dataset contains 59 videos (~110 minutes in total) and 200 audios (33 minutes in total).
% We evaluate \name across 9 different DNN-based analytic pipelines, with 5 types of data, 4 analytic tasks, 6 configuration knobs, 59 videos, and 200 audios. \jc{earlier you said it can work on 3 analytic tasks (object detection, segmentation, audio-to-text), 4 input data (videos, LiDAR feeds, depth videos, audio waves), and ?? knobs (see Table~\ref{tab:rich-set-of-knobs} for the list of knobs that \name can handle). can we be consistent about it?}
\name achieves similar accuracy with 15-59\% resource usage reduction, or achieves 15\% higher accuracy with similar resource usage compared to the baselines on 9 different analytic pipelines.
We also show that the performance gain of \name over the baselines increases with more knobs. % become more fine-grained.

These results also show that rather than targeting a specific setting, \name can work in a {\em variety} of analytic tasks, input data types, and knobs.
That said, \name has limitations (more in \S\ref{sec:limitation_section}). We have not tested if \name will work for applications beyond our evaluation, such as knobs that alter the final DNN itself (\eg DNN selection) or generative tasks (\eg text generation, image generation).
    


\begin{comment}
    

That said, \name's gradient-ascent strategy
    % has two main limitations. 
    % First, \name adapts configurations based on gradient ascent, which has its own caveats, such as the possibility that the search 
is not guaranteed to converge quickly to the optimal configuration.
    % the converged configuration is sub-optimal.
    % However, we empirically show that \name can reach a near-optimal configuration within \fillme seconds (\S\ref{??}).
    Intuitively, this can be understood that gradient-ascent can always converge to optimal if configuration-accuracy relationship is {\em concave}---as the configuration uses more (compute/network) resources, the change in the input to the DNN becomes more marginal, and so does the DNN output.
    In practice, such concavity does hold in most cases.
    % because the configuration-accuracy relationship is mostly \textit{concave}. % due to the following observation:
    % As the configuration uses more (compute/network) resources, the change in the input to the DNN becomes more marginal, and so does the DNN output.
    % are given to the analytic system (\eg by increasing the value of one configuration knob), 
    % the accuracy of DNN inference results improves slower and slower as the .
    For example, as a video analytic system increases the video encoding resolution, the pixel change becomes more marginal (mostly on ``high-frequency'' details), causing the DNN output to stabilize (objects' confidence scores will change more slowly and less frequently cross the confidence threshold, leading to fewer newly detected objects).
    % when we assign the system more and more resource by increasing the resolution, initially every pixel value change significantly.
    % Thus, the DNN inference results also tend to change significantly, making the accuracy significantly improved. 
    % At a higher resolution, however, most of the pixels no longer change except for those pixels that are related to the fine details (\eg the boundary of an object) when we further increase the resolution.
    % As a result, the inference results only changes a little, resulting in marginal accuracy improvement.
    % We also empirically confirm that the configuration--accuracy space is concave in \S\fillme.
    % By leveraging the concavity of the configuration--accuracy space, our gradient-ascent-based approach can quickly converge~\cite{?,?} and can converge to the global optimal (as there is no local optimal in the configuration--accuracy space under the resource budget).

\end{comment}

    % \jc{merged the "no dnn knob" para to two paras earlier}
    % The second limitation is that, though \name can be used to tune a wide range of configuration knobs, it does not apply to those knobs that alter the DNN itself, such as retraining the DNN weights~\cite{??}. 
    % Similar to \name, they also adapt to changes in input distribution. 
    % However, DNN retraining involves substantial computation and thus tends to adapt at a coarser timescale, while the knobs considered in \name require frequent adaptation.
    
    % \kt{Talk about the cases, where the accuracy improvement may not become more and more marginal.}
    % \kt{Other potential concerns: (1) why treat discrete configs as almost continuous variables, (2) why the better configuration at this second will likely lead to better result at the next second, (3) what if the content is noisy and makes the gradient noisy}
    


    
    % The intuition behind the fast convergence is that as long as the \outputgrad with respect to one configuration knob is non-zero, tuning that knob will likely improve accuracy.
    % % Further, as the input data is constantly changing over time, it is less likely for a local optimal to persist.
    % Thus, \name is unlikely to be stuck in a local optimum, which corroborates our empirical observation of \name.
    % (See \S\ref{??} for more details.)
    
    
    % Despite the low cost of \outputgrad estimation, the configuration adaptation based on gradient ascent in \name has its own caveats, including the inability to guarantee a quick convergence or the optimality of the converged configuration. 
    % However, our experiments demonstrate that \name can attain a much better configuration within \fillme seconds. 
    % It can be intuitively understood that if the \accgrad with respect to a particular configuration knob is non-zero, adjusting that knob will likely lead to improved accuracy. Additionally, since the input data is continuously changing over time, it is less likely for a local optimum to persist. As a result, \name is unlikely to become stuck in a local optimum, which is supported by our empirical findings on \name. (Further details can be found in Section \ref{??}.)
    
    % At a high level, \name uses a greedy gradient-ascent search to tune configurations and gradually improve accuracy under the resource constraint, but given the complex relationship between accuracy and configuration, 



  
    % \kt{Multiple times per second sounds weird. But one time per second sounds like we are adapting slowly, especially given that we need multiple steps to converge} 
    % than profiling-based work (\eg once every 15 seconds \kt{back this number up in footnote}), and can thus adapt to a new near-optimal within \fillme seconds after the optimal config changes.
    
    % \kt{needs to work on this rationale as we are not directly optimizing accuracy...}
    % We are more likely to find a near-optimal config compared to heuristics-based approaches as we adapt configurations based on the change of inference results, which correlates to accuracy (though we may not adapt right to the optimal configuration).
    % \kt{Across different tasks, different knobs}
    % Moreover, our approach can generalize to a wide range of knobs as we perform the adaptation based on the inference results.
    % That said, our approach cannot handle all knobs and we will illustrate those knobs that we cannot handle soon.
    
    
    
    

    
    % To reduce such GPU compute overhead, we calculate \outputgrad by splitting it into two terms:
    % \begin{packeditemize}
    %     \item calculating the change of DNN input when changing each knob by a little, which requires no extra GPU compute, and 
    %     \item calculating how much the change of current DNN input affects the inference results.
    % \end{packeditemize}
    % Note that The latter term can be measured by calculating the \textit{gradient} of the inference results with respect to the current DNN input through backpropagation algorithm.

    
    % We find that the first term does not require GPU and the latter term can be \textit{reused} across different knobs.
    % Our rationale is that, if changing a region of the current DNN input affects the accuracy a lot, it means that the DNN is uncertain about the inference results corresponding to this region. 
    % As we are changing each knob by a little amount when calculating \accgrad, the corresponding DNN input is still highly similar to the current DNN input, and the DNN is still likely to be uncertain about the inference results corresponding to this region.
    % As a result, this region will still have a significant impact on accuracy.
    
    % Further, the latter term corresponds to the \textit{gradient} of accuracy with respect to the DNN input, which can be directly calculated by the backpropagation algorithm (see \S\ref{??} for more illustrative examples and rationales).
    % As a result, by reusing the latter term across multiple knobs, calculating \accgrad only requires running backpropagation and no longer requires extra DNN inference (as backpropagation reuses the computation graph generated by existing DNN inference).

    
    

    
    % Our rationale is that: the ability of accuracy change
    % Ganesh: different DNN output, why single gradient?
    % Initial counterpoint: for a linear function, no matter how your DNN input changes, the output is still stable.
    % \kt{Here is just a placeholder argument. Will improve it later.}
    % This is because the granularity of existing knobs does not require an accurate pixel-by-pixel gradient.
    

    % As backpropagation can be even more expensive than DNN inference as it may require both extra GPU compute and extra GPU memory.  We will present a suite of techniques to further reduce this cost in \S\ref{???}.

    % \kt{Resource-constrained gradient ascent}
    % By obtaining \accgrad cheaply, we can then run gradient ascent to quickly adapt to a near-optimal configuration. 
    % Empirically, we find that we can adapt to a near-optimal configuration within 2 seconds.
    % Note that we can adapt even more faster by using more sophisticated optimization techniques\cite{??}, but we choose not to use those techniques to demonstrate the quick adaptation speed provided by our \accgrad only.

    % \kt{gradient ascent caveats}
    % \kt{Why local optimal OK, solution is greedy, 1. if the solution is far away why can you get there, 2. why you won't stick into local optimal}
    
    % \kt{Here is a placeholder para. Need to rewrite every sentence.}
    % At a high level, \name uses a greedy gradient-ascent search to tune configurations to gradually improve accuracy (constrained by resource usage), but given the complex relationship between accuracy and configuration, it cannot guarantee that (i) the search will quickly converge in a few steps, or (ii) the converged configuration is optimal.
    % Fortunately, our experiment shows that \name can converge at a much better configuration within 2-4 (??) seconds. 
    % Intuitively, as long as the \accgrad with respect to one configuration knob is non-zero, tuning that knob will likely improve accuracy.
    % Thus, with multiple configuration knobs, \name is unlikely to be stuck in a local optimum, which corroborates our empirical observation of \name when tuning more than three configuration knobs together.
    % (See \S\ref{??} for more details.)
    
    % First, prior work has shown that it suffices to tune each configuration knob with no more than six values (\eg \fillme uses \fillme levels of resolutions), so it does not take too long to 
    % Since \accgrad allows \name to tune all configuration knobs together, 
    
    % Gradient ascent does not guarantee that we can quickly adapt to a near-optimal config based on two reasons.
    % One, if the optimal config is \textit{far away} from the current config, it may take a long time to adapt to a near-optimal config.
    % In our case, the optimal config is not far from the current config, because each knob typically has less than 6 values.
    % As a result, the distance between the optimal config and the current config on each knob is less than 6.
    % As \accgrad allows us to change all knobs simultaneously, it means that we can achieve a near-optimal config within 6 steps.
    % We also empirically show that we can hit the optimal config within 6 steps.

    
    % we can change all the knobs simultaneously.
    % As each knob typically contains less than 10 values, even if we only change each knob by the smallest amount, we can hit the optimal config within \fillme steps.
    
    % \kt{Not sure if we need to bring up the point that increasing the knob always increases the accuracy.}
    % Second, one may worry that our solution may get stuck into a local optimal config.
    % However, as a local optimal config means that the accuracy of it cannot be improved by changing \textit{any} knob, the number of local optimal config will be smaller when there are multiple knobs.
    % Moreover, it is less likely for a local optimal to persist as the input video content is constantly changing.
    
    % less likely to happen when there are multiple knobs, as 
    % It is less likely to happen when there are multiple knobs as a local
    
    


    % We present \name, a configuration adaptation system that adapt the configuration by running \accgrad-based gradient ascent.
    % \name can quickly adapts to near-optimal config without extra DNN inference.

    
    
    % Note that we will introduce more techniques to further reduce the overhead (in terms of both network and GPU compute)  of obtaining \accgrad in \S\fillme.


    % We will 

    

    


    

    



    % \kt{a para here for gradient ascent and its caveats}



    
    % GPU compute overhead (we will further reduce GPU compute overhead and network overhead in \S\fillme).
    % \kt{propose gradient decoupling here without referring to }
    % One may think of calculating \accgrad in a knob-by-knob manner.
    % Concretely, to calculate this gradient for each knob, we need to calculate the accuracy between two configs (the current config, and the current config with the value of this knob increased) and then calculate the change of accuracy, divided by the change of knob value.
    % Previous work calculates the accuracy of a config by comparing inference results of that config with the inference results of the most resource-demanding config\kt{footnote chameleon here}, resulting in extra streaming and DNN inference overhead.
    % This overhead can be substantial \kt{quantify it}.
    % To reduce this overhead, our observation is: the change of accuracy between two configs is proportional to the corresponding change of inference results\kt{a pointer to how to measure the change of accuracy}.
    % \kt{It does not sounds like something that can reduce the cost of inference}
    % Intuitively, if the inference results of two configs are the same, their corresponding accuracy are also the same.
    % If the inference results changes significantly, the accuracy also tends to change significantly.
    % \kt{a pointer to empirical evidence}.

    % \item We take an alternative approach: we leverage\jc{"leverage" sounds like gradient is known but not used before and you just leverage it..} the \textit{gradient} of accuracy with respect to the current configuration (\accgrad for short) to adapt the config.
    % \jc{the next sentence is important, and needs some work}
    % This gradient enables us to quickly adapt to the optimal config, as gradient\jc{do you mean \accgrad?} points out the direction\jc{direction is a new term. avoid it} that increases accuracy\jc{accuracy on the current frame, current second, next second, or something else?} the most and those configs that are not on the gradient direction\jc{what do you mean by a config being on the gradient direction?!} increase accuracy slower\jc{what do you mean "increasing accuracy slower"?!} (compared to those configs that are on the gradient direction) and can be filtered out (unless the configurations are far away\jc{what do you mean "far away"?} from the current configuration, or the configs that align\jc{again, what does "aligning with gradient direction" mean?!} with gradient direction are out of resource budget\jc{this term is used without explanation}, we will further illustrate the details in \S\fillme). \jc{ok, I take it back. this sentence doesn't need some work; it needs a lot of work :) }



    % \item To illustrate why using gradient enables us to quickly adapt to the optimal, we start by describing the \textit{concavity} between the configurations and their corresponding accuracy. \\
    % We observe that, as the video analytic system consumes more and more resource (by changing the configuration), the accuracy improvement  becomes more and more marginal.
    % In other word, the gradient of accuracy diminishes when the config consumes more and more resource.
    % Mathematically, we formulate this observation by assuming the mapping between the configuration and the accuracy is concave.
    % \kt{Put a figure here and to illustrate why the observation transforms to concavity.}
    % We empirically measure this concavity in \S\fillme.


    % \item By introducing \accgrad, we can leverage the concavity of the mapping between configuration and accuracy to quickly converge to the optimal config.

    % \jc{the flow is broken here. the next para seems to assume that people are already convinced that having so-called "gradient" is highly useful. this is never established.}



    
% \kt{make a point after mentioning the cost reduction problem: the knobs are related to DNN input}
%     However, calculating \accgrad for each knob individually incurs high overhead, as it requires extra DNN inference (to obtain the inference results of a config besides the current config) on every knob.
%     As a result, the amount of extra DNN inference is proportional to the number of knobs.
%     This overhead can be substantial.
%     For example, one may need to tune more than 3000 knobs in order to tune the encoding quality of different spatial regions in the video~\cite{eaar,accmpeg}.
%     To calculate the \accgrad in real-time, one needs to perform >3000 extra DNN inference, costing >3000x GPU resource compared to using existing techniques~\cite{eaar,accmpeg}.

%     \kt{This point need to be mentioned much earlier}
%     To reduce this overhead, we calculate \accgrad for all knobs jointly by splitting the change of DNN output into two parts:
%     \begin{packeditemize}
%         \item calculating the DNN input change (No need for GPU), and 
%         \item calculating how the DNN input change affects inference results (note that this term corresponds to the \textit{gradient} of the inference results wrt DNN input and can be calculated using one single backpropagation).
%     \end{packeditemize}
%     As a result, calculating \accgrad only requires one backpropagation (which does not incur extra DNN inference, as backpropagation reuses the computation graph generated by existing DNN inference).
%     \kt{needs more explanation: change the input, why we can reuse the same backprop gradient}
%     \kt{If the inference results actually changes, why we can reuse the gradient}


    % \kt{Introduce gradient descent.}

    % \kt{Why using gradient descent}


    
    
    
    % We present a suite of techniques to further reduce the cost of camera-side compute, network bandwidth and GPU compute.


% Operators can use \name to tune a wide range of knobs that influences DNN input (as shown in Table~\ref{tab:rich-set-of-knobs}).
% That said, \name does {\em not} apply to knobs that alter the DNN itself, 
% such as retraining the DNN weights~\cite{ekya,noscope,mcdnn}.
% Similar to \name, they also adapt to changes in input distribution, they involve substantial computation and thus tend to happen at a coarser timescale than the knobs considered in \name. 




In short, the contributions of this paper are two-fold:
\begin{packeditemize}
    \item Design of \name, a new configuration-adaptation system that runs gradient ascent based on fast computation of \outputgrad.
    % \name's gradient-ascent-based search.
    \item Implemented a prototype of \name and integrated it with a benchmark of 9 DNN applications (which cover 5 data types, 4 analytic tasks, and 5 configuration knobs). \name achieves similar accuracy while reducing resource usage by 15-59\% or improves accuracy by 1-5\%  with the same or less resource usage when compared to state-of-the-art adaptation heuristics. 
\end{packeditemize}




\textbf{This work does not raise any ethical issues.}
    
    

    % \kt{2. Given 2 DNN output to estimate accuracy change (talk about golden config)}
    % \kt{quantify the overhead of not using saliency (maybe say multiple macroblocks)} \kt{Explain the difference between OneAdapt and prior work, especially compares with AccMPEG, compare saliency}
    % \kt{How to predict the second DNN output based on the first DNN output}
    
    % \item However, previous work would have had to calculate the gradient of accuracy in the following two steps:
    % \begin{packeditemize}
    %     \item First, obtain the inference results of a golden configuration as a reference point to calculate accuracy.
    %     \item Second, calculate the gradient of accuracy with respect to each knob (\ie temporarily increase the value of one knob, run DNN inference to get the inference results of changed config, calculate the change of accuracy divided by the change of knob value, and repeat this process for other knobs),\jc{i don't get this sentence at all. and this seems secondary to me}
    % \end{packeditemize}
    % where both steps requires extra DNN inference.
    % % \begin{packeditemize}
    % % \item calculating the change of accuracy by alternating the value of one knob in the current configuration while keeping the values of other knobs fixed,
    % % \item dividing the change of accuracy by the change of the knob value,
    % % \item repeating this process for all knobs,
    % % \end{packeditemize} resulting in extra DNN inference on both the golden config (in order to obtain a reference inference results to calculate the accuracy) and the configs nearby the current config.

    % \item To reduce the overhead of the first step (obtain the inference results of a golden configuration as a reference point), we leverage the inference results of the current configuration as a reference point to \textit{estimate} the accuracy of other configurations.
    % Concretely, the accuracy change of other configurations compared to the current configuration is proportional to the corresponding inference results change: if there is no inference results change, there is no accuracy change; if there is a large inference results change, the accuracy change also tend to be large.
    % \kt{Empirical numbers to back it up}

    % \item To reduce the overhead of the second step (running DNN inference to calculate the change of inference results), we can split the change of inference results into two parts. Specifically, we can calculate the inference results change by
    % \begin{packeditemize}
    %     \item calculating the DNN input change (No need for GPU), and 
    %     \item calculating how the DNN input change affects inference results (note that this term corresponds to the \textit{gradient} of the inference results wrt DNN input and can be calculated using one single backpropagation)
    % \end{packeditemize}
    % \kt{Empirical numbers to back this up.}

    % \item 
    % By integrating these two techniques together, one can estimate \accgrad without extra DNN inference and with constant GPU overhead (caused by backpropagation).
    % We present \name, a configuration adaptation system that adapts the configuration by \accgrad.

    % \item Compare \name against region-proposal-based approach and saliency-based approach.

    % \item Experiment result highlight.
    

    
    
    % Our insight comes from an empirical observation: 
    % Mathematically, this insight can be restated as: the mapping between the configuration and its corresponding accuracy is \textit{concave}.
    % By using gradient, we can leverage this concavity to quickly converge to the configuration with highest accuracy under the resource budget.
    
    
    % This is because gradient leverage an important structure in the configuration to efficiently skip those configurations that generate low accuracy.

    % \item 

    % % 1. better config --> locally better config
    % % 2. one knob --> 
    % % 3. multi-knob --> 
    % \item To calculate the gradient of accuracy with respect to each individual knobs, we state an observation. If we increase the value of just one knob:
    % \begin{packeditemize}
    % \item The resource consumption will increase (or decrease)
    % \item The corresponding inference results will become more (or less accurate)
    % \item more change in the inference results, more accuracy improvement (or degradation)
    % \end{packeditemize}
    % % This assumption allows us to quickly check if a different config (that differs from the current config on only one knob) has much higher accuracy: we only need to check if the config consumes more resource and if the inference results are highly different.
    % This assumption allows us to estimate the \textit{gradient} of accuracy wrt each knob.
    % Concretely, we estimate the gradient of accuracy wrt each knob by temporarily increasing that knob a little and checking the inference results difference and resource usage.
    


    % \item 
    % Based on this assumption, we propose a basic version of our proposal: BaseAdapt.
    % Every 1/3 seconds \kt{need to defend 1/3 second}, BaseAdapt will calculate the \accgrad of nearby configs by performing the following steps for each knob:
    % \begin{packeditemize}
    %     \item 
    %     Temporarily increase and decrease the value of the designated knob, obtain their inference results on this 1/3-second video and estimate the accuracy.
    %     Temporarily increase the value of the designated knob in the current config by 1 and obtain the inference results on the 1/3-second video
    %     \item Calculate the change of inference results (before and after increasing the knob value) and estimate the change of accuracy based on the change of inference results,
    % \end{packeditemize}
    % estimate the accuracy change of nearby configs based on the accuracy change of increasing each knobs (a forward pointer here) and then select the config in nearby configs that yield high accuracy within the resource budget.

    % \item 
    % This algorithm can frequently adapt by probing only a small subset of configurations (instead of profiling the whole config space like in profiling-based approach).
    % One may worry that BaseAdapt may converge slowly (as BaseAdapt may stuck in a local optimal, and the optimal config may not be in nearby configs).
    % That said, empirically we find that our solution can still quickly converge to the optimal config. 
    % This is because the locally optimal config only appears occasionally and does not persist, so it is less likely to stuck in a locally optimal config for a long time.
    % Also, it typically takes only 3 - 4 steps to go from the current config to adapt to the optimal config.
    % Empirical evidence here to support these points.
    % Advantage: Avoid the extra overhead caused by evaluating golden config and adaptation is much more frequent (once every 1/3 second) \\
    % Disadvantage:  a lot of extra DNN inference.


    % \item Solve the first issue. Insight: gradient

    % \item Solve the second issue. Insight: gradient decoupling.

    % \kt{propose gradient as a way to reduce the camera-side overhead.}
    
    % Changing the value of one single knob will result in consuming more (or less) resources the inference results would statistically become more (or less) accurate. The accuracy improvement (degradation) is proportional to how much the inference results changed.
    

    % \item
    % We assume that: if a config differs with the current config on \textit{just one knob}, 
    % \begin{packeditemize}
    % \item whether this config has higher accuracy or not depends on whether it has higher resource usage or not.
    % \item the absolute accuracy difference compared to the current config is small when the inference results of this config is small, and vise versa.
    % \end{packeditemize}
    % We empirically evaluate this assumption across a wide range of knobs. 

    % \item
    % The technique above allows us to make 
    

    

    % \item Our insight is that: if there is a config with higher accuracy under the budget
    % there is a config with higher accuracy nearby and we can find this config by merely checking its output.

    
    


    % \kt{Observation: check output to tell accuracy change}
    % \kt{Why better than profiling: 1. frequent 2. 3-4 steps to optimal 3. local optimal is not an issue}
    % \kt{Why better than heuristics: when there exist a config that has higher ACC under the budget, our approach can quickly converge to that config.}
    % However, heuristics do not leverage DNN input.  bounded by their compute, may not be able to find this optimal config
    % while there are cases where heuristics cannot identify such change and may still leverage a suboptimal config
    % config with lower accuracy due the compute limit of their heuristics (a pointer to illustrate why these work generate poor config)}

    
%     \item  Profiling-based.
%         Profiling-based approach leverages the inference results of golden configuration (the most resource-consuming configuration\footnote{Chameleon\cite{chameleon} uses multiple configurations as the reference point to estimate accuracy}) to estimate the accuracy of different configurations.
%         However, \textit{before} calculating the accuracy of different configs, this approach needs to spend extra bandwidth and compute to stream video to the server and run extra DNN inference.
% %         \begin{packeditemize}
% %         \item stream  video to the server
% %         \item spend extra inference to analyze golden configuration 
% %         % \jc{these two points are not separate. just say they use golden config but it takes more bandwidth and compute}
% %         \end{packeditemize}
%         Thus, when the resource (in terms of banwidth and/or GPU compute) is limited, this approach needs to profile less frequently, resulting in using outdated configurations when the optimal configuration has drifted away
%         % , or  significantly prune the search space (which may contain only suboptimal configurations).
%         % estimate the accuracy of a configuration by running {\em extra inference with much more expensive} configurations and comparing their inference results. 
%         % the difference with the inference results of the most expensive configuration 
%         % need extra inference to handle multiple knobs.
%         \kt{here we need to talk general solutions in this space}
%         \kt{The alternative should be something that use few configs}
%         \item 
%         Server-side configuration selection.
%         Existing design selects which regions need to be encoded in high quality based on bounding boxes (region proposals or detections) generated by the DNN to identify which regions need to be encoded in higher quality --> may miss regions critical to improving inference results but far from {\em any} bounding box --> selecting suoptimal regions
        
%         \item 
%         Sensor-side configuration selection.
%         Sensor-side has limited compute power --> relatively simple logic --> selecting suboptimal configuration
%         \kt{People may think of model cascading}
        % : the camera-side heuristics is inaccurate due to the compute limit of camera.
        % : the server-side region proposal is inaccurate since it use bounding box as the unit to assign resource.
    % \end{packeditemize}
    
    % \kt{bring cost considerations in the limitaion instead of saying "frequent"}
    % \kt{Get a sense of how other configurations is working --> condition change we cannot calcu}
    % \item 
    % The research question of this paper is: how to compare the current config with other configurations without extra inference?
    % \item 
    % These three lines of work share one common limitation: they cannot frequently and precisely estimate the accuracy of  different configurations.\\
    % Profiling-based approach --> need to stream uncompressed video and evaluate golden config --> accuracy estimation not frequent enough.\\
    % Configuration selection --> accuracy estimation not precise enough --> wrongfully estimate the accuracy of a different configuration and thus choose suboptimal configuration
    
    
    
    % \item 
    % We takes an alternative approach: instead of estimating the accuracy of \textit{all} configurations, we estimate the accuracy of a \textit{subset} of configurations that are close\kt{need to define what is ``close''.} to current configuration (we call this subset of configurations \textit{nearby configurations}).
    
    % Our insight is that we can rely on the current configuration (instead of the golden configuration) to anchor the accuracy of these nearby configs.
    % Concretely, if the inference results change \textit{for a certain amount}\kt{a pointer here that points to how to calculate this amount} from the current config to a nearby config, the absolute change of accuracy tends to also be proportional to this amount. We then identify whether the accuracy improves or drops by whether the nearby config consumes more resource or not.
    % A measurement to support this point: the linear correlation coefficient between accuracy and inference results change is greater than 0.7 in nearby configs
    
    
    
    % \item 
    % This insight inspires a basic version of our proposal: BaseAdapt.
    % Every 1/3 seconds \kt{need to defend 1/3 second}, BaseAdapt will estimate the accuracy of nearby configs by performing the following steps for each knob:
    % \begin{packeditemize}
    %     \item Temporarily increase the value of the designated knob in the current config and obtain the inference results on the 1/3-second video
    %     \item Calculate the change of inference results (before and after increasing the knob value) and estimate the change of accuracy based on the change of inference results,
    % \end{packeditemize}
    % estimate the accuracy change of nearby configs based on the accuracy change of increasing each knobs (a forward pointer here) and then select the config in nearby configs that yield high accuracy within the resource budget.
    % Advantage: the adaptation is frequent (once every 1/3 second) \\
    % Disadvantage: the profiling overhead is significant: the profiling overhead already consumes more than 50\% of the resource when adapting just one single knob. Moreover, this overhead is proportional to the \# of knobs, making this solution impractical.
    
    % \item 
    % To reduce the overhead, we optimize the most resource-demanding operation in BaseAdapt: calculate the change of inference results.
    % Our insight is that we can split the change of inference results to two parts. Specifically, we can calculating the inference results change by
    % \begin{packeditemize}
    %     \item calculating the DNN input change (No need for GPU), and 
    %     \item calculating how the DNN input change affects inference results (note that this term corresponds to the \textit{gradient} of the inference results wrt DNN input and can be calculated using one single backpropagation)
    % \end{packeditemize}
    % Calculating the change of inference results in this way reduces the overhead of BaseAdapt by more than 100x as it no longer requires extra DNN inference and only requires one single backpropagation.
    % Based on this optimization, we propose \name.
    
    % \item We propose a suite of techniques to further reduce the overhead of \name.
    
    % \item Claim that \name does not work for DNN knobs. 
    
    % \begin{packeditemize}
    %     \item We may stuck into a local optimal
    %     \kt{Yes, but not frequently, rationale: local optimal won't persist}
    %     \item The adaptation speed of our approach may be slow: it may take several steps to approach to the optimal.
    % \end{packeditemize}
    % \kt{empirically, current config -> optimal only takes 3-4 steps}
    % \kt{say that the overhead of BaseAdapt is significant (compared to normal inference/profiling-based approach)}
    
    % \item
    % How to calculate this difference with low overhead?
    % Our insight is that 
    
    % The issue of just knowing such information is that one may stuck into a configuration that has highest accuracy among nearby configurations.
    
    % This information is enough for an adaptation system to approach the optimal, as there is no stable local optimal in the configuration space within a given resource budget.
    % For those configurations that does not hit the resource budget, we ca
    
    
    % Profiling-based approach estimate accuracy with extra streaming and inference overhead, 
    % Configuration search can generate optimal configuration at the cost of streaming uncompressed video and , while configuration generation may constantly generate suboptimal configuration.
    % generating new configuration  new configuration may generate suboptimal configuration, 
    
    % --- extra inference is too expensive, simple heuristics not accurate enough, server-side feedback too coarse-grained.
    % estimating the accuracy by obtaining the inference results of the most expensive configuration as the ``ground-truth''.
    % 2. handling multiple knobs by either running extra inference or relying on inaccurate heuristics
    % \item To handle the first limitation, our insight is that: estimating the effect of changing the config on inference accuracy can be estimated without running expensive extra inference. 
    % specifically, the change of inference accuracy can be measured by the change of inference results.
    % If there is no change in inference results, the inference accuracy also does not change.
    % If the inference results change significantly, the accuracy change also tends to be significant.
    % We then infer whether the accuracy improves or not by whether the new config consumes more resource or not.
    % \kt{A jump here.}
    % Essentially, we can quickly calculate the {\em gradient between the change of a SINGLE config knob and  change of the DNN inference accuracy} by changing that knob and running one extra inference.
    % \kt{How does that help in terms of getting the accuracy w/ extra inference}
    % \kt{1. Why is nearby OK (local optimal) 2. not referring to the golden configuration (what enables us to quickly calculate the gradient)}
    % \kt{Golden configuration?? Nearby?? Gradient??}
    % \kt{??How to move to the optimal configuration as fast as possible?}
    % (some statistical evidence!)
    % while estimating the absolute number of accuracy requires the ``ground truth'', estimating the accuracy change when changing the current configuration to another configuration does not, as we can estimate the magnitude of accuracy by looking at the change of the output, and estimate the sign of accuracy change by whether the configuration consumes more resource or not.
    % \item This way of estimating the accuracy change via output change is not generally accurate. 
    % For example, there may be one configuration that the output changes a lot compared to the current configuration, but the accuracy of these two configurations are the same.
    % However, we find that this approach is statistically accurate when we only consider those configurations that only alters one knob compared to the current configuration.
    % \item 
    % \kt{Why does it work? Monotonicity}
    % this insight inspires a basic version of our proposal: BaseAdapt.
    % % We propose a solution BaseAdapt based on this insight. Once 
    % every $k$ frames, BaseAdapt will change each config knob by a small amount, estimate its change on inference accuracy, and change the config knobs in the direction that maximizes the inference accuracy within a resource budget. 
    % \item 
    % \kt{Why baseadapt is inefficient}
    % BaseAdapt frequently adapts the configs (every $k$ frames) --> it reacts to sudden changes in the input earlier and converges to a close-to-optimal config faster than existing solutions. 
    % BUT BaseAdapt does NOT handle more config knobs efficiently. 
    % \item our full solution OneAdapt can quickly calculate the {\em gradient between the change of a MULTIPLE config knob and  change of the DNN inference output.}
    % Specifically, we SPLIT this gradient to two parts: 
    % (1) calculating the output change by first calculating the DNN input change (No need for GPU), and 
    % (2) calculating how the DNN input change affects DNN output (one single backpropagation regardless of the \# of knobs).
    % both inference on the current configuration $c$ and all configurations that are close to $c$ (\ie the configurations that differs with $c$ on only one knob with the difference value smaller than a threshold), and then move to the closest configuration.
    % \item We find that this solution is better than the baseline when there is only one knob. However, the performance of this solution is suboptimal when there are multiple knobs, as calculating the change of output with respect to every knob requires extra inference to handle multiple knobs simultaneously (the second limitation).
    % To reduce the overhead caused by extra inference, we calculate the change of output by leveraging the differentiability of the DNN.
    % Specifically, we can calculate the output change by first calculating the DNN input change, and then calculating how the DNN input change affects DNN output.
    % The former can be calculated without accessing the DNN (thus requires no extra inference), and the latter can be calculated using backpropagation
    % \item With this insight, we present OneAdapt, a solution based on BaseAdapt that calculates the output change by leveraging the differentiability of the DNN.
    
    % Evaluation: across 4 types of data sources and 3 applications, \name achieves \fillme\% more throughput without hurting accuracy, or increases accuracy by \fillme\% with similar throughput.



% \tightsection{Introduction}
% % Deep-neural-network-based (DNN-based) analytics on data streams (\eg video
% % streams or LiDAR feeds) are everywhere.
% % For example, people leverage DNNs to analyze traffic video feeds for traffic monitorings~\cite{trafficvision, traffictechnologytoday, goodvision,intuvisiontech, vision-zero, msr}, analyze the information from multiple types of sensors (including camera, LiDAR and Radar sensors) to enable long-range vehicle and pedestrian detection for autonomous driving~\cite{tusimple,waymo,motional}.
% % The input data stream varies a lot over time.
% % For example, in autonomous driving, the number and the moving speed of vehicles and pedestrians varies a lot over time (\eg the number of vehicles and humans will be much higher when driving in daytime), areas (\eg the vehicle movement speed is much higher when driving in the highway), current location (\eg the number of pedestrains will be much higher at the crossroad), traffic condition (\eg the number of vehicles significantly increases in traffic congestion).
% % \jc{highlight the need for tuning configuration knobs when you bring up "data stream varies over time"}
% % This trend inspires system research for these applications~\cite{vigil,glimpse,mcdnn,videostorm,noscope,neurosurgeon,awstream,chameleon,focus,adascale,filterforward,vstore,cracking,dds,reducto,blazeit,yoda,vcm,elf,ekya}.
% % % \jc{can we cite some dnn-based analytics systems use cases, where the input distribution varies over time, in terms of frequency of object occurrences, shape/size, etc? be as concrete as possible please} \kt{done}

% % Deep-neural-network-based (DNN-based) analytics on data streams (\eg video
% % streams or LiDAR feeds) are everywhere.

% \kt{Rewrote this para.}
% Many applications send data streams to DNNs for analytical purposes.
% % Many applications rely on DNNs to perform accurate inference on various data streams (\eg video streams or LiDAR feeds).
% For example, DNNs are used to analyze traffic video feeds to monitor vehicle speed and spot traffic jams~\cite{trafficvision, traffictechnologytoday, goodvision,intuvisiontech, vision-zero, msr} , and analyze data streams from infrared cameras, LiDAR sensors, and radar sensors to detect vehicles and pedestrians for autonomous driving~\cite{tusimple,waymo-blog,motional}.
% % \jc{kuntai, the logic here is quite muddy.. it's unclear why content varying over time is interesting/important. 
% % maybe try a different flow: as these DNN-based applications require high accuracy, they use a great amount of compute and network resource. 
% % Many prior efforts have leveraged a common feature of these data streams: their content varies greatly over time. 
% % For example...
% % To leverage these opportunities, recent work exposes...
% % }
% As these DNN-based applications require high accuracy, they use a great amount of GPU compute and/or network resources, which makes DNN-based applications too expensive for people to afford\kt{citation here}.
% Fortunately, many prior efforts identify a resource-saving opportunity: the content of the data stream varies a lot over time and some of the content allows these applications to generate accurate analytic results with \textit{much less} resource usage.
% % (\ie the amount of resource required to provide accurate analytic results) varies alongside with the content of the data stream, and reduce the resource usage by using less resource when resource demand is low.
% % To reduce the resource usage, many prior efforts identifies the variability of the content of the data stream.
% % a common characteristic of these data streams---their contents vary greatly over time---to reduce the resource usage of these DNN-based applications.
% % The content of these data streams vary greatly over time.
% % For example, in autonomous driving, the number and the moving speed of vehicles are constantly changing over time (\eg the number of vehicles will be much higher compared to driving in night time), location (\eg cars move faster on the highway) and traffic condition (\eg the number of vehicles significantly increases in traffic congestion).
% % For example, in dashcam video streams, the number and the moving speed of vehicles are constantly changing over time (\eg the number of vehicles will be much larger during daytime than during night), location (\eg cars move faster on the highway) and traffic conditions (\eg the number of vehicles significantly increases in traffic congestion).
% % For example, in one traffic video stream that aims to localize vehicles on a traffic lane,
% For example, in a traffic video stream, the moving speed of vehicles can be much lower during red traffic light compared to green traffic light, so one can analyze less frames during red traffic light (and thus save GPU compute resource) and still accurately capture the motion of the vehicles.
% % \jc{highlight the need for tuning configuration knobs when you bring up "data stream varies over time"}
% % Facing this trend, the system research community develop \textit{adaptation-required knobs} to \textit{enable} saving resources when the data can be safely analyzed by using less resource without hurting accuracy and timely \textit{adapt} these knobs to save resource when such data appears. ~\cite{vigil,glimpse,mcdnn,videostorm,noscope,neurosurgeon,awstream,chameleon,focus,adascale,filterforward,vstore,cracking,dds,reducto,blazeit,yoda,vcm,elf,ekya}.
% % To save resources through such temporal variability in the data streams,
% Technically, to capture such resource-saving opportunity,
% recent proposals~\cite{vigil,glimpse,mcdnn,videostorm,noscope,neurosurgeon,awstream,chameleon,focus,adascale,filterforward,vstore,cracking,dds,reducto,blazeit,yoda,vcm,elf,ekya} expose internal tunable parameters (referred to as \textit{knobs}) and \textit{timely configure} these knobs (we denote the knobs together with their configured values as a \textit{configuration}) according to the content of the data streams to save resources (\eg GPU compute and network) while maintaining high inference accuracy.
% % \jc{can we cite some dnn-based analytics systems use cases, where the input distribution varies over time, in terms of frequency of object occurrences, shape/size, etc? be as concrete as possible please} \kt{done}



% % \jc{how about we pitch them as two parallel trends: (1) temporal variation of input, and (2) an increasingly number of knobs, $\rightarrow$ the challenge of timely adaptation in a large configuration space.}

% % We observe that these systems expose an \textit{increasing} number of internal knobs.
% % The underlying trend that drives this increase is two-fold (further discussion in \S\ref{subsec:numer_of_knobs}). 
% % % First, these systems need to develop new knobs to not only provide accurate analytic results under all kinds of resource budget due to heterogeneous deployment settings, but to also handle new emerging applications (\eg LiDAR-based object detection for autonomous driving and infrared-based human detection for night-time security monitoring).
% % First, these systems need to develop new knobs to not only trade-off between the accuracy and different kind of resources in order to handle all kinds of resource budget due to heterogeneous deployment settings, but to also handle new emerging applications (\eg LiDAR-based object detection for autonomous driving and infrared-based human detection for night-time security monitoring).
% % \ga{It'll be helpful to make it explicit that knobs also regulate the resource demand and hence can be used to handle heterogeneous resource budget.}
% % \kt{fixed}
% % % These knobs trade-off between accuracy and different kinds of resource in order to
% % Second, as the need of DNN-based analytics quickly grow, these systems need to tune existing type of knobs at a finer granularity to support more concurrent DNN-based analytic jobs. \ga{The need to partition isn't clear. Why were the knobs joined in the first place, before partitioning?} \kt{fixed}

% We observe that there is already a broad set of knobs\footnote{Previous work proposes at least 16 knobs includes 6 video encoding knobs~\cite{vstore, chameleon, dds, videostorm, awstream}, 9 frame filtering knobs~\cite{reducto, vigil, glimpse}, and the knobs that differentiate spatial video quality knob~\cite{dds,accmpeg,eaar}, which can be partitioned into thousands of knobs if tuned in fine granularity~\cite{accmpeg}.}\cite{vstore,chameleon,dds,videostorm,awstream,reducto,vigil,glimpse,dds,accmpeg}, 
% and the set is still growing, thanks to two trends.
% % We observe that the number of such configuration knobs is already huge (\eg more than 16 different knobs\footnote{These 16 knobs includes 6 video encoding knobs~\cite{vstore,chameleon,dds,videostorm,awstream}, 9 frame filtering knobs~\cite{reducto,vigil,glimpse}, and the knobs that differentiate spatial video quality knob~\cite{dds,accmpeg}, which can be partitioned to thousands of knobs if tuned in a fine granularity.} are introduced in video analytic systems~\cite{vstore,chameleon,dds,videostorm,awstream,reducto,vigil,glimpse,accmpeg}) and is still expanding.
% % We observe that these systems expose an expanding set of configuration knobs that leverages temporal variabilities in the data stream to save resource without hurting the accuracy.
% % % be adapted to the temporal variations of the input data stream to save resource.
% % There are two reasons behind this trend. 
% % First, these systems need to develop new knobs to not only provide accurate analytic results under all kinds of resource budget due to heterogeneous deployment settings, but to also handle new emerging applications (\eg LiDAR-based object detection for autonomous driving and infrared-based human detection for night-time security monitoring).
% First, when people deploy DNN-based analytic systems into practice, they found that these systems need more knobs to explore new resource-saving opportunities introduced by new types of data streams (\eg LiDAR feeds), new applications (\eg video captioning) and new deployment settings (\eg multi-camera video analytics~\cite{chameleon, vigil}, multi-server video analytics~\cite{elf}).
% % First, these systems need more knobs to not only trade between different type of resources to fit into more deployment settings (\eg the user may stream the data out from cheap camera through expensive LTE network for analytics. In this case, it is more ideal for the system to trade server-side compute for bandwidth~\cite{dds,eaar} instead of trade camera-side compute for bandwidth~\cite{vigil,glimpse,accmpeg} to simultaneously reduce the bandwidth usage without  the camera-side compute usage), but to also 
% % \ga{It'll be helpful to make it explicit that knobs also regulate the resource demand and hence can be used to handle heterogeneous resource budget.}
% % \kt{fixed}
% % These knobs trade-off between accuracy and different kinds of resource in order to
% Second, as these systems need to run more analytic jobs than before,
% % these systems need to support more concurrent analytic jobs under the same resource budget, which requires them to 
% they need to tune existing knobs at a finer granularity (by partitioning existing knobs into \textit{multiple} fine-grained knobs) to further reduce the resource usage of each analytic job.
% % further reduce the resource demand for running one analytic job without hurting the accuracy.
% For example, in a dashcam video stream, when the input video contains \textit{only one} small object, one may need to encode \textit{the whole video} in high fidelity in order to make this object detected, resulting in high bandwidth usage~\cite{chameleon,awstream}.
% % when the input video contains one small object, one may need to encode and stream the whole video into high resolution to detect such object, resulting in high bandwidth usage~\cite{chameleon,awstream}.
% However, prior effort~\cite{dds,eaar,accmpeg} shows that the areas that are not related to the object can be encoded in low fidelity to save bandwidth and realizes this potential by \textit{partitioning} the video into different areas and assigning different areas with different fidelities.
% % , by assigning different areas with different resolutions\footnote{In fact, prior work assigns different areas with different quantization parameters, a parameter that controls the fidelity of the encoded video without changing the resolution. We use resolution in the text for understandability consideration.}, it only needs to encode the area that contains the object into high resolution and other areas can be safely encoded in low resolution. This significantly reduces the bandwidth usage.

% % % redirected enumerate to packedenumerate for reformater in macro.tex. DON'T
% % % CHANGE!
% % \begin{enumerate}
% %   \item 
% % As DNN-based analytics are deployed on heterogeneous deployment settings that have different types of resource budgets, this requires the corresponding systems to propose new knobs in order to fit into
% % different resource budgets. Take video analytics as an example. If the
% % user analyzes the video feeds locally by a compute-constrained mobile
% % phone, the main focus for the systems is to fit into the compute budget
% % of the phone (\eg by skipping those frames that are highly similar to
% % their previous frames~\cite{reducto,glimpse}). However, if the user
% % instead streams the video feeds to a GPU-equipped server through a
% % bandwidth-limited LTE network, the main focus is instead fitting into
% % the limited LTE bandwidth (\eg by performing video
% % compression~\cite{accmpeg,vigil,glimpse,reducto}).

% %   \item As DNN-based analytics quickly expand, the corresponding systems need to
% %         partition existing knobs into more fine-grained version to capture more
% %         resource-saving opportunities. Take video-based vehicle detection as an
% %         example. Chameleon~\cite{chameleon} and AWStream~\cite{awstream}
% %         identify that the system only need to encode the video in a high
% %         encoding quality when the vehicle appears. To further explore the
% %         potential of varying video encoding quality, the following
% %         work~\cite{dds,eaar,accmpeg} finds that a lot of areas in the video do
% %         not need to be encoded in high quality (\eg the areas that contain
% %         non-vehicle-related backgrounds like trees and buildings) and proposes
% %         fine-grained spatial encoding quality to capture this opportunity.
% %   \item Since new applications quickly emerge (\eg LiDAR-based object detection,
% %         Infrared-based human detection \kt{a bunch of citations here}), this requires the deep learning systems
% %         to develop new knobs (or even developing new system components) to fit
% %         into the need of different applications. For example, in order to handle
% %         LiDAR data, people are proposing new encoding standard and new
% %         knobs~\cite{MPEG-point} to efficiently encode and process LiDAR data.
% %         \roy{I understand you are trying to distinguish old types of application
% %         and new ones, but I still feel the first and third items are kind of
% %         repetitive? Both items are trying to say there is the need for new
% %         knobs, right? Maybe merge them into one?}
% % \end{enumerate}

% % Not only the number of knobs are already huge (\eg in video analytics, previous work introduces 6 video codec encoding knobs~\cite{vstore,chameleon,dds,videostorm,awstream}, 9 frame filtering knobs~\cite{reducto,vigil,glimpse} and even thousands of knobs for fine-grained video encoding quality assignment~\cite{accmpeg}) and still expanding
% % % \ga{Quantify.}
% % , these knobs also need to be timely adapted~\cite{awstream,chameleon,dds,eaar,elf} due to input data change or resource budget change in order to achieve high inference accuracy.
% % Thus, the research question is: how to navigate the large configuration space (\ie all possible choices of knob values) and and pick the optimal configuration that generates accurate inference results under the current resource budget?


% % As the number of knobs are already huge (\eg more than 16 different knobs\footnote{These 16 knobs includes 6 video encoding knobs~\cite{vstore,chameleon,dds,videostorm,awstream}, 9 frame filtering knobs~\cite{reducto,vigil,glimpse}, and the knobs that differentiate spatial video quality knob~\cite{dds,accmpeg}, which may include thousands of knobs if tuned in a fine granularity.} are introduced in video analytic systems~\cite{vstore,chameleon,dds,videostorm,awstream,reducto,vigil,glimpse,accmpeg}) and is still expanding,
% % \ga{Quantify.}
% % , these knobs also need to be timely adapted~\cite{awstream,chameleon,dds,eaar,elf} due to input data change or resource budget change in order to achieve high inference accuracy.
% Given the \textit{large yet expanding} set of knobs, the research question of this paper is:
% \textit{among a large number of configurations, how to quickly adapt to optimal configuration that achieves high accuracy under a given resource budget?}


% The first way to address this problem is to frequently profile different configurations to obtain their resource usage and accuracy, and then pick the configuration that yeilds high inference accuracy without exceeding the resource budgets\cite{chameleon,awstream,vstore,videostorm}.
% % meets the resource
% % budget and generates the most accurate inference results
% However, each profiling
% needs to run \textit{extra} inference to analyze multiple configurations (some are expensive in terms of resource usage). %before obtaining the profile.
% % As a result, when the optimal configuration changes, this approach need to perform the extra inference to obtain the new optimal configuration, thus incurring high delay when the GPU resource is limited.
% Thus, when the GPU compute is limited, this approach needs to either profile less frequently, resulting in using outdated configurations when the optimal configuration has drifted away, or significantly prune the search space (which may contain only suboptimal configurations). %profile fewer configurations, which may miss the optimal configuration. 
% % Both of them lead to a sub-optimal trade-off between the accuracy and the resource usage.
% % \ga{Call out the downsides of extra inference.} \kt{fixed}









% % \kt{This para needs a rewrite}
% % The other approach performs no extra inference and instead, computes the
% % configuration based on recent DNN outputs (including intermediate outputs) through cheap heuristics~\cite{dds,eaar,elf} or through DNN-based configuration generator~\cite{accmpeg,casva}). 
% % \ga{What does ``derives the configuration'' mean?} \kt{fixed}
% % % However, there can be many configurations that meet the resource budget. \ga{There has been no mention of budget so far.}
% % % Without profiling most of them, it is difficult to separate the configurations that yield similar DNN output from those that yield more accurate DNN output by merely looking at recent DNN outputs.
% % % As a result, this approach waste resource on those configurations that yield similar DNN output and thus cannot quickly adapt to the optimal configuration. 
% % \ga{I don't fully follow this paragraph and it needs more explanation. That said, can I view the techniques in this paragraph as a pruning mechanism to identify the promising configurations?}
% % \kt{This para needs a rewrite}
% \kt{rewrote the next 3 paras}
% The second approach~\cite{dds,eaar,elf} performs no extra inference and instead generate new configuration by leveraging region proposal (DNN-generated bounding boxes that may contain objects inside).
% For example, based on the region proposal of the current frame, EAAR~\cite{eaar} encodes the bounding boxes inside the region proposal of the current video frame  in higher encoding quality on future frames so that the objects inside the region proposals are more likely to be detected.
% However, this approach may generate sub-optimal configuration, as this approach assigns the \textit{same} configuration (\eg encoding quality~\cite{dds,eaar}) for all the pixels inside each bounding box (unless multiple regions overlap) while an optimal configuration may assign \textit{different} configuration for different pixels inside a bounding box.
% For example, \kt{plot a figure here.}
% % This is sub-optimal as some pixels inside the bounding box can be in lower encoding quality (\eg those pixels that are outside the object but inside the region) and some pixels outside the bounding boxes may require higher encoding quality.
% % However, instead of comparing between different configurations, this approach generates new configuration by postprocessing region proposals.
% % As a result, it can only explore those configurations that are generatable from the heuristics, which may miss the optimal configuration that may not be generatable from the heuristics.
% % For example, EAAR~\cite{eaar} encodes the regions inside the region proposals with higher encoding quality so that the objects inside the region proposals are more likely to be detected.
% % However, as shown by AccMPEG\cite{accmpeg}, not all pixels inside the region proposal need to be in higher quality, and some pixels outside the region proposal needs to be in higher quality.





% % based on recent DNN outputs (including intermediate outputs)~\cite{dds,eaar,elf,accmpeg,casva}.
% % % \jc{i still dont quite get why we use dds here. isn't some bandit/RL-based solution a better fit?}
% % % For instance, DDS~\cite{dds} tunes encoding quality by first encoding all pixels at a low quality and streaming them to the server-side DNN, whose output (region proposal) is then used to tune the quality at different regions.
% % Though no extra inference is run, this approach tends to adapt {\em slowly}, as each DNN output reveals limited information regarding the \textit{highly complex} relationship between the configurations and DNN inference output/accuracy, due to the complexity of the DNN itself and the preprocessing modules before the DNN (\eg video codecs).
% % We take EAAR~\cite{eaar}, a system for video object detection, as an example.
% % EAAR adjusts the video encoding quality by collecting the regions from the DNN that may contain objects of interest and encoding these regions in higher encoding quality on future video frames.
% % % After that, it encodes these regions in high quality on the next video frame.
% % Thus, the objects inside these regions are much more likely to be detected.
% % % This approach then lets the sensor encode all these regions in high encoding quality on the next video frame so that the objects inside these regions can be accurately detected.
% % However, as the regions generated by the DNN may not include all the regions that contain the objects, the object detection DNN may miss some objects and thus EAAR needs to further adjust the regions corresponding to these missing objects.
% % For instance, the impact of configuration on DNN accuracy is affected by two complex blackboxes: DNN itself as well as the video codecs.
% % However, the \textit{adaptation speed} (\ie the time it takes to obtain the optimal configuration) of this approach can be slow.
% % For example, DDS~\cite{dds} tunes the encoding quality of different areas of the video in the following steps.
% % First, DDS let the camera encode the whole video into low quality and stream it to the server.
% % The server then analyzes the video to obtain the areas that may contain objects and let the camera resend those areas in high encoding quality for an extra round of inference.
% % % through cheap heuristics~\cite{dds,eaar,elf} or through DNN-based configuration generator~\cite{accmpeg,casva}).
% % However, the \textit{adaptation speed} (\ie the time it takes to obtain the optimal configuration) of this approach can be slow.
% % % explore many configurations to accumulate enough DNN outputs before converging to the optimal one.
% % % need to accumulate enough DNN outputs in order to obtain the optimal configuration.
% % % This is because this approach only examine one configuration at a time.
% % This is because they only get one DNN output at a time.
% % As the relationship between the configuration to the inference accuracy is highly complex (due to complexity inside the underlying system (\eg video codec) and the DNN itself), this approach needs to spend time accumulating enough DNN outputs before obtaining the optimal configuration, resulting in slow adaptation speed.
% % Thus, it is difficult to identify whether a new configuration improves accuracy or not based on the current DNN output.
% % the performance of other configurations.
% % the DNN ouput on just one configuration is not enough for this approach to immediately obtain the optimal configuration thus
% % As a result, 
% % this approach needs to accumulate enough DNN outputs to reach the optimal configuration. 
% % The optimal configuration may have already changed (due to the change of input content or resource budget) before this approach reaching it.
% % The optimal configuration may have already changed.

% % However, there can be many configurations that meet the resource budget.
% % Without profiling most of them, it is difficult to separate the configurations that yield similar DNN output from those that yield more accurate DNN output by merely looking at recent DNN outputs.
% % As a result, this approach waste resource on those configurations that yield similar DNN output and thus cannot quickly adapt to the optimal configuration. 


% Moreover, the heuristics used in the second approach are designed for specific types of knobs and are not directly applicable to other knobs (though these heuristics \textit{could} be augmented and used to adapt other knobs).
% % even if they can be purposely built to efficiently support some knobs. 
% % are hand-crafted for individual applications or configurations and thus not generalizable to other configurations and applications.
% For example, EAAR~\cite{eaar} generates new configuration of future frames based on region proposal of the current frame.
% As a result, EAAR may not be ideal for tuning, for example, determining whether to analyze this frame or not.
% This is because the optimal configuration of this frame may vary a lot compared to next frame.
% % This is because  as these knobs require the system to analyze the temporal characteristics of these frame, which are not analyzed by EAAR.
% % We take EAAR~\cite{eaar}, a system that serves object detection, as an example.
% % EAAR assigns the regions that may contain objects based on the current frame and encodes these regions with higher encoding quality to in the future frames to make more objects detected.
% % In a higher level, EAAR applies the decision generated from the current frame to the future frames.
% % However, this may not be a suitable way to adapt the knobs that, for example, decide which video frames can bypass the DNN inference.
% % This is because the optimal decision may vary a lot between the current frame and the future frames: if the current frame needs to be forwarded through the DNN, it is more likely that the next frame should bypass the DNN inference.
% % As a result, EAAR may not directly apply to the DNN-bypassing knobs.



% The third approach trains models (\eg saliency generator~\cite{accmpeg,??} or configuration generator~\cite{casva}) and leverages these models to generate new configuration.
% However, the accuracy of these models degrade over time and are not accurate enough to generate optimal configuration when the characteristics of the input data changes (\eg when a remote small object appears in the video). 
% % unless these models are as complex as the DNN and the.
% This is because the mapping between the input and its corresponding optimal configuration is highly complex due to the complexity of the DNN itself and the preprocessing modules before the DNN (\eg video codecs~\cite{h265,h264}).
% \kt{an example figure to support this point.}
% As a result, these models is not able to accurately learn this mapping (unless these models are as complex as the DNN and the preprocessing modules) and may produce sub-optimal configurations when the content of the input data shifts (\eg when a drone quickly flies away the ground), unless these models are frequently retrained, which requires extra inference to label the optimal configuration before retraining starts.
% % and then leverage this model to adapt the configuration.
% % However, as the compute of such model is limited due to \fillme, the model may no longer being able to predict the optimal configuration when the input content changes.
% % For example, \fillme.





% % Moreover, the heuristics used in the second approach are designed for specific types of knobs and are not directly applicable to other knobs (though these heuristics \textit{could} be augmented and used to adapt other knobs).
% % % even if they can be purposely built to efficiently support some knobs. 
% % % are hand-crafted for individual applications or configurations and thus not generalizable to other configurations and applications.
% % We take EAAR~\cite{eaar}, a system that serves object detection, as an example.
% % EAAR assigns the regions that may contain objects based on the current frame and encodes these regions with higher encoding quality to in the future frames to make more objects detected.
% % In a higher level, EAAR applies the decision generated from the current frame to the future frames.
% % However, this may not be a suitable way to adapt the knobs that, for example, decide which video frames can bypass the DNN inference.
% % This is because the optimal decision may vary a lot between the current frame and the future frames: if the current frame needs to be forwarded through the DNN, it is more likely that the next frame should bypass the DNN inference.
% % As a result, EAAR may not directly apply to the DNN-bypassing knobs.
% % However, EAAR may be sub-optimal if applied to the knobs that decide which video frames can bypass the DNN inference without hurting the inference accuracy.
% % This is because EAAR make an assumption that do not fit this set of knobs.
% % Concretely, the current design of EAAR generates the configuration on one frame and apply it to the future frames, which assumes that the optimal knobs on one frame generalizes to the future frames.
% % However, this assumption may not be true in the scenario of bypassing DNN inference: if one frame needs to be forwarded through the DNN, it is more likely that the next frame should bypass the DNN inference, and vise versa.
% % The violation of this assumption results in the sub-optimal adaptation behavior of EAAR: EAAR may continuously performing inference on a few frames and then continuously bypassing the DNN inference on the next few frames, while the optimal way is to perform inference intermittently.
% % This 
% % This is because making such decision requires the adaptation algorithm to analyze these frames without performing DNN inference on these frames, while the current design of EAAR lets the DNN ingest this frame first and then analyze this frame leverage the intermediate analytical results on this frame for further use.
% % performing DNN inference on this frame and then harnessing the intermediate outputs generated by the DNN inferences. 
% % As a result, EAAR either obtains no extra information on one frame besides the pixel values of this frame (thus cannot make accurate decision on whether letting this frame bypassing DNN inference or not), or analyzes this frame at the cost of performing DNN inference (thus this frame cannot bypass the DNN inference).
% % does not extract any information of one frame  while the current design of EAAR always inference on the current frame and are agnostic to the future frames.
% % making such a decision requires estimating the similarity of the inference results, between those discarded frames and reserved frames, while EAAR focusing on extracting the regions that may contain objects, where only a small subset of them will appear in the final inference results.
% % Take DDS~\cite{dds} as an example, which analyzes the video and then resends some areas of the video that may contain objects of higher fidelity.
% % As the recent areas are derived from the output of a specific DNN component (region proposal) that aims to facilitate object detection, this heuristic is not directly applicable to tasks like video classification.
% % Moreover, this heuristic does not apply to tune frame-discarding knobs~\cite{vigil,glimpse,reducto} that discard similar frames to save GPU compute, because the way DDS obtains the output to tune the knobs incur more GPU compute in the first place. 
% % the knobs in frame discarding techniques 
% % (\ie discarding the frames that produce similar inference results compared to previous frames~\cite{vigil,glimpse,reducto}) without further adjustments, since its adaptation logic (\ie resending some areas of the video that may contain objects) happens \textit{after} DNN inference while frame filtering needs to be performed \textit{before} DNN inference to save GPU compute cost. 
% % As a result, DDS does not directly generalize to other 
% % \ga{How is this paragraph on DDS pertaining to profiling and avoiding extra inference? The relationship isn't clear.} \kt{fixed}
% % \jc{not sure ganesh's comment was addressed. i think the confusion is whether you are criticizing dds's logic being inefficient or not generalizable. if it's the latter, just say it explicitly.}


% % An ideal configuration adaptation system should meet these two
% % requirements: 1. quickly adapt to optimal configuration in a large configuration
% % space without extra inference 2. minimum assumption to the underlying system.

% Therefore, an ideal configuration adaptation system needs to serve \textit{a wide range of knobs}, and compare between different configurations formed by these knobs  \textit{without extra inference}.

% % \kt{Pitch the cause of the previous work limitation as they only using DNN outputs -- which can change a lot between different configuration and video content -- to predict the performance on unknown configuration and unknown content.
% % Our approach combines the DNN parameters -- which does not change between different configuration and video content -- to better generalize the prediction of the performance on unknown configuration and unknown content.
% % }

% % \jc{i guess the rest of the intro hasn't been updated since last wednesday. just to recap, here's the flow:
% % \begin{packeditemize}
% %     \item start with a new abstraction, \accgrad, to more efficiently adapt configurations than prior schemes, especially in a large configuration space, and why?
% %     we present \name, the first efficient implementation of \accgrad
% %     we should clarify that prior work could expose this abstraction as well, but they suffer high overhead (why?). 
% %     \item \name approximates \accgrad based on two observations: 
% %     (1) the values of each configuration can be ordered in a way that \fillme, and
% %     (2) the more changes of confidence scores around the threshold, the more accuracy will change.
% %     \item based on the two observations, \name does \fillme
% %     \item operators can use \name to tune a range of configurations that influences dnn input. this class of config covers many existing systems. but notably, this doesn't cover \fillme (may point to a synergy with recent online learning papers like ekya --- in some sense, they also handle input drift, but they choose to retrain the model, and our approach is more lightweight.)
% % \end{packeditemize}}

% % \kt{Stress that knob is trading res usage for acc}
% % \kt{Adaptation goal: expose an abstraction: monitoring both }

% % \kt{
% % Expose 1 abstraction:
% % resource-knob gradient
% % DNN output (We use the change of confidence values around the threshold, see \S\ref{??} for further detail) gradient
% % % confidence change gradient
% % Say it correlates with accuracy?
% % With this gradient, we can 1). efficiently optimize knobs

% % Previous work, if repurposed, incurs extra inference.

% % Advantage: can be calculated without extra inference
% % }


% % To realize these two objectives, we expose a new abstraction: , which means the performance change divided by knobs change when changing the knobs by a little.
% % Concretely, performance gradient includes resource usage gradient, and DNN output gradient (we measure the DNN output change by measuring the absolute change of confidence scores around the confidence threshold. See \S\ref{??} for further details).


% \kt{rewrote this part}
% We advocate that the adaptation system for DNN-based analytics should expose a new abstraction: \textit{\outputgrad}, which estimates \textit{the gradient of DNN output with respect to each knob}.
% We present \name, a system that implements \outputgrad and uses it to adapt configurations with constant GPU overhead and no extra inference.
% % Based on \outputgrad, we present \name, a configuration adaptation system that implements \outputgrad with constant GPU overhead and with no extra inference.
% % Specifically, \name measures \outputgrad by how much a small change in the current value of each knob \textit{flips} the DNN-returned confidence scores from below (or above) the confidence threshold to above (or below). 
% Specifically, \name measures \outputgrad by how much a small change in the current value of each knob changes the output\footnote{We measure the change of output by summing up all values inside the output and measuring the change of the sum}.
% % We measure \outputgrad by how much a small change in the current value of each knob affects the DNN-returned confidence scores near (both below and above) the given confidence threshold.
% % Note that this measurement does not impose an extra burden on the application side since most of the applications already expose confidence scores to indicate the uncertainty of DNN outputs and use confidence thresholds to filter out DNN outputs with low confidence. %those uncertain results returned from the DNN.
% One may question that why \name studies the output of the DNN instead of the accuracy of the application.
% To answer this question, \name makes an assumption: when we \textit{only} change the value of \textit{one single knob} in a way that makes the system consume more resource, \textit{statistically} the accuracy will be improved. Moreover, more change on the output, more accuracy improvement.
% We empirically validate that this assumption over a wide range of knobs and applications (see \S\ref{??} for details).
% % We will talk about the applicability and the 
% % Moreover, more change in the output, more improvement on accuracy (see \S\ref{??} for more rationales).
% % We 
% %those uncertain results returned from the DNN.
% % Statistically, more changes in the ``near-confidence-threshold'' DNN outputs will likely cause more changes in the inference accuracy (as will be elaborated in \S\ref{subsec:correlation})\footnote{This correlation does \textit{not} assume that a confidence score always directly indicates the accuracy of its corresponding detection/classification results.}.
% % % \outputgrad correlates with how much the accuracy \textit{changes} with knobs 
% % Intuitively, this is because the confidence threshold determines whether a detection or classification result is accepted (as part of the accuracy calculation) or rejected (thus having no effect on the accuracy).
% % When the knob change only alters the DNN output by a little, the corresponding accuracy change also tends to be minor.
% % Thus, more change on the ``near-threshold'' DNN outputs, more changes on the inference accuracy.




% % how much the DNN output changes when varying each individual knob by a little (we measure the DNN output change by measuring the change of those confidence scores around the confidence threshold, see \S\ref{??} for the mathematical formulation and the intuition behind).
% % We call this metric \outputgrad for short.
% % when slightly changing the knob  (we call it \outputgrad for short).
% % We will cover the detail


% % \kt{Should we allocate a paragraph to talk about the overhead of calculating ground truth here?}
% % We acknowledge that using DNN output change cannot obtain the exact number of the accuracy change.
% % However, we still think that this is a valuable choice, as
% % directly calculating this accuracy change requires the underlying system to obtain the ground truth first (previous work define the ground truth as the inference results generated under the most expensive configuration to avoid the need for human annotation~\cite{dds,awstream,chameleon,vstore,videostorm,ekya,focus}).
% % This imposes non-trivial overhead due to extra inference on the most expensive configuration (\eg in Chameleon~\cite{chameleon}, calculating the ground truth\footnote{Chameleon is actually calculating multiple
% % resource-consuming configurations as the ``ground truth'', but the overhead is
% % still due to calculating ground truth.} consumes $\sim$50\% of the overall GPU
% % compute). 



% With the \outputgrad, the adaptation system can quickly adapt to the optimal configuration by assigning more resources to the knobs with high \outputgrad to improve the accuracy, or cut the resource usage of the knobs with low \outputgrad without hurting the accuracy.


% However, it can be expensive to calculate \outputgrad over a space of many knobs. %may incur high amount of extra inference.
% % This is because previous work needs to calculate \outputgrad in a knob-by-knob manner (\ie inference on the DNN and calculate the DNN output change by alternating the value of one knob while fixing other knobs, and repeat this process for all knobs). 
% Previous work~\cite{chameleon,vstore,videostorm,awstream} would have had to calculate \outputgrad in a knob-by-knob manner (\ie inference on the DNN and calculate the DNN output change by alternating the value of one knob while fixing other knobs, and repeat this process for all knobs). 
% % Thus, one more knob, one more extra inference.
% % Thus, more knobs will lead to more inference.


% To avoid such extra inference, \name leverages the \textit{differentiability} of the DNN to implement \outputgrad with constant GPU overhead and with no extra inference.
% % We show that \outputgrad, the first system that implements can be calculated without any extra inference and with constant GPU overhead.
% % We develop \name, a configuration adaptation system that optimizes the configuration based on \outputgrad.
% % The insight of \name is to leverage the \textit{differentiability} of DNN to reduce the cost of calculating \outputgrad.
% We {\em decouple} the calculation of \outputgrad (\ie how changing the knobs alters the DNN output) to how changing system knobs alters the DNN input and how changing the DNN input alters the DNN output.
% % Concretely, in order to calculate how changing the knobs alters the DNN output (\ie \outputgrad), we can calculate how changing system knobs alters the DNN input, and then calculate how changing the DNN input alters the DNN output.
% % \kt{Should we add a math formula of chain rule here? Like output/knob = output/input * input/knob?}
% The former can be calculated in a knob-by-knob manner without DNN inference (\ie no GPU compute), and the latter can be obtained via {\em backpropagation} (which is a constant GPU overhead without extra inference as it can reuse the existing computation graph of DNN inference).

% % We show that \outputgrad can be calculated with constant GPU overhead and without any extra inference, regardless of the number of the knobs, and develop \name, a configuration adaptation system, that optimizes the knobs based on \outputgrad.
% % \name reduces the cost of extra inference by treating \outputgrad as an actual gradient and leveraging the following two properties to decouple this gradient through the chain rule.
% % % \kt{I feel like this is the place to introduce the separation of the knob side v.s. the DNN side, as this separation is used (and only used) to reduce the cost of calculating the gradient}
% % \begin{packeditemize}
% %     \item 
% %     On the DNN side, the DNN output is differentiable to its input (via backpropagation algorithm).
% %     Thus, calculating how changing the DNN input alters the DNN output requires no extra inference.
% %     \item
% %     On the knob side, a wide range, \textit{not all}, of the knobs treat DNN as a \textit{black box} and affect DNN inference results solely by changing the DNN input.
% %     As a result, calculating how changing each individual knob alters DNN input requires no extra inference.
% % \end{packeditemize}
% % These two properties suggest that to calculate how changing the knobs alters the DNN output (\ie \outputgrad), we can first calculate how changing system knobs alters the DNN input, and then study how changing the DNN input alters the DNN output. 
% % \kt{Should we add a math formula of chain rule here? Like output/knob = output/input * input/knob?}
% % The former can be calculated in a knob-by-knob manner without the participant of the DNN (thus avoid extra DNN inference), and obtaining the latter only requires one backpropagation (this creates a constant GPU overhead, but it is reusing the computation graph created by existing DNN inference, thus incurring no extra inference).


% Operators can use \name to tune a wide range of applications and knobs that influences DNN input (as shown in Table~\ref{tab:rich-set-of-knobs}).
% That said, \name does {\em not} apply to all knobs and applications.
% In terms of knobs, \name does {\em not} apply to knobs that alter the DNN itself, 
% such as retraining the DNN weights~\cite{ekya,noscope,mcdnn}.
% Similar to \name, they also adapt to changes in input distribution, they involve substantial computation and thus tend to happen at a coarser timescale than the knobs considered in \name. 
% In terms of applications, \name does {\em not} apply to those applications that \fillme.
% % such as customizing the DNN according to the current content of the input~\cite{ekya,noscope,mcdnn}.
% % In some sense, both the DNN customization approach and \name are adapting to the varying content in the input data stream.
% % However, in order to maintain high accuracy, DNN customization approach needs to retrain the DNN when the input content varies, and thus incurs high GPU overhead, while \name adapts the knobs inside the underlying system that serves the DNN, which is much more lightweight.


% In short, the contributions of this paper are two-fold:
% \begin{packeditemize}
%     \item A new abstraction, \outputgrad, that enables quick adaptation of configurations for DNN-based analytics.
%     % \item A new abstraction, \outputgrad, that enables the configuration adaptation framework for DNN-based analytic systems to quickly adapt to optimal configuration through \accgrad.
%     \item A configuration adaptation system, \name, that implements \outputgrad with constant GPU overhead and without extra inference.
%     % \item An implementation, \name, that implements \outputgrad with constant GPU overhead and with no extra inference.

% \end{packeditemize}

% We evaluate \name across 7 different DNN-based analytic pipelines and across 54 videos. \name achieves similar accuracy with 10-43\% end-to-end delay reduction, or achieves 1-10\% higher accuracy with similar end-to-end delay compared to the baselines on 8 different applications.
% Also, we show that the performance gain of \name compared to the baselines becomes larger when there are more knobs or the knobs become more fine-grained.

% \textbf{This work does not raise any ethical issues.}







% % Expose abstraction:
% % confidence change gradient with respect to resource


% % Confidence scores -> a generalizable format
% % Confidence thresholds -> a widely adopted component in the accuracy of applications in real world.

% % % The key to achieve this goal is to calculate how much each knob changes the confidence scores that are close to the confidence thresholds 

% % To quickly adapt to optimal configuration without extra inference, the intuition of \name is to allocate more resource to the knobs that maximally change the confidence scores inside the inference results that are around  with confidence scores \textit{around} the confidence thresholds.
% % to maximally change \textit{which} inference results participants the accuracy
% % Concretely, \name calculates 


% % Why this works: two assumptions on the knobs 1. more resource, higher accuracy and 2. if the confidence scores around the confidence thresholds doesn't change, the accuracy barely change.

% % We present \name that efficiently calculates such metric on each knob.
% % The key for \name to success is to leverage the differentiability of DNN to \textit{predict} the performance of a run-time system.

% % our approach is to: grant more resources to the knobs can maximally change the part of the inference results that the confidence scores are around the confidence thresholds, and cut the resource usage of those knobs that barely change 


% % To quickly calculate this metric, we leverage the differentiability of the DNN to quickly obtain how DNN input affects the confidence scores around the confidence thresholds.



% % We present our system: \name, which meets these two requirements. 
% % To quickly adapt to optimal configuration, \name calculates the \textit{gradient} of accuracy with respect to each knob (hereinafter \accgrad, defined as the accuracy change if changing one knob valued by a little).
% % % leverages a property of DNN-based analytic system knobs: for most of the knobs, if changing the value of one knob results in spending more (or less) resource, the corresponding inference result would statistically become more (or less) accurate.
% % % This property suggests that each knob is able to \textit{trade resource for accuracy}.
% % % To quantitatively measure this ability, \name calculates the \textit{gradient} of accuracy with respect to each knob (hereinafter \accgrad, defined as how changing each individual knob by a little alters the accuracy).
% % With \accgrad, \name can quickly adapt to the optimal configuration in a
% % large configuration space by allocating more resources to those knobs with
% % high \accgrad to improve accuracy and cutting the resource usage of knobs with
% % \accgrad to save resource without hurting accuracy.





% % % insight that motivates \name is two properties we observe in deep learning
% % % system knobs. The first property is: for most of the knobs, if changing the
% % % value of one knob results in spending more (or less) resource, the corresponding
% % % inference result would statistically become more (or less) accurate. This
% % % property suggests that the change of accuracy with respect to knob value change
% % % % can reflect the ability of trading resource for accuracy for each individual
% % % knob. With \accchange, \name can quickly adapt to the optimal configuration in a
% % % large configuration space: \name can allocate more resources to those knobs with
% % % high \accchange to improve accuracy and cut the resource usage of knobs with
% % % \accchange to save resource without hurting accuracy.



% % % There is one more challenge to calculate \accgrad.


% % The first challenge of calculating \accgrad is: how to calculate the accuracy change when changing a knob value by a little?
% % Directly calculating this accuracy change requires the underlying system to obtain the ground truth first (previous work define the ground truth as the inference results generated under the most expensive configuration to avoid the need for human annotation~\cite{dds,awstream,chameleon,vstore,videostorm,ekya,focus}).
% % This imposes non-trivial overhead due to extra inference on the most expensive configuration (\eg in Chameleon~\cite{chameleon}, calculating the ground truth\footnote{Chameleon is actually calculating multiple
% % resource-consuming configurations as the ``ground truth'', but the overhead is
% % still due to calculating ground truth.} consumes $\sim$50\% of the overall GPU
% % compute). 
% % To resolve this issue, we develop a proxy for accuracy difference (we call this proxy \accproxy). 
% % % The main idea is to reuse the existing inference results and measure the accuracy change if the same input
% % % data \textit{were} processed by a new configuration. 
% % Concretely, \accproxy estimates the sign and the magnitude of accuracy change by the following rule:
% % \begin{packeditemize}
% % \item 
% % The \textit{sign} of accuracy change is determined by which input (between the two DNN input generated before and after changing one knob value) is of \textit{less distortion} compared to the DNN input generated under most expensive configuration.
% % \item 
% % We estimate the \textit{magnitude} of accuracy change through checking the \textit{dissimilarity} between the two inference results generated before and after the knob value change.
% % The intuition behind this estimation is that: if the inference results generated before and after the knob change are highly similar, the inference accuracy of these two inference results should also be highly similar.
% % \end{packeditemize}
% % By using this proxy, calculating accuracy difference no longer relies on the generation of ground truth, and 


% % However, even with the optimization above, trivially calculating \accgrad in a knob-by-knob manner (\ie
% % calculate the accuracy change by alternating the value of one knob value
% % while the value of other knobs value remaining unchanged, and repeat this process
% % for all knobs) still requires extra inference to get the inference results after each knob value change. 
% % To avoid such extra inference, \name leverages the following two properties:
% % \begin{packeditemize}
% %     \item
% %     On the knobs side, most of the knobs treat DNN as a \textit{black box} and affect DNN inference results solely by changing the DNN input.
% %     As a result, calculating how changing each individual knob alters DNN input requires no extra inference.
% %     \item 
% %     On the DNN side, the DNN itself is differentiable to its input (via backpropagation algorithm).
% %     Thus, calculating how changing the DNN input alters the accuracy requires no extra inference.
% % \end{packeditemize}
% % These two properties suggest that to calculate how changing the system knobs alters the accuracy (\ie~\accgrad), we can first calculate how changing system knobs alters the DNN input, and then study how changing the DNN input alters the accuracy. 
% % The former can be calculated in a knob-by-knob manner without the participant of the DNN (thus avoid extra DNN inference) and the latter only requires one backpropagation (thus incurring no extra inference).

% % compared to the ground truth DNN input, and estimate the magnitude of accuracy
% % change by comparing the difference of inference results between the old and the
% % new configuration. 
% % We find that the \textit{gradient} of this accuracy metric can be calculated \textit{without} extra inference.

% % \begin{comment}

% %   Deep learning applications on streaming data (\eg video streams or LiDAR
% %   feeds) are everywhere. For example, in autonomous driving, people use video
% %   cameras and LiDAR sensors and leverage object detection deep neural networks
% %   (DNNs) to sense the surrounding environment and avoid potential collisions. In
% %   augmented reality, people use video cameras and LiDAR sensors to localize the
% %   remote objects and render the virtual objects on top of real objects. This
% %   trend inspires system research for these applications, like live
% %   analytics~\cite{??}, retrospective analytics~\cite{??}, database for analytic
% %   purpose~\cite{vstore,noscope}, etc.

% %   We identify two important characteristics of these systems. First, they
% %   contain large configuration spaces (\eg in AWStream~\cite{awstream}, there are
% %   216 different configurations inside its configuration space). Second, these
% %   configurations need to be \textit{timely} adapted according to their input
% %   (\eg we may want to use higher video resolution when a small car enters the
% %   video frame in order to detect this small car) and the current resource budget
% %   so that they can generate the inference results as accurate as possible.

% %   As a result, the key challenge for these systems is: how to navigate the large
% %   configuration space and pick the optimal configuration that generates the most
% %   accurate inference results under the current resource budget.

% %   The first way to address this problem is to \textit{frequently profile} the
% %   system with different configurations to obtain their resource usage and
% %   inference accuracy, and then pick the configuration that meets the resource
% %   budget and generates the most accurate inference
% %   results~\cite{awstream,chameleon,vstore}. However, in order to profile, this
% %   approach has to perform \textit{extra} inference on the GPU, resulting in high
% %   GPU cost.

% %   The other approach performs no extra inference and instead, picks the
% %   configuration based on the recent configuration and its corresponding DNN
% %   output. However, there can be many configurations that meet the resource
% %   budget. Without profiling most of them, it is difficult to separate the
% %   configurations that yield similar DNN output from those that yield more
% %   accurate DNN output. In addition, the previous work in this approach designs
% %   hand-craft heuristics catered for different applications.

% %   Thus, the requirements of an ideal configuration adaptation system are
% %   three-fold:
% %   \begin{enumerate}
% %     \item No extra DNN inference
% %     \item Pruning out the configurations with similar accuracy
% %     \item Agnostic to the underlying applications
% %   \end{enumerate}

% %   We present our system: \name that meets these three requirements. The idea is
% %   to calculate the \textit{gradient} of inference accuracy with respect to the
% %   configurations to \textit{predict} which of them improve inference accuracy
% %   and which do not. The key insight that enables us to calculate this gradient
% %   is by decoupling this gradient into two terms. The first term is the gradient
% %   of inference accuracy with respect to the DNN input, which can be calculated
% %   by backpropagation without performing extra inference on any other
% %   configuration. The second term is the gradient of the DNN input with respect
% %   to the configurations, which does not require DNN inference.

% %   To make our system practical, we also identify another source of overhead
% %   introduced by calculating inference accuracy. In order to calculate inference
% %   accuracy, previous work needs to refer to the configuration with \textit{the
% %   most} resource usage and use the corresponding inference results as the
% %   ``ground truth'' to evaluate the accuracy of inference results generated from
% %   other configurations. Calculating the ``ground truth'' uses much higher
% %   resource usage (including the streaming cost of streaming the data and the GPU
% %   cost to generate inference results) than the current optimal configuration. To
% %   reduce this cost, we introduce a \textit{proxy} of accuracy that
% %   \textit{indirectly optimizes} accuracy by using the DNN input (instead of the
% %   DNN output), thus requiring no DNN inference.

% %   To conclude, the contributions of this paper are:
% %   \begin{enumerate}
% %     \item A way to calculate gradient with no extra inference
% %     \item An accuracy proxy that indirectly optimizes the accuracy without
% %           running extra inference.
% %   \end{enumerate}
% %   We quantitatively evaluate these two contributions, we perform experiments on
% %   XXX datasets, XXX applications and XXX

% % \end{comment}
% % 





==> intro_v7.tex <==

\tightsection{Introduction}
\label{sec:intro}


Many applications rely on deep neural nets (DNNs) for accurate inference on various types of input data~\cite{trafficvision, traffictechnologytoday, goodvision,intuvisiontech, vision-zero, msr,tusimple,waymo-blog,motional}.
For example, a DNN can analyze video frames to
detect vehicles and pedestrians, or analyze an audio stream to extract text. 
These applications often run DNN inference on cloud/edge servers, causing resource contention in both {\bf network bandwidth} to stream high-fidelity data (\eg high-quality video) from distributed sensors to the analytics servers and in {\bf GPU compute cycles} to run expensive DNN inference on many data points (\eg each video frame).






Many previous efforts have shown that {\em optimally tuning a range of knobs} (\eg video frame rate and resolution) can greatly save resource usage and achieve high accuracy.
Table~\ref{tab:rich-set-of-knobs} shows a list of example knobs.
We use a {\em configuration} to refer to a particular setting of the knobs used by an application (\eg a particular frame rate and resolution).
% Multiple knobs are often tuned together to save more resources (see Table~\ref{tab:rich-set-of-knobs} for a list of knobs considered).
% uses the {\em optimal setting} of these knobs, 
% high inference accuracy could be obtained while significantly reducing resource usage in both network bandwidth and GPU compute.
The challenge is that the optimal configuration {\em varies} over time with the input data, so it must be {\em adapted timely}. 
For instance, when the vehicles stop at the red light or move slowly, feeding the traffic video feed at a low frame rate to a DNN can still accurately detect vehicles,
% at only one frame per second (fps) in a traffic video, 
but when the light turns green, the DNN must analyze frames much more frequently (\eg 30fps) to detect fast-moving vehicles. 
In this case, the configuration of frame rate
% of feeding data to the DNN---
must be dynamically adapted depending on the video content.





% \kt{Define how people do it today.}
The key question, therefore, is as input data evolves over time, 
{\em how to quickly check if the current configuration should be changed.} In other words, whether a different configuration can yield much higher accuracy or lower resource usage without hurting accuracy. 







\mypara{Prior approaches}
To answer this question, two general approaches exist, but they fall short for different reasons (\S\ref{subsec:configuration-adaptation}).

First, {\em profiling-based} methods (\eg~\cite{awstream,chameleon,videostorm,vstore}) periodically run {\em extra} DNN inferences to profile the accuracy of alternative configurations and then use these profiles to identify the optimal configuration. 
% runs inference with many configurations to {\em profile} which configuration has the highest accuracy with minimum resource usage~\cite{awstream,chameleon,videostorm,vstore}. 
However, the extra DNN inferences incur significant GPU overhead.
% to run significantly more extra DNN inference on the same input data. 
% Moreover, it often uses extra bandwidth to stream input data at a much higher quality to test their inference accuracy.
For example, AWStream~\cite{awstream}'s profiling step test 
% runs DNN inferences with 
different combinations of resolutions, frame rates, and quantization parameters, which causes up-to 17$\times$ more GPU cycles than normal inference.
% , causing 17$\times$ extra GPU overhead. % than regular DNN inference.
With limited compute resource, the profiling overhead will slow down configuration adaptation and cause the configuration to be outdated when input data changes over time. 


Second, {\em heuristic-based} methods~\cite{dds,reducto,vigil,glimpse,eaar,accmpeg,casva,elf} avoid extra inference and pick the configuration using {\em cheap} heuristics.
Though they may adapt faster
% (\eg once every second) 
than profiling-based methods, but the cheap heuristics may sometimes pick suboptimal configurations that have low accuracy.
% pick the configuration with accuracy much lower than the optimal one (see \S\fillme for more rationales).
For instance, a typical heuristic selects a new frame to feed to DNN
when its pixels differ significantly from the last analyzed frame (\eg~\cite{reducto}).
However, a high pixel-level difference may fail to indicate frames with new objects of interest, when the video background moves quickly (\eg dashcam video from a moving vehicle) which causes great pixel changes.
% , frame difference is caused mostly by background pixels and thus becomes a poor indicator for the arrival or movement of objects of interest.
As a result, it might run the DNN on too many frames while the objects of interest remain the same.


Moreover, many existing techniques are designed only for {\em specific} data types or knobs.
% , and it is unclear how effective they will be on other types of data (\eg LiDAR point cloud, depth map, or audio waves).
% Even in video analytics, the proposed heuristics often work well only for {\em specific knobs}.
% and do not generalize to other types of knobs.
For example, Reducto~\cite{reducto} selects which frames to run DNN inference based on inter-frame difference, but the inter-frame difference is ill-suited to tuning the encoding quality parameters of a video frame, which depends on the content {\em within} a frame, rather than how it differs from other frames. 
% See \S\ref{subsec:configuration-adaptation} for more examples.
Likewise, DDS~\cite{dds} tunes the region-of-interest quality parameter within each frame, but its logic may not naturally extend to tuning  knobs of non-video input data, such as LiDAR point cloud, depth map, or audio waves.
% each fine-grained spatial block to improve inference accuracy on each frame, 
% but it is not aware whether the current frame is redundant given past inference results.




In short, prior work falls short on at least one of the three fronts: 
(1) frequent adaptation, (2) choice of near-optimal configuration, and (3) not tied to specific configuration knobs.
% (1) adapt frequently, (2) reach a near-optimal configuration, and (3) apply to a range of configuration knobs.


\myparashort{\name: Fast adaptation based on \outputgrad.}
This paper presents \name, a new approach to configuration adaptation that improves on all three fronts.
The key of \name is a new method to quickly estimate {\em gradient of the DNN inference accuracy with respect to each knob at current configuration}.
We refer to this gradient as the \outputgrad of each knob.
\outputgrad effectively shows how much can a small change in the configuration of each knob change DNN accuracy.
{\em If} \outputgrad can be estimated frequently, say every second, \name can adopt a {\em gradient ascent} strategy that uses the up-to-date \outputgrad to change the configuration of each knob in a way that maximally increases accuracy or reduces resource usage without hurting accuracy.
Our gradient-ascent strategy outperforms previous work for the following reasons:

\begin{packeditemize}
\item Compared to profiling-based methods, \name can update the \outputgrad's estimate and use it to adapt {\em more frequently} than waiting until the slow profiling finishes (\eg every minute~\cite{awstream}). 
% \name updates the \outputgrad's estimates every second, and so it does with the configuration.
More importantly, \outputgrad indicates that given the input data content, which knob's configuration should be changed to maximally increase accuracy or reduce resource usage without affecting accuracy. 
% This allows \name to adapt to changes in input data earlier than profiling-based methods which must wait until the next profiling (\eg every minute~\cite{awstream}). 

\item Compared to heuristics-based methods, \name's gradient-ascent can converge to a {\em closer-to-optimal} configuration.
Most heuristics used in prior work adapt configuration by analyzing only the input data, rather than how the data might affect the final DNN's output.
By contrast, we formally prove that under reasonable assumptions, 
% \outputgrad statistically indicates how the accuracy of the final DNN changes with each knob and 
\name's gradient-ascent strategy almost always converges (\S\ref{subsec:limitation}). 
We have also validated these properties in a wide range of empirical evaluations (\S\ref{sec:eval}).

\end{packeditemize}

\begin{figure}
    \centering
    \includegraphics[width=0.6\columnwidth]{figs/contrast_different_approach.jpg}
    \tightcaption{
    Contrasting our approach with prior work. Our approach quickly adapts to a near-optimal configuration after the change of input content, while profiling-based methods adapt slowly and heuristics adapt to a configuration with much lower accuracy than the optimal one.
    }
    \label{fig:adaptation-behavior}
\end{figure}


\myparashort{Cheap estimation of \outputgrad}
The key technical nugget of \name is how to quickly estimate \outputgrad for all knobs. 
Our insight is that this can be achieved by leveraging DNN's {\em differentiability}, with no extra DNN inference.
Differentiability is an inherent property of almost all DNNs~\cite{paszke2017automatic} but has so far been only used in DNN training. 
If a knob only transforms the raw input data to DNN's input (\eg frame filtering, image downscaling, etc), then the \outputgrad of a knob can be decoupled into:
\begin{packedenumerate}
\item {\em \dnngrad:} How the DNN's output changes with respect to the DNN's input.
\item {\em \inputgrad:} How the DNN's input changes with respect to the knob's configuration.
\end{packedenumerate}
Both can be computed efficiently: 
\dnngrad can be efficiently computed by a single backpropagation operation on the DNN, and 
computing \inputgrad does not need GPU.
Moreover, if the system has multiple knobs, \dnngrad can be calculated once and re-used to derive the \outputgrad of different knobs.  
Intuitively, this is because \dnngrad describes DNN's sensitivity to a change in the DNN's input, which is agnostic to {\em which} knob causes the change in DNN's input.
% For instance, the \dnngrad of an object-detection DNN will be high for pixels associated with key visual features of an object.

We also formally prove that the multiplication of \dnngrad and \inputgrad is correlated with the true gradient of inference accuracy with respect to each knob (\S\ref{sec:proof}). 
This is intuitively true because a significant change in the inference results (\ie large \outputgrad) is often accompanied by a substantial change in accuracy. 






As \name introduces the extra overhead of DNN backpropagation, 
% As the overhead of backpropagation is substantial (about 2x extra GPU memory usage and 1x extra GPU computation), 
\name provides a suite of techniques that reduce this GPU compute and memory overhead 
% (together with other types of overheads) 
in \S\ref{sec:cost}, including reusing the backpropagation results between different frames (which reduces the backpropagation overhead by 10$\times$), and removing unneeded computation in backpropagation.
We want to clarify that as long as there are sufficient resources for \name to run in real-time, the extra overhead of \name does \textit{not} increase the end-to-end delay (the delay of obtaining the inference results), as the adaptation logic of \name runs after generating the inference results.





We evaluate \name across 9 analytic pipelines (see Table~\ref{tab:pipeline} for the detail of these pipelines), which cover 4 analytic tasks (vehicle detection, human detection segmentation, audio-to-text), 5 types of input data (\eg LiDAR videos, audio waves), and 5 types of knobs (\eg video codec knobs, frame filtering thresholds).
% Our dataset contains 59 videos (~110 minutes in total) and 200 audios (33 minutes in total).
% We evaluate \name across 9 different DNN-based analytic pipelines, with 5 types of data, 4 analytic tasks, 6 configuration knobs, 59 videos, and 200 audios. \jc{earlier you said it can work on 3 analytic tasks (object detection, segmentation, audio-to-text), 4 input data (videos, LiDAR feeds, depth videos, audio waves), and ?? knobs (see Table~\ref{tab:rich-set-of-knobs} for the list of knobs that \name can handle). can we be consistent about it?}
\name achieves similar accuracy with 15-59\% resource usage reduction, or achieves 15\% higher accuracy with similar resource usage compared to the baselines on 9 different analytic pipelines.
We also show that the performance gain of \name over the baselines increases with more knobs. % become more fine-grained.

These results also show that rather than targeting a specific setting, \name can work in a {\em variety} of analytic tasks, input data types, and knobs.
That said, \name has limitations (more in \S\ref{sec:limitation_section}). We have not tested if \name will work for applications beyond our evaluation, such as knobs that alter the final DNN itself (\eg DNN selection) or generative tasks (\eg text generation, image generation).
    





In short, the contributions of this paper are two-fold:
\begin{packeditemize}
    \item Design of \name, a new configuration-adaptation system that runs gradient ascent based on fast computation of \outputgrad.
    % \name's gradient-ascent-based search.
    \item Implemented a prototype of \name and integrated it with a benchmark of 9 DNN applications (which cover 5 data types, 4 analytic tasks, and 5 configuration knobs). \name achieves similar accuracy while reducing resource usage by 15-59\% or improves accuracy by 1-5\%  with the same or less resource usage when compared to state-of-the-art adaptation heuristics. 
\end{packeditemize}




\textbf{This work does not raise any ethical issues.}
    
    


==> intro_v8_polished.tex <==

\section{Introduction}
\label{sec:intro}

The essence of many real-world applications revolves around the use of deep neural networks (DNNs) to perform analytics on a variety of streaming media data including RGB videos, LiDAR point clouds, depth videos, and audio waves. For instance, autonomous-driving applications typically rely on DNNs to detect vehicles in individual video frames using RGB videos and LiDAR point clouds \cite{tusimple,waymo,trafficvision, traffictechnologytoday,goodvision,intuvisiontech, vision-zero, msr,servai-1,servai-2,servai-3}. Similarly, smart-home applications utilize DNNs to extract text from audio segments \cite{smarthome-1,smarthome-2,smarthome-3}. These applications are collectively referred to as \textit{\textbf{streaming media analytics}} (refer to \S\ref{subsec:streaming-analytics} for an extensive description). It is important to note that while video analytics applications feature prominently in streaming media analytics, not all DNN-based applications - such as those concerning generative tasks - fall within its scope.

The operational requirements of many streaming media analytics systems are high in terms of either \textbf{network bandwidth} or \textbf{GPU cycles}, or sometimes both. This is because they are designed to run complex DNN inference on each frame or segment, which underscores the need for high-fidelity data, and thus potentially high GPU usage and network bandwidth in cases where the data is captured remotely.

In order to drive down resource usage, a substantial amount of previous solutions - for example, \cite{dds,eaar,elf,vigil,glimpse,accmpeg,reducto,casva} - employ an approach known as \textit{input filtering}. This approach entails downsampling or discarding data that does not significantly influence the outcome of the final DNN analysis. Following this, \textit{DNN inference} is run on the filtered input. Theoretically speaking, if the input filtering is associated with an optimal setting for the main controls (such as video frame rate and resolution), the bandwidth and GPU usage can be significantly reduced without negatively impacting inference accuracy. The four leading types of filtering controls are summarized in Table~\ref{tab:knob-categorization}.

However, the challenge of optimally adjusting the input filtering controls is known to be complex. This is due to the variable nature of the optimal settings, which change over time in response to evolving input data \cite{chameleon,awstream,vstore,casva,videostorm,reducto}. Accordingly, the optimal settings at any given time can be referred to as an optimal configuration. To illustrate, in traffic scenarios where vehicles are stationary at traffic lights or moving slowly, a DNN capable of accurately detecting vehicles can operate with a traffic video feed at a low frame rate. In contrast, when vehicles are moving at a faster pace, it becomes necessary to operate the DNN more frequently, perhaps at 30fps, in order to maintain accurate vehicle detection. Consequently, the frame rate configuration should be adaptable based on the nature of the video content.

To effectively respond to this challenge, an ideal adaptation logic should satisfy three requirements. Firstly, it should enable \textit{\textbf{Frequent Adaptation}} to cater for optimal configurations that change alongside the input data, whilst minimising GPU computation and network bandwidth overheads. Secondly, the process of \textit{\textbf{Near-optimal Adaptation}} should be accommodated, wherein the ability to adapt to situations that provide similar accuracy with fewer resources or an increase in accuracy with similar resources, or a combination of both, is integral. Thirdly, \textit{\textbf{Wide Applicability}} should be a key feature of the adaptation logic in order to facilitate the successful handling of a broad spectrum of analytic tasks, streaming media, and input filtering controls.

\mypara{Past Approaches}

Despite numerous efforts in the past, all proposals to date fall short on a minimum of one of these three requirements, as depicted in Figure\ref{fig:adaptation-behavior} (a detailed discussion is provided in \S\ref{subsec:configuration-adaptation}).


\begin{packeditemize}

\item \emph{Profiling-based} strategies, as exemplified in works such as~\cite{awstream,chameleon,videostorm,vstore}, employ periodic additional deep neural network (DNN) inferences in order to profile the accuracy of alternative configurations. However, this approach entails considerable graphical processing unit (GPU) overheads. For instance, AWStream's~\cite{awstream} profiling step, which tests a downsampled subset composed of all possible combinations of resolutions, frame rates, and quantization parameters, can increase GPU computation up to 17-fold compared to standard DNN inference. Consequently, when GPU computational power is constrained, the overhead associated with profiling decelerates the adaptation of configuration, potentially leading to outdated configurations when the nature of input data changes over time.

\item In contrast, many other approaches~\cite{dds,reducto,vigil,eear,accmpeg,casva,elf,wang2022minimizing} shun additional inference and instead adopt \emph{economical heuristics} for configuration adaptation. While such methods can be frequently updated, their inherent oversimplification in gauging which parts of the input are significant or irrelevant to final DNN often results in errors that compromise accuracy or escalate resource usage. A typical example is a seemingly viable heuristic that screens a new frame for DNN inference based on a significant difference in pixels from the most recent frame analysed~\cite{reducto,glimpse,rocket}. However, these pixel differences may be attributable to background rather than areas of interest, underscoring the inadequacy of such heuristics.

\item Additionally, a sizeable portion of the existing techniques are specifically tailored for determined analytical tasks, streaming media, and/or input filtering controls. For example, DDS~\cite{dds} and STAC~\cite{stac}, which choose regions in a frame that should be of high quality, not suitable for application with non-video input data like LiDAR point clouds, depth maps, or audio waves. Nor can they readily adapt controls other than video encoding quality.

\end{packeditemize}




\section{Our Approach: Fast Gradient-Based Adaptation}
In this paper, we introduce \name, a novel system for configuration adaptation that offers significant advancements in comparison to existing solutions. \name is primarily based on a new technique for rapidly estimating \accgrad, referring to the gradient of Deep Neural Network (DNN) inference accuracy in relation to alterations in each filtering knob from its current position. It is essential to highlight that we define \accgrad as a numerical gradient, as opposed to the analytical gradient, which is commonplace in optimization of discrete system knobs \cite{pcc-vivace,ramazanov2011stability,chistyakov2015stability}.

The rapid approximation of \accgrad underpins the fundamental observation that the filtering knobs affect inference accuracy depending on their changes on the DNN's input. This implies that the \accgrad of each knob, i.e., how the DNN's accuracy changes with alterations in the knob, can be divided into two distinct parts: 

\begin{packedenumerate}
\item \inputgrad: This component illustrates how alterations in each knob affect the DNN's input. Given that the acquisition of the DNN's input can be performed on a Central Processing Unit (CPU), the GPU computation process is circumvented.
\item \dnngrad: This component explains the variation in the DNN's accuracy relative to alterations in the DNN's input. This can be achieved through a backpropagation operation, which can significantly accelerate the process by discarding the gradients of DNN weights. As these gradients represent a substantial overhead and are not needed for \dnngrad computation, their removal reduces the computational burden (refer to Section \ref{sec:cost} for additional cost reduction techniques).
\end{packedenumerate}

Given this, both \inputgrad and \dnngrad can be computed with minimal overhead. Considering that \dnngrad represents the DNN's sensitivity to input changes irrespective of the knob causing it, \dnngrad can be calculated once and applied in conjunction with the \inputgrad of different knobs to determine their \accgrad. 

The estimation of \accgrad requires minimal additional GPU computation, enabling \name to update the estimate frequently, for instance, every second. Subsequently, a gradient-ascent strategy is employed to update the configuration in a manner that optimally enhances accuracy or reduces resource usage without undermining accuracy \cite{pcc-vivace}. As configuration-accuracy relationships are primarily concave, this strategy is likely to converge towards a nearly optimal configuration. 

The concavity can be intuitively understood as if we increase the knob slightly (for instance, increasing frame rate), the improvement in accuracy is more pronounced when the system's accuracy is low. However, this gain diminishes if the system is already generating accurate inference results. 

The design rationale and the workings of the \name system, including why \accgrad can be effective in configuration adaptation and why \name converges, are elaborated on in Section \ref{sec:design}.

\begin{comment}
\end{comment}

\begin{packedenumerate}
\item {\em \inputgrad:} This represents the alteration in the input of the DNN with respect to the configuration of the knob. It is noteworthy that \inputgrad can be obtained without executing any DNN operations on the GPU.
\item {\em \dnngrad:} This represents the alteration in the accuracy of the DNN with respect to the modification in the DNN's input. Surprisingly, \dnngrad can be obtained by performing a single backpropagation operation on the DNN.
\end{packedenumerate}

To further elucidate why \accgrad can be decoupled into \inputgrad and \dnngrad, we provide a formal proof that under plausible assumptions, the inner product of \dnngrad and \inputgrad is congruous with \accgrad (\S\ref{subsec:outputgrad}). We have empirically substantiated their correlations as well (\S\ref{subsec:outputgrad}).

Both \inputgrad and \dnngrad can be computed efficiently. Notably, the computation of \inputgrad does not necessitate any GPU operations. The \dnngrad can be calculated by a single backpropagation and subsequently re-utilized to compute the \outputgrad of various knobs, given that \dnngrad describes DNN's sensitivity to any alteration in the DNN's input, regardless of which knob initiates the change.  

Even though \name introduces the additional overhead of DNN backpropagation during GPU computation, \name offers two techniques that alleviate this overhead: avoiding calculation of gradients for DNN parameters and reutilizing the gradient across different frames (see \S\ref{sec:cost} for a detailed discussion). These optimizations diminish GPU cycles utilized for backpropagation to a mere 19\% of forward DNN inference, having a minimal effect on \name as indicated in Figure~\ref{fig:reusing-saliency}.

\begin{figure}
    \centering
    \includegraphics[width=0.8\columnwidth]{figs/contrast_different_approach.jpg}
    \tightcaption{
    A comparison of our proposed method with two existing approaches. Our method swiftly adjusts to a near-optimal configuration following a change in input content, whereas the profiling-based methods adapt at a slower pace and heuristics adjust to a configuration with considerably lower accuracy than the optimal one. (This figure is for illustrative purposes; an actual example can be found in Figure~\ref{fig:adaptivity}).
    }
    \label{fig:adaptation-behavior}
\end{figure}

To provide context for the contribution of \name, though the concept of using DNN gradients is not new in video analytics systems~\cite{stac,saliency_hotmobile}, \name, to the best of our knowledge, is the first to facilitate fast approximation of the accuracy's gradient in relation to the four popular kinds of filtering knobs (\accgrad). The resulting frequent application of gradient ascent empowers \name to exceed the performance of both profiling-based and heuristic-based approaches, as shown in Figure~\ref{fig:adaptation-behavior}.

Contrary to profiling-based methods, we approximate \accgrad and adjust more in frequent cycles, while profiling-based systems adapt configuration following the completion of slow profiling. In contrast to heuristic-based methods, our gradient-ascent is capable of converging to an optimal configuration. Previous research adapts configuration by either analyzing the input data or the output of the DNN, rather than considering how changes in the input data influence the final accuracy of the DNN. By contrast, \accgrad directly indicates the variation of DNN accuracy with a change in the configuration. 

In our evaluation of \name, we tested on nine different streaming-media analytics pipelines (refer to Table~\ref{tab:pipeline}). These pipelines incorporate five types of input data as well as five filtering knobs. They are applicable in four real-world scenarios such as autonomous driving and traffic analytics. We contrasted \name with the latest profiling-based and heuristic-based schemes, both of which were designed to optimize each type of knob.

The key results were:
\begin{packedenumerate}
\item \name achieves comparable accuracy while diminishing bandwidth usage or GPU compute between 15-59\%. When allocated the same resource budget, \name enhances accuracy by 15\%.

\item In comparison to a naive implementation, \name reduces the GPU computation overhead and the GPU memory overhead of \accgrad approximation by 87\% and 12\% respectively. Thus, the estimation of \accgrad is five times faster than operating DNN inference on an equivalent volume of input data.

\item Contrary to prior solutions designed specifically for individual filtering knobs, \name improves all knobs utilizing the same logic. 
\end{packedenumerate}


Following this, however, it is essential to acknowledge the limitations inherent to \name, as delineated in Section \ref{sec:limitation_section}. To elaborate, \name is not fully compatible with analytical applications whose operational features do not significantly influence the input filtering stage, such as DNN selection. Similarly, \name struggles to accommodate DNN applications that do not incorporate streaming media analysis, an example of which are generative tasks.

\begin{comment}

While \name proves advantageous for tasks demanding analytics—object detection and segmentation, predominately focused on by preceding video analytic systems~\cite{dds,eaar,accmpeg,awstream,chameleon,elf,vigil,glimpse,reducto,saliency_hotmobile,casva}, its effectiveness in executing other analytical tasks remains untested. This includes tasks in which operational features considerably alter the final DNN itself (for instance, DNN selection) or tasks categorized as generative (such as text and image generation).

In brief, the key contributions of this study can be distilled into two main aspects:

\begin{packeditemize}
    \item The conceptualization of \name, a novel configuration-adaptive system operationalizing gradient ascent grounded on rapid estimation of \accgrad.
    
    \item Development and integration of a \name prototype with a benchmark of nine DNN applications. These applications incorporate five data types, four analytic tasks, and five configuration knobs. Remarkably, \name maintains accuracy while decreasing resource usage by approximately 15-59\%. Alternatively, it augments accuracy by 1-5\% even when using equal or lesser resources compared to other leading adaptation heuristics. 
\end{packeditemize}

\end{comment}

\textbf{This study does not present any ethical issues.}



==> introduction.tex <==
\section{Introduction}
Deep-neural-network-based (DNN-based) analytics on data streams (\eg video
streams or LiDAR feeds) are everywhere. This trend inspires system research for
these applications.

We observe that these systems expose an \textit{increasing} number of internal knobs.
The underlying trend that drives this increase is two-fold (we will further discuss these two points in \S\ref{subsec:numer_of_knobs}). First, these systems need to develop new knobs to achieve high analytic accuracy under different resource budgets induced by different deployment settings (\eg deploying on powerful GPU-equipped camera or on cheap compute-limited camera) and handle new emerging applications (\eg LiDAR-based object detection for autonomous driving and infrared-based human detection for night time).
Second, in order to support more DNN-based analytic tasks with limited resource, these systems need to partition existing knobs to a more fine-grained version to further reduce the resource demand for each single DNN analytic task.

% % redirected enumerate to packedenumerate for reformater in macro.tex. DON'T
% % CHANGE!
% \begin{enumerate}
%   \item 
% As DNN-based analytics are deployed on heterogeneous deployment settings that have different types of resource budgets, this requires the corresponding systems to propose new knobs in order to fit into
% different resource budgets. Take video analytics as an example. If the
% user analyzes the video feeds locally by a compute-constrained mobile
% phone, the main focus for the systems is to fit into the compute budget
% of the phone (\eg by skipping those frames that are highly similar to
% their previous frames~\cite{reducto,glimpse}). However, if the user
% instead streams the video feeds to a GPU-equipped server through a
% bandwidth-limited LTE network, the main focus is instead fitting into
% the limited LTE bandwidth (\eg by performing video
% compression~\cite{accmpeg,vigil,glimpse,reducto}).

%   \item As DNN-based analytics quickly expand, the corresponding systems need to
%         partition existing knobs into more fine-grained version to capture more
%         resource-saving opportunities. Take video-based vehicle detection as an
%         example. Chameleon~\cite{chameleon} and AWStream~\cite{awstream}
%         identify that the system only need to encode the video in a high
%         encoding quality when the vehicle appears. To further explore the
%         potential of varying video encoding quality, the following
%         work~\cite{dds,eaar,accmpeg} finds that a lot of areas in the video do
%         not need to be encoded in high quality (\eg the areas that contain
%         non-vehicle-related backgrounds like trees and buildings) and proposes
%         fine-grained spatial encoding quality to capture this opportunity.
%   \item Since new applications quickly emerge (\eg LiDAR-based object detection,
%         Infrared-based human detection \kt{a bunch of citations here}), this requires the deep learning systems
%         to develop new knobs (or even developing new system components) to fit
%         into the need of different applications. For example, in order to handle
%         LiDAR data, people are proposing new encoding standard and new
%         knobs~\cite{MPEG-point} to efficiently encode and process LiDAR data.
%         \roy{I understand you are trying to distinguish old types of application
%         and new ones, but I still feel the first and third items are kind of
%         repetitive? Both items are trying to say there is the need for new
%         knobs, right? Maybe merge them into one?}
% \end{enumerate}

Not only the number of knobs are huge, these knobs also need to be timely adapted~\cite{awstream,chameleon,dds,eaar,elf} due to input data change or resource budget change in order to achieve high inference accuracy.
Thus, the research question is: how to navigate the large configuration space formed by high number of knobs and and pick the optimal configuration that generates accurate inference results under the current resource budget?

The first way to address this problem is to \textit{frequently profile} the
system with different configurations to obtain their resource usage and
inference accuracy, and then pick the configuration that meets the resource
budget and generates the most accurate inference results. However, this approach
needs to perform \textit{extra} inference.


The other approach performs no extra inference and instead, derive the
configuration from recent DNN outputs (including intermediate outputs). However,
there can be many configurations that meet the resource budget. Without
profiling most of them, it is difficult to separate the configurations that
yield similar DNN output from those that yield more accurate DNN output.

\kt{example added}
In addition, the previous work in this approach designs hand-crafted heuristics catered only for individual applications or configurations. 
Take video object detection as an example. DDS~\cite{dds} adjusts the spatial encoding quality by performing inference on the low quality video and then resend those regions that might contain objects in high quality.
This heuristics cannot be reused to perform frame discarding (\ie discarding those frames that produces similar inference results comapred to previous frames~\cite{vigil,glimpse,reducto}), since its adaptation logic (\ie resending regions that may contain objects) happens \textit{after} DNN inference while frame filtering need to be performed \textit{before} DNN inference to save GPU compute cost.


An ideal configuration adaptation systems should meet these two
requirements: 1. quickly adapt to optimal configuration in a large configuration
space without extra inference 2. minimum assumption to the underlying system

We present our system: \name, which meets these two requirements. 
The main
insight that motivates \name is two properties we observe in deep learning
system knobs. The first property is: for most of the knobs, if changing the
value of one knob results in spending more (or less) resource, the corresponding
inference result would statistically become more (or less) accurate. This
property suggests that the change of accuracy with respect to knob value change
can reflect the ability of trading resource for accuracy for each individual
knob. With \accchange, \name can quickly adapt to the optimal configuration in a
large configuration space: \name can allocate more resources to those knobs with
high \accchange to improve accuracy and cut the resource usage of knobs with
\accchange to save resource without hurting accuracy.

However, trivially calculating \accchange in a knob-by-knob manner (\ie
calculate the accuracy difference by alternating the value of one knob value
while the value of other knobs value remaining unchanged, and repeat the process
for all knobs) results in extra inference. To avoid such extra inference, \name
leverages the second property of deep learning system knobs: most of the knobs
treat DNN as a \textit{black box} and affect DNN inference results solely by
changing the input to the DNN. Thus, to calculate \accchange, we can first
calculate how system knobs changes the DNN input, and then study how the DNN
input changes the accuracy. The former does not involve DNN inference, and the
latter can be calculated without extra DNN inference (see \S\ref{??} for how we
calculate this term) and can be shared across different knobs.

There is one more
challenge to calculate \accchange: how to obtain the ground truth for the
accuracy metric? As human annotation can be expensive, previous work leverages
inference results generated under \textit{the most resource-consuming
configuration} as the ``ground truth'' and uses it to evaluate inference
accuracy. This metric works well for evaluation purpose, but previous work
frequently calculate this metric during \textit{run-time}, resulting in
non-trivial computation overhead due to frequently deriving ground truth from
the most resource-consuming configuration (\eg in Chameleon~\cite{chameleon},
calculating the ground truth\footnote{Chameleon is actually calculating multiple
resource-consuming configurations as the ``ground truth'', but the overhead is
still due to calculating ground truth.} consumes $\sim$50\% of the overall GPU
compute). To resolve this issue, we introduce a cheap run-time approximation of
the above accuracy metric: accuracy \textit{proxy}. The main idea is to reuse
the existing inference results and measure the accuracy change if the same input
data \textit{were} processed by a new configuration. Concretely, we estimate the
sign of accuracy change by checking which input (among the DNN input generated
from the old and the new configuration) has smaller pixel-wise difference
compared to the ground truth DNN input, and estimate the magnitude of accuracy
change by comparing the difference of inference results between the old and the
new configuration. By making one assumption, we prove that this accuracy metric
can be calculated \textit{without extra} inference.

To conclude, the contribution of this paper is two-fold: 1. quickly adapt to
optimal configuration by using accuracy-knob gradient 2. Two techniques to
remove the need of the extra inference when calculating accuracy-knob gradient.


\begin{comment}

  Deep learning applications on streaming data (\eg video streams or LiDAR
  feeds) are everywhere. For example, in autonomous driving, people use video
  cameras and LiDAR sensors and leverage object detection deep neural networks
  (DNNs) to sense the surrounding environment and avoid potential collisions. In
  augmented reality, people use video cameras and LiDAR sensors to localize the
  remote objects and render the virtual objects on top of real objects. This
  trend inspires system research for these applications, like live
  analytics~\cite{??}, retrospective analytics~\cite{??}, database for analytic
  purpose~\cite{vstore,noscope}, etc.

  We identify two important characteristics of these systems. First, they
  contain large configuration spaces (\eg in AWStream~\cite{awstream}, there are
  216 different configurations inside its configuration space). Second, these
  configurations need to be \textit{timely} adapted according to their input
  (\eg we may want to use higher video resolution when a small car enters the
  video frame in order to detect this small car) and the current resource budget
  so that they can generate the inference results as accurate as possible.

  As a result, the key challenge for these systems is: how to navigate the large
  configuration space and pick the optimal configuration that generates the most
  accurate inference results under the current resource budget.

  The first way to address this problem is to \textit{frequently profile} the
  system with different configurations to obtain their resource usage and
  inference accuracy, and then pick the configuration that meets the resource
  budget and generates the most accurate inference
  results~\cite{awstream,chameleon,vstore}. However, in order to profile, this
  approach has to perform \textit{extra} inference on the GPU, resulting in high
  GPU cost.

  The other approach performs no extra inference and instead, picks the
  configuration based on the recent configuration and its corresponding DNN
  output. However, there can be many configurations that meet the resource
  budget. Without profiling most of them, it is difficult to separate the
  configurations that yield similar DNN output from those that yield more
  accurate DNN output. In addition, the previous work in this approach designs
  hand-craft heuristics catered for different applications.

  Thus, the requirements of an ideal configuration adaptation system are
  three-fold:
  \begin{enumerate}
    \item No extra DNN inference
    \item Pruning out the configurations with similar accuracy
    \item Agnostic to the underlying applications
  \end{enumerate}

  We present our system: \name that meets these three requirements. The idea is
  to calculate the \textit{gradient} of inference accuracy with respect to the
  configurations to \textit{predict} which of them improve inference accuracy
  and which do not. The key insight that enables us to calculate this gradient
  is by decoupling this gradient into two terms. The first term is the gradient
  of inference accuracy with respect to the DNN input, which can be calculated
  by backpropagation without performing extra inference on any other
  configuration. The second term is the gradient of the DNN input with respect
  to the configurations, which does not require DNN inference.

  To make our system practical, we also identify another source of overhead
  introduced by calculating inference accuracy. In order to calculate inference
  accuracy, previous work needs to refer to the configuration with \textit{the
  most} resource usage and use the corresponding inference results as the
  ``ground truth'' to evaluate the accuracy of inference results generated from
  other configurations. Calculating the ``ground truth'' uses much higher
  resource usage (including the streaming cost of streaming the data and the GPU
  cost to generate inference results) than the current optimal configuration. To
  reduce this cost, we introduce a \textit{proxy} of accuracy that
  \textit{indirectly optimizes} accuracy by using the DNN input (instead of the
  DNN output), thus requiring no DNN inference.

  To conclude, the contributions of this paper are:
  \begin{enumerate}
    \item A way to calculate gradient with no extra inference
    \item An accuracy proxy that indirectly optimizes the accuracy without
          running extra inference.
  \end{enumerate}
  We quantitatively evaluate these two contributions, we perform experiments on
  XXX datasets, XXX applications and XXX

\end{comment}


==> motivate.tex <==



\begin{table*}[h]
    \begin{tabular}{ c c c c}
        \hline
        Systems & Knobs & Trade-off between accuracy and & Can be handled by \name \\
        \hline
        % \footnotesize Streaming delay & \footnotesize Video encoding parameters, region-of-interest \\
        % \footnotesize Number of data frames & \footnotesize Data frame difference thresholds \\
        % \footnotesize DNN inference time & \footnotesize model selection, model customization \\
        \cite{awstream,dds,chameleon,vstore,videostorm,deepdecision,adascale} & Resolution & Bandwidth usage (and GPU compute) & \cmark \\
        \cite{awstream,vstore} & Quantization parameter & Bandwidth usage & \cmark \\
        \cite{deepdecision} & Video bitrate & Bandwidth usage & \cmark\\
        \cite{vstore} & Encoding preset & Bandwidth usage & \cmark  \\
        \cite{awstream,chameleon,vstore,videostorm,deepdecision} & Frame rate & Bnadwidth usage and GPU compute  & \cmark \\
        \cite{reducto,glimpse,vigil} & Frame filtering threshold & Bandwidth usage and GPU compute & \cmark \\
        \cite{accmpeg,dds,eaar,saliency_hotmobile} & Fine-grained spatial quality assignment & Bandwidth usage & \cmark \\
        % \cite{cinet,vigil} & Region cropping & Bandwidth usage and GPU compute & \cmark \\
        \cite{noscope,ekya} & Model customization & GPU compute  \\
        \cite{chameleon} & Model selection & GPU compute &  \\
        \cite{cloudseg} & Server-side super resolution & Bandwidth usage  \\
        \cite{videostorm} & Server-side DNN parameter & GPU compute \\
        \hline
    

\end{tabular}
\caption{Distributed AI systems introduce rich types of knobs to trade-off between analytic accuracy and end-to-end delay (including sensor-side delay, streaming delay and server-side inference delay)}
\label{tab:rich-set-of-knobs}
\end{table*}
    

\begin{figure}
    \includegraphics[width=1.\columnwidth]{figs/contrast-previous-and-ours.jpg}
    \caption{Contrasting how previous work and our approach recognize crucial areas on the input. The color indicates the importance of}
    \label{fig:feedback-contrast}
\end{figure}


\section{Motivation}

\subsection{Systems for deep learning applications}


\begin{itemize}
    \item Deep learning applications for data streams are everywhere.
    \item System research on these applications are rapidly emerging.
    \item Performance metrics: 1). accuracy 2). end-to-end delay
    \item Systems for these applications need to be adaptive.
    \item In order to be adaptive, these systems define a set of parameters, and timely vary the value of these parameters 
\end{itemize}


Nowadays, distributed AI applications are everywhere. \kt{several examples here}

Facing this growing demand, system research on those distributed AI applications are rapidly expanding. From sensor-side data filtering~\cite{glimpse} and compression~\cite{vigil,cinet,accmpeg,VCM}, server-side model selection~\cite{chameleon}, training~\cite{noscope,ekya} to server-sensor co-optimization on configuration optimization~\cite{awstream}, data-of-interest detection~\cite{eaar,dds}, parallel inference~\cite{elf}.

\mypara{Performance metrics}
The performance metrics of these pipelines are analytic accuracy\footnote{We use the analytic results on the uncompressed video with the most expensive anlaytic model as the ground truth to measure accuracy} and end-to-end delay, including sensor-side processing delay, streaming delay and server-side inference delay.


\mypara{Estimating the accuracy is the key}
Different from end-to-end delay that can be cheaply controlled and estimated, accuracy is much more difficult to estimate. This is because

% \mypara{Ai analytic pipelines propose a lot of knobs}
% As different applications may have different requirements to anlaytic accuracy and end-to-end delay, these distributed AI systems introduce rich set of tunable hyper-parameters (we call these tunable hyper-parameters \textit{knobs}) to trade-off between analytic accuracy and end-to-end delay.
% (Table ~\ref{tab:rich-set-of-knobs} illustrates the rich set of knobs of distributed AI anlaytic systems and their corresponding trade-off).
% % Despite their superior performance, all of these systems introduces internel knobs that matters a lot to their performance. 



% System research on AI applications are emerging.

% \begin{figure}
%     \includegraphics[width=1\columnwidth]{figs/delay-breakdown.png}
% \end{figure}


% These systems invent different type of knobs to trade-off between accuracy and end-to-end delay, which is mainly determined by three parts:
% \begin{itemize}
%     \item Sensor processing delay
%     \item Streaming delay
%     \item DNN processing delay, which is mainly determined by number of data frames (the \textit{minimum} amount of data that can be consumed by the DNN) to be processed and inference time of the DNN.
% \end{itemize}
% \kt{Mention that sensor processing delay is typically used as a cost to optimize other delays}


% A category of related work

% Limitation discussion: we do not handle DNN change in our framework.


\subsection{Trends of knobs}

\begin{itemize}
    \item 
    Terminologies: 
    1. Knob: a parameter that controls the system, \eg video resolution
    2. Values: the values that the configuration parameter can choose from (\eg 480p, 720p, 1080p)
    3. Configuration: defined as the chosen value of all parameters inside one system. This is the minimum unit in order to let the system run. 
    4. Configuration space: the set of all possible configurations.
    \item Number of knobs are growing. First, new knobs are emerging to explore new trade-offs. Second, old knobs are breaking down to multiple find-grained parameters to squeeze out more potential from the same trade-off.
    \item 
    Exploring more knobs can provide more performance gain.
    1. multiple configurations can optimize multiple components of the end-to-end delay, while one configuration typically optimizes only one component of the end-to-end delay.
    \eg video encoding quality $\rightarrow$ streaming delay; server-side DNN selection $\rightarrow$ server-side delay
    2. even in the case that multiple configurations are actually reducing the same components of the delay, having multiple configurations allow the system to capture more opportunities to reduce the delay.
    \eg video resolution $\rightarrow$ can reduce the streaming delay when the objects are large. video frame rate $\rightarrow$ can reduce streaming delay when the objects only appears in a subset of frames.
    So having both of them may result in a much higher gain when the objects are large and only appears in a subset of frames.
    
    
    % \item Most of the parameters are operating on DNN input.
\end{itemize}







\subsection{Configuration adaptation}


\begin{itemize}
    \item
    Previous work observes that: optimal configuration varies as the video content and the resource budget changes.
    As a result, we need to \textit{adapt} the configurations.
    \item 
    The first type of work deploys heuristics that are \textit{agnostic to real-time DNN output} to adapt the configuration.
    However, as previous work shows, without real-time DNN output, these heuristics are inaccurate and resulting in either resource waste or low inference accuracy.
    \item The second way to address this problem is to \textit{frequently profile} the system with different configurations to obtain their resource usage and inference accuracy, and then pick the configuration that meets the resource budget and generates the most accurate inference results.
    However, this approach needs to perform \textit{extra} inference.
    \item The other approach performs no extra DNN inference and instead, picks the configuration based on the recent configuration and its corresponding DNN output (\eg pick the configuration through cheap heuristics~\cite{dds,eaar,elf} or through DNN-based configuration generator~\cite{accmpeg,casva}).
    However, there can be many configurations that meet the resource budget.
    Without profiling most of them, it is difficult to separate the configurations that yield similar DNN output from those that yield more accurate DNN output.
    As a result, they cannot quickly identify the optimal configuration.
    \item
    In addition, the previous work in this approach designs hand-crafted heuristics catered only for individual applications or configurations.
    \item 
    We desire a configuration adaptation system that meets three requirements: 1. quickly adapt to optimal configuration in a large configuration space without extra inference
    % pruning out the configurations that yield similar inference accuracy 
    2. minimum assumption to the underlying applications
\end{itemize}


% \mypara{Termiologies}
% To avoid potential confusion, we clarify several terms that we will use.
% \begin{packeditemize}
%     \item \textbf{Hyper-parameters (HPs):} the tunable hyper-parameters inside distributed AI systems. \qz{do you mean that HPs can also be referred to as knobs?}
%     \item \textbf{Knob values:} the candidate values that one knob can choose from.
%     \item \textbf{Configuration:} the concrete \textit{choice} of knob value for each knob. The configuration represents  
% \end{packeditemize}




\begin{comment}


\mypara{More knobs, more gain}
Further, as AI systems keep on developing new knobs that may rely on different characteristics \qz{this word sounds weird, maybe say more knobs are available for tuning in AI systems and allow us to save resource usage in different fashions} to reduce the resource usage (and thus reduce the delay),  tuning more knobs altogether may provide huge potential. 
Take camera-based object detection as an example.
Assume that only 20\% of the frame is occupied by the objects, and the object only appear in 20\% of the frames.
In this case, tuning frame filtering knobs or tuning spatial encoding quality reduce the number of pixels streamed out by 5x, thus achieving 5x saving on streaming delay in ideal cases\footnote{The actual streaming delay reduction will be lower because codec compression becomes more efficient when there are more pixels for the codec to use as reference.}.
However, if we tune frame filtering knobs and spatial encoding quality knobs together, we only need to stream out $20\% \times 20\% = 4\%$ pixels, resulting in a 25x reduction on the streaming delay. \yh{add an example showing the benefits brought by coupling more knobs on reducing e2e delay }

\mypara{Knobs need to be frequently tuned}
To achieve the best \qz{optimal} trade-off between analytic accuracy and end-to-end delay, however, these knobs need to be \textit{frequently} tuned according to the incoming video content.
Take AccMPEG~\cite{accmpeg} as an example system and camera-based vehicle detection as an example application.
AccMPEG introduces the encoding quality of different spatial areas as its knob.
It will aggressively compress those areas that are not related to the vehicles to reduce the streaming delay.
So when a new object arrives, AccMPEG need to quickly adjust \qz{adapt} its knob to avoid aggressive compression on the areas related to the new incoming object.
If AccMPEG does not adjust this knob, this object may be missed and result in low analytic accuracy.
\kt{Provide empirical evidences here}



\mypara{Previous work make inaccurate prediction of accuracy under current video content}
In order to adjust the configuration, previous work either leverages a sensor-side model to predict the accuracy of different configurations, or use server-side feedback to perform this prediction.
However, both of these two approaches predict accuracy in a sub-optimal way.

\kt{Then say previous work cannot get this}

\kt{Emphasize there are a lot of knobs}
\kt{Emphasize that there are certain set of knobs that achieves combinitorial effect}

\begin{table*}
    \begin{tabular}{ c c c c }
        \hline
        Place & Analytic model & Number of inferences per second & Total FLOPs per second \\
        Server & EfficientDet~\cite{efficientdet} (300G FLOPS) & 30 & 9000G FLOPs \\ 
        Sensor & MobileNet SSD (2.3 GFLOPS)~\cite{ssd,ssd-runtime} & 23~\cite{ssd-fps,ssd-fps2} & 53G FLOPs (169x) \\
        \hline
    \end{tabular}
    \caption{Comparison between server-side and sensor-side compute. The server has hundreds times more compute than the sensor.}
    \label{tab:sensor-server-comparison}
\end{table*}

The first type of work use sensor-side model to obtain knob-accuracy impact.
This model can be completely offline~\cite{vigil,glimpse,accmpeg} or periorically downloaded from the server~\cite{awstream,reducto}.
However, as shown in Table compared to the server that can run heavy analytic models (that contains hundreds of layers and requires hundereds of GFLOPs~\cite{efficientdet,retinanet,amoebanet}) in real time (\eg 30 inferences per second), the sensor can only afford several GFLOPs even with the help of external hardware acceleration\cite{ssd,ssd-runtime}.
As a result, the sensor-side model will have low accuracy when there are sudden changes in the incoming video content (\kt{several examples here}), resulting in sub-optimal accuracy-delay trade-off.


The second type of work infer knob-accuracy impact from real-time server-side output (including intermediate output, like region proposals~\cite{dds,elf,eaar}).
% Some previous work will directly obtain the knob-accuracy impact on a small chunk of video by exhaustively enumerate all knobs and their corresponding values and calculate the accuracy of these values on the whole video. 
% However, this procedure introduces high streaming delay (the video need to be streamed in an uncompressed manner, which requires >10x time to stream from the camera to the server) and inference delay (one may need to even analyze >200 configurations to tune just 3 knobs~\cite{awstream}). 
% As a result, this approach cannot obtain the knob-accuracy impact \textit{in real-time}. 
% The other type of work will infer the knob-accuracy impact from the intermediate output of the DNN.
As shown in Figure~\ref{fig:feedback-contrast}, after obtaining the DNN output\footnote{Some previous work may perform filtering to remove those outputs that, for example, have low confidence~\cite{dds,eaar}.}, previous work will overlay these outputs on the input to obtain a set of pixels, and assume those knobs that related to the pixels have high knob-accuracy impact. 
However, the pixels that indicates high knob-accuracy impact do not necessarily align with the shape of inference results.
Instead, some pixels outside the bounding boxes may contribute to the analytic results, and some pixels inside the bounding boxes may have low accuracy impact.
This is because the pixels that outside the bounding boxes also participant in the computation of obtaining the inference results; the contribution of pixels inside the bounding boxes may be inhibited by the internel DNN computation (like ReLU activation and pooling).
As a result, it cannot deliver accurate knob-accuracy impact by simply overlaying the output on the input.


% These knobs need to be adjusted with the feedback from server-side DNN.

% First type of work: fixed parameter

% Second type of work: camera-side heuristics

% Thrid type of work: real-time feedback

% However, their feedback is suboptimal because they essentially rely on the output of the DNN to provide feedback.
% The output only encodes the results of the computation, but loses the information of how the DNN perform this computation.
% The latter is aso important to determine the relationship between knobs and the final analytic accuracy.


% An example here.

\end{comment}

==> motivate_0129.tex <==
%!TEX root = main.tex
%!TEX spellcheck = en_US 


\tightsection{Motivation}
\label{sec:motivate}

We start with the background of video streaming for distributed video analytics, including its need, performance metrics and design space. 
We then use empirical measurements to elucidate the key limitations of prior solutions. 

% \jc{need a brief primer on object detection and semantic segmentation}

\tightsubsection{Video streaming for video analytics}
\label{subsec:dva}


% \mypara{Distributed video analytics (DVA)}
% Many AI applications extract useful information from live video streams in a {\em distributed} fashion, because the analytics happens partially or completely in servers connected to cameras through network links.

%DNNs achieve very high accuracy on these vision tasks and are thus widely used.

\cameranew{
\mypara{Example vision tasks}
This paper consider three example vision tasks, object detection, semantic segmentation, and face recognition. 
Figure~\ref{fig:??} shows example outputs of typical object detection models (a label per bounding box) and semantic segmentation (a label per pixel).
These tasks are widely used in real-world scenarios to either detect/segment objects of interest and use the results for high-level applications (\eg vehicle collision detection). 
}

\myparashort{Why streaming videos out from cameras?}
There are two contributing trends.
% Two trends contribute to the wide spread of distributed video analytics and much recent effort (\eg~\cite{awstream,cloudseg}).
%On one hand, low prices of high-definition cameras have led to a dramatic proliferation of video sensors~\cite{McKinsey,infowatch16,thenewstack,asmag}. % whose video feeds need automatic and accurate analysis~\cite{thenewstack,asmag}. 
On one hand, computer vision accuracy has been greatly improved by deep learning at the cost of increased compute demand.
On the other hand, low prices of high-definition network-connected cameras make them widely deployed in traffic monitoring~\cite{killer-app}, video analytics in retail stores~\cite{retail-video}, and inspection of warehouses or remote industrial sites~\cite{george2019towards}. 
Thus, the camera operators must scale out the compute costs of analyzing ever more camera feeds~\cite{McKinsey,thenewstack,asmag}, and an economical way of scaling out camera networks is to {\em offload the compute-intensive inference (partially or completely) to centralized GPU servers}. 
% have enabled cheaply scaling out the analytics of ever more cameras~\cite{McKinsey,thenewstack,asmag}.
% While one can always add accelerators~\cite{jetson,deeplens} to cameras, 
For instance, buying 180 HD cameras and an NVIDIA Tesla T4 GPU (with a throughput of 5,700fps~\cite{tesla-benchmark}) to process the feeds each at 30fps (total 5,400fps) costs $\$25\times180$\textrm{(cameras)\cite{amazon-hd-cam}}$+\$2000$\textrm{(GPU)\cite{amazon-gpu}}$=\$6.5$K; whereas buying 180 NVIDIA Jetson TX2 cameras (each runs ResNet50 barely at 30fps) costs about $\$600$\cite{jetson-price}$\times180$ $= \$108$K, 1-2 orders of magnitude more expensive.
% Therefore, camera network operators increasingly stream videos from network-connected cameras to servers for deep learning inference in traffic monitoring~\cite{killer-app}, surveillance in buildings, video analytics in retail stores~\cite{retail-video}, and inspection of warehouses or remote industrial sites with drone cameras~\cite{george2019towards}. 
That said, in some settings, video feeds must be processed locally due to privacy regulations, but they are beyond the scope of this work.



\cameraold{
% \myparashort{Why saving bandwidth?}
%First, while they are not as much, it's growing fast.
We aim to reduce bandwidth usage of video analytics for three reasons.
First, while many Internet videos are still destined to viewers, the video feeds processed by analytics engines have grown dramatically;
by one analysis, the amount of data generated by new video surveillance cameras installed in 2015 is equal to all Netflix's current users steaming 1.2 hours of ultra-high HD content simultaneously~\cite{infowatch16}.
%Second, the cost can be higher per stream than streaming video to users
Second, many cameras are deployed in the wild with only cellular network coverage~\cite{IoT-cellular}, so setting up network connections and sending videos upstream to remote servers can be expensive (more so than streaming videos from CDN servers to wifi-connected PCs).
%Third, compared to servers, the cost cannot be amortized
Finally, while purchasing GPU servers is not cheap, it is a one-time cost that is amortized over time (so cheaper in the long run); while the communication cost is not amortized thereby incurring substantial operational costs for many large-scale camera networks.%~\cite{IoT-cellular}. 
}


%
%Although video feeds destined to analytics are currently not as many as Internet videos destined to viewers
%
%
%the volume of video streams is experiencing a super-linear growth of video sensors whose video streams are tied to the continuous activity of all video sensors~\cite{ChicagoCam,LondonCCTV,VideoAnalyticsMarket,slate-video-news,infowatch16}.
%
%
%
%
%and the need for bandwidth efficient streaming.
%
%
%
%
%This work mostly focuses on reducing the bandwidth usage while maintaining high accuracy. 
%This is because lower bandwidth demand means that the server-side DNN will receive data more quickly and the communication cost will be lower. 
%Unlike cost of purchasing in-house servers can be amortized over time, the communication cost cannot and could be a major contributing factor to the operational cost of a large-scale camera network~\cite{IoT-cellular}. 


% : Buying 180 HD cameras (at less than \$30 each) and a NVIDIA Tesla T4 GPU (at \$2,000) that has a benchmarked ResNet throughput of 5,400 images per second~\cite{tesla-benchmark} is at least one order of magnitude cheaper than buying 180 NVIDA Jetson TX2 cameras (at more than \$600 each) which achieves the same throughput~\cite{jetson-benchmark}.
%\jc{get a quote on the cost of 100 hd cameras + 100 cloud gpus vs. 100 jetson cameras}


% \jc{introduce object detection and face recognition, and they are widely used} \hh{If you have references for each of these scenarios, it would be very helpful to add a citation for each to back up the claim of wide usage.}


\mypara{Performance metrics}
An ideal video streaming protocol for video analytics should balance among three metrics: accuracy, bandwidth usage, and freshness.
Here, we define them in multi-class object detection and semantics segmentation. %and \S\ref{subsec:eval-method} will define them in face recognition and semantics segmentation as well.
\begin{packeditemize}
	\item {\em Accuracy:} 
	\cameranew{We define accuracy by the {\em similarity} between the DNN output when the video is streamed under limited bandwidth and the DNN output on the original (highest quality) video, rather than the human-annotated labels.
	This allows us to capture any negative impact of video compression and streaming on DNN inference, without being affected by any errors made by the DNN itself.
% 	of video streaming protocol and the inference results under unlimited bandwidth.
	We measure accuracy }
    \cameraold{Accuracy is measured}by the standard metrics: {\em F1 score} for object detection (the harmonic mean of precision and recall for the detected objects' location and class labels) and IoU for semantic segmentation. 
    We use the outputs of running the server-side DNN over the video in its highest quality as the reference and treat them as the ground truth when calculating accuracy.
	This is consistent with other work (\eg~\cite{awstream,chameleon,videostorm}). %\jc{need to be changed once eval is updated}
% 	Similarly, we use F1 score as an accuracy metric in face recognition by calculating precision and recall of the detected faces' location and identities.
% 	As a baseline, we consider the best possible accuracy to be that achieved when the highest quality video is sent to the server in its entirety.
    \cameranew{
    \item {\em Bandwidth usage:}
    % \item {\em Cost:}
    In general, the costs of operating a video analytics system include the camera cost, the network cost paid to stream the video from the camera to the server, and the cost of the server.
    In this paper, we focus on reducing the streaming cost through reducing the bandwidth usage. 
    \S\ref{subsec:cost-accuracy-delay} will highlight deployment settings in which the total costs of a video analytics system are dominated by the network cost, thus reducing bandwidth usage is crucial.
    % We further divide this sum by the number of cameras and the number of frames to make this metric agnostic to them.
%     }
% 	\item {\em Bandwidth usage:} 
% 	\cameranew{
%     To reduce the cost, our work focuses 
%     So we also put bandwidth usage here as a metric.
    }
	We measure the bandwidth usage by size of the sent video divided by its duration. 
% 	\eg if some camera-server connections go through cellular networks that charge proportional to the data usage.
	\item {\em Average response delay (freshness):} %\kt{Response delay -> Processing delay for consisitancy?}
	Finally, we define freshness by the average processing delay per object, \ie the expected time between when an object first appears in the video feed and when its region is reported and correctly classified, which includes both the time to transmit to the server and run inference. 
	We report the average delay. 
	%\hh{This one reads a little funny.  It sounds like objects that aren't detected would decrease the average delay.  Could we just say that the processing delay is the time between when pixels are produced and the analytics produces the final result for those pixels?}
\end{packeditemize}
% \hh{Consider cutting the paragraph below for space}.
% DVA requires streaming support that simultaneously achieves high accuracy, low bandwidth, and low response delay.









%\jc{need to make a stronger case for saving (even just 2x) bandwidth. see more details in todos}
% Note that processing delay and bandwidth demand are related not always correlated,
% , but bandwidth demand sometimes can be reduced at the cost of increased processing delay, 
% \eg by adding more  frames, one can significantly reduce the video size but at the same time the server needs to accumulate more frames before being able to decode the video and run inference. 
% For the sake of explanation, we preclude the use of tricks and compare different solutions in accuracy and bandwidth demand while keeping processing delay at a constant low value.
% However, we will evaluate all three dimensions in \S\ref{sec:eval}.

% \jc{also need to make clear how much computing power we assume on the client and server}

%\begin{itemize}
%    \item video analytics is popular. a common practice is to stream videos to a remote server for compute-intensive analysis
%    \item two main metrics of success: accuracy, real-timeness. in this paper, we focus on object detection, face recognition.
%\end{itemize}




%\jc{when is it a good trade to reduce the number of bits transported at the expense of server-side GPU resources?}


\tightsubsection{Design space of video analytics systems}

\cameranew{
Next, we describe the broader design space of how video analytics systems can potentially navigate the balances among these performance metrics along five dimensions:
% To demonstrate how existing works explored the design space of serving a single video stream for analytic purpose, we present a overview on the existing design dimensions. These dimensions are:

\begin{packeditemize}

\item {\em Leveraging camera-side compute power:}
Since cameras (video sources) can naturally access the raw video, one can leverage the camera's local compute power (if any) to discard frames~\cite{noscope,glimpse}/regions~\cite{eaar,vigil} that do not contain important information.
As we will elaborate in \S\ref{subsec:machine-centric}, the accuracy of such local discard logic may cause significant accuracy drops.
% The advantages for camera are that the camera not shared by any other video stream and could assess the raw video with no delay. To leverage this property, Vigil\cite{vigil} and Glimpse\cite{glimpse} harvest the compute at the camera to propose key frames and reduce the inference cost.


\item {\em Model distillation:} DNNs are often trained on large datasets, but when used exclusively for a specific video scene, a DNN can be ``shrunk'' to a smaller size (\eg via knowledge distillation), in order to save compute cost without hurting accuracy (\eg NoScope\cite{noscope}).
This approach is efficient only when dealing with scenes where the object set and background change very slowly~\cite{noscope}.
% but are actually used on a single video stream. By training on this video stream, we could effectively ``shrink'' the deep learning models, thus save the inference cost. (e.g.: NoScope\cite{noscope}).

\item {\em Video codec optimization:} 
Unlike traditional video codecs that optimizes for human visual quality, video analytics emphasizes inference accuracy and thus opens up possibility to more analytics-oriented video codec (\eg analytics-aware super resolution~\cite{cloudseg}).\cameraold{\item Edge-based optimization. The edge strike a balance between the two extreme: accessing the video content fast and free but has limited compute (like the camera) and equipping sufficient compute but are bounded by the network latency and bandwidth  (like the server). Thus, there are a lot of previous works that exploits this design dimension (e.g. EAAR\cite{eaar}).}



\item {\em Temporal configuration adaptation:} 
To cope with the temporal dynamism of video content, one can adapt its configurations (\eg frame rate, resolution or DNN models) over time to save compute costs~\cite{chameleon} or network costs~\cite{awstream}.
That said, this approach fails to exploit the uneven spatial distribution of important information in videos. 



\item {\em Spatial quality adaptation:}
Information of interest (\eg target objects) is sparsely distributed in each frame, so some pixels are more critical to accurate DNN inference than others.
One can encode each frame with a spatially uneven quality distribution (\eg RoI encoding~\cite{eaar}) such that the video quality is aligned with DNN's ``attention'' to save bandwidth~\cite{eaar,vigil} and increase accuracy~\cite{mnih2014recurrent}. 
% Our work also lies in this design dimension.
% Note that this optimization could also reduce the streaming delay through transferring less data through network.

\end{packeditemize}

In this paper, we take a pragmatic stance to focus on a specific point in this design space---no change to the camera (no camera-side logic, except encoding), the server-side DNN (no model distillation) or the video codec, and using server-side DNN output to drive the temporal and spatial adaptation of quality levels.

}

\begin{figure}
\centering
\includegraphics[width=0.92\columnwidth]{figs/contrast-user-machine-new.pdf}
\tightcaption{Contrasting video streaming for human viewers and machine-centric video streaming leads to unique bandwidth-saving opportunities. 
% such as frame dropping and spatial cropping.
}
\label{fig:contrast}
\end{figure}

\tightsubsection{Potential room for improvement}
\label{subsec:machine-centric}


% We argue that video streaming for video analytics presents abundant opportunities to improve accuracy and bandwidth usage, but the opportunities are largely untapped since current solutions are largely based on protocols designed for traditional video applications (\eg YouTube, Netflix).


% \mypara{New opportunities} 
Traditional video streaming maximizes human quality of experience (QoE)---a high video resolution and smooth playback (minimum stalls, frame drops or quality switches)~\cite{festive,conviva-understanding,akamai-qoe}. 
For machine-centric video streaming, however, it is crucial that server-received video has sufficient pixels in regions that heavily affect the DNN's ability to identify/classify objects; however, the received video does not have to be high definition or smooth at all.

% \ktedit{XXX}
% \kt{???}

% Traditional video streaming strives to maintain a high video resolution and smooth playback (minimum stalls, frame drops or quality switches)~\cite{festive,conviva-understanding,akamai-qoe}.
% In contrast, 
% video streaming for video analytics is {\em machine-centric}. 

% These differences open up new opportunities that would not have been possible in traditional video streaming. 
This contrast has profound implications that machine-centric streaming could achieve high ``quality'' (\ie accuracy) with much less bandwidth.
Each frame can be spatially encoded with {\em non-uniform quality levels}.
In object detection, for instance, one may give low quality to or even blackout the areas other than the objects of interest (Figure~\ref{fig:contrast}(b))\footnote{This may look like region-of-interest (ROI) encoding~\cite{meddeb2016region}, but even ROI encoding does not completely remove the background either, and the ROIs are defined with respect to human perception.}. 
While rarely used in traditional video streaming,
% , but seeks to maintain a smooth quality degradation from where users are likely to see to the background.
this scheme could significantly reduce bandwidth consumption and response delay, especially because objects of interest usually only occupy a fraction of the video size.
Figure~\ref{fig:motivation-spatial-cdf} shows that across three different scenarios (the datasets will be described in \S\ref{subsec:eval-method}), in 50-80\% of frames, the objects of interest (cars or pedestrians) only occupy less than 20\% of the spatial area.
We also observe similar uneven distributions of important pixels in face recognition and semantic segmentation.
% \hh{Without tick marks on the axes, I don't think you can draw these conclusions from the chart.  Is this just a placeholder for now?}
% Second, along the temporal dimension, frames can be sampled non-uniformly so that more frames should be sampled when objects are moving quickly and fewer frames are sampled when objects are moving slowly (or no object of interest is present).
% This opens up more opportunities to save bandwidth, since fast-moving objects may not be dominant.
% For instance, we found that in \fillme dataset, \fillme\% of the objects moves at very low speeds so that a frame rate of 1 frame-per-second (fps) is sufficient to identify its location, whereas the original videos are 30fps.
The question then is how to fully explore the potential room for improvement?


\begin{figure}
\centering
\includegraphics[width=0.67\columnwidth]{figs/motivation-cdf.pdf}
\tightcaption{Bandwidth-saving opportunities: Over 50-80\% of frames, the objects (cars or pedestrians) only account for less than 20\% of the frame area, so most pixels do not contribute to the accuracy of video analytics.
%This property suggests assigning quality levels non-uniformly could greatly reduce bandwidth demand without hurting accuracy.
}
\label{fig:motivation-spatial-cdf}
\end{figure}


%\begin{itemize}
%    \item unique opportunities in video streaming compared to traditional video streaming (Figure~\ref{fig:contrast}):
%    \begin{itemize}
%        \item no need for uniform frame sampling
%        \item no need for background, etc
%    \end{itemize}
%\end{itemize}




% \tightsubsection{Taxonomy of current solutions}
% \label{subsec:taxonomy}


\begin{figure}
\centering
\includegraphics[width=0.65\columnwidth]{figs/det_demonstrate_tradeoff.pdf}
\tightcaption{Current solutions exhibit a rigid bandwidth-accuracy tradeoff: any gain in accuracy comes at a cost in bandwidth.
The results are based on the traffic videos in our dataset %\kt{do we need to add cloudseg in this graph?} 
(\S\ref{subsec:eval-method}).}
\label{fig:motivation-tradeoff}
\end{figure}

\mypara{Limitations of existing solutions}
Existing solutions for video streaming are essentially {\em source-driven}---the decisions of how the video should be compressed or pruned are made at the source with no real-time feedback from the server-side DNN that analyzes the video.
However, they show unfavorable trade-off between bandwidth and accuracy  (illustrated in Figure~\ref{fig:motivation-tradeoff}): any gain of accuracy comes at the cost of considerably more bandwidth usage.
The fundamental problem is that any heuristic that fits camera's limited compute capacity is unlikely to precisely imitate a much more complex DNN, with no real-time feedback from it. 

This problem manifests itself differently in two types of source-driven solutions.
The first type is {\em uniform-quality streaming} that modifies the existing video streaming protocols and adapts the quality level to maximize inference accuracy under a bandwidth constraint.
AWStream~\cite{awstream} uses DASH/H.264 and periodically re-profiles the inference accuracy under each quality level. %and select a lower-than-throughput quality level with maximum inference accuracy. 
CloudSeg~\cite{cloudseg} sends a video at low quality but upsizes the video by super resolution by the server.
They have two limitations: 
First, they do not leverage the uneven distribution of important pixels; instead, the videos are encoded by traditional codecs with a spatially uniform quality. 
Second, while AWStream does get feedback from the server DNN, it is not based on real-time video content, so it cannot suggest actions such as increasing quality on a specific region in the current frame.

The second type is {\em camera-side heuristics} that identifies important pixels/regions/frames that contain information needed by the server-side analytics engine (\eg queried objects)  by running various local heuristics (\eg checking significant inter-frame difference~\cite{glimpse}, a cheap vision model~\cite{adascale,nn-meets-pn,vigil,noscope}), or some DNN layers~\cite{cracking,ddnn}.
These solutions essentially trade camera-side compute power to run inference for better accuracy/bandwidth trade-off~\cite{cracking}. 
For instance, some solutions (\eg~\cite{glimpse,noscope,eaar}) rely on the inter-frame differences to signal which frames contain objects, but any false positives (\eg pixel changes on the background) will cost unnecessary bandwidth usage and any false negatives will preclude the server from detecting important information (as illustrated in Figure \ref{fig:contrast-model}). 
% \jc{mention EAAR as relying on camera logic to select frames, though it uses some server-side information (region proposal) like Glimpse}
\cameranew{
We will discuss more related work in \S\ref{subsec:eval-overall}.
}

\begin{comment}

\mypara{Existing solutions} 
The question then is how to fully explore the potential room for improvement?
Existing solutions for video streaming are essentially {\em source-driven}---the decisions of how the video should be compressed or pruned are made at the source with no real-time feedback from the server-side DNN that analyzes the video.
These solutions fall in two categories:
\begin{packeditemize}
\item {\em Camera-side heuristics:}
A camera can run various local heuristics (\eg checking significant inter-frame difference~\cite{glimpse}, a cheap vision model~\cite{adascale,nn-meets-pn,vigil,noscope}), or some DNN layers~\cite{cracking,ddnn} to identify regions/frames that contain information (\eg queried objects) critical to the server-side analytics engine and send only these frames/regions to save bandwidth.
Camera-side heuristics essentially trade camera-side compute power to run inference for better accuracy/bandwidth tradeoffs~\cite{cracking}.
% For instance, Glimpse~\cite{glimpse} uses pixel changes to identify and send only frames in which queried objects are likely to emerge; and Vigil~\cite{vigil} identifies frames with most detected objects and sends only the object regions in those frames.
% Similar ideas can also be found in other video pipelines (\eg~\cite{noscope,fvc}) that are designed to save computation cost.
% uses a cheap inference model to discard frames that do not require complex DNN inference. 
% \jc{explain edge accelerator and/or noscope in more details if we end up using it as a baseline too, for e.g., Edge-based accelerators, such as EdgeTPUs or GPUs, speed up AI processing at the camera using better hardware albeit at higher cost while the model accuracy still does not match the server-side models.}

\item {\em Adaptive video streaming:} 
One can also to revamp existing video streaming protocol and adapt the quality level to maximize inference accuracy under the bandwidth constraint.
For instance, AWStream~\cite{awstream} is built on DASH/H.264 and periodically re-profiles the relationship between quality levels and inference accuracy, in order to select a lower-than-throughput quality level with maximum inference accuracy. 
CloudSeg~\cite{cloudseg} sends a video at low quality but upsizes the video by super resolution on the server side.
% Similar ideas can be found in other work~\cite{cloudseg,adascale}.
% image resolution and other encoding knobs should be tuned to improve accuracy, rather than visual quality. 

% \kt{cloudseg? It does not fall into two folders above.}
\end{packeditemize}



\mypara{Limitations of source-driven approach}
The premise of these techniques is that the camera-side logic can identify what is needed by the server-side analytics engine, thus achieving high accuracy with low bandwidth.
In reality, however, their bandwidth/accuracy tradeoffs (illustrated in Figure~\ref{fig:motivation-tradeoff}) can be quite rigid: any gain of accuracy comes at the cost of considerable more bandwidth usage.
% One can see that the tradeoffs are rigid---higher accuracy can only be achieved at the cost of greatly increased bandwidth usage.
The intuition is that any heuristic that fits camera's limited compute capacity is unlikely to precisely imitate a much more complex DNN, with no real-time feedback from it.
% (After all, if cameras can run a sufficiently complex logic that imitates the server-side DNN, there would be not need to send videos to the server in the first place.)
For instance, Glimpse~\cite{glimpse} and NoScope~\cite{noscope} rely on the inter-frame differences to signal which frames contain objects, but any false positives (\eg pixel changes on the background) will cost unnecessary bandwidth usage and any false negatives (\eg small objects) will preclude the server from detecting important information. 
On the other hand, analytics-aware streaming \kt{illustrate that these type of methods treats each objects uniformly, which essentially pays too much bw on high-confident (mostly large) objs and too little bw on low-confident (mostly small) objs? The following reason cannot explain why DDS still have performance gain even when the video is completely static, though it is still valid.} (\eg~\cite{awstream}) relies on accurate relationship between video quality and inference accuracy.
% that must be profiled constantly as the video content varies.
Such relationship is inherently dynamic: when the video content contains large objects (\eg a car passing closely in front of a camera), a low-resolution video still yields high accuracy, but when the video contains mostly tiny objects (\eg a car driving away from a camera), low resolution will not suffice.
Thus, frequent profiling is needed anytime the video changes its characteristics.

\end{comment}



\cameranew{

\begin{figure}[t]
\centering
\includegraphics[width=1\columnwidth]{figs/drone_16.jpg}
\tightcaption{Contrasting the inference results between cheap model (SSD-mobilenet-v2) and heavy model (Faster-rcnn-resnet101) on the same image. Heavy model is much more accurate when the video content is challenging.
\jc{update these figures?}
% \jc{this figure is a bit weird. why the small model (the left one) cannot detect large objects but can detect smaller ones?}
% \kt{The object size are nearly the same except for the one that lies in the middle of the road.}
}
\label{fig:contrast-model}
\end{figure}


}

\cameranew{
\tightsubsection{Tradeoffs among accuracy, cost and delay}
\label{subsec:cost-accuracy-delay}

Before diving to our design, we provide a framework to understand the performance---in costs, response delay, and accuracy---of existing solutions and our technique. 
% We will use the same framework to put the performance of our solution into perspective too.
An additional benefit of a performance framework like this is to provide performance clarity among current solutions which are often designed for different performance objectives (\eg minimize cost under given accuracy and delay constraints) and with different assumptions of the deployment settings (\eg resource availability of cameras, network, and servers).
The performance framework allows fair comparison among these solutions (and future ones) along the same metrics and in the same deployment settings. 
Although the exact performance of a solution can vary greatly in practice with factors such as the exact video content and choice of camera/server software, the framework focuses on primary factors that influence the performance of various solutions differently (while making identical assumptions about the accuracy and the latency of server-side DNN that affect all solutions) and is useful to qualitatively identify the ``operating regime'' of each solution (when one solution strikes a better performance tradeoffs than others).
We will illustrate the comparisons among these solutions using three concrete performance objectives and deployment settings.


% \kt{State that we could achive accuracy 1 if we stream the video in ultra-high quality from the camera to the server and inference on the server.}

% It is not enough to know that there is a potential new room for us to improve.
% Leveraging that room or not itself is a design choice.
% Every design choices will have the scenario where it is valid, and where it is likely to be sub-optimal. 
% However, the analysis that previous works provided are not able to inform people whether their approach works or not under {\bf a new scenario} that they did not talk about.


% Since it is relatively difficult to model inference accuracy, we instead study the cost model and delay model given the accuracy target $acc$ and the video analytic pipeline (VAP for short).
For each solution $\Pipeline$, a deployment setting $\Setting$ and a desirable accuracy target $\Accuracy$ \kt{(relative to the inference results at the server under unlimited bandwidth)}, we can estimate the cost and the response delay as follows:

\mypara{Cost model} 
We measure the cost by the cost to process, stream and analyze each frame from one camera, at a fixed frame rate of $30$ frames per second (FPS) and, for chunk-based streaming methods~\cite{awstream}, we use video chunk size of $15$ frames. % if the VAP chops the video to video chunks. 
As defined in \S\ref{subsec:dva}, the total costs are comprised of three parts: 
$$\Cost_{\camera}^{\Setting}(\Model^{\Pipeline}(\Accuracy))+\Cost_{\network}^{\Setting}(\Size^{\Pipeline}(\Accuracy))+\Cost_{\inference}^{\Setting}(\Workload^{\Pipeline}(\Accuracy))$$
where $Model^{\Pipeline}(\Accuracy)$, $Size^{\Pipeline}(\Accuracy)$ and $Workload^{\Pipeline}(\Accuracy)$ denote the client-side logic, network traffic, and the server-side workload (in fraction of frames analyzed by the server-side DNN) needed by $\Pipeline$ to achieve accuracy $\Accuracy$.
And $\Cost_{\camera}^{\Setting}(\cdot)$, $\Cost_{\network}^{\Setting}(\cdot)$ and $\Cost_{\inference}^{\Setting}(\cdot)$ are 
the camera cost, the network cost, and the server cost, respectively. 
Note that this model assumes each cost component depends only on one factor (\eg the server cost depends only on the fraction of frames to be analyzed by the server-side DNN). 
But this may ignore minor factors; \eg the server cost may also include that of periodic profiling of configurations~\cite{awstream}, though that only applies to particular solutions.

\mypara{Response delay model}
We measure the average response delay by the average delay spent to locally process (including buffering, encoding and possibly analyzing), stream and analyze (server-side inference and decoding) each frame. 
Optionally, the server-side inference results need to be given to the analyst but this delay would contribute equally to all solutions' response delay.
% We also fix the same frame rate and same chunk size as stated above. 
Thus, the average response delay could be represented as
% & t_{avg}^{VAP} && = t_{buf}^{VAP}+t_{cam}^{VAP} 
% + (1-\%cam)\cdot(t_{stream}+t_{serv}+t_{latency}),\\
% & t_{wst}^{VAP} && = t_{cam}^{VAP}+
% [\%cam<1]\cdot(t_{buf}^{VAP}+t_{stream}+t_{serv}),
$$
\Time_{\camera}^{\Setting}(\Model^{\Pipeline}(\Accuracy)) + \Workload^{\Pipeline} \cdot (\Time_{\network}^{\Setting}(\Size^{\Pipeline}(\Accuracy)) + \Time_{\inference}),
$$
where $\Time_{\camera}^{\Setting}(\cdot)$,
$\Time_{\network}^{\Setting}(\cdot)$ and
$\Time_{\inference}$ 
denote the average delay for the camera to locally process a frame, the streaming delay to send the video to the server, the server-side processing delay, respectively.
% Note that we assume that the decoding time at the server is nearly negligible (thanks to NVDEC~\cite{nvdec}).
% Note that this model only works on previous solutions. We will present the average response delay of \name at \S\ref{sec:overview}.

The aforementioned estimation of cost and response delay applies directly to existing solutions that stream each frame at most once, and it can later be extended to analyze the performance of our proposed solution that potentially streams a frame for multiple times.

% Our camera-side cost model is:
% $$
% \frac{cost_{cam}^{VAP}(acc)}{\#frames},
% $$
% where $VAP$ denotes the corresponding VAP, $cost_{cam}^{VAP}$ denotes the purchase cost at the camera side, which is a function of the accuracy target $acc$, and $\#frames$ denotes the number of frames streamed from one camera to the server.
% Our bandwidth cost model is:
% $$
% cost_{net}^{mode_{net}}(size^{VAP}(acc)),
% $$
% % Note that we need r_{\name} in delay calculation.
% where $cost_{net}^{mode_{net}}$ is the billing function for bandwidth, which differs with respect to different billing mode $mode_{net}$, and $size^{VAP}(acc)$ is the minimum average size of a single frame in order to hit accuracy target $acc$. Our server cost model is:
% $$
% cost_{serv}^{mode_{serv}}(\%cam, \#infs^{VAP}),
% $$
% where $cost_{serv}$ is the cost at server side dependng on the server-side billing mode $mode_{serv}$, which is a function of the percentage of camera-processed-only frames $\%cam$, and the number of DNN inference per frame $\#infs_{VAP}$.

% \mypara{Delay model} Note that we measure all the delay in seconds. 
% The first part of the delay is the time for the camera to buffer enough frames  $t_{buf}^{VAP}$ to construct a video chunk before sent. For those VAPs that chop videos to video chunks, 
% in the average case, $t_{buf}^{VAP} = \frac{15-1}{2\times30}\approx 0.23$ and in the worst case, 
% $t_{buf}^{VAP}=\frac{15-1}{30}\approx 0.47$. Otherwise, 
% $t_{buf}^{VAP}=0$
% The second part is the time for camera to do post-processing on the last frame of the video chunk (this is because previous frames are already post-processed while waiting for the corresponding next frame). 
% We denote this time as $t_{cam}^{VAP}$. 
% The third part is the streaming delay, we denote this time as $t_{stream}$.
% The fourth part of the delay is the time for the DNN to perform inference. This delay is equal to one-time inference on the DNN since the server could inference on multiple frames in parallel.
% The fifth part of the delay is the time for the server to transmit the results back to the camera. We call it $t_{latency}$ since it only depends on the network latency.
% Thus, for all VAPs except for \name, we write:
% \begin{alignat*}{2}
% & t_{avg}^{VAP} && = t_{buf}^{VAP}+t_{cam}^{VAP} 
% + (1-\%cam)\cdot(t_{stream}+t_{serv}+t_{latency}),\\
% & t_{wst}^{VAP} && = t_{cam}^{VAP}+
% [\%cam<1]\cdot(t_{buf}^{VAP}+t_{stream}+t_{serv}),
% \end{alignat*}
% where
% $[\%cam<1]$ means the truth value of proposition $\%cam<1$ and $t_{avg}^{VAP}$, $t_{wst}^{VAP}$ are the average delay and worst-time delay correspondingly.
% We will present the delay model for \name in  \S\ref{sec:overview}.


\begin{figure}[t]
\centering
    \subfloat[Cost v.s. accuracy]
    {
        \includegraphics[width=0.45\columnwidth]{figs/dds-suboptimal-cost-acc.pdf}
        \label{fig:suboptimal-cost-acc}
    }
    \subfloat[Worst-time delay v.s. accuracy]
    {   
        \includegraphics[width=0.45\columnwidth]{figs/dds-suboptimal-delay-acc.pdf}
        \label{fig:suboptimal-delay-acc}
    }
\tightcaption{The cost-delay-accuracy trade-off in real scenario on one video in example scenario 2. Vigil is the best.}
\label{fig:suboptimal-cost-delay-acc}
\end{figure}

\begin{figure}[t]
\centering
    \subfloat[Cost v.s. accuracy]
    {
        \includegraphics[width=0.45\columnwidth]{figs/dds_usecase_cost_acc.pdf}
        \label{fig:cost-acc}
    }
    \subfloat[Average delay v.s. accuracy]
    {   
        \includegraphics[width=0.45\columnwidth]{figs/dds_usecase_delay_acc.pdf}
        \label{fig:delay-acc}
    }
\tightcaption{The cost-delay-accuracy trade-off in real scenario on one video in example scenario 3. \name is the best.}
\label{fig:cost-delay-acc}
\end{figure}






}
% \tightsubsection{Limitations of current solutions}
% \label{subsec:limitation}


% So this approach is suboptimal, unless one can update the profile anytime there is a sudden change in content.

% In adaptive encoding, for instance, maintaining the relationship between quality levels and accuracy (as in~\cite{awstream}) can help, but this relationship will be obsolete whenever the video content varies:
% when the video content contains a large object (\eg a car passing through a camera), compressing the whole video with a low resolution will still yield high accuracy, but when the video content is a tiny object (\eg a car driving away from the camera), low resolution will not suffice.
% So this approach is suboptimal, unless one can update the profile anytime there is a sudden change in content.

% We argue that prior source-driven approaches have fundamental limitations due to the fact that they must make critical decisions that affect bandwidth/accuracy tradeoffs locally, with no real-time feedback from the analytics engine.
% The key reason behind the rigid tradeoff is that these solutions hope some simple heuristic that fits the camera's compute capacity can determine what the much more complex server-side DNN need to maintain high inference accuracy.
% After all, if the camera can run a sufficiently complex heuristic that imitates the server-side DNN, there would be not need to send videos to the server for more compute-intensive inference. 

% \mypara{Suboptimal performance}
% To put their performance into perspective, we consider an idealized solution, called {\em oracle}. 
% It sends out only regions around ground truth objects in the highest quality. 
% Since the oracle scheme uses hindsight information, its performance is not realistic. Nevertheless, it shows the potential bandwidth saving when achieving a high accuracy.
% Figure~\ref{fig:motivation-tradeoff} shows that the three schemes need \fillme-\fillme\% more bandwidth than the oracle to achieve the same accuracy. 
% We observe the same performance gap between them and the oracle on other videos, too. 
% Why does their performance fall so far behind the potential of machine-centric video streaming? 

% assumption made by these solutions that there exists some simple heuristic that fits the camera's compute capacity and can determine how the video should be compressed/streamed to maintain high inference accuracy.

%To get performance similar to ``oracle'', such hypothetical camera-side heuristic essentially needs to know when and where the objects of interest appear in the video.
% \mypara{Understanding the performance gap}

% Although prior work has considered various heuristics (a look-up table~\cite{awstream}, threshold on inter-frame difference~\cite{glimpse}, or a shallow neural-network model~\cite{adascale,nn-meets-pn,vigil,noscope}), none of them seems sufficient.
% In camera-side filtering, for instance, if one uses the pixel-level difference to determine which frame contains objects and send these frames~\cite{glimpse}, any false positives of this heuristics can cause unnecessary bandwidth consumption and any false negatives will prevent the powerful server-side network from having a chance to detect the object.
% In adaptive encoding, for instance, maintaining the relationship between quality levels and accuracy (as in~\cite{awstream}) can help, but this relationship will be obsolete whenever the video content varies:
% when the video content contains a large object (\eg a car passing through a camera), compressing the whole video with a low resolution will still yield high accuracy, but when the video content is a tiny object (\eg a car driving away from the camera), low resolution will not suffice.
% So this approach is suboptimal, unless one can update the profile anytime there is a sudden change in content.


%may render the relationship obsolete.\footnote{AWStream will update relationship periodically~\cite{awstream}, but as we will see in \S\ref{??}, it is challenging to update this profile frequently enough without excessive use of bandwidth.}
%Similar, a simple heuristic (\eg a shallow neural net) is unlikely to work, since it is less accurate than the server-side DNN.
%For instance, if one uses the heuristics to determine which frame contains objects and send these frames, any false positives can cause unnecessary bandwidth consumption, and any false negatives from the simple, camera-side network will prevent the powerful server-side network from having a chance to detect the object. 


%In short, the limitation of the heuristic-based approach is that any camera-side heuristic is incapable of making optimal adaptation decisions without knowing how the server-side DNN would react to the current video content. 
%After all, if the camera can run a sufficiently complex heuristic that imitates the server-side DNN, there would be not need to send videos to the server for more compute-intensive inference. 

%Moreover, some camera-side heuristics also need to be updated whenever the server-side DNN changes, which may lead to 


%\begin{itemize}
%    \item ideally driven by {\em real-time content of interest}, which is time varying and dnn-dependent
%    \item a taxonomy of existing techniques (changing codec is an option though not practical)
%    \begin{itemize}
%        \item client-side filtering
%        \item adaptive encoding
%    \end{itemize}
%    \item empirically compare accuracy of the prior approaches (glimpse, noscope, awstream) with the oracle
%    \item discussion:
%    \begin{itemize}
%        \item client-side filtering: not dnn/task dependent
%        \item adaptive encoding: not real-time content-dependent
%    \end{itemize}
%\end{itemize}



\cameranew{

\mypara{Example scenario 1 (response-delay-dominant)} 
Let us start with a simple setting where the performance objective is to minimize the response delay while preserving high accuracy (\eg FPS gaming through AR) without a cost budget, and any server has a high network latency with the camera.
In this case, the best solution would be having camera equipped with a high-end GPU to analyze each frame locally.
Any solution that sends frames to a remote server will suffer from network latency.
% all video streaming approaches need to go through the network and are affected by network latency. 
% To avoid this latency, we could put a high-end GPU at the camera side to inference right after the frame has been captured. Thus, in this scenario, it is the best to process all the frames at the camera.

\jc{need to mention figure 5}

The next two scenarios use the same performance objective---minimizing the cost while achieving accuracy over 0.8 and response delay less than 1.5 seconds---but have different deployment settings.

\mypara{Example scenario 2 (server-side-cost-dominant)} 
We assume the deployment setting in this scenario is that the camera is connected to the server with a wired network with unlimited bandwidth and negligible network latency and the cloud server rented for a year (\ie in total $10^9$ frames) 
% (if longer, the renting cost will be higher than directly buying the GPUs) 
% and optimize the cost with accuracy target $0.8$ and average delay target $1$ seconds. Running wired traffic camera through cloud server is a concrete example. 

% $$\Cost_{cam}^{\Setting}(\Model^{\Pipeline}(\Accuracy))+\Cost_{net}^{\Setting}(\Size^{\Pipeline}(\Accuracy))+\Cost_{srv}^{\Setting}(\Workload^{\Pipeline}(\Accuracy))$$



\mypara{Cost} As for the camera-side cost, from \cite{wired-camera-cost}, we know that a wired camera is about 150\$. We let all VAPs use this camera (this will make the cost of Glimpse strictly smaller) except for Vigil. For Vigil, to support 30fps inference on Mobilenet-inception-v2, we need at least 3 NVIDIA Jetson TX2 \cite{jetson-inference-speed} while each of them cost 490\$\cite{jetson-price}. Thus, we write:
$\Cost_{cam}=3\times 490\times 10^{-9}$ for Vigil and
$\Cost_{cam}=150\times 10^{-9}$ for other solutions.
As for the network cost, since the camera is wired, the bandwidth cost is a one-time cost that are the same fr all VAPs and could be amortized through time. Thus, we write $\Cost_{\network}= 0$ for all solutions.
%$Renting one NVIDIA GTX 1080 would be about 71.8\$ per month %$\cite{rent-gtx1080-price}. 
%The detection model faster-rcnn-resnet101 will run in 106ms on NVIDIA GTX Titan X. Based on the FLOPs listed in \cite{gpu-flops-comparision}, we infer that a NVIDIA GTX 1080 could run faster-rcnn-resnet101 at about 7.5 fps.
As for the server-side cost, from \cite{google-gpu-pricing}, we know that one NVIDIA Tesla K80 GPU will be $206.590\$$ per month.
Based on \cite{titanX, model-zoo,k80}, we infer that a NVIDIA Tesla K80 GPU could support about 10 fps inference on Faster-rcnn-resnet101.
Thus, to achieve 1 inference per frame, we need about 7437\$ per year.
Based on this, we write:
$
\Cost_{srv} = \Workload^{\Pipeline}\times 7437\times 10^{-9}
$
According to the information above and based on our experimental results, we plot the cost v.s. accuracy of pure server (AWStream will be strictly worse due to profiling cost at server-side), Vigil, Glimpse, pure camera and \name in Figure \ref{fig:suboptimal-cost-acc}.

% $$
% \Time_{\buffer}^{\Pipeline} + \Time_{\process}^\Pipeline + \Ratio^{\Pipeline} \cdot (\Time_{\network}^{\Setting}(\Size^{\Pipeline}(\Accuracy)) + \Time_{\inference}+\Time_{\latency}^{\Pipeline}),
% $$

% $$
% \Time_{\camera}^{\Setting}(\Model^{\Pipeline}(\Accuracy)) + \Workload^{\Pipeline} \cdot (\Time_{\network}^{\Setting}(\Size^{\Pipeline}(\Accuracy)) + \Time_{\inference}),
% $$

\mypara{Delay}
For Glimpse, we assume it only needs to encode the last captured frame, \ie $\Time_{\camera}=\frac{1}{30}$. This will make Glimpse strictly better since Glimpse needs to perform tracking on the camera.
As for Vigil and the pure camera approach, we say $\Time_{\camera}=\frac{1}{11.5}$~\cite{jetson-inference-speed}.
For the pure server approach and \name, they have to buffer enough frames to fill in the video chunk. Thus, 
$
\Time_{\camera} = \frac{14}{2\times 30}.
$
As for the factor $\Workload$, we empirically found that $\Workload\approx 0.16$ for both Vigil and Glimpse. Trivially, $\Workload = 0$ for the pure camera approach and $\Workload=1$ for the pure server approach.
Since the camera is wired with unlimited bandwidth, the streaming delay is negligible. Hence we say 
$
\Time_{\network} = 0.
$
Since the server could work at 10 FPS, the server-side time for all methods is $\Time_{\inference}=0.1$.
Based on these information and our experimental results, we plot the delay v.s. accuracy in \ref{fig:suboptimal-delay-acc}. 


From Figure \ref{fig:suboptimal-cost-delay-acc}, we see that Vigil is the best choice under this scenario. \kt{The pure camera approach suffers low accuracy as it could only afford a cheap model, which would miss objects (as illustrated in Figure \ref{fig:contrast-model}).} 

\mypara{Example scenario 3 (network-cost-dominant)} Now we assume that we stream from a lot of 4G-connected cameras to a personal cluster for a year (i.e. about $10^9$ frames).

\mypara{Cost} As for the camera-side cost, a LTE-conected camera is about 216\$~\cite{camera-price}. This camera is enough for all pipelines except for Vigil. For Vigil, we still use the same way stated in the last scenario to calculate its camera cost. Thus,
$\Cost_{cam}=3\times 490\times 10^{-9}$ for Vigil and
$\Cost_{cam}=216\times 10^{-9}$ for other solutions.
As for the cost on the network, An AT\&T unlimited family plan would be \$35 per month~\cite{4G-plan} for a 13Mbps uploading speed~\cite{upload-speed} on a single camera. Thus, streaming with an average speed of 1Mbps per year will cost about \$32. Accordingly, we write:
$
\Cost_{\network}=30\times\times \Size^{\Pipeline}(\Accuracy)\times 32\times 10^{-9}
$
The $30$ here is the frame rate.
As for the server-side cost, the per-camera per-frame server-side cost could be amortized over time. Hence we write:
$
\Cost_{\inference}=0
$
for all solutions.
According to the information above and based on our experimental results, we plot the cost v.s. accuracy of pure server (AWStream will have strictly higher cost due to profiling), Vigil, Glimpse, pure camera and \name in Figure \ref{fig:cost-acc}.

\mypara{Delay}
The $\Time_{\camera}$, $\Workload$ and $\Time_{\inference}$ are exactly the same as in example scenario 2. As for the network time, we let three camera share the 13Mbps upload bandwidth (except for the pure server approach to ensure the bandwidth is sufficient for real-time purpose) and calculate the streaming time by the frame/chunk size divided by the bandwidth.  Based on these information and our experimental results, we plot the delay v.s. accuracy in \ref{fig:delay-acc}.

% For Glimpse, we assume it only needs to encode the captured frame, \ie $\Time_{\camera}=\frac{1}{30}$. This will make Glimpse strictly better since Glimpse requires tracking.
% As for Vigil and the pure camera approach, we say $\Time_{\camera}=\frac{1}{11.5}$~\cite{jetson-inference-speed}.
% For the pure server approach and \name, they have to buffer 15 frames and encode them before sent. Thus, 
% $
% \Time_{\camera} = \frac{16}{2\times 30}.
% $

% We know that $t_{cam}^{VAP}=\frac{1}{40}$ for those VAP which only encodes at the camera (it has sufficient compute to encode at 40FPS in 720p). We also use this value for Glimpse. For Vigil, $t_{cam}^{VAP}=\frac{1}{11.5}$~\cite{jetson-inference-speed}. 
% We let three camera share the 13Mbps upload bandwidth (except for the pure server approach) to achieve real time and calculate the streaming time. The server could run Faster-rcnn-resnet101 (which is what we use) in about 0.1s~\cite{model-zoo}. So $t_{serv}=0.1$ (we assume that the server is able to decode the video much more faster than inference on each frame). The latency for 4G network is about 0.05s~\cite{4G-latency}. As for \name, the encoding time $t_{enc}$ (will be introduced in \S\ref{sec:overview}) is about $\frac{15}{40}$ seconds. Based on these information and our experimental results, we plot the delay v.s. accuracy in \ref{fig:delay-acc}.

From Figure \ref{fig:cost-delay-acc}, we see that \name is the best choice under this scenario.


}

==> motivate_new.tex <==




\section{Motivation}




\vspace{0.2cm}

\tightsubsection{DNN-based analytics systems}

\kt{Change system to pipeline}




\mypara{Background} 
Today, DNN-based analytics applications are ubiquitous~\cite{tusimple,waymo,trafficvision, traffictechnologytoday,goodvision,intuvisiontech, vision-zero, msr,servai-1,servai-2,servai-3}.
In this paper, we pick four applications: 
autonomous driving, traffic analytics, human detection for home security and audio-to-text for smart home.
We pick these tasks not only because they are critical to real-world applications, but also because they take as input various types of data streams, \eg RGB videos, LiDAR videos and audio waves (see Table~\ref{tab:applications}).
% vehicle detection for autonomous driving, voice recognition for smart home and human detection for home security, all of which analyze data streams (\eg video frames or point cloud) collected from sensors to extract information (\eg detect bounding boxes of objects of interest).
% with various types of sensors.
% \kt{Maybe call it input preparation sounds better. Input processing sounds like irrelavent to data streaming}

Figure~\ref{fig:dnn-analytics-application-flow} depicts a typical pipeline of these applications. 
First, they collect and process data from sensors (we denote the sensed raw data as \textit{input data}) to the DNN input.
Then, the DNN input may need to be streamed to an analytics server (in edge or cloud) through a {\em bandwidth-constraint} link, so not all data points (\eg video frame) in their highest fidelity will be collected.
Then, the server runs DNN inference to return 
% They collect data from sensors, prepare the input for the DNN (which may require network-based data streaming), perform DNN inference, and obtain 
the inference results (\eg vehicle bounding boxes for autonomous driving) using limited GPU resources.
% We assume that the inference results are a collection of elements (\eg object bounding boxes in object detection, classification labels in classification, pixel labels in semantic segmentation), where each element is associated with a corresponding confidence score. Only those elements with a confidence score higher than a confidence threshold will be counted when calculating accuracy.
% This assumption does not hold for all DNN-based applications (\eg this assumption does not hold in a generative task like image generation, as it only generates the pixel values for each pixel, but does not associate confidence scores to those pixels).
% However, this assumption covers a wide range of applications, like video analytic tasks (\eg object detection, semantic segmentation, classification) and audio-based tasks (\eg audio-to-text).




\begin{figure}
    \centering
    \includegraphics[width=0.9\columnwidth]{figs/multiapp.pdf}
    \tightcaption{
    In DNN-based analytics applications, various types of source data collected from sensors are processed by an input processing module to generate DNN input. 
    The DNN is then run on the input to get inference output.
    % analytic results based on DNN input using constrained GPU resources.
    Since the DNN inference module may be located on a remote edge device or cloud server, the input processing module may need to stream the data to the DNN through a bandwidth-constraint network.
    % As the DNN inference module may locate on a remote edge device/cloud server, the input processing module may need to connect to the DNN inference module through a {\em bandwidth-constraint} network. \kt{Junchen can you read this figure and see if it works?}
    }
    \label{fig:dnn-analytics-application-flow}
\end{figure}

\begin{table}[]
\centering
\footnotesize
\begin{tabular}{ccc}
\hline
Example application & Analytic task        & Data type                                                             \\ \hline
Autonomous driving  & Vehicle detection    & \begin{tabular}[c]{@{}c@{}}RGB video,\\ LiDAR point cloud\end{tabular}   \\ \hline
Traffic monitoring  & Vehicle segmentation & RGB video                                                                \\ \hline
Security monitoring & Human detection      & \begin{tabular}[c]{@{}c@{}}RGB video,\\ Infrared, Depth map\end{tabular} \\ \hline
Smart home          & Audio to text        & Audio                                                                    \\ \hline
\end{tabular}
\vspace{0.2cm}
\tightcaption{Example applications of our solution.} 
\label{tab:applications}
\end{table}


% \begin{table}[t]
% \centering
% \footnotesize
%     \begin{tabular}{c c c}
%         \hline
%         Example application & Analytic task & Data sources\\
%         \hline
%         Autonomous driving & Vehicle detection & RGB video, LiDAR point cloud \\
%         Traffic monitoring & Vehicle segmentation & RGB video \\
%         Security monitoring & Human detection & RGB video, Infrared, Depth map \\
%         Smart home & Voice to text & Audio   \\
%         \hline
% \end{tabular}
% \tightcaption{Example applications of our solution.} 
% \label{tab:applications}
% \end{table}    






\mypara{Objective}
% In practice, however, a real system of these applications may not have enough {\em network bandwidth} to stream all uncompressed data from sensors to a remote more powerful server, and/or enough {\em GPU compute resource} to run expensive DNN inference on all input data (\eg all frames of a video stream). 
% This means that they may not have enough resources to stream uncompressed data out (if the sensor cannot run DNN-based analytics by itself) and perform inference on every part of the input data (\eg on every frame of the video). 
As a result, the objective for these DNN-based analytic systems is to improve \textit{inference accuracy} without increasing the resource usage (in terms of network bandwidth and GPU cycles), or reduce the resource usage without hurting the inference accuracy.
% under the average bandwidth and/or GPU computation budget.
Following prior work~\cite{awstream,chameleon,dds,accmpeg,ekya,yoda}, we define accuracy as the similarity between the inference results and the inference results generated under unlimited bandwidth and/or GPU computation budget (see \S\ref{subsec:eval-setup} for detailed definition).
This directly shows the impact of saving resource usage on inference accuracy. 
% \jc{update this with the objective table on the whiteboard}
% \kt{I guess we need to defend why average budget, let me think of an argument...}


\kt{Defend the choice of streaming to server for anlaytics}



\tightsubsection{The need for timely configuration adaptation}
\label{subsec:numer_of_knobs}


\begin{table}[t]
\footnotesize
    \begin{tabular}{c c}
        \hline
        Knobs & \begin{tabular}[x]{@{}c@{}}Trade-off between\\accuracy and\end{tabular}\\
        \hline
        % \footnotesize Streaming delay & \footnotesize Video encoding parameters, region-of-interest \\
        % \footnotesize Number of data frames & \footnotesize Data frame difference thresholds \\
        % \footnotesize DNN inference time & \footnotesize model selection, model customization \\
        Resolution~\cite{awstream,dds,chameleon,vstore,videostorm,deepdecision,adascale,casva} & $B$ (\& $G$)  \\
        Quantization parameter~\cite{awstream,vstore,casva} & $B$ \\
        % Video bitrate~\cite{deepdecision} & $B$ \\
        % Encoding preset~\cite{vstore} & Encoding delay  \\
        Frame rate~\cite{awstream,chameleon,vstore,videostorm,deepdecision} & $B$ \& $G$   \\
        Frame filtering thresholds~\cite{reducto,glimpse,vigil}  & $B$ \& $G$ \\
        Fine-grained video compression~\cite{accmpeg,dds,eaar,saliency_hotmobile} & $B$  \\
        Feature compression~\cite{vcm,neurosurgeon} & $B$  \\
        Audio sampling rate~\cite{huang2001spoken, hirsch01_eurospeech, narayanan2018toward, gao2019mixedbandwidth, hokking2016speech} & $B$ (\& $G$)\\
        % \cite{cinet,vigil} & Region cropping & Bandwidth usage and GPU compute & \cmark \\
        % \cite{noscope,ekya} & Model customization & GPU compute  \\
        % \cite{chameleon} & Model selection & GPU compute &  \\
        % \cite{cloudseg} & Server-side super resolution & Bandwidth usage  \\
        % \cite{videostorm} & Server-side DNN parameter & GPU compute \\
        \hline
\end{tabular}
\vspace{0.2cm}
\tightcaption{A list of configuration knobs that prior work has shown to be effective in reducing bandwidth usage ($B$) and/or GPU compute ($G$) without hurting inference accuracy.
This work does not consider DNN itself as a configuration knob. (We will discuss this limitation in \S\ref{subsec:limitation}.)
% Distributed AI systems introduce rich types of knobs to reduce bandwidth usage ($B$) and/or GPU compute ($G$) without hurting inference accuracy.
% {\footnotemark}
} 
\label{tab:rich-set-of-knobs}
\end{table}    




% expose internal tunable parameters (referred to as knobs) and
% timely configure these knobs (we denote the knobs together
% with their configured values as a configuration)

Prior work has shown that high accuracy {\em could} be obtained with significantly lower network and/or GPU usage if the internal parameters of these DNN analytics pipelines (hereinafter \textit{knobs}) are configured optimally (we denote the knobs together with their configured values as a configuration).
Table \ref{tab:rich-set-of-knobs} summarizes the knobs used in this work.
% and timely adapts them 
% based on the input data streams to save network and compute resources.
The {\em optimal} setting of configuration is the one that yields the highest accuracy with low resource usage in bandwidth and GPU cycles (this will be more rigorously defined in \S\ref{sec:eval}).
% For instance, consider 
When detecting vehicles in a traffic video, for instance, we can significantly reduce the frame sampling rate of data collection and DNN inference, if the vehicles are moving slowly (\eg at a red light), and the DNN can still accurately determine the position and movement of the vehicles.
% during a red light, the speed of vehicles is low, allowing us to significantly reduce the frame sampling rate of data collection and DNN inference, while still accurately determining the position and movement of the vehicles. 



% \mypara{Configurations must be adapted frequently}
The optimal settings of these configurations, as argued in prior work,(\eg~\cite{awstream,chameleon,casva}) are highly {\em dependent} on
% must be \textit{tailored} to 
the content of the source data.
Therefore, as the content varies over time, these configurations must be adapted timely.
In the vehicle-detection example, when the green light is on, vehicles start to speed up, so the frames must be analyzed much more frequently by the DNN to 
% and analysis of more video frames by using a high frame rate is necessary to 
accurately capture the motion of those moving vehicles.
To put it in perspective, prior work has shown that in video analytics for object detection, adapting once every 4 seconds makes 10\% more frames to have over 80\% accuracy compared to adapting once every 8 seconds~\cite{chameleon}.
In other applications (semantic segmentation, audio-to-text, and face generation) and configurations studied in this work, we observe a similar need for timely adaptation at a timescale of a few seconds. 
% \jc{a forward pointer and add a few words}


% \jc{i suggest we cite numbers from prior work to illustrate the huge potential by adapting configs must be optimally and timely. this seems to be repeating the same argument made by many previous papers. for experts, they just need to be reminded with some concrete numbers from prior work; for non-experts, citing numbers prior work helps them to understand what's new and what's not.}
% \kt{done}



% Choosing a low frame sampling rate when the vehicles are moving quickly will lead to inaccurate inference results as it cannot accurately capture the position and movement of the vehicles. 
% On the other hand, using a high frame sampling rate when the vehicles are moving slowly may result in excessive resource usage.


% \mypara{config can save this resource, why saving resource can improve accuracy, raise 2 examples}

% \mypara{Optimal settings depend on the content of the video, configurations need to be adapted}



% \mypara{Data stream variation}
% Moreover, the inputs to the DNN-base analytic applications are non-stationary (in terms of content and quantity) across time (\eg\ a new object-of-interest may suddenly appears) and space (\eg\ traffic condition in downtown and rural area), a considerable amount of previous work~\cite{awstream,chameleon,accmpeg,dds,vigil,reducto,glimpse} has shown that leveraging such dynamic and timely adapt to the input can achieve a higher accuracy and lower end-to-end delay than not adapting.

% \jc{too much noise. the key message should: temporal variation of input {\em could} allow resource saving without hurting accuracy. the message itself and why is it so are not clear}

% \mypara{System research for these applications} In order to handle heterogeneous applications and varying input data stream, the corresponding system research is rapidly expanding.
% Prior work leverages techniques from sensor-side data filtering~\cite{glimpse,reducto} and compression~\cite{dds,eaar,awstream,chameleon,vigil,cinet,accmpeg,VCM}, server-side model selection~\cite{chameleon} and customization~\cite{noscope,ekya,mcdnn,blazeit} to server-sensor co-optimization on adapting video encoding parameters~\cite{awstream}, data-of-interest detection~\cite{eaar,dds,elf}. 



% \mypara{Performance metrics}
% We measure the performance of analytic systems in two metrics under a certain resource budget: \textit{accuracy} and \textit{end-to-end delay}.
% Following prior work~\cite{awstream,chameleon,dds,accmpeg,ekya,yoda}, we define accuracy as the similarity between the current inference results and the inference results generated with unlimited resources.
% The end-to-end delay includes the camera processing, streaming, and DNN inference (more details in \S\ref{sec:eval_setup}).
% End-to-end delay captures the resource usage of different parts of the system, including camera-side compute cost (reflected in camera processing delay), bandwidth usage (reflected in streaming delay) and GPU cost (included in DNN inference delay).



% \jc{Not sure about the metric. If we use accuracy and end-to-end delay, the improvement tends to be smaller as tuning the knobs in eval only reduces a part of the delay. I am considering using resource usage (network and GPU) instead of end-to-end delay (the improvement will be larger). Can we defend this metric by saying resource usage is smaller means that more jobs can be run concurrently?}


% As previous work observes, the optimal configuration changes frequently~\cite{?,?}.
% In the example above, the optimal sampling rate changes when the traffic light turns from red to green or from green to red, which happens once every tens of seconds.
% As a result, the configuration adaptation also needs to be frequent to reduce the time of sticking to the old configuration after the optimal configuration changes.

% To quantify this potential, we specify an idealized policy to show the potential of adapting once per $x$ second (note that lowering $x$ increases adaptation frequency).
% Concretely, we divide the data into $x$-second chunks. 
% At each chunk, we obtain a configuration that yields the highest accuracy under the resource budget based on the first-second video (by profiling all configurations on the first-second video) and sticks to that configuration for that video chunk.

% \jc{kuntai, I commented out a para here. it's merged with the last para. please check}
% \mypara{Configurations need to be adapted frequently}
% As previous work observes~\cite{awstream,chameleon}, the optimal configuration is frequently changing. 
% For instance, in the aforementioned traffic monitoring example, the optimal frame sampling rate changes when the traffic light switches from red to green or vice versa, which occurs every few seconds. 
% Thus, a frequent adaptation of the configuration is necessary to minimize the amount of time spent using an outdated configuration.



% To measure the potential of optimally adapting these configurations, we consider an idealized policy that adapts the configuration with the optimal value once every $x$ seconds (with a lower value of $x$ resulting in a higher frequency of adaptation) without extra computation or network overhead. 
% Specifically, we divide the data into $x$-second segments. 
% At each segment, we determine the configuration that delivers the highest accuracy under the resource budget, based on the first second of video (by profiling all configurations on the first second of video), and use that configuration for the whole $x$-second video segment.

% We show that, under \kt{fill a resource budget here}, increasing profiling frequency from once per  \fillme seconds to once per \fillme seconds provides significant accuracy gain (\fillme\%), though the gain saturates when the frequency is higher than once per \fillme second..


% This is because the accuracy of a configuration can greatly depend on the content of input data. 
% When the input data becomes more challenging, (such as faster-moving vehicles), using the same configuration will result in decreased accuracy. 
% In that case, we need to switch to a configuration that provides increased accuracy, even if it requires additional network and GPU compute resource.
% Conversely, when the video content becomes less demanding, we can then to switch to a configuration that uses fewer resources, while still maintaining the desired level of accuracy.




% \mypara{Performance metrics}
% We measure the performance of configuration adaptation systems by measuring their accuracy under various resource budgets.
% Following prior work~\cite{awstream,chameleon,dds,accmpeg,ekya,yoda}, we define accuracy as the similarity between the current inference results and the inference results generated under the most resource-demanding configuration.
% % The end-to-end delay includes the camera processing, streaming, and DNN inference (more details in \S\ref{sec:eval_setup}).
% % End-to-end delay captures the resource usage of different parts of the system, including camera-side compute cost (reflected in camera processing delay), bandwidth usage (reflected in streaming delay) and GPU cost (included in DNN inference delay).
% In terms of resource budget, we will limit two kinds of resources (network and GPU compute).
% We will also compare the sensor-side overhead between different configuration adaptation systems.
% \kt{change performance metric to accuracy v.s. resource consumption}

% As traditional notion of accuracy requires expensive human annotation as the ground truth,
% we define \textit{accuracy} as the similarity between the current inference results and the inference results generated with unlimited resource (this aligns with previous work~).
% The \textit{end-to-end delay} measures the elapsed time from the moment the inputs are generated to the moment all DNN output on such input has been received. 
% For example, in a scenario where a camera streams the video to a GPU-equipped server for analytics~\cite{awstream,dds,eaar,elf,accmpeg,reducto,vigil,glimpse}, its end-to-end delay includes the delays from video encoding, streaming, decoding, and DNN inference. 

% \jc{need to clarify what resources mean? computer (cpu or gpu), memory, or bandwidth?}

% \jc{the text on performance metrics could be tightened. instead, we need a couple of paragraphs on the various applications we target, for two reasons: (1) if not, people may view this as just another video analytics paper, and (2) we need to first scope the paper, in case people feel this is targeting all ML applications. maybe a figure would help, like the one we had in accmpeg (e.g., different sources, different DNNs, different tasks, BUT they all have input pre-processing that influences the resource usage and the accuracy of the downstream dnns)}
% \roy{fixed}
% \kt{figure added}


% While resource usage is another popular performance metric used to evaluate these systems, we consider it to be implicitly included by the end-to-end delay.
% Since, with a fixed amount of resource and the same input content, the systems requiring more resource typically lead to a longer computing/transmitting time compared with the ones with lower resource requirement (\eg\ when using a link with fixed amount of bandwidth, the systems transmitting larger files will have a higher end-to-end delay since the transmission time will be higher).

% \mypara{Terminologies}
% In order for these systems to adapt to the input content and the resource limits, these systems define and implement a set of tunable parameters and timely vary the value of these parameters, which we define them as \textit{knobs}, $k$.
% And we specifically refer the word ``\textit{values}'', $v$, to be the values that the systems' knobs can choose from.
% Furthermore, a combination of all the parameters' inside one system forms a system's \textit{configuration}, $c=(v_1, \ldots, v_n)$, which is the minimum unit in order to let the system run. 
% For example, in a video analytics application featuring input video's resolution as knob $k_1$ with possible value $v_1 = \{480p, 720p, 1080p\}$ and input video's frame rate as knob $k_2$ with possible values $v_2 = \{10 \text{ FPS}, 30 \text{ FPS}\}$, one of the configurations for such a application can be $c_1 = (480p, 10\text{ FPS})$.
% The set of the systems' all such possible configurations, $\{c_1, \ldots, c_n\}$ forms a space we defined as \textit{configuration space} of the systems.
 


% Nowadays, distributed AI applications are everywhere. \kt{several examples here}



% \mypara{Performance metrics}
% The performance metrics of these pipelines are analytic accuracy\footnote{We use the analytic results on the uncompressed video with the most expensive anlaytic model as the ground truth to measure accuracy} and end-to-end delay, including sensor-side processing delay, streaming delay and server-side inference delay.


% \mypara{Estimating the accuracy is the key}
% Different from end-to-end delay that can be cheaply controlled and estimated, accuracy is much more difficult to estimate. This is because

% \mypara{Ai analytic pipelines propose a lot of knobs}
% As different applications may have different requirements to anlaytic accuracy and end-to-end delay, these distributed AI systems introduce rich set of tunable hyper-parameters (we call these tunable hyper-parameters \textit{knobs}) to trade-off between analytic accuracy and end-to-end delay.
% (Table ~\ref{tab:rich-set-of-knobs} illustrates the rich set of knobs of distributed AI anlaytic systems and their corresponding trade-off).
% % Despite their superior performance, all of these systems introduces internel knobs that matters a lot to their performance. 



% System research on AI applications are emerging.

% \begin{figure}
%     \includegraphics[width=1\columnwidth]{figs/delay-breakdown.png}
% \end{figure}


% These systems invent different type of knobs to trade-off between accuracy and end-to-end delay, which is mainly determined by three parts:
% \begin{itemize}
%     \item Sensor processing delay
%     \item Streaming delay
%     \item DNN processing delay, which is mainly determined by number of data frames (the \textit{minimum} amount of data that can be consumed by the DNN) to be processed and inference time of the DNN.
% \end{itemize}
% \kt{Mention that sensor processing delay is typically used as a cost to optimize other delays}


% A category of related work

% Limitation discussion: we do not handle DNN change in our framework.


% \subsection{Characteristics on the set of knobs}




% \jc{this subsection should start by showing that one can tune configurations based on input characteristics to save resource without affecting accuracy}


% \myparashort{More knobs are being proposed.}
% The number of knobs exposed by DNN-based analytics systems are already large and still growing. 
% For example, prior work on video analytics uses various combinations of 16 knobs: 6 video encoding knobs~\cite{vstore,chameleon,dds,videostorm,awstream}, 9 frame filtering knobs~\cite{reducto,vigil,glimpse}, knobs that differentiate spatial video quality knob~\cite{dds,accmpeg,eaar, elf} (which can be up-to thousands of knobs if tuned per macroblock~\cite{accmpeg}), server-side processing thresholds~\cite{dds,eaar,elf}).
% and new functionalities (\eg new encoding standard for point cloud data~\cite{MPEG-point}, multi-sensor fusion~\cite{chameleon}, parallel inference~\cite{eaar,elf}).
% This trend is driven by the need to explore new resource-saving opportunities in new types of data streams (\eg LiDAR feeds), new applications (\eg video captioning), and new deployment settings (\eg new settings in distributed video analytics where the camera needs to stream the video to the server~\cite{awstream,dds,chameleon,vigil,glimpse,reducto,dds,eaar,elf} like multi-camera video analytics~\cite{chameleon,glimpse} and multi-server video anlaytics~\cite{elf}).

% \begin{comment}


%     % \mypara{Number of knobs are already large}
%     \mypara{There are many knobs to tune}
%     The number of knobs exposed by DNN-based analytics systems are already large.
%     For example, prior work on video analytics uses various combinations of 16 knobs: 6 video encoding knobs~\cite{vstore,chameleon,dds,videostorm,awstream}, 9 frame filtering knobs~\cite{reducto,vigil,glimpse}, and the knobs that differentiate spatial video quality knob~\cite{dds,accmpeg,eaar}, which can be up-to thousands of knobs if tuned per macroblock~\cite{accmpeg}.
%     % can be partitioned to even  thousands of knobs~\cite{accmpeg,eaar} if tuned in a fine granularity.
%     \jc{merge the first two paras, especially they overlap a lot..}
    
%     \mypara{New knobs are proposed} We observe that DNN-based analytic systems are constantly proposing new knobs (\eg video encoding parameters~\cite{awstream,dds,chameleon,vstore,videostorm}, frame filtering thresholds~\cite{vigil,glimpse,reducto}, server-side processing thresholds~\cite{dds,eaar,elf}).
%     and new functionalities (\eg new encoding standard for point cloud data~\cite{MPEG-point}, multi-sensor fusion~\cite{chameleon}, parallel inference~\cite{eaar,elf}). The reason behind this trend is that these systems need more knobs to explore new resource-saving opportunities in new types of data streams (\eg LiDAR feeds), new applications (\eg video captioning) and new deployment settings (\eg new settings in distributed video analytics where the camera need to stream the video to the server~\cite{awstream,dds,chameleon,vigil,glimpse,reducto,dds,eaar,elf} like multi-camera video analytics~\cite{chameleon,glimpse} and multi-server video anlaytics~\cite{elf}).
    
% \end{comment}
    % \begin{enumerate}
    % \item
    % As DNN-based analytics are deployed on heterogeneous deployment settings that are of different resource budgets, this requires the corresponding systems to propose new knobs in order to fit into
    % different resource budgets while achieving high inference accuracy. Take video analytics as an example. If the
    % user analyzes the video feeds locally by a compute-constrained mobile
    % phone, the main focus for the systems is to fit into the compute budget
    % of the phone (\eg by skipping those frames that are highly similar to
    % their previous frames~\cite{reducto,glimpse}). However, if the user
    % instead streams the video feeds to a GPU-equipped server through a
    % bandwidth-limited LTE network, the main focus is instead fitting into
    % the limited LTE bandwidth (\eg by performing video
    % compression~\cite{accmpeg,vigil,glimpse,reducto}).
    
    % \item
    % Since new applications quickly emerge (\eg LiDAR-based object detection,
    % Infrared-based human detection \kt{a bunch of citations here}), this requires the deep learning systems
    % to develop new knobs (or even developing new system components) to fit
    % into the need of different applications. For example, in order to handle
    % LiDAR data, people are proposing new encoding standard and new
    % knobs~\cite{MPEG-point} to efficiently encode and process LiDAR data.
    
    % \end{enumerate}


    
    % As DNN-based analytics quickly expand, the corresponding systems need to
    % partition existing knobs into more fine-grained version to capture more
    % resource-saving opportunities. Take video-based vehicle detection as an
    % example. Chameleon~\cite{chameleon} and AWStream~\cite{awstream}
    % identify that the system only need to encode the video in a high
    % encoding quality when the vehicle appears. To further explore the
    % potential of varying video encoding quality, the following
    % work~\cite{dds,eaar,accmpeg} finds that a lot of areas in the video do
    % not need to be encoded in high quality (\eg the areas that contain
    % non-vehicle-related backgrounds like trees and buildings) and proposes
    % fine-grained spatial encoding quality to capture this opportunity.
    % \mypara{Knobs become more fine-grained}
    % As the need of DNN-based analytics grows quickly, these systems need to support more concurrent analytic jobs under the same resource budget, which requires them to tune existing knobs at a finer granularity (by partitioning existing knobs to multiple fine-grained knobs) to further reduce the resource demand for running one analytic job without hurting the accuracy.
    % For example, in distributed video analytics, to detect small objects in the input video, one may need to encode and stream the whole video in high resolution to detect such objects (high bandwidth usage)~\cite{chameleon,awstream}.
    % However, prior work~\cite{dds,eaar,accmpeg} shows that, by assigning different areas with different resolutions\footnote{In fact, prior work assign different areas with different quantization parameters, a parameter that controls the fidelity of the encoded video without changing the resolution. We use resolution in the text for understandability consideration.}, it only needs to encode the surrounding macroblocks of objects in high resolution and other areas can be encoded in low resolution, which maintains high accuracy using significantly less network resource.
    
        
    % \mypara{More gains by tuning more knobs jointly}
    % % Tuning more knobs can provide more performance gain.
    % This is because the input data from one source may simultaneously include several resource-saving opportunities that require different knobs to capture.
    % % (as one knob typically captures one resource-saving opportunity)
    % For example, in rural driving videos, the analytics system can save GPU compute resource by discarding the frames through frame filtering knobs~\cite{vigil,glimpse,reducto} when no vehicles and pedestrians appear.
    % Moreover, when the vehicles and pedestrians appear, the system can encode just the areas that include these objects in high encoding quality and encode the remaining areas in low encoding quality through fine-grained video encoding knobs~\cite{dds,eaar,accmpeg} to save the streaming bandwidth required to stream the video to the server for analytics.
    % Further, when the vehicles move quickly in the video, one can further save bandwidth by enabling a more expensive motion compensation algorithm of the video codec~\cite{vstore,videostorm} (as a cheap motion compensation algorithm may not be able to identify the correct motion of the vehicles, resulting in inefficient video compression).
    % the user may deploy a dashcam and stream the video to a remote GPU-equipped server for analytics.
    % In this scenario, for most of the time no vehicles and pedestrians appear in the field-of-view of the dashcam and the corresponding video frames can be safely discarded to save GPU compute.
    % In order to accurately discard the frames where the vehicles and pedestrians do not appear, it requires the system to incorporate multiple frame filtering thresholds, as shown in Reducto~\cite{reducto}.
    % Moreover, on those frames that the vehicles and pedestrians appear, they typically reside in small areas in the frame (\eg a distant car at the end of the road).
    % In this case, one can encode just these small areas in high fidelity by assigning these areas both high resolution and high encoding quality.
    % % through, for example, partitioning the video into different areas and adjusting the resolution and the quantization parameter for the areas that the vehicles and pedestrians appear~\cite{dds,eaar,accmpeg} to save streaming bandwidth.
    % This may introduce several knobs (even thousands of knobs in AccMPEG~\cite{accmpeg}) to identify and encode these areas in high fidelity~\cite{dds,eaar,accmpeg}.
    % Further, as the dashcam itself is moving quickly, in order to accurately detect and encode the motions of the vehicles, one may want to perform more accurate motion compensation by selecting a higher encoding preset~\cite{vstore,videostorm} and encode the residue after motion compensation in higher fidelity by increasing the encoding quality of motion-compensated frames when the vehicles appear to further improve the accuracy.
    
    % 1. multiple configurations can optimize multiple components of the end-to-end delay, while one configuration typically optimizes only one component of the end-to-end delay.
    % \eg video encoding quality $\rightarrow$ streaming delay; server-side DNN selection $\rightarrow$ server-side delay
    % 2. even in the case that multiple configurations are actually reducing the same components of the delay, having multiple configurations allow the system to capture more opportunities to reduce the delay.
    % \eg video resolution $\rightarrow$ can reduce the streaming delay when the objects are large. video frame rate $\rightarrow$ can reduce streaming delay when the objects only appears in a subset of frames.
    % So having both of them may result in a much higher gain when the objects are large and only appears in a subset of frames.
    
    
    % \item Most of the parameters are operating on DNN input.





% \begin{figure*}[t]
%     \centering
%     \includegraphics[width=1.5\columnwidth]{figs/workflow.pdf}
%     \tightcaption{Workflow of \name.}
%     \label{fig:workflow}
% \end{figure*}





% \begin{figure}[t]
%     \centering
%     % \includegraphics[width=0.5\columnwidth]{figs/placeholder-eval-overall-1.pdf}
%     % \subfloat[][\centering{Object detection\\~~~~(Dashcam)}]
%     % {
%     %     \includegraphics[width=0.24\textwidth]{figs/detection_dashcam_FPN.pdf}
%     %     \label{subfig:1}
%     % }
%     \subfloat[][Profiling-based]
%     {
%         \includegraphics[width=0.32\columnwidth]{figs/behavior_profile.pdf} 
%         \label{subfig:1}
%     }
%     \subfloat[][Heuristics-based]
%     {
%         \includegraphics[width=0.32\columnwidth]{figs/behavior_output.pdf} 
%         \label{subfig:1}
%     }
%     \subfloat[][OneAdapt]
%     {
%         \includegraphics[width=0.32\columnwidth]{figs/behavior_oneadapt_arrow.pdf} 
%         \label{subfig:1}
%     }
    
%     \tightcaption{Contrasting \name with profiling-based approach and output-based approach. \name quickly approaches a near-optimal configuration via \outputgrad, while the profiling-based method requires a high amount of extra inference to derive the optimal configuration, and the configurations that the heuristics-based and output-driven approaches pick are of much lower accuracy than the optimal configuration.}
%     \label{fig:compare}
% \end{figure}





\tightsubsection{Existing configuration adaptation systems}
\label{subsec:configuration-adaptation}
% \kt{Need to finish this.}

% \begin{packeditemize}
%     \item Given that configuration needs to be adapted frequenty, three performance objectives: adayt frequently, converge to a near-optimal config, being generalizable
%     \item Profiling-based work
%     \item No extra inference => what should be the technique to use to get new configurations =>
%     \kt{1. the techniques all sounds like heuristics 2. key is no extra inference}
%     \begin{packedenumerate}
%         \item Video codec parameters (CASVA) -> use video segment size as the feedback. Encoding two small objects may have the same file size as one large object, but the former requires lower resolution while the latter requires larger one.
%         \item Video frame filtering: Reducto  FilterForward. Both limitation: send out frames when large object slowly moves
%         \item Fine-grained video quality assignment (camera-side heuristics (need to explicitly mention saliency) \& Server-driven).
%         \item DNN model selection and customization
%     \end{packedenumerate}
% \end{packeditemize}

% \jc{this part is important. right now the discussion is a bit dry. people have to parse through the lines to understand the tradeoffs, and even when they do, it's hard to get a sense how bad it could be. can you add a (real or synthetic) example that compares the adaptation behaviors of various baselines, like the one we drew on board?}


% \jc{a general feeling: this section sounds too similar to the middle of intro, and it's too abstract. it's ok to stay high level in intro, but we need more meat here. }


The key research question therefore is how to timely identify if a different configuration is better
% ---higher accuracy under a given resource budget, or much less resource usage while maintaining similar accuracy or both---
than the current configuration. 
We discuss two high-level categories of techniques.
% how to frequently identify the optimal configuration (the configuration with the highest accuracy under the resource budget)? 

% To adapt the large yet expanding set of knobs, prior works propose several techniques to determine how to select the \textit{configuration} (\ie the assigned values of all knobs) based on the current content of the input data stream. We classify them into two categories.
    

% As previous work shows, the knobs inside DNN-based analytic systems also need to be timely adapted~\cite{awstream,chameleon,dds,eaar,elf} to cope with the change of input data content (\eg timely stop the vehicle when a child suddenly runs across the street) in order to reduce the end-to-end delay while maintaining high accuracy.
% Thus, the research question is: how to navigate the large configuration space (\ie all possible choices of knob values) and  pick the optimal configuration that generates accurate inference results under the current resource budget?

    
% The first way to address this problem is to \textit{frequently profile} the
% system with different configurations to obtain their resource usage and
% inference accuracy, and then pick the configuration that meets the resource
% budget and generates the most accurate inference results~\cite{chameleon,awstream,vstore,videostorm}. 
% However, this approach
% needs to analyze extra configurations (in order to obtain the profile), thus requiring \textit{extra} inference to obtain the optimal configuration.
% As a result, when the optimal configuration changes, this approach needs to perform the extra inference to obtain the new optimal configuration, thus incurring high delay when the GPU resource is limited. 



\myparashort{Profiling-based methods: optimal though slow.} 
The first approach \textit{periodically profiles}
% different configurations to obtain their 
resource usage and
inference accuracy of different configurations by using them to run DNN inference, and then pick the best configuration (one that yields high inference accuracy and low resource usage)~\cite{chameleon,awstream,vstore,videostorm}.
% meets the resource
% budget and generates the most accurate inference results
However, each profiling
needs to run multiple \textit{extra} DNN inferences and thus significantly increases the GPU computation overhead. %before obtaining the profile.
% As a result, when the optimal configuration changes, this approach need to perform the extra inference to obtain the new optimal configuration, thus incurring high delay when the GPU resource is limited.
% Thus, when the GPU compute is limited, this approach needs to either profile less frequently, resulting in using outdated configurations when the optimal configuration has drifted away, or significantly prune the search space (which may contain only suboptimal configurations). 
%profile fewer configurations, which may miss the optimal configuration. 
% Both of them lead to a sub-optimal trade-off between the accuracy and the resource usage.
% \ga{Call out the downsides of extra inference.} \kt{fixed}
% The first type of work adapts the configuration by maintaining a profile (the resource usage and inference accuracy of each configuration).
% Concretely, this approach frequently update their profile by calculating the resource usage and accuracy of different configurations (we call this operation profiling), and picks the configuration that yields high inference accuracy without exceeding the resource budgets. 
% However, each profiling needs to run extra inference to analyze multiple configurations. 
% Thus, when the GPU compute is limited, this approach needs to either profile less frequently (resulting in using outdated configuratin when new events in the video happens and changes the optimal configuration), or profile less configurations (resulting in using sub-optimal configuration).
For instance, AWStream~\cite{awstream} runs full profiling on just 3 knobs (resolution, frame rate, and quantization parameter) on a \textit{10-second}
% \jc{is this what awstream uses?} 
video, and its GPU computation is equivalent to running normal DNN inference on  
% consumes the same amount of GPU computation as analyzing 
more than an \textit{8-minute} video (\ie an almost 50$\times$ increase in GPU usage). 
As a result, if GPU resource is limited,
% is not sufficient to support frequent profiling, 
this approach must either profile less frequently, causing it to use outdated configurations when the optimal configuration changes
% before launching the next profiling 
(as shown in Figure~\ref{fig:adaptation-behavior}), or profile only fewer configurations, which may miss the optimal configuration.
\S\ref{sec:eval} will also test smarter variants of profiling (profiling only top $k$ configurations and profiling fewer values per knob) and shows that they still use much GPU resource for extra inference and are thus slow to adapt to change in source data.
% there is a substantial room for improvement.
% For instance, one may run Chameleon~\cite{chameleon} (a state-of-the-art profiling-based algorithm) and tunes video frame rate and video resolution to detect cars in this dashcam video~\cite{youtube-example-profiling}. 
% From the beginning to the 256th second, as no car appears in this video, Chameleon will use a low frame rate and a low resolution to maximally save GPU compute.
% At the 257th second, a large moving car appears in the video.
% Say Chameleon happens to launch its profiling at the 257th second.
% Following Chameleon’s profiling logic, Chameleon needs to analyze 7 configurations and thus profiling these configurations may take 10 seconds for the profiling to finish\footnote{top-5 configurations, plus two expensive configurations —> ~10 seconds}.
% As a result, Chameleon will still use low resolution and low frame rate from the 257th second to the 267th second, resulting in low detection accuracy of this car (as the frame rate is too low to accurately capture the motion of this car) in this 10 seconds.



% Both of them lead to a sub-optimal trade-off between accuracy and resource usage.
% \ga{Call out the downsides of extra inference.} \kt{fixed}
% \jc{if possible, quantify it with some concrete numbers.} \kt{done}
% \jc{what if the GPU resource is not limited? reviewers may argue that awstream and chameleon cares about average GPU usage, and since they run in the cloud, they can scale up resource usage instantly if they choose to, and spread the burst across jobs. please clarify if they still can be improved in such settings or not.} \kt{rewrite part of the sentences to handle this case}

% \jc{can this be merged with the first type? i know there's some subtle difference, but it's unnecessarily complicated}
% The second approach performs no extra DNN inference and instead, picks the configuration based on the recent configuration and its corresponding DNN output (\eg pick the configuration through cheap heuristics~\cite{dds,eaar,elf} or through DNN-based configuration generator~\cite{accmpeg,casva}).
% However, there can be many configurations that meet the resource budget.\jc{this point is not coming across. back it up with a concrete example?}
% Without profiling most of them, it is difficult to separate the configurations that yield similar DNN output from those that yield more accurate DNN output.
% As a result, they cannot quickly identify the optimal configuration.

% \kt{1Reducto (threshold-based), DDS (server-side region proposal, RP not aware of DNN task), AccMPEG/saliency (cheap model), CASVA (cheap feature)}

% \jc{this example seems to repeat the intro example. why not briefly mention it and give another example or give more quantitative details?}

% \jc{Kuntai, ping me once you have free time to discuss this. the output-driven type comes out of the blue. we should be consistent with the intro. } 

% \mypara{Heuristics with no extra inference} 
\mypara{No extra inference though suboptimal}
An alternative approach~\cite{reducto,vigil,glimpse,accmpeg,casva,filterforward,dds,eaar,elf,fischer2021saliency} avoids extra inference and instead selects new configurations by analyzing the source data using simple heuristics.
This approach can adapt frequently as it does not require extra inference by the final DNN.
% allowing it to frequently 
% % This approach can quickly adapt 
% their configurations (\eg once every second~\cite{accmpeg}).
% to the input data as it performs no extra DNN inference.
% Since the process of obtaining the new configuration must be much less complex than final DNN inference, 
However, since these heuristics are simpler than the final DNN, they may select a suboptimal configuration (illustrated in Figure~\ref{fig:adaptation-behavior}).
% with high DNN inference accuracy 
% even though they adapt much earlier than the profiling-based method.
Here, we discuss three heuristics. % in this category and briefly explain why they fall short.

One line of work~\cite{reducto,glimpse,eaar} selects the frames most worthy for analysis by computing the difference between the current frame and previously analyzed frame\footnote{Reducto calculates frame differences based on various features of the source data (\eg pixel  feature~\cite{glimpse}, Edge feature~\cite{marr1980theory} and Haar feature~\cite{viola2001rapid}), while other papers simpler difference metrics~\cite{glimpse,eaar}.} and sends the current frame out for DNN inference if the difference is greater than a threshold.
As elaborated in \S\ref{sec:intro}, this method fails when the background pixels in a video change a lot between frames, making high frame difference a poor signal to decide if a frame should be analyzed or not.





% especially when the content of input data does not meet their assumptions.
% To further illustrate this point, we partition prior works into three categories according to the configuration they adapt.
% (\eg the video input data contains mostly large, easy-to-detect objects~\cite{accmpeg,vigil} or the video background is stationary~\cite{reducto,vigil,casva}).
% However, as these cheap heuristics are much less complex than the DNN, they generally generate configuration with accuracy much lower than the optimal configuration when the content of input data does not satisfy their assumptions, as shown in Figure~\ref{fig:adaptation-behavior}.


% \kt{\hl{New text of discussing prior works here.}}


\begin{comment}

One line of work focuses on filtering the input data that can be filtered without hurting the inference accuracy.
This approach evaluates send out the current frame when the likeliness of containing objects~\cite{filterforward} or the dis-similarity compared to previously-sent frame is greater than a threshold.
For example, Reducto~\cite{reducto} calculates frame difference between the current frame and previously sent frame\footnote{Reducto calculates frame differences based on various features of the input data (\eg pixel  feature~\cite{glimpse}, Edge feature~\cite{marr1980theory} and Haar feature~\cite{viola2001rapid}).}, and sent the current frame out if the difference is greater than a threshold.
% If the frame difference between the current frame and the previously-sent frame is larger than a threshold, Reducto will send out the current frame (as the objects likely move a lot in the current frame compared to previously-sent frame and thus this frame need to be sent out for analytics).
Reducto works well when the video background is stationary.
However, when the video background is quickly moving (\eg in dashcam video feeds), Reducto will send out frames even when there is no object appearing in the video (as the frame difference is constantly high due to the quick movement of the background), thus having not enough resource to frequently send out frames when the object-of-interest appears, resulting in low accuracy.

\end{comment}

% For example, Reducto cannot tune the resolution of each frame to reduce bandwidth usage without hurting the inference accuracy.

The heuristics can be smarter than computing frame difference.
A line of work reduces bandwidth usage by only encoding small spatial regions in high quality~\cite{dds,eaar,vigil,accmpeg,fischer2021saliency}, and they do so by running a {\em shallow NN} on each frame to select areas (sometimes called ``saliency'') whose pixel values are near the objects of interest.
However, these shallow NNs, unlike the final DNN, are inadequate to recognize small objects.
As acknowledged in one of the latest work~\cite{accmpeg}, it rarely recognizes small vehicles in highway video feeds and thus fails to encode them in high quality.
% Following a similar idea, some recent work~\cite{casva} also uses a shallow NN, but it feeds the NN with even simple features, such as current bandwidth usage, which eventually selects suboptimal configurations as we shown in \S\ref{sec:eval}.


Other heuristics try to leverage information naturally emitted from the final DNN, such as region proposals (an intermediate output of some DNNs that indicates which regions in the source data may contain objects).
This approach can also adapt quickly, but as shown in~\cite{accmpeg}, region proposals only indicate whether {\em some} objects are in the region, rather than whether raising the quality of that region will likely affect the ability for the DNN to detect the objects of interest.
% the inference of a particular DNN in consideration.

% In short, while a variety of heuristics are proposed to adapt configuration quickly without extra inference, they often select suboptimal configurations.

\mypara{Designed for specific configurations or DNNs}
Moreover, most techniques are studied and evaluated {\em only} on RGB video feeds, and it is unclear whether they will be effective on other types of data (\eg LiDAR point cloud, depth map, or audio waves).
Even in video analytics, the proposed heuristics often work well only for {\em specific knobs}.
As elaborated in \S\ref{sec:intro}, Reducto~\cite{reducto}'s frame-different detector is 
% For example, Reducto's logic~\cite{reducto} uses inter-frame difference to select the frames that most need to be analyzed, and thus is 
ill-suited to tuning the encoding quality parameter of each frame, which depends on the content of the new frame, rather than how it differs from the previous frame.
Likewise, DDS~\cite{dds} tunes the encoding quality parameters of each fine-grained spatial block to improve inference accuracy on each frame, but it is not aware of whether the current frame is redundant given past inference results, thus it cannot generalize to knobs such as frame selection.
Moreover, DDS relies on region proposals, which are common in object detection DNNs but not in other types of DNNs (\eg classification DNNs~\cite{vit,vgg} and semantic segmentation DNNs~\cite{unet,fcn-resnet101}).


\begin{comment}
Moreover, most prior work mainly focuses on analytics of RGB video feeds and is not generalizable to other applications or different sources of data (\eg 3D LiDAR data, audio data, etc). 
% \jc{why not a separate para?}
% Further, these techniques are tailored for frame filtering knobs and may be suboptimal when tuning other configuration knobs.
For example, Reducto cannot be repurposed for tuning the resolution of the video, as whether this frame should be encoded in high resolution depends on, for example, the size of the objects in this frame and does not depend on whether the current frame contains objects.


Another line of work focuses on adapting the encoding quality of different areas in the input video~\cite{dds,eaar,vigil,accmpeg,fischer2021saliency}.
Some of these works use cheap models~\cite{accmpeg,fischer2021saliency,vigil} to identify the areas in the input video that are highly related to the inference results (typically these areas are on the objects)\footnote{These areas are also named as salient regions in multi-media literature~\cite{fischer2021saliency}.} and encode these areas in higher encoding quality to allow the DNNs detect more objects.
These approaches adapt very frequently (\eg once per second~\cite{accmpeg}).
However, as these models are much cheaper than the final analytical DNNs, they may fail to detect these difficult-to-detect objects (\eg a small vehicle in a drone video or a human from the other side of the road).
For example, AccMPEG~\cite{accmpeg} trains a cheap MobileNet-SSD~\cite{ssd} model and runs this model once per second to detect these areas, and encode these areas in higher encoding quality.
However, as shown in~\cite{accmpeg,kisantal2019augmentation}, when there are a lot of small objects, the cheap model of AccMPEG fails to put those small objects in high encoding quality, making the small objects unable to be detected.
Figure~\ref{fig:previous-work-illustrative} shows an example, where AccMPEG fails to put some of the small objects into areas that will be encoded in high quality (the highlighted area).


Instead of relying on cheap models, one may also use region proposal~\cite{faster-rcnn} (an intermediate DNN output that indicates which regions in the input data may contain objects) to find the areas that need to be encoded in high encoding quality~\cite{dds,eaar}.
This approach can also quickly adapt (\eg once per second~\cite{dds}) to the change of input data.
That said, as the region proposal only classifies the region as containing objects or not~\cite{dds}, it may wrongfully include objects that are not of interest (\eg wrongfully include traffic signs in vehicle detection applications) and spend more resources on these objects than needed, resulting in low accuracy (as shown in Figure~\ref{fig:adaptation-behavior}).
This method is also not directly applicable to other applications, as it relies on region proposal of the DNNs, which is common in object detection DNNs but not in other types of DNNs (\eg classification DNNs~\cite{vit,vgg} and semantic segmentation DNNs~\cite{unet,fcn-resnet101}).
Also, as the region proposal highlights the \textit{spatial} regions that are more important, it is not aware of whether the inference results of current frame is  in terms of tuning knobs that operate on \textit{temporal} dimensions (\eg frame filtering knobs).
As a result, this approach may not generalize to tasks like classification and semantic segmentation and knobs like frame filtering knobs.


The third line of work focuses on tuning the encoding parameters of video codecs~\cite{casva}.
For example, CASVA~\cite{casva} obtain the resolution, frame rate and the quantization parameter by analyzing the history network statistics (\eg current bandwidth usage) using a reinforcement learning model.
However, CASVA is not aware of the analytic DNN.
As a result, CASVA cannot identify whether the current video frame contains the object of interest or not, making CASVA unable to increase the resolution or frame rate when the object of interest suddenly appears in the video, or decrease the resolution or frame rate when the object of interest dissapears in the video.



\begin{figure}
    \centering
    \includegraphics[width=0.5\columnwidth]{figs/Illustrative-AccMPEG.png}
    \tightcaption{
    \hl{AccMPEG illustration
    }}
    \label{fig:previous-work-illustrative}
\end{figure}
% \begin{packeditemize}
%     \item Adapting video encoding knobs (\eg video resolution)~\cite{casva}. 
%     However, the heuristics in this approach collect f
%     \item 
%     Adapting frame filtering thresholds (\eg pixel difference threshold)~\cite{reducto,filterforward,glimpse}.
%     \item 
%     Adapting 
% \end{packeditemize}
% For instance, 
% To further illustrate when will these heuristics generate a configuration with lower accuracy than the optimal one, We use Reducto~\cite{reducto} as an example. 

\end{comment}

% \mypara{Techniques specific to certain knobs or data types \kt{\hl{Call it frequent adaptation?}}}
% % \mypara{Output-driven} 
% The third line of work~\cite{dds,elf,eaar} also performs no extra inference and generates the new configuration by postprocessing historical DNN outputs (including intermediate outputs).
% Existing works rely on region proposal~\cite{faster-rcnn} (an intermediate DNN output that indicates which regions in the input data may contain objects) to tune the encoding quality of different spatial areas~\cite{dds,eaar} or tune the way to partition the input data for multi-server analytics~\cite{elf}.
% This approach can also quickly adapt (\eg once per second~\cite{dds}) to the change of input data.
% However, while region proposal is a common component in object detection DNNs, it is less common in classification DNNs~\cite{vit} and semantic segmentation DNNs~\cite{unet}.
% Also, as the region proposal highlights the \textit{spatial} regions that are more important, it may be less useful in terms of tuning knobs that operate on \textit{temporal} dimensions (\eg frame filtering knobs).
% As a result, this approach may not generalize to tasks like classification and semantic segmentation and knobs like frame filtering knobs.
% Moreover, as the region proposal only classifies the region as containing objects or not~\cite{dds}, it may wrongfully include objects that are not of interest (\eg wrongfully include traffic signs in vehicle detection applications) and spend more resources on these objects than needed, resulting in low accuracy (as shown in Figure~\ref{fig:adaptation-behavior}).


% For those works that analyze input data through cheap heuristics, their issue is that their cheap heuristics may generate configurations with much lower accuracy than the optimal configuration.
% For example, \kt{use reducto example here}.

% As for leverage inference results, existing works focus on video analytics and leverage region proposal (the regions that may contain objects) to identify which areas in the input video contains objects.

% Existing works focuses on video analytic applications and tune four types of configuration knobs.


% \mypara{Video encoding parameters}
% The first type of work indicates 

% \mypara{Fine-grained encoding quality assignment} 
% Take AccMPEG~\cite{accmpeg}, a recent proposal in this category, as an example.
% AccMPEG leverages a cheap DNN to identify which regions should be encoded in high quality (these regions are typically where the objects of interest appear).

% When AccMPEG processes the following video frame (we visualize this frame in the following figure), the heuristic that AccMPEG leverages (a shallow DNN) fails to put those small objects in high encoding quality, making the small objects unable to be detected.

% \mypara{Video frame filtering}
% One commonly used technique is to allow the camera to run a simple logic that identifies which frames are unimportant to the video analytic task and can be discarded~\cite{glimpse,reducto,filterforward,microsoft-rocket} or encoded with low quality.
% This approach is effective when the video content is relatively stable and the objects of interest are infrequent and easy to spot, such as in wildlife camera feeds where animals are the only moving objects on a static background and are therefore readily detectable.

% However, when the camera itself is quickly moving (\eg in dashcam videos or drone videos), these cheap heuristics may wrongfully send out frames that can be filtered out without sacrificing accuracy.
% We take Reducto, the state-of-the-art approach, as an example.
% Reducto calculates the frame difference\footnote{The frame difference in Reducto is calculated using multiple frame difference calculator, we use the phrase ``frame difference'' to make it easier for the reader to understand.} between the newly captured frame and previously sent frame, and send out the newly captured frame if the frame difference is large enough.
% In this downtown driving video~\cite{youtube-example-reducto}, as the video mainly contains large, slowly-moving vehicles, Reducto will choose a large frame difference thresholds to filter out most of the frames while maintaining accurate results.
% At the $1487^{th}$ second, all vehicles stop due to red light and people start to go across the street.
% As people are much smaller than the vehicles, they create small frame differences.
% Following Reducto's profiling logic, most of the frames will be filtered out.
% However, this significantly hurts the inference accuracy of detecting human as people are quickly walking through the street.

% \mypara{DNN model selection and customization}



% \mypara{Deriving configuration from DNN outputs} The second approach performs no extra inference and adapts the
% configuration based on recent DNN outputs, including the final outputs and the intermediate outputs (such as the raw bounding boxes that \textit{may} contain objects~\cite{dds,eaar,elf}) from the analytic DNN and other auxiliary DNNs (such as sensor-side cheap DNNs~\cite{accmpeg,casva}).
% For example, EAAR~\cite{eaar} tunes the encoding quality by collecting the regions generated from the DNN that may contain objects and then encodes these regions in higher encoding quality on future video frames.
% As a result, the objects that lie in these regions are much more likely to be detected.
% % For example, DDS~\cite{dds} tunes the encoding quality of different areas of the video in the following steps.
% % First, DDS lets the camera encode the whole video into low quality and streams it to the server.
% % The server then analyzes the video to obtain the areas that may contain objects and let the camera resend those areas in high encoding quality for an extra round of inference.

% However, the \textit{adaptation speed} (\ie the time it takes to obtain the optimal configuration) of this approach can be slow.
% This is because this approach only collects one DNN output at a time.
% % \jc{i don't get from the dds example that picking config based on dnn output is not a good idea.. partly because the dds's output does seem to contain rich information already?}
% As the relationship between the configuration to the inference accuracy is highly complex (due to complexity inside the analytic system (\eg video codec) and the DNN itself), this approach needs to spend time accumulating enough DNN outputs to obtain the optimal configuration, resulting in slow adaptation speed.
% Concretely, in EAAR, the regions generated by the DNN inference on one frame may miss some difficult-to-detect objects (like those tiny and distant vehicles) and EAAR needs to further adjust its regions in the future to include these objects.
% We demonstrate the slow adaptation speed of this approach in Figure~\ref{fig:adaptation-behavior}.

% % \jc{way too abstract and handwavy. im fine to drop it if you are not ready to add details} \kt{fixed}
% % In addition, the previous work in this approach designs hand-crafted heuristics catered only for individual applications or configurations.
% Moreover, the heuristics that previous work uses to compute the new configuration are not directly applicable to other knobs.
% % even if they can purposely-build to efficiently support some knobs. 
% % are hand-crafted for individual applications or configurations and thus not generalizable to other configurations and applications.
% Take EAAR as an example. 
% EAAR assigns the regions that may contain objects with higher encoding quality and thus detects more objects.
% However, EAAR may not be directly applicable to the knobs that saves GPU compute resource by avoiding the DNN inference on some frames.
% This is because adapting these knobs requires analyze the discarded frames \textit{before} inference to determine whether to perform inference on these frames, while the way EAAR analyzes one frame is by performing inference on this frame and \textit{then} extracting the intermediate results generated from the inference.
% Take DDS~\cite{dds} as an example, which analyzes the video and then resends some areas of the video that may contain objects of higher fidelity.
% As the resending areas are derived from the output of a specific DNN component (region proposal) that aims to facilitate object detection, this heuristic is not directly applicable to tasks like video classification, where the commonly-used DNN architecture for this task~\cite{i3d} does not contain region proposal module. 
% Moreover, this heuristic does not apply to tune frame-discarding knobs
% % the knobs in frame discarding techniques 
% (\ie discarding the frames that produce similar inference results compared to previous frames~\cite{vigil,glimpse,reducto}) without further adjustments, since its adaptation logic (\ie resending some areas of the video that may contain objects) happens \textit{after} DNN inference while frame filtering needs to be performed \textit{before} DNN inference to save GPU compute cost. 

% An ideal configuration adaptation systems should meet these two
% requirements: 1. quickly adapt to optimal configuration in a large configuration
% space without extra inference 2. minimum assumption to the underlying system
\mypara{Summary} 
In short, previous work fails to meet at least one of the three requirements: {\em (i)} adapt timely, {\em (ii)} converges to a near-optimal configuration, and {\em (iii)} apply to a wide range of configurations and applications.


% \mypara{Termiologies}
% To avoid potential confusion, we clarify several terms that we will use.
% \begin{packeditemize}
%     \item \textbf{Hyper-parameters (HPs):} the tunable hyper-parameters inside distributed AI systems. \qz{do you mean that HPs can also be referred to as knobs?}
%     \item \textbf{Knob values:} the candidate values that one knob can choose from.
%     \item \textbf{Configuration:} the concrete \textit{choice} of knob value for each knob. The configuration represents  
% \end{packeditemize}




% \begin{comment}


% \mypara{More knobs, more gain}
% Further, as AI systems keep on developing new knobs that may rely on different characteristics \qz{this word sounds weird, maybe say more knobs are available for tuning in AI systems and allow us to save resource usage in different fashions} to reduce the resource usage (and thus reduce the delay),  tuning more knobs altogether may provide huge potential. 
% Take camera-based object detection as an example.
% Assume that only 20\% of the frame is occupied by the objects, and the object only appear in 20\% of the frames.
% In this case, tuning frame filtering knobs or tuning spatial encoding quality reduce the number of pixels streamed out by 5x, thus achieving 5x saving on streaming delay in ideal cases\footnote{The actual streaming delay reduction will be lower because codec compression becomes more efficient when there are more pixels for the codec to use as reference.}.
% However, if we tune frame filtering knobs and spatial encoding quality knobs together, we only need to stream out $20\% \times 20\% = 4\%$ pixels, resulting in a 25x reduction on the streaming delay. \yh{add an example showing the benefits brought by coupling more knobs on reducing e2e delay }

% \mypara{Knobs need to be frequently tuned}
% To achieve the best \qz{optimal} trade-off between analytic accuracy and end-to-end delay, however, these knobs need to be \textit{frequently} tuned according to the incoming video content.
% Take AccMPEG~\cite{accmpeg} as an example system and camera-based vehicle detection as an example application.
% AccMPEG introduces the encoding quality of different spatial areas as its knob.
% It will aggressively compress those areas that are not related to the vehicles to reduce the streaming delay.
% So when a new object arrives, AccMPEG need to quickly adjust \qz{adapt} its knob to avoid aggressive compression on the areas related to the new incoming object.
% If AccMPEG does not adjust this knob, this object may be missed and result in low analytic accuracy.
% \kt{Provide empirical evidences here}



% \mypara{Previous work make inaccurate prediction of accuracy under current video content}
% In order to adjust the configuration, previous work either leverages a sensor-side model to predict the accuracy of different configurations, or use server-side feedback to perform this prediction.
% However, both of these two approaches predict accuracy in a sub-optimal way.

% \kt{Then say previous work cannot get this}

% \kt{Emphasize there are a lot of knobs}
% \kt{Emphasize that there are certain set of knobs that achieves combinitorial effect}

% \begin{table*}
%     \begin{tabular}{ c c c c }
%         \hline
%         Place & Analytic model & Number of inferences per second & Total FLOPs per second \\
%         Server & EfficientDet~\cite{efficientdet} (300G FLOPS) & 30 & 9000G FLOPs \\ 
%         Sensor & MobileNet SSD (2.3 GFLOPS)~\cite{ssd,ssd-runtime} & 23~\cite{ssd-fps,ssd-fps2} & 53G FLOPs (169x) \\
%         \hline
%     \end{tabular}
%     \caption{Comparison between server-side and sensor-side compute. The server has hundreds times more compute than the sensor.}
%     \label{tab:sensor-server-comparison}
% \end{table*}

% The first type of work use sensor-side model to obtain knob-accuracy impact.
% This model can be completely offline~\cite{vigil,glimpse,accmpeg} or periorically downloaded from the server~\cite{awstream,reducto}.
% However, as shown in Table compared to the server that can run heavy analytic models (that contains hundreds of layers and requires hundereds of GFLOPs~\cite{efficientdet,retinanet,amoebanet}) in real time (\eg 30 inferences per second), the sensor can only afford several GFLOPs even with the help of external hardware acceleration\cite{ssd,ssd-runtime}.
% As a result, the sensor-side model will have low accuracy when there are sudden changes in the incoming video content (\kt{several examples here}), resulting in sub-optimal accuracy-delay trade-off.


% The second type of work infer knob-accuracy impact from real-time server-side output (including intermediate output, like region proposals~\cite{dds,elf,eaar}).
% % Some previous work will directly obtain the knob-accuracy impact on a small chunk of video by exhaustively enumerate all knobs and their corresponding values and calculate the accuracy of these values on the whole video. 
% % However, this procedure introduces high streaming delay (the video need to be streamed in an uncompressed manner, which requires >10x time to stream from the camera to the server) and inference delay (one may need to even analyze >200 configurations to tune just 3 knobs~\cite{awstream}). 
% % As a result, this approach cannot obtain the knob-accuracy impact \textit{in real-time}. 
% % The other type of work will infer the knob-accuracy impact from the intermediate output of the DNN.
% As shown in Figure~\ref{fig:feedback-contrast}, after obtaining the DNN output\footnote{Some previous work may perform filtering to remove those outputs that, for example, have low confidence~\cite{dds,eaar}.}, previous work will overlay these outputs on the input to obtain a set of pixels, and assume those knobs that related to the pixels have high knob-accuracy impact. 
% However, the pixels that indicates high knob-accuracy impact do not necessarily align with the shape of inference results.
% Instead, some pixels outside the bounding boxes may contribute to the analytic results, and some pixels inside the bounding boxes may have low accuracy impact.
% This is because the pixels that outside the bounding boxes also participant in the computation of obtaining the inference results; the contribution of pixels inside the bounding boxes may be inhibited by the internel DNN computation (like ReLU activation and pooling).
% As a result, it cannot deliver accurate knob-accuracy impact by simply overlaying the output on the input.


% % These knobs need to be adjusted with the feedback from server-side DNN.

% % First type of work: fixed parameter

% % Second type of work: camera-side heuristics

% % Thrid type of work: real-time feedback

% % However, their feedback is suboptimal because they essentially rely on the output of the DNN to provide feedback.
% % The output only encodes the results of the computation, but loses the information of how the DNN perform this computation.
% % The latter is aso important to determine the relationship between knobs and the final analytic accuracy.


% % An example here.

% \end{comment}

==> motivation-short.tex <==
%!TEX root = main.tex
%!TEX spellcheck = en_US 


\tightsection{Motivation}
\label{sec:motivate}

We start with the background of video streaming for distributed video analytics, including its need, performance metrics, and design space. 
We then use empirical measurements to elucidate the key limitations of prior solutions. 

% \jc{need a brief primer on object detection and semantic segmentation}

\tightsubsection{Video streaming for video analytics}
\label{subsec:dva}


% \mypara{Distributed video analytics (DVA)}
% Many AI applications extract useful information from live video streams in a {\em distributed} fashion, because the analytics happens partially or completely in servers connected to cameras through network links.

%DNNs achieve very high accuracy on these vision tasks and are thus widely used.



\begin{figure}[t]
\centering
    \subfloat[Input]
    {
        \includegraphics[width=0.3\hsize]{figs/demonstrate_input.jpg}
        %\hspace{-1mm}
        %\label{fig:cost-acc-1}
    }
    \subfloat[Object detection]
    {   
        \includegraphics[width=0.3\hsize]{figs/demonstrate_obj.jpg}
        %\label{fig:cost-acc-2}
    }
    \subfloat[Sem. segmentation]
    {
        \includegraphics[width=0.3\hsize]{figs/demonstrate_seg.jpg}
        %\label{fig:delay-acc}
    }
\tightcaption{The input and output of object detection and semantic segmentation on one example image. We use red to label the car and blue to label the truck.}
\label{fig:vision-tasks}
\vspace{-0.2cm}
\end{figure}

\mypara{Vision tasks under consideration}
We consider three computer vision tasks---object detection, semantic segmentation, and face recognition. 
Figure~\ref{fig:vision-tasks} shows an example input and output of object detection (one label for each bounding box) and semantic segmentation (one label for each pixel).
These tasks are widely used in real-world scenarios to detect/segment objects of interest and their results are used as input to high-level applications (\eg vehicle collision detection). 


\myparashort{Why streaming videos out from cameras?}
% There are two contributing trends.
% Two trends contribute to the wide spread of distributed video analytics and much recent effort (\eg~\cite{awstream,cloudseg}).
%On one hand, low prices of high-definition cameras have led to a dramatic proliferation of video sensors~\cite{McKinsey,infowatch16,thenewstack,asmag}. % whose video feeds need automatic and accurate analysis~\cite{thenewstack,asmag}. 
\cameranew{
On one hand, computer vision accuracy has been improved by deep learning at the cost of increased compute demand.
On the other hand, low prices of high-definition network-connected cameras make them widely deployed in traffic monitoring~\cite{killer-app}, video analytics in retail stores~\cite{retail-video}, and inspection of warehouses or remote industrial sites~\cite{george2019towards}. 
Thus, the camera operators must scale out the compute costs of analyzing ever more camera feeds~\cite{McKinsey,thenewstack,asmag}.
One solution is to {\em offload the compute-intensive inference (partially or completely) to centralized GPU servers}. 
(Sometimes, video feeds must be kept local due to privacy regulations, but it is beyond our scope.)
% have enabled cheaply scaling out the analytics of ever more cameras~\cite{McKinsey,thenewstack,asmag}.
% While one can always add accelerators~\cite{jetson,deeplens} to cameras, 
For the sake of discussion, let us calculate the costs of 60 HD cameras each running ResNet50 classification at 90FPS.
We use ResNet50 classifier because our applications require more complex DNN models (\eg FasterRCNN-ResNet101) cannot run on Jetson TX2~\cite{jetson-fasterrcnn} at 30FPS. 
Now, buying 60 Raspberry Pi 4 Cameras and an NVIDIA Tesla T4 GPU (with a throughput of running ResNet50 at 5,700FPS~\cite{tesla-benchmark}) costs $\$23\times60$\textrm{(cameras)\cite{amazon-hd-cam}}$+\$2000$\textrm{(GPU)\cite{amazon-gpu}}$=\$3.4$K.
Buying 60 NVIDIA Jetson TX2 cameras (each running ResNet50 at 89FPS~\cite{jetson-benchmark-2}) costs about $\$400$\cite{jetson-price}$\times60= \$24$K, which is one order of magnitude more expensive.
These numbers may vary over time, but the price gap between two approaches is likely to remain.
The calculation does not include the network bandwidth to send the videos to a server, which is what we will minimize.
% Therefore, camera network operators increasingly stream videos from network-connected cameras to servers for deep learning inference in traffic monitoring~\cite{killer-app}, surveillance in buildings, video analytics in retail stores~\cite{retail-video}, and inspection of warehouses or remote industrial sites with drone cameras~\cite{george2019towards}. 
}


\cameraold{
% \myparashort{Why saving bandwidth?}
%First, while they are not as much, it's growing fast.
We aim to reduce bandwidth usage of video analytics for three reasons.
First, while many Internet videos are still destined to viewers, the video feeds processed by analytics engines have grown dramatically;
by one analysis, the amount of data generated by new video surveillance cameras installed in 2015 is equal to all Netflix's current users steaming 1.2 hours of ultra-high HD content simultaneously~\cite{infowatch16}.
%Second, the cost can be higher per stream than streaming video to users
Second, many cameras are deployed in the wild with only cellular network coverage~\cite{IoT-cellular}, so setting up network connections and sending videos upstream to remote servers can be expensive (more so than streaming videos from CDN servers to wifi-connected PCs).
%Third, compared to servers, the cost cannot be amortized
Finally, while purchasing GPU servers is not cheap, it is a one-time cost that is amortized over time (so cheaper in the long run); while the communication cost is not amortized thereby incurring substantial operational costs for many large-scale camera networks.%~\cite{IoT-cellular}. 
}


%
%Although video feeds destined to analytics are currently not as many as Internet videos destined to viewers
%
%
%the volume of video streams is experiencing a super-linear growth of video sensors whose video streams are tied to the continuous activity of all video sensors~\cite{ChicagoCam,LondonCCTV,VideoAnalyticsMarket,slate-video-news,infowatch16}.
%
%
%
%
%and the need for bandwidth efficient streaming.
%
%
%
%
%This work mostly focuses on reducing the bandwidth usage while maintaining high accuracy. 
%This is because lower bandwidth demand means that the server-side DNN will receive data more quickly and the communication cost will be lower. 
%Unlike cost of purchasing in-house servers can be amortized over time, the communication cost cannot and could be a major contributing factor to the operational cost of a large-scale camera network~\cite{IoT-cellular}. 


% : Buying 180 HD cameras (at less than \$30 each) and a NVIDIA Tesla T4 GPU (at \$2,000) that has a benchmarked ResNet throughput of 5,400 images per second~\cite{tesla-benchmark} is at least one order of magnitude cheaper than buying 180 NVIDA Jetson TX2 cameras (at more than \$600 each) which achieves the same throughput~\cite{jetson-benchmark}.
%\jc{get a quote on the cost of 100 hd cameras + 100 cloud gpus vs. 100 jetson cameras}


% \jc{introduce object detection and face recognition, and they are widely used} \hh{If you have references for each of these scenarios, it would be very helpful to add a citation for each to back up the claim of wide usage.}


\mypara{Performance metrics}
An ideal video streaming protocol for video analytics should balance three metrics: accuracy, bandwidth usage, and freshness.
% Here, we define them in multi-class object detection and semantics segmentation. %and \S\ref{subsec:eval-method} will define them in face recognition and semantics segmentation as well.
\begin{packeditemize}
	\item {\em Accuracy:} 
	\cameranew{We define accuracy by the {\em similarity} between the DNN output on each frame when the video is streamed to the server under limited bandwidth and the DNN output on each frame when the original (highest quality) video is streamed to the server.
	By using the DNN output on the highest-quality video (rather than the human-annotated labels) as the ``ground truth'', we can reveal any negative impact of video compression and streaming on DNN inference, without being affected by any errors made by the DNN itself. This is consistent with recent work (\eg~\cite{awstream,chameleon,videostorm}).
% 	of video streaming protocol and the inference results under unlimited bandwidth.
	We measure the accuracy} by\cameraold{ the standard metrics:} {\em F1 score} in object detection (the harmonic mean of precision and recall for the detected objects' location and class labels) and by IoU in semantic segmentation (the intersection over union of pixels associated to the same class). 
%    We use the outputs of running the server-side DNN over the video in its highest quality as the reference and treat them as the ground truth when calculating accuracy.
%	This is consistent with other work (\eg~\cite{awstream,chameleon,videostorm}). %\jc{need to be changed once eval is updated}
% 	Similarly, we use F1 score as an accuracy metric in face recognition by calculating precision and recall of the detected faces' location and identities.
% 	As a baseline, we consider the best possible accuracy to be that achieved when the highest quality video is sent to the server in its entirety.
    \cameranew{
    \item {\em Bandwidth usage:}
    % \item {\em Cost:}
    In general, the total cost of operating a video analytics system includes the camera cost, the network cost paid to stream the video from the camera to the server, and the cost of the server.
    In this paper, we focus on reducing the network cost through reducing the bandwidth usage. 
    \S\ref{subsec:limitations} will highlight the deployment settings in which the total costs of a video analytics system are dominated by the network cost and thus reducing bandwidth usage is crucial.}
    % We further divide this sum by the number of cameras and the number of frames to make this metric agnostic to them.
%     }
% 	\item {\em Bandwidth usage:} 
% 	\cameranew{
%     To reduce the cost, our work focuses 
%     So we also put bandwidth usage here as a metric.
	We measure the bandwidth usage by the size of the sent video divided by its duration. 
% 	\eg if some camera-server connections go through cellular networks that charge proportional to the data usage.
    \cameranew{
	\item {\em Average response delay (freshness):} %\kt{Response delay -> Processing delay for consisitancy?}
	Finally, we define freshness by the average processing delay per object (or per pixel for semantic segmentation), \ie the expected time between when an object (or a pixel) first appears in the video feed and when its region is detected and correctly classified, which includes the time to send it to the server and to run inference on it.\footnote{\cameranew{Average response delay is meaningful if the follow-up analysis can by updated when a new objects/pixel is detected/classified (\eg estimating the average speed of vehicles on a road). %and dynamically updating their results when more results are available.
	That said, this definition does not apply to applications that are sensitive to {\em worst-case} delays rather than average delay, \eg if one queries for the total number of vehicles, the answer will not be completed until all vehicles are detected. 
% 	analytic results until the last object has been received (like count the number of the objects in each frame). 
% 	For these applications, the worst-time response delay might be a better metric. 
% 	However, other applications may care more about the average properties of the objects (like calculating the average size of the objects). 
% 	These applications could update their analytic results when the new inference results come and thus care more about the average response delay.
	}}
	
%	We report the average delay. 
	%\hh{This one reads a little funny.  It sounds like objects that aren't detected would decrease the average delay.  Could we just say that the processing delay is the time between when pixels are produced and the analytics produces the final result for those pixels?}
	}
\end{packeditemize}
% \hh{Consider cutting the paragraph below for space}.
% DVA requires streaming support that simultaneously achieves high accuracy, low bandwidth, and low response delay.









%\jc{need to make a stronger case for saving (even just 2x) bandwidth. see more details in todos}
% Note that processing delay and bandwidth demand are related not always correlated,
% , but bandwidth demand sometimes can be reduced at the cost of increased processing delay, 
% \eg by adding more  frames, one can significantly reduce the video size but at the same time the server needs to accumulate more frames before being able to decode the video and run inference. 
% For the sake of explanation, we preclude the use of tricks and compare different solutions in accuracy and bandwidth demand while keeping processing delay at a constant low value.
% However, we will evaluate all three dimensions in \S\ref{sec:eval}.

% \jc{also need to make clear how much computing power we assume on the client and server}

%\begin{itemize}
%    \item video analytics is popular. a common practice is to stream videos to a remote server for compute-intensive analysis
%    \item two main metrics of success: accuracy, real-timeness. in this paper, we focus on object detection, face recognition.
%\end{itemize}




%\jc{when is it a good trade to reduce the number of bits transported at the expense of server-side GPU resources?}


\tightsubsection{Design space of video analytics systems}

\cameranew{
Next, we discuss the design space of how video analytics systems can potentially navigate the tradeoffs among these performance metrics along five dimensions:
% To demonstrate how existing works explored the design space of serving a single video stream for analytic purpose, we present a overview on the existing design dimensions. These dimensions are:

\begin{packeditemize}

\item {\em Leveraging camera-side compute power:}
Since the camera can naturally access the raw video, one can leverage the camera's local compute power (if any) to discard frames~\cite{noscope,glimpse} or regions~\cite{eaar,vigil} that may not contain important information.
As we will elaborate in \S\ref{subsec:machine-centric}, the accuracy of such local filtering heuristics may cause significant accuracy drops.
% The advantages for camera are that the camera not shared by any other video stream and could assess the raw video with no delay. To leverage this property, Vigil\cite{vigil} and Glimpse\cite{glimpse} harvest the compute at the camera to propose key frames and reduce the inference cost.


\item {\em Model distillation:} DNNs are often trained on large datasets, but when used exclusively for a specific category of video scenes, a DNN can be shrunk to a much smaller size (\eg via knowledge distillation), in order to save compute cost (GPU cycles) without hurting accuracy (\eg~\cite{noscope}).
This approach is efficient only in training smaller DNNs that work well on less expensive hardware.
% but are actually used on a single video stream. By training on this video stream, we could effectively ``shrink'' the deep learning models, thus save the inference cost. (e.g.: NoScope\cite{noscope}).

\item {\em Video codec optimization:} 
Unlike traditional video codecs that optimize for human visual quality, video analytics emphasizes inference accuracy and thus opens up possibility to more analytics-oriented video codecs (\eg analytics-aware super resolution~\cite{cloudseg}).\cameraold{\item Edge-based optimization. The edge strike a balance between the two extreme: accessing the video content fast and free but has limited compute (like the camera) and equipping sufficient compute but are bounded by the network latency and bandwidth  (like the server). Thus, there are a lot of previous works that exploits this design dimension (e.g. EAAR\cite{eaar}).}



\item {\em Temporal configuration adaptation:} 
To cope with the temporal variance of video content, one can adapt the key configurations (\eg the frame rate, resolution and DNN model) to save compute costs~\cite{chameleon} or network costs~\cite{awstream}.
That said, it fails to exploit the uneven spatial distribution of important information in videos. 



\item {\em Spatial quality adaptation:}
Information of interest (\eg target objects) is sparsely distributed in each frame, so some pixels are more critical to accurate DNN inference than others.
One can save bandwidth usage by encoding each frame with a spatially uneven quality distribution (\eg region-of-interest encoding~\cite{eaar}) so that high video quality is used only where pixels are critical to DNN inference~\cite{eaar,vigil}. 
% Our work also lies in this design dimension.
% Note that this optimization could also reduce the streaming delay through transferring less data through network.

\end{packeditemize}
In this paper, we take a pragmatic stance to focus on a specific point in the design space---no camera-side frame-dropping heuristics, no model distillation (use the server-side DNN as-is), and no change to the video codec; instead, we use the server-side DNN output to drive spatial quality adaptation.

}

\begin{figure}
\centering
\includegraphics[width=0.9\columnwidth]{figs/contrast-user-machine-new.pdf}
\tightcaption{Unlike video streaming for human viewers, machine-centric video streaming has unique bandwidth-saving opportunities. 
% such as frame dropping and spatial cropping.
}
\label{fig:contrast}
\end{figure}

\tightsubsection{Potential room for improvement}
\label{subsec:machine-centric}


% We argue that video streaming for video analytics presents abundant opportunities to improve accuracy and bandwidth usage, but the opportunities are largely untapped since current solutions are largely based on protocols designed for traditional video applications (\eg YouTube, Netflix).


% \mypara{New opportunities} 
Traditional video streaming maximizes human quality of experience (QoE)---a high video resolution and smooth playback (minimum stalls, frame drops or quality switches)~\cite{festive,conviva-understanding,akamai-qoe}. 
For machine-centric video streaming, however, it is crucial that the server-received video has sufficient video quality in the regions that heavily affect the DNN's ability to identify/classify objects; however, the received video does not have to be smooth or have high quality everywhere.

% \ktedit{XXX}
% \kt{???}

% Traditional video streaming strives to maintain a high video resolution and smooth playback (minimum stalls, frame drops or quality switches)~\cite{festive,conviva-understanding,akamai-qoe}.
% In contrast, 
% video streaming for video analytics is {\em machine-centric}. 

% These differences open up new opportunities that would not have been possible in traditional video streaming. 
This contrast has a profound implication---machine-centric streaming could achieve high ``quality'' (\ie accuracy) using much less bandwidth.
Each frame can be spatially encoded with {\em non-uniform quality levels}.
In object detection, for instance, one may give low quality to (or even blackout) the areas other than the objects of interest (Figure~\ref{fig:contrast}(b))\footnote{This may look like region-of-interest (ROI) encoding~\cite{meddeb2016region}, but even ROI encoding does not completely remove the background either, and the ROIs are defined with respect to human perception.}. 
While rarely used in traditional video streaming,
% , but seeks to maintain a smooth quality degradation from where users are likely to see to the background.
this scheme could significantly reduce bandwidth consumption and response delay, especially because objects of interest usually only occupy a fraction of the video size.
Figure~\ref{fig:motivation-spatial-cdf} shows that across three different scenarios (the datasets will be described in \S\ref{subsec:eval-method}), in 50-80\% of frames, the objects of interest (cars or pedestrians) only occupy less than 20\% of the spatial area of a frame.
We also observe similar uneven distributions of important pixels in face recognition and semantic segmentation.
% \hh{Without tick marks on the axes, I don't think you can draw these conclusions from the chart.  Is this just a placeholder for now?}
% Second, along the temporal dimension, frames can be sampled non-uniformly so that more frames should be sampled when objects are moving quickly and fewer frames are sampled when objects are moving slowly (or no object of interest is present).
% This opens up more opportunities to save bandwidth, since fast-moving objects may not be dominant.
% For instance, we found that in \fillme dataset, \fillme\% of the objects moves at very low speeds so that a frame rate of 1 frame-per-second (fps) is sufficient to identify its location, whereas the original videos are 30fps.
The question then is how to fully explore the potential room for improvement?


\begin{figure}
\centering
\includegraphics[width=0.6\columnwidth]{figs/motivation-cdf.jpg}
\tightcaption{Bandwidth-saving opportunities: Over 50-80\% of frames, the objects (cars or pedestrians) occupy less than 20\% of the frame area, so most pixels do not contribute to the accuracy of video analytics.
%This property suggests assigning quality levels non-uniformly could greatly reduce bandwidth demand without hurting accuracy.
}
\label{fig:motivation-spatial-cdf}
\vspace{-0.2cm}
\end{figure}


%\begin{itemize}
%    \item unique opportunities in video streaming compared to traditional video streaming (Figure~\ref{fig:contrast}):
%    \begin{itemize}
%        \item no need for uniform frame sampling
%        \item no need for background, etc
%    \end{itemize}
%\end{itemize}




% \tightsubsection{Taxonomy of current solutions}
% \label{subsec:taxonomy}

\subsection{\hspace{-0.3cm}Preliminary comparison of existing solutions}
\label{subsec:limitations}
\cameranew{
We present a framework to compare the performance, in accuracy, total cost, and response delay, of four baselines: camera-side local inference (``Camera-only''), server-side inference (``AWStream''), and selecting frames/regions by the camera and sending them to server for further analysis (``Vigil'' and ``Glimpse''). 
We then analyze the sources of their (suboptimal) performance in \S\ref{subsec:sources-of-limitations}.
The tests are performed on the traffic videos in our dataset (\S\ref{subsec:eval-method}). 
We will give more details about their implementations and include more baselines in the full evaluation (\S\ref{sec:eval}).
}

\cameranew{
% \mypara{Comparison among existing solutions}
For each solution $\Pipeline$, we use a fixed camera-side logic $\Local_{\Pipeline}$ and a fixed server-side DNN $\Remote_{\Pipeline}$. 
We use $\Workload_{\Pipeline}$ to denote the data (frames or videos, depending on the solution) sent from the camera to the server.
They together determine the accuracy of $\Pipeline$: $\Accuracy(\Local_{\Pipeline},\Remote_{\Pipeline},\Workload_{\Pipeline})$.\footnote{Of course, the value $\Workload{\Pipeline}$ and accuracy are video-dependent, but we omit it for simplicity since we compare solutions on the same videos.}
Note that $\Workload_{\Pipeline}$ is tunable by changing the internal configurations of $\Pipeline$, and with fixed $\Local_{\Pipeline}$ and $\Remote_{\Pipeline}$, the cost-delay-accuracy tradeoff of $\Pipeline$ will be governed by $\Workload_{\Pipeline}$.
We use the same server-side DNN (FasterRCNN-ResNet101) to make sure the accuracies are calculated with the same ground truth. 

Figure~\ref{fig:delay-acc} shows the delay-accuracy  tradeoffs of the four solutions (and our solution which will be introduced in next section). Here, the delay is the average response delay per frame as measured in our testbed. 
(We explain the hardware choice in \S\ref{subsec:eval-method}.)
Note that the local model running on the camera (``Camera-only'') has relatively lower accuracy than Vigil (which uses both the local DNN and the server DNN) and AWStream (which fully relies on the server DNN results). 
We will explain the reasons in \S\ref{subsec:sources-of-limitations}.

Figure~\ref{fig:cost-acc-1} and Figure~\ref{fig:cost-acc-2} show the costs to achieve their respective performance in Figure~\ref{fig:delay-acc} under two price settings. 
We measure the cost by the average total cost of analyzing a 720p HD video at 30FPS ($\sim$5Mbps) for an hour.
}


\begin{figure}[t]
\captionsetup[subfigure]{justification=centering}
\centering
    \subfloat[Delay-accuracy]
    {
        \includegraphics[height=0.23\columnwidth]{figs/acc-delay.pdf}
        \label{fig:delay-acc}
    }
    \subfloat[Cost vs accuracy (Setting~1)]
    {
    % \captionsetup{justification=centering}
        \includegraphics[height=0.23\columnwidth]{figs/acc-cost-1.pdf}
        \label{fig:cost-acc-1}
    }
    \subfloat[Cost vs accuracy (Setting~2)]
    {   
        \includegraphics[height=0.23\columnwidth]{figs/acc-cost-2.pdf}
        \label{fig:cost-acc-2}
    }
\tightcaption{The trade-offs among cost, delay, and accuracy on the traffic videos in our dataset under two settings. The cost in setting~1 is dominated by the network cost, so schemes that save bandwidth usage are more favorable. 
The cost in setting~2 is dominated by the server cost, so saving bandwidth does not yield better solutions.}
\label{fig:cost-delay-acc}
\vspace{-0.2cm}
\end{figure}




\begin{packeditemize}

\cameranew{
\item {\em Setting 1 (Total cost is dominated by network):} A camera is connected to an {\em in-house} server through an {\em LTE} network. 
Since the camera and the server are purchased upfront, their costs amortized per frame will approach zero in the long run, but the LTE cost is paid by time. 
Here, we consider the AT\&T 4G LTE plan, \$50 per month~\cite{4G-plan} for 30GB data (before the speed drops to measly 128kbps)~\cite{upload-speed}, or equivalently \$0.75 for streaming at 1Mbps for one hour.
% \footnote{\jc{more about how IoT companies strike better deals with cellular carriers, but may not be much cheaper given their prices are similar and LTE is the only choice in the wild.}}
Thus, the per-hour total cost of a solution $\Pipeline$ is $\Cost_{\Pipeline}\approx\$0.75\cdot\Size(\Workload_{\Pipeline})$, where $\Size(\Workload)$ is the total bandwidth usage (in Mbps) to send $\Workload$.
}


\cameranew{
\item {\em Setting 2 (Total cost is dominated by server):} A camera is connected to a {\em cloud} server through {\em cheap} wired network.
Unlike the previous setting, the cloud server is paid by usage so its cost grows with more server-side compute, but the network cost is negligible compared to 4G LTE plans.
To run the server-side DNN at 30FPS, we assume that we need 3 NVIDIA Telsa K80 cards and it costs \$0.405 per hour~\cite{google-gpu-pricing} (and other cloud providers have similar price ranges).
The per-hour total cost of $\Pipeline$, therefore, is $\Cost_{\Pipeline}\approx\$0.405\cdot\Fraction(\Workload_{\Pipeline})$, where $\Fraction(\Workload)$ is the number of frames in $\Workload$ divided by all frames.
}


\end{packeditemize}


\cameranew{
%According to Figure~\ref{fig:cost-acc-1} and Figure~\ref{fig:cost-acc-2}, 
In the first setting (Figure~\ref{fig:cost-acc-1}, where the total cost is dominated by the network cost), prior solutions show unfavorable cost-accuracy tradeoffs (when compared with our solution). 
However, in the second setting (Figure~\ref{fig:cost-acc-2}, where the total cost is dominated by the server cost), prior solutions in general strike good cost-accuracy tradeoffs (compared with ours).
This is largely because some of them (Vigil and Glimpse) are designed to minimize server-side compute cost, which this paper does not explicitly optimize.
%since they are explicitly designed to , even better than ours, because the total cost is dominated by the server cost, which we do not explicitly optimize.
%In the remainder of this paper, we focus on the first setting and look closely why existing solutions are suboptimal.

}



%\mypara{Limitations of existing solutions}
\tightsubsection{Sources of the limitations}
\label{subsec:sources-of-limitations}

Existing solutions for video streaming are essentially {\em source}-driven---the decisions of which pixels/frames should be compressed and sent to the server are made by the source (camera), with little real-time feedback from the server-side DNN that analyzes the video.
The fundamental issue of source-driven protocol is that any heuristic that fits camera's limited compute capacity is hard to precisely identify the minimum information that is needed by the server-side DNN to achieve high accuracy.
The result is a unfavorable trade-off between bandwidth and accuracy 
(\eg Figure~\ref{fig:cost-acc-1}):
any gain of accuracy comes at the cost of considerably more bandwidth usage.

\begin{figure}[t]
\centering
\includegraphics[width=1\columnwidth]{figs/drone_16.pdf}
\tightcaption{Contrasting the inference results between a cheap model (SSD-MobileNet-v2) and a compute-intensive model (FasterRCNN-ResNet101) on the same image. The compute-intensive model is more accurate when the video content is challenging (\eg  having many small objects).
%\jc{update these figures?}
% \jc{this figure is a bit weird. why the small model (the left one) cannot detect large objects but can detect smaller ones?}
% \kt{The object size are nearly the same except for the one that lies in the middle of the road.}
}
\label{fig:contrast-model}
\vspace{-0.2cm}
\end{figure}

This problem manifests itself differently in two types of source-driven solutions.
The first type is {\em uniform-quality streaming}, which modifies the existing video protocols and adapts the quality level to maximize inference accuracy under a bandwidth constraint.
For instance, AWStream~\cite{awstream} uses DASH/H.264 and periodically re-profiles the relationship between inference accuracy and video quality. %and select a lower-than-throughput quality level with maximum inference accuracy. 
CloudSeg~\cite{cloudseg} sends a video at a low quality but upscales the video using super resolution on the server.
They have two limitations.
First, they do not leverage the uneven distribution of important pixels; instead, the videos are encoded by traditional codecs with the same quality level on each frame.
Second, while they get feedback from the server DNN, it is not based on real-time video content, so it cannot suggest actions like increasing quality on a specific region in the current frame.

The second type is {\em camera-side heuristics} that identifies important pixels/regions/frames that might contain information needed by the server-side analytics engine (\eg queried objects)  by running various local heuristics (\eg checking significant inter-frame difference~\cite{glimpse,eaar}, a cheap vision model~\cite{vigil,adascale,nn-meets-pn,noscope}), or some DNN layers~\cite{cracking,ddnn}.
These solutions essentially leverage the camera-side compute power to save server compute cost and network cost~\cite{cracking}. 
%For instance, some solutions (\eg~\cite{glimpse,noscope,eaar}) rely on the inter-frame differences to signal which frames contain objects. 
However, these cheap camera-side heuristics are inherently less accurate than the more complex DNN models on the server, especially when the video content is challenging (\eg consisting of many small objects, which is typical for drone and traffic videos, as illustrated in Figure \ref{fig:contrast-model}).
Any false negatives of these camera-side heuristics will preclude the server from detecting important information; any false positives (\eg pixel changes on the background) will cost unnecessary bandwidth usage. 
% \jc{mention EAAR as relying on camera logic to select frames, though it uses some server-side information (region proposal) like Glimpse}
%We will discuss more related work in \S\ref{subsec:eval-overall}.




\cameraold{





We measure the total cost by the average cost to process, stream and analyze a 720p HD video at and 30FPS ($\sim$5Mbps) for an hour.
Given the per-frame pricing model of the camera $\Cost^{\camera}$, the network $\Cost^{\network}$ and the server $\Cost^{\inference}$, the total cost of $\Pipeline$ is:
$$\Cost_{\Pipeline}=\Cost^{\camera}(\Local_{\Pipeline})+\Cost^{\network}(\Workload_{\Pipeline})+\Cost^{\inference}(\Remote_{\Pipeline},\Workload_{\Pipeline}).$$
Similarly, given average per-frame delay of the camera $\Time^{\camera}$, the network $\Time^{\network}$, and the server $\Time^{\inference}$,
%, and the fraction of objects analyzed by the server $\Fraction_{\Pipeline}$ (largely proportional to $\Workload_{\Pipeline}$), 
the average response delay of $\Pipeline$  can be expressed by:
$$\Time_{\Pipeline}=\Time^{\camera}(\Local_{\Pipeline})+\Time^{\network}(\Workload_{\Pipeline})+\Time^{\inference}(\Remote_{\Pipeline},\Workload_{\Pipeline}).$$
To restrict the variables and for a fair comparison, we evaluate these solutions under the same task (object detection) and DNN models (\eg the FasterRCNN-ResNet101 as the server-side model and SSD-MobileNet-v2 as the camera-local DNN model). We elaborate on these choices in \S\ref{subsec:eval-method}.
It is crucial that we preserve the key distinction  between solutions---what to send to the server ($\Workload_{\Pipeline}$) and the camera-side logic $\Local_{\Pipeline}$---so the comparison is meaningful after the restrictions.
\jc{mention what's real and what's simulated}

%In the ensuing discussion, we seek to minimize the cost while achieving accuracy target of 0.8 and response delay less than 1.5 seconds, and compare existing solutions (and ours which will be introduced in the next section) 
%under two concrete deployment settings. 



To calculate the delay, we use \fillme as the camera, \fillme as the server, and \fillme as the network, and benchmark their average per-frame delay of each solution (please refer to
\kt{finish the appendix}Appendix~\ref{app:??} for details).
Figure~\ref{fig:cost-delay-acc} shows the accuracy-cost tradeoffs of the four solutions. 

\begin{packeditemize}
\item {\em Setting \#1 (Cost dominated by network):} A camera is connected to an {\em in-house} server with {\em LTE} networks. 
Since the camera and the server are purchased with a one-time upfront cost, their costs per frame will converge to zero in the long run, but the LTE data are paid by time and bandwidth usage. 
In particular, we consider an example AT\&T 4G LTE plan of \$50 per month~\cite{4G-plan} for 30GB data (before speed drops a measly 128kbps)~\cite{upload-speed}, or equivalently \$0.75 for streaming at 1Mbps for one hour.\footnote{\jc{more about how IoT companies strike better deals with cellular carriers, but may not be much cheaper given their prices are similar and LTE is the only choice in the wild.}}
Thus, the per-frame total cost of a solution $\Pipeline$ is $\Cost_{\Pipeline}\approx\Cost^{\network}(\Workload_{\Pipeline})=\$0.75\cdot\Size(\Workload_{\Pipeline})$, where $\Size(\Workload)$ is the total bandwidth usage (in Mbps) to send data in $\Workload$ (after video encoding).




\item {\em Setting \#2 (Cost dominated by server):} A camera is connected to a {\em cloud} server through {\em cheap} wired network.
Unlike the previous setting, the cloud server is paid by usage so its cost grows with more server-side compute, but the network cost is negligible compared to 4G LTE plans, so is the one-time upfront cost of camera.
To run the server-side DNN at 30FPS, we assume that we need 3 NVIDIA Telsa K80 cards and it costs \$0.405 per hour, based on the quote from Google Cloud~\cite{google-gpu-pricing}. (Other cloud providers have similar price ranges.)
The per-frame total cost of $\Pipeline$, therefore, is $\Cost_{\Pipeline}\approx\Cost^{\inference}(\Remote_{\Pipeline},\Workload_{\Pipeline})=\$0.405\cdot\Fraction(\Workload_{\Pipeline})$, where $\Fraction(\Workload)$ is the fraction of all frames in $\Workload$.



\end{packeditemize}




As we will see, in the first setting, prior solutions show an unfavorable tradeoff between cost (which is dominated by network cost) and accuracy (compared to our solution), whereas in the second setting, some prior solutions are performant as the cost is dominated by the server cost, which we do not explicitly optimize.




\mypara{Cost} As for the camera-side cost, from \cite{wired-camera-cost}, we know that a wired camera is about 150\$. We let all VAPs use this camera (this will make the cost of Glimpse strictly smaller) except for Vigil. For Vigil, to support 30fps inference on Mobilenet-inception-v2, we need at least 3 NVIDIA Jetson TX2 \cite{jetson-inference-speed} while each of them cost 490\$\cite{jetson-price}. Thus, we write:
$\Cost_{cam}=3\times 490\times 10^{-9}$ for Vigil and
$\Cost_{cam}=150\times 10^{-9}$ for other solutions.
As for the network cost, since the camera is wired, the bandwidth cost is a one-time cost that are the same fr all VAPs and could be amortized through time. Thus, we write $\Cost_{\network}= 0$ for all solutions.
%$Renting one NVIDIA GTX 1080 would be about 71.8\$ per month %$\cite{rent-gtx1080-price}. 
%The detection model faster-rcnn-resnet101 will run in 106ms on NVIDIA GTX Titan X. Based on the FLOPs listed in \cite{gpu-flops-comparision}, we infer that a NVIDIA GTX 1080 could run faster-rcnn-resnet101 at about 7.5 fps.
As for the server-side cost, from \cite{google-gpu-pricing}, we know that one NVIDIA Tesla K80 GPU will be $206.590\$$ per month.
Based on \cite{titanX, model-zoo,k80}, we infer that a NVIDIA Tesla K80 GPU could support about 10 fps inference on Faster-rcnn-resnet101.
Thus, to achieve 1 inference per frame, we need about 7437\$ per year.
Based on this, we write:
$
\Cost_{srv} = \Workload^{\Pipeline}\times 7437\times 10^{-9}
$
According to the information above and based on our experimental results, we plot the cost v.s. accuracy of pure server (AWStream will be strictly worse due to profiling cost at server-side), Vigil, Glimpse, pure camera and \name in Figure \ref{fig:suboptimal-cost-acc}.

% $$
% \Time_{\buffer}^{\Pipeline} + \Time_{\process}^\Pipeline + \Ratio^{\Pipeline} \cdot (\Time_{\network}^{\Setting}(\Size^{\Pipeline}(\Accuracy)) + \Time_{\inference}+\Time_{\latency}^{\Pipeline}),
% $$

% $$
% \Time_{\camera}^{\Setting}(\Model^{\Pipeline}(\Accuracy)) + \Workload^{\Pipeline} \cdot (\Time_{\network}^{\Setting}(\Size^{\Pipeline}(\Accuracy)) + \Time_{\inference}),
% $$

\mypara{Delay}
For Glimpse, we assume it only needs to encode the last captured frame, \ie $\Time_{\camera}=\frac{1}{30}$. This will make Glimpse strictly better since Glimpse needs to perform tracking on the camera.
As for Vigil and the pure camera approach, we say $\Time_{\camera}=\frac{1}{11.5}$~\cite{jetson-inference-speed}.
For the pure server approach and \name, they have to buffer enough frames to fill in the video chunk. Thus, 
$
\Time_{\camera} = \frac{14}{2\times 30}.
$
As for the factor $\Workload$, we empirically found that $\Workload\approx 0.16$ for both Vigil and Glimpse. Trivially, $\Workload = 0$ for the pure camera approach and $\Workload=1$ for the pure server approach.
Since the camera is wired with unlimited bandwidth, the streaming delay is negligible. Hence we say 
$
\Time_{\network} = 0.
$
Since the server could work at 10 FPS, the server-side time for all methods is $\Time_{\inference}=0.1$.
Based on these information and our experimental results, we plot the delay v.s. accuracy in \ref{fig:suboptimal-delay-acc}. 


From Figure \ref{fig:suboptimal-cost-delay-acc}, we see that Vigil is the best choice under this scenario. \kt{The pure camera approach suffers low accuracy as it could only afford a cheap model, which would miss objects (as illustrated in Figure \ref{fig:contrast-model}).} 


Further, to for the same DNN model, we assume similar camera hardware (\jc{Kuntai, the camera specs}) and server hardware (\jc{Kuntai, the server specs here}).

and a solution $\Pipeline$, we denote accuracy by 
$\Accuracy(\Local_{\Pipeline},\Remote_{\Pipeline},\Workload_{\Pipeline})$, whose inputs are the camera-side model $\Local_{\Pipeline}$, the server-side model $\Remote_{\Pipeline}$, and data (\eg encoded videos) sent to the server $\Workload_{\Pipeline}$.
The total cost and the response delay can be respectively decomposed to three parts (camera, network, and server):
\begin{align*}
\Cost_{\Setting,\Pipeline}&=\Cost^{\camera}_{\Setting}(\Local_{\Pipeline})+\Cost^{\network}_{\Setting}(\Workload_{\Pipeline})+\Cost^{\inference}_{\Setting}(\Remote_{\Pipeline},\Workload_{\Pipeline})\\
%\\
%&=\Cost_{\camera}^{\Setting,\Pipeline}(\Accuracy)+\Cost_{\network}^{\Setting}(\Size^{\Pipeline}(\Accuracy))+\Cost_{\inference}^{\Setting}(\Workload^{\Pipeline}(\Accuracy))
\Time_{\Setting,\Pipeline}&=\Time^{\camera}_{\Setting}(\Local_{\Pipeline})+\Workload_{\Pipeline}(\Time^{\network}_{\Setting}+\Time^{\inference}_{\Setting}(\Remote_{\Pipeline}))
\end{align*}
where $\Cost_{\camera}^{\Setting}$, $\Cost_{\network}^{\Setting}$ and $\Cost_{\inference}^{\Setting}$  ($\Time_{\camera}^{\Setting}$, $\Time_{\network}^{\Setting}$, and $\Time_{\inference}$) are the costs (delays) of the camera, the network, and the server, respectively.





Moreover, since they are designed with different target metrics and under different deployment settings (\eg resource availability of cameras, network, and servers), we assume the same camera hardware (\jc{Kuntai, the camera specs}) and server hardware (\jc{Kuntai, the server specs here})




We measure the total cost (and response delay) by the average cost (and delay) to process, stream and analyze each frame.

\begin{align*}
\Cost_{\Setting,\Pipeline}(\Video)&=\Cost^{\camera}_{\Setting,\Pipeline}(\Accuracy)+\Cost^{\network}_{\Setting,\Pipeline}(\Accuracy)+\Cost^{\inference}_{\Setting,\Pipeline}(\Accuracy)\\
%\\
%&=\Cost_{\camera}^{\Setting,\Pipeline}(\Accuracy)+\Cost_{\network}^{\Setting}(\Size^{\Pipeline}(\Accuracy))+\Cost_{\inference}^{\Setting}(\Workload^{\Pipeline}(\Accuracy))
\Time_{\Setting,\Pipeline}(\Accuracy)&=\Time^{\camera}_{\Setting,\Pipeline}(\Accuracy)+\Workload_{\Pipeline}(\Accuracy)\cdot(\Time^{\network}_{\Setting,\Pipeline}(\Accuracy)+\Time^{\inference}_{\Setting,\Pipeline}(\Accuracy))
\end{align*}
where $\Workload_{\Pipeline}(\Accuracy)$ is the fraction of frames analyzed by the server-side DNN to achieve accuracy $\Accuracy$.
%$$\Cost_{\network}^{\Setting}(\Size^{\Pipeline}(\Accuracy))+\Cost_{\inference}^{\Setting}(\Workload^{\Pipeline}(\Accuracy))$$
%$$\Time^{\Setting,\Pipeline}(a)=\Time_{\camera}^{\Setting}(\Model^{\Pipeline}(\Accuracy)) + \Workload^{\Pipeline} \cdot (\Time_{\network}^{\Setting}(\Size^{\Pipeline}(\Accuracy)) + \Time_{\inference})$$
%where $Model^{\Pipeline}(\Accuracy)$, $Size^{\Pipeline}(\Accuracy)$ and $Workload^{\Pipeline}(\Accuracy)$ denote the client-side logic, network traffic, and the fraction of frames analyzed by the server-side DNN to achieve accuracy $\Accuracy$.
%And $\Cost_{\camera}^{\Setting}$ ($\Time_{\camera}^{\Setting}$), $\Cost_{\network}^{\Setting}$ ($\Time_{\network}^{\Setting}$) and $\Cost_{\inference}^{\Setting}$ ($\Time_{\inference}$) are the costs (delays) of the camera, the network, and the server, respectively.


%$$\Cost^{\Setting,\Pipeline}(a)=\Cost_{\camera}^{\Setting}(\Model^{\Pipeline}(\Accuracy))+\Cost_{\network}^{\Setting}(\Size^{\Pipeline}(\Accuracy))+\Cost_{\inference}^{\Setting}(\Workload^{\Pipeline}(\Accuracy))$$
%$$\Time^{\Setting,\Pipeline}(a)=\Time_{\camera}^{\Setting}(\Model^{\Pipeline}(\Accuracy)) + \Workload^{\Pipeline} \cdot (\Time_{\network}^{\Setting}(\Size^{\Pipeline}(\Accuracy)) + \Time_{\inference})$$
%where $Model^{\Pipeline}(\Accuracy)$, $Size^{\Pipeline}(\Accuracy)$ and $Workload^{\Pipeline}(\Accuracy)$ denote the client-side logic, network traffic, and the fraction of frames analyzed by the server-side DNN to achieve accuracy $\Accuracy$.
%And $\Cost_{\camera}^{\Setting}$ ($\Time_{\camera}^{\Setting}$), $\Cost_{\network}^{\Setting}$ ($\Time_{\network}^{\Setting}$) and $\Cost_{\inference}^{\Setting}$ ($\Time_{\inference}$) are the costs (delays) of the camera, the network, and the server, respectively.
\jc{all the caveats!, video dependent}

It is evident that when there is no constraint on the total cost, the ideal solution is to put as much compute power on the camera (an expensive camera) to achieve high accuracy and low process delay.
In the ensuing discussion, we seek to minimize the cost while achieving accuracy target of 0.8 and response delay less than 1.5 seconds, and compare existing solutions (and ours which will be introduced in the next section) 
under two concrete deployment settings. 
For a fair comparison, we compare these solutions under the same settings of task and DNN models: 
(details will be explained in \S\ref{subsec:eval-method}: object detection as the task, SSD-MobileNet-v2 as the camera-local DNN model (if a solution needs a local model (\eg Vigil), the FasterRCNN-ResNet101 as the server-side model.
Moreover, since they are designed with different target metrics and under different deployment settings (\eg resource availability of cameras, network, and servers), we assume the same camera hardware (\jc{Kuntai, the camera specs}) and server hardware (\jc{Kuntai, the server specs here})





\cameraold{
\begin{figure}
\centering
\includegraphics[width=0.65\columnwidth]{figs/det_demonstrate_tradeoff.pdf}
\tightcaption{Current solutions exhibit a rigid bandwidth-accuracy tradeoff: any gain in accuracy comes at a cost in bandwidth.
The results are based on the traffic videos in our dataset %\kt{do we need to add cloudseg in this graph?} 
(\S\ref{subsec:eval-method}).}
\label{fig:motivation-tradeoff}
\end{figure}
}



\begin{comment}

\mypara{Existing solutions} 
The question then is how to fully explore the potential room for improvement?
Existing solutions for video streaming are essentially {\em source-driven}---the decisions of how the video should be compressed or pruned are made at the source with no real-time feedback from the server-side DNN that analyzes the video.
These solutions fall in two categories:
\begin{packeditemize}
\item {\em Camera-side heuristics:}
A camera can run various local heuristics (\eg checking significant inter-frame difference~\cite{glimpse}, a cheap vision model~\cite{adascale,nn-meets-pn,vigil,noscope}), or some DNN layers~\cite{cracking,ddnn} to identify regions/frames that contain information (\eg queried objects) critical to the server-side analytics engine and send only these frames/regions to save bandwidth.
Camera-side heuristics essentially trade camera-side compute power to run inference for better accuracy/bandwidth tradeoffs~\cite{cracking}.
% For instance, Glimpse~\cite{glimpse} uses pixel changes to identify and send only frames in which queried objects are likely to emerge; and Vigil~\cite{vigil} identifies frames with most detected objects and sends only the object regions in those frames.
% Similar ideas can also be found in other video pipelines (\eg~\cite{noscope,fvc}) that are designed to save computation cost.
% uses a cheap inference model to discard frames that do not require complex DNN inference. 
% \jc{explain edge accelerator and/or noscope in more details if we end up using it as a baseline too, for e.g., Edge-based accelerators, such as EdgeTPUs or GPUs, speed up AI processing at the camera using better hardware albeit at higher cost while the model accuracy still does not match the server-side models.}

\item {\em Adaptive video streaming:} 
One can also to revamp existing video streaming protocol and adapt the quality level to maximize inference accuracy under the bandwidth constraint.
For instance, AWStream~\cite{awstream} is built on DASH/H.264 and periodically re-profiles the relationship between quality levels and inference accuracy, in order to select a lower-than-throughput quality level with maximum inference accuracy. 
CloudSeg~\cite{cloudseg} sends a video at low quality but upsizes the video by super resolution on the server side.
% Similar ideas can be found in other work~\cite{cloudseg,adascale}.
% image resolution and other encoding knobs should be tuned to improve accuracy, rather than visual quality. 

% \kt{cloudseg? It does not fall into two folders above.}
\end{packeditemize}



\mypara{Limitations of source-driven approach}
The premise of these techniques is that the camera-side logic can identify what is needed by the server-side analytics engine, thus achieving high accuracy with low bandwidth.
In reality, however, their bandwidth/accuracy tradeoffs (illustrated in Figure~\ref{fig:motivation-tradeoff}) can be quite rigid: any gain of accuracy comes at the cost of considerable more bandwidth usage.
% One can see that the tradeoffs are rigid---higher accuracy can only be achieved at the cost of greatly increased bandwidth usage.
The intuition is that any heuristic that fits camera's limited compute capacity is unlikely to precisely imitate a much more complex DNN, with no real-time feedback from it.
% (After all, if cameras can run a sufficiently complex logic that imitates the server-side DNN, there would be not need to send videos to the server in the first place.)
For instance, Glimpse~\cite{glimpse} and NoScope~\cite{noscope} rely on the inter-frame differences to signal which frames contain objects, but any false positives (\eg pixel changes on the background) will cost unnecessary bandwidth usage and any false negatives (\eg small objects) will preclude the server from detecting important information. 
On the other hand, analytics-aware streaming \kt{illustrate that these type of methods treats each objects uniformly, which essentially pays too much bw on high-confident (mostly large) objs and too little bw on low-confident (mostly small) objs? The following reason cannot explain why DDS still have performance gain even when the video is completely static, though it is still valid.} (\eg~\cite{awstream}) relies on accurate relationship between video quality and inference accuracy.
% that must be profiled constantly as the video content varies.
Such relationship is inherently dynamic: when the video content contains large objects (\eg a car passing closely in front of a camera), a low-resolution video still yields high accuracy, but when the video contains mostly tiny objects (\eg a car driving away from a camera), low resolution will not suffice.
Thus, frequent profiling is needed anytime the video changes its characteristics.

\end{comment}



\cameranew{

\begin{figure}[t]
\centering
    \subfloat[SSD inception v2]
    {
        \includegraphics[width=0.4\columnwidth]{figs/ssd_inception_v2_crop.jpg}
        \label{subfig:1}
    }
    \subfloat[Faster rcnn resnet101]
    {   
        \includegraphics[width=0.4\columnwidth]{figs/faster_rcnn_resnet101_crop.jpg}
        \label{subfig:2}
    }
\tightcaption{Contrasting the inference results between cheap model (SSD-inception-v2) and heavy model (Faster-rcnn-resnet101) on the same image. Heavy model is much more accurate when the video content is challenging.
%\jc{update these figures?}
% \jc{this figure is a bit weird. why the small model (the left one) cannot detect large objects but can detect smaller ones?}
% \kt{The object size are nearly the same except for the one that lies in the middle of the road.}
}
\label{fig:contrast-model}
\end{figure}


}

\cameranew{
\tightsubsection{Tradeoffs among accuracy, cost and delay}
\label{subsec:cost-accuracy-delay}

Before diving to our design, we provide a framework to understand the performance---in costs, response delay, and accuracy---of existing solutions and our technique. 
% We will use the same framework to put the performance of our solution into perspective too.
An additional benefit of a performance framework like this is to provide performance clarity among current solutions which are often designed for different performance objectives (\eg minimize cost under given accuracy and delay constraints) and with different assumptions of the deployment settings (\eg resource availability of cameras, network, and servers).
The performance framework allows fair comparison among these solutions (and future ones) along the same metrics and in the same deployment settings. 
Although the exact performance of a solution can vary greatly in practice with factors such as the exact video content and choice of camera/server software, the framework focuses on primary factors that influence the performance of various solutions differently (while making identical assumptions about the accuracy and the latency of server-side DNN that affect all solutions) and is useful to qualitatively identify the ``operating regime'' of each solution (when one solution strikes a better performance tradeoffs than others).
We will illustrate the comparisons among these solutions using three concrete performance objectives and deployment settings.


% \kt{State that we could achive accuracy 1 if we stream the video in ultra-high quality from the camera to the server and inference on the server.}

% It is not enough to know that there is a potential new room for us to improve.
% Leveraging that room or not itself is a design choice.
% Every design choices will have the scenario where it is valid, and where it is likely to be sub-optimal. 
% However, the analysis that previous works provided are not able to inform people whether their approach works or not under {\bf a new scenario} that they did not talk about.


% Since it is relatively difficult to model inference accuracy, we instead study the cost model and delay model given the accuracy target $acc$ and the video analytic pipeline (VAP for short).
For each solution $\Pipeline$, a deployment setting $\Setting$ and a desirable accuracy target $\Accuracy$ \kt{(relative to the inference results at the server under unlimited bandwidth)}, we can estimate the cost and the response delay as follows:

\mypara{Cost model} 
We measure the cost by the cost to process, stream and analyze each frame from one camera, at a fixed frame rate of $30$ frames per second (FPS) and, for chunk-based streaming methods~\cite{awstream}, we use video chunk size of $15$ frames. % if the VAP chops the video to video chunks. 
As defined in \S\ref{subsec:dva}, the total costs are comprised of three parts: 
$$\Cost_{\camera}^{\Setting}(\Model^{\Pipeline}(\Accuracy))+\Cost_{\network}^{\Setting}(\Size^{\Pipeline}(\Accuracy))+\Cost_{\inference}^{\Setting}(\Workload^{\Pipeline}(\Accuracy))$$
where $Model^{\Pipeline}(\Accuracy)$, $Size^{\Pipeline}(\Accuracy)$ and $Workload^{\Pipeline}(\Accuracy)$ denote the client-side logic, network traffic, and the server-side workload (in fraction of frames analyzed by the server-side DNN) needed by $\Pipeline$ to achieve accuracy $\Accuracy$.
And $\Cost_{\camera}^{\Setting}(\cdot)$, $\Cost_{\network}^{\Setting}(\cdot)$ and $\Cost_{\inference}^{\Setting}(\cdot)$ are 
the camera cost, the network cost, and the server cost, respectively. 
Note that this model assumes each cost component depends only on one factor (\eg the server cost depends only on the fraction of frames to be analyzed by the server-side DNN). 
But this may ignore minor factors; \eg the server cost may also include that of periodic profiling of configurations~\cite{awstream}, though that only applies to particular solutions.

\mypara{Response delay model}
We measure the average response delay by the average delay spent to locally process (including buffering, encoding and possibly analyzing), stream and analyze (server-side inference and decoding) each frame. 
Optionally, the server-side inference results need to be given to the analyst but this delay would contribute equally to all solutions' response delay.
% We also fix the same frame rate and same chunk size as stated above. 
Thus, the average response delay could be represented as
% & t_{avg}^{VAP} && = t_{buf}^{VAP}+t_{cam}^{VAP} 
% + (1-\%cam)\cdot(t_{stream}+t_{serv}+t_{latency}),\\
% & t_{wst}^{VAP} && = t_{cam}^{VAP}+
% [\%cam<1]\cdot(t_{buf}^{VAP}+t_{stream}+t_{serv}),
$$
\Time_{\camera}^{\Setting}(\Model^{\Pipeline}(\Accuracy)) + \Workload^{\Pipeline} \cdot (\Time_{\network}^{\Setting}(\Size^{\Pipeline}(\Accuracy)) + \Time_{\inference}),
$$
where $\Time_{\camera}^{\Setting}(\cdot)$,
$\Time_{\network}^{\Setting}(\cdot)$ and
$\Time_{\inference}$ 
denote the average delay for the camera to locally process a frame, the streaming delay to send the video to the server, the server-side processing delay, respectively.
% Note that we assume that the decoding time at the server is nearly negligible (thanks to NVDEC~\cite{nvdec}).
% Note that this model only works on previous solutions. We will present the average response delay of \name at \S\ref{sec:overview}.

The aforementioned estimation of cost and response delay applies directly to existing solutions that stream each frame at most once, and it can later be extended to analyze the performance of our proposed solution that potentially streams a frame for multiple times.

% Our camera-side cost model is:
% $$
% \frac{cost_{cam}^{VAP}(acc)}{\#frames},
% $$
% where $VAP$ denotes the corresponding VAP, $cost_{cam}^{VAP}$ denotes the purchase cost at the camera side, which is a function of the accuracy target $acc$, and $\#frames$ denotes the number of frames streamed from one camera to the server.
% Our bandwidth cost model is:
% $$
% cost_{net}^{mode_{net}}(size^{VAP}(acc)),
% $$
% % Note that we need r_{\name} in delay calculation.
% where $cost_{net}^{mode_{net}}$ is the billing function for bandwidth, which differs with respect to different billing mode $mode_{net}$, and $size^{VAP}(acc)$ is the minimum average size of a single frame in order to hit accuracy target $acc$. Our server cost model is:
% $$
% cost_{serv}^{mode_{serv}}(\%cam, \#infs^{VAP}),
% $$
% where $cost_{serv}$ is the cost at server side dependng on the server-side billing mode $mode_{serv}$, which is a function of the percentage of camera-processed-only frames $\%cam$, and the number of DNN inference per frame $\#infs_{VAP}$.

% \mypara{Delay model} Note that we measure all the delay in seconds. 
% The first part of the delay is the time for the camera to buffer enough frames  $t_{buf}^{VAP}$ to construct a video chunk before sent. For those VAPs that chop videos to video chunks, 
% in the average case, $t_{buf}^{VAP} = \frac{15-1}{2\times30}\approx 0.23$ and in the worst case, 
% $t_{buf}^{VAP}=\frac{15-1}{30}\approx 0.47$. Otherwise, 
% $t_{buf}^{VAP}=0$
% The second part is the time for camera to do post-processing on the last frame of the video chunk (this is because previous frames are already post-processed while waiting for the corresponding next frame). 
% We denote this time as $t_{cam}^{VAP}$. 
% The third part is the streaming delay, we denote this time as $t_{stream}$.
% The fourth part of the delay is the time for the DNN to perform inference. This delay is equal to one-time inference on the DNN since the server could inference on multiple frames in parallel.
% The fifth part of the delay is the time for the server to transmit the results back to the camera. We call it $t_{latency}$ since it only depends on the network latency.
% Thus, for all VAPs except for \name, we write:
% \begin{alignat*}{2}
% & t_{avg}^{VAP} && = t_{buf}^{VAP}+t_{cam}^{VAP} 
% + (1-\%cam)\cdot(t_{stream}+t_{serv}+t_{latency}),\\
% & t_{wst}^{VAP} && = t_{cam}^{VAP}+
% [\%cam<1]\cdot(t_{buf}^{VAP}+t_{stream}+t_{serv}),
% \end{alignat*}
% where
% $[\%cam<1]$ means the truth value of proposition $\%cam<1$ and $t_{avg}^{VAP}$, $t_{wst}^{VAP}$ are the average delay and worst-time delay correspondingly.
% We will present the delay model for \name in  \S\ref{sec:overview}.




}
% \tightsubsection{Limitations of current solutions}
% \label{subsec:limitation}


% So this approach is suboptimal, unless one can update the profile anytime there is a sudden change in content.

% In adaptive encoding, for instance, maintaining the relationship between quality levels and accuracy (as in~\cite{awstream}) can help, but this relationship will be obsolete whenever the video content varies:
% when the video content contains a large object (\eg a car passing through a camera), compressing the whole video with a low resolution will still yield high accuracy, but when the video content is a tiny object (\eg a car driving away from the camera), low resolution will not suffice.
% So this approach is suboptimal, unless one can update the profile anytime there is a sudden change in content.

% We argue that prior source-driven approaches have fundamental limitations due to the fact that they must make critical decisions that affect bandwidth/accuracy tradeoffs locally, with no real-time feedback from the analytics engine.
% The key reason behind the rigid tradeoff is that these solutions hope some simple heuristic that fits the camera's compute capacity can determine what the much more complex server-side DNN need to maintain high inference accuracy.
% After all, if the camera can run a sufficiently complex heuristic that imitates the server-side DNN, there would be not need to send videos to the server for more compute-intensive inference. 

% \mypara{Suboptimal performance}
% To put their performance into perspective, we consider an idealized solution, called {\em oracle}. 
% It sends out only regions around ground truth objects in the highest quality. 
% Since the oracle scheme uses hindsight information, its performance is not realistic. Nevertheless, it shows the potential bandwidth saving when achieving a high accuracy.
% Figure~\ref{fig:motivation-tradeoff} shows that the three schemes need \fillme-\fillme\% more bandwidth than the oracle to achieve the same accuracy. 
% We observe the same performance gap between them and the oracle on other videos, too. 
% Why does their performance fall so far behind the potential of machine-centric video streaming? 

% assumption made by these solutions that there exists some simple heuristic that fits the camera's compute capacity and can determine how the video should be compressed/streamed to maintain high inference accuracy.

%To get performance similar to ``oracle'', such hypothetical camera-side heuristic essentially needs to know when and where the objects of interest appear in the video.
% \mypara{Understanding the performance gap}

% Although prior work has considered various heuristics (a look-up table~\cite{awstream}, threshold on inter-frame difference~\cite{glimpse}, or a shallow neural-network model~\cite{adascale,nn-meets-pn,vigil,noscope}), none of them seems sufficient.
% In camera-side filtering, for instance, if one uses the pixel-level difference to determine which frame contains objects and send these frames~\cite{glimpse}, any false positives of this heuristics can cause unnecessary bandwidth consumption and any false negatives will prevent the powerful server-side network from having a chance to detect the object.
% In adaptive encoding, for instance, maintaining the relationship between quality levels and accuracy (as in~\cite{awstream}) can help, but this relationship will be obsolete whenever the video content varies:
% when the video content contains a large object (\eg a car passing through a camera), compressing the whole video with a low resolution will still yield high accuracy, but when the video content is a tiny object (\eg a car driving away from the camera), low resolution will not suffice.
% So this approach is suboptimal, unless one can update the profile anytime there is a sudden change in content.


%may render the relationship obsolete.\footnote{AWStream will update relationship periodically~\cite{awstream}, but as we will see in \S\ref{??}, it is challenging to update this profile frequently enough without excessive use of bandwidth.}
%Similar, a simple heuristic (\eg a shallow neural net) is unlikely to work, since it is less accurate than the server-side DNN.
%For instance, if one uses the heuristics to determine which frame contains objects and send these frames, any false positives can cause unnecessary bandwidth consumption, and any false negatives from the simple, camera-side network will prevent the powerful server-side network from having a chance to detect the object. 


%In short, the limitation of the heuristic-based approach is that any camera-side heuristic is incapable of making optimal adaptation decisions without knowing how the server-side DNN would react to the current video content. 
%After all, if the camera can run a sufficiently complex heuristic that imitates the server-side DNN, there would be not need to send videos to the server for more compute-intensive inference. 

%Moreover, some camera-side heuristics also need to be updated whenever the server-side DNN changes, which may lead to 


%\begin{itemize}
%    \item ideally driven by {\em real-time content of interest}, which is time varying and dnn-dependent
%    \item a taxonomy of existing techniques (changing codec is an option though not practical)
%    \begin{itemize}
%        \item client-side filtering
%        \item adaptive encoding
%    \end{itemize}
%    \item empirically compare accuracy of the prior approaches (glimpse, noscope, awstream) with the oracle
%    \item discussion:
%    \begin{itemize}
%        \item client-side filtering: not dnn/task dependent
%        \item adaptive encoding: not real-time content-dependent
%    \end{itemize}
%\end{itemize}



\cameranew{

\mypara{Example scenario 1 (response-delay-dominant)} 
Let us start with a simple setting where the performance objective is to minimize the response delay while preserving high accuracy (\eg FPS gaming through AR) without a cost budget, and any server has a high network latency with the camera.
In this case, the best solution would be having camera equipped with a high-end GPU to analyze each frame locally.
Any solution that sends frames to a remote server will suffer from network latency.
% all video streaming approaches need to go through the network and are affected by network latency. 
% To avoid this latency, we could put a high-end GPU at the camera side to inference right after the frame has been captured. Thus, in this scenario, it is the best to process all the frames at the camera.

\jc{need to mention figure 5}

The next two scenarios use the same performance objective---minimizing the cost while achieving accuracy over 0.8 and response delay less than 1.5 seconds---but have different deployment settings.

\mypara{Example scenario 2 (server-side-cost-dominant)} 
We assume the deployment setting in this scenario is that the camera is connected to the server with a wired network with unlimited bandwidth and negligible network latency and the cloud server rented for a year (\ie in total $10^9$ frames) 
% (if longer, the renting cost will be higher than directly buying the GPUs) 
% and optimize the cost with accuracy target $0.8$ and average delay target $1$ seconds. Running wired traffic camera through cloud server is a concrete example. 

% $$\Cost_{cam}^{\Setting}(\Model^{\Pipeline}(\Accuracy))+\Cost_{net}^{\Setting}(\Size^{\Pipeline}(\Accuracy))+\Cost_{srv}^{\Setting}(\Workload^{\Pipeline}(\Accuracy))$$



\mypara{Cost} As for the camera-side cost, from \cite{wired-camera-cost}, we know that a wired camera is about 150\$. We let all VAPs use this camera (this will make the cost of Glimpse strictly smaller) except for Vigil. For Vigil, to support 30fps inference on Mobilenet-inception-v2, we need at least 3 NVIDIA Jetson TX2 \cite{jetson-inference-speed} while each of them cost 490\$\cite{jetson-price}. Thus, we write:
$\Cost_{cam}=3\times 490\times 10^{-9}$ for Vigil and
$\Cost_{cam}=150\times 10^{-9}$ for other solutions.
As for the network cost, since the camera is wired, the bandwidth cost is a one-time cost that are the same fr all VAPs and could be amortized through time. Thus, we write $\Cost_{\network}= 0$ for all solutions.
%$Renting one NVIDIA GTX 1080 would be about 71.8\$ per month %$\cite{rent-gtx1080-price}. 
%The detection model faster-rcnn-resnet101 will run in 106ms on NVIDIA GTX Titan X. Based on the FLOPs listed in \cite{gpu-flops-comparision}, we infer that a NVIDIA GTX 1080 could run faster-rcnn-resnet101 at about 7.5 fps.
As for the server-side cost, from \cite{google-gpu-pricing}, we know that one NVIDIA Tesla K80 GPU will be $206.590\$$ per month.
Based on \cite{titanX, model-zoo,k80}, we infer that a NVIDIA Tesla K80 GPU could support about 10 fps inference on FasterRCNN-ResNet101.
Thus, to achieve 1 inference per frame, we need about 7437\$ per year.
Based on this, we write:
$
\Cost_{srv} = \Workload^{\Pipeline}\times 7437\times 10^{-9}
$
According to the information above and based on our experimental results, we plot the cost v.s. accuracy of pure server (AWStream will be strictly worse due to profiling cost at server-side), Vigil, Glimpse, pure camera and \name in Figure \ref{fig:suboptimal-cost-acc}.

% $$
% \Time_{\buffer}^{\Pipeline} + \Time_{\process}^\Pipeline + \Ratio^{\Pipeline} \cdot (\Time_{\network}^{\Setting}(\Size^{\Pipeline}(\Accuracy)) + \Time_{\inference}+\Time_{\latency}^{\Pipeline}),
% $$

% $$
% \Time_{\camera}^{\Setting}(\Model^{\Pipeline}(\Accuracy)) + \Workload^{\Pipeline} \cdot (\Time_{\network}^{\Setting}(\Size^{\Pipeline}(\Accuracy)) + \Time_{\inference}),
% $$

\mypara{Delay}
For Glimpse, we assume it only needs to encode the last captured frame, \ie $\Time_{\camera}=\frac{1}{30}$. This will make Glimpse strictly better since Glimpse needs to perform tracking on the camera.
As for Vigil and the pure camera approach, we say $\Time_{\camera}=\frac{1}{11.5}$~\cite{jetson-inference-speed}.
For the pure server approach and \name, they have to buffer enough frames to fill in the video chunk. Thus, 
$
\Time_{\camera} = \frac{14}{2\times 30}.
$
As for the factor $\Workload$, we empirically found that $\Workload\approx 0.16$ for both Vigil and Glimpse. Trivially, $\Workload = 0$ for the pure camera approach and $\Workload=1$ for the pure server approach.
Since the camera is wired with unlimited bandwidth, the streaming delay is negligible. Hence we say 
$
\Time_{\network} = 0.
$
Since the server could work at 10 FPS, the server-side time for all methods is $\Time_{\inference}=0.1$.
Based on these information and our experimental results, we plot the delay v.s. accuracy in \ref{fig:suboptimal-delay-acc}. 


From Figure \ref{fig:suboptimal-cost-delay-acc}, we see that Vigil is the best choice under this scenario. \kt{The pure camera approach suffers low accuracy as it could only afford a cheap model, which would miss objects (as illustrated in Figure \ref{fig:contrast-model}).} 

\mypara{Example scenario 3 (network-cost-dominant)} Now we assume that we stream from a lot of 4G-connected cameras to a personal cluster for a year (i.e. about $10^9$ frames).

\mypara{Cost} As for the camera-side cost, a LTE-conected camera is about 216\$~\cite{camera-price}. This camera is enough for all pipelines except for Vigil. For Vigil, we still use the same way stated in the last scenario to calculate its camera cost. Thus,
$\Cost_{cam}=3\times 490\times 10^{-9}$ for Vigil and
$\Cost_{cam}=216\times 10^{-9}$ for other solutions.
As for the cost on the network, An AT\&T unlimited family plan would be \$35 per month~\cite{4G-plan} for a 13Mbps uploading speed~\cite{upload-speed} on a single camera. Thus, streaming with an average speed of 1Mbps per year will cost about \$32. Accordingly, we write:
$
\Cost_{\network}=30\times\times \Size^{\Pipeline}(\Accuracy)\times 32\times 10^{-9}
$
The $30$ here is the frame rate.
As for the server-side cost, the per-camera per-frame server-side cost could be amortized over time. Hence we write:
$
\Cost_{\inference}=0
$
for all solutions.
According to the information above and based on our experimental results, we plot the cost v.s. accuracy of pure server (AWStream will have strictly higher cost due to profiling), Vigil, Glimpse, pure camera and \name in Figure \ref{fig:cost-acc}.

\mypara{Delay}
The $\Time_{\camera}$, $\Workload$ and $\Time_{\inference}$ are exactly the same as in example scenario 2. As for the network time, we let three camera share the 13Mbps upload bandwidth (except for the pure server approach to ensure the bandwidth is sufficient for real-time purpose) and calculate the streaming time by the frame/chunk size divided by the bandwidth.  Based on these information and our experimental results, we plot the delay v.s. accuracy in \ref{fig:delay-acc}.

% For Glimpse, we assume it only needs to encode the captured frame, \ie $\Time_{\camera}=\frac{1}{30}$. This will make Glimpse strictly better since Glimpse requires tracking.
% As for Vigil and the pure camera approach, we say $\Time_{\camera}=\frac{1}{11.5}$~\cite{jetson-inference-speed}.
% For the pure server approach and \name, they have to buffer 15 frames and encode them before sent. Thus, 
% $
% \Time_{\camera} = \frac{16}{2\times 30}.
% $

% We know that $t_{cam}^{VAP}=\frac{1}{40}$ for those VAP which only encodes at the camera (it has sufficient compute to encode at 40FPS in 720p). We also use this value for Glimpse. For Vigil, $t_{cam}^{VAP}=\frac{1}{11.5}$~\cite{jetson-inference-speed}. 
% We let three camera share the 13Mbps upload bandwidth (except for the pure server approach) to achieve real time and calculate the streaming time. The server could run Faster-rcnn-resnet101 (which is what we use) in about 0.1s~\cite{model-zoo}. So $t_{serv}=0.1$ (we assume that the server is able to decode the video much more faster than inference on each frame). The latency for 4G network is about 0.05s~\cite{4G-latency}. As for \name, the encoding time $t_{enc}$ (will be introduced in \S\ref{sec:overview}) is about $\frac{15}{40}$ seconds. Based on these information and our experimental results, we plot the delay v.s. accuracy in \ref{fig:delay-acc}.

From Figure \ref{fig:cost-delay-acc}, we see that \name is the best choice under this scenario.


}

}

==> motivation_v4.tex <==





\section{Background}




\vspace{0.2cm}

\tightsubsection{DNN-based streaming media analytics}
\label{subsec:streaming-analytics}



DNN-based analytics applications are ubiquitous~\cite{tusimple,waymo,trafficvision, traffictechnologytoday,goodvision,intuvisiontech, vision-zero, msr,servai-1,servai-2,servai-3}.
\hl{
In this paper, we focus on streaming media analytics, where the analytic tasks are performed on various types of streaming media (\eg RGB video, LiDAR video, depth video, InfraRed video and audio) to perform classification, detection or segmentation tasks. 
Streaming media analytics are widely used in applications like autonomous driving (which require running object detection on RGB and LiDAR video), human detection (which require human detection using InfraRed video for detection accuracy at night) and smart home (which require word detection on audio data)}
\jc{the definition of ``streaming media analytics'' is still unclear. maybe say each application of ``streaming media analytics'' is defined by the type of streaming media and the task of analytics. and streaming media can be one of xxx types, and the task of analytics can be one of xxx tasks.}
\jc{also worth mentioning that streaming media analytics includes video analytics}
\jc{can you update table 2 soon to reflect the new definitions?}
% We pick these tasks not only because they are critical to real-world applications, but also because they take as input various types of data streams, \eg RGB videos, LiDAR videos and audio waves (see Table~\ref{tab:applications}).
% vehicle detection for autonomous driving, voice recognition for smart home and human detection for home security, all of which analyze data streams (\eg video frames or point cloud) collected from sensors to extract information (\eg detect bounding boxes of objects of interest).
% with various types of sensors.
% \kt{Maybe call it input preparation sounds better. Input processing sounds like irrelavent to data streaming}

\hl{A typical architecture of streaming media analytic system contains two components: input filtering (typically at the sensor side) and DNN inference (typically in edge or cloud).
Figure~\ref{fig:dnn-analytics-application-flow} depicts a typical architecture of streaming media analytics. }
First, they collect and process data (typically at the sensor side) to the DNN input. 
We denote the sensed raw data as \textit{input data}.
Then, the DNN input may need to be streamed to an analytics server (in edge or cloud) through a {\em bandwidth-constraint} link when there is no sufficient compute for DNN inference at the sensor side, so not all data frames (\eg video frame) in their highest fidelity will be collected.
Then, the server runs DNN inference to get
% They collect data from sensors, prepare the input for the DNN (which may require network-based data streaming), perform DNN inference, and obtain 
inference results (\eg vehicle bounding boxes for autonomous driving) using \textit{limited} GPU resources.
% We assume that the inference results are a collection of elements (\eg object bounding boxes in object detection, classification labels in classification, pixel labels in semantic segmentation), where each element is associated with a corresponding confidence score. Only those elements with a confidence score higher than a confidence threshold will be counted when calculating accuracy.
% This assumption does not hold for all DNN-based applications (\eg this assumption does not hold in a generative task like image generation, as it only generates the pixel values for each pixel, but does not associate confidence scores to those pixels).
% However, this assumption covers a wide range of applications, like video analytic tasks (\eg object detection, semantic segmentation, classification) and audio-based tasks (\eg audio-to-text).




\begin{figure}
    \centering
    \includegraphics[width=0.9\columnwidth]{figs/multiapp.pdf}
    \tightcaption{
    In DNN-based analytics applications, various types of source data collected from sensors are processed by an input processing module to generate DNN input. 
    The DNN is then run on the input to get inference output.
    % analytic results based on DNN input using constrained GPU resources.
    Since the DNN inference module may be located on a remote edge device or cloud server, the input processing module may need to stream the data to the DNN through a bandwidth-constraint network.
    % As the DNN inference module may locate on a remote edge device/cloud server, the input processing module may need to connect to the DNN inference module through a {\em bandwidth-constraint} network. \kt{Junchen can you read this figure and see if it works?}
    }
    \label{fig:dnn-analytics-application-flow}
\end{figure}



% \begin{table}[t]
% \centering
% \footnotesize
%     \begin{tabular}{c c c}
%         \hline
%         Example application & Analytic task & Data sources\\
%         \hline
%         Autonomous driving & Vehicle detection & RGB video, LiDAR point cloud \\
%         Traffic monitoring & Vehicle segmentation & RGB video \\
%         Security monitoring & Human detection & RGB video, Infrared, Depth map \\
%         Smart home & Voice to text & Audio   \\
%         \hline
% \end{tabular}
% \tightcaption{Example applications of our solution.} 
% \label{tab:applications}
% \end{table}    






\mypara{Objective}
% In practice, however, a real system of these applications may not have enough {\em network bandwidth} to stream all uncompressed data from sensors to a remote more powerful server, and/or enough {\em GPU compute resource} to run expensive DNN inference on all input data (\eg all frames of a video stream). 
% This means that they may not have enough resources to stream uncompressed data out (if the sensor cannot run DNN-based analytics by itself) and perform inference on every part of the input data (\eg on every frame of the video). 
The objective for these DNN-based analytic systems is to improve \textit{inference accuracy} without increasing the resource usage (in terms of network bandwidth and GPU cycles), or reduce the resource usage without hurting the inference accuracy.
% under the average bandwidth and/or GPU computation budget.
Following prior work~\cite{awstream,chameleon,dds,accmpeg,ekya,yoda}, we define accuracy as the similarity between the inference results and the inference results generated under unlimited bandwidth and/or GPU computation budget (see \S\ref{subsec:eval-setup} for detailed definition).
This directly shows the impact of saving resource usage on inference accuracy. 
% \jc{update this with the objective table on the whiteboard}
% \kt{I guess we need to defend why average budget, let me think of an argument...}


% \kt{Defend the choice of streaming to server for anlaytics}


% \subsection{Taxonomy of configuration knobs}

\begin{table}[]
\footnotesize
\begin{tabular}{|l|l|l|}
\hline
\multicolumn{1}{|c|}{\textbf{}} & \multicolumn{1}{c|}{Spatial}    & \multicolumn{1}{c|}{Temporal} \\ \hline
Uniform filtering               & QP, resolution, crf             & frame rate                    \\ \hline
Nonuniform filtering            & QP of different spatial regions & frame difference thresholds   \\ \hline
\end{tabular}
\caption{\kt{expand this table with references}
\jc{can we re-org this table as follows: 
(1) four columns each representing a type of knob, e.g., Uniform filtering on pixels (i.e., QP, resolution, CRF). 
(2) multiple rows, each presenting a prior approach. and if an approach can handle one knob, there will be a check sign.
this way, the table will show that only OneAdapt and Profiling are able to deal with all types of knobs. }}
\label{tab:knob-categorization}
\end{table}


% \kt{Add a new subsection here to introduce the taxonomy of config knobs. The goal is to give people a background on existing knobs. See Table~\ref{tab:knob-categorization}.}

% We present a taxonomy of configuration knobs presented by existing streaming media analytic systems.

% First, there are some knobs that control the input data filtering process and some other knobs that control the DNN inference process.
% This paper focus on handling the input data filtering knobs.

% As for input data filtering knobs, we categorize them along two dimensions.
% The first dimension is whether the knob filters input data at spatial dimension (\eg video resolution) or time dimension (\eg video frame rate).
% The second dimension is whether the knob filters the input data uniformly (\eg video resolution) or non-uniformly (\eg the encoding quality of different spatial regions of the video).




% To better put prior work into perspective, we categorize knobs along two dimensions.
% The first dimension is whether the knob filters input data at time dimension (\eg video frame rate) or spatial dimensions (\eg video resolution).
% We call the former \textit{temporal knobs} and the latter \textit{spatial knobs} (note that currently there are no knobs presented by prior work that belongs to both).
% The second dimension is whether the knob filters input data uniformly (\eg video frame rate and video resolution) or non-uniformly
% The second dimension is whether the knob filters the data uniformly (\eg video frame rate, video resolution) or filters the data non-uniformly (\eg frame difference thresholds, the encoding quality of different spatial regions).


% \tightsubsection{Internel knobs of analytic systems}

% Prior work has shown that high accuracy {\em could} be obtained with significantly lower network and/or GPU usage if the internal parameters (hereinafter \textit{knobs}) of these DNN analytics pipelines are configured optimally.




\tightsubsection{Configuration adaptation}
\label{subsec:numer_of_knobs}



  




% expose internal tunable parameters (referred to as knobs) and
% timely configure these knobs (we denote the knobs together
% with their configured values as a configuration)

\kt{Mention DNN knobs here}
\hl{We observe that prior work optimizes the trade-off between accuracy and resource usage (GPU cycles or bandwidth usage) by adjusting there internal parameters (hereinafter \textit{knobs}).
To systematically introduce existing knobs appeared in prior work, we categorize knobs along two dimensions.
The first dimension is whether the knob filters input data at time dimension (\eg video frame rate) or spatial dimensions (\eg video resolution).
We call the former \textit{temporal knobs} and the latter \textit{spatial knobs}\footnote{Note that currently there are no knobs presented by prior work that belongs to both}.
The second dimension is whether the knob filters the data uniformly (\eg video frame rate, video resolution) or non-uniformly (\eg the encoding quality of different spatial regions). We put the knobs from prior work in Table~\ref{tab:knob-categorization} along these two dimensions.}


Prior work has shown that high accuracy {\em could} be obtained with significantly lower network and/or GPU usage if 
% the internal parameters (hereinafter \textit{knobs}) 
the knobs of these DNN analytics pipelines are configured optimally.
We denote the knobs together with their configured values as a configuration.
The {\em optimal} setting of configuration is the one that yields the highest accuracy with low resource usage in bandwidth and GPU cycles (this will be more rigorously defined in \S\ref{sec:eval}).
% For instance, consider 
When detecting vehicles in a traffic video, for instance, we can significantly reduce the frame sampling rate of data collection and DNN inference, if the vehicles are moving slowly (\eg at a red light), and the DNN can still accurately determine the position and movement of the vehicles.




% and timely adapts them 
% based on the input data streams to save network and compute resources.
% during a red light, the speed of vehicles is low, allowing us to significantly reduce the frame sampling rate of data collection and DNN inference, while still accurately determining the position and movement of the vehicles. 






\begin{table}[t]
\centering
\footnotesize
\begin{tabular}{ccc}
\hline
Example application & Analytic task        & Data type                                                             \\ \hline
Autonomous driving  & Vehicle detection    & \begin{tabular}[c]{@{}c@{}}RGB video,\\ LiDAR point cloud\end{tabular}   \\ \hline
Traffic analytics  & Vehicle segmentation & RGB video                                                                \\ \hline
Home security & Human detection      & \begin{tabular}[c]{@{}c@{}}RGB video,\\ Infrared, Depth map\end{tabular} \\ \hline
Smart home          & Audio to text        & Audio                                                                    \\ \hline
\end{tabular}
\vspace{0.2cm}
\tightcaption{Example applications of our solution.} 
\label{tab:applications}
\end{table}

\begin{table}[t]
\footnotesize
    \begin{tabular}{c c}
        \hline
        Knobs & \begin{tabular}[x]{@{}c@{}}Trade-off between\\accuracy and\end{tabular}\\
        \hline
        % \footnotesize Streaming delay & \footnotesize Video encoding parameters, region-of-interest \\
        % \footnotesize Number of data frames & \footnotesize Data frame difference thresholds \\
        % \footnotesize DNN inference time & \footnotesize model selection, model customization \\
        Resolution~\cite{awstream,dds,chameleon,vstore,videostorm,deepdecision,adascale,casva} & $B$ (\& $G$)  \\
        Quantization parameter~\cite{awstream,vstore,casva} & $B$ \\
        % Video bitrate~\cite{deepdecision} & $B$ \\
        % Encoding preset~\cite{vstore} & Encoding delay  \\
        Frame rate~\cite{awstream,chameleon,vstore,videostorm,deepdecision} & $B$ \& $G$   \\
        Frame filtering thresholds~\cite{reducto,glimpse,vigil}  & $B$ \& $G$ \\
        Fine-grained video compression~\cite{accmpeg,dds,eaar,saliency_hotmobile} & $B$  \\
        Feature compression~\cite{vcm,neurosurgeon} & $B$  \\
        Audio sampling rate~\cite{huang2001spoken, hirsch01_eurospeech, narayanan2018toward, gao2019mixedbandwidth, hokking2016speech} & $B$ (\& $G$)\\
        % \cite{cinet,vigil} & Region cropping & Bandwidth usage and GPU compute & \cmark \\
        % \cite{noscope,ekya} & Model customization & GPU compute  \\
        % \cite{chameleon} & Model selection & GPU compute &  \\
        % \cite{cloudseg} & Server-side super resolution & Bandwidth usage  \\
        % \cite{videostorm} & Server-side DNN parameter & GPU compute \\
        \hline
\end{tabular}
\vspace{0.2cm}
\tightcaption{A list of knobs that prior work has shown to be effective in reducing bandwidth usage ($B$) and/or GPU compute ($G$) without hurting inference accuracy.
This work does not consider knobs that alter the DNN itself. (We will discuss this limitation in \S\ref{sec:limitation_section}.)
% Distributed AI systems introduce rich types of knobs to reduce bandwidth usage ($B$) and/or GPU compute ($G$) without hurting inference accuracy.
% {\footnotemark}
} 
\label{tab:rich-set-of-knobs}
\end{table}  


% \mypara{Configurations must be adapted frequently}
The optimal settings of these configurations, as shown in prior work(\eg~\cite{awstream,chameleon,casva}), are highly {\em dependent} on
% must be \textit{tailored} to 
the content of the input data.
Therefore, as the content varies over time, these configurations must be adapted timely.
In the vehicle-detection example, when the green light is on, vehicles start to speed up, so the frames must be analyzed much more frequently by the DNN to 
% and analysis of more video frames by using a high frame rate is necessary to 
accurately capture the motion of those moving vehicles.
To put it in perspective, prior work has shown that in video object detection, 
10\% more video frames will have an accuracy over 80\% if adapting once every 4 seconds instead of once every 8 seconds.
% adapting once every 4 seconds makes 10\% more frames to have over 80\% accuracy compared to adapting once every 8 seconds~\cite{chameleon}.
In other applications (semantic segmentation, audio-to-text, and face generation) and configurations studied in this work, we observe a similar need for timely adaptation at a timescale of a few seconds. 
% \jc{a forward pointer and add a few words}









\tightsubsection{Existing configuration adaptation schemes}
\label{subsec:configuration-adaptation}
% \kt{Need to finish this.}



The key research question therefore is how to timely identify if a different configuration is better
% ---higher accuracy under a given resource budget, or much less resource usage while maintaining similar accuracy or both---
than the current configuration. 
There are two high-level categories of techniques.
% how to frequently identify the optimal configuration (the configuration with the highest accuracy under the resource budget)? 





\myparashort{Profiling-based methods: optimal though slow.} 
The first approach \textit{periodically profiles}
% different configurations to obtain their 
resource usage and
inference accuracy of different configurations by using them to run DNN inference, and then pick the best configuration (one that yields high inference accuracy and low resource usage)~\cite{chameleon,awstream,vstore,videostorm}.
% meets the resource
% budget and generates the most accurate inference results
However, each profiling
needs to run multiple \textit{extra} DNN inferences and thus significantly increases the GPU computation overhead. %before obtaining the profile.
For instance, AWStream~\cite{awstream} runs full profiling on just 3 knobs (resolution, frame rate, and quantization parameter) on a \textit{10-second}
% \jc{is this what awstream uses?} 
video, and its GPU computation is equivalent to running normal DNN inference on  
% consumes the same amount of GPU computation as analyzing 
more than an \textit{8-minute} video (\ie an almost 50$\times$ increase in GPU usage). 
As a result, if GPU resource is limited,
% is not sufficient to support frequent profiling, 
this approach must either profile less frequently, causing it to use outdated configurations when the optimal configuration changes
% before launching the next profiling 
(as shown in Figure~\ref{fig:adaptation-behavior}), or profile only fewer configurations, which may miss the optimal configuration.
\S\ref{sec:eval} will also test smarter variants of profiling (profiling only top $k$ configurations and profiling fewer values per knob) and shows that they still use much GPU resource for extra inference and are thus slow to adapt to change in source data.




% \mypara{Heuristics with no extra inference} 
\mypara{No extra inference though suboptimal}
An alternative approach~\cite{reducto,vigil,glimpse,accmpeg,casva,filterforward,dds,eaar,elf,fischer2021saliency} avoids extra inference and instead selects new configurations by analyzing the input data and filter out those data that are of the interest of the final DNN using simple heuristics.
This approach can adapt frequently as it does not require extra inference by the final DNN.
% allowing it to frequently 
% % This approach can quickly adapt 
% their configurations (\eg once every second~\cite{accmpeg}).
% to the input data as it performs no extra DNN inference.
% Since the process of obtaining the new configuration must be much less complex than final DNN inference, 
However, they may select a suboptimal configuration (illustrated in Figure~\ref{fig:adaptation-behavior}).
% with high DNN inference accuracy 
% even though they adapt much earlier than the profiling-based method.
Here, we discuss three types of heuristics. % in this category and briefly explain why they fall short.

\jc{see my comments in the caption of Table 1. the following items can refer to Table 1 once it's updated}

\begin{packeditemize}

\item \textit{Heuristics adapting temporal non-uniform knobs:} 
One line of work~\cite{reducto,glimpse,eaar} selects the frames most worthy for analysis \hl{by applying temporal non-uniform knobs (\eg} by computing the difference between the current frame and previously analyzed frame\footnote{Reducto calculates frame differences based on various features of the source data (\eg pixel  feature~\cite{glimpse}, Edge feature~\cite{marr1980theory} and Haar feature~\cite{viola2001rapid}), while other papers simpler difference metrics~\cite{glimpse,eaar}.} and sends the current frame out for DNN inference if the difference is greater than a threshold).
As elaborated in \S\ref{sec:intro}, this method fails when the background pixels in a video change a lot between frames, making high frame difference a poor signal to decide if a frame should be analyzed or not.




\item \textit{Heuristics adapting spatial non-uniform knobs:}
% The heuristics can be smarter than computing frame difference.
\hl{
Another line of work~\cite{dds,eaar,vigil,accmpeg,fischer2021saliency} reduces bandwidth usage by calculates the regions of interest, and assigns regions of interest higher encoding quality by applying non-uniform spatial knobs.
% A line of work reduces bandwidth usage by only encoding small spatial regions in high quality, and they do so by running a {\em shallow NN} on each frame to select areas (sometimes called ``saliency'') whose pixel values are near the objects of interest.
Some of these work identifies regions of interest by running a \textit{shallow neural network} on each frame.
However, these shallow NNs, unlike the final DNN, are inadequate to recognize small objects.}
As acknowledged in one of the latest work~\cite{accmpeg}, it rarely recognizes small vehicles in highway video feeds and thus fails to encode them in high quality.
Other heuristics try to leverage information naturally emitted from the final DNN, such as region proposals (an intermediate output of some DNNs that indicates which regions in the source data may contain objects).
This approach can also adapt quickly, but as shown in~\cite{accmpeg}, region proposals only indicate whether {\em some} objects are in the region, rather than whether raising the quality of that region will likely affect the ability for the DNN to detect the objects of interest.


\item \textit{Heuristics adapting uniform knobs}: \hl{Recent proposal also propose heuristics based on reinforcement learning~\cite{casva} that adapts uniform knobs such as resolution and frame rate. This heuristics rely on the file size of the encoded video to adapt the knobs. However, this heuristics will use a relatively fixed configuration when the camera itself moves (\eg dashcam), regardless of whether the objects of interest appears a not. This is because the file size of the video typically depends on the movement speed of \textit{all} pixels, so the file size is always large and the appearance of new object creates negligable impact on the file size when the camera itself moves.}

\end{packeditemize}

% the inference of a particular DNN in consideration.

% In short, while a variety of heuristics are proposed to adapt configuration quickly without extra inference, they often select suboptimal configurations.

\mypara{Designed for specific configurations or DNNs}
Moreover, most techniques are studied and evaluated {\em only} on RGB video feeds, and it is unclear whether they will be effective on other types of data (\eg LiDAR point cloud, depth map, or audio waves).
Even in video analytics, the proposed heuristics often work well only for {\em specific knobs}.
As elaborated in \S\ref{sec:intro}, Reducto~\cite{reducto}'s frame-different detector is 
% For example, Reducto's logic~\cite{reducto} uses inter-frame difference to select the frames that most need to be analyzed, and thus is 
ill-suited to tuning the encoding quality parameter of each frame, which depends on the content of the new frame, rather than how it differs from the previous frame.
Likewise, DDS~\cite{dds} tunes the encoding quality parameters of each fine-grained spatial block to improve inference accuracy on each frame, but it is not aware of whether the current frame is redundant given past inference results, thus it cannot generalize to knobs such as frame selection.
Moreover, DDS relies on region proposals, which are common in object detection DNNs but not in other types of DNNs (\eg classification DNNs~\cite{vit,vgg} and semantic segmentation DNNs~\cite{unet,fcn-resnet101}).


% An ideal configuration adaptation systems should meet these two
% requirements: 1. quickly adapt to optimal configuration in a large configuration
% space without extra inference 2. minimum assumption to the underlying system
\mypara{Summary} 
In short, previous work fails to meet at least one of the three requirements: {\em (i)} adapt timely, {\em (ii)} converges to a near-optimal configuration, and {\em (iii)} apply to a wide range of configurations and applications.



==> old_text.tex <==


\vspace{5cm}






\vspace{0.2cm}


Recent work has approached this challenge by revamping existing network protocols with different models of user utility.
Recent work has approached this problem by leveraging the tolerance of video analytics to suboptimal quality of videos, so in theory downsized videos can achieve high analytics accuracy, just as Internet video viewers can tolerate slight quality degradation.


\vspace{0.2cm}


Recent work has approached this challenge by revamping existing network protocols with different models of user utility.
Recent work has approached this problem by leveraging the tolerance of video analytics to suboptimal quality of videos, so in theory downsized videos can achieve high analytics accuracy, just as Internet video viewers can tolerate slight quality degradation.


\vspace{0.2cm}


Recent work has approached this challenge by revamping existing network protocols with different models of user utility.
Recent work has approached this problem by leveraging the tolerance of video analytics to suboptimal quality of videos, so in theory downsized videos can achieve high analytics accuracy, just as Internet video viewers can tolerate slight quality degradation.


\vspace{0.2cm}


Recent work has approached this challenge by revamping existing network protocols with different models of user utility.
Recent work has approached this problem by leveraging the tolerance of video analytics to suboptimal quality of videos, so in theory downsized videos can achieve high analytics accuracy, just as Internet video viewers can tolerate slight quality degradation.


\vspace{0.2cm}


Recent work has approached this challenge by revamping existing network protocols with different models of user utility.
Recent work has approached this problem by leveraging the tolerance of video analytics to suboptimal quality of videos, so in theory downsized videos can achieve high analytics accuracy, just as Internet video viewers can tolerate slight quality degradation.


\vspace{0.2cm}


Recent work has approached this challenge by revamping existing network protocols with different models of user utility.
Recent work has approached this problem by leveraging the tolerance of video analytics to suboptimal quality of videos, so in theory downsized videos can achieve high analytics accuracy, just as Internet video viewers can tolerate slight quality degradation.


\vspace{0.2cm}


Recent work has approached this challenge by revamping existing network protocols with different models of user utility.
Recent work has approached this problem by leveraging the tolerance of video analytics to suboptimal quality of videos, so in theory downsized videos can achieve high analytics accuracy, just as Internet video viewers can tolerate slight quality degradation.


\vspace{0.2cm}


Recent work has approached this challenge by revamping existing network protocols with different models of user utility.
Recent work has approached this problem by leveraging the tolerance of video analytics to suboptimal quality of videos, so in theory downsized videos can achieve high analytics accuracy, just as Internet video viewers can tolerate slight quality degradation.


\vspace{0.2cm}


Recent work has approached this challenge by revamping existing network protocols with different models of user utility.
Recent work has approached this problem by leveraging the tolerance of video analytics to suboptimal quality of videos, so in theory downsized videos can achieve high analytics accuracy, just as Internet video viewers can tolerate slight quality degradation.


==> overview.tex <==

\section{Overview}

$\bullet$ We present \name, a configuration adaptation system that meets three requirements: 1. quickly adapt to optimal configuration with no extra inference 3. minimum assumption to the underlying applications


\section{\accgrad}



\subsection{Key idea: accuracy-knob gradient}

\begin{itemize}
    \item How to quickly adapt to optimal configuration with no extra inference? 
    This is not doable in general systems.
    In deep learning system knobs, however, we identify three enablers of deep learning system knobs.
    \item \textit{Accuracy-Resource Property}: For most of the knobs, if changing the value of one knob result in spending more (or less) resource, the corresponding inference results also become more (or less) accurate.
    
    \item Examples and non-examples
    \item \textit{Black-box Property}: Most of the knobs treat DNN as a black box and change the DNN input.
    \item Examples and non-examples
\end{itemize}




% To obtain the knob-accuracy impact in real-time, we present \name. We first show that knob-accuracy impact is a better feedback for the underlying system, and discuss the APIs and mechanisms of obtaining accuracy gradient.

% % \subsection{Accuracy gradient as a better predictor}
% \kt{Introduce API}

% To better predict the accuracy, the key is to know the impact of knobs on accuracy in real-time.

% Obtaining knob-accuracy impact enables us to do two things.
% First, it can cheaply identify whether the current configuration is locally optimal or not.
% This is because checking the local optimality is essentially go through each knob and compare between the accuracy gain of changing the knob and the extra delay caused by the knob.
% In other word, we can check the local optimality by directly comparing between the knob-accuracy impact and extra delay.
% Second, it can better estimate the accuracy change of an unknown configuration under the same video content.


% One may worry that knob-accuracy impact will let the system stuck in the local optimal.
% We argue that for one single knob, when it goes from the cheapest value to the most expensive value, the accuracy gain will become smaller but the streaming delay will still grow in a steady pace. 
% As a result, the overall accuracy - delay objective is in general \textit{concave} and have no local optimal.



\begin{itemize}
    \item 
    \accres suggests that the change of accuracy with respect to knob value change can reflect the ability of trading resource for accuracy for each individual knob. 
    
    \item In order to measure this change, we propose a new metric: \accgrad, defined as the difference of accuracy, divided by the difference of two consecutive values of one knob.
    \item With \accgrad, \name can quickly adapt to optimal by allocate more resources to those knobs with high \accgrad to improve accuracy, and cut the resource usage of those knobs with low \accgrad to save resource.
    \item Compared to frequent profiling: avoid extra inference.
    \item Compared to server-side DNN output: use DNN parameters as a reliable performance estimator.
    \item Show an example like AccMPEG.
    % \item Present accuracy gradient as the solution and define accuracy gradient as the diff of accuracy divided by the diff of two consecutive parameter values.
    % % \item With accuracy gradient, we can prune out those configurations that yeild similar accuracy without extra inference.
    % % \jc{Gradient -> which parameters does not improve accuracy; which parameters does improve accuracy}
    % \item First, accuracy gradient can be calculated without extra inference. We will further discuss this in \S\ref{subsec:decoupling}.
    % \item Second, accuracy gradient can help \name to quickly approach to optimal. With accuracy gradient, \name can identify which parameters have huge impact on accuracy and improve accuracy by adapting these parameters. On the other hand, accuracy gradient also allows \name to identify which parameters have little impact on accuracy and save resource usage from these parameters.
\end{itemize}

\subsection{Decoupling \accgrad}

\begin{itemize}
    \item How to calculate this gradient? A direct way is to calculate the gradient in a knob-by-knob manner. However, this requires extra inference.
    \item To reduce this cost, we find \blackbox useful: as most of the knobs affect the DNN output only by changing the DNN input, we can first calculate how system knobs affect the DNN input (\ie the gradient of DNN input with respect to the knobs), and then study how the DNN input affects the inference accuracy (\ie the gradient of inference accuracy with respect to the input).
    \item Why decoupling at DNN input? The trade-off between cost reduction and knob incoporation.
\end{itemize}

\begin{comment}
Calculating the knob-accuracy impact in real-time can consumes a lot of resource.
For example, a naive way to calculate knob-accuracy impact is to enumerate every knob, change that knob a bit and observe the change of accuracy.
However, this requires running the end-to-end system $O(n)$ times, where $n$ is the number of knobs. 
\kt{Write a running example here}


To overcome this difficulty, our approach is to obtain knob-accuracy impact by get the gradient of knobs with respect to accuracy (we call this gradient \textit{knob-accuracy gradient}).
Obtaining knob-accuracy gradient requires us to 
To answer this, we use chain rule to decouple the gradient into two parts:
$$
\frac{\partial Acc}{\partial k_i} = \frac{\partial Acc}{\partial I}\cdot \frac{\partial I}{\partial k_i},
$$
where $Acc$ means the accuracy function, $k_i$ means the $i^{th}$ knob, $I$ means the input of the DNN\footnote{As both of the two gradient is of matrix format, the $\cdot$ should be the inner product. We use $\cdot$ for simplicity.}.
It makes use of two key properties of AI pipelines to drastically reduce the cost of calculating this gradient:
\begin{packeditemize}
    \item The analytic DNN is analytically differentiable.
    \item For a large subset of knobs, obtaining the numerical gradient of the input to DNN with respect to knobs can be done locally on the camera and thus does not require sensor-server communication.
\end{packeditemize}
\end{comment}

% \subsection{Workflow of \name}


% \begin{itemize}
%     \item Show a workflow figure of \name. 
% \end{itemize}




% \subsection{Accuracy gradient as a better feedback}

% \begin{itemize}
%     \item We find that: how much the analytic accuracy change differs if we change different knobs is essentially asking what is the \textit{gradient} of analytic accuracy with respect to the knob values.
%     \item With the accuracy gradient, we can better predict the analytic accuracy of those knob values we did not explore yet.
% \end{itemize}

% Our goal is to calculate the gradient of accuracy with respect to knobs (we call this gradient \textit{accuracy gradient}) by only evaluating the system under one configuration.

% Accuracy gradient enables us to better predict the accuracy of different configurations under similar video content.
% As a result, one can pick a chheaper configuration while still achieving the same accuracy with accuracy gradient.


\begin{comment}

\subsection{Programming interface of \name}


\begin{figure}
    \centering
    \includegraphics[width=1\columnwidth]{figs/raw-input-inference.jpg}
    \caption{\name handles those hyper-parameters that preprocess the input to the DNN.}
    \label{fig:raw-input-inference}
\end{figure}



\subsection{API of HPs} 

As shown in Figure~\ref{fig:raw-input-inference}, \name abstracts the underlying AI systems into two stages.
In the preprocessing stage, the AI system pre-processes the raw sensing data to obtain the input to the DNN.
In the inference stage, the DNN performs inference and obtain the analytic results.
\name focuses on those HPs for preprocessing stage (we will show most of the HPs fall into this category in \S\ref{subsec:hp-examples}, together with some example HPs that do not belong to this category).
As the preprocessing does not incur the compute-intensive server-side DNNs, we assume that this step can be locally done at the camera.

Based on this observation, the programming interface of \name towards HPs are:
\begin{small}
\begin{verbatim}
prep(Data raw, List hps)-> (Data input, Bytes encoded)
proxy(Result result) -> Float pseudo_acc
\end{verbatim}
\end{small}

The first function \texttt{prep} pre-processes the raw sensed data \texttt{raw} based on a list of HPs \texttt{hps}, and return the codec-encoded byte stream \texttt{encoded} and the input data \texttt{input} that server-side DNN will receive.

The second function aims to provide a differentiable proxy towards accuracy (since most of the existing accuracy function is not differentiable).
As most of the DNNs will return confidence scores to describe the confidence of the analytic results the DNN derives, we use the sum of the confidence scores as the default proxy.
This complies with recent computer vision advances on evaluating the quality of inference results.

Further, we empirically verify this assumption on different types of HPs and different videos.


\subsection{Examples}
\label{subsec:hp-examples}


This assumption precludes those HPs that directly changes server-side DNN (\eg customizing the server-side DNN or switching between different server-side DNNs).
That said, the vast majority of HPs, including HPs of traditioanal data encoding codecs (\eg frame rate, resolution, quantization parameters etc), DNN-based encoding codec (\eg feature compression, super resolution), fine-grained data quality assignments (\eg region-of-interest selection, macroblock encoding quality selection), sensor-side data filtering (\eg filtering the frames through cheap object detector or through cheap feature extractors) still fit in our assumption. 



% \mypara{API of DNNs}
% We require that the DNN to implement two APIs:
% \begin{small}
% \begin{verbatim}
% inference(Data input)-> Result result
% backprop(Result result, Function f)-> Data grad
% \end{verbatim}
% \end{small}



\subsection{Workflow of \name}

Contrast between conventional workflow and ours workflow

\end{comment}







% \subsection{Workflow and API of \name}
% \kt{Goal: how to use the API in our system to calculate accuracy gradient}

% \begin{figure}
%     \includegraphics[width=1\columnwidth]{figs/workflow.jpg}
%     \caption{Workflow of \name \kt{Plot this figure in a "call stack" way, MAKE THE FONT LARGER}}
%     \label{fig:workflow}
% \end{figure}

% \mypara{Workflow of \name} Based on the approach above, we present the workflow of \name in Figure \ref{fig:workflow}.


% Our system enables the application to obtain the gradient of accuracy with respect to the knobs through the following API:
% $$AccGrad = calc(V_t, \{knob_i\}_{i=1}^n)$$

% \mypara{Towards knobs}

% $knob'_i = reduce(knob_i)$
% This reduce the knob to lower knob value

% \mypara{Towards DNN}
% We require the DNN to implement two APIs:
% \begin{packeditemize}
%     \item \texttt{result = inference(V)}
%     \item \texttt{saliency = backprop(result, grad)}
% \end{packeditemize}

% \mypara{Towards application}
% We require the application to implement:
% \begin{packeditemize}
%     \item \texttt{encode(V, knobs)} This one should be locally done on the camera
%     \item \texttt{proxy(results)}
% \end{packeditemize}


% \subsection{How to use the API}






% \subsection{Reduce the cost of accuracy gradient}


% \mypara{Accuracy gradient sampling}


% \mypara{Accuracy gradient compression}



==> overview_v2.tex <==

% \begin{figure*}[t]
%     \centering
%     \includegraphics[width=1.5\columnwidth]{figs/workflow.pdf}
%     \caption{Workflow of \name.}
%     \label{fig:workflow}
% \end{figure*}



% \begin{figure}[t]
%     \centering
%     % \includegraphics[width=0.5\columnwidth]{figs/placeholder-eval-overall-1.pdf}
%     % \subfloat[][\centering{Object detection\\~~~~(Dashcam)}]
%     % {
%     %     \includegraphics[width=0.24\textwidth]{figs/detection_dashcam_FPN.pdf}
%     %     \label{subfig:1}
%     % }
%     \subfloat[][Profiling]
%     {
%         \includegraphics[width=0.32\columnwidth]{figs/behavior_profile.pdf} 
%         \label{subfig:1}
%     }
%     \subfloat[][Output-based]
%     {
%         \includegraphics[width=0.32\columnwidth]{figs/behavior_output.pdf} 
%         \label{subfig:1}
%     }
%     \subfloat[][OneAdapt]
%     {
%         \includegraphics[width=0.32\columnwidth]{figs/behavior_oneadapt_arrow.pdf} 
%         \label{subfig:1}
%     }
    
%     \tightcaption{Contrasting \name with profiling-based approach and output-based approach. \name quickly approaches the optimal point via the gradient vector, while the profiling-based method requires a high amount of extra inference to derive the optimal configuration, and the output-based method approaches the optimal configuration slowly.}
%     \label{fig:compare}
% \end{figure}


% \begin{figure}[h]
%     \includegraphics[width=1.15\columnwidth]{figs/gradient.jpg}
%     \caption{Gradient \name.}
%     \label{fig:workflow}
% \end{figure}

% \begin{figure*}[h]
%     \centering
%     \includegraphics[width=1.5\columnwidth]{figs/timeline.jpg}
%     \caption{Workflow of \name. \kt{Place a overall workflow figure here.} }
%     \label{fig:workflow}
% \end{figure*}


% \begin{figure*}[h]
%     \includegraphics[width=2.4\columnwidth]{figs/adaptation-time-series.pdf}
%     \caption{Adaptation behavior of \name}
%     \label{fig:workflow}
% \end{figure*}

% \begin{packeditemize}
%     \item Sketch three requirements (1). adapt frequently (2). reach a near-optimal configuration (3). be applicable to a range of configs \& apps.
%     \item \S 3.1
%     \item Introducing \outputgrad 
%     \item Calculating \outputgrad with no extra inference. Need two figures here. 1). Show what is backpropagation 2). show how is backpropagation saves cost.
%     \item Correlation between \outputgrad and accuracy.
%     \item \S 3.2
%     \item Optimizing accuracy through gradient ascent.
%     \item This gradient-ascent-based algorithm allows us to simultaneously achieve 3 objectives.
%     \item Talking about its caveats
%     \item \S 3.3.
%     \item Run people through an end-to-end example, where the sensor and the server are separated by network.
%     Figure: a timeline figure between the sensor and the server Key highlights: when the inference results are obtained, and when the configuration is updated.
% \end{packeditemize}





\tightsection{Design of \name}
\label{sec:design}
% \tightsection{\outputgrad}
% \jc{Junchen can you check this part? I did a full rewrite to Sec 3.1}

We present \name, a configuration adaptation system that aims at improving along the three requirements mentioned above --- frequent adaptation to near-optimal configuration on various configuration knobs. %---over prior solutions.

The basic idea of \name (illustrated in Figure~\ref{fig:adaptation-behavior}) is to calculate frequently
% The key for \name to meet the three requirements is to calculate 
the {\em gradient} of how DNN inference output changes with each configuration knob, which we refer to as the {\em \outputgrad}.
Using the up-to-date estimate of \outputgrad, \name incrementally updates the configuration to improve the DNN inference results but still stays in the (compute/network) resource budget or maximally reduces the resource usage with minimum change on the DNN inference results.
% Figure~\ref{fig:adaptation-behavior} illustrates an example: after a change of input data, \name can adapt more frequently and gradually converge to a near-optimal configuration.


We begin by defining \outputgrad (\S\ref{subsec:outputgrad}) and presenting the key insight that the inherent differentiability of DNNs enables fast calculation of \outputgrad without extra DNN inference (\S\ref{subsec:differentiability-outputgrad}).
Then we introduce \name's gradient-ascent strategy based on \outputgrad (\S\ref{subsec:gradient-ascent}) and state the caveats and benefits of \name (\S\ref{subsec:limitation}).

% changes the configuration to another configuration that meets the (compute/network) resource budget and greatly improves accuracy.\jc{confirm with kuntai}
% to improve accuracy within the resource budget. 



% after the content of the input data changes.
% that allows operators to achieve the following three requirements simultaneously:
% \begin{packeditemize}
%     \item Adapt frequently
%     \item Reach a near-optimal configuration
%     \item Apply to a wide range of configurations and applications
% \end{packeditemize}


% \subsection{Modeling of knobs}

% \name focuses on handling a subset of knobs that satisfies the following two properties:

% \begin{enumerate}
%     \item \textit{\accres}: For each knob, there exists one direction (either increasing or decreasing), if \name fix other knobs and change this knob according to this direction, the resource consumption and the accuracy statistically increases.
%     % (we assume that this direction is increasing the knob value by default) if changing the value of one knob result in spending more (or less) resource, the corresponding inference results also become more (or less) accurate.
%     \item \textit{\blackbox}: Most of the knobs treat DNN as a black box and change the DNN input. We illustrate this point in Figure~\ref{??}.
% \end{enumerate}





\tightsubsection{\outputgrad: Estimating how configuration affects DNN inference}
\label{subsec:outputgrad}



\begin{figure*}[t]
    \centering
    % \includegraphics[width=0.5\columnwidth]{figs/placeholder-eval-overall-1.pdf}
    % \subfloat[][\centering{Object detection\\~~~~(Dashcam)}]
    % {
    %     \includegraphics[width=0.24\textwidth]{figs/detection_dashcam_FPN.pdf}
    %     \label{subfig:1}
    % }
    \subfloat[][Calculating \outputgrad using its definition]
    {
        \includegraphics[width=1.6\columnwidth]{figs/gradient-before-new.pdf} 
        % {figs/gradient-before_haodong.jpg} 
        \label{subfig:gradient-before}
    }
    \\
    \subfloat[][Calculating \outputgrad using \name]
    {
        \includegraphics[width=1.6\columnwidth]{figs/gradient-after-new.pdf} 
        % {figs/gradient-after_haodong.jpg} 
        \label{subfig:gradient-after}
    }
    % \subfloat[][Pipeline \circled{8}]
    % {
    %     \includegraphics[width=0.24\textwidth]{figs/lidar_video_e2e.pdf} 
    %     \label{subfig:1}
    % }
    % \subfloat[][Keypoint detection (Skate)]
    % {
    %     \includegraphics[width=0.22\textwidth]{figs/placeholder-eval-overall-2.pdf}
    %     \label{subfig:2}
    % }
    % \\
    % \subfloat[][Adapting configuration using \outputgrad]
    % {
    % \centering
    %     \includegraphics[width=1.8\columnwidth]{figs/workflow.pdf} 
    %     % {figs/gradient-after_haodong.jpg} 
    %     \label{fig:workflow}
    % }
    \tightcaption{Comparison between calculating \outputgrad naively and calculating \outputgrad using \name. \name calculates \outputgrad with \textit{no extra inference}. Note that the image of the DNN is cropped from this\cite{dnnimagesource} GitHub page.}
\end{figure*}








% takes a different approach by focusing on the \textit{gradient} of inference results in relation to the current configuration, referred to as \outputgrad.

% \mypara{Definition and example}
% Intuitively, the \outputgrad is the amount that the DNN inference output would change
% % \footnote{\kt{Talk about how to calculate inference results change. The calculation depends on whether Haodong's experiment works or not.}} 
% if a small adjustment was made to each knob in the current configuration.

% Though it sounds conceptual, \outputgrad can be explained with a simple 
% video analytics system that feeds each video frame to a DNN that determines whether it contains vehicles or not. 
% % Before that, we first explain the concept of \outputgrad in a concrete example.
% % consider an analytic system that analyzes a dashcam video feed by running a DNN to classify each video frame as containing a vehicle or not.
% Following prior work~\cite{chameleon,??}, we assume the system can tune two configuration knobs, frame rate and resolution.
% Suppose that the current configuration is 20fps and 480p, and the DNN output\footnote{Typical DNN output is more than a single value. Here, we assume that for a given video segment, the output of DNN inference is the average confidence of all detected objects. We will explain in \S\ref{??} how we turn the DNN output to a single value in general cases.} on a video segment is 0.9, and if we slightly increase the frame rate from 20fps to 21fps, the DNN output on the same video segment becomes 0.91.
% Then the \outputgrad of frame rate is (0.91-0,9)/(21-20)=0.01.
% Following a similar procedure, we calculate the \outputgrad of the resolution, say its value is -0.02.


% We now define \outputgrad first, then explain how to estimate \outputgrad efficiently, and finally why using \outputgrad to adapt configuration improves accuracy.
% describe the assumptions we make to calculate \outputgrad, define \outputgrad and then explain how to calculate \outputgrad and why one can use it to improve inference accuracy.


\mypara{Terminology}
% To formally define \outputgrad, 
We first introduce terminology to describe the DNN output.
% in a way that is relevant to this work. 
This is necessary because \name works with various DNN tasks and source data types (see Table~\ref{tab:pipeline} for a list).
% , from object detection in video and audio-to-text translation (see Table~\ref{??} for a list).
We split the source data stream into fixed-length (by default, one-second-long) intervals, called {\em adaptation intervals}.
In each adaptation interval, the data is first preprocessed with the current configuration and then fed to DNN (see Figure~\ref{fig:workflow}), and the DNN output contains multiple {\em elements}. 
% Note that there might be multiple DNN inferences within an adaptation interval.
An element can be a detected object in object detection, a detected text in audio-text translation, or the classification of a pixel in semantic segmentation.
Most DNNs for these tasks will associate each element with a confidence {\em score}, and only elements with a score over a confidence {\em threshold} will be counted towards accuracy. 
\name works with any DNN tasks that return elements with confidence scores as output. 

For the DNN output in an adaptation interval, we define the {\em \summary} by the number of elements in an adaptation interval whose confidence scores exceed the confidence threshold.
The rationale of \summary will be explained in detail later in \S\ref{subsec:gradient-ascent}.
For now, we can think of \summary as a one-value summarization of the DNN output whose change indicates the change in inference accuracy.

Though the definitions may not be universally applicable, it naturally applies to most prior work in video analytics as well as the new applications mentioned in Table~\ref{tab:applications}.
% developers do not need to make major changes to the DNN to use \name.






% \mypara{Assumption to the DNNs}
% We require the DNNs to expose the confidence scores in their inference results and the confidence threshold.
% Note that it does not impose an extra burden on the applications since most of the applications already expose confidence scores to indicate the uncertainty of DNN outputs and use confidence thresholds to filter out DNN outputs with low confidence. 
%those uncertain results returned from the DNN.

\mypara{Definition of \outputgrad}
\outputgrad is how much a small change in the current value of each knob changes the \summary (the number of DNN-returned elements in an adaptation interval with confidence scores over the confidence threshold).
Here, we use $\Output_\Config(\Data)$ to denote the \summary 
% averaged number of elements with confidence over the threshold in the DNN output 
at source data $\Data$ using configuration $\Config=(\Knob_i)_{i=1,\dots,n}$ ($n$ knob values). The \outputgrad of knob $\Knob_i$ is

\vspace{-0.2cm}
\begin{@empty}
\footnotesize
\begin{equation*}
\frac{\Delta \Output}{\Delta k_i} = \frac{\Output_{(\dots,\Knob_i+\delta,\dots)}(\Data)-\Output_{(\dots,\Knob_i,\dots)}(\Data)}{(k_i+\delta) - k_i}.
\end{equation*}
\end{@empty}

% Specifically, we use the following 
% \jc{Kuntai, please write the math expression here}
% confidence scores greater than the confidence threshold averaged across different data frames (\eg video frames).
% Intuitively, the \outputgrad is the amount that the DNN inference output would change
% if a small adjustment was made to each knob in the current configuration.
To help understand \outputgrad, we use a simple 
video analytics system that feeds each video frame to a DNN that performs vehicle detection with a confidence score of 0.5. 
Figure~\ref{subfig:gradient-before} illustrates \outputgrad in this example.
Following prior work~\cite{chameleon,vstore,videostorm,casva}, we assume the system can tune two configuration knobs, frame rate, and resolution.
Suppose that the current configuration is 10 frames per second (fps) and 480p.
% The analytic system will take a one-second-long, 20fps and 480p video and analyzes it through DNN.
When taking 1-second input, the DNN outputs 34 vehicle bounding boxes with confidence scores greater than 0.5 on these 10 frames, an average of 3.4 vehicles per frame.
% \footnote{Typical DNN output is more than a single value. Here, we assume that for a given video segment, the output of DNN inference is the average confidence of all detected objects. We will explain in \S\ref{??} how we turn the DNN output to a single value in general cases.} 
If we slightly increase the frame rate from 10fps to 15fps, the DNN outputs 66 vehicle bounding boxes with confidence scores greater than 0.5, on average 4.4 vehicles per frame.
Then the \outputgrad of the current frame rate is 

\vspace{-0.3cm}
\begin{@empty}
\footnotesize
\begin{align*}
\frac{\Delta \Output}{\Delta \text{framerate}}&=\frac{\Output_{(480p,15fps)}-\Output_{(480p,10fps)}}{15fps-10fps}=\frac{4.4-3.4}{15-10}=0.2.
% ,\\
% \frac{\Delta \Output}{\Delta \text{resolution}}&=\frac{\Output_{(720p,10fps)}-\Output_{(480p,10fps)}}{720p-480p}=0.01.
\end{align*}
\end{@empty}
% is (3.8-3.4)/(15-10)=0.08.
Following a similar procedure, we assume that the \outputgrad of the resolution will be:

\vspace{-0.3cm}
\begin{@empty}
\footnotesize
\begin{align*}
\frac{\Delta \Output}{\Delta \text{resolution}}&=\frac{\Output_{(720p,10fps)}-\Output_{(480p,10fps)}}{720p-480p}=\frac{5.8-3.4}{720-480}=0.01.
\end{align*}
\end{@empty}




\begin{figure*}
    \centering
    \includegraphics[width=1.6\columnwidth]{figs/workflow.pdf} 
    \tightcaption{Adapting configuration using \outputgrad. 
    \hl{Note that the generation of DNN output happens \textbf{before} the configuration adaptation process and thus the delay of obtaining the inference results is \textbf{not} affected by the configuration adaptation process (unless there is no sufficient resource for \name to perform the inference and the adaptation in real-time).}}
    \label{fig:workflow}
\end{figure*}

% Figure~\ref{subfig:gradient-before} illustrates the calculation of \outputgrad in the vehicle detection example.
% In this figure, we use $\Output_\Config(\Data)$ to denote the averaged number of above-threshold confidence scores in the DNN output at input data $\Data$ using configuration $\Config=(\Knob_i)_{i=1,\dots,n}$ (a vector of $n$ knob values), then \outputgrad of knob $\Knob_i$ is


% As a result, we have 
% \begin{@empty}
% \footnotesize
% \begin{align*}
% \frac{\Delta \Output}{\Delta \text{framerate}}&=\frac{\Output_{(480p,15fps)}-\Output_{(480p,10fps)}}{15fps-10fps}=0.08,\\
% \frac{\Delta \Output}{\Delta \text{resolution}}&=\frac{\Output_{(720p,10fps)}-\Output_{(480p,10fps)}}{720p-480p}=0.01.
% \end{align*}
% \end{@empty}








% We will soon show that there is a statistical correlation between \outputgrad and the accuracy of other configurations



% , each with 5 possible values (1 to 5 for simplicity),
% We assume that the current configuration is $(\Knob_1=2,\Knob_2=2)$.
% The \outputgrad of the two configuration knobs are:
% \jc{Use a concrete example. don't use values 1-5}

% \vspace{-0.3cm}
% \begin{@empty}
% \footnotesize
% \begin{align*}
%    & \frac{\Delta \Output}{\Delta \Knob_1}=\frac{\Output(\Knob_1=3,\Knob_2=2)-\Output(\Knob_1=2,\Knob_2=2)}{3-2}=0.2\\
%    & \frac{\Delta \Output}{\Delta \Knob_2}=\frac{\Output(\Knob_1=2,\Knob_2=3)-\Output(\Knob_1=2,\Knob_2=2)}{3-2}=0.2=0.1,
% \end{align*}
% \end{@empty}
% where $O(res=a, fps=b)$ means the corresponding inference results when configuring $res=a$ and $fps=b$.
% \kt{I guess we need a figure here.}


Essentially, \outputgrad indicates how the \summary of DNN inference results (\eg the number of detected objects) change with the value of each configuration knob. 
As shown in \S\ref{subsec:gradient-ascent}, \name's fast adaptation algorithm relies on \outputgrad to tune knob values in the ``direction'' that most improves accuracy or reduces resource usage without hurting accuracy (\S\ref{subsec:limitation}).
But first, we need to calculate \outputgrad quickly and using minimum GPU cycles. 


\tightsubsection{Using DNN differentiability to calculate \outputgrad}
\label{subsec:differentiability-outputgrad}

As shown in Figure~\ref{subfig:gradient-before}, a naive calculation of \outputgrad requires 
% through its definition results in high GPU overhead (
$n$ extra DNN inferences for $n$ configuration knobs.
However, we calculate \outputgrad \textit{with no extra DNN inference} by taking advantage of the {\bf differentiability of DNNs}. 

First, we decouple \outputgrad into two terms:
\begin{packedenumerate}
    \item {\em \dnngrad:} how the number of above-threshold confidence scores changes with different parts of DNN input (\Input).
    \item {\em \inputgrad:} how much different parts of DNN input change with each knob value of the current configuration (\Config). %in relation to the change in the current configuration.
\end{packedenumerate}

Formally, we use $\Input_{\Config}(\Data)$ to denote the DNN input of configuration $\Config$ at source data $\Data$. The \outputgrad of $\Knob_i$ on \Data can be expressed by
\vspace{-0.3cm}
\begin{align}
{\color{black}\underbrace{\highlight{white}{$\frac{\displaystyle \Delta \Output}{\displaystyle \Delta \Knob_i}$}}_{\text{\sf \footnotesize \textcolor{black!85}{\outputgrad}}}}=
{\color{black}\underbrace{\highlight{white}{$\frac{\displaystyle \Delta \Output}{\displaystyle \Delta \Input_\Config(\Data)}$}}_{\text{\sf \footnotesize \textcolor{black!85}{\dnngrad}}}}\otimes
{\color{black}\underbrace{\highlight{white}{$\frac{\displaystyle \Delta \Input_\Config(\Data)}{\displaystyle \Delta \Knob_i}$}}_{\text{\sf \footnotesize \textcolor{black!85}{\inputgrad}}}}
\label{eq:grad-decouple}
\vspace{-0.08cm}
\end{align}
Here, $\otimes$ means inner product.

The decoupling makes the calculation of \outputgrad much more resource-efficient for three reasons:
\begin{packeditemize}
\item The first term (\dnngrad) can be estimated by the DNN's derivation at input $\Input_\Config(\Data)$ via one backpropagation\footnote{
% \kt{Illustrate how we make the \# of above-threshold confidence scores differentiable here.}
To make $\Output$ differentiable, we define it to be $\sum_{e} Sigmoid(\alpha(Score_e-\beta))$ where $Score_e$ is the score of element $e$, $\beta$ is the confidence threshold (see \S\ref{subsec:eval-setup} for its exact value in each application), and $\alpha$ is a hyperparameter (by default, we use 20). Note that this function is almost identical to \summary when $\alpha$ is sufficiently large.
}.
This is a constant GPU-time operation without extra inference as it reuses the layer-wise features computed as part of the DNN inference of the current configuration.
\S\ref{sec:cost} will further reduce the compute overhead of backpropagation.

\item Second, the \dnngrad needs to be calculated once and re-used to derive \outputgrad of different knobs without extra DNN inference.
This is because the \dnngrad describes DNN's sensitivity to its input and thus remains largely similar if the change in DNN input is not dramatic.
For instance, the \dnngrad of an object-detection DNN is high on pixels associated with key visual features of an object.
% \jc{edit ends here}

\item Finally, computing this term does not involve any DNN inference, as it only runs the preprocessing part of the DNN analytics system multiple times.

\end{packeditemize}



% Additionally, 





% Therefore, computing \outputgrad for multiple configuration knobs only requires a one-time backpropagation on GPU and no extra DNN inference.

Figure~\ref{subfig:gradient-after} shows an example of how \outputgrad is calculated from \dnngrad and \inputgrad.
% We use $\Input_{\Config}(\Data)$ to denote the DNN input of configuration $\Config$ at input data $\Data$.
% The decoupling can be written as \outputgrad $\approx$ \inputgrad $\otimes$ \dnngrad, concretely,

\vspace{-0.3cm}
\begin{@empty}
\scriptsize
\begin{align*}
\frac{\Output_{(480p,15fps)}-\Output_{(480p,10fps)}}{15fps-10fps} &\approx \frac{\Input_{(480p,15fps)}-\Input_{(480p,10fps)}}{15fps-10fps} \otimes \frac{\Delta \Output}{\Delta \Input}\bigg|_{\Input=\Input_{(480p,10fps)}},\\
\frac{\Output_{(720p,10fps)}-\Output_{(480p,10fps)}}{720p-480p} &\approx \frac{\Input_{(720p,10fps)}-\Input_{(480p,10fps)}}{720p-480p} \otimes \frac{\Delta \Output}{\Delta \Input}\bigg|_{\Input=\Input_{(480p,10fps)}},
\end{align*}
\end{@empty}
where $\otimes$ represents inner product and $\frac{\Delta \Output}{\Delta \Input}|_{\Input=\Input_{(480p,10fps)}}$ is \dnngrad of the  current configuration $(480p,10fps)$ on the current source data $\Data$.

Importantly, Figure~\ref{subfig:gradient-after} shows that to calculate \outputgrad, \name saves extra GPU inference by decoupling \outputgrad and re-using the backpropagation results for different knobs.
This example has two knobs, thus the saving may seem marginal, but our evaluation shows more savings when \name is used to adapt more knobs together in more realistic DNN analytics systems (Figure~\ref{fig:fine-grained-knobs}). 



% \kt{\hl{Claim we are the first one who uses backprop for config adaptation here. I think it's better to mention saliency-based works  in related work rather than here.}}
We want to clarify that while \name is the first to leverage DNN differentiability for configuration adaptation, DNN differentiability has already been widely used in DNN training, DNN interpretability, and localization of areas most responsible for the DNN output~\cite{vision-saliency-1,vision-saliency-2}.
It should also be pointed out that \dnngrad differs from the traditional notion of ``saliency'' used in video compression~\cite{fischer2021saliency,hadizadeh2013saliency}, in that \dnngrad is derived directly from a particular DNN to capture how the input influences the DNN output. 

% Note that \name is the first system that leverages the differentiability of DNNs for configuration adaptation, though not the first one that leverages differentiability of DNNs in DNN serving system\footnote{For example, in computer vision community, people use backpropagation to localize which areas of the objects are responsible for the DNN output~\cite{vision-saliency-1,vision-saliency-2}.}. 
% We also aware that there is a recent trend in multi-media community that compress videos by estimating the saliency (\ie the regions in the input video that may contain objects) and encoding these regions in encoding quality.
% Also, there is a line of work from multi-media community~\cite{fischer2021saliency,chen2022context} that leverages saliency estimators to  estimates the areas in the DNN input that contain objects, and then enocde these areas in higher encoding quality so that the objects in these areas can be better detected.
% The notion of saliency may conceptually seems similar to \dnngrad (as both highlight the areas that are related to objects), 
% Also, conceptually \dnngrad is similar to saliency (the areas in the input video that may contain objects) in multi-media community that 

% However, these saliency estimato
% \kt{1. Backpropagation is used in model serving system for explanation.
% But we are the first one to use it for config adaptation
% 2. MM community use saliency to compress video.
% It may seems similar, but our saliency is aware of the final DNN and they are not (drawbacks).}
% \mypara{\dnngrad v.s. existing saliency estimators}
% \dnngrad captures the saliency of the DNN (defined as a map that quantifies the importance of different areas in the DNN input), where there are existing works that also serves the same purposes~\cite{accmpeg,dds,eaar,vigil,fischer2021saliency}.
% However, \dnngrad outperforms existing saliency map estimation algorithms.
% \begin{packeditemize}
%     \item Compared to generating saliency using cheap models~\cite{accmpeg,vigil,fischer2021saliency}, \dnngrad prioritizes those objects according to the likeliness of changing the number of objects detected (where cheap models may mark all objects~\cite{fischer2021saliency} as salient or wrongfully assign saliency to those objects that are detected with high confidence~\cite{accmpeg}).
%     \item One may also generate saliency based on region proposals (an intermediate result generated alongside DNN inference that includes regions potentially containing objects). Compared to this approach, \dnngrad can further rank the pixels inside each object, where this approach will mark all pixels inside an object as salient/non-salient.
% \end{packeditemize}

% \kt{Compare our saliency v.s. others saliency here}


% \mypara{Assumption to configuration knobs}





% First, 
% Second, \dnngrad further prioritizes the pixels inside and outside the object bounding boxes according to the likeliness of changing the number of objects detected, where 

% However, \name calculates this saliency using backpropagation instead of using cheap saliency estimators, allowing \name to derive a metric (\outputgrad) that directly correlates with inference accuracy.
% The cheap saliency estimators fail to correlate with inference accuracy in some cases.
% For example, one may use cheap neural network to estimate saliency~\cite{accmpeg,?,?}.
% However, these cheap saliency estimators will \kt{finish this.}






% Specifically, \name measures \outputgrad by how much a small change in the current value of each knob \textit{flips} the DNN-returned confidence scores from below (or above) the confidence threshold to above (or below). 
% It does not impose an extra burden on the applications to require them to expose confidence scores and confidence thresholds since most of the applications already expose confidence scores to indicate the uncertainty of DNN outputs and use confidence thresholds to filter out DNN outputs with low confidence. %those uncertain results returned from the DNN.
% Statistically, more changes in the ``near-confidence-threshold'' DNN outputs will likely cause more changes in the inference accuracy (as will be elaborated in \S\ref{subsec:correlation})\footnote{This correlation does \textit{not} assume that a confidence score always directly indicates the accuracy of its corresponding detection/classification results.}.
% % \outputgrad correlates with how much the accuracy \textit{changes} with knobs 
% Intuitively, this is because the confidence threshold determines whether a detection or classification result is accepted (as part of the accuracy calculation) or rejected (thus having no effect on the accuracy).




% \pagebreak


% We advocate that the adaptation system for DNN-based analytics should provide a new abstraction: \outputgrad, which estimates the gradient of DNN output with respect to individual knobs.
% We define \outputgrad on a designated knob as the change of the DNN-returned \textit{confidence scores} around (both below and above) the \textit{confidence threshold}, divided by the small amount of change of the knob.
% % when changing this knob by a little.
% This definition requires the application to expose the confidence scores inside their inference results and the confidence threshold used to filter the results.
% For most of the applications, the DNN-returned confidence scores and confidence threshold are naturally available, since most of the applications use confidence scores to quantify the uncertainty of the DNN inference results. The application then filters those results with low confidence scores (as these results may contain spurious results) through a confidence threshold.

% We found that \outputgrad nicely correlates with how much the inference accuracy changes with the knobs.
% Intuitively, this is because the confidence threshold determines whether a detection or a classification result is accepted (and thus participating in the accuracy calculation) or rejected (and thus having no effect on the accuracy).
% Thus, more changes of confidence scores near the confidence threshold will likely cause more changes on the inference accuracy.

% This gradient information can help us quickly adapt to the optimal configuration, 
% % among a large number of configurations 
% by assigning more resources to those knobs with high \outputgrad to improve the accuracy and cut the resource usage of those knobs with low \outputgrad to save resource usage (without hurting the accuracy).
% As shown in Figure~\ref{fig:compare}, \name quickly find the optimal configuration through \outputgrad, while the profiling-based approach needs to profile all configurations to obtain the optimal one, and the output-driven approach adapts slowly.




% \begin{figure*}[t]
%     \centering
%     \includegraphics[width=2.2\columnwidth]{figs/workflow.pdf}
%     \caption{Workflow of \name. \kt{$\Delta resolution$ $240p, 1fps$ }people won't immediately realize it's adding. Need some handholding, picking the new configuration}
%     \label{fig:workflow}
% \end{figure*}



% To quickly adapt to optimal configuration with no extra inference, \name calculates the \textit{gradient} of accuracy with respect to the knob (hereinafter \outputgrad).\jc{i suppose you will clean up all \accgrad and replace them with \outputgrad?}
% We define \accgrad as the accuracy change divided by the knob value change when changing the knob value by a little.

% With this gradient, \name can quickly adapt to the optimal configuration in a large configuration space by granting more resource to the knobs with high \accgrad to improve the accuracy, and cutting the resource usage of those knobs with low \accgrad to reduce the resource usage without hurting accuracy.

\tightsubsection{Adaptation by \outputgrad-based gradient ascent}
\label{subsec:gradient-ascent}


% \jc{(1) 3.2 and 3.3 are still a bit too abstract. please use a concrete example like the one in 31
% (2) it’s not clear from 32 (upfront) why configgrad-based gradient ascent can adapt quickly. this should be upfront, not embedded or in the end
% same thing with 33. it’s unclear why this is a smart design
% (3) i dont see the assumptions in 31, 32, 33 be explicitly called out and justified.. did i miss them?}
% \kt{I explicitly called out the assumptions in 31. I will deprioritize other issues before Sunday.}

With \outputgrad, 
% To adapt configurations using \outputgrad, 
\name runs gradient ascent (depicted in Figure~\ref{fig:workflow}) to converge to a near-optimal configuration.
% First, we partition the input data stream (\eg video frames) into {\em adaptation intervals}, each of one second.
In each adaptation interval, we perform inference using the current configuration $\Config_{cur}$ (\eg current resolution and frame rate), compute \outputgrad, and then use the following strategy to select a new configuration $\Config$ based on \outputgrad. 

The goal of \name's gradient ascent is maximizing a weighted sum between \summary (number of elements with scores over the confidence threshold) and resource usage (we will discuss alternative formulations shortly):

\vspace{-0.4cm}
\begin{@empty}
\small
\begin{align}
{\color{black}\underbrace{\highlight{white}{$\Output_{\Config}(\Data)$}}_{\text{\sf \footnotesize \textcolor{black!85}{\summary}}}}-\lambda {\color{black}\underbrace{\highlight{white}{$\Resource(\Config)$}}_{\text{\sf \footnotesize \textcolor{black!85}{resource usage}}}} \label{eq:objective}
\end{align} 
\end{@empty} 
Here, $\Resource(\Config)$ is the resource usage (in either bandwidth or GPU cycles, defined per application) of \Config.
The hyperparameter $\lambda$ governs the tradeoff between accuracy and resource usage: higher $\lambda$ will emphasize resource-saving and lower $\lambda$ will emphasize accuracy improvement.
\hl{Note that we will vary $\lambda$ and study its impact in \S\ref{sec:eval}.}
% As shown in prior work, for most configuration knobs (\eg frame rate, resolution, etc), $Resource(\Config)$ can be accurately pre-profiled and does not vary with input content as much as inference results.

Given the current configuration $\Config_t$ at the interval $t$ and the \outputgrad $\Grad_t$ (a vector of each knob's \outputgrad), the new configuration used for the next interval $t+1$ should be the one that maximizes the improvement of the objective. 
Formally, we can express it by 

\vspace{-0.4cm}
\begin{@empty}
\small
\begin{align}
\Config_{t+1}=\textrm{argmax}_{\Config}{\color{black}\underbrace{\highlight{white}{$(\Config-\Config_t)\cdot \Grad_t$}}_{\text{\sf \footnotesize \textcolor{black!85}{change in \summary}}}}-\lambda {\color{black}\underbrace{\highlight{white}{$(\Resource(\Config)-\Resource(\Config_t))$}}_{\text{\sf \footnotesize \textcolor{black!85}{change in resource}}}} \label{eq:gradient}
\end{align}
\end{@empty}
% $\Config_{t+1}=\textrm{argmax}_{\Config} (\Config-\Config_t)\cdot Grad_t-\lambda (\Resource(\Config)-\Resource(\Config_t))$
The new configuration $\Config_{t+1}$ will be used for the next adaptation interval. 
Following prior work~\cite{chameleon,dds,reducto}, we pre-profile the resource usage of each configuration $\Resource(\Config)$, which might vary with source data, but the relative difference among them has little variance.

In many applications, the objective in Eq.~\ref{eq:objective}, which linearly combines resource usage and \summary, is less reasonable than optimizing \summary with a fixed constraint on resource usage.
For instance, one may choose to maximize \summary (which relates to accuracy as explained shortly), conditioned on the bandwidth usage of the configuration within a budget.
Figure~\ref{fig:workflow} shows an example of how \name's gradient-based adaptation process works in the vehicle detection example.
% We will still use the vehicle detection example, where a traffic camera streams its video data to a GPU-equipped server to determine which frame contains vehicles.
In each adaptation interval, the sensor encodes the video in an adaptation interval using the current configuration (frame rate and resolution) and sends it to a DNN running on a GPU-equipped server.
The server receives this video and runs DNN inference to get the inference results and runs backpropagation to get \dnngrad and send it back to the sensor. 
While the server runs DNN inference, the sensor runs encoding multiple times with different to obtain \inputgrad (the change in DNN input with respect to each knob).
Once the sensor receives \dnngrad, it uses Eq.~\ref{eq:grad-decouple} to calculate \outputgrad.
It then runs the gradient ascent strategy in Eq.~\ref{eq:gradient} to adapt the configuration and uses the new configuration in the next interval. 
% \jc{kuntai, remember to justify why resource usage of a config can be known in advance? what about the frame-diff threshold in reducto?}

% the encoded video that the camera sent, decodes this video, and runs DNN inference to obtain the inference results.
% Then, the server calculates the saliency using the backpropagation and streams the saliency back to the camera.
% Finally, the camera receives the saliency, calculates \outputgrad, and adapts the configuration accordingly.
% \jc{kuntai, please update figure~\ref{fig:workflow} to include the gradient-based adaptation process.}

% 



\tightsubsection{Caveats and benefits}
\label{subsec:limitation}

While our evaluation shows \name's gradient-ascent strategy performs well for a wide range of DNN tasks, data types, and configuration knobs, it is important to understand its limits and why it works in practice. 

\mypara{Why \name improves accuracy}
Second, in the objective of gradient ascent (Eq.~\ref{eq:objective}), the change in the first term of \summary (\Output) should reflect the change in inference accuracy.
This connection may be intuitively true since a significant change in the inference results is often accompanied by a substantial change in accuracy.
That said, a big change in the \summary may indicate either more increase or decrease in accuracy. 
To decide the direction of change, we use the empirical observation that when a change in knob value increases the resource usage, the impact on inference accuracy should be positive (\eg higher encoding resolution leads to higher bandwidth usage and likely more accurate inference, or higher frame rate leads to higher GPU usage and likely more accurate inference). 

Figure~\ref{fig:accuracy-proxy} empirically verify whether the change in output ($\Delta \Output_\Config(\Data)$) is proportional to the change in accuracy (\ie the accuracy of the configuration $\Config$, minutes the accuracy of current configuration).
We pick three configuration knobs (frame sampling rate, resolution, quantization parameter) that are widely used by prior work~\cite{chameleon,casva,awstream,videostorm,vstore,mcdnn} and a 6-second video chunk to verify the correlation between DNN output change and accuracy change on all configurations (125 configurations in total).
Figure~\ref{fig:accuracy-proxy} shows that on one 9-second video chunk, the change of DNN output (X-axis) nicely correlates with the accuracy change (Y-axis), with a Pearson coefficient of 0.702.


\mypara{Why \name converges}
First, like other gradient-based heuristics, \name does not guarantee to always converge to a global optimum configuration. 
That said, we empirically observe that the relationship between configuration $\Config$ and their \summary ($\Output$) and resource usage ($\Resource$) is mostly {\em concave}.
As a result of the concavity, gradient-ascent can {\em eventually} converge to a global optimal configuration. 
The concavity can be intuitively understood that as the configuration uses more (compute/network) resources, the change in the input to the DNN becomes more marginal, and so does the DNN output.
For example, as a video analytic system increases the video encoding resolution, the pixel change becomes more marginal (mostly on ``high-frequency'' details), causing the DNN output to stabilize (objects' confidence scores will change more slowly and less frequently cross the confidence threshold, leading to fewer newly detected objects).




Another potential reason for \name to fail to converge is the evolution of source data content---the \outputgrad calculated from one adaptation interval may not apply to the next adaptation interval due to temporal change in the content. 
That said, we observe that \name converges to the optimal configuration within 3-5 intervals (seconds) as shown in Figure~\ref{fig:converge-fast}, and within 1-2 intervals for configurations that require frequent adaptation (such as macroblock-level encoding quality).
Thus, as long as the best configuration last for a few seconds, \name can identify the best configuration faster than profiling-based methods.
% Both profiling-based methods and \name require the continuity of resource/accuracy relationship at a timescale of several to 10s of seconds. 



% explain it with the example in fig 6. (need to update fig 6)
% caveats: 
% why not local optimum: concavity => connection with newton's method
% why leading to higher accuracy
% content change 

% limitation: not applicable to dnn knobs





% \mypara{\outputgrad correlates with accuracy}
% A key question is how \outputgrad is related to inference accuracy.
% We found that there is a statistical correlation between \outputgrad and the inference accuracy of other configurations. 
% This is because \outputgrad captures the change in the inference results, and a significant change in the inference results is often accompanied by a substantial change in accuracy.

% We found that \outputgrad statistically correlates with the inference accuracy.
% This is because \outputgrad captures the change in the inference results, where a large change in inference results likely corresponds to a large change in accuracy.

\begin{comment}
However, the change in the inference results cannot determine whether the accuracy improves or decreases.
To handle this issue, we make an assumption that for a designated knob $\Knob_i$, increasing it while keeping other knobs fixed will either statistically not decrease the accuracy (we denote this case as $sgn(i)=1$) or not increase the accuracy (we denote this case as $sgn(i)=-1$).
We found that this assumption holds for a wide range of knobs (see Table~\ref{tab:rich-set-of-knobs}), as increasing these knobs causes the resource usage pipeline increases/decreases and thus the corresponding accuracy also increases/decreases.
For example, increasing the frame rate while fixing the  resolution in the video analytics system typically leads to more accurate inference results as more frames are analyzed. 
Similarly, increasing the resolution while fixing the frame rate enhances the clarity of the boundaries of the object, and is likely to generate more accurate inference results.

% To give a concrete example, when tuning the frame rate and resolution of the aforementioned video analytic system, increasing the frame rate while fixing the resolution typically leads to more accurate results as more frames are being analyzed. 
% Similarly, increasing the resolution while fixing the frame rate also makes the detail of the video (like the boundary of the vehicles) clearer and thus is likely to generate more accurate inference results.

Using this assumption, we then derive the (signed) output change with respect to the current configuration (frame rate $\Knob_1=20fps$, resolution $\Knob_2=480p$) using the following formula:

\vspace{-0.3cm}
\begin{@empty}
\footnotesize
\begin{equation*}
\Delta \Output_\Config(\Data)= \sum_{i=1}^n \left|\frac{\Delta \Output}{\Delta \Knob_i}\right| \cdot sgn(i) \cdot (\Knob_i - \Knob_{i,cur}) =  0.08 \cdot (\Knob_i - 10\textrm{fps}) + 0.01 \cdot (\Knob_2 - 480\textrm{p}) 
\end{equation*}
\end{@empty}
% To examine the correlation between \outputgrad and the accuracy of other configurations, we calculate the change in accuracy with respect to the change of the current configuration ($O(res=2,fps=2)$) using the following formula
% \begin{@empty}
% \footnotesize
% \begin{equation*}
% \Delta O(res,fps) = \frac{\Delta O}{\Delta (res, fps)} \cdot \Delta (res, fps) = \frac{\Delta O}{\Delta res}(res-2) + \frac{\Delta O}{\Delta fps}(fps-2).
% \end{equation*}
% \end{@empty}
% And check if the output change is proportional to the accuracy change

  



And then, we verify whether the change in output ($\Delta \Output_\Config(\Data)$) is proportional to the change in accuracy (\ie the accuracy of the configuration $\Config$, minutes the accuracy of current configuration):
% \begin{@empty}
% \footnotesize
% \begin{equation*}
% \Delta \Output(\Input, \Config) \propto Acc(\Output(\Input, \Config)) - Acc(\Output(\Input, \Config_{cur})),
% \end{equation*}
% \end{@empty}
% where $Acc$ represents the inference accuracy.
We pick three configuration knobs (frame sampling rate, resolution, quantization parameter) that are widely used by prior work~\cite{chameleon,casva,awstream,videostorm,vstore,mcdnn} and a 6-second video chunk to verify the correlation between DNN output change and accuracy change on all configurations (125 configurations in total).
As shown in Figure~\ref{fig:accuracy-proxy}, on one 9-second video chunk, the change of DNN output (X-axis) nicely correlates with the accuracy change (Y-axis), with a Pearson coefficient of 0.702.


\end{comment}






% that maximally improves the change in DNN output $\Delta \Output(\Data,\Config)$ under the resource budget.
% As the change in DNN output statistically correlates with the change in accuracy, this will likely maximize the accuracy of the new configuration $\Config$.
% We then use this configuration for the next adaptation interval.
% identify a new configuration that maximally improves accuracy without exceeding the resource budget.
% We use this new configuration for the next adaptation interval, and at the end of the interval, we repeat the same adaptation steps.
% As the content of the input data is continuous, the new configuration is likely to generate more accurate inference results compared to the original configuration.
% Note that 
% As a result, the inference results of the new configuration are likely to be more accurate than the current configuration

\mypara{Why \name beats alternatives}
By performing gradient ascent based on \outputgrad, \name outperforms previous work on all three requirements (\ie adapt frequently, converge to a near-optimal configuration, and generalize to different types of knobs and analytic tasks).
First, compared to profiling-based work, \name adapts much more frequently (as \name updates its configuration \textit{at every second} but profiling-based work updates its configuration once every minute~\cite{awstream}) and earlier (as \name adapts to the change of input content right at the next adaptation interval but the profiling-based work need to wait till the next profiling).
Second, compared to the heuristics-based approach, \name can adapt to a near-optimal configuration, where the accuracy of the heuristics-based approach can be much lower than the optimal configuration.
Third, \name can generalize to different applications and DNNs (as \name only assumes the DNNs to be differentiable, which holds for almost all DNNs) and a wide range of knobs (as \name applies to most of existing knobs, see Table~\ref{tab:rich-set-of-knobs}).




% \tightsubsection{Limitations}
% \label{sec:limits}

\mypara{Limitation} 
% We acknowledge that \outputgrad only works for configuration knobs that affect DNN input (\ie input preprocessing part of a DNN analytics system).
The idea of decoupling \outputgrad assumes that the configuration knobs only influence DNN input (\ie knobs of input preprocessing part of a DNN analytics system).
A wide range of knobs falls into this assumption (\eg video codec encoding parameters~\cite{awstream,vstore,videostorm,chameleon,casva}, frame filtering thresholds~\cite{glimpse,reducto,filterforward}, fine-grained encoding quality assignment~\cite{dds,eaar,accmpeg,vigil}, see  Table~\ref{tab:rich-set-of-knobs} for a list of existing knobs that \name covers).
That said, it does {\em not} include knobs that modify/select the final DNN itself.

% However, this assumption makes \name not applicable to knobs that alter the DNN itself, such as retraining the DNN weights based on the current input~\cite{ekya,noscope,mcdnn}.
% In some sense, both the DNN customization approach and \name are adapting to the varying content in the input data stream.
% However, in order to maintain high accuracy, the DNN customization approach needs to retrain the DNN when the input content varies (which adds high GPU overhead).
% In contrast, \name adapts the knobs as part of the DNN-based inference process and only reuses the DNN inference result (for backpropagation), which is much more lightweight.


% \jc{need a paragraph to explain customization of specific applications, and why it still works under evolving content}
% overall, why it's better?

% Our gradient-ascent-based approach has its own caveats as it cannot guarantee that (i) the search will quickly converge in a few steps, and (ii) the search may get stuck in a local optimal.
% To answer this question, we measure how fast \name can converge to a near-optimal configuration (a top-1\% configuration).
% \kt{Not sure how to answer this question}





% The intuition behind the fast convergence is that as long as the \outputgrad with respect to one configuration knob is non-zero, tuning that knob will likely improve accuracy.
% % Further, as the input data is constantly changing over time, it is less likely for a local optimal to persist.
% Thus, \name is unlikely to be stuck in a local optimum, which corroborates our empirical observation of \name.
% \kt{Other potential concerns: (1) why treat discrete configs as almost continuous variables, (2) why the better configuration at this second will likely lead to a better result at the next second, (3) what if the content is noisy and makes the gradient noisy}



% However, directly calculating \outputgrad needs a substantial amount of extra inference.
% If we calculate \outputgrad knob-by-knob, we will need to calculate the accuracy change by changing one knob at a time.
% The amount of GPU compute will grow at least linearly with more knobs. 
% % This is because calculating \outputgrad in a knob-by-knob manner (\ie calculate the accuracy change by alternating the value of one knob while the value of other knobs remaining unchanged, and repeat this process for all knobs) results in extra inference (see \S\ref{subsec:calculate-accgrad} for details).
% % Moreover, more knobs will lead to more inference and reduces the applicability of \outputgrad on a large set of knobs.

% \mypara{Leveraging DNN differentiability} To reduce such overhead, \name harnesses the differentiability of the DNN to calculate \outputgrad with constant GPU overhead and with no extra inference.
% Intuitively, in order to calculate how DNN output changes with respect to the knob change (\ie \outputgrad), we can calculate how DNN output changes with respect to the DNN input change, and then study how DNN input changes with respect to the knob change.
% % how changing system knobs alters the DNN input, and then calculate how changing the DNN input alters the DNN output.
% Formally, we denote the configuration (\ie the values of all knobs) as $c$, the DNN input as $I$, and the DNN output as $O$. The intuition above can be written as the following chain rule:
% \begin{equation}
%     \frac{\partial O}{\partial c} = \frac{\partial O}{\partial I} \cdot \frac{\partial I}{\partial c},
% \end{equation}
% The first term $\frac{\partial O}{\partial I}$ can be obtained via backpropagation (a constant GPU overhead, but no extra inference is incurred as backpropagation reuses the computation graph created by existing DNN inference).
% The second term $\frac{\partial I}{\partial c}$ can be calculated in a knob-by-knob manner but since it only computes the DNN input (not DNN inference), it does not have extra GPU overhead. 
% without incurring DNN inference as calculating the DNN input change does not require DNN inference.

% The key enabler for \name to remove the extra inference is the following two observations to existing knobs for DNN-based analytic systems.



% that the knob only alters the DNN input. does not cover those knobs that alter the DNN itself, 




% \begin{enumerate}
%     \item \textit{Accuracy-Resource Property}: For a large class of knobs,  increasing the value of one knob always results in spending more (or less) resource, and also making the corresponding inference results more (or less accurate).
%     The amount of accuracy improvement (or degradation) depends on how much the knob increase alters the inference results.
%     \item \textit{Black-box Property}: Most of the knobs treat DNN as a black box and change the inference results solely by changing the DNN input.
% \end{enumerate}

% By leveraging the first assumption, \name estimates the accuracy change through inference results change, thus avoid calculating the inference results under the most expensive configuration as the ground truth.
% By leveraging the second assumption, \name decouples the gradient using chain rule and avoid the inference on the new configurations.


% Note that not all knobs satisfies the two properties above. We list some examples in Table \ref{??} and some non-examples down below.

% For \accres, we find that the sensing configuration knobs that directly change the raw sensed data, like the aperture and the ISO of the camera, the Gamma correction value of the camera, the positioning direction of the directional microphone, etc., do not satisfy \accres as varying these knobs typically have little impact on the encoded file size and the encoding cost of the input data.
% However, the sensing configuration knobs are typically pre-configured (like the positioning direction of the microphone) or self-adapted (like the aperture and the ISO of the camera) by the sensor.
% As a result, these knobs are typically not dynamically programmable so \name cannot change these knobs anyway.

% The non-examples for \blackbox are the knobs that optimize DNN inference, like DNN selection~\cite{chameleon} and DNN customization~\cite{noscope,ekya,mcdnn}.
% We acknowledge the effectiveness of these knobs in terms of saving GPU cost.
% However, we argue that these knobs requires the system to change or replace the DNN in real-time, which make them not generally applicable in all deployment settings (\eg when performing inference through third-party API).
% % However, switching or editing the DNN may result in significant overhead (\eg some other components may be customized for this DNN and may require retraining upon DNN changing~\cite{accmpeg}) or even not doable (\eg when performing inference through cloud API).




% \tightsubsection{Workflow of \name}














% We demonstrate the workflow of \name using the example of traffic cam-based vehicle detection
% Figure~\ref{fig:workflow} demonstrates the workflow of \name.
% \name assumes that the analytic systems are made up of two components: \textit{input processing} and \textit{DNN-based inference}.
% First, \name processes the data stream $x$ through input processing using the current configuration $c$ to obtain the DNN input $I$.
% \name then forwards $I$ through the DNN and obtain the DNN output $O$.
% After that, \name performs DNN backpropagation and obtains the gradient $\frac{\partial O}{\partial I}$.
% In the meantime, \name alters every knob in $c$ and obtains the corresponding change on the DNN input.
% \name then stacks together the DNN input changes of individual knobs ($\frac{\partial I}{\partial c}$) and 
% % \name then stacks these DNN input changes to obtain $\frac{\partial I}{\partial c}$ and 
% multiplies it with $\frac{\partial O}{\partial I}$ to obtain \outputgrad $\frac{\partial O}{\partial c}$.
% Finally, \name updates the configuration $c$ according to the \outputgrad.
% We will present the details of each step in the next section.









% \subsection{Accuracy gradient as a better feedback}

% \begin{itemize}
%     \item We find that: how much the analytic accuracy change differs if we change different knobs is essentially asking what is the \textit{gradient} of analytic accuracy with respect to the knob values.
%     \item With the accuracy gradient, we can better predict the analytic accuracy of those knob values we did not explore yet.
% \end{itemize}

% Our goal is to calculate the gradient of accuracy with respect to knobs (we call this gradient \textit{accuracy gradient}) by only evaluating the system under one configuration.

% Accuracy gradient enables us to better predict the accuracy of different configurations under similar video content.
% As a result, one can pick a chheaper configuration while still achieving the same accuracy with accuracy gradient.


% \begin{comment}

% \subsection{Programming interface of \name}


% \begin{figure}
%     \centering
%     \includegraphics[width=1\columnwidth]{figs/raw-input-inference.jpg}
%     \caption{\name handles those hyper-parameters that preprocess the input to the DNN.}
%     \label{fig:raw-input-inference}
% \end{figure}



% \subsection{API of HPs} 

% As shown in Figure~\ref{fig:raw-input-inference}, \name abstracts the underlying AI systems into two stages.
% In the preprocessing stage, the AI system pre-processes the raw sensing data to obtain the input to the DNN.
% In the inference stage, the DNN performs inference and obtain the analytic results.
% \name focuses on those HPs for preprocessing stage (we will show most of the HPs fall into this category in \S\ref{subsec:hp-examples}, together with some example HPs that do not belong to this category).
% As the preprocessing does not incur the compute-intensive server-side DNNs, we assume that this step can be locally done at the camera.

% Based on this observation, the programming interface of \name towards HPs are:
% \begin{small}
% \begin{verbatim}
% prep(Data raw, List hps)-> (Data input, Bytes encoded)
% proxy(Result result) -> Float pseudo_acc
% \end{verbatim}
% \end{small}

% The first function \texttt{prep} pre-processes the raw sensed data \texttt{raw} based on a list of HPs \texttt{hps}, and return the codec-encoded byte stream \texttt{encoded} and the input data \texttt{input} that server-side DNN will receive.

% The second function aims to provide a differentiable proxy towards accuracy (since most of the existing accuracy function is not differentiable).
% As most of the DNNs will return confidence scores to describe the confidence of the analytic results the DNN derives, we use the sum of the confidence scores as the default proxy.
% This complies with recent computer vision advances on evaluating the quality of inference results.

% Further, we empirically verify this assumption on different types of HPs and different videos.


% \subsection{Examples}
% \label{subsec:hp-examples}


% This assumption precludes those HPs that directly changes server-side DNN (\eg customizing the server-side DNN or switching between different server-side DNNs).
% That said, the vast majority of HPs, including HPs of traditioanal data encoding codecs (\eg frame rate, resolution, quantization parameters etc), DNN-based encoding codec (\eg feature compression, super resolution), fine-grained data quality assignments (\eg region-of-interest selection, macroblock encoding quality selection), sensor-side data filtering (\eg filtering the frames through cheap object detector or through cheap feature extractors) still fit in our assumption. 



% % \mypara{API of DNNs}
% % We require that the DNN to implement two APIs:
% % \begin{small}
% % \begin{verbatim}
% % inference(Data input)-> Result result
% % backprop(Result result, Function f)-> Data grad
% % \end{verbatim}
% % \end{small}



% \subsection{Workflow of \name}

% Contrast between conventional workflow and ours workflow

% \end{comment}







% \subsection{Workflow and API of \name}
% \kt{Goal: how to use the API in our system to calculate accuracy gradient}

% \begin{figure}
%     \includegraphics[width=1\columnwidth]{figs/workflow.jpg}
%     \caption{Workflow of \name \kt{Plot this figure in a "call stack" way, MAKE THE FONT LARGER}}
%     \label{fig:workflow}
% \end{figure}

% \mypara{Workflow of \name} Based on the approach above, we present the workflow of \name in Figure \ref{fig:workflow}.


% Our system enables the application to obtain the gradient of accuracy with respect to the knobs through the following API:
% $$AccGrad = calc(V_t, \{knob_i\}_{i=1}^n)$$

% \mypara{Towards knobs}

% $knob'_i = reduce(knob_i)$
% This reduce the knob to lower knob value

% \mypara{Towards DNN}
% We require the DNN to implement two APIs:
% \begin{packeditemize}
%     \item \texttt{result = inference(V)}
%     \item \texttt{saliency = backprop(result, grad)}
% \end{packeditemize}

% \mypara{Towards application}
% We require the application to implement:
% \begin{packeditemize}
%     \item \texttt{encode(V, knobs)} This one should be locally done on the camera
%     \item \texttt{proxy(results)}
% \end{packeditemize}


% \subsection{How to use the API}






% \subsection{Reduce the cost of accuracy gradient}


% \mypara{Accuracy gradient sampling}


% \mypara{Accuracy gradient compression}



==> overview_v3.tex <==

% \begin{figure*}[t]
%     \centering
%     \includegraphics[width=1.5\columnwidth]{figs/workflow.pdf}
%     \caption{Workflow of \name.}
%     \label{fig:workflow}
% \end{figure*}



% \begin{figure}[t]
%     \centering
%     % \includegraphics[width=0.5\columnwidth]{figs/placeholder-eval-overall-1.pdf}
%     % \subfloat[][\centering{Object detection\\~~~~(Dashcam)}]
%     % {
%     %     \includegraphics[width=0.24\textwidth]{figs/detection_dashcam_FPN.pdf}
%     %     \label{subfig:1}
%     % }
%     \subfloat[][Profiling]
%     {
%         \includegraphics[width=0.32\columnwidth]{figs/behavior_profile.pdf} 
%         \label{subfig:1}
%     }
%     \subfloat[][Output-based]
%     {
%         \includegraphics[width=0.32\columnwidth]{figs/behavior_output.pdf} 
%         \label{subfig:1}
%     }
%     \subfloat[][OneAdapt]
%     {
%         \includegraphics[width=0.32\columnwidth]{figs/behavior_oneadapt_arrow.pdf} 
%         \label{subfig:1}
%     }
    
%     \tightcaption{Contrasting \name with profiling-based approach and output-based approach. \name quickly approaches the optimal point via the gradient vector, while the profiling-based method requires a high amount of extra inference to derive the optimal configuration, and the output-based method approaches the optimal configuration slowly.}
%     \label{fig:compare}
% \end{figure}


% \begin{figure}[h]
%     \includegraphics[width=1.15\columnwidth]{figs/gradient.jpg}
%     \caption{Gradient \name.}
%     \label{fig:workflow}
% \end{figure}

% \begin{figure*}[h]
%     \centering
%     \includegraphics[width=1.5\columnwidth]{figs/timeline.jpg}
%     \caption{Workflow of \name. \kt{Place a overall workflow figure here.} }
%     \label{fig:workflow}
% \end{figure*}


% \begin{figure*}[h]
%     \includegraphics[width=2.4\columnwidth]{figs/adaptation-time-series.pdf}
%     \caption{Adaptation behavior of \name}
%     \label{fig:workflow}
% \end{figure*}

% \begin{packeditemize}
%     \item Sketch three requirements (1). adapt frequently (2). reach a near-optimal configuration (3). be applicable to a range of configs \& apps.
%     \item \S 3.1
%     \item Introducing \outputgrad 
%     \item Calculating \outputgrad with no extra inference. Need two figures here. 1). Show what is backpropagation 2). show how is backpropagation saves cost.
%     \item Correlation between \outputgrad and accuracy.
%     \item \S 3.2
%     \item Optimizing accuracy through gradient ascent.
%     \item This gradient-ascent-based algorithm allows us to simultaneously achieve 3 objectives.
%     \item Talking about its caveats
%     \item \S 3.3.
%     \item Run people through an end-to-end example, where the sensor and the server are separated by network.
%     Figure: a timeline figure between the sensor and the server Key highlights: when the inference results are obtained, and when the configuration is updated.
% \end{packeditemize}





\jc{Outline:
if you agree, how about the following order? you will
introduce the optimization goal first (current eq 2) and
then introduce ConfigGrad, and
before explaining how to calculate ConfigGrad (currently the beginning of 3.2), you should explain why ConfigGrad can help the optimization goal. (this needs some math rigor)
finally, explain how to calculate ConfigGrad and how to pick the next config
}
\tightsection{Design of \name}
\label{sec:design}
% \tightsection{\outputgrad}
% \jc{Junchen can you check this part? I did a full rewrite to Sec 3.1}

We present \name, a configuration adaptation system that aims at improving along the three requirements mentioned above --- frequent adaptation to near-optimal configuration on various configuration knobs. %---over prior solutions.

The basic idea of \name (illustrated in Figure~\ref{fig:adaptation-behavior}) is to calculate frequently
% The key for \name to meet the three requirements is to calculate 
the {\em gradient} of how DNN inference output changes with each configuration knob, which we refer to as the {\em \outputgrad}.
Using the up-to-date estimate of \outputgrad, \name incrementally updates the configuration to improve the DNN inference results but still stays in the (compute/network) resource budget or maximally reduces the resource usage with minimum change on the DNN inference results.
% Figure~\ref{fig:adaptation-behavior} illustrates an example: after a change of input data, \name can adapt more frequently and gradually converge to a near-optimal configuration.


We begin by defining \outputgrad (\S\ref{subsec:outputgrad}) and presenting the key insight that the inherent differentiability of DNNs enables fast calculation of \outputgrad without extra DNN inference (\S\ref{subsec:differentiability-outputgrad}).
Then we introduce \name's gradient-ascent strategy based on \outputgrad (\S\ref{subsec:gradient-ascent}) and state the caveats and benefits of \name (\S\ref{subsec:limitation}).

% changes the configuration to another configuration that meets the (compute/network) resource budget and greatly improves accuracy.\jc{confirm with kuntai}
% to improve accuracy within the resource budget. 



% after the content of the input data changes.
% that allows operators to achieve the following three requirements simultaneously:
% \begin{packeditemize}
%     \item Adapt frequently
%     \item Reach a near-optimal configuration
%     \item Apply to a wide range of configurations and applications
% \end{packeditemize}


% \subsection{Modeling of knobs}

% \name focuses on handling a subset of knobs that satisfies the following two properties:

% \begin{enumerate}
%     \item \textit{\accres}: For each knob, there exists one direction (either increasing or decreasing), if \name fix other knobs and change this knob according to this direction, the resource consumption and the accuracy statistically increases.
%     % (we assume that this direction is increasing the knob value by default) if changing the value of one knob result in spending more (or less) resource, the corresponding inference results also become more (or less) accurate.
%     \item \textit{\blackbox}: Most of the knobs treat DNN as a black box and change the DNN input. We illustrate this point in Figure~\ref{??}.
% \end{enumerate}





\tightsubsection{\outputgrad: Estimating how configuration affects DNN inference}
\label{subsec:outputgrad}



\begin{figure*}[t]
    \centering
    % \includegraphics[width=0.5\columnwidth]{figs/placeholder-eval-overall-1.pdf}
    % \subfloat[][\centering{Object detection\\~~~~(Dashcam)}]
    % {
    %     \includegraphics[width=0.24\textwidth]{figs/detection_dashcam_FPN.pdf}
    %     \label{subfig:1}
    % }
    \subfloat[][Calculating \outputgrad using its definition]
    {
        \includegraphics[width=1.6\columnwidth]{figs/gradient-before-new.pdf} 
        % {figs/gradient-before_haodong.jpg} 
        \label{subfig:gradient-before}
    }
    \\
    \subfloat[][Calculating \outputgrad using \name]
    {
        \includegraphics[width=1.6\columnwidth]{figs/gradient-after-new.pdf} 
        % {figs/gradient-after_haodong.jpg} 
        \label{subfig:gradient-after}
    }
    % \subfloat[][Pipeline \circled{8}]
    % {
    %     \includegraphics[width=0.24\textwidth]{figs/lidar_video_e2e.pdf} 
    %     \label{subfig:1}
    % }
    % \subfloat[][Keypoint detection (Skate)]
    % {
    %     \includegraphics[width=0.22\textwidth]{figs/placeholder-eval-overall-2.pdf}
    %     \label{subfig:2}
    % }
    % \\
    % \subfloat[][Adapting configuration using \outputgrad]
    % {
    % \centering
    %     \includegraphics[width=1.8\columnwidth]{figs/workflow.pdf} 
    %     % {figs/gradient-after_haodong.jpg} 
    %     \label{fig:workflow}
    % }
    \tightcaption{Comparison between calculating \outputgrad naively and calculating \outputgrad using \name. \name calculates \outputgrad with \textit{no extra inference}. Note that the image of the DNN is cropped from this\cite{dnnimagesource} GitHub page.}
\end{figure*}








% takes a different approach by focusing on the \textit{gradient} of inference results in relation to the current configuration, referred to as \outputgrad.

% \mypara{Definition and example}
% Intuitively, the \outputgrad is the amount that the DNN inference output would change
% % \footnote{\kt{Talk about how to calculate inference results change. The calculation depends on whether Haodong's experiment works or not.}} 
% if a small adjustment was made to each knob in the current configuration.

% Though it sounds conceptual, \outputgrad can be explained with a simple 
% video analytics system that feeds each video frame to a DNN that determines whether it contains vehicles or not. 
% % Before that, we first explain the concept of \outputgrad in a concrete example.
% % consider an analytic system that analyzes a dashcam video feed by running a DNN to classify each video frame as containing a vehicle or not.
% Following prior work~\cite{chameleon,??}, we assume the system can tune two configuration knobs, frame rate and resolution.
% Suppose that the current configuration is 20fps and 480p, and the DNN output\footnote{Typical DNN output is more than a single value. Here, we assume that for a given video segment, the output of DNN inference is the average confidence of all detected objects. We will explain in \S\ref{??} how we turn the DNN output to a single value in general cases.} on a video segment is 0.9, and if we slightly increase the frame rate from 20fps to 21fps, the DNN output on the same video segment becomes 0.91.
% Then the \outputgrad of frame rate is (0.91-0,9)/(21-20)=0.01.
% Following a similar procedure, we calculate the \outputgrad of the resolution, say its value is -0.02.


% We now define \outputgrad first, then explain how to estimate \outputgrad efficiently, and finally why using \outputgrad to adapt configuration improves accuracy.
% describe the assumptions we make to calculate \outputgrad, define \outputgrad and then explain how to calculate \outputgrad and why one can use it to improve inference accuracy.


\mypara{Terminology}
% To formally define \outputgrad, 
We first introduce terminology to describe the DNN output.
% in a way that is relevant to this work. 
This is necessary because \name works with various DNN tasks and source data types (see Table~\ref{tab:pipeline} for a list).
% , from object detection in video and audio-to-text translation (see Table~\ref{??} for a list).
We split the source data stream into fixed-length (by default, one-second-long) intervals, called {\em adaptation intervals}.
In each adaptation interval, the data is first preprocessed with the current configuration and then fed to DNN (see Figure~\ref{fig:workflow}), and the DNN output contains multiple {\em elements}. 
% Note that there might be multiple DNN inferences within an adaptation interval.
An element can be a detected object in object detection, a detected text in audio-text translation, or the classification of a pixel in semantic segmentation.
Most DNNs for these tasks will associate each element with a confidence {\em score}, and only elements with a score over a confidence {\em threshold} will be counted towards accuracy. 
\name works with any DNN tasks that return elements with confidence scores as output. 

For the DNN output in an adaptation interval, we define the {\em \summary} by the number of elements in an adaptation interval whose confidence scores exceed the confidence threshold.
The rationale of \summary will be explained in detail later in \S\ref{subsec:gradient-ascent}.
For now, we can think of \summary as a one-value summarization of the DNN output whose change indicates the change in inference accuracy.

Though the definitions may not be universally applicable, it naturally applies to most prior work in video analytics as well as the new applications mentioned in Table~\ref{tab:applications}.
% developers do not need to make major changes to the DNN to use \name.






% \mypara{Assumption to the DNNs}
% We require the DNNs to expose the confidence scores in their inference results and the confidence threshold.
% Note that it does not impose an extra burden on the applications since most of the applications already expose confidence scores to indicate the uncertainty of DNN outputs and use confidence thresholds to filter out DNN outputs with low confidence. 
%those uncertain results returned from the DNN.

\mypara{Definition of \outputgrad}
\outputgrad is how much a small change in the current value of each knob changes the \summary (the number of DNN-returned elements in an adaptation interval with confidence scores over the confidence threshold).
Here, we use $\Output_\Config(\Data)$ to denote the \summary 
% averaged number of elements with confidence over the threshold in the DNN output 
at source data $\Data$ using configuration $\Config=(\Knob_i)_{i=1,\dots,n}$ ($n$ knob values). The \outputgrad of knob $\Knob_i$ is

\vspace{-0.2cm}
\begin{@empty}
\footnotesize
\begin{equation*}
\frac{\Delta \Output}{\Delta k_i} = \frac{\Output_{(\dots,\Knob_i+\delta,\dots)}(\Data)-\Output_{(\dots,\Knob_i,\dots)}(\Data)}{(k_i+\delta) - k_i}.
\end{equation*}
\end{@empty}

% Specifically, we use the following 
% \jc{Kuntai, please write the math expression here}
% confidence scores greater than the confidence threshold averaged across different data frames (\eg video frames).
% Intuitively, the \outputgrad is the amount that the DNN inference output would change
% if a small adjustment was made to each knob in the current configuration.
To help understand \outputgrad, we use a simple 
video analytics system that feeds each video frame to a DNN that performs vehicle detection with a confidence score of 0.5. 
Figure~\ref{subfig:gradient-before} illustrates \outputgrad in this example.
Following prior work~\cite{chameleon,vstore,videostorm,casva}, we assume the system can tune two configuration knobs, frame rate, and resolution.
Suppose that the current configuration is 10 frames per second (fps) and 480p.
% The analytic system will take a one-second-long, 20fps and 480p video and analyzes it through DNN.
When taking 1-second input, the DNN outputs 34 vehicle bounding boxes with confidence scores greater than 0.5 on these 10 frames, an average of 3.4 vehicles per frame.
% \footnote{Typical DNN output is more than a single value. Here, we assume that for a given video segment, the output of DNN inference is the average confidence of all detected objects. We will explain in \S\ref{??} how we turn the DNN output to a single value in general cases.} 
If we slightly increase the frame rate from 10fps to 15fps, the DNN outputs 66 vehicle bounding boxes with confidence scores greater than 0.5, on average 4.4 vehicles per frame.
Then the \outputgrad of the current frame rate is 

\vspace{-0.3cm}
\begin{@empty}
\footnotesize
\begin{align*}
\frac{\Delta \Output}{\Delta \text{framerate}}&=\frac{\Output_{(480p,15fps)}-\Output_{(480p,10fps)}}{15fps-10fps}=\frac{4.4-3.4}{15-10}=0.2.
% ,\\
% \frac{\Delta \Output}{\Delta \text{resolution}}&=\frac{\Output_{(720p,10fps)}-\Output_{(480p,10fps)}}{720p-480p}=0.01.
\end{align*}
\end{@empty}
% is (3.8-3.4)/(15-10)=0.08.
Following a similar procedure, we assume that the \outputgrad of the resolution will be:

\vspace{-0.3cm}
\begin{@empty}
\footnotesize
\begin{align*}
\frac{\Delta \Output}{\Delta \text{resolution}}&=\frac{\Output_{(720p,10fps)}-\Output_{(480p,10fps)}}{720p-480p}=\frac{5.8-3.4}{720-480}=0.01.
\end{align*}
\end{@empty}




\begin{figure*}
    \centering
    \includegraphics[width=1.6\columnwidth]{figs/workflow.pdf} 
    \tightcaption{Adapting configuration using \outputgrad. 
    \hl{Note that the generation of DNN output happens \textbf{before} the configuration adaptation process and thus the delay of obtaining the inference results is \textbf{not} affected by the configuration adaptation process (unless there is no sufficient resource for \name to perform the inference and the adaptation in real-time).}}
    \label{fig:workflow}
\end{figure*}

% Figure~\ref{subfig:gradient-before} illustrates the calculation of \outputgrad in the vehicle detection example.
% In this figure, we use $\Output_\Config(\Data)$ to denote the averaged number of above-threshold confidence scores in the DNN output at input data $\Data$ using configuration $\Config=(\Knob_i)_{i=1,\dots,n}$ (a vector of $n$ knob values), then \outputgrad of knob $\Knob_i$ is


% As a result, we have 
% \begin{@empty}
% \footnotesize
% \begin{align*}
% \frac{\Delta \Output}{\Delta \text{framerate}}&=\frac{\Output_{(480p,15fps)}-\Output_{(480p,10fps)}}{15fps-10fps}=0.08,\\
% \frac{\Delta \Output}{\Delta \text{resolution}}&=\frac{\Output_{(720p,10fps)}-\Output_{(480p,10fps)}}{720p-480p}=0.01.
% \end{align*}
% \end{@empty}








% We will soon show that there is a statistical correlation between \outputgrad and the accuracy of other configurations



% , each with 5 possible values (1 to 5 for simplicity),
% We assume that the current configuration is $(\Knob_1=2,\Knob_2=2)$.
% The \outputgrad of the two configuration knobs are:
% \jc{Use a concrete example. don't use values 1-5}

% \vspace{-0.3cm}
% \begin{@empty}
% \footnotesize
% \begin{align*}
%    & \frac{\Delta \Output}{\Delta \Knob_1}=\frac{\Output(\Knob_1=3,\Knob_2=2)-\Output(\Knob_1=2,\Knob_2=2)}{3-2}=0.2\\
%    & \frac{\Delta \Output}{\Delta \Knob_2}=\frac{\Output(\Knob_1=2,\Knob_2=3)-\Output(\Knob_1=2,\Knob_2=2)}{3-2}=0.2=0.1,
% \end{align*}
% \end{@empty}
% where $O(res=a, fps=b)$ means the corresponding inference results when configuring $res=a$ and $fps=b$.
% \kt{I guess we need a figure here.}


Essentially, \outputgrad indicates how the \summary of DNN inference results (\eg the number of detected objects) change with the value of each configuration knob. 
As shown in \S\ref{subsec:gradient-ascent}, \name's fast adaptation algorithm relies on \outputgrad to tune knob values in the ``direction'' that most improves accuracy or reduces resource usage without hurting accuracy (\S\ref{subsec:limitation}).
But first, we need to calculate \outputgrad quickly and using minimum GPU cycles. 


\tightsubsection{Using DNN differentiability to calculate \outputgrad}
\label{subsec:differentiability-outputgrad}

As shown in Figure~\ref{subfig:gradient-before}, a naive calculation of \outputgrad requires 
% through its definition results in high GPU overhead (
$n$ extra DNN inferences for $n$ configuration knobs.
However, we calculate \outputgrad \textit{with no extra DNN inference} by taking advantage of the {\bf differentiability of DNNs}. 

First, we decouple \outputgrad into two terms:
\begin{packedenumerate}
    \item {\em \dnngrad:} how the number of above-threshold confidence scores changes with different parts of DNN input (\Input).
    \item {\em \inputgrad:} how much different parts of DNN input change with each knob value of the current configuration (\Config). %in relation to the change in the current configuration.
\end{packedenumerate}

Formally, we use $\Input_{\Config}(\Data)$ to denote the DNN input of configuration $\Config$ at source data $\Data$. The \outputgrad of $\Knob_i$ on \Data can be expressed by
\vspace{-0.3cm}
\begin{align}
{\color{black}\underbrace{\highlight{white}{$\frac{\displaystyle \Delta \Output}{\displaystyle \Delta \Knob_i}$}}_{\text{\sf \footnotesize \textcolor{black!85}{\outputgrad}}}}=
{\color{black}\underbrace{\highlight{white}{$\frac{\displaystyle \Delta \Output}{\displaystyle \Delta \Input_\Config(\Data)}$}}_{\text{\sf \footnotesize \textcolor{black!85}{\dnngrad}}}}\otimes
{\color{black}\underbrace{\highlight{white}{$\frac{\displaystyle \Delta \Input_\Config(\Data)}{\displaystyle \Delta \Knob_i}$}}_{\text{\sf \footnotesize \textcolor{black!85}{\inputgrad}}}}
\label{eq:grad-decouple}
\vspace{-0.08cm}
\end{align}
Here, $\otimes$ means inner product.

The decoupling makes the calculation of \outputgrad much more resource-efficient for three reasons:
\begin{packeditemize}
\item The first term (\dnngrad) can be estimated by the DNN's derivation at input $\Input_\Config(\Data)$ via one backpropagation\footnote{
% \kt{Illustrate how we make the \# of above-threshold confidence scores differentiable here.}
To make $\Output$ differentiable, we define it to be $\sum_{e} Sigmoid(\alpha(Score_e-\beta))$ where $Score_e$ is the score of element $e$, $\beta$ is the confidence threshold (see \S\ref{subsec:eval-setup} for its exact value in each application), and $\alpha$ is a hyperparameter (by default, we use 20). Note that this function is almost identical to \summary when $\alpha$ is sufficiently large.
}.
This is a constant GPU-time operation without extra inference as it reuses the layer-wise features computed as part of the DNN inference of the current configuration.
\S\ref{sec:cost} will further reduce the compute overhead of backpropagation.

\item Second, the \dnngrad needs to be calculated once and re-used to derive \outputgrad of different knobs without extra DNN inference.
This is because the \dnngrad describes DNN's sensitivity to its input and thus remains largely similar if the change in DNN input is not dramatic.
For instance, the \dnngrad of an object-detection DNN is high on pixels associated with key visual features of an object.
% \jc{edit ends here}

\item Finally, computing this term does not involve any DNN inference, as it only runs the preprocessing part of the DNN analytics system multiple times.

\end{packeditemize}



% Additionally, 





% Therefore, computing \outputgrad for multiple configuration knobs only requires a one-time backpropagation on GPU and no extra DNN inference.

Figure~\ref{subfig:gradient-after} shows an example of how \outputgrad is calculated from \dnngrad and \inputgrad.
% We use $\Input_{\Config}(\Data)$ to denote the DNN input of configuration $\Config$ at input data $\Data$.
% The decoupling can be written as \outputgrad $\approx$ \inputgrad $\otimes$ \dnngrad, concretely,

\vspace{-0.3cm}
\begin{@empty}
\scriptsize
\begin{align*}
\frac{\Output_{(480p,15fps)}-\Output_{(480p,10fps)}}{15fps-10fps} &\approx \frac{\Input_{(480p,15fps)}-\Input_{(480p,10fps)}}{15fps-10fps} \otimes \frac{\Delta \Output}{\Delta \Input}\bigg|_{\Input=\Input_{(480p,10fps)}},\\
\frac{\Output_{(720p,10fps)}-\Output_{(480p,10fps)}}{720p-480p} &\approx \frac{\Input_{(720p,10fps)}-\Input_{(480p,10fps)}}{720p-480p} \otimes \frac{\Delta \Output}{\Delta \Input}\bigg|_{\Input=\Input_{(480p,10fps)}},
\end{align*}
\end{@empty}
where $\otimes$ represents inner product and $\frac{\Delta \Output}{\Delta \Input}|_{\Input=\Input_{(480p,10fps)}}$ is \dnngrad of the  current configuration $(480p,10fps)$ on the current source data $\Data$.

Importantly, Figure~\ref{subfig:gradient-after} shows that to calculate \outputgrad, \name saves extra GPU inference by decoupling \outputgrad and re-using the backpropagation results for different knobs.
This example has two knobs, thus the saving may seem marginal, but our evaluation shows more savings when \name is used to adapt more knobs together in more realistic DNN analytics systems (Figure~\ref{fig:fine-grained-knobs}). 



% \kt{\hl{Claim we are the first one who uses backprop for config adaptation here. I think it's better to mention saliency-based works  in related work rather than here.}}
We want to clarify that while \name is the first to leverage DNN differentiability for configuration adaptation, DNN differentiability has already been widely used in DNN training, DNN interpretability, and localization of areas most responsible for the DNN output~\cite{vision-saliency-1,vision-saliency-2}.
It should also be pointed out that \dnngrad differs from the traditional notion of ``saliency'' used in video compression~\cite{fischer2021saliency,hadizadeh2013saliency}, in that \dnngrad is derived directly from a particular DNN to capture how the input influences the DNN output. 

% Note that \name is the first system that leverages the differentiability of DNNs for configuration adaptation, though not the first one that leverages differentiability of DNNs in DNN serving system\footnote{For example, in computer vision community, people use backpropagation to localize which areas of the objects are responsible for the DNN output~\cite{vision-saliency-1,vision-saliency-2}.}. 
% We also aware that there is a recent trend in multi-media community that compress videos by estimating the saliency (\ie the regions in the input video that may contain objects) and encoding these regions in encoding quality.
% Also, there is a line of work from multi-media community~\cite{fischer2021saliency,chen2022context} that leverages saliency estimators to  estimates the areas in the DNN input that contain objects, and then enocde these areas in higher encoding quality so that the objects in these areas can be better detected.
% The notion of saliency may conceptually seems similar to \dnngrad (as both highlight the areas that are related to objects), 
% Also, conceptually \dnngrad is similar to saliency (the areas in the input video that may contain objects) in multi-media community that 

% However, these saliency estimato
% \kt{1. Backpropagation is used in model serving system for explanation.
% But we are the first one to use it for config adaptation
% 2. MM community use saliency to compress video.
% It may seems similar, but our saliency is aware of the final DNN and they are not (drawbacks).}
% \mypara{\dnngrad v.s. existing saliency estimators}
% \dnngrad captures the saliency of the DNN (defined as a map that quantifies the importance of different areas in the DNN input), where there are existing works that also serves the same purposes~\cite{accmpeg,dds,eaar,vigil,fischer2021saliency}.
% However, \dnngrad outperforms existing saliency map estimation algorithms.
% \begin{packeditemize}
%     \item Compared to generating saliency using cheap models~\cite{accmpeg,vigil,fischer2021saliency}, \dnngrad prioritizes those objects according to the likeliness of changing the number of objects detected (where cheap models may mark all objects~\cite{fischer2021saliency} as salient or wrongfully assign saliency to those objects that are detected with high confidence~\cite{accmpeg}).
%     \item One may also generate saliency based on region proposals (an intermediate result generated alongside DNN inference that includes regions potentially containing objects). Compared to this approach, \dnngrad can further rank the pixels inside each object, where this approach will mark all pixels inside an object as salient/non-salient.
% \end{packeditemize}

% \kt{Compare our saliency v.s. others saliency here}


% \mypara{Assumption to configuration knobs}





% First, 
% Second, \dnngrad further prioritizes the pixels inside and outside the object bounding boxes according to the likeliness of changing the number of objects detected, where 

% However, \name calculates this saliency using backpropagation instead of using cheap saliency estimators, allowing \name to derive a metric (\outputgrad) that directly correlates with inference accuracy.
% The cheap saliency estimators fail to correlate with inference accuracy in some cases.
% For example, one may use cheap neural network to estimate saliency~\cite{accmpeg,?,?}.
% However, these cheap saliency estimators will \kt{finish this.}






% Specifically, \name measures \outputgrad by how much a small change in the current value of each knob \textit{flips} the DNN-returned confidence scores from below (or above) the confidence threshold to above (or below). 
% It does not impose an extra burden on the applications to require them to expose confidence scores and confidence thresholds since most of the applications already expose confidence scores to indicate the uncertainty of DNN outputs and use confidence thresholds to filter out DNN outputs with low confidence. %those uncertain results returned from the DNN.
% Statistically, more changes in the ``near-confidence-threshold'' DNN outputs will likely cause more changes in the inference accuracy (as will be elaborated in \S\ref{subsec:correlation})\footnote{This correlation does \textit{not} assume that a confidence score always directly indicates the accuracy of its corresponding detection/classification results.}.
% % \outputgrad correlates with how much the accuracy \textit{changes} with knobs 
% Intuitively, this is because the confidence threshold determines whether a detection or classification result is accepted (as part of the accuracy calculation) or rejected (thus having no effect on the accuracy).




% \pagebreak


% We advocate that the adaptation system for DNN-based analytics should provide a new abstraction: \outputgrad, which estimates the gradient of DNN output with respect to individual knobs.
% We define \outputgrad on a designated knob as the change of the DNN-returned \textit{confidence scores} around (both below and above) the \textit{confidence threshold}, divided by the small amount of change of the knob.
% % when changing this knob by a little.
% This definition requires the application to expose the confidence scores inside their inference results and the confidence threshold used to filter the results.
% For most of the applications, the DNN-returned confidence scores and confidence threshold are naturally available, since most of the applications use confidence scores to quantify the uncertainty of the DNN inference results. The application then filters those results with low confidence scores (as these results may contain spurious results) through a confidence threshold.

% We found that \outputgrad nicely correlates with how much the inference accuracy changes with the knobs.
% Intuitively, this is because the confidence threshold determines whether a detection or a classification result is accepted (and thus participating in the accuracy calculation) or rejected (and thus having no effect on the accuracy).
% Thus, more changes of confidence scores near the confidence threshold will likely cause more changes on the inference accuracy.

% This gradient information can help us quickly adapt to the optimal configuration, 
% % among a large number of configurations 
% by assigning more resources to those knobs with high \outputgrad to improve the accuracy and cut the resource usage of those knobs with low \outputgrad to save resource usage (without hurting the accuracy).
% As shown in Figure~\ref{fig:compare}, \name quickly find the optimal configuration through \outputgrad, while the profiling-based approach needs to profile all configurations to obtain the optimal one, and the output-driven approach adapts slowly.




% \begin{figure*}[t]
%     \centering
%     \includegraphics[width=2.2\columnwidth]{figs/workflow.pdf}
%     \caption{Workflow of \name. \kt{$\Delta resolution$ $240p, 1fps$ }people won't immediately realize it's adding. Need some handholding, picking the new configuration}
%     \label{fig:workflow}
% \end{figure*}



% To quickly adapt to optimal configuration with no extra inference, \name calculates the \textit{gradient} of accuracy with respect to the knob (hereinafter \outputgrad).\jc{i suppose you will clean up all \accgrad and replace them with \outputgrad?}
% We define \accgrad as the accuracy change divided by the knob value change when changing the knob value by a little.

% With this gradient, \name can quickly adapt to the optimal configuration in a large configuration space by granting more resource to the knobs with high \accgrad to improve the accuracy, and cutting the resource usage of those knobs with low \accgrad to reduce the resource usage without hurting accuracy.

\tightsubsection{Selecting the next configuration}
\label{subsec:gradient-ascent}


% \jc{(1) 3.2 and 3.3 are still a bit too abstract. please use a concrete example like the one in 31
% (2) it’s not clear from 32 (upfront) why configgrad-based gradient ascent can adapt quickly. this should be upfront, not embedded or in the end
% same thing with 33. it’s unclear why this is a smart design
% (3) i dont see the assumptions in 31, 32, 33 be explicitly called out and justified.. did i miss them?}
% \kt{I explicitly called out the assumptions in 31. I will deprioritize other issues before Sunday.}

With \outputgrad, \name runs \textit{gradient ascent} to converge to a near-optimal configuration.
In each adaptation interval, we perform inference using the current configuration $\Config_{cur}$ (\eg current resolution and frame rate), compute \outputgrad, and then use the following strategy to select a new configuration $\Config$ for the next adaptation interval.
% the gradient of the objective function $Obj(k)$ with respect to the current configuration $\Config_{cur}$ and update the current configuration by running gradient ascent.

% In each adaptation interval, we perform inference using the current configuration $\Config_{cur}$ (\eg current resolution and frame rate), obtain the gradient of the objective function $Obj(k)$ with respect to the current configuration $\Config_{cur}$ and update the current configuration by running gradient ascent.

Formally, the goal of \name is to maximize a weighted sum between the accuracy $Acc$ (defined as the \textit{similarity} between the current inference results and the inference results generated under unlimited resource)\kt{need to defend this definition} and the resource usage $\Resource$:
\begin{equation}
\underbrace{Acc(\Config)}_{\text{\sf \footnotesize \textcolor{black!85}{accuracy}}}
- \underbrace{\lambda \Resource(\Config)}_{{\text{\sf \footnotesize \textcolor{black!85}{resource usage}}}},
\label{eq:objective}
\end{equation}
% where $\Config$ i \name maximizes this weighted sum by running gradient ascent (depicted in FIgure~\ref{fig:workflow}).
where $\lambda$ is a hyperparameter that governs the tradeoff between accuracy and resource usage: higher $\lambda$ will emphasize resource-saving and lower $\lambda$ will emphasize accuracy improvement.
We will vary $\lambda$ and examine its effect on \name in \S\ref{??}.



\mypara{Ideal way of picking new configuration}
Ideally, \name would update the $i^{th}$ knob $\Knob_{cur,i}$ in the current configuration $\Config_{cur}$ by:
\begin{@empty}
\footnotesize
\begin{align*}
\Knob_i^*=\Knob_{cur,i}+ \alpha \left(
\underbrace{
\frac{Acc(\Config_{cur} + \Delta\Knob_i) -Acc(\Config_{cur})) }{\Delta \Knob_i}
}_{\text{\sf \footnotesize \textcolor{black!85}{gradient of accuracy}}}
- 
\lambda 
\underbrace{\frac{\Resource(\Knob_{cur} + \Delta\Knob_i) - \Resource(\Knob_{cur}) }{\Delta\Knob_i}
}_{\text{\sf \footnotesize \textcolor{black!85}{gradient of resource usage}}}
\right),
\end{align*}
\end{@empty}
where $\Knob_i^*$ is the updated value of the $i^{th}$ knob, $\Delta\Knob_i$ is a small increase on the $i^{th}$ knob, $\alpha$ is the learning rate for gradient descent (see \S\ref{??} for the concrete value we use): increasing the learning rate $\alpha$ increases the convergence speed of \name, but may miss the optimal value of the accuracy.

% We calculate $\frac{\Resource(\Knob_{cur,i} + \Delta\Knob_i) - \Resource(\Knob_{cur,i}) }{\Delta\Knob_i}$ by following its definition, which imposes extra overhead on \name (we will evaluate this overhead in \S\ref{??}) but does not require extra DNN inference.

We calculate the gradient of resource usage by using the pre-profiled resource usage of each configuration $\Resource(\Config)$ (this aligns with prior work~\cite{chameleon,dds,reducto}), which might vary with source data, but the relative difference among them has little variance.

However, it is computationally expensive to calculate the gradient of accuracy $$
\frac{ Acc(\Config_{cur} + \Delta\Knob_i) -Acc(\Config_{cur})) }{\Delta \Knob_i}$$
as calculating the accuracy $Acc$ requires generating the inference results under unlimited resources (recall that we define accuracy as the similarity between this inference results and the current inference results).

\name instead leverages \outputgrad to approximate the gradient of accuracy.
The rationale behind this approximation is that \outputgrad correlates with the gradient of accuracy:
if one knob is of large \outputgrad, increasing this knob will significantly change the DNN output $\Output$, and thus also significantly affects the accuracy $Acc$, leading to a large change of accuracy.
We will further explain when and why \outputgrad can approximate the gradient of accuracy in \S\ref{??}.
% On the contrary, if the \outputgrad of one knob is small, increasing this knob does not affect the DNN $\Output$, and thus the corresponding accuracy change is also marginal.


\mypara{\name way of picking new configuration} As a result, \name picks the new configuration by
\begin{@empty}
\footnotesize
\begin{align*}
\Knob_i^*=\Knob_{cur,i}+ \alpha \left(
\underbrace{
\frac{\Output(\Config_{cur,i} + \Delta\Knob_i) -\Output(\Config_{cur,i}))}{\Delta \Knob_i}
}_{\text{\sf \footnotesize \textcolor{black!85}{\outputgrad}}}
- 
\lambda 
\underbrace{
\frac{\Resource(\Knob_{cur,i} + \Delta\Knob_i) - \Resource(\Knob_{cur,i}) }{\Delta\Knob_i}
}_{\text{\sf \footnotesize \textcolor{black!85}{gradient of resource usage}}}
\right),
\end{align*}
\end{@empty}
where $\Output$ is \summary  (\ie the number of above-threshold confidence scores).
% note that we take the absolute value to \outputgrad, as we assume that increasing the knob values increases the resource usage (and thus increases the accuracy).



% To further support the claim that \outputgrad correlates with the gradient of accuracy, we empirically 
% We notice that the \textit{cosine similarity} between \outputgrad and AccGrad is higher than 0.95 (we provide a formal proof that AccGrad is equals to \outputgrad using an idealized accuracy function, see \S\ref{??}), so substituting it with the accuracy can still guide \name to the optimal configuration.

% % To adapt configurations using \outputgrad, 
% \name runs gradient ascent (depicted in Figure~\ref{fig:workflow}) to converge to a near-optimal configuration.
% % First, we partition the input data stream (\eg video frames) into {\em adaptation intervals}, each of one second.
% In each adaptation interval, we perform inference using the current configuration $\Config_{cur}$ (\eg current resolution and frame rate), compute \outputgrad, and then use the following strategy to select a new configuration $\Config$ based on \outputgrad. 

% The goal of \name's gradient ascent is maximizing a weighted sum between \summary (number of elements with scores over the confidence threshold) and resource usage (we will discuss alternative formulations shortly):

% \vspace{-0.4cm}
% \begin{@empty}
% \small
% \begin{align}
% {\color{black}\underbrace{\highlight{white}{$\Output_{\Config}(\Data)$}}_{\text{\sf \footnotesize \textcolor{black!85}{\summary}}}}-\lambda {\color{black}\underbrace{\highlight{white}{$\Resource(\Config)$}}_{\text{\sf \footnotesize \textcolor{black!85}{resource usage}}}} \label{eq:objective}
% \end{align} 
% \end{@empty} 
% Here, $\Resource(\Config)$ is the resource usage (in either bandwidth or GPU cycles, defined per application) of \Config.
% The hyperparameter $\lambda$ governs the tradeoff between accuracy and resource usage: higher $\lambda$ will emphasize resource-saving and lower $\lambda$ will emphasize accuracy improvement.
% \hl{Note that we will vary $\lambda$ and study its impact in \S\ref{sec:eval}.}
% % As shown in prior work, for most configuration knobs (\eg frame rate, resolution, etc), $Resource(\Config)$ can be accurately pre-profiled and does not vary with input content as much as inference results.

% Given the current configuration $\Config_t$ at the interval $t$ and the \outputgrad $\Grad_t$ (a vector of each knob's \outputgrad), the new configuration used for the next interval $t+1$ should be the one that maximizes the improvement of the objective. 
% Formally, we can express it by 

% \vspace{-0.4cm}
% \begin{@empty}
% \small
% \begin{align}
% \Config_{t+1}=\textrm{argmax}_{\Config}{\color{black}\underbrace{\highlight{white}{$(\Config-\Config_t)\cdot \Grad_t$}}_{\text{\sf \footnotesize \textcolor{black!85}{change in \summary}}}}-\lambda {\color{black}\underbrace{\highlight{white}{$(\Resource(\Config)-\Resource(\Config_t))$}}_{\text{\sf \footnotesize \textcolor{black!85}{change in resource}}}} \label{eq:gradient}
% \end{align}
% \end{@empty}
% % $\Config_{t+1}=\textrm{argmax}_{\Config} (\Config-\Config_t)\cdot Grad_t-\lambda (\Resource(\Config)-\Resource(\Config_t))$
% The new configuration $\Config_{t+1}$ will be used for the next adaptation interval. 
% Following prior work~\cite{chameleon,dds,reducto}, we pre-profile the resource usage of each configuration $\Resource(\Config)$, which might vary with source data, but the relative difference among them has little variance.

In many applications, the objective in Eq.~\ref{eq:objective}, which linearly combines resource usage and \summary, is less reasonable than optimizing \summary with a fixed constraint on resource usage.
For instance, one may choose to maximize \summary (which relates to accuracy as explained shortly), conditioned on the bandwidth usage of the configuration within a budget.
Figure~\ref{fig:workflow} shows an example of how \name's gradient-based adaptation process works in the vehicle detection example.
% We will still use the vehicle detection example, where a traffic camera streams its video data to a GPU-equipped server to determine which frame contains vehicles.
In each adaptation interval, the sensor encodes the video in an adaptation interval using the current configuration (frame rate and resolution) and sends it to a DNN running on a GPU-equipped server.
The server receives this video and runs DNN inference to get the inference results and runs backpropagation to get \dnngrad and send it back to the sensor. 
While the server runs DNN inference, the sensor runs encoding multiple times with different to obtain \inputgrad (the change in DNN input with respect to each knob).
Once the sensor receives \dnngrad, it uses Eq.~\ref{eq:grad-decouple} to calculate \outputgrad.
It then runs the gradient ascent strategy in Eq.~\ref{eq:gradient} to adapt the configuration and uses the new configuration in the next interval. 
% \jc{kuntai, remember to justify why resource usage of a config can be known in advance? what about the frame-diff threshold in reducto?}

% the encoded video that the camera sent, decodes this video, and runs DNN inference to obtain the inference results.
% Then, the server calculates the saliency using the backpropagation and streams the saliency back to the camera.
% Finally, the camera receives the saliency, calculates \outputgrad, and adapts the configuration accordingly.
% \jc{kuntai, please update figure~\ref{fig:workflow} to include the gradient-based adaptation process.}

% 



\tightsubsection{Caveats and benefits}
\label{subsec:limitation}

While our evaluation shows \name's gradient-ascent strategy performs well for a wide range of DNN tasks, data types, and configuration knobs, it is important to understand its limits and why it works in practice. 

\kt{Let Yuhan run an experiment on this}
\mypara{Why \name improves accuracy}
Second, in the objective of gradient ascent (Eq.~\ref{eq:objective}), the change in the first term of \summary (\Output) should reflect the change in inference accuracy.
This connection may be intuitively true since a significant change in the inference results is often accompanied by a substantial change in accuracy.
That said, a big change in the \summary may indicate either more increase or decrease in accuracy. 
To decide the direction of change, we use the empirical observation that when a change in knob value increases the resource usage, the impact on inference accuracy should be positive (\eg higher encoding resolution leads to higher bandwidth usage and likely more accurate inference, or higher frame rate leads to higher GPU usage and likely more accurate inference). 

Figure~\ref{fig:accuracy-proxy} empirically verify whether the change in output ($\Delta \Output_\Config(\Data)$) is proportional to the change in accuracy (\ie the accuracy of the configuration $\Config$, minutes the accuracy of current configuration).
We pick three configuration knobs (frame sampling rate, resolution, quantization parameter) that are widely used by prior work~\cite{chameleon,casva,awstream,videostorm,vstore,mcdnn} and a 6-second video chunk to verify the correlation between DNN output change and accuracy change on all configurations (125 configurations in total).
Figure~\ref{fig:accuracy-proxy} shows that on one 9-second video chunk, the change of DNN output (X-axis) nicely correlates with the accuracy change (Y-axis), with a Pearson coefficient of 0.702.


\mypara{Why \name converges}
First, like other gradient-based heuristics, \name does not guarantee to always converge to a global optimum configuration. 
That said, we empirically observe that the relationship between configuration $\Config$ and their \summary ($\Output$) and resource usage ($\Resource$) is mostly {\em concave}.
As a result of the concavity, gradient-ascent can {\em eventually} converge to a global optimal configuration. 
The concavity can be intuitively understood that as the configuration uses more (compute/network) resources, the change in the input to the DNN becomes more marginal, and so does the DNN output.
For example, as a video analytic system increases the video encoding resolution, the pixel change becomes more marginal (mostly on ``high-frequency'' details), causing the DNN output to stabilize (objects' confidence scores will change more slowly and less frequently cross the confidence threshold, leading to fewer newly detected objects).




Another potential reason for \name to fail to converge is the evolution of source data content---the \outputgrad calculated from one adaptation interval may not apply to the next adaptation interval due to temporal change in the content. 
That said, we observe that \name converges to the optimal configuration within 3-5 intervals (seconds) as shown in Figure~\ref{fig:converge-fast}, and within 1-2 intervals for configurations that require frequent adaptation (such as macroblock-level encoding quality).
Thus, as long as the best configuration last for a few seconds, \name can identify the best configuration faster than profiling-based methods.
% Both profiling-based methods and \name require the continuity of resource/accuracy relationship at a timescale of several to 10s of seconds. 



% explain it with the example in fig 6. (need to update fig 6)
% caveats: 
% why not local optimum: concavity => connection with newton's method
% why leading to higher accuracy
% content change 

% limitation: not applicable to dnn knobs





% \mypara{\outputgrad correlates with accuracy}
% A key question is how \outputgrad is related to inference accuracy.
% We found that there is a statistical correlation between \outputgrad and the inference accuracy of other configurations. 
% This is because \outputgrad captures the change in the inference results, and a significant change in the inference results is often accompanied by a substantial change in accuracy.

% We found that \outputgrad statistically correlates with the inference accuracy.
% This is because \outputgrad captures the change in the inference results, where a large change in inference results likely corresponds to a large change in accuracy.

\begin{comment}
However, the change in the inference results cannot determine whether the accuracy improves or decreases.
To handle this issue, we make an assumption that for a designated knob $\Knob_i$, increasing it while keeping other knobs fixed will either statistically not decrease the accuracy (we denote this case as $sgn(i)=1$) or not increase the accuracy (we denote this case as $sgn(i)=-1$).
We found that this assumption holds for a wide range of knobs (see Table~\ref{tab:rich-set-of-knobs}), as increasing these knobs causes the resource usage pipeline increases/decreases and thus the corresponding accuracy also increases/decreases.
For example, increasing the frame rate while fixing the  resolution in the video analytics system typically leads to more accurate inference results as more frames are analyzed. 
Similarly, increasing the resolution while fixing the frame rate enhances the clarity of the boundaries of the object, and is likely to generate more accurate inference results.

% To give a concrete example, when tuning the frame rate and resolution of the aforementioned video analytic system, increasing the frame rate while fixing the resolution typically leads to more accurate results as more frames are being analyzed. 
% Similarly, increasing the resolution while fixing the frame rate also makes the detail of the video (like the boundary of the vehicles) clearer and thus is likely to generate more accurate inference results.

Using this assumption, we then derive the (signed) output change with respect to the current configuration (frame rate $\Knob_1=20fps$, resolution $\Knob_2=480p$) using the following formula:

\vspace{-0.3cm}
\begin{@empty}
\footnotesize
\begin{equation*}
\Delta \Output_\Config(\Data)= \sum_{i=1}^n \left|\frac{\Delta \Output}{\Delta \Knob_i}\right| \cdot sgn(i) \cdot (\Knob_i - \Knob_{i,cur}) =  0.08 \cdot (\Knob_i - 10\textrm{fps}) + 0.01 \cdot (\Knob_2 - 480\textrm{p}) 
\end{equation*}
\end{@empty}
% To examine the correlation between \outputgrad and the accuracy of other configurations, we calculate the change in accuracy with respect to the change of the current configuration ($O(res=2,fps=2)$) using the following formula
% \begin{@empty}
% \footnotesize
% \begin{equation*}
% \Delta O(res,fps) = \frac{\Delta O}{\Delta (res, fps)} \cdot \Delta (res, fps) = \frac{\Delta O}{\Delta res}(res-2) + \frac{\Delta O}{\Delta fps}(fps-2).
% \end{equation*}
% \end{@empty}
% And check if the output change is proportional to the accuracy change

  



And then, we verify whether the change in output ($\Delta \Output_\Config(\Data)$) is proportional to the change in accuracy (\ie the accuracy of the configuration $\Config$, minutes the accuracy of current configuration):
% \begin{@empty}
% \footnotesize
% \begin{equation*}
% \Delta \Output(\Input, \Config) \propto Acc(\Output(\Input, \Config)) - Acc(\Output(\Input, \Config_{cur})),
% \end{equation*}
% \end{@empty}
% where $Acc$ represents the inference accuracy.
We pick three configuration knobs (frame sampling rate, resolution, quantization parameter) that are widely used by prior work~\cite{chameleon,casva,awstream,videostorm,vstore,mcdnn} and a 6-second video chunk to verify the correlation between DNN output change and accuracy change on all configurations (125 configurations in total).
As shown in Figure~\ref{fig:accuracy-proxy}, on one 9-second video chunk, the change of DNN output (X-axis) nicely correlates with the accuracy change (Y-axis), with a Pearson coefficient of 0.702.


\end{comment}






% that maximally improves the change in DNN output $\Delta \Output(\Data,\Config)$ under the resource budget.
% As the change in DNN output statistically correlates with the change in accuracy, this will likely maximize the accuracy of the new configuration $\Config$.
% We then use this configuration for the next adaptation interval.
% identify a new configuration that maximally improves accuracy without exceeding the resource budget.
% We use this new configuration for the next adaptation interval, and at the end of the interval, we repeat the same adaptation steps.
% As the content of the input data is continuous, the new configuration is likely to generate more accurate inference results compared to the original configuration.
% Note that 
% As a result, the inference results of the new configuration are likely to be more accurate than the current configuration


\mypara{Why \name beats alternatives}
By performing gradient ascent based on \outputgrad, \name outperforms previous work on all three requirements (\ie adapt frequently, converge to a near-optimal configuration, and generalize to different types of knobs and analytic tasks).
First, compared to profiling-based work, \name adapts much more frequently (as \name updates its configuration \textit{at every second} but profiling-based work updates its configuration once every minute~\cite{awstream}) and earlier (as \name adapts to the change of input content right at the next adaptation interval but the profiling-based work need to wait till the next profiling).
Second, compared to the heuristics-based approach, \name can adapt to a near-optimal configuration, where the accuracy of the heuristics-based approach can be much lower than the optimal configuration.
Third, \name can generalize to different applications and DNNs (as \name only assumes the DNNs to be differentiable, which holds for almost all DNNs) and a wide range of knobs (as \name applies to most of existing knobs, see Table~\ref{tab:rich-set-of-knobs}).




% \tightsubsection{Limitations}
% \label{sec:limits}

\mypara{Limitation} 
% We acknowledge that \outputgrad only works for configuration knobs that affect DNN input (\ie input preprocessing part of a DNN analytics system).
The idea of decoupling \outputgrad assumes that the configuration knobs only influence DNN input (\ie knobs of input preprocessing part of a DNN analytics system).
A wide range of knobs falls into this assumption (\eg video codec encoding parameters~\cite{awstream,vstore,videostorm,chameleon,casva}, frame filtering thresholds~\cite{glimpse,reducto,filterforward}, fine-grained encoding quality assignment~\cite{dds,eaar,accmpeg,vigil}, see  Table~\ref{tab:rich-set-of-knobs} for a list of existing knobs that \name covers).
That said, it does {\em not} include knobs that modify/select the final DNN itself.


\mypara{Example applications that \name applies}

\mypara{Overhead of backpropagation}

% However, this assumption makes \name not applicable to knobs that alter the DNN itself, such as retraining the DNN weights based on the current input~\cite{ekya,noscope,mcdnn}.
% In some sense, both the DNN customization approach and \name are adapting to the varying content in the input data stream.
% However, in order to maintain high accuracy, the DNN customization approach needs to retrain the DNN when the input content varies (which adds high GPU overhead).
% In contrast, \name adapts the knobs as part of the DNN-based inference process and only reuses the DNN inference result (for backpropagation), which is much more lightweight.


% \jc{need a paragraph to explain customization of specific applications, and why it still works under evolving content}
% overall, why it's better?

% Our gradient-ascent-based approach has its own caveats as it cannot guarantee that (i) the search will quickly converge in a few steps, and (ii) the search may get stuck in a local optimal.
% To answer this question, we measure how fast \name can converge to a near-optimal configuration (a top-1\% configuration).
% \kt{Not sure how to answer this question}





% The intuition behind the fast convergence is that as long as the \outputgrad with respect to one configuration knob is non-zero, tuning that knob will likely improve accuracy.
% % Further, as the input data is constantly changing over time, it is less likely for a local optimal to persist.
% Thus, \name is unlikely to be stuck in a local optimum, which corroborates our empirical observation of \name.
% \kt{Other potential concerns: (1) why treat discrete configs as almost continuous variables, (2) why the better configuration at this second will likely lead to a better result at the next second, (3) what if the content is noisy and makes the gradient noisy}



% However, directly calculating \outputgrad needs a substantial amount of extra inference.
% If we calculate \outputgrad knob-by-knob, we will need to calculate the accuracy change by changing one knob at a time.
% The amount of GPU compute will grow at least linearly with more knobs. 
% % This is because calculating \outputgrad in a knob-by-knob manner (\ie calculate the accuracy change by alternating the value of one knob while the value of other knobs remaining unchanged, and repeat this process for all knobs) results in extra inference (see \S\ref{subsec:calculate-accgrad} for details).
% % Moreover, more knobs will lead to more inference and reduces the applicability of \outputgrad on a large set of knobs.

% \mypara{Leveraging DNN differentiability} To reduce such overhead, \name harnesses the differentiability of the DNN to calculate \outputgrad with constant GPU overhead and with no extra inference.
% Intuitively, in order to calculate how DNN output changes with respect to the knob change (\ie \outputgrad), we can calculate how DNN output changes with respect to the DNN input change, and then study how DNN input changes with respect to the knob change.
% % how changing system knobs alters the DNN input, and then calculate how changing the DNN input alters the DNN output.
% Formally, we denote the configuration (\ie the values of all knobs) as $c$, the DNN input as $I$, and the DNN output as $O$. The intuition above can be written as the following chain rule:
% \begin{equation}
%     \frac{\partial O}{\partial c} = \frac{\partial O}{\partial I} \cdot \frac{\partial I}{\partial c},
% \end{equation}
% The first term $\frac{\partial O}{\partial I}$ can be obtained via backpropagation (a constant GPU overhead, but no extra inference is incurred as backpropagation reuses the computation graph created by existing DNN inference).
% The second term $\frac{\partial I}{\partial c}$ can be calculated in a knob-by-knob manner but since it only computes the DNN input (not DNN inference), it does not have extra GPU overhead. 
% without incurring DNN inference as calculating the DNN input change does not require DNN inference.

% The key enabler for \name to remove the extra inference is the following two observations to existing knobs for DNN-based analytic systems.



% that the knob only alters the DNN input. does not cover those knobs that alter the DNN itself, 




% \begin{enumerate}
%     \item \textit{Accuracy-Resource Property}: For a large class of knobs,  increasing the value of one knob always results in spending more (or less) resource, and also making the corresponding inference results more (or less accurate).
%     The amount of accuracy improvement (or degradation) depends on how much the knob increase alters the inference results.
%     \item \textit{Black-box Property}: Most of the knobs treat DNN as a black box and change the inference results solely by changing the DNN input.
% \end{enumerate}

% By leveraging the first assumption, \name estimates the accuracy change through inference results change, thus avoid calculating the inference results under the most expensive configuration as the ground truth.
% By leveraging the second assumption, \name decouples the gradient using chain rule and avoid the inference on the new configurations.


% Note that not all knobs satisfies the two properties above. We list some examples in Table \ref{??} and some non-examples down below.

% For \accres, we find that the sensing configuration knobs that directly change the raw sensed data, like the aperture and the ISO of the camera, the Gamma correction value of the camera, the positioning direction of the directional microphone, etc., do not satisfy \accres as varying these knobs typically have little impact on the encoded file size and the encoding cost of the input data.
% However, the sensing configuration knobs are typically pre-configured (like the positioning direction of the microphone) or self-adapted (like the aperture and the ISO of the camera) by the sensor.
% As a result, these knobs are typically not dynamically programmable so \name cannot change these knobs anyway.

% The non-examples for \blackbox are the knobs that optimize DNN inference, like DNN selection~\cite{chameleon} and DNN customization~\cite{noscope,ekya,mcdnn}.
% We acknowledge the effectiveness of these knobs in terms of saving GPU cost.
% However, we argue that these knobs requires the system to change or replace the DNN in real-time, which make them not generally applicable in all deployment settings (\eg when performing inference through third-party API).
% % However, switching or editing the DNN may result in significant overhead (\eg some other components may be customized for this DNN and may require retraining upon DNN changing~\cite{accmpeg}) or even not doable (\eg when performing inference through cloud API).




% \tightsubsection{Workflow of \name}














% We demonstrate the workflow of \name using the example of traffic cam-based vehicle detection
% Figure~\ref{fig:workflow} demonstrates the workflow of \name.
% \name assumes that the analytic systems are made up of two components: \textit{input processing} and \textit{DNN-based inference}.
% First, \name processes the data stream $x$ through input processing using the current configuration $c$ to obtain the DNN input $I$.
% \name then forwards $I$ through the DNN and obtain the DNN output $O$.
% After that, \name performs DNN backpropagation and obtains the gradient $\frac{\partial O}{\partial I}$.
% In the meantime, \name alters every knob in $c$ and obtains the corresponding change on the DNN input.
% \name then stacks together the DNN input changes of individual knobs ($\frac{\partial I}{\partial c}$) and 
% % \name then stacks these DNN input changes to obtain $\frac{\partial I}{\partial c}$ and 
% multiplies it with $\frac{\partial O}{\partial I}$ to obtain \outputgrad $\frac{\partial O}{\partial c}$.
% Finally, \name updates the configuration $c$ according to the \outputgrad.
% We will present the details of each step in the next section.









% \subsection{Accuracy gradient as a better feedback}

% \begin{itemize}
%     \item We find that: how much the analytic accuracy change differs if we change different knobs is essentially asking what is the \textit{gradient} of analytic accuracy with respect to the knob values.
%     \item With the accuracy gradient, we can better predict the analytic accuracy of those knob values we did not explore yet.
% \end{itemize}

% Our goal is to calculate the gradient of accuracy with respect to knobs (we call this gradient \textit{accuracy gradient}) by only evaluating the system under one configuration.

% Accuracy gradient enables us to better predict the accuracy of different configurations under similar video content.
% As a result, one can pick a chheaper configuration while still achieving the same accuracy with accuracy gradient.


% \begin{comment}

% \subsection{Programming interface of \name}


% \begin{figure}
%     \centering
%     \includegraphics[width=1\columnwidth]{figs/raw-input-inference.jpg}
%     \caption{\name handles those hyper-parameters that preprocess the input to the DNN.}
%     \label{fig:raw-input-inference}
% \end{figure}



% \subsection{API of HPs} 

% As shown in Figure~\ref{fig:raw-input-inference}, \name abstracts the underlying AI systems into two stages.
% In the preprocessing stage, the AI system pre-processes the raw sensing data to obtain the input to the DNN.
% In the inference stage, the DNN performs inference and obtain the analytic results.
% \name focuses on those HPs for preprocessing stage (we will show most of the HPs fall into this category in \S\ref{subsec:hp-examples}, together with some example HPs that do not belong to this category).
% As the preprocessing does not incur the compute-intensive server-side DNNs, we assume that this step can be locally done at the camera.

% Based on this observation, the programming interface of \name towards HPs are:
% \begin{small}
% \begin{verbatim}
% prep(Data raw, List hps)-> (Data input, Bytes encoded)
% proxy(Result result) -> Float pseudo_acc
% \end{verbatim}
% \end{small}

% The first function \texttt{prep} pre-processes the raw sensed data \texttt{raw} based on a list of HPs \texttt{hps}, and return the codec-encoded byte stream \texttt{encoded} and the input data \texttt{input} that server-side DNN will receive.

% The second function aims to provide a differentiable proxy towards accuracy (since most of the existing accuracy function is not differentiable).
% As most of the DNNs will return confidence scores to describe the confidence of the analytic results the DNN derives, we use the sum of the confidence scores as the default proxy.
% This complies with recent computer vision advances on evaluating the quality of inference results.

% Further, we empirically verify this assumption on different types of HPs and different videos.


% \subsection{Examples}
% \label{subsec:hp-examples}


% This assumption precludes those HPs that directly changes server-side DNN (\eg customizing the server-side DNN or switching between different server-side DNNs).
% That said, the vast majority of HPs, including HPs of traditioanal data encoding codecs (\eg frame rate, resolution, quantization parameters etc), DNN-based encoding codec (\eg feature compression, super resolution), fine-grained data quality assignments (\eg region-of-interest selection, macroblock encoding quality selection), sensor-side data filtering (\eg filtering the frames through cheap object detector or through cheap feature extractors) still fit in our assumption. 



% % \mypara{API of DNNs}
% % We require that the DNN to implement two APIs:
% % \begin{small}
% % \begin{verbatim}
% % inference(Data input)-> Result result
% % backprop(Result result, Function f)-> Data grad
% % \end{verbatim}
% % \end{small}



% \subsection{Workflow of \name}

% Contrast between conventional workflow and ours workflow

% \end{comment}







% \subsection{Workflow and API of \name}
% \kt{Goal: how to use the API in our system to calculate accuracy gradient}

% \begin{figure}
%     \includegraphics[width=1\columnwidth]{figs/workflow.jpg}
%     \caption{Workflow of \name \kt{Plot this figure in a "call stack" way, MAKE THE FONT LARGER}}
%     \label{fig:workflow}
% \end{figure}

% \mypara{Workflow of \name} Based on the approach above, we present the workflow of \name in Figure \ref{fig:workflow}.


% Our system enables the application to obtain the gradient of accuracy with respect to the knobs through the following API:
% $$AccGrad = calc(V_t, \{knob_i\}_{i=1}^n)$$

% \mypara{Towards knobs}

% $knob'_i = reduce(knob_i)$
% This reduce the knob to lower knob value

% \mypara{Towards DNN}
% We require the DNN to implement two APIs:
% \begin{packeditemize}
%     \item \texttt{result = inference(V)}
%     \item \texttt{saliency = backprop(result, grad)}
% \end{packeditemize}

% \mypara{Towards application}
% We require the application to implement:
% \begin{packeditemize}
%     \item \texttt{encode(V, knobs)} This one should be locally done on the camera
%     \item \texttt{proxy(results)}
% \end{packeditemize}


% \subsection{How to use the API}






% \subsection{Reduce the cost of accuracy gradient}


% \mypara{Accuracy gradient sampling}


% \mypara{Accuracy gradient compression}



==> overview_v4.tex <==

% \begin{figure*}[t]
%     \centering
%     \includegraphics[width=1.5\columnwidth]{figs/workflow.pdf}
%     \caption{Workflow of \name.}
%     \label{fig:workflow}
% \end{figure*}



% \begin{figure}[t]
%     \centering
%     % \includegraphics[width=0.5\columnwidth]{figs/placeholder-eval-overall-1.pdf}
%     % \subfloat[][\centering{Object detection\\~~~~(Dashcam)}]
%     % {
%     %     \includegraphics[width=0.24\textwidth]{figs/detection_dashcam_FPN.pdf}
%     %     \label{subfig:1}
%     % }
%     \subfloat[][Profiling]
%     {
%         \includegraphics[width=0.32\columnwidth]{figs/behavior_profile.pdf} 
%         \label{subfig:1}
%     }
%     \subfloat[][Output-based]
%     {
%         \includegraphics[width=0.32\columnwidth]{figs/behavior_output.pdf} 
%         \label{subfig:1}
%     }
%     \subfloat[][OneAdapt]
%     {
%         \includegraphics[width=0.32\columnwidth]{figs/behavior_oneadapt_arrow.pdf} 
%         \label{subfig:1}
%     }
    
%     \tightcaption{Contrasting \name with profiling-based approach and output-based approach. \name quickly approaches the optimal point via the gradient vector, while the profiling-based method requires a high amount of extra inference to derive the optimal configuration, and the output-based method approaches the optimal configuration slowly.}
%     \label{fig:compare}
% \end{figure}


% \begin{figure}[h]
%     \includegraphics[width=1.15\columnwidth]{figs/gradient.jpg}
%     \caption{Gradient \name.}
%     \label{fig:workflow}
% \end{figure}

% \begin{figure*}[h]
%     \centering
%     \includegraphics[width=1.5\columnwidth]{figs/timeline.jpg}
%     \caption{Workflow of \name. \kt{Place a overall workflow figure here.} }
%     \label{fig:workflow}
% \end{figure*}


% \begin{figure*}[h]
%     \includegraphics[width=2.4\columnwidth]{figs/adaptation-time-series.pdf}
%     \caption{Adaptation behavior of \name}
%     \label{fig:workflow}
% \end{figure*}

% \begin{packeditemize}
%     \item Sketch three requirements (1). adapt frequently (2). reach a near-optimal configuration (3). be applicable to a range of configs \& apps.
%     \item \S 3.1
%     \item Introducing \outputgrad 
%     \item Calculating \outputgrad with no extra inference. Need two figures here. 1). Show what is backpropagation 2). show how is backpropagation saves cost.
%     \item Correlation between \outputgrad and accuracy.
%     \item \S 3.2
%     \item Optimizing accuracy through gradient ascent.
%     \item This gradient-ascent-based algorithm allows us to simultaneously achieve 3 objectives.
%     \item Talking about its caveats
%     \item \S 3.3.
%     \item Run people through an end-to-end example, where the sensor and the server are separated by network.
%     Figure: a timeline figure between the sensor and the server Key highlights: when the inference results are obtained, and when the configuration is updated.
% \end{packeditemize}





% \jc{Outline:
% if you agree, how about the following order? you will
% introduce the optimization goal first (current eq 2) and
% then introduce ConfigGrad, and
% before explaining how to calculate ConfigGrad (currently the beginning of 3.2), you should explain why ConfigGrad can help the optimization goal. (this needs some math rigor)
% finally, explain how to calculate ConfigGrad and how to pick the next config
% }
\kt{less math}
\tightsection{Design of \name}
\label{sec:design}
% \tightsection{\outputgrad}
% \jc{Junchen can you check this part? I did a full rewrite to Sec 3.1}

% \jc{this section still feels hard to parse. needs to be simplified, and use less math.}

We present \name, a configuration adaptation system that aims at improving along the three requirements mentioned above --- frequent adaptation to near-optimal configuration on various configuration knobs. %---over prior solutions.
% \jc{to show \name can work on a range of settings, you explicitly say that \name is built on a unifying terminology that applies to different knobs, tasks, and input data types.
% consider laying out all the terminologies at the beginning of 3. right now, they are spread in different places.}

\kt{here}
\kt{merge 3.2 3.3, swap 3.4 3.5}
The basic idea of \name is to frequently estimate 
% The key for \name to meet the three requirements is to calculate 
the {\em gradient} of how inference accuracy changes with each configuration knob, which we refer to as the {\em \accgrad}.
Using the up-to-date estimate of \accgrad, \name incrementally updates the configuration to improve the DNN inference results but still stays in the (compute/network) resource budget or maximally reduces the resource usage with minimum change on the DNN inference results.
% Figure~\ref{fig:adaptation-behavior} illustrates an example: after a change of input data, \name can adapt more frequently and gradually converge to a near-optimal configuration.


We begin by introducing the adaptation goal of \name (\S\ref{subsec:adaptation-goal}), and then introduce the gradient ascent strategy of \name (\S\ref{subsec:gradient-ascent}).
To perform gradient ascent with minimum resource overhead (in terms of GPU cycles), we introduce \outputgrad (\S\ref{subsec:outputgrad}) and present the key insight that the inherent \textbf{differentiability of DNNs enables fast calculation of \outputgrad without extra DNN inference} (\S\ref{subsec:differentiability-outputgrad}).
Last, we state the caveats and benefits of \name (\S\ref{subsec:limitation}).

% changes the configuration to another configuration that meets the (compute/network) resource budget and greatly improves accuracy.\jc{confirm with kuntai}
% to improve accuracy within the resource budget. 



% after the content of the input data changes.
% that allows operators to achieve the following three requirements simultaneously:
% \begin{packeditemize}
%     \item Adapt frequently
%     \item Reach a near-optimal configuration
%     \item Apply to a wide range of configurations and applications
% \end{packeditemize}


% \subsection{Modeling of knobs}

% \name focuses on handling a subset of knobs that satisfies the following two properties:

% \begin{enumerate}
%     \item \textit{\accres}: For each knob, there exists one direction (either increasing or decreasing), if \name fix other knobs and change this knob according to this direction, the resource consumption and the accuracy statistically increases.
%     % (we assume that this direction is increasing the knob value by default) if changing the value of one knob result in spending more (or less) resource, the corresponding inference results also become more (or less) accurate.
%     \item \textit{\blackbox}: Most of the knobs treat DNN as a black box and change the DNN input. We illustrate this point in Figure~\ref{??}.
% \end{enumerate}



\tightsubsection{Terminologies}

% \footnotesize
% \begin{tabular}{|m{0.12\columnwidth}|m{0.49\columnwidth}|m{0.25\columnwidth}|}

We first introduce unified terminology to describe the DNN output on various DNN tasks and types of input data (all notations and terminologies are summarized in Table~\ref{tab:notations}).
% in a way that is relevant to this work. 
% , from object detection in video and audio-to-text translation (see Table~\ref{??} for a list).
We split the source data stream into fixed-length (by default, one-second-long) intervals, called {\em adaptation intervals}.
In the $t^{th}$ adaptation interval, the input data $\Data_t$ is first preprocessed with the current configuration $\Config_t$ and then fed to DNN (see Algorithm~\ref{alg:adapt}), and the DNN output $Res(\Config_t; \Data_t)$ ($Res(\Config_t)$ for short) contains multiple {\em elements}. 
% Note that there might be multiple DNN inferences within an adaptation interval.
An element $e$ can be a detected object in object detection or a detected text in audio-text translation.
Most DNNs for these tasks will associate each element with a confidence {\em score}, and only elements with a score over a confidence {\em threshold} $\theta$ will be counted towards accuracy. 
% \name works with any DNN tasks that return elements with confidence scores as output. 

We then define the following notations:
\begin{packeditemize}
\item $Acc(\Config_t; \Data_t)$ ($Acc(\Config_t)$ for short) is the accuracy of the inference results generated using input data $\Data_t$ and configuration $\Config_t$. 
Following prior work~\cite{awstream,chameleon,dds,accmpeg,ekya,boggart}, we define accuracy as the \textbf{similarity} between the current inference results and the inference results generated from the most resource-consuming configuration $\Config^*$. 
This definition of accuracy is less ideal than calculating accuracy using human-annotated ground truth, but it directly shows the impact of adapting configurations on inference results.
\item $\Output(\Config_t; \Data_t)$ ($\Output(\Config_t)$ for short) is the \summary of the inference results generated using input data $\Data_t$ and configuration $\Config_t$. We define \summary as the number of above-threshold elements (see \S\ref{sec:definition-of-summary} for the formal definition).
\item $\Resource(\Config_t; \Data_t)$ ($\Resource(\Config_t)$ for short) is the resource usage (bandwidth and/or GPU cycles, defined per application) the $t^{th}$ adaptation interval.
\end{packeditemize}

% For the DNN output in an adaptation interval, we define the {\em \summary} by the number of elements in an adaptation interval whose confidence scores exceed the confidence threshold.
% The rationale of \summary will be explained in detail later in \S\ref{subsec:gradient-ascent}.
% For now, we can think of \summary as a one-value summarization of the DNN output whose change indicates the change in inference accuracy.

% Though the definitions may not be universally applicable, it naturally applies to most prior work in video analytics as well as the new applications mentioned in Table~\ref{tab:applications}.
% developers do not need to make major changes to the DNN to use \name.

\begin{table}[]
\footnotesize
\begin{tabular}{|m{0.13\columnwidth}|m{0.45\columnwidth}|m{0.27\columnwidth}|}
\hline
{\bf Notation}                                                                                              & {\bf Definition}                                                                                                                                                                                                                                 & {\bf Example}                                                                                                         \\ \hline \hline
$n$                                                                                                   & Number of knobs                                                                                                                                                                                                                            & $n=2$                                                                                                           \\ \hline
$t$                                                                                                   & $t^{\textrm{th}}$ adaptation interval (by default, each interval is 1 second)                                                                                                                                                                                         & $t=1$                                                                                                           \\ \hline
$T$                                                                                                   & Total number of adaptation intervals                                                                                                                                                                                                       & $T=60$                                                                                                          \\ \hline
$\Config_t$                                                                                           & Configuration: a vector of knobs with their selected values at interval $t$                                                                                                                                                                & $\Config_1=$(frame rate=10, resolution=480p)                                                                    \\ \hline
$\Knob_{i,t}$                                                                                         & The value of $i^{\textrm{th}}$ knob in configuration $\Config_t$                                                                                                                                                                                    & $\Knob_{2,1}$=480p                                                                                              \\ \hline
$\Delta \Knob_i$                                                                                      & A small increase on the $i^{\textrm{th}}$ knob                                                                                                                                                                                                      & $\Delta \Knob_2$=120p                                                                                           \\ \hline
$\Data_t$                                                                                             & input data at interval t                                                                                                                                                                                                                   &                                                                                                                 \\ \hline
\begin{tabular}[c]{@{}l@{}}$\Resource(\Config_t; \Data_t)$\\ or\\ $\Resource(\Config_t)$\end{tabular} & Resource usage of config $\Config_t$ under $\Data_t$. We omit $\Data_t$ for simplicity                                                                                                                                                     &     $\Resource(\Config_1)=$5Mbps                                                                                                            \\ \hline
\begin{tabular}[c]{@{}l@{}}$Res(\Config_t; \Data_t)$\\ or\\ $Res(\Config_t)$\end{tabular}             & Inference results of config $\Config_t$ under $\Data_t$. We omit $\Data_t$ for simplicity.                                                                                                                                                 & 
\begin{tabular}[c]{@{}l@{}}$Res(\Config_1)=\{$\\
(obj1, ``car'', score: 0.2),\\
(obj2, ``bike'', score: 0.8)\\ $\}$
\end{tabular} 
 \\ \hline
$e$                                                                                                   & An element in the inference results (\eg a detected object). Each element is associated with a confidence score.                                                                                                                           & \begin{tabular}[c]{@{}l@{}}$e=$\\
(obj1, ``car'', score: 0.2)
\end{tabular}                                                                 \\ \hline
$\theta$                                                                                              & Confidence threshold                                                                                                                                                                                                                       & $\theta=0.5$ (default)                                                                                                   \\ \hline
\begin{tabular}[c]{@{}l@{}}$\Input(\Config_t; \Data_t)$\\ or\\ $\Input(\Config_t)$\end{tabular}         & DNN input generated by configuration $\Config_t$ using input data $\Data_t$. We omit $\Data_t$ for simplicity.                                                                                                                                           & ~                                                                                         \\ \hline
\begin{tabular}[c]{@{}l@{}}$\Output(\Config_t; \Data_t)$\\ or\\ $\Output(\Config_t)$\end{tabular}         & Output utility: number of above-confidence-threshold elements. We omit $\Data_t$ for simplicity.                                                                                                                                           & $\Output(\Config_1)=1$                                                                                          \\ \hline
\begin{tabular}[c]{@{}l@{}}$Acc(\Config_t; x_t)$\\ or\\ $Acc(\Config_t)$\end{tabular}                 & Accuracy of the configuration $\Config_t$ under input data $\Data_t$, defined as the similarity between the current inference result $Res(\Config_t)$ and the inference results generated using the most resource-demanding configuration. & $Acc(\Config_1)=100\%$                                                                                          \\ \hline
$\alpha$                                                                                              & Learning rate of \name                                                                                                                                                                                                                     & $\alpha=0.5$ (default)                                                                                                    \\ \hline
$\lambda$                                                                                             & The hyperparameter that trade-off between accuracy and resource usage.                                                                                                                                                                     & $\lambda=1$                                                                                                  \\ \hline
\end{tabular}
\vspace{0.1cm}
\tightcaption{Notations of \name}
\label{tab:notations}
\end{table}






% \kt{3 columns: notation, meaning, example}





\tightsubsection{Adaptation goal of \name}
\label{subsec:adaptation-goal}


% \jc{(1) 3.2 and 3.3 are still a bit too abstract. please use a concrete example like the one in 31
% (2) it’s not clear from 32 (upfront) why configgrad-based gradient ascent can adapt quickly. this should be upfront, not embedded or in the end
% same thing with 33. it’s unclear why this is a smart design
% (3) i dont see the assumptions in 31, 32, 33 be explicitly called out and justified.. did i miss them?}
% \kt{I explicitly called out the assumptions in 31. I will deprioritize other issues before Sunday.}

% We first introduce terminology to describe the DNN output.
% % in a way that is relevant to this work. 
% This is necessary because \name works with various DNN tasks and source data types (see Table~\ref{tab:pipeline} for a list).
% , from object detection in video and audio-to-text translation (see Table~\ref{??} for a list).
% \name splits the source data stream into fixed-length (by default, one-second-long) intervals, called {\em adaptation intervals}.
% In the $i^{th}$ adaptation interval, the data is first preprocessed with the configuration $\Config_i$ and then fed to DNN (see Figure~\ref{fig:workflow}) to obtain the inference results.

% \mypara{Adaptation goal} The goal of \name is: given the configuration of the current interval $\Config_{cur}$, pick the configuration $k^*$ for the next adaptation interval so that a weighted sum between the accuracy and the resource usage is improved.
% Formally, we write this adaptation goal as:
% \begin{align}
% \nonumber
% \text{On the current adaptation interval, find}~~\Config^*&, \text{such that}
% \\
% \underbrace{Acc(\Config^*)}_{\text{\sf \footnotesize \textcolor{black!85}{accuracy}}}
% - 
% \lambda 
% \underbrace{\Resource(\Config^*)}_{{\text{\sf \footnotesize \textcolor{black!85}{resource usage}}}}
% \geq 
% Acc(
% \underbrace{\Config_{cur}}_{\text{\sf \footnotesize \textcolor{black!85}{ current configuration}}}
% ) - &\lambda \Resource(\Config_{cur})
% \end{align}

% \jc{is this in conflict with the "objective" paragraph in 2.1?}
The adaptation goal of \name is to pick configurations (\eg video resolution and frame rate) for all adaptation intervals such that a weighted sum between the accuracy $Acc$ and the resource usage $\Resource$ is maximized:
\begin{equation}
\max_{\Config_1,\cdots,\Config_T}
\sum_{t=1}^T
\underbrace{Acc(\Config_t)}_{\text{\sf \footnotesize \textcolor{black!85}{accuracy of $t^{th}$ interval}}}
- \lambda \underbrace{\Resource(\Config_t)}_{{\text{\sf \footnotesize \textcolor{black!85}{resource usage of $t^{th}$ interval}}}},
\label{eq:objective}
\end{equation}
where
% \begin{packeditemize}
% \item $n$ is the total number of adaptation intervals.
% \item $k_1,\cdots k_n$ are the configurations for each adaptation interval.
% \item $Acc(\Config_t)$ is the accuracy of the $t^{th}$ adaptation interval.
% Following prior work~\cite{awstream,chameleon,dds,accmpeg,ekya,boggart}, we define accuracy as the \textbf{similarity} between the current inference results and the inference results generated from the most resource-consuming configuration. This definition of accuracy is less ideal than calculating accuracy using human-annotated ground truth, but it allows the system to optimize the inference results in the absence of annotated human data, which is the common case in current video analytic applications like traffic footage analytics.
% \item 
% $\Resource(\Config_t)$ is the resource usage (in either bandwidth or GPU cycles, defined per application) the $t^{th}$ adaptation interval.
% \item
$\lambda$ is a hyperparameter that governs the tradeoff between accuracy and resource usage: higher $\lambda$ will emphasize resource-saving and lower $\lambda$ will emphasize accuracy improvement.
We will vary $\lambda$ and examine its effect on \name in \S\ref{sec:eval}.
% \end{packeditemize}


Note that in many applications, the objective in Eq.~\ref{eq:objective}, which linearly combines accuracy and resource usage, is less ideal than optimizing accuracy with a fixed constraint on resource usage.
For instance, one may choose to maximize accuracy, conditioned on the bandwidth usage of the configuration within a budget~\cite{awstream,dds,accmpeg}.
% However, \kt{We need something to defend this formulation}
% Figure~\ref{fig:workflow} shows an example of how \name's gradient-based adaptation process works in the vehicle detection example.
% We will still use the vehicle detection example, where a traffic camera streams its video data to a GPU-equipped server to determine which frame contains vehicles.
% In each adaptation interval, the sensor encodes the video in an adaptation interval using the current configuration (frame rate and resolution) and sends it to a DNN running on a GPU-equipped server.
% The server receives this video and runs DNN inference to get the inference results and runs backpropagation to get \dnngrad and send it back to the sensor. 
% While the server runs DNN inference, the sensor runs encoding multiple times with different to obtain \inputgrad (the change in DNN input with respect to each knob).
% Once the sensor receives \dnngrad, it uses Eq.~\ref{eq:grad-decouple} to calculate \outputgrad.
% It then runs the gradient ascent strategy in Eq.~\ref{eq:gradient} to adapt the configuration and uses the new configuration in the next interval. 


% , and the DNN output contains multiple {\em elements}. 
% % Note that there might be multiple DNN inferences within an adaptation interval.
% An element can be a detected object in object detection, a detected text in audio-text translation, or the classification of a pixel in semantic segmentation.
% Most DNNs for these tasks will associate each element with a confidence {\em score}, and only elements with a score over a confidence {\em threshold} will be counted towards accuracy. 
% \name works with any DNN tasks that return elements with confidence scores as output. 




% \tightsubsection{Observations}

% Explain here that:
% \begin{packeditemize}
%     \item The optimization is concave w.r.t. the configuration $\rightarrow$ gradient-ascent-based optimization to leverage this concavity.
%     \item A better configuration for this adaptation interval is also better for the next adaptation interval unless the video content changes significantly (\eg a new object comes in) $\rightarrow$ it is OK to adjust the configuration gradually over time.
%     \item The two observations inspire a gradient-ascent-based approach.
% \end{packeditemize}





To fulfill the adaptation goal, \name takes a \textbf{gradient ascent strategy}.
% In each adaptation interval, \name first performs DNN inference to obtain the inference results, computes the \textit{gradient}  with respect to the configuration (we will explain how to calculate this gradient shortly) and update the configuration using the gradient.
% \name gradually updates the configuration $\Config$ (\eg current resolution and frame rate) using the \textit{gradient} of the accuracy and the resource usage.


% Ideally, \name would update the $i^{th}$ knob $\Knob_{cur,i}$ in the current configuration $\Config_{cur}$ by:
% \begin{@empty}
% \footnotesize
% \begin{align*}
% \Knob_i^*=\Knob_{cur,i}+ \alpha \left(
% \underbrace{
% \frac{Acc(\Config_{cur} + \Delta\Knob_i) -Acc(\Config_{cur})) }{\Delta \Knob_i}
% }_{\text{\sf \footnotesize \textcolor{black!85}{gradient of accuracy}}}
% - 
% \lambda 
% \underbrace{\frac{\Resource(\Knob_{cur} + \Delta\Knob_i) - \Resource(\Knob_{cur}) }{\Delta\Knob_i}
% }_{\text{\sf \footnotesize \textcolor{black!85}{gradient of resource usage}}}
% \right),
% \end{align*}
% \end{@empty}
% where $\Knob_i^*$ is the updated value of the $i^{th}$ knob, $\Delta\Knob_i$ is a small increase on the $i^{th}$ knob, $\alpha$ is the learning rate for gradient descent (see \S\ref{??} for the concrete value we use): increasing the learning rate $\alpha$ increases the convergence speed of \name, but may miss the optimal value of the accuracy.


% % In each adaptation interval, we perform inference using the current configuration $\Config_{cur}$ (\eg current resolution and frame rate), compute \outputgrad, and then use the following strategy to select a new configuration $\Config$ for the next adaptation interval.
% % the gradient of the objective function $Obj(k)$ with respect to the current configuration $\Config_{cur}$ and update the current configuration by running gradient ascent.

% % In each adaptation interval, we perform inference using the current configuration $\Config_{cur}$ (\eg current resolution and frame rate), obtain the gradient of the objective function $Obj(k)$ with respect to the current configuration $\Config_{cur}$ and update the current configuration by running gradient ascent.

% Formally, the goal of \name is to maximize a weighted sum between the accuracy $Acc$ (defined as the \textit{similarity} between the current inference results and the inference results generated under unlimited resource)\kt{need to defend this definition} and the resource usage $\Resource$:
% \begin{equation}
% \underbrace{Acc(\Config)}_{\text{\sf \footnotesize \textcolor{black!85}{accuracy}}}
% - \underbrace{\lambda \Resource(\Config)}_{{\text{\sf \footnotesize \textcolor{black!85}{resource usage}}}},
% \label{eq:objective}
% \end{equation}
% % where $\Config$ i \name maximizes this weighted sum by running gradient ascent (depicted in FIgure~\ref{fig:workflow}).
% where $\lambda$ is a hyperparameter that governs the tradeoff between accuracy and resource usage: higher $\lambda$ will emphasize resource-saving and lower $\lambda$ will emphasize accuracy improvement.
% We will vary $\lambda$ and examine its effect on \name in \S\ref{??}.



\mypara{Ideal way of picking new configuration}
Ideally, \name would update the $i^{th}$ knob $\Knob_{t,i}$ in the current configuration $\Config_{t}$ using the gradient of the objective function in Equation~\ref{eq:objective}:
\begin{@empty}
\footnotesize
\begin{align}
\Knob_{t+1,i}=\Knob_{t,i}+ \alpha \left(
\underbrace{
\frac{\Acc(\Config_t+\Delta \Knob_i) - \Acc(\Config_t)) }{\Delta \Knob_i}
}_{\text{\sf \footnotesize \textcolor{black!85}{gradient of accuracy (\textbf{\accgrad})}}}
- 
\lambda 
\underbrace{\frac{\Resource(\Config_t+\Delta \Knob_i) -\Resource(\Config_t)) }{\Delta \Knob_i}
}_{\text{\sf \footnotesize \textcolor{black!85}{gradient of resource usage}}}
\right),
\end{align}
\label{eq:ideal-adaptation}
\end{@empty}
where $\Knob_{t+1,i}$ is the value of the $i^{th}$ knob on the next adaptation interval, $\Delta\Knob_i$ is a small increase on the $i^{th}$ knob, $\alpha$ is the learning rate for gradient descent:
% \footnote{We normalize the range of all knobs to [0,1] and use 0.5 as our learning rate.}: 
increasing the learning rate $\alpha$ increases the convergence speed of \name, but \name may not converge to a near-optimal configuration if $\alpha$ is too large. We let $\alpha=0.5$ by default.

% We calculate $\frac{\Resource(\Knob_{cur,i} + \Delta\Knob_i) - \Resource(\Knob_{cur,i}) }{\Delta\Knob_i}$ by following its definition, which imposes extra overhead on \name (we will evaluate this overhead in \S\ref{??}) but does not require extra DNN inference.

From Equation~\ref{eq:ideal-adaptation}, we see that updating the configuration requires calculating the gradient of accuracy (hereinafter \accgrad) and the gradient of resource usage.
We calculate the gradient of resource usage by using the pre-profiled resource usage of each configuration $\Resource(\Config)$ (this aligns with prior work~\cite{chameleon,dds,reducto}), which might vary with different input data, but the relative difference among them has little variance.
However, it is computationally expensive to calculate \accgrad using its definition
% $$
% \frac{\Acc(\Config_t+\Delta \Knob_i) - \Acc(\Config_t)) }{\Delta \Knob_i}
% $$
as calculating the accuracy $Acc$ requires generating the inference results using the most resource-consuming configuration.
% (recall that we define accuracy as the similarity between this inference results and the current inference results).

\mypara{\outputgrad as an approximation}
\name instead leverages \outputgrad to approximate the gradient of accuracy and to update the configuration:
% The rationale behind this approximation is that:
% if one knob is of large \outputgrad, increasing this knob will significantly change the DNN output $\Output$, and thus also significantly affects the accuracy $Acc$, leading to a large change of accuracy.
% We will further explain when and why \outputgrad can approximate the gradient of accuracy in \S\ref{??}.
% On the contrary, if the \outputgrad of one knob is small, increasing this knob does not affect the DNN $\Output$, and thus the corresponding accuracy change is also marginal.

\vspace{-0.3cm}
\begin{@empty}
\footnotesize
\begin{align}
\Knob_{t+1,i}=\Knob_{t,i}+ \alpha 
\left(
\underbrace{
\frac{\Output(\Config_t+\Delta \Knob_i) - \Output(\Config_t)) }{\Delta \Knob_i}
}_{\text{\sf \footnotesize \textcolor{black!85}{\textbf{\outputgrad}}}}
- 
\lambda 
\underbrace{
\frac{\Resource(\Config_t+\Delta \Knob_i) - \Resource(\Config_t)) }{\Delta \Knob_i}
}_{\text{\sf \footnotesize \textcolor{black!85}{gradient of resource usage}}}
\right).
\label{eq:real-adaptation}
\end{align}
\end{@empty}
\noindent
% \kt{Add a circle in configgrad} \kt{talk about resource usage gradient: why it is easy to get}
% \kt{talk about how to perform gradient ascent in one step}
% where we will explain what is \outputgrad and how to calculate \outputgrad in the following sections.
We will introduce the definition of \outputgrad and illustrate why it can be used to approximate the gradient of accuracy in the next section.
% The pseudo-code of \name's adaptation logic using \outputgrad is presented in Algorithm~\ref{alg:adapt}.
% In the following sections, we will focus on three questions regarding \outputgrad:
% \begin{packeditemize}
% \item What is \outputgrad
% \item Why \outputgrad can be used to approximate the gradient of accuracy
% \item How to calculate \outputgrad
% \end{packeditemize}
% note that we take the absolute value to \outputgrad, as we assume that increasing the knob values increases the resource usage (and thus increases the accuracy).



% To further support the claim that \outputgrad correlates with the gradient of accuracy, we empirically 
% We notice that the \textit{cosine similarity} between \outputgrad and AccGrad is higher than 0.95 (we provide a formal proof that AccGrad is equals to \outputgrad using an idealized accuracy function, see \S\ref{??}), so substituting it with the accuracy can still guide \name to the optimal configuration.

% % To adapt configurations using \outputgrad, 
% \name runs gradient ascent (depicted in Figure~\ref{fig:workflow}) to converge to a near-optimal configuration.
% % First, we partition the input data stream (\eg video frames) into {\em adaptation intervals}, each of one second.
% In each adaptation interval, we perform inference using the current configuration $\Config_{cur}$ (\eg current resolution and frame rate), compute \outputgrad, and then use the following strategy to select a new configuration $\Config$ based on \outputgrad. 

% The goal of \name's gradient ascent is maximizing a weighted sum between \summary (number of elements with scores over the confidence threshold) and resource usage (we will discuss alternative formulations shortly):

% \vspace{-0.4cm}
% \begin{@empty}
% \small
% \begin{align}
% {\color{black}\underbrace{\highlight{white}{$\Output_{\Config}(\Data)$}}_{\text{\sf \footnotesize \textcolor{black!85}{\summary}}}}-\lambda {\color{black}\underbrace{\highlight{white}{$\Resource(\Config)$}}_{\text{\sf \footnotesize \textcolor{black!85}{resource usage}}}} \label{eq:objective}
% \end{align} 
% \end{@empty} 
% Here, $\Resource(\Config)$ is the resource usage (in either bandwidth or GPU cycles, defined per application) of \Config.
% The hyperparameter $\lambda$ governs the tradeoff between accuracy and resource usage: higher $\lambda$ will emphasize resource-saving and lower $\lambda$ will emphasize accuracy improvement.
% \hl{Note that we will vary $\lambda$ and study its impact in \S\ref{sec:eval}.}
% % As shown in prior work, for most configuration knobs (\eg frame rate, resolution, etc), $Resource(\Config)$ can be accurately pre-profiled and does not vary with input content as much as inference results.

% Given the current configuration $\Config_t$ at the interval $t$ and the \outputgrad $\Grad_t$ (a vector of each knob's \outputgrad), the new configuration used for the next interval $t+1$ should be the one that maximizes the improvement of the objective. 
% Formally, we can express it by 

% \vspace{-0.4cm}
% \begin{@empty}
% \small
% \begin{align}
% \Config_{t+1}=\textrm{argmax}_{\Config}{\color{black}\underbrace{\highlight{white}{$(\Config-\Config_t)\cdot \Grad_t$}}_{\text{\sf \footnotesize \textcolor{black!85}{change in \summary}}}}-\lambda {\color{black}\underbrace{\highlight{white}{$(\Resource(\Config)-\Resource(\Config_t))$}}_{\text{\sf \footnotesize \textcolor{black!85}{change in resource}}}} \label{eq:gradient}
% \end{align}
% \end{@empty}
% % $\Config_{t+1}=\textrm{argmax}_{\Config} (\Config-\Config_t)\cdot Grad_t-\lambda (\Resource(\Config)-\Resource(\Config_t))$
% The new configuration $\Config_{t+1}$ will be used for the next adaptation interval. 
% Following prior work~\cite{chameleon,dds,reducto}, we pre-profile the resource usage of each configuration $\Resource(\Config)$, which might vary with source data, but the relative difference among them has little variance.

% In many applications, the objective in Eq.~\ref{eq:objective}, which linearly combines resource usage and \summary, is less reasonable than optimizing \summary with a fixed constraint on resource usage.
% For instance, one may choose to maximize \summary (which relates to accuracy as explained shortly), conditioned on the bandwidth usage of the configuration within a budget.
% Figure~\ref{fig:workflow} shows an example of how \name's gradient-based adaptation process works in the vehicle detection example.
% In each adaptation interval, the sensor encodes the video in an adaptation interval using the current configuration (frame rate and resolution) and sends it to a DNN running on a GPU-equipped server.
% The server receives this video and runs DNN inference to get the inference results and runs backpropagation to get \dnngrad and send it back to the sensor. 
% While the server runs DNN inference, the sensor runs encoding multiple times with different to obtain \inputgrad (the change in DNN input with respect to each knob).
% Once the sensor receives \dnngrad, it uses Eq.~\ref{eq:grad-decouple} to calculate \outputgrad.
% It then runs the gradient ascent strategy in Eq.~\ref{eq:gradient} to adapt the configuration and uses the new configuration in the next interval. 
% \jc{kuntai, remember to justify why resource usage of a config can be known in advance? what about the frame-diff threshold in reducto?}

% the encoded video that the camera sent, decodes this video, and runs DNN inference to obtain the inference results.
% Then, the server calculates the saliency using the backpropagation and streams the saliency back to the camera.
% Finally, the camera receives the saliency, calculates \outputgrad, and adapts the configuration accordingly.
% \jc{kuntai, please update figure~\ref{fig:workflow} to include the gradient-based adaptation process.}

% 






\tightsubsection{Approximating \accgrad using \outputgrad}
\label{subsec:outputgrad}



\begin{figure*}[t]
    \centering
    % \includegraphics[width=0.5\columnwidth]{figs/placeholder-eval-overall-1.pdf}
    % \subfloat[][\centering{Object detection\\~~~~(Dashcam)}]
    % {
    %     \includegraphics[width=0.24\textwidth]{figs/detection_dashcam_FPN.pdf}
    %     \label{subfig:1}
    % }
    \subfloat[][Calculating \outputgrad using its definition]
    {
        \includegraphics[width=1.6\columnwidth]{figs/gradient-before-new.pdf} 
        % {figs/gradient-before_haodong.jpg} 
        \label{subfig:gradient-before}
    }
    \\
    \subfloat[][Calculating \outputgrad using \name]
    {
        \includegraphics[width=1.6\columnwidth]{figs/gradient-after-new.pdf} 
        % {figs/gradient-after_haodong.jpg} 
        \label{subfig:gradient-after}
    }
    % \subfloat[][Pipeline \circled{8}]
    % {
    %     \includegraphics[width=0.24\textwidth]{figs/lidar_video_e2e.pdf} 
    %     \label{subfig:1}
    % }
    % \subfloat[][Keypoint detection (Skate)]
    % {
    %     \includegraphics[width=0.22\textwidth]{figs/placeholder-eval-overall-2.pdf}
    %     \label{subfig:2}
    % }
    % \\
    % \subfloat[][Adapting configuration using \outputgrad]
    % {
    % \centering
    %     \includegraphics[width=1.8\columnwidth]{figs/workflow.pdf} 
    %     % {figs/gradient-after_haodong.jpg} 
    %     \label{fig:workflow}
    % }
    \tightcaption{Comparison between calculating \outputgrad naively and calculating \outputgrad using \name. \name calculates \outputgrad with \textit{no extra inference}. Note that the image of the DNN is cropped from this\cite{dnnimagesource} GitHub page.}
\end{figure*}








% takes a different approach by focusing on the \textit{gradient} of inference results in relation to the current configuration, referred to as \outputgrad.

% \mypara{Definition and example}
% Intuitively, the \outputgrad is the amount that the DNN inference output would change
% % \footnote{\kt{Talk about how to calculate inference results change. The calculation depends on whether Haodong's experiment works or not.}} 
% if a small adjustment was made to each knob in the current configuration.

% Though it sounds conceptual, \outputgrad can be explained with a simple 
% video analytics system that feeds each video frame to a DNN that determines whether it contains vehicles or not. 
% % Before that, we first explain the concept of \outputgrad in a concrete example.
% % consider an analytic system that analyzes a dashcam video feed by running a DNN to classify each video frame as containing a vehicle or not.
% Following prior work~\cite{chameleon,??}, we assume the system can tune two configuration knobs, frame rate and resolution.
% Suppose that the current configuration is 20fps and 480p, and the DNN output\footnote{Typical DNN output is more than a single value. Here, we assume that for a given video segment, the output of DNN inference is the average confidence of all detected objects. We will explain in \S\ref{??} how we turn the DNN output to a single value in general cases.} on a video segment is 0.9, and if we slightly increase the frame rate from 20fps to 21fps, the DNN output on the same video segment becomes 0.91.
% Then the \outputgrad of frame rate is (0.91-0,9)/(21-20)=0.01.
% Following a similar procedure, we calculate the \outputgrad of the resolution, say its value is -0.02.


% We now define \outputgrad first, then explain how to estimate \outputgrad efficiently, and finally why using \outputgrad to adapt configuration improves accuracy.
% describe the assumptions we make to calculate \outputgrad, define \outputgrad and then explain how to calculate \outputgrad and why one can use it to improve inference accuracy.


% \mypara{Terminology}
% To formally define \outputgrad, 
% We first introduce terminology to describe the DNN output.
% % in a way that is relevant to this work. 
% This is necessary because \name works with various DNN tasks and source data types (see Table~\ref{tab:pipeline} for a list).
% % , from object detection in video and audio-to-text translation (see Table~\ref{??} for a list).
% Recall that we split the source data stream into fixed-length (by default, one-second-long) intervals, called {\em adaptation intervals}.
% In each adaptation interval, the data is first preprocessed with the current configuration and then fed to DNN (see Algorithm~\ref{alg:adapt}), 
Recall that \name assumes the DNN output contains multiple {\em elements}. 
% Note that there might be multiple DNN inferences within an adaptation interval.
An element can be a detected object in object detection, a detected text in audio-text translation, or the classification of a pixel in semantic segmentation.
Most DNNs for these tasks will associate each element with a confidence {\em score}, and only elements with a score over a confidence {\em threshold} will be counted towards accuracy. 
% \name works with any DNN tasks that return elements with confidence scores as output. 

For the DNN output in an adaptation interval, we define the {\em \summary} by the number of elements in an adaptation interval whose confidence scores exceed the confidence threshold.
The rationale of \summary will be explained in detail later in \S\ref{subsec:gradient-ascent}.
For now, we can think of \summary as a one-value summarization of the DNN output whose change indicates the change in inference accuracy.

Though the definitions may not be universally applicable, it naturally applies to most prior work in video analytics as well as the new applications mentioned in Table~\ref{tab:applications}.
% developers do not need to make major changes to the DNN to use \name.






% \mypara{Assumption to the DNNs}
% We require the DNNs to expose the confidence scores in their inference results and the confidence threshold.
% Note that it does not impose an extra burden on the applications since most of the applications already expose confidence scores to indicate the uncertainty of DNN outputs and use confidence thresholds to filter out DNN outputs with low confidence. 
%those uncertain results returned from the DNN.

\mypara{Definition of \outputgrad}
\outputgrad is how much a small change in the current value of each knob changes the \summary (the number of DNN-returned elements in an adaptation interval with confidence scores over the confidence threshold).
Here, we use $\Output(\Config_t)$ to denote the \summary 
% averaged number of elements with confidence over the threshold in the DNN output 
under configuration $\Config_t$ (see \S\ref{sec:definition-of-summary} for the formal definition).
% \kt{Illustrate how we make the \# of above-threshold confidence scores differentiable here.}


We then define the \outputgrad of knob $\Knob_i$ is

\vspace{-0.2cm}
\begin{@empty}
\footnotesize
\begin{equation*}
\frac{\Delta \Output}{\Delta k_i} = \frac{\Output{(\dots,\Knob_{t,i}+\Delta \Knob_i,\dots)}-\Output{(\dots,\Knob_{t,i},\dots)}}{(\Knob_{t,i}+\Delta \Knob_i) - \Delta \Knob_i}.
\end{equation*}
\end{@empty}

% Specifically, we use the following 
% \jc{Kuntai, please write the math expression here}
% confidence scores greater than the confidence threshold averaged across different data frames (\eg video frames).
% Intuitively, the \outputgrad is the amount that the DNN inference output would change
% if a small adjustment was made to each knob in the current configuration.
To help understand \outputgrad, we use a simple 
video analytics system that feeds each video frame to a DNN that performs vehicle detection with a confidence score of 0.5. 
Figure~\ref{subfig:gradient-before} illustrates \outputgrad in this example.
Following prior work~\cite{chameleon,vstore,videostorm,casva}, we assume the system can tune two configuration knobs, frame rate, and resolution.
Suppose that the current configuration is 10 frames per second (fps) and 480p.
% The analytic system will take a one-second-long, 20fps and 480p video and analyzes it through DNN.
When taking 1-second input, the DNN outputs 34 vehicle bounding boxes with confidence scores greater than 0.5 on these 10 frames, an average of 3.4 vehicles per frame.
% \footnote{Typical DNN output is more than a single value. Here, we assume that for a given video segment, the output of DNN inference is the average confidence of all detected objects. We will explain in \S\ref{??} how we turn the DNN output to a single value in general cases.} 
If we slightly increase the frame rate from 10fps to 15fps, the DNN outputs 66 vehicle bounding boxes with confidence scores greater than 0.5, on average 4.4 vehicles per frame.
Then the \outputgrad of the current frame rate is 

\vspace{-0.3cm}
\begin{@empty}
\footnotesize
\begin{align*}
\frac{\Delta \Output}{\Delta \text{framerate}}&=\frac{\Output{(480p,15fps)}-\Output{(480p,10fps)}}{15fps-10fps}=\frac{4.4-3.4}{15-10}=0.2.
% ,\\
% \frac{\Delta \Output}{\Delta \text{resolution}}&=\frac{\Output_{(720p,10fps)}-\Output_{(480p,10fps)}}{720p-480p}=0.01.
\end{align*}
\end{@empty}
% is (3.8-3.4)/(15-10)=0.08.
Following a similar procedure, we assume that the \outputgrad of the resolution will be:

\vspace{-0.3cm}
\begin{@empty}
\footnotesize
\begin{align*}
\frac{\Delta \Output}{\Delta \text{resolution}}&=\frac{\Output{(720p,10fps)}-\Output{(480p,10fps)}}{720p-480p}=\frac{5.8-3.4}{720-480}=0.01.
\end{align*}
\end{@empty}






\begin{figure*}
    \centering
    \includegraphics[width=1.6\columnwidth]{figs/workflow.pdf} 
    \tightcaption{Adapting configuration using \outputgrad. 
    Note that as the adaptation process happens \textbf{after} obtaining the inference results, the end-to-end delay (\ie the delay of obtaining the inference results) is not affected by \name unless the resources are not enough for \name to process the input in real time.
    }
    \label{fig:workflow}
\end{figure*}

% Figure~\ref{subfig:gradient-before} illustrates the calculation of \outputgrad in the vehicle detection example.
% In this figure, we use $\Output_\Config(\Data)$ to denote the averaged number of above-threshold confidence scores in the DNN output at input data $\Data$ using configuration $\Config=(\Knob_i)_{i=1,\dots,n}$ (a vector of $n$ knob values), then \outputgrad of knob $\Knob_i$ is


% As a result, we have 
% \begin{@empty}
% \footnotesize
% \begin{align*}
% \frac{\Delta \Output}{\Delta \text{framerate}}&=\frac{\Output_{(480p,15fps)}-\Output_{(480p,10fps)}}{15fps-10fps}=0.08,\\
% \frac{\Delta \Output}{\Delta \text{resolution}}&=\frac{\Output_{(720p,10fps)}-\Output_{(480p,10fps)}}{720p-480p}=0.01.
% \end{align*}
% \end{@empty}








% We will soon show that there is a statistical correlation between \outputgrad and the accuracy of other configurations



% , each with 5 possible values (1 to 5 for simplicity),
% We assume that the current configuration is $(\Knob_1=2,\Knob_2=2)$.
% The \outputgrad of the two configuration knobs are:
% \jc{Use a concrete example. don't use values 1-5}

% \vspace{-0.3cm}
% \begin{@empty}
% \footnotesize
% \begin{align*}
%    & \frac{\Delta \Output}{\Delta \Knob_1}=\frac{\Output(\Knob_1=3,\Knob_2=2)-\Output(\Knob_1=2,\Knob_2=2)}{3-2}=0.2\\
%    & \frac{\Delta \Output}{\Delta \Knob_2}=\frac{\Output(\Knob_1=2,\Knob_2=3)-\Output(\Knob_1=2,\Knob_2=2)}{3-2}=0.2=0.1,
% \end{align*}
% \end{@empty}
% where $O(res=a, fps=b)$ means the corresponding inference results when configuring $res=a$ and $fps=b$.
% \kt{I guess we need a figure here.}


% Essentially, \outputgrad indicates how the \summary of DNN inference results (\eg the number of detected objects) change with the value of each configuration knob. 
% As shown in \S\ref{subsec:gradient-ascent}, \name's fast adaptation algorithm relies on \outputgrad to tune knob values in the ``direction'' that most improves accuracy or reduces resource usage without hurting accuracy (\S\ref{subsec:limitation}).
% But first, we need to calculate \outputgrad quickly and using minimum GPU cycles. 


\mypara{Why \outputgrad can approximate gradient of accuracy}
Intuitively, \outputgrad captures how much the inference results change when adjusting the configuration by a little.
As a significant change in the inference results (\ie large \outputgrad) is often accompanied by a substantial change in accuracy, the corresponding gradient of accuracy also tends to be large.
That said, a big change in the \summary may indicate either more increase or decrease in accuracy. 
To decide the direction of change, we use the empirical observation that when a change in knob value increases the resource usage, the impact on inference accuracy should be positive (\eg higher encoding resolution leads to higher bandwidth usage and likely more accurate inference, or higher frame rate leads to higher GPU usage and likely more accurate inference). 

To further support this point, we provide a theorem that shows the correlation between \accgrad and \outputgrad.

% \jc{the theorem is way too long. how about you move the assumptions out from the theorem, and the theorem can simply say under xxx assumptions, we have xxx.}

\mypara{Theorem} using a simple accuracy function that counts the number of correctly-detected elements minus the number of wrongfully-detected elements, under the following assumptions:
\begin{packeditemize}
% \item : $Acc(\Config) = \sum_{e\in Res(\Config)} C(e) \cdot step(e.score - \theta)$, where $e$ is an element (\eg an object bounding box with its confidence score) in inference results $Res(\Config)$, $C(e)=1$ if $e$ is detected under the most expensive configuration, and $C(e)=-1$ if not, $step(x) = Sigmoid\left(\alpha x\right)$.
\item 
The accuracy of all elements increases when we give the system more resources by increasing/decreasing the knob values (we assume increasing the knob value increases resource usage for simplicity).
% $\forall e \in Res(\Config),
% \frac{\partial (C(e) \cdot step(e.score-\theta))}{\partial \Config} > 0,$
\item 
Except for the confidence score, other properties of each element (\eg bounding box coordinates) do not affect the accuracy.
% $\forall e \in Res(\Config)$, $\frac{\partial C(e)}{\partial \Config} = 0.$ 
\item 
Different elements do not overlap (\eg object bounding boxes do not mutually overlap).
% $$\left| \frac{\sum_{e\in Res(\Config)} \partial step(e.score-\theta)}{\partial \Config} \right| =  \sum_{e\in Res(\Config)} \left|\frac{\partial step(e.score-\theta)}{\partial \Config} \right|,$$ where $|\cdot|$ means taking element-wise absolute value.
\end{packeditemize}
we have $
\underbrace{\frac{\partial Acc(\Config)}{\partial \Config}}_{\text{\sf \footnotesize \textcolor{black!85}{\accgrad}}} = \bigg| \underbrace{\frac{\partial \Output(\Config)}{\partial \Config}}_{{\text{\sf \footnotesize \textcolor{black!85}{\outputgrad}}}}\bigg|
$.


% gradient of accuracy is exactly \outputgrad under a special case of accuracy function (count the number of elements (\ie object detection bounding boxes) that are correctly detected) and two assumptions:
% \begin{packeditemize}
% \item If an element (\eg an object) is confidently detected (\ie with a confidence score above threshold), it will either be 
% \item There is only one object that the confidence score is around the confidence threshold (\eg the absolute difference between the confidence score and the threshold is smaller than 0.1).
% \end{packeditemize}




Please see \S\ref{sec:proof} for the proof of this theorem. 

As real applications will use a different accuracy function (\eg F1 score~\cite{dds,eaar,chameleon,awstream,vstore,boggart,reducto}) compared to the proof above, we empirically verify whether the change in output (\ie \outputgrad)) is proportional to the change in accuracy (\ie \accgrad).
We pick three configuration knobs (frame sampling rate, resolution, quantization parameter) that are widely used by prior work~\cite{chameleon,casva,awstream,videostorm,vstore,mcdnn} and a 6-second video chunk to verify the correlation between \outputgrad and \accgrad on all configurations (125 configurations in total).
Figure~\ref{fig:accuracy-proxy} shows that on one 9-second video chunk, the change of DNN output (X-axis) nicely correlates with the accuracy change (Y-axis), with a Pearson coefficient of 0.702.

% \kt{Plot this figure if we have time}
% \kt{no we don't}
% As our accuracy function varies between applications, we also empirically examine the correlation between \outputgrad and the gradient of accuracy.
% Concretely, on a 1-minute-long video, we partition this video to 60 one-second adaptation intervals, obtain \outputgrad and the gradient of accuracy on each interval, and then calculate the cosine similarity between them.
% We found that the cosine similarity is higher than \fillme\% for most of the cases.





\tightsubsection{Using DNN differentiability to calculate \outputgrad}
\label{subsec:differentiability-outputgrad}

Recall that \name calculates \outputgrad on every adaptation interval.
As a result, \outputgrad needs to be calculated with minimum overhead (in terms of GPU overhead, see \S\ref{sec:cost} for optimizations on other types of overhead).
As shown in Figure~\ref{subfig:gradient-before}, a naive calculation of \outputgrad requires 
% through its definition results in high GPU overhead (
$n$ extra DNN inferences for $n$ configuration knobs.
However, we calculate \outputgrad \textit{with no extra DNN inference} by taking advantage of the {\bf differentiability of DNNs}. 

First, we decouple \outputgrad into two terms:
\begin{packedenumerate}
    \item {\em \dnngrad:} how the number of above-threshold confidence scores changes with different parts of DNN input (\Input).
    \item {\em \inputgrad:} how much different parts of DNN input change with each knob value of the current configuration (\Config). %in relation to the change in the current configuration.
\end{packedenumerate}

Formally, we use $\Input(\Config; \Data)$ ($\Input(\Config)$ for short) to denote the DNN input of configuration $\Config$ at source data $\Data$ . The \outputgrad of $\Knob_i$ on \Data can be expressed by:
% \vspace{-0.3cm}
% \begin{align}
$
{\color{black}\underbrace{\highlight{white}{$\frac{\displaystyle \Delta \Output}{\displaystyle \Delta \Knob_i}$}}_{\text{\sf \footnotesize \textcolor{black!85}{\outputgrad}}}}=
{\color{black}\underbrace{\highlight{white}{$\frac{\displaystyle \Delta \Output}{\displaystyle \Delta \Input(\Config)}$}}_{\text{\sf \footnotesize \textcolor{black!85}{\dnngrad}}}}\otimes
{\color{black}\underbrace{\highlight{white}{$\frac{\displaystyle \Delta \Input(\Config)}{\displaystyle \Delta \Knob_i}$}}_{\text{\sf \footnotesize \textcolor{black!85}{\inputgrad}}}},
$
% \label{eq:grad-decouple}
% \vspace{-0.08cm}
% \end{align}
where $\otimes$ means inner product.

The decoupling makes the calculation of \outputgrad much more resource-efficient for three reasons:
\begin{packeditemize}
\item The first term (\dnngrad) can be estimated by the DNN's derivation at input $\Input_\Config(\Data)$ via one backpropagation\footnote{
% \kt{Illustrate how we make the \# of above-threshold confidence scores differentiable here.}
To make $\Output$ differentiable, we define it to be $\sum_{e} Sigmoid(\alpha(Score_e-\beta))$ where $Score_e$ is the score of element $e$, $\beta$ is the confidence threshold (see \S\ref{subsec:eval-setup} for its exact value in each application), and $\alpha$ is a hyperparameter (by default, we use 20). Note that this function is almost identical to \summary when $\alpha$ is sufficiently large.
}.
This is a constant GPU-time operation without extra inference as it reuses the layer-wise features computed as part of the DNN inference of the current configuration.
\S\ref{sec:cost} will further reduce the compute overhead of backpropagation.

\item Second, the \dnngrad needs to be calculated once and re-used to derive \outputgrad of different knobs without extra DNN inference.
This is because the \dnngrad describes DNN's sensitivity to its input and thus remains largely similar if the change in DNN input is not dramatic.
For instance, the \dnngrad of an object-detection DNN is high on pixels associated with key visual features of an object.
% \jc{edit ends here}

\item Finally, computing this term does not involve any DNN inference, as it only runs the preprocessing part of the DNN analytics system multiple times.

\end{packeditemize}



% Additionally, 





% Therefore, computing \outputgrad for multiple configuration knobs only requires a one-time backpropagation on GPU and no extra DNN inference.

Figure~\ref{subfig:gradient-after} shows an example of how \outputgrad is calculated from \dnngrad and \inputgrad.
% We use $\Input_{\Config}(\Data)$ to denote the DNN input of configuration $\Config$ at input data $\Data$.
% The decoupling can be written as \outputgrad $\approx$ \inputgrad $\otimes$ \dnngrad, concretely,

\vspace{-0.3cm}
\begin{@empty}
\scriptsize
\begin{align*}
\frac{\Output_{(480p,15fps)}-\Output_{(480p,10fps)}}{15fps-10fps} &\approx \frac{\Input_{(480p,15fps)}-\Input_{(480p,10fps)}}{15fps-10fps} \otimes \frac{\Delta \Output}{\Delta \Input}\bigg|_{\Input=\Input_{(480p,10fps)}},\\
\frac{\Output_{(720p,10fps)}-\Output_{(480p,10fps)}}{720p-480p} &\approx \frac{\Input_{(720p,10fps)}-\Input_{(480p,10fps)}}{720p-480p} \otimes \frac{\Delta \Output}{\Delta \Input}\bigg|_{\Input=\Input_{(480p,10fps)}},
\end{align*}
\end{@empty}
where $\otimes$ represents inner product and $\frac{\Delta \Output}{\Delta \Input}|_{\Input=\Input_{(480p,10fps)}}$ is \dnngrad of the  current configuration $(480p,10fps)$ on the current source data $\Data$.

Importantly, Figure~\ref{subfig:gradient-after} shows that \name saves extra GPU inference by decoupling \outputgrad and re-using the backpropagation results for different knobs.
This example has two knobs, thus the saving may seem marginal, but our evaluation shows more savings when \name is used to adapt more knobs together in more realistic DNN analytics systems (Figure~\ref{fig:fine-grained-knobs}). 


After showing the way \name calculates \outputgrad, we write the adaptation logic of \name in Algorithm~\ref{alg:adapt}.


\begin{algorithm}[ht]
\algrenewcommand{\algorithmiccomment}[1]{\hfill// #1}
\renewcommand{\algorithmicrequire}{\textbf{Input:}}
\renewcommand{\algorithmicensure}{\textbf{Output:}}
% \renewcommand\thealgorithm{}
\caption{\name adaptation logic at adaptation interval $t$}
\begin{algorithmic}[1]
    \Require{inference results $results$, configuration $(\Knob_{t,1},\cdots,\Knob_{t,n})$ at adaptation interval $t$, input data $\Data_t$, DNN input $input$}
    \Ensure{updated configuration $(\Knob_{t+1,1},\cdots,\Knob_{t+1,n})$}
    % \State{$input$ $\gets$ process($\Data_t$, $(\Knob_{t,1},\cdots,\Knob_{t,n})$)} \algorithmiccomment{input processing}
    % \State{$results$ $\gets$ DNN($input$)}  \algorithmiccomment{DNN inference}
    % \State{\color{red}\quad // ~ Delay of inference results only depends on previous 2 lines} 
    \State{$DNNGrad$ $\gets$ $\left|\frac{\partial \Output(results[-1])}{\partial input}\right|$}  \algorithmiccomment{backpropagation using the results on the last data frame, see \S\ref{subsec:saliency_sampling}.}
    \For{$i \gets 1$ to $n$}  \algorithmiccomment{$n$ is number of knobs}
        \State{$InputGrad_i$ = $\left|\frac{process(\Data_t, (\cdots, k_{t,i} + \Delta k_i, \cdots)) - input}{\Delta k_i}\right|$}
        \State{$ConfigGrad_i = DNNGrad \otimes InputGrad_i$}
        \State{$ResourceGrad_i = \frac{\Resource(\cdots, k_{t,i} + \Delta k_i, \cdots)-\Resource(\cdots, k_{t,i}, \cdots)}{\Delta k_i}$}
        \State{$k_{t+1,i} = k_{t,i} + \alpha 
        \left(
        ConfigGrad_i
         - \lambda~ ResourceGrad_i \right)$}
    \EndFor
    
\end{algorithmic}
\label{alg:adapt}
\end{algorithm}


% \kt{\hl{Claim we are the first one who uses backprop for config adaptation here. I think it's better to mention saliency-based works  in related work rather than here.}}
We want to clarify that while \name is \textbf{the first} to leverage DNN differentiability for configuration adaptation, DNN differentiability has already been widely used in DNN training, DNN interpretability, and localization of areas most responsible for the DNN output~\cite{vision-saliency-1,vision-saliency-2}.
It should also be pointed out that \dnngrad differs from the traditional notion of ``saliency'' used in video compression~\cite{fischer2021saliency,hadizadeh2013saliency}, in that \dnngrad is derived directly from a particular DNN to capture how the input influences the DNN output. 

% Note that \name is the first system that leverages the differentiability of DNNs for configuration adaptation, though not the first one that leverages differentiability of DNNs in DNN serving system\footnote{For example, in computer vision community, people use backpropagation to localize which areas of the objects are responsible for the DNN output~\cite{vision-saliency-1,vision-saliency-2}.}. 
% We also aware that there is a recent trend in multi-media community that compress videos by estimating the saliency (\ie the regions in the input video that may contain objects) and encoding these regions in encoding quality.
% Also, there is a line of work from multi-media community~\cite{fischer2021saliency,chen2022context} that leverages saliency estimators to  estimates the areas in the DNN input that contain objects, and then enocde these areas in higher encoding quality so that the objects in these areas can be better detected.
% The notion of saliency may conceptually seems similar to \dnngrad (as both highlight the areas that are related to objects), 
% Also, conceptually \dnngrad is similar to saliency (the areas in the input video that may contain objects) in multi-media community that 

% However, these saliency estimato
% \kt{1. Backpropagation is used in model serving system for explanation.
% But we are the first one to use it for config adaptation
% 2. MM community use saliency to compress video.
% It may seems similar, but our saliency is aware of the final DNN and they are not (drawbacks).}
% \mypara{\dnngrad v.s. existing saliency estimators}
% \dnngrad captures the saliency of the DNN (defined as a map that quantifies the importance of different areas in the DNN input), where there are existing works that also serves the same purposes~\cite{accmpeg,dds,eaar,vigil,fischer2021saliency}.
% However, \dnngrad outperforms existing saliency map estimation algorithms.
% \begin{packeditemize}
%     \item Compared to generating saliency using cheap models~\cite{accmpeg,vigil,fischer2021saliency}, \dnngrad prioritizes those objects according to the likeliness of changing the number of objects detected (where cheap models may mark all objects~\cite{fischer2021saliency} as salient or wrongfully assign saliency to those objects that are detected with high confidence~\cite{accmpeg}).
%     \item One may also generate saliency based on region proposals (an intermediate result generated alongside DNN inference that includes regions potentially containing objects). Compared to this approach, \dnngrad can further rank the pixels inside each object, where this approach will mark all pixels inside an object as salient/non-salient.
% \end{packeditemize}

% \kt{Compare our saliency v.s. others saliency here}


% \mypara{Assumption to configuration knobs}





% First, 
% Second, \dnngrad further prioritizes the pixels inside and outside the object bounding boxes according to the likeliness of changing the number of objects detected, where 

% However, \name calculates this saliency using backpropagation instead of using cheap saliency estimators, allowing \name to derive a metric (\outputgrad) that directly correlates with inference accuracy.
% The cheap saliency estimators fail to correlate with inference accuracy in some cases.
% For example, one may use cheap neural network to estimate saliency~\cite{accmpeg,?,?}.
% However, these cheap saliency estimators will \kt{finish this.}






% Specifically, \name measures \outputgrad by how much a small change in the current value of each knob \textit{flips} the DNN-returned confidence scores from below (or above) the confidence threshold to above (or below). 
% It does not impose an extra burden on the applications to require them to expose confidence scores and confidence thresholds since most of the applications already expose confidence scores to indicate the uncertainty of DNN outputs and use confidence thresholds to filter out DNN outputs with low confidence. %those uncertain results returned from the DNN.
% Statistically, more changes in the ``near-confidence-threshold'' DNN outputs will likely cause more changes in the inference accuracy (as will be elaborated in \S\ref{subsec:correlation})\footnote{This correlation does \textit{not} assume that a confidence score always directly indicates the accuracy of its corresponding detection/classification results.}.
% % \outputgrad correlates with how much the accuracy \textit{changes} with knobs 
% Intuitively, this is because the confidence threshold determines whether a detection or classification result is accepted (as part of the accuracy calculation) or rejected (thus having no effect on the accuracy).




% \pagebreak


% We advocate that the adaptation system for DNN-based analytics should provide a new abstraction: \outputgrad, which estimates the gradient of DNN output with respect to individual knobs.
% We define \outputgrad on a designated knob as the change of the DNN-returned \textit{confidence scores} around (both below and above) the \textit{confidence threshold}, divided by the small amount of change of the knob.
% % when changing this knob by a little.
% This definition requires the application to expose the confidence scores inside their inference results and the confidence threshold used to filter the results.
% For most of the applications, the DNN-returned confidence scores and confidence threshold are naturally available, since most of the applications use confidence scores to quantify the uncertainty of the DNN inference results. The application then filters those results with low confidence scores (as these results may contain spurious results) through a confidence threshold.

% We found that \outputgrad nicely correlates with how much the inference accuracy changes with the knobs.
% Intuitively, this is because the confidence threshold determines whether a detection or a classification result is accepted (and thus participating in the accuracy calculation) or rejected (and thus having no effect on the accuracy).
% Thus, more changes of confidence scores near the confidence threshold will likely cause more changes on the inference accuracy.

% This gradient information can help us quickly adapt to the optimal configuration, 
% % among a large number of configurations 
% by assigning more resources to those knobs with high \outputgrad to improve the accuracy and cut the resource usage of those knobs with low \outputgrad to save resource usage (without hurting the accuracy).
% As shown in Figure~\ref{fig:compare}, \name quickly find the optimal configuration through \outputgrad, while the profiling-based approach needs to profile all configurations to obtain the optimal one, and the output-driven approach adapts slowly.




% \begin{figure*}[t]
%     \centering
%     \includegraphics[width=2.2\columnwidth]{figs/workflow.pdf}
%     \caption{Workflow of \name. \kt{$\Delta resolution$ $240p, 1fps$ }people won't immediately realize it's adding. Need some handholding, picking the new configuration}
%     \label{fig:workflow}
% \end{figure*}



% To quickly adapt to optimal configuration with no extra inference, \name calculates the \textit{gradient} of accuracy with respect to the knob (hereinafter \outputgrad).\jc{i suppose you will clean up all \accgrad and replace them with \outputgrad?}
% We define \accgrad as the accuracy change divided by the knob value change when changing the knob value by a little.

% With this gradient, \name can quickly adapt to the optimal configuration in a large configuration space by granting more resource to the knobs with high \accgrad to improve the accuracy, and cutting the resource usage of those knobs with low \accgrad to reduce the resource usage without hurting accuracy.

% \tightsubsection{Selecting the next configuration}
% \label{subsec:gradient-ascent}


% % \jc{(1) 3.2 and 3.3 are still a bit too abstract. please use a concrete example like the one in 31
% % (2) it’s not clear from 32 (upfront) why configgrad-based gradient ascent can adapt quickly. this should be upfront, not embedded or in the end
% % same thing with 33. it’s unclear why this is a smart design
% % (3) i dont see the assumptions in 31, 32, 33 be explicitly called out and justified.. did i miss them?}
% % \kt{I explicitly called out the assumptions in 31. I will deprioritize other issues before Sunday.}

% With \outputgrad, \name runs \textit{gradient ascent} to converge to a near-optimal configuration.
% In each adaptation interval, we perform inference using the current configuration $\Config_{cur}$ (\eg current resolution and frame rate), compute \outputgrad, and then use the following strategy to select a new configuration $\Config$ for the next adaptation interval.
% % the gradient of the objective function $Obj(k)$ with respect to the current configuration $\Config_{cur}$ and update the current configuration by running gradient ascent.

% % In each adaptation interval, we perform inference using the current configuration $\Config_{cur}$ (\eg current resolution and frame rate), obtain the gradient of the objective function $Obj(k)$ with respect to the current configuration $\Config_{cur}$ and update the current configuration by running gradient ascent.

% Formally, the goal of \name is to maximize a weighted sum between the accuracy $Acc$ (defined as the \textit{similarity} between the current inference results and the inference results generated under unlimited resource)\kt{need to defend this definition} and the resource usage $\Resource$:
% \begin{equation}
% \underbrace{Acc(\Config)}_{\text{\sf \footnotesize \textcolor{black!85}{accuracy}}}
% - \underbrace{\lambda \Resource(\Config)}_{{\text{\sf \footnotesize \textcolor{black!85}{resource usage}}}},
% \label{eq:objective}
% \end{equation}
% % where $\Config$ i \name maximizes this weighted sum by running gradient ascent (depicted in FIgure~\ref{fig:workflow}).
% where $\lambda$ is a hyperparameter that governs the tradeoff between accuracy and resource usage: higher $\lambda$ will emphasize resource-saving and lower $\lambda$ will emphasize accuracy improvement.
% We will vary $\lambda$ and examine its effect on \name in \S\ref{??}.



% \mypara{Ideal way of picking new configuration}
% Ideally, \name would update the $i^{th}$ knob $\Knob_{cur,i}$ in the current configuration $\Config_{cur}$ by:
% \begin{@empty}
% \footnotesize
% \begin{align*}
% \Knob_i^*=\Knob_{cur,i}+ \alpha \left(
% \underbrace{
% \frac{Acc(\Config_{cur} + \Delta\Knob_i) -Acc(\Config_{cur})) }{\Delta \Knob_i}
% }_{\text{\sf \footnotesize \textcolor{black!85}{gradient of accuracy}}}
% - 
% \lambda 
% \underbrace{\frac{\Resource(\Knob_{cur} + \Delta\Knob_i) - \Resource(\Knob_{cur}) }{\Delta\Knob_i}
% }_{\text{\sf \footnotesize \textcolor{black!85}{gradient of resource usage}}}
% \right),
% \end{align*}
% \end{@empty}
% where $\Knob_i^*$ is the updated value of the $i^{th}$ knob, $\Delta\Knob_i$ is a small increase on the $i^{th}$ knob, $\alpha$ is the learning rate for gradient descent (see \S\ref{??} for the concrete value we use): increasing the learning rate $\alpha$ increases the convergence speed of \name, but may miss the optimal value of the accuracy.

% % We calculate $\frac{\Resource(\Knob_{cur,i} + \Delta\Knob_i) - \Resource(\Knob_{cur,i}) }{\Delta\Knob_i}$ by following its definition, which imposes extra overhead on \name (we will evaluate this overhead in \S\ref{??}) but does not require extra DNN inference.

% We calculate the gradient of resource usage by using the pre-profiled resource usage of each configuration $\Resource(\Config)$ (this aligns with prior work~\cite{chameleon,dds,reducto}), which might vary with source data, but the relative difference among them has little variance.

% However, it is computationally expensive to calculate the gradient of accuracy $$
% \frac{ Acc(\Config_{cur} + \Delta\Knob_i) -Acc(\Config_{cur})) }{\Delta \Knob_i}$$
% as calculating the accuracy $Acc$ requires generating the inference results under unlimited resources (recall that we define accuracy as the similarity between this inference results and the current inference results).

% \name instead leverages \outputgrad to approximate the gradient of accuracy.
% The rationale behind this approximation is that \outputgrad correlates with the gradient of accuracy:
% if one knob is of large \outputgrad, increasing this knob will significantly change the DNN output $\Output$, and thus also significantly affects the accuracy $Acc$, leading to a large change of accuracy.
% We will further explain when and why \outputgrad can approximate the gradient of accuracy in \S\ref{??}.
% % On the contrary, if the \outputgrad of one knob is small, increasing this knob does not affect the DNN $\Output$, and thus the corresponding accuracy change is also marginal.


% \mypara{\name way of picking new configuration} As a result, \name picks the new configuration by
% \begin{@empty}
% \footnotesize
% \begin{align*}
% \Knob_i^*=\Knob_{cur,i}+ \alpha \left(
% \underbrace{
% \frac{\Output(\Config_{cur,i} + \Delta\Knob_i) -\Output(\Config_{cur,i}))}{\Delta \Knob_i}
% }_{\text{\sf \footnotesize \textcolor{black!85}{\outputgrad}}}
% - 
% \lambda 
% \underbrace{
% \frac{\Resource(\Knob_{cur,i} + \Delta\Knob_i) - \Resource(\Knob_{cur,i}) }{\Delta\Knob_i}
% }_{\text{\sf \footnotesize \textcolor{black!85}{gradient of resource usage}}}
% \right),
% \end{align*}
% \end{@empty}
% where $\Output$ is \summary  (\ie the number of above-threshold confidence scores).
% % note that we take the absolute value to \outputgrad, as we assume that increasing the knob values increases the resource usage (and thus increases the accuracy).



% % To further support the claim that \outputgrad correlates with the gradient of accuracy, we empirically 
% % We notice that the \textit{cosine similarity} between \outputgrad and AccGrad is higher than 0.95 (we provide a formal proof that AccGrad is equals to \outputgrad using an idealized accuracy function, see \S\ref{??}), so substituting it with the accuracy can still guide \name to the optimal configuration.

% % % To adapt configurations using \outputgrad, 
% % \name runs gradient ascent (depicted in Figure~\ref{fig:workflow}) to converge to a near-optimal configuration.
% % % First, we partition the input data stream (\eg video frames) into {\em adaptation intervals}, each of one second.
% % In each adaptation interval, we perform inference using the current configuration $\Config_{cur}$ (\eg current resolution and frame rate), compute \outputgrad, and then use the following strategy to select a new configuration $\Config$ based on \outputgrad. 

% % The goal of \name's gradient ascent is maximizing a weighted sum between \summary (number of elements with scores over the confidence threshold) and resource usage (we will discuss alternative formulations shortly):

% % \vspace{-0.4cm}
% % \begin{@empty}
% % \small
% % \begin{align}
% % {\color{black}\underbrace{\highlight{white}{$\Output_{\Config}(\Data)$}}_{\text{\sf \footnotesize \textcolor{black!85}{\summary}}}}-\lambda {\color{black}\underbrace{\highlight{white}{$\Resource(\Config)$}}_{\text{\sf \footnotesize \textcolor{black!85}{resource usage}}}} \label{eq:objective}
% % \end{align} 
% % \end{@empty} 
% % Here, $\Resource(\Config)$ is the resource usage (in either bandwidth or GPU cycles, defined per application) of \Config.
% % The hyperparameter $\lambda$ governs the tradeoff between accuracy and resource usage: higher $\lambda$ will emphasize resource-saving and lower $\lambda$ will emphasize accuracy improvement.
% % \hl{Note that we will vary $\lambda$ and study its impact in \S\ref{sec:eval}.}
% % % As shown in prior work, for most configuration knobs (\eg frame rate, resolution, etc), $Resource(\Config)$ can be accurately pre-profiled and does not vary with input content as much as inference results.

% % Given the current configuration $\Config_t$ at the interval $t$ and the \outputgrad $\Grad_t$ (a vector of each knob's \outputgrad), the new configuration used for the next interval $t+1$ should be the one that maximizes the improvement of the objective. 
% % Formally, we can express it by 

% % \vspace{-0.4cm}
% % \begin{@empty}
% % \small
% % \begin{align}
% % \Config_{t+1}=\textrm{argmax}_{\Config}{\color{black}\underbrace{\highlight{white}{$(\Config-\Config_t)\cdot \Grad_t$}}_{\text{\sf \footnotesize \textcolor{black!85}{change in \summary}}}}-\lambda {\color{black}\underbrace{\highlight{white}{$(\Resource(\Config)-\Resource(\Config_t))$}}_{\text{\sf \footnotesize \textcolor{black!85}{change in resource}}}} \label{eq:gradient}
% % \end{align}
% % \end{@empty}
% % % $\Config_{t+1}=\textrm{argmax}_{\Config} (\Config-\Config_t)\cdot Grad_t-\lambda (\Resource(\Config)-\Resource(\Config_t))$
% % The new configuration $\Config_{t+1}$ will be used for the next adaptation interval. 
% % Following prior work~\cite{chameleon,dds,reducto}, we pre-profile the resource usage of each configuration $\Resource(\Config)$, which might vary with source data, but the relative difference among them has little variance.

% In many applications, the objective in Eq.~\ref{eq:objective}, which linearly combines resource usage and \summary, is less reasonable than optimizing \summary with a fixed constraint on resource usage.
% For instance, one may choose to maximize \summary (which relates to accuracy as explained shortly), conditioned on the bandwidth usage of the configuration within a budget.
% Figure~\ref{fig:workflow} shows an example of how \name's gradient-based adaptation process works in the vehicle detection example.
% % We will still use the vehicle detection example, where a traffic camera streams its video data to a GPU-equipped server to determine which frame contains vehicles.
% In each adaptation interval, the sensor encodes the video in an adaptation interval using the current configuration (frame rate and resolution) and sends it to a DNN running on a GPU-equipped server.
% The server receives this video and runs DNN inference to get the inference results and runs backpropagation to get \dnngrad and send it back to the sensor. 
% While the server runs DNN inference, the sensor runs encoding multiple times with different to obtain \inputgrad (the change in DNN input with respect to each knob).
% Once the sensor receives \dnngrad, it uses Eq.~\ref{eq:grad-decouple} to calculate \outputgrad.
% It then runs the gradient ascent strategy in Eq.~\ref{eq:gradient} to adapt the configuration and uses the new configuration in the next interval. 
% \jc{kuntai, remember to justify why resource usage of a config can be known in advance? what about the frame-diff threshold in reducto?}

% the encoded video that the camera sent, decodes this video, and runs DNN inference to obtain the inference results.
% Then, the server calculates the saliency using the backpropagation and streams the saliency back to the camera.
% Finally, the camera receives the saliency, calculates \outputgrad, and adapts the configuration accordingly.
% \jc{kuntai, please update figure~\ref{fig:workflow} to include the gradient-based adaptation process.}

% 



\tightsubsection{Caveats and benefits}
\label{subsec:limitation}

While our evaluation shows \name's gradient-ascent strategy performs well for a wide range of DNN tasks, data types, and configuration knobs, it is important to understand its limits and why it works in practice. 

% \kt{Let Yuhan run an experiment on this}
% \mypara{Why \name improves accuracy}
% Second, in the objective of gradient ascent (Eq.~\ref{eq:objective}), the change in the first term of \summary (\Output) should reflect the change in inference accuracy.
% This connection may be intuitively true since a significant change in the inference results is often accompanied by a substantial change in accuracy.
% That said, a big change in the \summary may indicate either more increase or decrease in accuracy. 
% To decide the direction of change, we use the empirical observation that when a change in knob value increases the resource usage, the impact on inference accuracy should be positive (\eg higher encoding resolution leads to higher bandwidth usage and likely more accurate inference, or higher frame rate leads to higher GPU usage and likely more accurate inference). 

% Figure~\ref{fig:accuracy-proxy} empirically verify whether the change in output ($\Delta \Output_\Config(\Data)$) is proportional to the change in accuracy (\ie the accuracy of the configuration $\Config$, minutes the accuracy of current configuration).
% We pick three configuration knobs (frame sampling rate, resolution, quantization parameter) that are widely used by prior work~\cite{chameleon,casva,awstream,videostorm,vstore,mcdnn} and a 6-second video chunk to verify the correlation between DNN output change and accuracy change on all configurations (125 configurations in total).
% Figure~\ref{fig:accuracy-proxy} shows that on one 9-second video chunk, the change of DNN output (X-axis) nicely correlates with the accuracy change (Y-axis), with a Pearson coefficient of 0.702.


\mypara{Why \name converges}
First, like other gradient-based heuristics, \name does not guarantee to always converge to a global optimum configuration. 
That said, we empirically observe that the relationship between configuration $\Config$ and their corresponding accuracy $\Acc(\Config)$ and resource usage $\Resource(\Config)$ is mostly \textbf{concave}.
This concavity means that the accuracy improvement becomes more and more marginal as we grant the system more and more resources by adjusting the configuration
As a result of the concavity, gradient-ascent can eventually converge to a global optimal configuration. 
The concavity can be intuitively understood that as the configuration uses more (compute/network) resources, the change in the input to the DNN becomes more marginal, and so does the inference results and inference accuracy.
For example, as a video analytic system increases the video encoding resolution, the pixel change becomes more marginal (mostly on ``high-frequency'' details), causing the DNN output to stabilize (objects' confidence scores will change more slowly and less frequently cross the confidence threshold, leading to fewer newly detected objects) and leading to less improvement on accuracy.
% \kt{Maybe add some visualizations}




Another potential reason for \name to fail to converge is the evolution of source data content---the \outputgrad calculated from one adaptation interval may not apply to the next adaptation interval due to temporal change in the content. 
That said, we observe that \name converges to the optimal configuration within 3-5 intervals (seconds) as shown in Figure~\ref{fig:converge-fast}, and within 1-2 intervals for configurations that require frequent adaptation (such as macroblock-level encoding quality).
Thus, as long as the best configuration last for a few seconds, \name can identify the best configuration faster than profiling-based methods.
% Both profiling-based methods and \name require the continuity of resource/accuracy relationship at a timescale of several to 10s of seconds. 



% explain it with the example in fig 6. (need to update fig 6)
% caveats: 
% why not local optimum: concavity => connection with newton's method
% why leading to higher accuracy
% content change 

% limitation: not applicable to dnn knobs





% \mypara{\outputgrad correlates with accuracy}
% A key question is how \outputgrad is related to inference accuracy.
% We found that there is a statistical correlation between \outputgrad and the inference accuracy of other configurations. 
% This is because \outputgrad captures the change in the inference results, and a significant change in the inference results is often accompanied by a substantial change in accuracy.

% We found that \outputgrad statistically correlates with the inference accuracy.
% This is because \outputgrad captures the change in the inference results, where a large change in inference results likely corresponds to a large change in accuracy.

\begin{comment}
However, the change in the inference results cannot determine whether the accuracy improves or decreases.
To handle this issue, we make an assumption that for a designated knob $\Knob_i$, increasing it while keeping other knobs fixed will either statistically not decrease the accuracy (we denote this case as $sgn(i)=1$) or not increase the accuracy (we denote this case as $sgn(i)=-1$).
We found that this assumption holds for a wide range of knobs (see Table~\ref{tab:rich-set-of-knobs}), as increasing these knobs causes the resource usage pipeline increases/decreases and thus the corresponding accuracy also increases/decreases.
For example, increasing the frame rate while fixing the  resolution in the video analytics system typically leads to more accurate inference results as more frames are analyzed. 
Similarly, increasing the resolution while fixing the frame rate enhances the clarity of the boundaries of the object, and is likely to generate more accurate inference results.

% To give a concrete example, when tuning the frame rate and resolution of the aforementioned video analytic system, increasing the frame rate while fixing the resolution typically leads to more accurate results as more frames are being analyzed. 
% Similarly, increasing the resolution while fixing the frame rate also makes the detail of the video (like the boundary of the vehicles) clearer and thus is likely to generate more accurate inference results.

Using this assumption, we then derive the (signed) output change with respect to the current configuration (frame rate $\Knob_1=20fps$, resolution $\Knob_2=480p$) using the following formula:

\vspace{-0.3cm}
\begin{@empty}
\footnotesize
\begin{equation*}
\Delta \Output_\Config(\Data)= \sum_{i=1}^n \left|\frac{\Delta \Output}{\Delta \Knob_i}\right| \cdot sgn(i) \cdot (\Knob_i - \Knob_{i,cur}) =  0.08 \cdot (\Knob_i - 10\textrm{fps}) + 0.01 \cdot (\Knob_2 - 480\textrm{p}) 
\end{equation*}
\end{@empty}
% To examine the correlation between \outputgrad and the accuracy of other configurations, we calculate the change in accuracy with respect to the change of the current configuration ($O(res=2,fps=2)$) using the following formula
% \begin{@empty}
% \footnotesize
% \begin{equation*}
% \Delta O(res,fps) = \frac{\Delta O}{\Delta (res, fps)} \cdot \Delta (res, fps) = \frac{\Delta O}{\Delta res}(res-2) + \frac{\Delta O}{\Delta fps}(fps-2).
% \end{equation*}
% \end{@empty}
% And check if the output change is proportional to the accuracy change

  



And then, we verify whether the change in output ($\Delta \Output_\Config(\Data)$) is proportional to the change in accuracy (\ie the accuracy of the configuration $\Config$, minutes the accuracy of current configuration):
% \begin{@empty}
% \footnotesize
% \begin{equation*}
% \Delta \Output(\Input, \Config) \propto Acc(\Output(\Input, \Config)) - Acc(\Output(\Input, \Config_{cur})),
% \end{equation*}
% \end{@empty}
% where $Acc$ represents the inference accuracy.
We pick three configuration knobs (frame sampling rate, resolution, quantization parameter) that are widely used by prior work~\cite{chameleon,casva,awstream,videostorm,vstore,mcdnn} and a 6-second video chunk to verify the correlation between DNN output change and accuracy change on all configurations (125 configurations in total).
As shown in Figure~\ref{fig:accuracy-proxy}, on one 9-second video chunk, the change of DNN output (X-axis) nicely correlates with the accuracy change (Y-axis), with a Pearson coefficient of 0.702.


\end{comment}






% that maximally improves the change in DNN output $\Delta \Output(\Data,\Config)$ under the resource budget.
% As the change in DNN output statistically correlates with the change in accuracy, this will likely maximize the accuracy of the new configuration $\Config$.
% We then use this configuration for the next adaptation interval.
% identify a new configuration that maximally improves accuracy without exceeding the resource budget.
% We use this new configuration for the next adaptation interval, and at the end of the interval, we repeat the same adaptation steps.
% As the content of the input data is continuous, the new configuration is likely to generate more accurate inference results compared to the original configuration.
% Note that 
% As a result, the inference results of the new configuration are likely to be more accurate than the current configuration


\mypara{Why \name beats alternatives}
By performing gradient ascent through estimating \accgrad, \name outperforms previous work on all three requirements (\ie adapt frequently, converge to a near-optimal configuration, and generalize to different types of knobs and analytic tasks).
First, compared to profiling-based work, \name adapts much more frequently (as \name updates its configuration \textit{at every second} but profiling-based work updates its configuration once every minute~\cite{awstream}) and earlier (as \name adapts to the change of input content right at the next adaptation interval but the profiling-based work need to wait till the next profiling).
Second, compared to the heuristics-based approach, \name can adapt to a near-optimal configuration, where the accuracy of the heuristics-based approach can be much lower than the optimal configuration.
Third, \name can generalize to different applications and DNNs (as \name only assumes the DNNs to be differentiable, which holds for almost all DNNs) and a wide range of knobs (as \name applies to most of existing knobs, see Table~\ref{tab:rich-set-of-knobs}).

We want to clarify that the extra overhead of \name  \textbf{does not increase end-to-end delay} (defined as the delay from the time when the source data is collected to the time when the inference results are generated), as adapts after obtaining the inference results (as shown in Algorithm~\ref{alg:adapt}) unless there is not enough resource (in terms of bandwidth and GPU cycles) for \name to adapt in real-time.


% \mypara{Why \name converges}
% First, like other gradient-based heuristics, \name does not guarantee to always converge to a global optimum configuration. 
% That said, we empirically observe that the relationship between configuration $\Config$ and their corresponding accuracy $\Acc(\Config)$ and resource usage $\Resource(\Config)$ is mostly \textbf{concave}.
% As a result of the concavity, gradient-ascent can eventually converge to a global optimal configuration. 
% The concavity can be intuitively understood that as the configuration uses more (compute/network) resources, the change in the input to the DNN becomes more marginal, and so does the DNN output.
% For example, as a video analytic system increases the video encoding resolution, the pixel change becomes more marginal (mostly on ``high-frequency'' details), causing the DNN output to stabilize (objects' confidence scores will change more slowly and less frequently cross the confidence threshold, leading to fewer newly detected objects).
% \kt{Maybe add some visualizations}
% \kt{This need a better proof}





% \tightsubsection{Limitations}
% \label{sec:limits}


% \mypara{Example applications that \name applies}

\mypara{Why picking future configuration based on current configuration}
As the \name picks the configuration of the next adaptation interval based on the current adaptation interval, it is possible that the configuration that yields high accuracy on the current adaptation interval generates inaccurate inference results at the next adaptation interval.
However, this scenario only happens when the content of the input data changes (\eg when the vehicle stops in front of the red light) and thus does not happen frequently.



\mypara{Running gradient ascent over discrete configuration space}
Before running \name, we first linearly normalize all knob values to [0,1], where $0$ corresponds to the knob value with the least resource usage and 1 with the most resource usage.
We then calculate the updated knob value using Equation~\ref{eq:real-adaptation} and pick the closest value among all available knob values.



\mypara{Why gradient ascent over discrete configuration space}
As gradient-based approach is mostly used on continuous space (\eg DNN parameters in DNN training), one may worry that gradient-based approach may fail on discrete configuration space.
We want to clarify that gradient-based approach can converge to a near-optimal configuration when the objective function (\ie the weighted sum between accuracy and resource usage) is concave~\cite{ramazanov2011stability,chistyakov2015stability}.



% \mypara{Limitation} 
% % We acknowledge that \outputgrad only works for configuration knobs that affect DNN input (\ie input preprocessing part of a DNN analytics system).


% \kt{Two potential limitations: 
% 1. \name is not ideal in scenario where the vast majority of adaptation intervals do not need to be analyzed.
% 2. \name does not apply to knobs that the optimal value frequently changes between adaptation interval (\eg adaptation interval=1frame, knob=whether to encode this frame or not).
% Not sure if we should include them.}

% Also, as \name requires DNN inference on every adaptation interval (in order to calculate \outputgrad for that interval), it is not ideal when most of the adaptation intervals do not need to be analyzed (\eg security camera footage at late night).







% \mypara{Overhead of backpropagation}

% However, this assumption makes \name not applicable to knobs that alter the DNN itself, such as retraining the DNN weights based on the current input~\cite{ekya,noscope,mcdnn}.
% In some sense, both the DNN customization approach and \name are adapting to the varying content in the input data stream.
% However, in order to maintain high accuracy, the DNN customization approach needs to retrain the DNN when the input content varies (which adds high GPU overhead).
% In contrast, \name adapts the knobs as part of the DNN-based inference process and only reuses the DNN inference result (for backpropagation), which is much more lightweight.


% \jc{need a paragraph to explain customization of specific applications, and why it still works under evolving content}
% overall, why it's better?

% Our gradient-ascent-based approach has its own caveats as it cannot guarantee that (i) the search will quickly converge in a few steps, and (ii) the search may get stuck in a local optimal.
% To answer this question, we measure how fast \name can converge to a near-optimal configuration (a top-1\% configuration).
% \kt{Not sure how to answer this question}





% The intuition behind the fast convergence is that as long as the \outputgrad with respect to one configuration knob is non-zero, tuning that knob will likely improve accuracy.
% % Further, as the input data is constantly changing over time, it is less likely for a local optimal to persist.
% Thus, \name is unlikely to be stuck in a local optimum, which corroborates our empirical observation of \name.
% \kt{Other potential concerns: (1) why treat discrete configs as almost continuous variables, (2) why the better configuration at this second will likely lead to a better result at the next second, (3) what if the content is noisy and makes the gradient noisy}



% However, directly calculating \outputgrad needs a substantial amount of extra inference.
% If we calculate \outputgrad knob-by-knob, we will need to calculate the accuracy change by changing one knob at a time.
% The amount of GPU compute will grow at least linearly with more knobs. 
% % This is because calculating \outputgrad in a knob-by-knob manner (\ie calculate the accuracy change by alternating the value of one knob while the value of other knobs remaining unchanged, and repeat this process for all knobs) results in extra inference (see \S\ref{subsec:calculate-accgrad} for details).
% % Moreover, more knobs will lead to more inference and reduces the applicability of \outputgrad on a large set of knobs.

% \mypara{Leveraging DNN differentiability} To reduce such overhead, \name harnesses the differentiability of the DNN to calculate \outputgrad with constant GPU overhead and with no extra inference.
% Intuitively, in order to calculate how DNN output changes with respect to the knob change (\ie \outputgrad), we can calculate how DNN output changes with respect to the DNN input change, and then study how DNN input changes with respect to the knob change.
% % how changing system knobs alters the DNN input, and then calculate how changing the DNN input alters the DNN output.
% Formally, we denote the configuration (\ie the values of all knobs) as $c$, the DNN input as $I$, and the DNN output as $O$. The intuition above can be written as the following chain rule:
% \begin{equation}
%     \frac{\partial O}{\partial c} = \frac{\partial O}{\partial I} \cdot \frac{\partial I}{\partial c},
% \end{equation}
% The first term $\frac{\partial O}{\partial I}$ can be obtained via backpropagation (a constant GPU overhead, but no extra inference is incurred as backpropagation reuses the computation graph created by existing DNN inference).
% The second term $\frac{\partial I}{\partial c}$ can be calculated in a knob-by-knob manner but since it only computes the DNN input (not DNN inference), it does not have extra GPU overhead. 
% without incurring DNN inference as calculating the DNN input change does not require DNN inference.

% The key enabler for \name to remove the extra inference is the following two observations to existing knobs for DNN-based analytic systems.



% that the knob only alters the DNN input. does not cover those knobs that alter the DNN itself, 




% \begin{enumerate}
%     \item \textit{Accuracy-Resource Property}: For a large class of knobs,  increasing the value of one knob always results in spending more (or less) resource, and also making the corresponding inference results more (or less accurate).
%     The amount of accuracy improvement (or degradation) depends on how much the knob increase alters the inference results.
%     \item \textit{Black-box Property}: Most of the knobs treat DNN as a black box and change the inference results solely by changing the DNN input.
% \end{enumerate}

% By leveraging the first assumption, \name estimates the accuracy change through inference results change, thus avoid calculating the inference results under the most expensive configuration as the ground truth.
% By leveraging the second assumption, \name decouples the gradient using chain rule and avoid the inference on the new configurations.


% Note that not all knobs satisfies the two properties above. We list some examples in Table \ref{??} and some non-examples down below.

% For \accres, we find that the sensing configuration knobs that directly change the raw sensed data, like the aperture and the ISO of the camera, the Gamma correction value of the camera, the positioning direction of the directional microphone, etc., do not satisfy \accres as varying these knobs typically have little impact on the encoded file size and the encoding cost of the input data.
% However, the sensing configuration knobs are typically pre-configured (like the positioning direction of the microphone) or self-adapted (like the aperture and the ISO of the camera) by the sensor.
% As a result, these knobs are typically not dynamically programmable so \name cannot change these knobs anyway.

% The non-examples for \blackbox are the knobs that optimize DNN inference, like DNN selection~\cite{chameleon} and DNN customization~\cite{noscope,ekya,mcdnn}.
% We acknowledge the effectiveness of these knobs in terms of saving GPU cost.
% However, we argue that these knobs requires the system to change or replace the DNN in real-time, which make them not generally applicable in all deployment settings (\eg when performing inference through third-party API).
% % However, switching or editing the DNN may result in significant overhead (\eg some other components may be customized for this DNN and may require retraining upon DNN changing~\cite{accmpeg}) or even not doable (\eg when performing inference through cloud API).




% \tightsubsection{Workflow of \name}














% We demonstrate the workflow of \name using the example of traffic cam-based vehicle detection
% Figure~\ref{fig:workflow} demonstrates the workflow of \name.
% \name assumes that the analytic systems are made up of two components: \textit{input processing} and \textit{DNN-based inference}.
% First, \name processes the data stream $x$ through input processing using the current configuration $c$ to obtain the DNN input $I$.
% \name then forwards $I$ through the DNN and obtain the DNN output $O$.
% After that, \name performs DNN backpropagation and obtains the gradient $\frac{\partial O}{\partial I}$.
% In the meantime, \name alters every knob in $c$ and obtains the corresponding change on the DNN input.
% \name then stacks together the DNN input changes of individual knobs ($\frac{\partial I}{\partial c}$) and 
% % \name then stacks these DNN input changes to obtain $\frac{\partial I}{\partial c}$ and 
% multiplies it with $\frac{\partial O}{\partial I}$ to obtain \outputgrad $\frac{\partial O}{\partial c}$.
% Finally, \name updates the configuration $c$ according to the \outputgrad.
% We will present the details of each step in the next section.









% \subsection{Accuracy gradient as a better feedback}

% \begin{itemize}
%     \item We find that: how much the analytic accuracy change differs if we change different knobs is essentially asking what is the \textit{gradient} of analytic accuracy with respect to the knob values.
%     \item With the accuracy gradient, we can better predict the analytic accuracy of those knob values we did not explore yet.
% \end{itemize}

% Our goal is to calculate the gradient of accuracy with respect to knobs (we call this gradient \textit{accuracy gradient}) by only evaluating the system under one configuration.

% Accuracy gradient enables us to better predict the accuracy of different configurations under similar video content.
% As a result, one can pick a chheaper configuration while still achieving the same accuracy with accuracy gradient.


% \begin{comment}

% \subsection{Programming interface of \name}


% \begin{figure}
%     \centering
%     \includegraphics[width=1\columnwidth]{figs/raw-input-inference.jpg}
%     \caption{\name handles those hyper-parameters that preprocess the input to the DNN.}
%     \label{fig:raw-input-inference}
% \end{figure}



% \subsection{API of HPs} 

% As shown in Figure~\ref{fig:raw-input-inference}, \name abstracts the underlying AI systems into two stages.
% In the preprocessing stage, the AI system pre-processes the raw sensing data to obtain the input to the DNN.
% In the inference stage, the DNN performs inference and obtain the analytic results.
% \name focuses on those HPs for preprocessing stage (we will show most of the HPs fall into this category in \S\ref{subsec:hp-examples}, together with some example HPs that do not belong to this category).
% As the preprocessing does not incur the compute-intensive server-side DNNs, we assume that this step can be locally done at the camera.

% Based on this observation, the programming interface of \name towards HPs are:
% \begin{small}
% \begin{verbatim}
% prep(Data raw, List hps)-> (Data input, Bytes encoded)
% proxy(Result result) -> Float pseudo_acc
% \end{verbatim}
% \end{small}

% The first function \texttt{prep} pre-processes the raw sensed data \texttt{raw} based on a list of HPs \texttt{hps}, and return the codec-encoded byte stream \texttt{encoded} and the input data \texttt{input} that server-side DNN will receive.

% The second function aims to provide a differentiable proxy towards accuracy (since most of the existing accuracy function is not differentiable).
% As most of the DNNs will return confidence scores to describe the confidence of the analytic results the DNN derives, we use the sum of the confidence scores as the default proxy.
% This complies with recent computer vision advances on evaluating the quality of inference results.

% Further, we empirically verify this assumption on different types of HPs and different videos.


% \subsection{Examples}
% \label{subsec:hp-examples}


% This assumption precludes those HPs that directly changes server-side DNN (\eg customizing the server-side DNN or switching between different server-side DNNs).
% That said, the vast majority of HPs, including HPs of traditioanal data encoding codecs (\eg frame rate, resolution, quantization parameters etc), DNN-based encoding codec (\eg feature compression, super resolution), fine-grained data quality assignments (\eg region-of-interest selection, macroblock encoding quality selection), sensor-side data filtering (\eg filtering the frames through cheap object detector or through cheap feature extractors) still fit in our assumption. 



% % \mypara{API of DNNs}
% % We require that the DNN to implement two APIs:
% % \begin{small}
% % \begin{verbatim}
% % inference(Data input)-> Result result
% % backprop(Result result, Function f)-> Data grad
% % \end{verbatim}
% % \end{small}



% \subsection{Workflow of \name}

% Contrast between conventional workflow and ours workflow

% \end{comment}







% \subsection{Workflow and API of \name}
% \kt{Goal: how to use the API in our system to calculate accuracy gradient}

% \begin{figure}
%     \includegraphics[width=1\columnwidth]{figs/workflow.jpg}
%     \caption{Workflow of \name \kt{Plot this figure in a "call stack" way, MAKE THE FONT LARGER}}
%     \label{fig:workflow}
% \end{figure}

% \mypara{Workflow of \name} Based on the approach above, we present the workflow of \name in Figure \ref{fig:workflow}.


% Our system enables the application to obtain the gradient of accuracy with respect to the knobs through the following API:
% $$AccGrad = calc(V_t, \{knob_i\}_{i=1}^n)$$

% \mypara{Towards knobs}

% $knob'_i = reduce(knob_i)$
% This reduce the knob to lower knob value

% \mypara{Towards DNN}
% We require the DNN to implement two APIs:
% \begin{packeditemize}
%     \item \texttt{result = inference(V)}
%     \item \texttt{saliency = backprop(result, grad)}
% \end{packeditemize}

% \mypara{Towards application}
% We require the application to implement:
% \begin{packeditemize}
%     \item \texttt{encode(V, knobs)} This one should be locally done on the camera
%     \item \texttt{proxy(results)}
% \end{packeditemize}


% \subsection{How to use the API}






% \subsection{Reduce the cost of accuracy gradient}


% \mypara{Accuracy gradient sampling}


% \mypara{Accuracy gradient compression}



==> overview_v5.tex <==

\tightsection{Design of \name}
\label{sec:design}

We present \name, a configuration adaptation system that aims at improving along the three requirements mentioned above --- frequent adaptation to near-optimal configuration on various configuration knobs. 
The basic idea of \name is to frequently estimate 
the {\em gradient} of how inference accuracy changes with each configuration knob, which we refer to as the {\em \accgrad}.
Using the up-to-date estimate of \accgrad, \name uses a gradient-ascent strategy to update the configuration to improve an objective metric that combines inference accuracy and resource usage (\S\ref{subsec:adaptation-goal}). 
% to improve the DNN inference results but still stays in the (compute/network) resource budget or maximally reduces the resource usage with minimum change on the DNN inference results.
% Figure~\ref{fig:adaptation-behavior} illustrates an example: after a change of input data, \name can adapt more frequently and gradually converge to a near-optimal configuration.
To efficiently calculate \accgrad, \name approximates it by estimating \outputgrad, another metric that can be efficiently calculated by leveraging DNN's inherent differentiability (\S\ref{subsec:outputgrad}) and statistically correlated with \accgrad (\S\ref{subsec:outputgrad-properties}).
Finally, we will discuss the caveats of \name's gradient-based adaptation.

\begin{table}[]
\footnotesize
\begin{tabular}{|m{0.13\columnwidth}|m{0.45\columnwidth}|m{0.27\columnwidth}|}
\hline
{\bf Notation}                                                                                              & {\bf Definition}                                                                                                                                                                                                                                 & {\bf Example}                                                                                                         \\ \hline \hline
$n$                                                                                                   & Number of knobs                                                                                                                                                                                                                            & $n=2$                                                                                                           \\ \hline
$t$                                                                                                   & $t^{\textrm{th}}$ adaptation interval (by default, each interval is 1 second)                                                                                                                                                                                         & $t=1$                                                                                                           \\ \hline
$T$                                                                                                   & Total number of adaptation intervals                                                                                                                                                                                                       & $T=60$                                                                                                          \\ \hline
$\Config_t$                                                                                           & Configuration: a vector of knobs with their selected values at interval $t$                                                                                                                                                                & $\Config_1=$(frame rate=10, resolution=480p)                                                                    \\ \hline
$\Knob_{i,t}$                                                                                         & The value of $i^{\textrm{th}}$ knob in configuration $\Config_t$                                                                                                                                                                                    & $\Knob_{2,1}$=480p                                                                                              \\ \hline
$\Delta \Knob_i$                                                                                      & A small increase on the $i^{\textrm{th}}$ knob                                                                                                                                                                                                      & $\Delta \Knob_2$=120p                                                                                           \\ \hline
$\Data_t$                                                                                             & input data at interval t                                                                                                                                                                                                                   &                                                                                                                 \\ \hline
\begin{tabular}[c]{@{}l@{}}$\Resource(\Config_t; \Data_t)$\\ or\\ $\Resource(\Config_t)$\end{tabular} & Resource usage of config $\Config_t$ under $\Data_t$. We omit $\Data_t$ for simplicity                                                                                                                                                     &     $\Resource(\Config_1)=$5Mbps                                                                                                            \\ \hline
\begin{tabular}[c]{@{}l@{}}$Res(\Config_t; \Data_t)$\\ or\\ $Res(\Config_t)$\end{tabular}             & Inference results of config $\Config_t$ under $\Data_t$. We omit $\Data_t$ for simplicity.                                                                                                                                                 & 
\begin{tabular}[c]{@{}l@{}}$Res(\Config_1)=\{$\\
(obj1, ``car'', score: 0.2),\\
(obj2, ``bike'', score: 0.8)\\ $\}$
\end{tabular} 
 \\ \hline
$e$                                                                                                   & An element in the inference results (\eg a detected object). Each element is associated with a confidence score.                                                                                                                           & \begin{tabular}[c]{@{}l@{}}$e=$\\
(obj1, ``car'', score: 0.2)
\end{tabular}                                                                 \\ \hline
$\theta$                                                                                              & Confidence threshold                                                                                                                                                                                                                       & $\theta=0.5$ (default)                                                                                                   \\ \hline
\begin{tabular}[c]{@{}l@{}}$\Input(\Config_t; \Data_t)$\\ or\\ $\Input(\Config_t)$\end{tabular}         & DNN input generated by configuration $\Config_t$ using input data $\Data_t$. We omit $\Data_t$ for simplicity.                                                                                                                                           & ~                                                                                         \\ \hline
\begin{tabular}[c]{@{}l@{}}$\Output(\Config_t; \Data_t)$\\ or\\ $\Output(\Config_t)$\end{tabular}         & Output utility: number of above-confidence-threshold elements. We omit $\Data_t$ for simplicity.                                                                                                                                           & $\Output(\Config_1)=1$                                                                                          \\ \hline
\begin{tabular}[c]{@{}l@{}}$Acc(\Config_t; x_t)$\\ or\\ $Acc(\Config_t)$\end{tabular}                 & Accuracy of the configuration $\Config_t$ under input data $\Data_t$, defined as the similarity between the current inference result $Res(\Config_t)$ and the inference results generated using the most resource-demanding configuration. & $Acc(\Config_1)=100\%$                                                                                          \\ \hline
$\alpha$                                                                                              & Learning rate of \name                                                                                                                                                                                                                     & $\alpha=0.5$ (default)                                                                                                    \\ \hline
$\lambda$                                                                                             & The hyperparameter that trade-off between accuracy and resource usage.                                                                                                                                                                     & $\lambda=1$                                                                                                  \\ \hline
\end{tabular}
\vspace{0.1cm}
\tightcaption{Summary of the notations used in \name}
\label{tab:notations}
\end{table}

\tightsubsection{Terminology}
\label{subsec:terminology}

% \footnotesize
% \begin{tabular}{|m{0.12\columnwidth}|m{0.49\columnwidth}|m{0.25\columnwidth}|}

To adapt configuration for various DNN pipelines (see Table~\ref{tab:pipeline} for a summary of considered pipelines), we first introduce a unified terminology to describe their input/output behaviors.
Table~\ref{tab:notations} summarizes the notations and their meanings.
% in a way that is relevant to this work. 
% , from object detection in video and audio-to-text translation (see Table~\ref{??} for a list).

We split the input data into fixed-length (by default, one-second-long) intervals, called {\em adaptation intervals}.
In the $t^{\textrm{th}}$ adaptation interval, the input data $\Data_t$ is first preprocessed with the current configuration $\Config_t$ (\eg video resolution and frame rate) to get the DNN input $\Input(\Config_t; \Data_t)$, 
% (see Algorithm~\ref{alg:adapt})
and the DNN takes it as input and returns $Res(\Config_t; \Data_t)$ as output.
DNN output $Res(\Config_t, \Data_t)$ contains multiple {\em elements}. 
% Note that there might be multiple DNN inferences within an adaptation interval.
For the DNNs in our considered tasks, each element is associated with a confidence {\em score}, and only elements with a score over a confidence {\em threshold} $\theta$ will be counted towards accuracy. 

The definitions of an element $e$ and input data $\Data$ vary with the considered application.
An element is a detected object in object detection, a detected text in audio-to-text translation, or a segmented mask of a detected instance in instance segmentation.
Input data can be a sequence of RGB frames in videos, point-cloud frames in LiDAR, or an audio wave segment in audio data.


% \name works with any DNN tasks that return elements with confidence scores as output. 

Based on these notations, we can define the following concepts:
\begin{packeditemize}
\item $Acc(\Config_t; \Data_t)$ is the accuracy of the inference results generated using input data $\Data_t$ and configuration $\Config_t$. 
Following prior work~\cite{awstream,chameleon,dds,accmpeg,ekya,boggart}, we define accuracy as the \textbf{similarity} between the current inference results and the inference results generated from the most resource-consuming configuration $\Config^*$.\footnote{This notion of accuracy is well studied in the literature. While it does not compare DNN output with human-annotated ground truth, it better captures the impact of adapting configurations on inference results.} 
% This definition of accuracy is less ideal than calculating accuracy using human-annotated ground truth, but 
% It directly shows the impact of adapting configurations on inference results.
\item $\Output(\Config_t; \Data_t)$ is the \summary of the inference results generated using input data $\Data_t$ and configuration $\Config_t$. We define \summary as the number of above-threshold elements (see \S\ref{subsec:outputgrad}).
% (see \S\ref{sec:definition-of-summary} for the formal definition).
\item $\Resource(\Config_t)$ is the resource usage (bandwidth and/or GPU cycles, defined per application) at the $t^{\textrm{th}}$ adaptation interval. 
We share the assumption with most works in this space~\cite{chameleon,awstream} that resource usage is determined by the configuration, and thus $\Resource(\Config)$ is already profiled offline. 
\end{packeditemize}

Without ambiguity, we omit $\Data_t$ in DNN input $\Input(\Config_t)$, output $Res(\Config_t)$, inference accuracy $Acc(\Config_t)$, and \summary $\Output(\Config_t)$.

% For the DNN output in an adaptation interval, we define the {\em \summary} by the number of elements in an adaptation interval whose confidence scores exceed the confidence threshold.
% The rationale of \summary will be explained in detail later in \S\ref{subsec:gradient-ascent}.
% For now, we can think of \summary as a one-value summarization of the DNN output whose change indicates the change in inference accuracy.

% Though the definitions may not be universally applicable, it naturally applies to most prior work in video analytics as well as the new applications mentioned in Table~\ref{tab:applications}.
% developers do not need to make major changes to the DNN to use \name.







% \kt{3 columns: notation, meaning, example}




\kt{It's better to define notations above in the text instead of defining it at very beginning}

% \tightsubsection{Adaptation goal of \name}
\tightsubsection{Adaptation goal and gradient-ascent}
\label{subsec:adaptation-goal}





% \jc{(1) 3.2 and 3.3 are still a bit too abstract. please use a concrete example like the one in 31
% (2) it’s not clear from 32 (upfront) why configgrad-based gradient ascent can adapt quickly. this should be upfront, not embedded or in the end
% same thing with 33. it’s unclear why this is a smart design
% (3) i dont see the assumptions in 31, 32, 33 be explicitly called out and justified.. did i miss them?}
% \kt{I explicitly called out the assumptions in 31. I will deprioritize other issues before Sunday.}

% We first introduce terminology to describe the DNN output.
% % in a way that is relevant to this work. 
% This is necessary because \name works with various DNN tasks and source data types (see Table~\ref{tab:pipeline} for a list).
% , from object detection in video and audio-to-text translation (see Table~\ref{??} for a list).
% \name splits the source data stream into fixed-length (by default, one-second-long) intervals, called {\em adaptation intervals}.
% In the $i^{th}$ adaptation interval, the data is first preprocessed with the configuration $\Config_i$ and then fed to DNN (see Figure~\ref{fig:workflow}) to obtain the inference results.

% \mypara{Adaptation goal} The goal of \name is: given the configuration of the current interval $\Config_{cur}$, pick the configuration $k^*$ for the next adaptation interval so that a weighted sum between the accuracy and the resource usage is improved.
% Formally, we write this adaptation goal as:
% \begin{align}
% \nonumber
% \text{On the current adaptation interval, find}~~\Config^*&, \text{such that}
% \\
% \underbrace{Acc(\Config^*)}_{\text{\sf \footnotesize \textcolor{black!85}{accuracy}}}
% - 
% \lambda 
% \underbrace{\Resource(\Config^*)}_{{\text{\sf \footnotesize \textcolor{black!85}{resource usage}}}}
% \geq 
% Acc(
% \underbrace{\Config_{cur}}_{\text{\sf \footnotesize \textcolor{black!85}{ current configuration}}}
% ) - &\lambda \Resource(\Config_{cur})
% \end{align}

% \jc{is this in conflict with the "objective" paragraph in 2.1?}
The adaptation goal of \name is to pick the configurations for all adaptation intervals such that the following weighted sum between the accuracy $Acc$ and the resource usage $\Resource$ is maximized:
\begin{equation}
% \max_{\Config_1,\cdots,\Config_T}
\sum_{t=1}^T
\underbrace{Acc(\Config_t)}_{\text{\sf \footnotesize \textcolor{black!85}{accuracy of $t^{th}$ interval}}}
- \lambda \underbrace{\Resource(\Config_t)}_{{\text{\sf \footnotesize \textcolor{black!85}{resource usage of $t^{th}$ interval}}}},
\label{eq:objective}
\end{equation}
where
% \begin{packeditemize}
% \item $n$ is the total number of adaptation intervals.
% \item $k_1,\cdots k_n$ are the configurations for each adaptation interval.
% \item $Acc(\Config_t)$ is the accuracy of the $t^{th}$ adaptation interval.
% Following prior work~\cite{awstream,chameleon,dds,accmpeg,ekya,boggart}, we define accuracy as the \textbf{similarity} between the current inference results and the inference results generated from the most resource-consuming configuration. This definition of accuracy is less ideal than calculating accuracy using human-annotated ground truth, but it allows the system to optimize the inference results in the absence of annotated human data, which is the common case in current video analytic applications like traffic footage analytics.
% \item 
% $\Resource(\Config_t)$ is the resource usage (in either bandwidth or GPU cycles, defined per application) the $t^{th}$ adaptation interval.
% \item
$\lambda$ is a hyperparameter that governs the tradeoff between accuracy and resource usage: higher $\lambda$ will emphasize resource-saving and lower $\lambda$ will emphasize accuracy improvement.
We will vary $\lambda$ and examine its effect on \name in \S\ref{sec:eval}.
% \end{packeditemize}
Note that this objective can be extended to perform {\em budgeted} optimization (\eg to maximize accuracy under a budget of resource usage, we can add a change the term $\Resource(\Config_t)$ to a large penalty when resource usage extends the budget).
We leave this extension to future work. 

% Note that in many applications, the objective in Eq.~\ref{eq:objective}, which linearly combines accuracy and resource usage, is less ideal than optimizing accuracy with a fixed constraint on resource usage.
% For instance, one may choose to maximize accuracy, conditioned on the bandwidth usage of the configuration within a budget~\cite{awstream,dds,accmpeg}.

% However, \kt{We need something to defend this formulation}
% Figure~\ref{fig:workflow} shows an example of how \name's gradient-based adaptation process works in the vehicle detection example.
% We will still use the vehicle detection example, where a traffic camera streams its video data to a GPU-equipped server to determine which frame contains vehicles.
% In each adaptation interval, the sensor encodes the video in an adaptation interval using the current configuration (frame rate and resolution) and sends it to a DNN running on a GPU-equipped server.
% The server receives this video and runs DNN inference to get the inference results and runs backpropagation to get \dnngrad and send it back to the sensor. 
% While the server runs DNN inference, the sensor runs encoding multiple times with different to obtain \inputgrad (the change in DNN input with respect to each knob).
% Once the sensor receives \dnngrad, it uses Eq.~\ref{eq:grad-decouple} to calculate \outputgrad.
% It then runs the gradient ascent strategy in Eq.~\ref{eq:gradient} to adapt the configuration and uses the new configuration in the next interval. 


% , and the DNN output contains multiple {\em elements}. 
% % Note that there might be multiple DNN inferences within an adaptation interval.
% An element can be a detected object in object detection, a detected text in audio-text translation, or the classification of a pixel in semantic segmentation.
% Most DNNs for these tasks will associate each element with a confidence {\em score}, and only elements with a score over a confidence {\em threshold} will be counted towards accuracy. 
% \name works with any DNN tasks that return elements with confidence scores as output. 




% \tightsubsection{Observations}

% Explain here that:
% \begin{packeditemize}
%     \item The optimization is concave w.r.t. the configuration $\rightarrow$ gradient-ascent-based optimization to leverage this concavity.
%     \item A better configuration for this adaptation interval is also better for the next adaptation interval unless the video content changes significantly (\eg a new object comes in) $\rightarrow$ it is OK to adjust the configuration gradually over time.
%     \item The two observations inspire a gradient-ascent-based approach.
% \end{packeditemize}




% In each adaptation interval, \name first performs DNN inference to obtain the inference results, computes the \textit{gradient}  with respect to the configuration (we will explain how to calculate this gradient shortly) and update the configuration using the gradient.
% \name gradually updates the configuration $\Config$ (\eg current resolution and frame rate) using the \textit{gradient} of the accuracy and the resource usage.


% Ideally, \name would update the $i^{th}$ knob $\Knob_{cur,i}$ in the current configuration $\Config_{cur}$ by:
% \begin{@empty}
% \footnotesize
% \begin{align*}
% \Knob_i^*=\Knob_{cur,i}+ \alpha \left(
% \underbrace{
% \frac{Acc(\Config_{cur} + \Delta\Knob_i) -Acc(\Config_{cur})) }{\Delta \Knob_i}
% }_{\text{\sf \footnotesize \textcolor{black!85}{gradient of accuracy}}}
% - 
% \lambda 
% \underbrace{\frac{\Resource(\Knob_{cur} + \Delta\Knob_i) - \Resource(\Knob_{cur}) }{\Delta\Knob_i}
% }_{\text{\sf \footnotesize \textcolor{black!85}{gradient of resource usage}}}
% \right),
% \end{align*}
% \end{@empty}
% where $\Knob_i^*$ is the updated value of the $i^{th}$ knob, $\Delta\Knob_i$ is a small increase on the $i^{th}$ knob, $\alpha$ is the learning rate for gradient descent (see \S\ref{??} for the concrete value we use): increasing the learning rate $\alpha$ increases the convergence speed of \name, but may miss the optimal value of the accuracy.


% % In each adaptation interval, we perform inference using the current configuration $\Config_{cur}$ (\eg current resolution and frame rate), compute \outputgrad, and then use the following strategy to select a new configuration $\Config$ for the next adaptation interval.
% % the gradient of the objective function $Obj(k)$ with respect to the current configuration $\Config_{cur}$ and update the current configuration by running gradient ascent.

% % In each adaptation interval, we perform inference using the current configuration $\Config_{cur}$ (\eg current resolution and frame rate), obtain the gradient of the objective function $Obj(k)$ with respect to the current configuration $\Config_{cur}$ and update the current configuration by running gradient ascent.

% Formally, the goal of \name is to maximize a weighted sum between the accuracy $Acc$ (defined as the \textit{similarity} between the current inference results and the inference results generated under unlimited resource)\kt{need to defend this definition} and the resource usage $\Resource$:
% \begin{equation}
% \underbrace{Acc(\Config)}_{\text{\sf \footnotesize \textcolor{black!85}{accuracy}}}
% - \underbrace{\lambda \Resource(\Config)}_{{\text{\sf \footnotesize \textcolor{black!85}{resource usage}}}},
% \label{eq:objective}
% \end{equation}
% % where $\Config$ i \name maximizes this weighted sum by running gradient ascent (depicted in FIgure~\ref{fig:workflow}).
% where $\lambda$ is a hyperparameter that governs the tradeoff between accuracy and resource usage: higher $\lambda$ will emphasize resource-saving and lower $\lambda$ will emphasize accuracy improvement.
% We will vary $\lambda$ and examine its effect on \name in \S\ref{??}.


\begin{figure}
    \centering
    \includegraphics[width=1.05\columnwidth]{figs/gradientascent-illustrated.pdf}
    \vspace{-0.2cm}
    \tightcaption{\name uses gradient-ascent to gradually update configuration every adaptation interval to gradualy improve the performance goal in Equation~\ref{eq:objective}.
    % Adapting configuration using \outputgrad. 
    % Note that as the adaptation process happens \textbf{after} obtaining the inference results, the end-to-end delay (\ie the delay of obtaining the inference results) is not affected by \name unless the resources are not enough for \name to process the input in real time.
    }
    \label{fig:workflow}
\end{figure}


\kt{A table here to show how the gradient-ascent-based approach works}

To optimize towards this goal, \name uses a standard \textbf{gradient-ascent strategy}.
% \mypara{Ideal way of picking new configuration}
At the end of each adaptation interval $t$, \name updates the $i^{\textrm{th}}$ knob $\Knob_{t,i}$ in the current configuration $\Config_{t}$ using the gradient of Equation~\ref{eq:objective}:

\vspace{-0.3cm}
\begin{@empty}
\footnotesize
\begin{align}
\Knob_{t+1,i}=\Knob_{t,i}+ \alpha \left(
\underbrace{
\frac{\Acc(\Config_t+\Delta \Knob_i) - \Acc(\Config_t)) }{\Delta \Knob_i}
}_{\text{\sf \footnotesize \textcolor{black!85}{gradient of accuracy (\textbf{\accgrad})}}}
- 
\lambda 
\underbrace{\frac{\Resource(\Config_t+\Delta \Knob_i) -\Resource(\Config_t)) }{\Delta \Knob_i}
}_{\text{\sf \footnotesize \textcolor{black!85}{gradient of resource usage}}}
\right),
\label{eq:ideal-adaptation}
\end{align}

\end{@empty}
where $\Knob_{t+1,i}$ is the configuration of the $i^{th}$ knob in the next adaptation interval, $\Delta\Knob_i$ is a small increase on the $i^{th}$ knob, $\alpha$ is the learning rate for gradient descent.
For now, we assume the configuration of each knob can be tuned continuously. 
Of course, this is a simplifying assumption. 
In \S\ref{subsec:limitation}, we will extend it to discrete configuration values and discuss the convergence of this gradient-ascent strategy.

% \footnote{We normalize the range of all knobs to [0,1] and use 0.5 as our learning rate.}: 
% increasing the learning rate $\alpha$ increases the convergence speed of \name, but \name may not converge to a near-optimal configuration if $\alpha$ is too large. We let $\alpha=0.5$ by default.

% We calculate $\frac{\Resource(\Knob_{cur,i} + \Delta\Knob_i) - \Resource(\Knob_{cur,i}) }{\Delta\Knob_i}$ by following its definition, which imposes extra overhead on \name (we will evaluate this overhead in \S\ref{??}) but does not require extra DNN inference.

The gradient-ascent strategy in Equation~\ref{eq:ideal-adaptation}
% \jc{why it's pointing to 3.2 not (2)? can we fix it?} 
requires calculating the gradient of accuracy (hereinafter \accgrad) and the gradient of resource usage along each knob $i$.
We calculate the gradient of resource usage by using the pre-profiled resource usage of each configuration $\Resource(\Config)$ (this aligns with prior work~\cite{chameleon,dds,reducto}), which might vary with different input data, but the relative difference among them has little variance.

However, if we calculate \accgrad by its definition, it would be prohibitively expensive (see Figure~\ref{subfig:gradient-before}). 
Obtaining $Acc(\Config)$ of any configuration $\Config$ will require running inference on the most resource-intensive configuration $\Config^*$.
Moreover, to get the \accgrad of each knob would require running an extra inference to test the impact of a small change in configuration on DNN output. 




\tightsubsection{Fast approximation of \accgrad}
\label{subsec:outputgrad}



\begin{figure*}[t]
    \centering
    \subfloat[][Calculating \outputgrad using its definition]
    {
        \includegraphics[width=1.6\columnwidth]{figs/gradient-before-new.pdf} 
        % {figs/gradient-before_haodong.jpg} 
        \label{subfig:gradient-before}
    }
    \\
    \subfloat[][Calculating \outputgrad using \name]
    {
        \includegraphics[width=1.6\columnwidth]{figs/gradient-after-new.pdf} 
        % {figs/gradient-after_haodong.jpg} 
        \label{subfig:gradient-after}
    }
    \tightcaption{Comparison between calculating \outputgrad naively and calculating \outputgrad using \name. \name calculates \outputgrad with \textit{no extra inference}. Image of the DNN credited to~\cite{dnnimagesource}.}
    \label{fig:gradient-contrast}
\end{figure*}

To estimate \accgrad efficiently, we introduce a new metric, called \outputgrad, to approximate it.
Here, we formally define \outputgrad and explain how to calculate it efficiently. 
The next subsection will elaborate on its statistical correlation with \accgrad.



\mypara{DNN \summary}
Recall from \S\ref{subsec:terminology} that the DNN output contains multiple {\em elements} each associated with a confidence {\em score}.
An element can be a detected object in object detection, a detected text in audio-text translation, or the classification of a pixel in semantic segmentation.
Since only elements with a score over confidence {\em threshold} will be counted towards accuracy, we define {\em \summary} of a DNN output by the number of elements in an adaptation interval whose confidence scores exceed the confidence threshold (see Equation~\ref{eq:outputgrad}).\footnote{This definition applies to all applications mentioned in Table~\ref{tab:applications}, but future work is needed to extend the definition to a wider range of DNN pipelines.}
We use $\Output(\Config_t)$ to denote the \summary 
% averaged number of elements with confidence over the threshold in the DNN output 
of DNN output $Res(\Config_t; \Data_t)$ under configuration $\Config_t$. 
% (see \S\ref{sec:definition-of-summary} for the formal definition).
% \jc{please avoid forward pointers to appendix for formal definitions. if the formal definition is important, it should be in the main text.}

\Summary offers a single-value summarization of the DNN output whose change indicates the change in inference accuracy. 
(More rationale of \summary will be given in \S\ref{subsec:outputgrad-properties}).


\mypara{\outputgrad definition}
With the definition of \summary, \outputgrad is how much a small change in the current value of each knob changes the \summary.
% (the number of DNN-returned elements in an adaptation interval with confidence scores over the confidence threshold).
% \kt{Illustrate how we make the \# of above-threshold confidence scores differentiable here.}
The \outputgrad of knob $\Knob_i$ can be written as

\vspace{-0.2cm}
\begin{@empty}
\footnotesize
\begin{equation*}
\frac{\Delta \Output}{\Delta k_i} = \frac{\Output{(\dots,\Knob_{t,i}+\Delta \Knob_i,\dots)}-\Output{(\dots,\Knob_{t,i},\dots)}}{(\Knob_{t,i}+\Delta \Knob_i) - \Delta \Knob_i}.
\end{equation*}
\end{@empty}

To help understand \outputgrad, we use a simple 
video analytics system that feeds each video frame to a DNN that performs vehicle detection with a confidence score of 0.5. 
Figure~\ref{subfig:gradient-before} illustrates \outputgrad in this example.
Following prior work~\cite{chameleon,vstore,videostorm,casva}, we assume the system can tune two configuration knobs, frame rate, and resolution.
Suppose that the current configuration is 10 frames per second (fps) and 480p.
% The analytic system will take a one-second-long, 20fps and 480p video and analyzes it through DNN.
When taking 1-second input, the DNN outputs 34 vehicle bounding boxes with confidence scores greater than 0.5 on these 10 frames, an average of 3.4 vehicles per frame.
% \footnote{Typical DNN output is more than a single value. Here, we assume that for a given video segment, the output of DNN inference is the average confidence of all detected objects. We will explain in \S\ref{??} how we turn the DNN output to a single value in general cases.} 
If we slightly increase the frame rate from 10fps to 15fps, the DNN outputs 66 vehicle bounding boxes with confidence scores greater than 0.5, on average 4.4 vehicles per frame.
Then the \outputgrad of the current frame rate is 

\vspace{-0.3cm}
\begin{@empty}
\footnotesize
\begin{align*}
\frac{\Delta \Output}{\Delta \text{framerate}}&=\frac{\Output{(480p,15fps)}-\Output{(480p,10fps)}}{15fps-10fps}=\frac{4.4-3.4}{15-10}=0.2.
% ,\\
% \frac{\Delta \Output}{\Delta \text{resolution}}&=\frac{\Output_{(720p,10fps)}-\Output_{(480p,10fps)}}{720p-480p}=0.01.
\end{align*}
\end{@empty}
% is (3.8-3.4)/(15-10)=0.08.
Following a similar procedure, we assume that the \outputgrad of the resolution will be:

\vspace{-0.3cm}
\begin{@empty}
\footnotesize
\begin{align*}
\frac{\Delta \Output}{\Delta \text{resolution}}&=\frac{\Output{(720p,10fps)}-\Output{(480p,10fps)}}{720p-480p}=\frac{5.8-3.4}{720-480}=0.01.
\end{align*}
\end{@empty}






% \begin{figure*}
%     \centering
%     \includegraphics[width=1.6\columnwidth]{figs/workflow.pdf} 
%     \tightcaption{Adapting configuration using \outputgrad. 
%     Note that as the adaptation process happens \textbf{after} obtaining the inference results, the end-to-end delay (\ie the delay of obtaining the inference results) is not affected by \name unless the resources are not enough for \name to process the input in real time.
%     }
%     \label{fig:workflow}
% \end{figure*}


% \tightsubsection{Using DNN differentiability to calculate \outputgrad}
% \label{subsec:differentiability-outputgrad}

% Recall that \name calculates \outputgrad on every adaptation interval.
% As a result, \outputgrad needs to be calculated with minimum overhead (in terms of GPU overhead, see \S\ref{sec:cost} for optimizations on other types of overhead).
% As shown in Figure~\ref{subfig:gradient-before}, a naive calculation of \outputgrad requires 
% through its definition results in high GPU overhead (
% $n$ extra DNN inferences for $n$ configuration knobs.

\mypara{How to calculate \outputgrad efficiently} 
The insight of \name is that \outputgrad can be computed efficiently \textit{with no extra DNN inference} by taking advantage of the {\bf differentiability of DNNs}. 
As our considered application pipelines use knobs to transform the raw input data to DNN's input (\eg frame filtering, image downscaling, etc), the computation of \outputgrad of a knob can be written as the multiplication of two separate gradients, each can be computed efficiently:
\begin{packedenumerate}
\item {\em \dnngrad:} How the DNN's output changes with respect to the DNN's input. 
% This can be obtained by a single backpropagation  on the DNN;
\item {\em \inputgrad:} How the DNN's input changes with respect to the knob's configuration. 
% This can be obtained without DNN operations on GPU.
\end{packedenumerate}
% \begin{packedenumerate}
%     \item {\em \dnngrad:} how the number of above-threshold confidence scores changes with different parts of DNN input (\Input).
%     \item {\em \inputgrad:} how much different parts of DNN input change with each knob value of the current configuration (\Config). %in relation to the change in the current configuration.
% \end{packedenumerate}
% Formally, we use $\Input(\Config; \Data)$ ($\Input(\Config)$ for short) to denote the DNN input of configuration $\Config$ at source data $\Data$ . 

Formally, the \outputgrad of $\Knob_i$ on \Data can be expressed by:
% \vspace{-0.3cm}
% \begin{align}
$$
{\color{black}\underbrace{\highlight{white}{$\frac{\displaystyle \Delta \Output}{\displaystyle \Delta \Knob_i}$}}_{\text{\sf \footnotesize \textcolor{black!85}{\outputgrad}}}}=
{\color{black}\underbrace{\highlight{white}{$\frac{\displaystyle \Delta \Output}{\displaystyle \Delta \Input(\Config)}$}}_{\text{\sf \footnotesize \textcolor{black!85}{\dnngrad}}}}\otimes
{\color{black}\underbrace{\highlight{white}{$\frac{\displaystyle \Delta \Input(\Config)}{\displaystyle \Delta \Knob_i}$}}_{\text{\sf \footnotesize \textcolor{black!85}{\inputgrad}}}},
$$
% \label{eq:grad-decouple}
% \vspace{-0.08cm}
% \end{align}
where $\otimes$ means inner product, and $\Input(\Config)$ denotes the DNN input of configuration $\Config$.

The decoupling makes the calculation of \outputgrad much more resource-efficient for three reasons:
\begin{packeditemize}
\item \dnngrad can be estimated by the DNN's derivation at input $\Input_\Config(\Data)$ via one backpropagation\footnote{
% \kt{Illustrate how we make the \# of above-threshold confidence scores differentiable here.}
To make $\Output$ differentiable, we define it to be $\sum_{e} Sigmoid(\alpha(Score_e-\beta))$ where $Score_e$ is the score of element $e$, $\beta$ is the confidence threshold (see \S\ref{subsec:eval-setup} for its exact value in each application), and $\alpha$ is a hyperparameter (by default, we use 20). Note that this function is almost identical to \summary when $\alpha$ is sufficiently large.
}.
This is a constant GPU-time operation without extra inference as it reuses the layer-wise features computed as part of the DNN inference of the current configuration.
\S\ref{sec:cost} will further reduce the compute overhead of backpropagation.

\item \dnngrad needs to be calculated once and re-used to derive \outputgrad of different knobs without extra DNN inference.
This is because the \dnngrad describes DNN's sensitivity to its input and thus remains largely similar if the change in DNN input is not dramatic.
For instance, the \dnngrad of an object-detection DNN is high on pixels associated with key visual features of an object.
% \jc{edit ends here}

\item Finally, computing \inputgrad does not involve any DNN inference, as it only runs the preprocessing part of the DNN analytics system multiple times.

\end{packeditemize}



% Additionally, 





% Therefore, computing \outputgrad for multiple configuration knobs only requires a one-time backpropagation on GPU and no extra DNN inference.

To reuse the same example from Figure~\ref{subfig:gradient-before}, Figure~\ref{subfig:gradient-after} shows how \outputgrad is calculated from \dnngrad and \inputgrad.
% We use $\Input_{\Config}(\Data)$ to denote the DNN input of configuration $\Config$ at input data $\Data$.
% The decoupling can be written as \outputgrad $\approx$ \inputgrad $\otimes$ \dnngrad, concretely,

\vspace{-0.3cm}
\begin{@empty}
\scriptsize
\begin{align*}
\frac{\Output_{(480p,15fps)}-\Output_{(480p,10fps)}}{15fps-10fps} &\approx \frac{\Input_{(480p,15fps)}-\Input_{(480p,10fps)}}{15fps-10fps} \otimes \frac{\Delta \Output}{\Delta \Input}\bigg|_{\Input=\Input_{(480p,10fps)}},\\
\frac{\Output_{(720p,10fps)}-\Output_{(480p,10fps)}}{720p-480p} &\approx \frac{\Input_{(720p,10fps)}-\Input_{(480p,10fps)}}{720p-480p} \otimes \frac{\Delta \Output}{\Delta \Input}\bigg|_{\Input=\Input_{(480p,10fps)}},
\end{align*}
\end{@empty}
where $\otimes$ represents inner product and $\frac{\Delta \Output}{\Delta \Input}|_{\Input=\Input_{(480p,10fps)}}$ is \dnngrad of the current configuration $(480p,10fps)$.
Figure~\ref{subfig:gradient-after} shows that \name saves extra GPU inference by decoupling \outputgrad and re-using the backpropagation results for different knobs.
This example has two knobs, thus the saving may seem marginal, but our evaluation shows more savings when \name is used to adapt more knobs together in more realistic DNN analytics systems (Figure~\ref{fig:fine-grained-knobs}). 

\begin{comment}
    

After showing the way \name calculates \outputgrad, we write the adaptation logic of \name in Algorithm~\ref{alg:adapt}.


\begin{algorithm}[ht]
\algrenewcommand{\algorithmiccomment}[1]{\hfill// #1}
\renewcommand{\algorithmicrequire}{\textbf{Input:}}
\renewcommand{\algorithmicensure}{\textbf{Output:}}
% \renewcommand\thealgorithm{}
\caption{\name adaptation logic at adaptation interval $t$}
\begin{algorithmic}[1]
    \Require{inference results $results$, configuration $(\Knob_{t,1},\cdots,\Knob_{t,n})$ at adaptation interval $t$, input data $\Data_t$, DNN input $input$}
    \Ensure{updated configuration $(\Knob_{t+1,1},\cdots,\Knob_{t+1,n})$}
    % \State{$input$ $\gets$ process($\Data_t$, $(\Knob_{t,1},\cdots,\Knob_{t,n})$)} \algorithmiccomment{input processing}
    % \State{$results$ $\gets$ DNN($input$)}  \algorithmiccomment{DNN inference}
    % \State{\color{red}\quad // ~ Delay of inference results only depends on previous 2 lines} 
    \State{$DNNGrad$ $\gets$ $\left|\frac{\partial \Output(results[-1])}{\partial input}\right|$}  \algorithmiccomment{backpropagation using the results on the last data frame, see \S\ref{subsec:saliency_sampling}.}
    \For{$i \gets 1$ to $n$}  \algorithmiccomment{$n$ is number of knobs}
        \State{$InputGrad_i$ = $\left|\frac{process(\Data_t, (\cdots, k_{t,i} + \Delta k_i, \cdots)) - input}{\Delta k_i}\right|$}
        \State{$ConfigGrad_i = DNNGrad \otimes InputGrad_i$}
        \State{$ResourceGrad_i = \frac{\Resource(\cdots, k_{t,i} + \Delta k_i, \cdots)-\Resource(\cdots, k_{t,i}, \cdots)}{\Delta k_i}$}
        \State{$k_{t+1,i} = k_{t,i} + \alpha 
        \left(
        ConfigGrad_i
         - \lambda~ ResourceGrad_i \right)$}
    \EndFor
    
\end{algorithmic}
\label{alg:adapt}
\end{algorithm}


\end{comment}

% \kt{\hl{Claim we are the first one who uses backprop for config adaptation here. I think it's better to mention saliency-based works  in related work rather than here.}}
We want to clarify that while \name is \textbf{the first} to leverage DNN differentiability for configuration adaptation, DNN differentiability has already been widely used in DNN training, DNN interpretability, and localization of areas most responsible for the DNN output~\cite{vision-saliency-1,vision-saliency-2}.
It should also be pointed out that \dnngrad differs from the traditional notion of ``saliency'' used in video compression~\cite{fischer2021saliency,hadizadeh2013saliency}, in that \dnngrad is derived directly from a particular DNN to capture how the input influences the DNN output. 

% Note that \name is the first system that leverages the differentiability of DNNs for configuration adaptation, though not the first one that leverages differentiability of DNNs in DNN serving system\footnote{For example, in computer vision community, people use backpropagation to localize which areas of the objects are responsible for the DNN output~\cite{vision-saliency-1,vision-saliency-2}.}. 
% We also aware that there is a recent trend in multi-media community that compress videos by estimating the saliency (\ie the regions in the input video that may contain objects) and encoding these regions in encoding quality.
% Also, there is a line of work from multi-media community~\cite{fischer2021saliency,chen2022context} that leverages saliency estimators to  estimates the areas in the DNN input that contain objects, and then enocde these areas in higher encoding quality so that the objects in these areas can be better detected.
% The notion of saliency may conceptually seems similar to \dnngrad (as both highlight the areas that are related to objects), 
% Also, conceptually \dnngrad is similar to saliency (the areas in the input video that may contain objects) in multi-media community that 

% However, these saliency estimato
% \kt{1. Backpropagation is used in model serving system for explanation.
% But we are the first one to use it for config adaptation
% 2. MM community use saliency to compress video.
% It may seems similar, but our saliency is aware of the final DNN and they are not (drawbacks).}
% \mypara{\dnngrad v.s. existing saliency estimators}
% \dnngrad captures the saliency of the DNN (defined as a map that quantifies the importance of different areas in the DNN input), where there are existing works that also serves the same purposes~\cite{accmpeg,dds,eaar,vigil,fischer2021saliency}.
% However, \dnngrad outperforms existing saliency map estimation algorithms.
% \begin{packeditemize}
%     \item Compared to generating saliency using cheap models~\cite{accmpeg,vigil,fischer2021saliency}, \dnngrad prioritizes those objects according to the likeliness of changing the number of objects detected (where cheap models may mark all objects~\cite{fischer2021saliency} as salient or wrongfully assign saliency to those objects that are detected with high confidence~\cite{accmpeg}).
%     \item One may also generate saliency based on region proposals (an intermediate result generated alongside DNN inference that includes regions potentially containing objects). Compared to this approach, \dnngrad can further rank the pixels inside each object, where this approach will mark all pixels inside an object as salient/non-salient.
% \end{packeditemize}

% \kt{Compare our saliency v.s. others saliency here}


% \mypara{Assumption to configuration knobs}





% First, 
% Second, \dnngrad further prioritizes the pixels inside and outside the object bounding boxes according to the likeliness of changing the number of objects detected, where 

% However, \name calculates this saliency using backpropagation instead of using cheap saliency estimators, allowing \name to derive a metric (\outputgrad) that directly correlates with inference accuracy.
% The cheap saliency estimators fail to correlate with inference accuracy in some cases.
% For example, one may use cheap neural network to estimate saliency~\cite{accmpeg,?,?}.
% However, these cheap saliency estimators will \kt{finish this.}






% Specifically, \name measures \outputgrad by how much a small change in the current value of each knob \textit{flips} the DNN-returned confidence scores from below (or above) the confidence threshold to above (or below). 
% It does not impose an extra burden on the applications to require them to expose confidence scores and confidence thresholds since most of the applications already expose confidence scores to indicate the uncertainty of DNN outputs and use confidence thresholds to filter out DNN outputs with low confidence. %those uncertain results returned from the DNN.
% Statistically, more changes in the ``near-confidence-threshold'' DNN outputs will likely cause more changes in the inference accuracy (as will be elaborated in \S\ref{subsec:correlation})\footnote{This correlation does \textit{not} assume that a confidence score always directly indicates the accuracy of its corresponding detection/classification results.}.
% % \outputgrad correlates with how much the accuracy \textit{changes} with knobs 
% Intuitively, this is because the confidence threshold determines whether a detection or classification result is accepted (as part of the accuracy calculation) or rejected (thus having no effect on the accuracy).




% \pagebreak


% We advocate that the adaptation system for DNN-based analytics should provide a new abstraction: \outputgrad, which estimates the gradient of DNN output with respect to individual knobs.
% We define \outputgrad on a designated knob as the change of the DNN-returned \textit{confidence scores} around (both below and above) the \textit{confidence threshold}, divided by the small amount of change of the knob.
% % when changing this knob by a little.
% This definition requires the application to expose the confidence scores inside their inference results and the confidence threshold used to filter the results.
% For most of the applications, the DNN-returned confidence scores and confidence threshold are naturally available, since most of the applications use confidence scores to quantify the uncertainty of the DNN inference results. The application then filters those results with low confidence scores (as these results may contain spurious results) through a confidence threshold.

% We found that \outputgrad nicely correlates with how much the inference accuracy changes with the knobs.
% Intuitively, this is because the confidence threshold determines whether a detection or a classification result is accepted (and thus participating in the accuracy calculation) or rejected (and thus having no effect on the accuracy).
% Thus, more changes of confidence scores near the confidence threshold will likely cause more changes on the inference accuracy.

% This gradient information can help us quickly adapt to the optimal configuration, 
% % among a large number of configurations 
% by assigning more resources to those knobs with high \outputgrad to improve the accuracy and cut the resource usage of those knobs with low \outputgrad to save resource usage (without hurting the accuracy).
% As shown in Figure~\ref{fig:compare}, \name quickly find the optimal configuration through \outputgrad, while the profiling-based approach needs to profile all configurations to obtain the optimal one, and the output-driven approach adapts slowly.




% \begin{figure*}[t]
%     \centering
%     \includegraphics[width=2.2\columnwidth]{figs/workflow.pdf}
%     \caption{Workflow of \name. \kt{$\Delta resolution$ $240p, 1fps$ }people won't immediately realize it's adding. Need some handholding, picking the new configuration}
%     \label{fig:workflow}
% \end{figure*}



% To quickly adapt to optimal configuration with no extra inference, \name calculates the \textit{gradient} of accuracy with respect to the knob (hereinafter \outputgrad).\jc{i suppose you will clean up all \accgrad and replace them with \outputgrad?}
% We define \accgrad as the accuracy change divided by the knob value change when changing the knob value by a little.

% With this gradient, \name can quickly adapt to the optimal configuration in a large configuration space by granting more resource to the knobs with high \accgrad to improve the accuracy, and cutting the resource usage of those knobs with low \accgrad to reduce the resource usage without hurting accuracy.

% \tightsubsection{Selecting the next configuration}
% \label{subsec:gradient-ascent}


% % \jc{(1) 3.2 and 3.3 are still a bit too abstract. please use a concrete example like the one in 31
% % (2) it’s not clear from 32 (upfront) why configgrad-based gradient ascent can adapt quickly. this should be upfront, not embedded or in the end
% % same thing with 33. it’s unclear why this is a smart design
% % (3) i dont see the assumptions in 31, 32, 33 be explicitly called out and justified.. did i miss them?}
% % \kt{I explicitly called out the assumptions in 31. I will deprioritize other issues before Sunday.}

% With \outputgrad, \name runs \textit{gradient ascent} to converge to a near-optimal configuration.
% In each adaptation interval, we perform inference using the current configuration $\Config_{cur}$ (\eg current resolution and frame rate), compute \outputgrad, and then use the following strategy to select a new configuration $\Config$ for the next adaptation interval.
% % the gradient of the objective function $Obj(k)$ with respect to the current configuration $\Config_{cur}$ and update the current configuration by running gradient ascent.

% % In each adaptation interval, we perform inference using the current configuration $\Config_{cur}$ (\eg current resolution and frame rate), obtain the gradient of the objective function $Obj(k)$ with respect to the current configuration $\Config_{cur}$ and update the current configuration by running gradient ascent.

% Formally, the goal of \name is to maximize a weighted sum between the accuracy $Acc$ (defined as the \textit{similarity} between the current inference results and the inference results generated under unlimited resource)\kt{need to defend this definition} and the resource usage $\Resource$:
% \begin{equation}
% \underbrace{Acc(\Config)}_{\text{\sf \footnotesize \textcolor{black!85}{accuracy}}}
% - \underbrace{\lambda \Resource(\Config)}_{{\text{\sf \footnotesize \textcolor{black!85}{resource usage}}}},
% \label{eq:objective}
% \end{equation}
% % where $\Config$ i \name maximizes this weighted sum by running gradient ascent (depicted in FIgure~\ref{fig:workflow}).
% where $\lambda$ is a hyperparameter that governs the tradeoff between accuracy and resource usage: higher $\lambda$ will emphasize resource-saving and lower $\lambda$ will emphasize accuracy improvement.
% We will vary $\lambda$ and examine its effect on \name in \S\ref{??}.



% \mypara{Ideal way of picking new configuration}
% Ideally, \name would update the $i^{th}$ knob $\Knob_{cur,i}$ in the current configuration $\Config_{cur}$ by:
% \begin{@empty}
% \footnotesize
% \begin{align*}
% \Knob_i^*=\Knob_{cur,i}+ \alpha \left(
% \underbrace{
% \frac{Acc(\Config_{cur} + \Delta\Knob_i) -Acc(\Config_{cur})) }{\Delta \Knob_i}
% }_{\text{\sf \footnotesize \textcolor{black!85}{gradient of accuracy}}}
% - 
% \lambda 
% \underbrace{\frac{\Resource(\Knob_{cur} + \Delta\Knob_i) - \Resource(\Knob_{cur}) }{\Delta\Knob_i}
% }_{\text{\sf \footnotesize \textcolor{black!85}{gradient of resource usage}}}
% \right),
% \end{align*}
% \end{@empty}
% where $\Knob_i^*$ is the updated value of the $i^{th}$ knob, $\Delta\Knob_i$ is a small increase on the $i^{th}$ knob, $\alpha$ is the learning rate for gradient descent (see \S\ref{??} for the concrete value we use): increasing the learning rate $\alpha$ increases the convergence speed of \name, but may miss the optimal value of the accuracy.

% % We calculate $\frac{\Resource(\Knob_{cur,i} + \Delta\Knob_i) - \Resource(\Knob_{cur,i}) }{\Delta\Knob_i}$ by following its definition, which imposes extra overhead on \name (we will evaluate this overhead in \S\ref{??}) but does not require extra DNN inference.

% We calculate the gradient of resource usage by using the pre-profiled resource usage of each configuration $\Resource(\Config)$ (this aligns with prior work~\cite{chameleon,dds,reducto}), which might vary with source data, but the relative difference among them has little variance.

% However, it is computationally expensive to calculate the gradient of accuracy $$
% \frac{ Acc(\Config_{cur} + \Delta\Knob_i) -Acc(\Config_{cur})) }{\Delta \Knob_i}$$
% as calculating the accuracy $Acc$ requires generating the inference results under unlimited resources (recall that we define accuracy as the similarity between this inference results and the current inference results).

% \name instead leverages \outputgrad to approximate the gradient of accuracy.
% The rationale behind this approximation is that \outputgrad correlates with the gradient of accuracy:
% if one knob is of large \outputgrad, increasing this knob will significantly change the DNN output $\Output$, and thus also significantly affects the accuracy $Acc$, leading to a large change of accuracy.
% We will further explain when and why \outputgrad can approximate the gradient of accuracy in \S\ref{??}.
% % On the contrary, if the \outputgrad of one knob is small, increasing this knob does not affect the DNN $\Output$, and thus the corresponding accuracy change is also marginal.


% \mypara{\name way of picking new configuration} As a result, \name picks the new configuration by
% \begin{@empty}
% \footnotesize
% \begin{align*}
% \Knob_i^*=\Knob_{cur,i}+ \alpha \left(
% \underbrace{
% \frac{\Output(\Config_{cur,i} + \Delta\Knob_i) -\Output(\Config_{cur,i}))}{\Delta \Knob_i}
% }_{\text{\sf \footnotesize \textcolor{black!85}{\outputgrad}}}
% - 
% \lambda 
% \underbrace{
% \frac{\Resource(\Knob_{cur,i} + \Delta\Knob_i) - \Resource(\Knob_{cur,i}) }{\Delta\Knob_i}
% }_{\text{\sf \footnotesize \textcolor{black!85}{gradient of resource usage}}}
% \right),
% \end{align*}
% \end{@empty}
% where $\Output$ is \summary  (\ie the number of above-threshold confidence scores).
% % note that we take the absolute value to \outputgrad, as we assume that increasing the knob values increases the resource usage (and thus increases the accuracy).



% % To further support the claim that \outputgrad correlates with the gradient of accuracy, we empirically 
% % We notice that the \textit{cosine similarity} between \outputgrad and AccGrad is higher than 0.95 (we provide a formal proof that AccGrad is equals to \outputgrad using an idealized accuracy function, see \S\ref{??}), so substituting it with the accuracy can still guide \name to the optimal configuration.

% % % To adapt configurations using \outputgrad, 
% % \name runs gradient ascent (depicted in Figure~\ref{fig:workflow}) to converge to a near-optimal configuration.
% % % First, we partition the input data stream (\eg video frames) into {\em adaptation intervals}, each of one second.
% % In each adaptation interval, we perform inference using the current configuration $\Config_{cur}$ (\eg current resolution and frame rate), compute \outputgrad, and then use the following strategy to select a new configuration $\Config$ based on \outputgrad. 

% % The goal of \name's gradient ascent is maximizing a weighted sum between \summary (number of elements with scores over the confidence threshold) and resource usage (we will discuss alternative formulations shortly):

% % \vspace{-0.4cm}
% % \begin{@empty}
% % \small
% % \begin{align}
% % {\color{black}\underbrace{\highlight{white}{$\Output_{\Config}(\Data)$}}_{\text{\sf \footnotesize \textcolor{black!85}{\summary}}}}-\lambda {\color{black}\underbrace{\highlight{white}{$\Resource(\Config)$}}_{\text{\sf \footnotesize \textcolor{black!85}{resource usage}}}} \label{eq:objective}
% % \end{align} 
% % \end{@empty} 
% % Here, $\Resource(\Config)$ is the resource usage (in either bandwidth or GPU cycles, defined per application) of \Config.
% % The hyperparameter $\lambda$ governs the tradeoff between accuracy and resource usage: higher $\lambda$ will emphasize resource-saving and lower $\lambda$ will emphasize accuracy improvement.
% % \hl{Note that we will vary $\lambda$ and study its impact in \S\ref{sec:eval}.}
% % % As shown in prior work, for most configuration knobs (\eg frame rate, resolution, etc), $Resource(\Config)$ can be accurately pre-profiled and does not vary with input content as much as inference results.

% % Given the current configuration $\Config_t$ at the interval $t$ and the \outputgrad $\Grad_t$ (a vector of each knob's \outputgrad), the new configuration used for the next interval $t+1$ should be the one that maximizes the improvement of the objective. 
% % Formally, we can express it by 

% % \vspace{-0.4cm}
% % \begin{@empty}
% % \small
% % \begin{align}
% % \Config_{t+1}=\textrm{argmax}_{\Config}{\color{black}\underbrace{\highlight{white}{$(\Config-\Config_t)\cdot \Grad_t$}}_{\text{\sf \footnotesize \textcolor{black!85}{change in \summary}}}}-\lambda {\color{black}\underbrace{\highlight{white}{$(\Resource(\Config)-\Resource(\Config_t))$}}_{\text{\sf \footnotesize \textcolor{black!85}{change in resource}}}} \label{eq:gradient}
% % \end{align}
% % \end{@empty}
% % % $\Config_{t+1}=\textrm{argmax}_{\Config} (\Config-\Config_t)\cdot Grad_t-\lambda (\Resource(\Config)-\Resource(\Config_t))$
% % The new configuration $\Config_{t+1}$ will be used for the next adaptation interval. 
% % Following prior work~\cite{chameleon,dds,reducto}, we pre-profile the resource usage of each configuration $\Resource(\Config)$, which might vary with source data, but the relative difference among them has little variance.

% In many applications, the objective in Eq.~\ref{eq:objective}, which linearly combines resource usage and \summary, is less reasonable than optimizing \summary with a fixed constraint on resource usage.
% For instance, one may choose to maximize \summary (which relates to accuracy as explained shortly), conditioned on the bandwidth usage of the configuration within a budget.
% Figure~\ref{fig:workflow} shows an example of how \name's gradient-based adaptation process works in the vehicle detection example.
% % We will still use the vehicle detection example, where a traffic camera streams its video data to a GPU-equipped server to determine which frame contains vehicles.
% In each adaptation interval, the sensor encodes the video in an adaptation interval using the current configuration (frame rate and resolution) and sends it to a DNN running on a GPU-equipped server.
% The server receives this video and runs DNN inference to get the inference results and runs backpropagation to get \dnngrad and send it back to the sensor. 
% While the server runs DNN inference, the sensor runs encoding multiple times with different to obtain \inputgrad (the change in DNN input with respect to each knob).
% Once the sensor receives \dnngrad, it uses Eq.~\ref{eq:grad-decouple} to calculate \outputgrad.
% It then runs the gradient ascent strategy in Eq.~\ref{eq:gradient} to adapt the configuration and uses the new configuration in the next interval. 
% \jc{kuntai, remember to justify why resource usage of a config can be known in advance? what about the frame-diff threshold in reducto?}

% the encoded video that the camera sent, decodes this video, and runs DNN inference to obtain the inference results.
% Then, the server calculates the saliency using the backpropagation and streams the saliency back to the camera.
% Finally, the camera receives the saliency, calculates \outputgrad, and adapts the configuration accordingly.
% \jc{kuntai, please update figure~\ref{fig:workflow} to include the gradient-based adaptation process.}

% 

\subsection{Relationship between \outputgrad and \accgrad}
\label{subsec:outputgrad-properties}



In theory, \outputgrad is different from \accgrad, but in practice, they are highly correlated. 
% Intuitively, \outputgrad captures how much the inference results change when adjusting the configuration by a little.
This can be intuitively explained as follows: a high \outputgrad means a great change in the inference output, which often causes a greater change in accuracy and thus a high \accgrad.
% As a significant change in the inference results (\ie large \outputgrad) is often accompanied by a substantial change in accuracy, the corresponding gradient of accuracy also tends to be large.

To formalize this intuition, we rigorously prove that they are statistically correlated under specific conditions. 
% \jc{Kuntai, the following paragraphs will be changed after you updated Appendix B}
\begin{packeditemize}
\item First, we assume the accuracy of DNN output is defined as counting the number of correctly-detected elements minus the number of wrongfully-detected elements.
As optimizing this accuracy function is equivalent to optimizing the precision (\ie the fraction of detected objects that are correctly detected), it is a good approximation of the F1 score (a metric that is widely used by prior work~\cite{dds,eaar,awstream,chameleon,accmpeg,casva,vstore,ekya,videostorm}) when the recall is high (\ie there is not many objects that should be detected but not).
\item Second, the accuracy of DNN output increases as the configuration of a knob changes towards using more resources (\eg higher resolution or selecting more frames). This observation aligns with prior work~\cite{awstream,chameleon,dds,eaar,accmpeg,vstore,videostorm,reducto,boggart}.
% The accuracy of all elements increases when we give the system more resources by increasing/decreasing the knob values (we assume increasing the knob value increases resource usage for simplicity).
% $\forall e \in Res(\Config),
% \frac{\partial (C(e) \cdot step(e.score-\theta))}{\partial \Config} > 0,$
% $\forall e \in Res(\Config)$, $\frac{\partial C(e)}{\partial \Config} = 0.$ 
\item 
Third, different elements do not overlap (\eg object bounding boxes do not mutually overlap, or the detected words in the audio do not overlap).
This assumption holds as a wide range of DNNs perform non-maximum suppression~\cite{nms,detectron2,seqnms} to remove overlapped elements in their inference results.
% $$\left| \frac{\sum_{e\in Res(\Config)} \partial step(e.score-\theta)}{\partial \Config} \right| =  \sum_{e\in Res(\Config)} \left|\frac{\partial step(e.score-\theta)}{\partial \Config} \right|,$$ where $|\cdot|$ means taking element-wise absolute value.
\end{packeditemize}
Formally, if these conditions hold, we can formally prove that $
\underbrace{\frac{\partial Acc(\Config)}{\partial \Config}}_{\text{\sf \footnotesize \textcolor{black!85}{\accgrad}}} = \bigg| \underbrace{\frac{\partial \Output(\Config)}{\partial \Config}}_{{\text{\sf \footnotesize \textcolor{black!85}{\outputgrad}}}}\bigg|
$.
The proof can be found in \S\ref{sec:proof}.

% \mypara{Theorem} using a simple accuracy function that counts the number of correctly-detected elements minus the number of wrongfully-detected elements, under the following assumptions:

% we have $
% \underbrace{\frac{\partial Acc(\Config)}{\partial \Config}}_{\text{\sf \footnotesize \textcolor{black!85}{\accgrad}}} = \bigg| \underbrace{\frac{\partial \Output(\Config)}{\partial \Config}}_{{\text{\sf \footnotesize \textcolor{black!85}{\outputgrad}}}}\bigg|
% $.

While there can be exceptions to these conditions, these conditions corroborate the observations in many previous studies.
For instance, higher encoding resolution leads to higher bandwidth usage and likely more accurate inference, or higher frame rate leads to higher GPU usage and likely more accurate inference~\cite{awstream,chameleon,dds,eaar,accmpeg,vstore,videostorm,reducto,boggart}.

% \jc{the theorem is way too long. how about you move the assumptions out from the theorem, and the theorem can simply say under xxx assumptions, we have xxx.}

% To further support this point, we provide a theorem that shows the correlation between \accgrad and \outputgrad.



% That said, a big change in the \summary may indicate either more increase or decrease in accuracy. 
% To decide the direction of change, we use the empirical observation that when a change in knob value increases the resource usage, the impact on inference accuracy should be positive (\eg higher encoding resolution leads to higher bandwidth usage and likely more accurate inference, or higher frame rate leads to higher GPU usage and likely more accurate inference). 




% gradient of accuracy is exactly \outputgrad under a special case of accuracy function (count the number of elements (\ie object detection bounding boxes) that are correctly detected) and two assumptions:
% \begin{packeditemize}
% \item If an element (\eg an object) is confidently detected (\ie with a confidence score above threshold), it will either be 
% \item There is only one object that the confidence score is around the confidence threshold (\eg the absolute difference between the confidence score and the threshold is smaller than 0.1).
% \end{packeditemize}




% Please see \S\ref{sec:proof} for the proof of this theorem. 

In \S\ref{sec:eval}, we also empirically verify that the change in output (\ie \outputgrad)) is proportional to the change in accuracy (\ie \accgrad).
Note that in the evaluation, we also tested a more complex accuracy definition (F1 score) as well as a range of configuration knobs (frame sampling rate, resolution, quantization parameter), both of which are widely used in~\cite{dds,eaar,chameleon,awstream,vstore,boggart,reducto}.
There are 125 configurations in total. 
% As real applications will use a different accuracy function (\eg F1 score~\cite{dds,eaar,chameleon,awstream,vstore,boggart,reducto}) compared to the proof above, we empirically verify whether the change in output (\ie \outputgrad)) is proportional to the change in accuracy (\ie \accgrad).
% We pick three configuration knobs (frame sampling rate, resolution, quantization parameter) that are widely used by prior work~\cite{chameleon,casva,awstream,videostorm,vstore,mcdnn} and a 6-second video chunk to verify the correlation between \outputgrad and \accgrad on all configurations (125 configurations in total).
Figure~\ref{fig:accuracy-proxy} shows that on one 9-second video chunk, the change of DNN output (X-axis) nicely correlates with the accuracy change (Y-axis), with a Pearson coefficient of 0.702.

% \kt{Plot this figure if we have time}
% \kt{no we don't}
% As our accuracy function varies between applications, we also empirically examine the correlation between \outputgrad and the gradient of accuracy.
% Concretely, on a 1-minute-long video, we partition this video to 60 one-second adaptation intervals, obtain \outputgrad and the gradient of accuracy on each interval, and then calculate the cosine similarity between them.
% We found that the cosine similarity is higher than \fillme\% for most of the cases.




\tightsubsection{Caveats and benefits}
\label{subsec:limitation}

While our evaluation shows \name's gradient-ascent strategy performs well for a wide range of DNN tasks, input data types, and configuration knobs, it is important to understand its limits and why it works in practice. 

% \kt{Let Yuhan run an experiment on this}
% \mypara{Why \name improves accuracy}
% Second, in the objective of gradient ascent (Eq.~\ref{eq:objective}), the change in the first term of \summary (\Output) should reflect the change in inference accuracy.
% This connection may be intuitively true since a significant change in the inference results is often accompanied by a substantial change in accuracy.
% That said, a big change in the \summary may indicate either more increase or decrease in accuracy. 
% To decide the direction of change, we use the empirical observation that when a change in knob value increases the resource usage, the impact on inference accuracy should be positive (\eg higher encoding resolution leads to higher bandwidth usage and likely more accurate inference, or higher frame rate leads to higher GPU usage and likely more accurate inference). 

% Figure~\ref{fig:accuracy-proxy} empirically verify whether the change in output ($\Delta \Output_\Config(\Data)$) is proportional to the change in accuracy (\ie the accuracy of the configuration $\Config$, minutes the accuracy of current configuration).
% We pick three configuration knobs (frame sampling rate, resolution, quantization parameter) that are widely used by prior work~\cite{chameleon,casva,awstream,videostorm,vstore,mcdnn} and a 6-second video chunk to verify the correlation between DNN output change and accuracy change on all configurations (125 configurations in total).
% Figure~\ref{fig:accuracy-proxy} shows that on one 9-second video chunk, the change of DNN output (X-axis) nicely correlates with the accuracy change (Y-axis), with a Pearson coefficient of 0.702.


\mypara{Why \name converges}
Like other gradient-based heuristics, it is difficult to guarantee that \name will always converge to a global optimum configuration. 
Nonetheless, \name does converge to a near-optimal configuration in most cases.
We empirically observe that \name converges to the optimal configuration within 3-5 intervals (seconds) as shown in Figure~\ref{fig:converge-fast} and within 1-2 intervals for configurations that require frequent adaptation (such as macroblock-level encoding quality).
% , \name may fail to converge when the input data content evolves so quickly that the best configuration last for less than a couple of seconds.
% the \outputgrad calculated from one adaptation interval does not apply to the next adaptation interval anymore.
Thus, as long as the best configuration last for at least a few seconds, \name can identify the best configuration faster than profiling-based methods.


The reason is that the relationship between configuration $\Config$ and their corresponding accuracy $\Acc(\Config)$ and the relationship between $\Config$ and resource usage $\Resource(\Config)$ are both roughly \textbf{concave}.
This concavity means that as configuration changes in the direction of using more resources, the improvement in accuracy will diminish as accuracy approaches 100\%.
% The concavity can be intuitively understood that as the configuration uses more (compute/network) resources, the change in the input to the DNN becomes more marginal, and so does the inference results and inference accuracy.
For example, as a video analytic system increases the video encoding resolution, the pixel change becomes more marginal (mostly on ``high-frequency'' details), causing the DNN output to stabilize (objects' confidence scores will change more slowly and less frequently cross the confidence threshold, leading to fewer newly detected objects) and leading to less improvement on accuracy~\cite{awstream,chameleon,vstore,videostorm,casva}.
A well-known consequence of such concavity is that gradient-ascent can eventually converge to a global optimal configuration~\cite{gradient-descent-convex,flaxman2004online}. 
% \kt{Maybe add some visualizations}



% That said, \name may fail to converge when the input data content evolves so quickly that 
% % Another potential reason for \name to fail to converge is the evolution of input data content---
% the \outputgrad calculated from one adaptation interval does not apply to the next adaptation interval anymore. % due to temporal change in the content. 
% Both profiling-based methods and \name require the continuity of resource/accuracy relationship at a timescale of several to 10s of seconds. 



% explain it with the example in fig 6. (need to update fig 6)
% caveats: 
% why not local optimum: concavity => connection with newton's method
% why leading to higher accuracy
% content change 

% limitation: not applicable to dnn knobs





% \mypara{\outputgrad correlates with accuracy}
% A key question is how \outputgrad is related to inference accuracy.
% We found that there is a statistical correlation between \outputgrad and the inference accuracy of other configurations. 
% This is because \outputgrad captures the change in the inference results, and a significant change in the inference results is often accompanied by a substantial change in accuracy.

% We found that \outputgrad statistically correlates with the inference accuracy.
% This is because \outputgrad captures the change in the inference results, where a large change in inference results likely corresponds to a large change in accuracy.

\begin{comment}
However, the change in the inference results cannot determine whether the accuracy improves or decreases.
To handle this issue, we make an assumption that for a designated knob $\Knob_i$, increasing it while keeping other knobs fixed will either statistically not decrease the accuracy (we denote this case as $sgn(i)=1$) or not increase the accuracy (we denote this case as $sgn(i)=-1$).
We found that this assumption holds for a wide range of knobs (see Table~\ref{tab:rich-set-of-knobs}), as increasing these knobs causes the resource usage pipeline increases/decreases and thus the corresponding accuracy also increases/decreases.
For example, increasing the frame rate while fixing the  resolution in the video analytics system typically leads to more accurate inference results as more frames are analyzed. 
Similarly, increasing the resolution while fixing the frame rate enhances the clarity of the boundaries of the object, and is likely to generate more accurate inference results.

% To give a concrete example, when tuning the frame rate and resolution of the aforementioned video analytic system, increasing the frame rate while fixing the resolution typically leads to more accurate results as more frames are being analyzed. 
% Similarly, increasing the resolution while fixing the frame rate also makes the detail of the video (like the boundary of the vehicles) clearer and thus is likely to generate more accurate inference results.

Using this assumption, we then derive the (signed) output change with respect to the current configuration (frame rate $\Knob_1=20fps$, resolution $\Knob_2=480p$) using the following formula:

\vspace{-0.3cm}
\begin{@empty}
\footnotesize
\begin{equation*}
\Delta \Output_\Config(\Data)= \sum_{i=1}^n \left|\frac{\Delta \Output}{\Delta \Knob_i}\right| \cdot sgn(i) \cdot (\Knob_i - \Knob_{i,cur}) =  0.08 \cdot (\Knob_i - 10\textrm{fps}) + 0.01 \cdot (\Knob_2 - 480\textrm{p}) 
\end{equation*}
\end{@empty}
% To examine the correlation between \outputgrad and the accuracy of other configurations, we calculate the change in accuracy with respect to the change of the current configuration ($O(res=2,fps=2)$) using the following formula
% \begin{@empty}
% \footnotesize
% \begin{equation*}
% \Delta O(res,fps) = \frac{\Delta O}{\Delta (res, fps)} \cdot \Delta (res, fps) = \frac{\Delta O}{\Delta res}(res-2) + \frac{\Delta O}{\Delta fps}(fps-2).
% \end{equation*}
% \end{@empty}
% And check if the output change is proportional to the accuracy change

  



And then, we verify whether the change in output ($\Delta \Output_\Config(\Data)$) is proportional to the change in accuracy (\ie the accuracy of the configuration $\Config$, minutes the accuracy of current configuration):
% \begin{@empty}
% \footnotesize
% \begin{equation*}
% \Delta \Output(\Input, \Config) \propto Acc(\Output(\Input, \Config)) - Acc(\Output(\Input, \Config_{cur})),
% \end{equation*}
% \end{@empty}
% where $Acc$ represents the inference accuracy.
We pick three configuration knobs (frame sampling rate, resolution, quantization parameter) that are widely used by prior work~\cite{chameleon,casva,awstream,videostorm,vstore,mcdnn} and a 6-second video chunk to verify the correlation between DNN output change and accuracy change on all configurations (125 configurations in total).
As shown in Figure~\ref{fig:accuracy-proxy}, on one 9-second video chunk, the change of DNN output (X-axis) nicely correlates with the accuracy change (Y-axis), with a Pearson coefficient of 0.702.


\end{comment}






% that maximally improves the change in DNN output $\Delta \Output(\Data,\Config)$ under the resource budget.
% As the change in DNN output statistically correlates with the change in accuracy, this will likely maximize the accuracy of the new configuration $\Config$.
% We then use this configuration for the next adaptation interval.
% identify a new configuration that maximally improves accuracy without exceeding the resource budget.
% We use this new configuration for the next adaptation interval, and at the end of the interval, we repeat the same adaptation steps.
% As the content of the input data is continuous, the new configuration is likely to generate more accurate inference results compared to the original configuration.
% Note that 
% As a result, the inference results of the new configuration are likely to be more accurate than the current configuration


\mypara{Why \name beats alternatives}
\name outperforms previous work on all three requirements (\ie adapt frequently, converge to a near-optimal configuration, and generalize to different types of knobs and analytic tasks).

First, compared to profiling-based work, \name adapts much more frequently (as \name updates its configuration \textit{at every second} but profiling-based work updates its configuration once every minute~\cite{awstream}) and earlier (as \name adapts to the change of input content right at the next second but the profiling-based work need to wait till the next profiling).

Second, compared to heuristics-based methods, \name's gradient ascent can converge to a {\em closer-to-optimal} configuration.
Most heuristics used in prior work adapt configuration by analyzing only the input data, rather than how the data might affect the final DNN's output and accuracy.
By contrast, \accgrad directly indicates DNN accuracy varies with a small change in the configuration. 
% compared to the heuristics-based approach, \name can adapt to a near-optimal configuration, where the accuracy of the heuristics-based approach can be much lower than the optimal configuration.

Third, we show that \name can generalize to 4 analytic tasks (vehicle detection, human detection segmentation, audio-to-text), 5 types of input data (\eg LiDAR videos, audio waves), and 5 types of knobs (\eg video codec knobs, frame filtering thresholds) in our evaluation (\S\ref{sec:eval}. 
That said, we have not tested if \name will work for applications (\eg text generation and image generation) and knobs (\eg knobs that alter the final DNN itself like DNN selection) beyond our evaluation.

% Third, \name can generalize to different applications and DNNs (as \name only assumes the DNNs to be differentiable, which holds for almost all DNNs) and a wide range of knobs (as \name applies to most of existing knobs, see Table~\ref{tab:rich-set-of-knobs}).

Further, the adaptation logic of \name does not increase the end-to-end delay (the delay of obtaining the inference results), as \name runs its logic after obtaining the inference results.


% \mypara{Why \name converges}
% First, like other gradient-based heuristics, \name does not guarantee to always converge to a global optimum configuration. 
% That said, we empirically observe that the relationship between configuration $\Config$ and their corresponding accuracy $\Acc(\Config)$ and resource usage $\Resource(\Config)$ is mostly \textbf{concave}.
% As a result of the concavity, gradient-ascent can eventually converge to a global optimal configuration. 
% The concavity can be intuitively understood that as the configuration uses more (compute/network) resources, the change in the input to the DNN becomes more marginal, and so does the DNN output.
% For example, as a video analytic system increases the video encoding resolution, the pixel change becomes more marginal (mostly on ``high-frequency'' details), causing the DNN output to stabilize (objects' confidence scores will change more slowly and less frequently cross the confidence threshold, leading to fewer newly detected objects).
% \kt{Maybe add some visualizations}
% \kt{This need a better proof}





% \tightsubsection{Limitations}
% \label{sec:limits}


% \mypara{Example applications that \name applies}

\mypara{Why picking future configuration based on current configuration}
As the \name updates the configuration based on the current interval, it is possible that the inference accuracy of the updated configuration on the next interval is much lower even if the updated configuration yields high accuracy on the current interval.
However, this scenario only happens when the content of the input data changes significantly (\eg when the vehicle stops in front of the red light) and thus does not happen frequently.



\mypara{Running gradient ascent over discrete configuration space}
Before running \name, we first linearly normalize all knob values to [0,1], where $0$ corresponds to the knob value with the least resource usage and 1 with the most resource usage.
We then calculate the updated knob value using Equation~\ref{eq:ideal-adaptation} and pick the closest value among all available knob values.



% \mypara{Why gradient ascent over discrete configuration space}
As gradient-based approach is mostly used on continuous space (\eg DNN parameters in DNN training), one may worry that gradient-based approach may fail on discrete configuration space.
We want to clarify that gradient-based approach can converge to a near-optimal configuration when the objective function (\ie the weighted sum between accuracy and resource usage) is concave~\cite{ramazanov2011stability,chistyakov2015stability}.



% \mypara{Limitation} 
% % We acknowledge that \outputgrad only works for configuration knobs that affect DNN input (\ie input preprocessing part of a DNN analytics system).


% \kt{Two potential limitations: 
% 1. \name is not ideal in scenario where the vast majority of adaptation intervals do not need to be analyzed.
% 2. \name does not apply to knobs that the optimal value frequently changes between adaptation interval (\eg adaptation interval=1frame, knob=whether to encode this frame or not).
% Not sure if we should include them.}

% Also, as \name requires DNN inference on every adaptation interval (in order to calculate \outputgrad for that interval), it is not ideal when most of the adaptation intervals do not need to be analyzed (\eg security camera footage at late night).







% \mypara{Overhead of backpropagation}

% However, this assumption makes \name not applicable to knobs that alter the DNN itself, such as retraining the DNN weights based on the current input~\cite{ekya,noscope,mcdnn}.
% In some sense, both the DNN customization approach and \name are adapting to the varying content in the input data stream.
% However, in order to maintain high accuracy, the DNN customization approach needs to retrain the DNN when the input content varies (which adds high GPU overhead).
% In contrast, \name adapts the knobs as part of the DNN-based inference process and only reuses the DNN inference result (for backpropagation), which is much more lightweight.


% \jc{need a paragraph to explain customization of specific applications, and why it still works under evolving content}
% overall, why it's better?

% Our gradient-ascent-based approach has its own caveats as it cannot guarantee that (i) the search will quickly converge in a few steps, and (ii) the search may get stuck in a local optimal.
% To answer this question, we measure how fast \name can converge to a near-optimal configuration (a top-1\% configuration).
% \kt{Not sure how to answer this question}





% The intuition behind the fast convergence is that as long as the \outputgrad with respect to one configuration knob is non-zero, tuning that knob will likely improve accuracy.
% % Further, as the input data is constantly changing over time, it is less likely for a local optimal to persist.
% Thus, \name is unlikely to be stuck in a local optimum, which corroborates our empirical observation of \name.
% \kt{Other potential concerns: (1) why treat discrete configs as almost continuous variables, (2) why the better configuration at this second will likely lead to a better result at the next second, (3) what if the content is noisy and makes the gradient noisy}



% However, directly calculating \outputgrad needs a substantial amount of extra inference.
% If we calculate \outputgrad knob-by-knob, we will need to calculate the accuracy change by changing one knob at a time.
% The amount of GPU compute will grow at least linearly with more knobs. 
% % This is because calculating \outputgrad in a knob-by-knob manner (\ie calculate the accuracy change by alternating the value of one knob while the value of other knobs remaining unchanged, and repeat this process for all knobs) results in extra inference (see \S\ref{subsec:calculate-accgrad} for details).
% % Moreover, more knobs will lead to more inference and reduces the applicability of \outputgrad on a large set of knobs.

% \mypara{Leveraging DNN differentiability} To reduce such overhead, \name harnesses the differentiability of the DNN to calculate \outputgrad with constant GPU overhead and with no extra inference.
% Intuitively, in order to calculate how DNN output changes with respect to the knob change (\ie \outputgrad), we can calculate how DNN output changes with respect to the DNN input change, and then study how DNN input changes with respect to the knob change.
% % how changing system knobs alters the DNN input, and then calculate how changing the DNN input alters the DNN output.
% Formally, we denote the configuration (\ie the values of all knobs) as $c$, the DNN input as $I$, and the DNN output as $O$. The intuition above can be written as the following chain rule:
% \begin{equation}
%     \frac{\partial O}{\partial c} = \frac{\partial O}{\partial I} \cdot \frac{\partial I}{\partial c},
% \end{equation}
% The first term $\frac{\partial O}{\partial I}$ can be obtained via backpropagation (a constant GPU overhead, but no extra inference is incurred as backpropagation reuses the computation graph created by existing DNN inference).
% The second term $\frac{\partial I}{\partial c}$ can be calculated in a knob-by-knob manner but since it only computes the DNN input (not DNN inference), it does not have extra GPU overhead. 
% without incurring DNN inference as calculating the DNN input change does not require DNN inference.

% The key enabler for \name to remove the extra inference is the following two observations to existing knobs for DNN-based analytic systems.



% that the knob only alters the DNN input. does not cover those knobs that alter the DNN itself, 




% \begin{enumerate}
%     \item \textit{Accuracy-Resource Property}: For a large class of knobs,  increasing the value of one knob always results in spending more (or less) resource, and also making the corresponding inference results more (or less accurate).
%     The amount of accuracy improvement (or degradation) depends on how much the knob increase alters the inference results.
%     \item \textit{Black-box Property}: Most of the knobs treat DNN as a black box and change the inference results solely by changing the DNN input.
% \end{enumerate}

% By leveraging the first assumption, \name estimates the accuracy change through inference results change, thus avoid calculating the inference results under the most expensive configuration as the ground truth.
% By leveraging the second assumption, \name decouples the gradient using chain rule and avoid the inference on the new configurations.


% Note that not all knobs satisfies the two properties above. We list some examples in Table \ref{??} and some non-examples down below.

% For \accres, we find that the sensing configuration knobs that directly change the raw sensed data, like the aperture and the ISO of the camera, the Gamma correction value of the camera, the positioning direction of the directional microphone, etc., do not satisfy \accres as varying these knobs typically have little impact on the encoded file size and the encoding cost of the input data.
% However, the sensing configuration knobs are typically pre-configured (like the positioning direction of the microphone) or self-adapted (like the aperture and the ISO of the camera) by the sensor.
% As a result, these knobs are typically not dynamically programmable so \name cannot change these knobs anyway.

% The non-examples for \blackbox are the knobs that optimize DNN inference, like DNN selection~\cite{chameleon} and DNN customization~\cite{noscope,ekya,mcdnn}.
% We acknowledge the effectiveness of these knobs in terms of saving GPU cost.
% However, we argue that these knobs requires the system to change or replace the DNN in real-time, which make them not generally applicable in all deployment settings (\eg when performing inference through third-party API).
% % However, switching or editing the DNN may result in significant overhead (\eg some other components may be customized for this DNN and may require retraining upon DNN changing~\cite{accmpeg}) or even not doable (\eg when performing inference through cloud API).




% \tightsubsection{Workflow of \name}














% We demonstrate the workflow of \name using the example of traffic cam-based vehicle detection
% Figure~\ref{fig:workflow} demonstrates the workflow of \name.
% \name assumes that the analytic systems are made up of two components: \textit{input processing} and \textit{DNN-based inference}.
% First, \name processes the data stream $x$ through input processing using the current configuration $c$ to obtain the DNN input $I$.
% \name then forwards $I$ through the DNN and obtain the DNN output $O$.
% After that, \name performs DNN backpropagation and obtains the gradient $\frac{\partial O}{\partial I}$.
% In the meantime, \name alters every knob in $c$ and obtains the corresponding change on the DNN input.
% \name then stacks together the DNN input changes of individual knobs ($\frac{\partial I}{\partial c}$) and 
% % \name then stacks these DNN input changes to obtain $\frac{\partial I}{\partial c}$ and 
% multiplies it with $\frac{\partial O}{\partial I}$ to obtain \outputgrad $\frac{\partial O}{\partial c}$.
% Finally, \name updates the configuration $c$ according to the \outputgrad.
% We will present the details of each step in the next section.









% \subsection{Accuracy gradient as a better feedback}

% \begin{itemize}
%     \item We find that: how much the analytic accuracy change differs if we change different knobs is essentially asking what is the \textit{gradient} of analytic accuracy with respect to the knob values.
%     \item With the accuracy gradient, we can better predict the analytic accuracy of those knob values we did not explore yet.
% \end{itemize}

% Our goal is to calculate the gradient of accuracy with respect to knobs (we call this gradient \textit{accuracy gradient}) by only evaluating the system under one configuration.

% Accuracy gradient enables us to better predict the accuracy of different configurations under similar video content.
% As a result, one can pick a chheaper configuration while still achieving the same accuracy with accuracy gradient.


% \begin{comment}

% \subsection{Programming interface of \name}


% \begin{figure}
%     \centering
%     \includegraphics[width=1\columnwidth]{figs/raw-input-inference.jpg}
%     \caption{\name handles those hyper-parameters that preprocess the input to the DNN.}
%     \label{fig:raw-input-inference}
% \end{figure}



% \subsection{API of HPs} 

% As shown in Figure~\ref{fig:raw-input-inference}, \name abstracts the underlying AI systems into two stages.
% In the preprocessing stage, the AI system pre-processes the raw sensing data to obtain the input to the DNN.
% In the inference stage, the DNN performs inference and obtain the analytic results.
% \name focuses on those HPs for preprocessing stage (we will show most of the HPs fall into this category in \S\ref{subsec:hp-examples}, together with some example HPs that do not belong to this category).
% As the preprocessing does not incur the compute-intensive server-side DNNs, we assume that this step can be locally done at the camera.

% Based on this observation, the programming interface of \name towards HPs are:
% \begin{small}
% \begin{verbatim}
% prep(Data raw, List hps)-> (Data input, Bytes encoded)
% proxy(Result result) -> Float pseudo_acc
% \end{verbatim}
% \end{small}

% The first function \texttt{prep} pre-processes the raw sensed data \texttt{raw} based on a list of HPs \texttt{hps}, and return the codec-encoded byte stream \texttt{encoded} and the input data \texttt{input} that server-side DNN will receive.

% The second function aims to provide a differentiable proxy towards accuracy (since most of the existing accuracy function is not differentiable).
% As most of the DNNs will return confidence scores to describe the confidence of the analytic results the DNN derives, we use the sum of the confidence scores as the default proxy.
% This complies with recent computer vision advances on evaluating the quality of inference results.

% Further, we empirically verify this assumption on different types of HPs and different videos.


% \subsection{Examples}
% \label{subsec:hp-examples}


% This assumption precludes those HPs that directly changes server-side DNN (\eg customizing the server-side DNN or switching between different server-side DNNs).
% That said, the vast majority of HPs, including HPs of traditioanal data encoding codecs (\eg frame rate, resolution, quantization parameters etc), DNN-based encoding codec (\eg feature compression, super resolution), fine-grained data quality assignments (\eg region-of-interest selection, macroblock encoding quality selection), sensor-side data filtering (\eg filtering the frames through cheap object detector or through cheap feature extractors) still fit in our assumption. 



% % \mypara{API of DNNs}
% % We require that the DNN to implement two APIs:
% % \begin{small}
% % \begin{verbatim}
% % inference(Data input)-> Result result
% % backprop(Result result, Function f)-> Data grad
% % \end{verbatim}
% % \end{small}



% \subsection{Workflow of \name}

% Contrast between conventional workflow and ours workflow

% \end{comment}







% \subsection{Workflow and API of \name}
% \kt{Goal: how to use the API in our system to calculate accuracy gradient}

% \begin{figure}
%     \includegraphics[width=1\columnwidth]{figs/workflow.jpg}
%     \caption{Workflow of \name \kt{Plot this figure in a "call stack" way, MAKE THE FONT LARGER}}
%     \label{fig:workflow}
% \end{figure}

% \mypara{Workflow of \name} Based on the approach above, we present the workflow of \name in Figure \ref{fig:workflow}.


% Our system enables the application to obtain the gradient of accuracy with respect to the knobs through the following API:
% $$AccGrad = calc(V_t, \{knob_i\}_{i=1}^n)$$

% \mypara{Towards knobs}

% $knob'_i = reduce(knob_i)$
% This reduce the knob to lower knob value

% \mypara{Towards DNN}
% We require the DNN to implement two APIs:
% \begin{packeditemize}
%     \item \texttt{result = inference(V)}
%     \item \texttt{saliency = backprop(result, grad)}
% \end{packeditemize}

% \mypara{Towards application}
% We require the application to implement:
% \begin{packeditemize}
%     \item \texttt{encode(V, knobs)} This one should be locally done on the camera
%     \item \texttt{proxy(results)}
% \end{packeditemize}


% \subsection{How to use the API}






% \subsection{Reduce the cost of accuracy gradient}


% \mypara{Accuracy gradient sampling}


% \mypara{Accuracy gradient compression}



==> plan.tex <==

% \newpage


% \begin{packedenumerate}


% \item Experiment

% \item Better implementation of \name
%      Plan: implement \name in Edge Video Services framework (Would be great if Zhengxu and Yitian can help)
%     If the implementation has some nontrivial things we can talk about, we can add an extra section on the implementation.


% \item More technical nuggets on system side of \name (\S 4)

% \begin{packedenumerate}
    
%     \item Backpropagation GPU compute ==> reuse gradient once every 10 frames + generate the gradient only for DNN input rather than DNN parameters (\S 4.1)
%      Backpropagation GPU memory ==> gradient checkpointing (\S 4.2), trade GPU computation for GPU memory
%     \item Bandwidth cost of streaming the gradient ==> downsampling the gradient (\S 4.3)
%     \item Encoding CPU cost ==> we only optimize for image input (encoding 1D media is not cost-demanding). Single-frame encoding for the spatial-only knobs, the results on temporal-only knobs (e.g. change frame rate) can be obtained based on the lossless data source. \kt{Prioritize}
% \end{packedenumerate}


% \item More detailed evaluation on the overhead of \name (\S 5)
%      Need several figures that focus on evaluating these overheads. 

% \item More on application-side properties (introduction)
%      Don't say these observation is new, say we use it to for example help convergence.
%      DNN differentiability \kt{Why differentiability: even in one knob, we can still compute much cheaper than extra inference.}
%      Configuration concavity ==> Need more experimental examples and more logics to help people understand in what case is configuration concave (\S 3.6).
%      \outputgrad correlates with \accgrad ==> Need more logic to help clarify when this correlation exists, will be the most tricky part. (\S 3.6)

% \item Question: what is the scope of application? \kt{1. What is the scope that we want to claim. 2. Why is that scope does not work 3. Propose a new scope that seems reasonable? 4. Evaluation experiments need to be added}
% \end{packedenumerate}

% \begin{packedenumerate}
% \item Writing

% \item Knob categorization
%      Uniform v.s. non-uniform
%      spatial v.s. temporal
%      Non-uniform : use threshold or not
%      Remaining: non-threshold-based frame selection ==> , threshold-based macroblock selection ==> no room of improvement \kt{Prioritize}

    
% \item More on related work (\S 6)
%      Need to illustrate why region-proposal-based logic does not work
%  Bayesian optimization
%          Bayesian optimization is typically used for continuous variables, and needs a way to make it work on discrete configuration knobs, but I guess this is a low priority. \kt{deprioritize}


% \item Use figures to substitute math in Section 3 to leave more space for system optimizations
% \item Refine the mathematical proof of why \accgrad is equal to \outputgrad 
%      Reviewers won’t read the appendix, so we need more intuition behind the mathematical proof (it is different from why the system is designed in the certain way)
%      \kt{Give a plan on how to do this}
% \item Change the scope of this paper to streaming media analytics
% \item Architecture of video analytic systems and API of OneAdapt

% \kt{1. Clarify the scope of applications, 4 data types (RGB, depth, LiDAR, audio), 3 tasks (classification, instance segmentation, object detection, keypoint, (semantic segmentation)), 4 types of knobs}
% \kt{Plan: start from RGB video object detection, enumerate each dimension (data type, tasks, type of knobs)}
% \kt{
% (streaming media analytics)
% (In section 3, for convenience, we use object detection for whole section 3, at the last subsection, extend it to other tasks)
% (data type)
% *RGB + detection + nonuniform spatial knob
% *LiDAR + detection + nonuniform spatial knob
% *depth + detection + nonuniform spatial knob 
% *InfraRed + detection + nonuniform spatial knob 
% *audio + detection + nonuniform spatial knob

% (task)
% *RGB + segmentation + nonuniform spatial knob
% RGB + classification + nonuniform spatial knob
% RGB + keypoint + nonuniform spatial knob

% (type of knobs)
% RGB + detection + uniform spatial knobs + uniform temporal knobs
% *RGB + detection + uniform spatial knobs
% *RGB + detection + nonuniform temporal knobs
% }
% \end{packedenumerate}


% \kt{Writing: write what is needed in paper to add change and to add figure 2. Knob categorization
% Experiment: 1. application scope, extra experiment. 2. CPU overhead 3. X-axis: overhead, Y-axis: accuracy gradient error.  (definition doesn't matter for paper writing's sake, cannot be too sensitive 1. figure good-looking, cost reduce a lot , cannot raise a lot 2. easy to explain)}





% \newpage





==> proof.tex <==

\mypara{Claim} Under the following assumptions:
\begin{packedenumerate}
\item $Acc(\Config) = \sum_{e\in Res(\Config)} C(e) \cdot step(e.score - \theta)$, where $e$ is an element in inference results $Res(\Config)$, $C(e)=1$ if $e$ is detected under the most expensive configuration, and $C(e)=-1$ if not, $step(x) = \sigma\left(10x\right)$, $\sigma$ is sigmoid function.
\item $
\forall e \in Res(\Config),
\frac{\partial (C(e) \cdot step(e.score-\theta))}{\partial \Config} > 0,
\frac{\partial C(e)}{\partial \Config} = 0.$ 
\item $\left| \frac{\sum_{e\in Res(\Config)} \partial step(e.score-\theta)}{\partial \Config} \right| =  \sum_{e\in Res(\Config)} \left|\frac{\partial step(e.score-\theta)}{\partial \Config} \right|$, where $|\cdot|$ means taking element-wise absolute value.
\end{packedenumerate}
we have
\begin{equation}
\frac{\partial Acc(\Config)}{\partial \Config} = \left|\frac{\partial \Output_\Config}{\partial \Config}\right|
\end{equation}

\mypara{Proof}
\begin{align*}
&\frac{\partial Acc(\Config)}{\partial \Config} \\
&= \frac{\partial \sum_{e\in Res(\Config)} C(e) \cdot step(e.score - \theta)}{\partial \Config} \\
&= \sum_{e\in Res(\Config)} \frac{\partial C(e) \cdot step(e.score - \theta)}{\partial \Config} \\
&=  \sum_{e\in Res(\Config)} \left|\frac{ \partial C(e) \cdot step(e.score - \theta)}{\partial \Config}\right| \\
&=  \sum_{e\in Res(\Config)} \left|C(e) \frac{ \partial step(e.score - \theta)}{\partial \Config}\right| \\
&=  \sum_{e\in Res(\Config)} |C(e)| \left| \frac{ \partial step(e.score - \theta)}{\partial \Config}\right| \\
&= \sum_{e\in Res(\Config)} \left| \frac{ \partial step(e.score - \theta)}{\partial \Config}\right| \\
&= \left|\partial \sum_{e\in Res(\Config)}  \frac{ step(e.score - \theta)}{\partial \Config}\right| \\
&= \left|\frac{\partial \Output_\Config}{\partial \Config}\right|.
\end{align*}

==> proof_new2.tex <==
\begin{figure}
    \centering
    \includegraphics[width=0.6\columnwidth]{figs/accgrad-outputgrad-cosine-similarity.pdf}
    \tightcaption{The CDF of the cosine similarity between \accgrad and \outputgrad across different configurations in pipeline~\circled{a} and videos in {\sf{Downtown}}. The average cosine similarity is over 0.91, indicating a strong correlation between \accgrad and \outputgrad.}
    \label{fig:accgrad-outputgrad-cosine-similarity}
\end{figure}



In this section, we prove the correlation between \accgrad and \name's estimation:

\mypara{Definitions}
For a given input, we let $Res(\Config)$ denote the output under a configuration $\Config$.
We define its accuracy as 
\begin{equation}
Acc(\Config) = \sum_{e\in Res(\Config)} f(e)C(e),
\label{eq:accuracy-definition}
\end{equation}
and the output utility as 
\begin{equation}
\Output(\Config) = \sum_{e \in Res(\Config)} f(e).
\label{eq:outputgrad}
\end{equation}
where $f(e)$ is a differentiable function that returns a value close to $1$ when $e$ is confidently detected (\ie the confidence score of $e$ is greater than the confidence threshold $\theta$) and close to $-1$, otherwise\footnote{Note that in our evaluation we use $f(e) = 2Sigmoid\left(20 (e.score-\theta)\right)-1$ (where $e.score$ is the confidence score of $e$ and $\theta$ is the confidence threshold), but the choice of $f$ does not affect the validity of our proof.
}, and $C(e)=1$ if $e$ is confidently detected under the most expensive configuration, and $C(e)=-1$ otherwise.

\mypara{Theorem}
For any knob $\Knob$ in configuration $\Config$, we have
$$
\underbrace{\frac{\Delta Acc(\Config)}{\Delta \Knob}}_{\text{\sf \footnotesize \textcolor{black!85}{\accgrad}}} \propto
\underbrace{\left|\frac{\partial \Output(\Config)}{\partial \Input}\right|}_{\text{\dnngrad}}
\otimes 
\underbrace{\left|\frac{\Delta \Input}{\Delta \Knob}\right|}_{\text{\inputgrad}}.
$$ 
across different knobs.


under the following assumptions:
%  (all these assumptions will be explained intuitively and validated empirically at the end of this section \jc{Kuntai, this will be TODO}):
\begin{packedenumerate}
\item 
For each $\Knob$ in the configuration $\Config$ and any element $e$ in $Res(\Config)$, we have:
% $$\frac{\partial f(e)C(e)}{\partial \Knob} \geq 0.$$
\begin{@empty}
\begin{equation}
\frac{\partial f(e)C(e)}{\partial \Knob} \geq 0.
\label{eq:acc-grad-property}
\end{equation}
\end{@empty}

\item Discrete chain rule: $\frac{\Delta f(e)}{\Delta k} \propto \frac{\partial f(e)}{\partial y} \otimes \frac{\Delta y}{\Delta k}$ across different knobs

\item The coordinates of object $e$ does not change with respect to configurations (\ie $\frac{\partial C(e)}{\partial k}=0$

\item 
For any element $e$ in $Res(\Config)$, there exists a binary matrix $M(e)$ s.t.
\begin{@empty}
\begin{equation}
M(e) \times \frac{\partial \Output(\Config)}{\partial \Input}=
M(e) \times \frac{ \partial  \sum_{e'\in Res(\Config)} f(e')}{\partial \Input} = \frac{\partial f(e)}{\partial \Input},
\label{eq:mask-property}
\end{equation}
\end{@empty}
where $\times$ means element-wise multiplication and $\Input$ refers to DNN input. 

\item 
Finally, we assume $\forall e$
\begin{@empty}
\begin{equation}
\left|
M(e) \times \frac{\partial \Output(\Config)}{\partial \Input}
\otimes 
\frac{\partial \Input}{\partial \Knob}
\right| = M(e) \times\left|
\frac{\partial \Output(\Config)}{\partial \Input}
\right|
\otimes
\left|
\frac{\partial \Input}{\partial \Knob}
\right|
\label{eq:non-negativity}
\end{equation}
\end{@empty}

\end{packedenumerate}


\mypara{Proof}


\begin{@empty}
\footnotesize
\begin{alignat*}{2}
&~~~~\frac{\Delta Acc(\Config)}{\Delta \Knob} \\
&= \frac{\Delta \sum_{e\in Res(k)}f(e)C(e)}{\Delta \Knob}
&\quad &\text{(definition of accuracy)}\\
&=\sum_{e\in Res(k)}\frac{\Delta f(e)C(e)}{\Delta \Knob}
&\quad &\text{(linearity of derivative)}\\    
&=\sum_{e\in Res(k)}\left|\frac{\Delta f(e)C(e)}{\Delta \Knob}\right|\
&\quad &\text{(equation~\ref{eq:acc-grad-property})}\\
&=\sum_{e\in Res(k)}\left|\frac{\Delta f(e)}{\Delta \Knob}\right|\
&\quad &(|C(e)|=1)\\
% &=\sum_{e\in Res(k)}\left|\frac{\partial f(e)}{\partial \Knob}\right|
% &\quad &\text{(equation~\ref{eq:acc-grad-property})}\\   
&=\sum_{e\in Res(k)}\left|\frac{\partial f(e)}{\partial \Input}\otimes \frac{\Delta \Input}{\Delta \Knob}\right|
&\quad &\text{assumption}\\   
% &=\sum_{e\in Res(k)}\left|M(e)\times \sum_{e'\in Res(\Config)}\frac{\partial f(e')}{\partial \Input}\otimes \frac{\partial \Input}{\partial \Knob}\right|
% &\quad &\text{(equation~\ref{eq:mask-property})}\\
% &=\sum_{e\in Res(k)}\left|M(e)\times \frac{\partial\sum_{e'\in Res(\Config)}  f(e')}{\partial \Input}\otimes \frac{\partial \Input}{\partial \Knob}\right|
% &\quad &\text{(linearity of derivative)}\\
&=\sum_{e\in Res(k)}\left|M(e)\times \frac{\partial \Output(\Config)}{\partial \Input}\otimes \frac{\Delta \Input}{\Delta \Knob}\right|
&\quad &\text{(equation~\ref{eq:mask-property})}\\
% &=\sum_{e\in Res(k)}M(e)\times \left|\frac{\partial \Output(\Config)}{\partial \Input}\otimes \frac{\Delta \Input}{\Delta \Knob}\right|
% &\quad &\text{($M(e) $is binary matrix)}\\
&=\sum_{e\in Res(k)}M(e)\times \left|\frac{\partial \Output(\Config)}{\partial \Input}\right|\otimes \left|\frac{\Delta \Input}{\Delta \Knob}\right|
&\quad &\text{(equation~\ref{eq:non-negativity})}\\
&=\left(\sum_{e\in Res(k)}M(e)\times \left|\frac{\partial \Output(\Config)}{\partial \Input}\right|
\right)
\otimes 
\left|\frac{\Delta \Input}{\Delta \Knob}\right|
&\quad &\text{(linearity of inner product)}\\
&=\left(
\left(\sum_{e\in Res(k)}M(e)\right)\times \left|\frac{\partial \Output(\Config)}{\partial \Input}\right|
\right)
\otimes 
\left|\frac{\Delta \Input}{\Delta \Knob}\right|
&\quad &\text{(distributivity)}\\
&=\left|\left(\sum_{e\in Res(k)}M(e)\right)\times \frac{\partial \Output(\Config)}{\partial \Input}\right|
\otimes 
\left|\frac{\Delta \Input}{\Delta \Knob}\right| 
&\quad &\text{($M(e)$ is non-negative)}\\
&=\left|\sum_{e\in Res(k)}M(e)\times \frac{\partial \Output(\Config)}{\partial \Input}\right|
\otimes 
\left|\frac{\Delta \Input}{\Delta \Knob}\right| 
&\quad &\text{(distributivity)}\\
&=\left|\sum_{e\in Res(k)}\frac{\partial f(e)}{\partial \Input}\right|
\otimes 
\left|\frac{\Delta \Input}{\Delta \Knob}\right|
&\quad &\text{(equation~\ref{eq:mask-property})}\\
&=\left|\frac{\partial \sum_{e\in Res(k)} f(e)}{\partial \Input}\right|
\otimes 
\left|\frac{\Delta \Input}{\Delta \Knob}\right|
&\quad &\text{(linearity of derivatives)}\\
&=\left|\frac{\partial \Output(\Config)}{\partial \Input}\right|
\otimes 
\left|\frac{\Delta \Input}{\Delta \Knob}\right|
&\quad &\text{(definition of \Output(\Config)}
\end{alignat*}
\end{@empty}



% This means that:
% \begin{@empty}
% \begin{equation}
% \frac{\partial f(e)C(e)}{\partial \Knob} = \left|\frac{\partial f(e)C(e)}{\partial \Knob}\right| = |C(e)|\left| \frac{\partial f(e)}{\partial \Knob}\right| = \left| \frac{\partial f(e)}{\partial \Knob}\right|.
% \label{eq:acc-grad-property}
% \end{equation}
% \end{@empty}

% \mypara{Justification of the assumptions}

% \jc{this part should intuitively explain each assumption and empirically validate that they hold in most cases}

% \jc{i copied and pasted the intuitive explanation of the assumptions here.}

% This assumption essentially means that for different elements, the nonzero values in $\frac{\partial f(e)}{\partial \Input}$ (which indicates the part of input data that corresponds to element $e$) do not overlap.


% This assumption means increasing the knob $\Knob$ makes the accuracy of element $e$ increase.

==> related.tex <==
%!TEX root = main.tex
%!TEX spellcheck = en_US 



\tightsection{Related work}
\label{sec:related}

\name bridges the gap between deep video analytics
and video streaming via a novel iterative refinement process.
Here, we discuss the most closely related work.

\mypara{Video object detection}
Vision research has a deep literature on object 
detection and tracking~\cite{yilmaz2006object,joshi2012survey}
and more recently deep learning-based approaches 
(e.g.,~\cite{ren2015faster}).
Recent works in computer vision have focused on
video object detection and have found it inefficient to apply 
object detection
frame by frame. In fact, the object detection tends to be slow to run 
at the real-time frame rate that is often augmented by tracking. The 
visual cues get weakened by defocus and motion blur
causing object detector to fail on corresponding frames.
Previous works have proposed ways to carry the temporal information
between key frames. In \cite{ImpressionNet}, 
only one keyframe is selected in each video segment for deep feature extraction
and the impression feature is
propagated down to the next keyframe.
In \cite{MobileVideoObjDet},
the authors generate feature maps with a joint convolutional
recurrent unit formed by combining a standard convolutional
layer with a convolutional LSTM. The recurrent layers
are able to propagate temporal cues across frames, allowing
the network to access a progressively greater quantity
of information as it processes the video. 
Finally, there are efforts towards scalable DNN architectures
and systems~\cite{sze2017efficient,zhang2017fast,zhang2017live}.
This work complements \name 
by designing new, server-side deep learning models. 
\name's distinctive advantage is explicitly optimizing
the bandwidth savings while maximizing the inference accuracy. 
%Additional efforts have also 
%focused on creating specialized models.
%These efforts 

\mypara{Active iterative refinement}
Iterative refinement over unlabeled data using active learning 
has shown promising gains
in several computer vision frameworks related to object 
classification~\cite{leroux2018iamnn}
and scene understanding~\cite{wang2018more}. The design goal is
recursive deep learning
models to predict the location and content of the 
region, and 
selectively choose a small subset of the regions to process in the 
next step. 
Recent variants of active learning~\cite{donmez2008proactive} 
take into account realistic constraints such as budget and
labeling errors.
Innovations in this space will complement the proposed pipeline.

\mypara{Internet video streaming} %Include how 
%H.265, scalable video coding and region of interest coding 
%do not suffice in terms of meeting video analytics requirements.
Recent innovations in video compression have provided better 
compression gains~\cite{h265}: 
the closest efforts are scalable video 
coding~\cite{ohm2005advances} and region-of-interest 
encoding~\cite{meddeb2016region}. 
However, the focus of these approaches is
content-agnostic.
Region-of-interest encoding requires
the viewer to specify the region of interest.  
Scalable video coding can utilize the bandwidth more efficiently
than traditional encoding methods, but its compression is still
performed at the pixel level. 
Similarly, the substantial literature on video streaming protocols---including adaptive bitrate streaming~\cite{seufert2015survey}---focuses on adapting bitrate of pre-coded video chunks/frames.
These approaches focus on user (\ie human) QoE, while 
\name streaming stack optimizes the inference accuracy for video analytics.
% addresses the scenario of a video
% transmission service with heterogeneous clients by encoding all 
% frames at multiple frame rates, spatial quality, and fidelity. 
% This coding approach focuses on the user QoE over all frames, while 
% \name streaming stack optimizes the inference accuracy for video analytics.



==> related_new.tex <==
%!TEX root = main.tex
%!TEX spellcheck = en_US 



\tightsection{Related work}
\label{sec:related}
\vspace{0.1cm}

% \name is an attempt to bridge distributed video analytics with limited network resources via a novel DNN-driven iterative video streaming protocol.
We discuss the most closely related work in three categories.


\mypara{Video analytics systems}
The need to scale video analytics has sparked much systems research: DNN sharing (\eg~\cite{mainstream,videoedge}), resource allocation (\eg~\cite{videostorm,starfish}), vision model cascades (\eg~\cite{noscope,fvc}), efficient execution frameworks (\eg~\cite{optasia,deeplens-sanjay,scanner}), as well as 
% Much of this work focuses on addressing challenges specific to one setting such as 
camera/edge/cloud collaboration (\eg~\cite{glimpse,vigil,nn-meets-pn,awstream,ddnn,cloudseg,eaar,dds-old}, see \S\ref{subsec:machine-centric} for a detailed discussion) or multi-camera collaboration (\eg~\cite{rexcam-hotmobile,chameleon}).
The most related work to \name is AWStream~\cite{awstream} which shares with \name the ethos of using a server DNN-generated profile. 
The key distinction is that such feedback is not real-time video content, so it cannot zoom in on specific regions on the current frames.
Vigil~\cite{vigil} sends cropped regions, but it is bottlenecked by the camera computing power (See \S\ref{subsec:machine-centric}).
% In \cite{dds-old}, the protocol can only {\em correct} those objects that are correctly detected but wrongfully labeled in low quality. Instead, \name is able to {\em detect} those objects that are completely missed in low quality.
\name shares the concept of server-driven streaming with its own preliminary design~\cite{dds-old} and the partially server-driven solutions~\cite{eaar,glimpse}.
But it is the first solution that achieves high accuracy (by correcting objects mislabeled {\em and} missed by the low-quality video or the camera-side model) in multiple vision tasks and DNN models, and fully utilizes the video streaming codec to minimize bandwidth usage. 
% these prior systems all rely on the video source to adapt to available bandwidth while \name is driven by both video content and the remote DNN inference task. 
% \jc{cite cloudseg, ``Cracking open the DNN black-box''}

\mypara{Vision applications}
Computer vision and deep learning have a substantial body of research (\eg~\cite{ren2015faster,DBLP:journals/pami/RenHG017,DBLP:conf/cvpr/RedmonDGF16,yilmaz2006object,joshi2012survey,DBLP:conf/cvpr/LiuWYLRS17,deng2018arcface}).
%, and more recently deep learning-based approaches (e.g.,~\cite{ren2015faster}).
Recent works on video object detection show it is inefficient to apply object detection DNN frame by frame; instead it should be augmented by tracking~\cite{ImpressionNet} (similar to \S\ref{subsec:optimization}) or by a temporal model such as LSTM~\cite{MobileVideoObjDet,tsm}.
% . In fact, the object detection DNN inference tends to be slower than real-time frame rate and is often augmented by tracking (just as in \S\ref{subsec:integration}). 
% The visual cues get weakened by defocus and motion blur causing object detector to fail on corresponding frames.
% Previous works have proposed to carry the temporal information between key frames. 
% In \cite{ImpressionNet}, only one keyframe is selected in each video segment for deep feature extraction and the impression feature is propagated down to the next keyframe.
% In \cite{MobileVideoObjDet}, the authors generate feature maps with a joint convolutional recurrent unit formed by combining a standard convolutional layer with a convolutional LSTM that
% propagates temporal cues across frames.
% , allowing the network to access a progressively greater quantity of information as it processes the video. 
% Finally, there are efforts towards scalable DNN architectures (\eg~\cite{sze2017efficient}).
This work complements \name by designing new, server-side deep learning models. 
\name's distinctive advantage is that it explicitly optimizes the bandwidth/accuracy tradeoffs in a way that is largely agnostic to the server-side DNN. 
%\jc{Aakanksha, please update the above paragraph if needed.}


\mypara{Internet video encoding/streaming}
Recent innovations in video encoding have provided better compression gains (\eg~\cite{h265}). 
The closest efforts to \name are scalable video coding~\cite{ohm2005advances} and region-of-interest (ROI) encoding~\cite{meddeb2016region}. 
However, these approaches optimize human-perceived quality.
Scalable video coding can utilize the bandwidth more efficiently than traditional encoding methods, but it still compresses video uniformly in its entirety. 
ROI encoding requires the viewer to specify the region of interest, and a recent proposal~\cite{eaar} uses the region-proposal network (RPN) to generate ROI regions.
% , but RPN results do not match 
Much work on adaptive bitrate streaming (\eg~\cite{seufert2015survey,festive,akamai-qoe,conviva-understanding}) has focused on adapting the bitrate of pre-coded video chunks to bandwidth fluctuation, but less on adapting encoding to the dynamic video content as \name does.
% These approaches focus on user (\ie human) QoE, while  \name streaming stack optimizes the inference accuracy for video analytics.

% \hh{Related work needs to cite earlier HotCloud paper, which was removed from lessons learned section to maintain anonymity.}

==> system.tex <==
%!TEX root = main.tex
%!TEX spellcheck = en_US 


\tightsection{\name interfaces}
\label{sec:interface}

%\hh{This section is very short.  Would it make sense to integrate it into the previous section as DDS programming interface?  We could also, then cut out the first two sentences.}

% We present \name's system design, focusing on its interface design and performance optimization.
%
%
%\subsection{Interfaces}
%
\name sits between the low-level functions (video codec and DNN inference) and the high-level applications (\eg object query or face recognition).
As illustrated in Figure~\ref{fig:apis}, it has ``south-bound'' APIs and ``north-bound'' APIs, both making minimum assumptions about the exact implementation of the low-level and high-level functions.


\mypara{South-bound APIs with codec}
\name only uses the APIs exposed by the standard MPEG video codecs. 
In particular, it implements two callback APIs.
The first, used in Stream A, is triggered once MPEG receives a segment $\Seg$ (a block of $n$ consecutive frames) from the video source (\eg camera hardware), and it will then retrieve from MPEG an encoded video with a quality level of $\Level_{\Low}$, \ie $\Video(\Seg, \Regions_{\Full},\Level_{\Low})$.
The second, used in Stream B, is triggered once the camera receives the feedback region set $\Regions_{\Feedback}$ from the server, and it will then retrieve the high-quality video, \ie $\Video(\Seg,\Regions_{\Feedback},\Level_{\High})$.
% Both APIs can be implemented using FFMpeg~\cite{ffmpeg}. 


\begin{figure}
\centering
\includegraphics[width=1.0\columnwidth]{figs/apis.pdf}
\tightcaption{\name sits between applications and DNN/video codec, and exposes north-bound and south-bound APIs.}
\label{fig:apis}
\end{figure}

\mypara{South-bound APIs with DNNs}
\name requires the server-side DNN to expose two APIs: 
(1) region proposals ($\Regions_{\Srv}$), each with a specified location; and 
(2) detection results ($\Detections_{\Srv}$) including the detected objects/identities each with a specified location and a detection confidence score.
The detection results API matches the output of most modern vision pipelines~\cite{google-tradeoff-benchmark}.
The region proposals can be readily obtained if the vision pipeline implements an RPN (\eg Faster/FastRCNN~\cite{DBLP:journals/pami/RenHG017}) that explicitly proposes regions.
Even when RPN is not used (\eg in Yolo~\cite{DBLP:conf/cvpr/RedmonDGF16}), it is common to run inference on grid-like candidate regions, and one can quantify an ``objectness'' score representing the likelihood it contains an object of any class. 
We evaluate \name's performance with different underlying DNNs in \S\ref{subsec:eval-indepth}.
% These APIs are available from a variety of DNNs pipelines.
% \jc{Xin, please give a few example of what these APIs are called in fastercnn, ssd, yolo, and face recognition pipelines}


\mypara{North-bound APIs}
\name implements the same analyst-facing (north-bound) APIs as the DNNs (\name can simply forward any function call to DNNs), so the high-level applications (\eg~\cite{optasia,deeplens-sanjay}) do not need to change and \name can be deployed transparently to analysts.
The only assumption is that, because \name runs the DNN twice on the same video segment, the two DNN detection results must be merged into a single detection result; we did this in a similar way as how DNNs internally to merge redundant results (\eg~\cite{tu2012fuzzy}).



\mypara{Camera-server interface}
Figure~\ref{fig:structure} shows the structure and the communication interface (highlighted in bold).
The function, \texttt{send\_to\_server}, which sends videos to server, can be implemented over existing protocols like HTTP.
It is useful to point out that Stream B can be equivalently implemented as a receiver-driven video streaming process, like DASH. 
The function \texttt{send\_feedback} can be seen as a request of a video segment sent to the video source (camera), and the camera, upon receiving the request, transcodes the original video (\eg encoding it in the high quality level and cropping out the feedback regions) and sends back the video.



\begin{figure}
\centering
\includegraphics[width=1.0\columnwidth]{figs/structure-client-server.pdf}
\tightcaption{\name interface between the camera and server, and how their communications (red arrows) fit in their workflows.}
\label{fig:structure}
\end{figure}


%\begin{itemize}
%	\item api w/ control algorithm
%	\item api between client \& server
%	\item explain with a diagram with two boxes of stream A and B
%\end{itemize}





%\mypara{Returning early results}
%One of the costs \name pays for the improved accuracy-bandwidth tradeoffs is the worst-case processing delay; the result of Stream B will wait for two ``round trips'' before it can be returned to the analysts.
%To address this problem, we observe that a large fraction of the DNN results on the low-quality video already has high confidence (though relying only on these results will cause lots of false negatives too).
%This allows \name to return these results in Stream A without waiting for Stream B, so majority of the results (\eg detected objects) can have an extremely low response delay.



%The new way of encoding Stream B videos can save bandwidth by up-to \fillme\%, and returning early results cuts the per-object response delay by \fillme\%.


%\begin{itemize}
%	\item leveraging codec
%	\item frame batching for real-timeness
%\end{itemize}
























==> todos.tex <==
\jc{
\begin{itemize}
\item add cloudseg in related work
\item add acknowledgement of no need for fancy hardware support on camera
\item explain that edge intelligent gpus are usually slower. it would cost a lot more to keep line speed
\item limitation section
\item how the parameters are chosen? 
\item cite "Cracking open the DNN black-box"
\item evaluate server-side cost in depth (the extra cost of two-pass cost)
\item sensitivity to the parameters (especially why gamma is set so low)
\item related work on roi encoding
\item Minor comments:
\begin{itemize}
    \item In Fig. 6, are the two DNNs used to process the low and high quality streams the same model?
    \item Sec 4.2: "by applying non-maximum suppression on the output of FasterRCNN..." => What does non-maximum suppression mean?
    \item Sec 4.3: It would be useful to specify the controller more formally, perhaps in the appendix.
\end{itemize}
\item crystallize the region proposal idea w.r.t vigil specifically
\item {\bf need to make a stronger case for saving (even just 2x) bandwidth. \url{https://www.verypossible.com/blog/wi-fi-vs-cellular-which-is-better-for-iot} and add more realistic comparison with awstream to show more improvement in accuracy or delay costs}
The use of region-proposals to get feedback is interesting but is just one of many design options in this space of video analytics. DDS trades-off reducing bandwidth while preserving accuracy and increasing server-side GPU usage. I am not convinced this is a great trade-off today since server-side GPU usage is significantly more expensive than bandwidth (just compare cost of GPU hours vs bandwidth on AWS, there is at least a 10X difference). Vigil and Glimpse are highly optimized for server-side GPU usage and DDS uses 10X more GPU resources (Figure 17) and 50\% more than Awstream; while DDS has better accuracy than Vigil and Glimpse, it has the same accuracy as Awstream. From a cost standpoint, one would likely choose Vigil/Glimpse and at high accuracy, one would choose Awstream -- there seems to be a narrow region where bandwidth is expensive/unavailable and one desires high accuracy, where perhaps DDS makes sense.
\item Figure 8: how does one get estimated bandwidth in a realistic application?
\item Section 5.2: "we empirically found that over 90\% of all final detected objects could have been detected in stream A" Why not go even lower resolution/scale then? Also, did you consider multiple rounds of feedback?
\item All evaluation results are reported using normalized accuracy. While that is useful to compare the schemes, what is the actual achieved accuracy values?
\item Section 7.2: What is the round trip delay between the camera and server? This can hurt DDS but not the other applications and is unspecified.
\item Figure 12 shows strictly no overlap between DDS and Awstream response delay values which seemed hard to believe -- Figure 19a shows that DDS can sometimes indeed result in higher response delay than Awstream and seems to be contradicting Figure 12!
\item Figure 15: is the gap in accuracy values relevant from an application point of view?
\item Section 7.4: the fact that you had to artificially reduce the available cellular bandwidth to show value of DDS seems to suggest that perhaps bandwidth is not a key metric to optimize? 
\item Why not use MaskRCNN, which is a better model in terms of accuracy, than FasterRCNN?
\item is an improvement of 2x good enough? 
\item comparison with NoScope
\end{itemize}
}
